A stable added-mass partitioned (AMP) algorithm for elastic solids and incompressible flow

A stable added-mass partitioned (AMP) algorithm is developed for fluid-structure interaction (FSI) problems involving viscous incompressible flow and compressible elastic solids. Deforming composite grids are used to effectively handle the evolving geometry and large deformations. The fluid is updated with an implicit-explicit (IMEX) fractional-step scheme whereby the velocity is advanced in one step, treating the viscous terms implicitly, and the pressure is computed in a second step. The AMP interface conditions for the fluid arise from the outgoing characteristic variables in the solid and are partitioned into a Robin (mixed) interface condition for the pressure, and interface conditions for the velocity. The latter conditions include an impedance-weighted average between fluid and solid velocities using a fluid impedance of a special form. A similar impedance-weighted average is used to define interface values for the solid. The new algorithm is verified for accuracy and stability on a number of useful benchmark problems including a radial-piston problem where exact solutions for radial and azimuthal motions are found and tested. Traveling wave exact solutions are also derived and numerically verified for a solid disk surrounded by an annulus of fluid. Fluid flow in a channel past a deformable solid annulus is computed and errors are estimated from a self-convergence grid refinement study. The AMP scheme is found to be stable and second-order accurate even for very difficult cases of very light solids.

==> tables/12_03_18/insElasticPiston.epgp.AmpSCF1NU0p05zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{8.0}{-3} &      & \num{1.4}{-3} &      & \num{8.9}{-4} &      & \num{1.4}{-3} &      & \num{6.4}{-3} &       \\ \hline
                epg2 &     2 & \num{1.8}{-3} &  4.5 & \num{3.5}{-4} &  4.0 & \num{2.1}{-4} &  4.3 & \num{3.5}{-4} &  4.0 & \num{1.5}{-3} &  4.4  \\ \hline
                epg4 &     4 & \num{4.3}{-4} &  4.2 & \num{8.9}{-5} &  3.9 & \num{5.0}{-5} &  4.1 & \num{8.9}{-5} &  3.9 & \num{3.5}{-4} &  4.1  \\ \hline
                epg8 &     8 & \num{1.1}{-4} &  4.1 & \num{2.3}{-5} &  3.9 & \num{1.2}{-5} &  4.1 & \num{2.3}{-5} &  3.9 & \num{8.8}{-5} &  4.0  \\ \hline
    rate             &       &  $2.08$       &      &  $1.98$       &      &  $2.05$       &      &  $1.98$       &      &  $2.06$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:34:11 2018}\label{table:insElasticPiston.epgp.AmpSCF1NU0p05zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.epgp.AmpSCF1e-3NU0p05zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{9.8}{-4} &      & \num{5.5}{-4} &      & \num{6.6}{-4} &      & \num{5.5}{-4} &      & \num{9.1}{-6} &       \\ \hline
                epg2 &     2 & \num{2.8}{-4} &  3.5 & \num{1.5}{-4} &  3.6 & \num{1.9}{-4} &  3.5 & \num{1.7}{-4} &  3.2 & \num{1.8}{-6} &  5.0  \\ \hline
                epg4 &     4 & \num{7.2}{-5} &  3.9 & \num{3.9}{-5} &  3.9 & \num{4.8}{-5} &  3.9 & \num{3.9}{-5} &  4.4 & \num{4.3}{-7} &  4.3  \\ \hline
                epg8 &     8 & \num{1.8}{-5} &  4.0 & \num{9.9}{-6} &  4.0 & \num{1.2}{-5} &  3.9 & \num{9.9}{-6} &  4.0 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $1.92$       &      &  $1.93$       &      &  $1.92$       &      &  $1.95$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1e-3NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:33:50 2018}\label{table:insElasticPiston.epgp.AmpSCF1e-3NU0p05zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.epgp.AmpSCF1e3NU0p05zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{2.9}{-2} &      & \num{4.1}{-3} &      & \num{8.8}{-4} &      & \num{4.1}{-3} &      & \num{6.7}{0} &       \\ \hline
                epg2 &     2 & \num{7.3}{-3} &  4.0 & \num{1.1}{-3} &  3.6 & \num{1.6}{-4} &  5.4 & \num{1.1}{-3} &  3.6 & \num{1.6}{0} &  4.2  \\ \hline
                epg4 &     4 & \num{1.7}{-3} &  4.3 & \num{3.0}{-4} &  3.8 & \num{3.2}{-5} &  5.1 & \num{3.0}{-4} &  3.8 & \num{3.7}{-1} &  4.4  \\ \hline
                epg8 &     8 & \num{4.0}{-4} &  4.2 & \num{7.7}{-5} &  3.9 & \num{6.9}{-6} &  4.7 & \num{7.7}{-5} &  3.9 & \num{8.4}{-2} &  4.4  \\ \hline
    rate             &       &  $2.07$       &      &  $1.91$       &      &  $2.33$       &      &  $1.91$       &      &  $2.11$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1e3NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:34:32 2018}\label{table:insElasticPiston.epgp.AmpSCF1e3NU0p05zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.epgp.shearAmpSCF1NU0p1zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.4}{-5} &      & \num{2.0}{-6} &      & \num{8.1}{-6} &      & \num{2.0}{-5} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{3.4}{-6} &  4.2 & \num{5.6}{-7} &  3.6 & \num{2.1}{-6} &  3.8 & \num{5.4}{-6} &  3.8  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{8.7}{-7} &  3.9 & \num{1.3}{-7} &  4.2 & \num{5.1}{-7} &  4.2 & \num{1.3}{-6} &  4.2  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{2.2}{-7} &  4.1 & \num{3.2}{-8} &  4.2 & \num{1.2}{-7} &  4.2 & \num{3.3}{-7} &  3.9  \\ \hline
    rate             &       &  $-nan$       &      &  $2.02$       &      &  $2.00$       &      &  $2.03$       &      &  $1.99$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:01:02 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1NU0p1zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.epgp.shearAmpSCF1e-3NU0p1zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{2.7}{-9} &      & \num{1.1}{-8} &      & \num{1.4}{-7} &      & \num{9.6}{-11} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{6.6}{-10} &  4.1 & \num{8.8}{-10} & 12.6 & \num{2.8}{-8} &  5.1 & \num{1.5}{-11} &  6.5  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{1.6}{-10} &  4.0 & \num{9.0}{-11} &  9.8 & \num{2.0}{-9} & 14.0 & \num{2.4}{-12} &  6.3  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{4.2}{-11} &  4.0 & \num{2.0}{-11} &  4.5 & \num{3.1}{-10} &  6.3 & \num{2.7}{-13} &  8.6  \\ \hline
    rate             &       &  $-nan$       &      &  $2.01$       &      &  $3.06$       &      &  $3.02$       &      &  $2.80$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e-3NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:00:39 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e-3NU0p1zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.epgp.shearAmpSCF1e3NU0p1zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.1}{-4} &      & \num{1.2}{-5} &      & \num{1.1}{-4} &      & \num{5.0}{-2} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{2.3}{-5} &  4.9 & \num{2.4}{-6} &  4.8 & \num{2.3}{-5} &  4.9 & \num{8.3}{-3} &  6.1  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{5.3}{-6} &  4.3 & \num{5.0}{-7} &  4.9 & \num{5.4}{-6} &  4.2 & \num{1.5}{-3} &  5.5  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{1.3}{-6} &  4.1 & \num{1.1}{-7} &  4.7 & \num{1.4}{-6} &  4.0 & \num{3.0}{-4} &  5.1  \\ \hline
    rate             &       &  $-nan$       &      &  $2.14$       &      &  $2.26$       &      &  $2.12$       &      &  $2.47$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e3NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:01:25 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e3NU0p1zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rep.AmpSCF1NU0p05zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{6.5}{-3} &      & \num{1.1}{-2} &      & \num{1.4}{-3} &      & \num{9.7}{-3} &      & \num{1.3}{-2} &       \\ \hline
                rep2 &     2 & \num{8.0}{-4} &  8.2 & \num{1.6}{-3} &  6.4 & \num{6.6}{-5} & 20.7 & \num{1.6}{-3} &  6.0 & \num{1.1}{-3} & 12.6  \\ \hline
                rep4 &     4 & \num{2.6}{-4} &  3.0 & \num{3.9}{-4} &  4.2 & \num{1.9}{-5} &  3.5 & \num{3.8}{-4} &  4.3 & \num{3.4}{-4} &  3.1  \\ \hline
                rep8 &     8 & \num{7.1}{-5} &  3.7 & \num{1.0}{-4} &  3.9 & \num{4.7}{-6} &  4.0 & \num{9.8}{-5} &  3.9 & \num{9.5}{-5} &  3.6  \\ \hline
    rate             &       &  $2.11$       &      &  $2.22$       &      &  $2.63$       &      &  $2.20$       &      &  $2.30$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:20:53 2018}\label{table:insElasticPiston.rep.AmpSCF1NU0p05zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rep.AmpSCF1e-3NU0p05zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.4}{-3} &      & \num{3.2}{-2} &      & \num{1.8}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  8.8 & \num{4.8}{-4} &  3.7 & \num{3.5}{-4} & 12.6 & \num{7.5}{-3} &  4.3 & \num{1.9}{-5} &  9.8  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.4}{-5} &  4.2 & \num{9.0}{-4} &  8.2 & \num{4.5}{-6} &  4.2  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  4.0 & \num{2.5}{-5} &  4.2 & \num{2.2}{-5} &  3.8 & \num{3.1}{-4} &  3.0 & \num{4.4}{-7} & 10.0  \\ \hline
    rate             &       &  $2.40$       &      &  $2.08$       &      &  $2.51$       &      &  $2.32$       &      &  $2.82$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:19:29 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3NU0p05zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rep.AmpSCF1e3NU0p05zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.3}{-2} &      & \num{1.3}{-2} &      & \num{4.6}{-4} &      & \num{5.9}{-3} &      & \num{5.4}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.5 & \num{1.3}{-3} &  9.9 & \num{1.1}{-4} &  4.0 & \num{1.4}{-3} &  4.3 & \num{1.5}{0} &  3.5  \\ \hline
                rep4 &     4 & \num{6.5}{-4} &  2.7 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.6}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{9.7}{-6} & 66.8 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.5 & \num{9.7}{-5} &  3.8 & \num{9.9}{-2} &  3.7  \\ \hline
    rate             &       &  $3.28$       &      &  $2.33$       &      &  $1.99$       &      &  $1.97$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:22:18 2018}\label{table:insElasticPiston.rep.AmpSCF1e3NU0p05zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rep.shearAmpSCF1NU0p1zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{10.0}{-7} &      & \num{5.7}{-6} &      & \num{1.9}{-6} &      & \num{1.2}{-5} &      & \num{1.4}{-5} &       \\ \hline
                rep2 &     2 & \num{1.6}{-7} &  6.1 & \num{1.7}{-6} &  3.3 & \num{3.7}{-7} &  5.1 & \num{4.5}{-6} &  2.6 & \num{2.2}{-6} &  6.1  \\ \hline
                rep4 &     4 & \num{3.3}{-8} &  5.0 & \num{4.0}{-7} &  4.2 & \num{8.8}{-8} &  4.3 & \num{1.1}{-6} &  4.2 & \num{4.5}{-7} &  5.0  \\ \hline
                rep8 &     8 & \num{4.0}{-9} &  8.1 & \num{9.6}{-8} &  4.2 & \num{2.0}{-8} &  4.3 & \num{2.6}{-7} &  4.2 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $2.61$       &      &  $1.97$       &      &  $2.17$       &      &  $1.86$       &      &  $2.31$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:07:40 2018}\label{table:insElasticPiston.rep.shearAmpSCF1NU0p1zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.5}{-6} &      & \num{1.3}{-5} &      & \num{1.4}{-3} &      & \num{4.3}{-3} &      & \num{1.1}{-5} &       \\ \hline
                rep2 &     2 & \num{1.5}{-7} & 10.5 & \num{2.2}{-6} &  6.1 & \num{4.1}{-4} &  3.3 & \num{1.4}{-3} &  3.2 & \num{3.0}{-6} &  3.7  \\ \hline
                rep4 &     4 & \num{1.5}{-8} &  9.5 & \num{5.4}{-7} &  4.0 & \num{1.0}{-4} &  4.0 & \num{3.2}{-4} &  4.3 & \num{7.0}{-7} &  4.3  \\ \hline
                rep8 &     8 & \num{2.0}{-9} &  7.8 & \num{1.5}{-7} &  3.6 & \num{2.6}{-5} &  3.9 & \num{8.0}{-5} &  4.0 & \num{1.7}{-7} &  4.0  \\ \hline
    rate             &       &  $3.21$       &      &  $2.14$       &      &  $1.91$       &      &  $1.94$       &      &  $2.01$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:02:02 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm1Imt0p6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.2}{-6} &      & \num{9.9}{-6} &      & \num{5.3}{-6} &      & \num{6.3}{-6} &      & \num{4.6}{-2} &       \\ \hline
                rep2 &     2 & \num{6.4}{-7} & 12.8 & \num{2.5}{-6} &  3.9 & \num{1.2}{-6} &  4.4 & \num{2.2}{-6} &  2.9 & \num{1.1}{-2} &  4.4  \\ \hline
                rep4 &     4 & \num{3.5}{-7} &  1.8 & \num{5.8}{-7} &  4.3 & \num{2.7}{-7} &  4.4 & \num{6.1}{-7} &  3.6 & \num{2.4}{-3} &  4.5  \\ \hline
                rep8 &     8 & \num{7.9}{-8} &  4.4 & \num{1.4}{-7} &  4.2 & \num{6.4}{-8} &  4.3 & \num{1.7}{-7} &  3.6 & \num{5.5}{-4} &  4.3  \\ \hline
    rate             &       &  $2.10$       &      &  $2.07$       &      &  $2.12$       &      &  $1.74$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sun Dec  2 23:13:30 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm1Imt0p6}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.2}{-8} &      & \num{2.3}{-8} &      & \num{6.3}{-9} &      & \num{2.4}{-8} &      & \num{6.2}{-8} &       \\ \hline
                rtw4 &     2 & \num{2.9}{-8} &  1.1 & \num{6.9}{-9} &  3.3 & \num{2.7}{-9} &  2.3 & \num{7.7}{-9} &  3.1 & \num{3.1}{-8} &  2.0  \\ \hline
                rtw8 &     4 & \num{1.2}{-8} &  2.4 & \num{2.4}{-9} &  2.9 & \num{1.1}{-9} &  2.5 & \num{2.9}{-9} &  2.6 & \num{1.6}{-8} &  1.9  \\ \hline
               rtw16 &     8 & \num{4.7}{-9} &  2.6 & \num{1.2}{-9} &  2.0 & \num{4.2}{-10} &  2.5 & \num{1.2}{-9} &  2.4 & \num{6.1}{-9} &  2.7  \\ \hline
    rate             &       &  $0.96$       &      &  $1.42$       &      &  $1.30$       &      &  $1.42$       &      &  $1.10$       &       \\ \hline
\end{tabular}
\caption{{\color{red}MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-7 Mon Dec  3 00:13:48 2018}}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3}
\end{center}
\end{table}
}

==> tables/12_03_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{5.6}{-8} &      & \num{3.1}{-8} &      & \num{4.3}{-8} &      & \num{3.4}{-7} &      & \num{4.5}{-8} &       \\ \hline
                rtw4 &     2 & \num{8.8}{-9} &  6.4 & \num{9.3}{-9} &  3.4 & \num{6.0}{-9} &  7.1 & \num{6.8}{-8} &  5.0 & \num{8.5}{-9} &  5.3  \\ \hline
                rtw8 &     4 & \num{2.0}{-9} &  4.4 & \num{2.5}{-9} &  3.8 & \num{1.3}{-9} &  4.6 & \num{1.6}{-8} &  4.2 & \num{2.3}{-9} &  3.6  \\ \hline
               rtw16 &     8 & \num{4.9}{-10} &  4.1 & \num{7.0}{-10} &  3.6 & \num{3.0}{-10} &  4.3 & \num{4.0}{-9} &  4.1 & \num{5.7}{-10} &  4.1  \\ \hline
    rate             &       &  $2.26$       &      &  $1.84$       &      &  $2.36$       &      &  $2.13$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=7 -amp=1e-7 Sun Dec  2 23:35:06 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3}
\end{center}
\end{table}


==> tables/12_03_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.1}{-8} &      & \num{1.3}{-8} &      & \num{9.2}{-10} &      & \num{6.1}{-9} &      & \num{8.8}{-8} &       \\ \hline
                rtw4 &     2 & \num{2.3}{-3} &  0.0 & \num{1.9}{-3} &  0.0 & \num{4.8}{-6} &  0.0 & \num{1.9}{-3} &  0.0 & \num{3.3}{-3} &  0.0  \\ \hline
                rtw8 &     4 & \num{3.2}{-3} &  0.7 & \num{8.0}{-4} &  2.4 & \num{7.3}{-7} &  6.5 & \num{8.0}{-4} &  2.4 & \num{9.7}{-4} &  3.4  \\ \hline
               rtw16 &     8 & \num{1.9}{-8} & 1.68e+05 & \num{1.6}{-9} & 4.94e+05 & \num{2.9}{-10} &2540.1 & \num{1.4}{-9} & 5.49e+05 & \num{4.5}{-8} & 2.17e+04  \\ \hline
    rate             &       &  $0.16$       &      &  $1.04$       &      &  $0.78$       &      &  $0.75$       &      &  $0.47$       &       \\ \hline
\end{tabular}
\caption{{\color{red}MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=8 -amp=1e-7 Mon Dec  3 00:52:12 2018}}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3}
\end{center}
\end{table}


==> tables/12_04_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.4}{-8} &      & \num{2.4}{-8} &      & \num{6.4}{-9} &      & \num{2.4}{-8} &      & \num{6.2}{-8} &       \\ \hline
                rtw4 &     2 & \num{3.5}{-8} &  1.0 & \num{8.9}{-9} &  2.6 & \num{3.4}{-9} &  1.9 & \num{9.5}{-9} &  2.5 & \num{4.0}{-8} &  1.6  \\ \hline
                rtw8 &     4 & \num{1.9}{-8} &  1.8 & \num{4.4}{-9} &  2.0 & \num{1.7}{-9} &  2.0 & \num{4.8}{-9} &  2.0 & \num{2.5}{-8} &  1.5  \\ \hline
               rtw16 &     8 & \num{8.4}{-9} &  2.3 & \num{2.3}{-9} &  1.9 & \num{7.6}{-10} &  2.2 & \num{2.3}{-9} &  2.1 & \num{1.1}{-8} &  2.3  \\ \hline
    rate             &       &  $0.69$       &      &  $1.11$       &      &  $1.02$       &      &  $1.11$       &      &  $0.82$       &       \\ \hline
\end{tabular}
\caption{\color{red}MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-7 Mon Dec  3 23:49:22 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3}
\end{center}
\end{table}


==> tables/12_04_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{5.7}{-8} &      & \num{3.7}{-8} &      & \num{4.3}{-8} &      & \num{3.4}{-7} &      & \num{4.3}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.1}{-8} &  5.3 & \num{1.2}{-8} &  3.0 & \num{6.3}{-9} &  6.8 & \num{6.9}{-8} &  4.9 & \num{9.1}{-9} &  4.8  \\ \hline
                rtw8 &     4 & \num{7.3}{-9} &  1.5 & \num{4.6}{-9} &  2.7 & \num{1.5}{-9} &  4.2 & \num{1.7}{-8} &  4.0 & \num{3.3}{-9} &  2.7  \\ \hline
               rtw16 &     8 & \num{2.8}{-9} &  2.6 & \num{2.2}{-9} &  2.1 & \num{4.2}{-10} &  3.5 & \num{4.2}{-9} &  4.0 & \num{10.0}{-10} &  3.3  \\ \hline
    rate             &       &  $1.36$       &      &  $1.36$       &      &  $2.21$       &      &  $2.10$       &      &  $1.78$       &       \\ \hline
\end{tabular}
\caption{{\color{red}MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=7 -amp=1e-7 Mon Dec  3 23:06:30 2018}}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3}
\end{center}
\end{table}


==> tables/12_04_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.1}{-8} &      & \num{1.3}{-8} &      & \num{9.2}{-10} &      & \num{6.1}{-9} &      & \num{8.8}{-8} &       \\ \hline
                rtw4 &     2 & \num{2.3}{-3} &  0.0 & \num{1.9}{-3} &  0.0 & \num{4.8}{-6} &  0.0 & \num{1.9}{-3} &  0.0 & \num{3.3}{-3} &  0.0  \\ \hline
                rtw8 &     4 & \num{3.2}{-3} &  0.7 & \num{8.0}{-4} &  2.4 & \num{7.3}{-7} &  6.5 & \num{8.0}{-4} &  2.4 & \num{9.7}{-4} &  3.4  \\ \hline
               rtw16 &     8 & \num{1.9}{-8} & 1.68e+05 & \num{1.6}{-9} & 4.94e+05 & \num{2.9}{-10} &2540.1 & \num{1.4}{-9} & 5.49e+05 & \num{4.5}{-8} & 2.17e+04  \\ \hline
    rate             &       &  $0.16$       &      &  $1.04$       &      &  $0.78$       &      &  $0.75$       &      &  $0.47$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=8 -amp=1e-7 Mon Dec  3 00:52:12 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3}
\end{center}
\end{table}


==> tables/ElasticPiston2DConvergence.tex <==
\begin{table}[H]
\caption{\label{fig:ElasticPiston2DConvergence}Convergence for 2D elastic piston.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.9e-03 &  & 3.3e-03 &  & 8.6e-07 &  & 2.7e-05 &  & 5.3e-05 & \\
1/40 & 5.0e-04 &  3.8 & 7.8e-04 &  4.2 & 2.5e-07 &  3.4 & 7.8e-06 &  3.5 & 1.4e-05 &  3.8\\
1/80 & 1.3e-04 &  3.8 & 2.2e-04 &  3.5 & 6.9e-08 &  3.6 & 2.2e-06 &  3.5 & 3.7e-06 &  3.8\\
1/160 & 3.5e-05 &  3.7 & 6.0e-05 &  3.7 & 1.9e-08 &  3.6 & 6.4e-07 &  3.4 & 1.0e-06 &  3.7\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/ElasticPistonConvergence.tex <==
\begin{table}[H]
\caption{\label{fig:ElasticPistonConvergence}Elastic piston convergence tables for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be 
$\bar{H} = \frac{1}{2},\, H = 1,\, \bar{\mu} = 10,$ and $\mu = .02.$}
\begin{center}
\begin{tabular}{c}
\das{Placeholder for heavy solid} $\rhos/\rho = 10^3$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\\
\end{tabular}

\begin{tabular}{c}
\das{Placeholder for medium solid} $\rhos/\rho = 1$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\\
\end{tabular}

% \caption{\label{fig:ElasticPistonConvergence}Convergence for elastic piston.\das{Placeholder for light solid $\rhos/\rho = 10^{-3}.$}}
\begin{tabular}{c}
\das{Placeholder for light solid} $\rhos/\rho = 10^{-3}$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}




% \begin{table}[H]
% \caption{\label{fig:ElasticPistonConvergenceHeavy}\das{Placeholder for heavy solid $\rhos/\rho = 10^3.$}}
% \begin{center}
% \begin{tabular}{ccccccccccc}
% \hline
% $h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
% \hline
% 1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
% 1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
% 1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
% 1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[H]
% \caption{\label{fig:ElasticPistonConvergenceMedium}Convergence for elastic piston.$\bar{H} = \frac{1}{2},\, H = 1,\, \rho = 1,\, \bar{\rho} = 1,\, \bar{\mu} = 10,\,
% \mu = .02.$ \das{Placeholder for medium solid $\rhos/\rho = 1.$} }
% \begin{center}
% \begin{tabular}{ccccccccccc}
% \hline
% $h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
% \hline
% 1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
% 1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
% 1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
% 1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}

% \begin{table}[H]
% \caption{\label{fig:ElasticPistonConvergence}Convergence for elastic piston.\das{Placeholder for light solid $\rhos/\rho = 10^{-3}.$}}
% \begin{center}
% \begin{tabular}{ccccccccccc}
% \hline
% $h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
% \hline
% 1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
% 1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
% 1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
% 1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}


==> tables/RadialElasticPistonConvergence.tex <==
\begin{table}[H]
\caption{\label{fig:RadialElasticPistonConvergence} Radial elastic piston convergence tables 
for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be \das{??}}
\begin{center}
\begin{tabular}{c}
\das{Placeholder for heavy solid} $\rhos/\rho = 10^3$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\\
\end{tabular}

\begin{tabular}{c}
\das{Placeholder for medium solid} $\rhos/\rho = 1$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\\
\end{tabular}

% \caption{\label{fig:ElasticPistonConvergence}Convergence for elastic piston.\das{Placeholder for light solid $\rhos/\rho = 10^{-3}.$}}
\begin{tabular}{c}
\das{Placeholder for light solid} $\rhos/\rho = 10^{-3}$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}






==> tables/RadialShearPistonConvergence.tex <==
\begin{table}[H]
\caption{\label{fig:RadialShearPistonConvergence} Radial shear piston convergence tables 
for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be \das{??}}
\begin{center}
\begin{tabular}{c}
\das{Placeholder for heavy solid} $\rhos/\rho = 10^3$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\\
\end{tabular}

\begin{tabular}{c}
\das{Placeholder for medium solid} $\rhos/\rho = 1$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\\
\end{tabular}

% \caption{\label{fig:ElasticPistonConvergence}Convergence for elastic piston.\das{Placeholder for light solid $\rhos/\rho = 10^{-3}.$}}
\begin{tabular}{c}
\das{Placeholder for light solid} $\rhos/\rho = 10^{-3}$
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.9e-04 &  & 1.4e-04 &  & 5.4e-05 &  & 1.6e-04 &  & 8.0e-04 & \\
1/40 & 1.9e-04 & 4.2 & 3.8e-05 & 3.7 & 1.2e-05 & 4.7 & 3.9e-05 & 4.0 & 1.9e-04 & 4.2\\
1/80 & 4.5e-05 & 4.1 & 9.9e-06 & 3.9 & 2.7e-06 & 4.3 & 9.9e-06 & 3.9 & 4.6e-05 & 4.1\\
1/160 & 1.1e-05 & 4.1 & 2.5e-06 & 3.9 & 6.4e-07 & 4.2 & 2.5e-06 & 3.9 & 1.2e-05 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}






==> tables/ShearSolutionConvergence.tex <==
\begin{table}[H]
\caption{\label{fig:ShearSolutionConvergence}Shear solution convergence tables for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be
$\bar{H} = \frac{1}{2}, H = 1, \rho = 1, \bar{\rho} = 10, 
\bar{\mu} = 10$, and $\mu = 10.$ }
\begin{center}
\begin{tabular}{c}
\das{placeholder heavy solid} $\rhos/\rho = 10^3$ 
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.3e-10 &  & 2.0e-03 &  & 3.4e-04 &  & 2.0e-03 &  & 1.9e-02 & \\
1/40 & 2.9e-10 & 0.5 & 5.0e-04 & 4.0 & 7.3e-05 & 4.7 & 5.0e-04 & 4.0 & 5.1e-03 & 3.8\\
1/80 & 6.3e-10 & 0.5 & 1.2e-04 & 4.0 & 1.7e-05 & 4.4 & 1.2e-04 & 4.0 & 1.3e-03 & 3.9\\
1/160 & 1.4e-09 & 0.5 & 3.1e-05 & 4.0 & 4.0e-06 & 4.2 & 3.1e-05 & 4.0 & 3.3e-04 & 4.0\\
\hline
\\
\end{tabular}

\begin{tabular}{c}
\das{placeholder medium solid} $\rhos/\rho = 1$ 
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.3e-10 &  & 2.0e-03 &  & 3.4e-04 &  & 2.0e-03 &  & 1.9e-02 & \\
1/40 & 2.9e-10 & 0.5 & 5.0e-04 & 4.0 & 7.3e-05 & 4.7 & 5.0e-04 & 4.0 & 5.1e-03 & 3.8\\
1/80 & 6.3e-10 & 0.5 & 1.2e-04 & 4.0 & 1.7e-05 & 4.4 & 1.2e-04 & 4.0 & 1.3e-03 & 3.9\\
1/160 & 1.4e-09 & 0.5 & 3.1e-05 & 4.0 & 4.0e-06 & 4.2 & 3.1e-05 & 4.0 & 3.3e-04 & 4.0\\
\hline
\\
\end{tabular}

\begin{tabular}{c}
\das{placeholder light solid} $\rhos/\rho = 10^{-3}$ 
\end{tabular}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.3e-10 &  & 2.0e-03 &  & 3.4e-04 &  & 2.0e-03 &  & 1.9e-02 & \\
1/40 & 2.9e-10 & 0.5 & 5.0e-04 & 4.0 & 7.3e-05 & 4.7 & 5.0e-04 & 4.0 & 5.1e-03 & 3.8\\
1/80 & 6.3e-10 & 0.5 & 1.2e-04 & 4.0 & 1.7e-05 & 4.4 & 1.2e-04 & 4.0 & 1.3e-03 & 3.9\\
1/160 & 1.4e-09 & 0.5 & 3.1e-05 & 4.0 & 4.0e-06 & 4.2 & 3.1e-05 & 4.0 & 3.3e-04 & 4.0\\
\hline
\end{tabular}

\end{center}
\end{table}


==> tables/SolidDisturbanceConvergence.tex <==
\begin{table}[H]
\caption{\label{fig:SolidDisturbanceConvergence}Convergence for solid disturbance.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.3e-02 &  & 5.0e-03 &  & 4.2e-04 &  & 3.7e-02 &  & 1.3e-01 & \\
1/40 & 1.7e-03 &  7.6 & 4.8e-04 & 10.4 & 6.0e-05 &  7.0 & 6.4e-03 &  5.8 & 1.7e-02 &  7.6\\
1/80 & 3.3e-04 &  5.2 & 6.5e-05 &  7.4 & 9.8e-06 &  6.1 & 1.2e-03 &  5.3 & 3.0e-03 &  5.7\\
1/160 & 6.4e-05 &  5.2 & 8.9e-06 &  7.3 & 1.6e-06 &  6.1 & 2.3e-04 &  5.2 & 5.2e-04 &  5.8\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/analysisAMP1D.tex <==
\begin{table}[h] 
\caption{\label{tab:analysisATP1dConvergence} AMP Scheme, $\rhos=100$, $\cp=150$, $\rho=14000$} 
\begin{center} 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline 
$N$ & $\Mr$ & $E^{(a)}$ & $r$ & $E^{(b)}$ & $r$ & $E^{(v)}$ & $r$ & $E^{(pI)}$ & $r$ \\ 
\hline 
 160 & 2.2e+04 & 1.5e-01 &     & 1.1e-04 &     & 5.7e-08 &     & 7.4e-08 &     \\ 
\hline 
 320 & 4.5e+04 & 3.9e-02 & 3.9 & 2.8e-05 & 4.0 & 1.4e-08 & 4.0 & 1.9e-08 & 4.0 \\ 
\hline 
 640 & 9.0e+04 & 9.7e-03 & 4.0 & 7.1e-06 & 4.0 & 3.6e-09 & 4.0 & 4.7e-09 & 4.0 \\ 
\hline 
1280 & 1.8e+05 & 2.4e-03 & 4.0 & 1.8e-06 & 4.0 & 8.9e-10 & 4.0 & 1.2e-09 & 4.0 \\ 
\hline 
rate &  & 1.99 &  & 2.00 &  & 2.00 &  & 2.00 &  \\ 
\hline 
\end{tabular} 
\end{center} 
\end{table} 


==> tables/analysisAMP1DHeavy.tex <==
\begin{table}[h] 
\caption{\label{tab:analysisATP1dConvergenceHeavy} 1D AMP Scheme, $\rhos=8000$, $\cp=4000$, $\rho=1$} 
\begin{center} 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline 
$N$ & $\Mr$ & $E^{(a)}$ & $r$ & $E^{(b)}$ & $r$ & $E^{(v)}$ & $r$ & $E^{(pI)}$ & $r$ \\ 
\hline 
 160 & 2.0e-02 & 1.5e-01 &     & 6.1e-04 &     & 1.5e-01 &     & 1.5e-01 &     \\ 
\hline 
 320 & 4.0e-02 & 3.9e-02 & 3.9 & 1.5e-04 & 4.0 & 3.9e-02 & 3.9 & 3.7e-02 & 3.9 \\ 
\hline 
 640 & 8.0e-02 & 9.7e-03 & 4.0 & 3.8e-05 & 4.0 & 9.7e-03 & 4.0 & 9.5e-03 & 3.9 \\ 
\hline 
1280 & 1.6e-01 & 2.4e-03 & 4.0 & 9.6e-06 & 4.0 & 2.4e-03 & 4.0 & 2.4e-03 & 3.9 \\ 
\hline 
rate &  & 1.99 &  & 2.00 &  & 2.00 &  & 1.97 &  \\ 
\hline 
\end{tabular} 
\end{center} 
\end{table} 


==> tables/analysisAMP1DLight.tex <==
\begin{table}[h] 
\caption{\label{tab:analysisATP1dConvergenceLight} 1D AMP Scheme, $\rhos=100$, $\cp=150$, $\rho=14000$} 
\begin{center} 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline 
$N$ & $\Mr$ & $E^{(a)}$ & $r$ & $E^{(b)}$ & $r$ & $E^{(v)}$ & $r$ & $E^{(pI)}$ & $r$ \\ 
\hline 
 160 & 2.2e+04 & 1.5e-01 &     & 1.1e-04 &     & 5.7e-08 &     & 7.4e-08 &     \\ 
\hline 
 320 & 4.5e+04 & 3.9e-02 & 3.9 & 2.8e-05 & 4.0 & 1.4e-08 & 4.0 & 1.9e-08 & 4.0 \\ 
\hline 
 640 & 9.0e+04 & 9.7e-03 & 4.0 & 7.1e-06 & 4.0 & 3.6e-09 & 4.0 & 4.7e-09 & 4.0 \\ 
\hline 
1280 & 1.8e+05 & 2.4e-03 & 4.0 & 1.8e-06 & 4.0 & 8.9e-10 & 4.0 & 1.2e-09 & 4.0 \\ 
\hline 
rate &  & 1.99 &  & 2.00 &  & 2.00 &  & 2.00 &  \\ 
\hline 
\end{tabular} 
\end{center} 
\end{table} 


==> tables/analysisATP1D.tex <==
\begin{table}[h] 
\caption{\label{tab:analysisATP1dConvergence} 1D ATP Scheme, $\rhos=100$, $\cp=150$, $\rho=14000$} 
\begin{center} 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline 
$N$ & $\Mr$ & $E^{(a)}$ & $r$ & $E^{(b)}$ & $r$ & $E^{(v)}$ & $r$ & $E^{(pI)}$ & $r$ \\ 
\hline 
 160 & 2.2e+04 & 1.5e-01 &     & 1.1e-04 &     & 5.6e-08 &     & 7.3e-08 &     \\ 
\hline 
 320 & 4.5e+04 & 3.9e-02 & 3.9 & 2.8e-05 & 4.0 & 1.4e-08 & 4.0 & 1.8e-08 & 4.0 \\ 
\hline 
 640 & 9.0e+04 & 9.7e-03 & 4.0 & 7.1e-06 & 4.0 & 3.5e-09 & 4.0 & 4.6e-09 & 4.0 \\ 
\hline 
1280 & 1.8e+05 & 2.4e-03 & 4.0 & 1.8e-06 & 4.0 & 8.8e-10 & 4.0 & 1.1e-09 & 4.0 \\ 
\hline 
rate &  & 1.99 &  & 2.00 &  & 2.00 &  & 2.00 &  \\ 
\hline 
\end{tabular} 
\end{center} 
\end{table} 


==> tables/analysisTP1D.tex <==
\begin{table}[h] 
\caption{\label{tab:analysisTP1dConvergence} 1D TP Scheme, $\rhos=8000$, $\cp=4000$, $\rho=1$} 
\begin{center} 
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline 
$N$ & $\Mr$ & $E^{(a)}$ & $r$ & $E^{(b)}$ & $r$ & $E^{(v)}$ & $r$ & $E^{(pI)}$ & $r$ \\ 
\hline 
 160 & 2.0e-02 & 1.5e-01 &     & 6.1e-04 &     & 1.5e-01 &     & 1.3e-01 &     \\ 
\hline 
 320 & 4.0e-02 & 3.9e-02 & 3.9 & 1.5e-04 & 4.0 & 3.9e-02 & 3.9 & 3.4e-02 & 4.0 \\ 
\hline 
 640 & 8.0e-02 & 9.7e-03 & 4.0 & 3.8e-05 & 4.0 & 9.7e-03 & 4.0 & 8.4e-03 & 4.0 \\ 
\hline 
1280 & 1.6e-01 & 2.4e-03 & 4.0 & 9.6e-06 & 4.0 & 2.4e-03 & 4.0 & 2.1e-03 & 4.0 \\ 
\hline 
rate &  & 1.99 &  & 2.00 &  & 2.00 &  & 2.00 &  \\ 
\hline 
\end{tabular} 
\end{center} 
\end{table} 


==> tables/insElasticPiston.epgp.AmpSCF1NUp05zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{8.7}{-3} &      & \num{5.7}{-4} &      & \num{8.8}{-4} &      & \num{5.6}{-4} &      & \num{7.5}{-3} &       \\ \hline
                epg2 &     2 & \num{1.8}{-3} &  4.8 & \num{2.7}{-4} &  2.1 & \num{2.1}{-4} &  4.2 & \num{2.7}{-4} &  2.1 & \num{1.5}{-3} &  4.9  \\ \hline
                epg4 &     4 & \num{4.3}{-4} &  4.3 & \num{8.2}{-5} &  3.3 & \num{5.1}{-5} &  4.1 & \num{8.1}{-5} &  3.3 & \num{3.5}{-4} &  4.3  \\ \hline
                epg8 &     8 & \num{1.1}{-4} &  4.1 & \num{2.2}{-5} &  3.7 & \num{1.2}{-5} &  4.1 & \num{2.2}{-5} &  3.7 & \num{8.9}{-5} &  4.0  \\ \hline
    rate             &       &  $2.12$       &      &  $1.58$       &      &  $2.04$       &      &  $1.57$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1NUp05zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:34:30 2018}\label{table:insElasticPiston.epgp.AmpSCF1NUp05zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.epgp.AmpSCF1e-3NUp05zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{1.0}{-3} &      & \num{5.0}{-4} &      & \num{6.7}{-4} &      & \num{5.0}{-4} &      & \num{9.1}{-6} &       \\ \hline
                epg2 &     2 & \num{2.8}{-4} &  3.5 & \num{1.4}{-4} &  3.5 & \num{1.9}{-4} &  3.6 & \num{1.7}{-4} &  3.0 & \num{1.8}{-6} &  5.0  \\ \hline
                epg4 &     4 & \num{7.3}{-5} &  3.9 & \num{3.8}{-5} &  3.8 & \num{4.9}{-5} &  3.9 & \num{3.8}{-5} &  4.5 & \num{4.3}{-7} &  4.3  \\ \hline
                epg8 &     8 & \num{1.8}{-5} &  4.0 & \num{9.7}{-6} &  3.9 & \num{1.2}{-5} &  4.0 & \num{9.7}{-6} &  3.9 & \num{1.1}{-7} &  3.9  \\ \hline
    rate             &       &  $1.93$       &      &  $1.90$       &      &  $1.93$       &      &  $1.93$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1e-3NUp05zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:33:34 2018}\label{table:insElasticPiston.epgp.AmpSCF1e-3NUp05zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.epgp.AmpSCF1e3NUp05zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{2.9}{-2} &      & \num{4.1}{-3} &      & \num{8.9}{-4} &      & \num{4.1}{-3} &      & \num{6.7}{0} &       \\ \hline
                epg2 &     2 & \num{7.3}{-3} &  4.0 & \num{1.1}{-3} &  3.6 & \num{1.6}{-4} &  5.4 & \num{1.1}{-3} &  3.6 & \num{1.6}{0} &  4.2  \\ \hline
                epg4 &     4 & \num{1.7}{-3} &  4.3 & \num{3.0}{-4} &  3.8 & \num{3.2}{-5} &  5.1 & \num{3.0}{-4} &  3.8 & \num{3.7}{-1} &  4.4  \\ \hline
                epg8 &     8 & \num{4.0}{-4} &  4.2 & \num{7.7}{-5} &  3.9 & \num{6.9}{-6} &  4.7 & \num{7.7}{-5} &  3.9 & \num{8.4}{-2} &  4.4  \\ \hline
    rate             &       &  $2.06$       &      &  $1.91$       &      &  $2.33$       &      &  $1.91$       &      &  $2.11$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1e3NUp05zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:43:42 2018}\label{table:insElasticPiston.epgp.AmpSCF1e3NUp05zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.epgp.shearAmpSCF1NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.4}{-5} &      & \num{2.0}{-6} &      & \num{8.0}{-6} &      & \num{2.0}{-5} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{3.4}{-6} &  4.2 & \num{5.6}{-7} &  3.6 & \num{2.1}{-6} &  3.7 & \num{5.4}{-6} &  3.8  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{8.7}{-7} &  3.9 & \num{1.3}{-7} &  4.2 & \num{5.1}{-7} &  4.2 & \num{1.3}{-6} &  4.2  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{2.2}{-7} &  4.1 & \num{3.2}{-8} &  4.2 & \num{1.2}{-7} &  4.2 & \num{3.3}{-7} &  3.9  \\ \hline
    rate             &       &  $-nan$       &      &  $2.01$       &      &  $2.00$       &      &  $2.03$       &      &  $1.99$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:15:36 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.epgp.shearAmpSCF1e-3NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{2.7}{-9} &      & \num{1.1}{-8} &      & \num{1.4}{-7} &      & \num{9.6}{-11} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{6.6}{-10} &  4.1 & \num{8.8}{-10} & 12.6 & \num{2.8}{-8} &  5.1 & \num{1.5}{-11} &  6.5  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{1.6}{-10} &  4.0 & \num{9.0}{-11} &  9.8 & \num{2.0}{-9} & 14.0 & \num{2.4}{-12} &  6.3  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{4.2}{-11} &  4.0 & \num{2.0}{-11} &  4.5 & \num{3.1}{-10} &  6.3 & \num{2.7}{-13} &  8.6  \\ \hline
    rate             &       &  $-nan$       &      &  $2.01$       &      &  $3.06$       &      &  $3.02$       &      &  $2.80$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e-3NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:14:52 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e-3NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.epgp.shearAmpSCF1e3NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.1}{-4} &      & \num{1.2}{-5} &      & \num{1.1}{-4} &      & \num{5.0}{-2} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{2.3}{-5} &  4.9 & \num{2.4}{-6} &  4.8 & \num{2.3}{-5} &  4.9 & \num{8.3}{-3} &  6.1  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{5.3}{-6} &  4.3 & \num{5.0}{-7} &  4.9 & \num{5.4}{-6} &  4.2 & \num{1.5}{-3} &  5.5  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{1.3}{-6} &  4.1 & \num{1.1}{-7} &  4.7 & \num{1.4}{-6} &  4.0 & \num{3.0}{-4} &  5.1  \\ \hline
    rate             &       &  $-nan$       &      &  $2.14$       &      &  $2.26$       &      &  $2.12$       &      &  $2.47$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e3NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:16:19 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e3NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.rep.AmpSCF1NUp05zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{6.6}{-3} &      & \num{1.1}{-2} &      & \num{1.3}{-3} &      & \num{9.9}{-3} &      & \num{1.1}{-2} &       \\ \hline
                rep2 &     2 & \num{8.6}{-4} &  7.7 & \num{1.7}{-3} &  6.4 & \num{7.1}{-5} & 17.9 & \num{1.6}{-3} &  6.1 & \num{1.1}{-3} &  9.7  \\ \hline
                rep4 &     4 & \num{2.6}{-4} &  3.3 & \num{3.9}{-4} &  4.2 & \num{1.8}{-5} &  3.9 & \num{3.8}{-4} &  4.2 & \num{3.4}{-4} &  3.4  \\ \hline
                rep8 &     8 & \num{6.6}{-5} &  4.0 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.7 & \num{9.9}{-5} &  3.9 & \num{9.0}{-5} &  3.8  \\ \hline
    rate             &       &  $2.17$       &      &  $2.22$       &      &  $2.61$       &      &  $2.20$       &      &  $2.26$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1NUp05zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:53:17 2018}\label{table:insElasticPiston.rep.AmpSCF1NUp05zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.rep.AmpSCF1e-3NUp05zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.5}{-3} &      & \num{3.2}{-2} &      & \num{1.8}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  8.8 & \num{4.9}{-4} &  3.7 & \num{3.6}{-4} & 12.4 & \num{7.5}{-3} &  4.3 & \num{1.9}{-5} &  9.8  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.7}{-5} &  4.2 & \num{9.0}{-4} &  8.3 & \num{4.5}{-6} &  4.2  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  4.0 & \num{2.5}{-5} &  4.2 & \num{2.3}{-5} &  3.8 & \num{3.1}{-4} &  2.9 & \num{4.4}{-7} & 10.1  \\ \hline
    rate             &       &  $2.41$       &      &  $2.07$       &      &  $2.50$       &      &  $2.32$       &      &  $2.82$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3NUp05zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:49:55 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3NUp05zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.rep.AmpSCF1e3NUp05zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.3}{-2} &      & \num{1.3}{-2} &      & \num{4.6}{-4} &      & \num{5.9}{-3} &      & \num{5.4}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.6 & \num{1.3}{-3} &  9.9 & \num{1.1}{-4} &  4.0 & \num{1.4}{-3} &  4.3 & \num{1.5}{0} &  3.5  \\ \hline
                rep4 &     4 & \num{6.5}{-4} &  2.7 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.6}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{1.2}{-5} & 56.0 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.5 & \num{9.7}{-5} &  3.8 & \num{9.9}{-2} &  3.7  \\ \hline
    rate             &       &  $3.20$       &      &  $2.33$       &      &  $1.99$       &      &  $1.97$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3NUp05zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:56:37 2018}\label{table:insElasticPiston.rep.AmpSCF1e3NUp05zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.rep.shearAmpSCF1NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{2.6}{-6} &      & \num{5.6}{-6} &      & \num{1.9}{-6} &      & \num{1.2}{-5} &      & \num{1.4}{-5} &       \\ \hline
                rep2 &     2 & \num{1.8}{-7} & 14.3 & \num{1.7}{-6} &  3.3 & \num{3.7}{-7} &  5.0 & \num{4.5}{-6} &  2.7 & \num{2.2}{-6} &  6.1  \\ \hline
                rep4 &     4 & \num{3.4}{-8} &  5.3 & \num{4.0}{-7} &  4.2 & \num{8.8}{-8} &  4.3 & \num{1.1}{-6} &  4.1 & \num{4.5}{-7} &  5.0  \\ \hline
                rep8 &     8 & \num{4.0}{-9} &  8.5 & \num{9.6}{-8} &  4.2 & \num{2.0}{-8} &  4.3 & \num{2.6}{-7} &  4.2 & \num{1.1}{-7} &  3.9  \\ \hline
    rate             &       &  $3.04$       &      &  $1.97$       &      &  $2.17$       &      &  $1.87$       &      &  $2.31$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Thu Aug 23 11:33:47 2018}\label{table:insElasticPiston.rep.shearAmpSCF1NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.rep.shearAmpSCF1e-3NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.5}{-6} &      & \num{1.3}{-5} &      & \num{1.4}{-3} &      & \num{4.3}{-3} &      & \num{1.1}{-5} &       \\ \hline
                rep2 &     2 & \num{1.4}{-7} & 10.6 & \num{2.2}{-6} &  6.0 & \num{4.1}{-4} &  3.3 & \num{1.4}{-3} &  3.2 & \num{3.0}{-6} &  3.7  \\ \hline
                rep4 &     4 & \num{1.5}{-8} &  9.5 & \num{5.4}{-7} &  4.0 & \num{1.0}{-4} &  4.0 & \num{3.2}{-4} &  4.3 & \num{7.0}{-7} &  4.3  \\ \hline
                rep8 &     8 & \num{1.9}{-9} &  7.8 & \num{1.5}{-7} &  3.6 & \num{2.6}{-5} &  3.9 & \num{8.0}{-5} &  4.0 & \num{1.7}{-7} &  4.0  \\ \hline
    rate             &       &  $3.21$       &      &  $2.13$       &      &  $1.91$       &      &  $1.94$       &      &  $2.01$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e-3NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Thu Aug 23 11:27:40 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e-3NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.rep.shearAmpSCF1e3NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.2}{-6} &      & \num{9.9}{-6} &      & \num{5.3}{-6} &      & \num{6.3}{-6} &      & \num{4.6}{-2} &       \\ \hline
                rep2 &     2 & \num{6.4}{-7} & 12.9 & \num{2.5}{-6} &  3.9 & \num{1.2}{-6} &  4.4 & \num{2.2}{-6} &  2.9 & \num{1.1}{-2} &  4.4  \\ \hline
                rep4 &     4 & \num{3.5}{-7} &  1.8 & \num{5.8}{-7} &  4.3 & \num{2.7}{-7} &  4.4 & \num{6.1}{-7} &  3.6 & \num{2.4}{-3} &  4.5  \\ \hline
                rep8 &     8 & \num{7.9}{-8} &  4.4 & \num{1.4}{-7} &  4.2 & \num{6.4}{-8} &  4.3 & \num{1.7}{-7} &  3.6 & \num{5.5}{-4} &  4.3  \\ \hline
    rate             &       &  $2.10$       &      &  $2.07$       &      &  $2.12$       &      &  $1.74$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Thu Aug 23 11:40:00 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NUp1zfmImtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.6}{-8} &      & \num{1.7}{-8} &      & \num{6.0}{-9} &      & \num{2.0}{-8} &      & \num{5.7}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.7}{-8} &  2.2 & \num{4.9}{-9} &  3.5 & \num{1.2}{-9} &  4.9 & \num{4.9}{-9} &  4.1 & \num{1.5}{-8} &  3.9  \\ \hline
                rtw8 &     4 & \num{3.4}{-9} &  4.9 & \num{1.1}{-9} &  4.4 & \num{2.7}{-10} &  4.6 & \num{1.1}{-9} &  4.4 & \num{4.5}{-9} &  3.3  \\ \hline
               rtw16 &     8 & \num{8.5}{-10} &  4.0 & \num{2.8}{-10} &  4.0 & \num{6.3}{-11} &  4.3 & \num{2.7}{-10} &  4.1 & \num{1.0}{-9} &  4.5  \\ \hline
    rate             &       &  $1.85$       &      &  $1.99$       &      &  $2.19$       &      &  $2.08$       &      &  $1.93$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NUp1zfmImtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-7 Thu Aug 23 12:59:36 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NUp1zfmImtp3}
\end{center}
\end{table}


==> tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCFp1NUp1zfmImtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{5.6}{-8} &      & \num{3.1}{-8} &      & \num{4.3}{-8} &      & \num{3.4}{-7} &      & \num{4.6}{-8} &       \\ \hline
                rtw4 &     2 & \num{8.8}{-9} &  6.3 & \num{9.2}{-9} &  3.4 & \num{6.0}{-9} &  7.1 & \num{6.7}{-8} &  5.0 & \num{8.6}{-9} &  5.3  \\ \hline
                rtw8 &     4 & \num{2.0}{-9} &  4.3 & \num{2.4}{-9} &  3.8 & \num{1.3}{-9} &  4.6 & \num{1.6}{-8} &  4.2 & \num{2.3}{-9} &  3.8  \\ \hline
               rtw16 &     8 & \num{5.1}{-10} &  4.0 & \num{6.6}{-10} &  3.6 & \num{3.0}{-10} &  4.3 & \num{3.9}{-9} &  4.1 & \num{5.6}{-10} &  4.1  \\ \hline
    rate             &       &  $2.24$       &      &  $1.86$       &      &  $2.36$       &      &  $2.13$       &      &  $2.10$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCFp1NUp1zfmImtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=.1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=7 -amp=1e-7 Thu Aug 23 13:01:34 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCFp1NUp1zfmImtp3}
\end{center}
\end{table}


==> tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NUp1zfmImtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{1.9}{-8} &      & \num{1.4}{-8} &      & \num{9.2}{-10} &      & \num{6.3}{-9} &      & \num{8.9}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.4}{-8} &  1.3 & \num{3.7}{-9} &  3.7 & \num{2.5}{-10} &  3.7 & \num{2.0}{-9} &  3.2 & \num{3.2}{-8} &  2.8  \\ \hline
                rtw8 &     4 & \num{3.3}{-9} &  4.4 & \num{8.8}{-10} &  4.2 & \num{5.7}{-11} &  4.4 & \num{5.3}{-10} &  3.8 & \num{1.1}{-8} &  3.0  \\ \hline
               rtw16 &     8 & \num{8.1}{-10} &  4.1 & \num{2.3}{-10} &  3.9 & \num{1.3}{-11} &  4.4 & \num{1.4}{-10} &  3.9 & \num{2.2}{-9} &  4.7  \\ \hline
    rate             &       &  $1.57$       &      &  $1.99$       &      &  $2.06$       &      &  $1.85$       &      &  $1.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NUp1zfmImtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=8 -amp=1e-7 Thu Aug 23 13:01:45 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NUp1zfmImtp3}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_1000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.4e-04 &  & 2.5e-05 &  & 7.0e-06 &  & 1.0e-05 &  & 3.5e-02 & \\
1/40 & 3.7e-05 & 3.7 & 1.3e-06 & 18.3 & 1.6e-06 & 4.5 & 1.3e-06 & 8.1 & 6.8e-03 & 5.2\\
1/80 & 8.8e-06 & 4.2 & 1.1e-07 & 12.2 & 3.6e-07 & 4.3 & 1.3e-07 & 9.7 & 1.4e-03 & 4.7\\
1/160 & 1.8e-06 & 5.0 & 2.2e-08 & 4.9 & 8.7e-08 & 4.2 & 2.4e-08 & 5.5 & 3.3e-04 & 4.4\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_100_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = 100.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 8.4e-05 &  & 4.5e-06 &  & 7.1e-06 &  & 1.1e-05 &  & 3.4e-03 & \\
1/40 & 1.3e-05 & 6.5 & 7.9e-07 & 5.7 & 1.6e-06 & 4.5 & 1.2e-06 & 9.6 & 6.5e-04 & 5.3\\
1/80 & 1.8e-06 & 7.2 & 1.5e-07 & 5.2 & 3.7e-07 & 4.3 & 1.5e-07 & 7.7 & 1.4e-04 & 4.7\\
1/160 & 2.0e-07 & 9.1 & 3.1e-08 & 4.8 & 8.8e-08 & 4.2 & 3.1e-08 & 4.8 & 3.1e-05 & 4.4\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_10_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = 10.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.4e-05 &  & 1.1e-05 &  & 8.4e-06 &  & 1.1e-05 &  & 2.4e-04 & \\
1/40 & 6.2e-06 & 3.9 & 1.9e-06 & 5.8 & 1.9e-06 & 4.5 & 1.9e-06 & 5.8 & 4.2e-05 & 5.5\\
1/80 & 1.3e-06 & 4.8 & 3.5e-07 & 5.3 & 4.3e-07 & 4.3 & 3.5e-07 & 5.3 & 8.7e-06 & 4.9\\
1/160 & 2.9e-07 & 4.5 & 7.3e-08 & 4.8 & 1.0e-07 & 4.2 & 7.3e-08 & 4.8 & 1.9e-06 & 4.5\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_1_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = 1.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 4.3e-05 &  & 3.2e-07 &  & 1.6e-05 &  & 1.4e-05 &  & 3.9e-05 & \\
1/40 & 1.0e-05 & 4.3 & 6.6e-07 & 0.5 & 3.4e-06 & 4.7 & 2.6e-06 & 5.5 & 7.7e-06 & 5.0\\
1/80 & 2.4e-06 & 4.2 & 2.6e-07 & 2.6 & 7.7e-07 & 4.4 & 5.0e-07 & 5.1 & 1.7e-06 & 4.6\\
1/160 & 5.8e-07 & 4.1 & 7.7e-08 & 3.4 & 1.8e-07 & 4.2 & 1.1e-07 & 4.7 & 3.8e-07 & 4.4\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_1_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .9, scf = 1}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.2e-04 &  & 2.4e-05 &  & 4.3e-05 &  & 3.1e-05 &  & 9.0e-05 & \\
1/40 & 2.9e-05 & 4.0 & 8.0e-06 & 3.0 & 1.1e-05 & 4.0 & 8.9e-06 & 3.5 & 2.1e-05 & 4.3\\
1/80 & 7.4e-06 & 4.0 & 2.2e-06 & 3.5 & 2.7e-06 & 4.0 & 2.4e-06 & 3.8 & 5.0e-06 & 4.1\\
1/160 & 2.0e-05 & 0.4 & 1.5e-06 & 1.5 & 7.1e-07 & 3.8 & 2.2e-04 & 0.0 & 3.4e-05 & 0.1\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_p001_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = .001}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.7e-05 &  & 1.7e-05 &  & 2.1e-05 &  & 3.1e-05 &  & 6.9e-08 & \\
1/40 & 4.4e-06 & 3.9 & 4.2e-06 & 4.0 & 4.4e-06 & 4.7 & 6.1e-06 & 5.0 & 1.4e-08 & 5.1\\
1/80 & 1.1e-06 & 4.0 & 1.1e-06 & 4.0 & 9.8e-07 & 4.4 & 1.3e-06 & 4.7 & 3.0e-09 & 4.5\\
1/160 & 2.7e-07 & 4.0 & 2.6e-07 & 4.0 & 2.3e-07 & 4.2 & 2.9e-07 & 4.4 & 7.1e-10 & 4.3\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_p01_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = .01}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.8e-05 &  & 1.6e-05 &  & 2.1e-05 &  & 3.0e-05 &  & 6.8e-07 & \\
1/40 & 4.5e-06 & 4.0 & 4.2e-06 & 4.0 & 4.4e-06 & 4.7 & 6.0e-06 & 5.0 & 1.4e-07 & 5.1\\
1/80 & 1.1e-06 & 4.0 & 1.0e-06 & 4.0 & 9.8e-07 & 4.4 & 1.3e-06 & 4.7 & 3.0e-08 & 4.5\\
1/160 & 2.8e-07 & 4.0 & 2.6e-07 & 4.0 & 2.3e-07 & 4.2 & 2.9e-07 & 4.4 & 7.0e-09 & 4.3\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_b_rs_p1_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = .1}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.2e-05 &  & 1.4e-05 &  & 2.0e-05 &  & 2.8e-05 &  & 6.5e-06 & \\
1/40 & 5.4e-06 & 4.1 & 3.7e-06 & 3.8 & 4.2e-06 & 4.7 & 5.5e-06 & 5.1 & 1.3e-06 & 5.1\\
1/80 & 1.3e-06 & 4.1 & 9.4e-07 & 3.9 & 9.5e-07 & 4.4 & 1.2e-06 & 4.7 & 2.8e-07 & 4.6\\
1/160 & 3.3e-07 & 4.0 & 2.4e-07 & 4.0 & 2.3e-07 & 4.2 & 2.7e-07 & 4.4 & 6.6e-08 & 4.3\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_rs_1000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .5, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.0e-03 &  & 1.6e-04 &  & 4.0e-05 &  & 1.6e-04 &  & 9.0e-02 & \\
1/40 & 3.8e-04 & 5.1 & 2.5e-05 & 6.3 & 7.7e-06 & 5.2 & 2.5e-05 & 6.3 & 2.3e-02 & 4.0\\
1/80 & 7.6e-05 & 5.0 & 4.4e-06 & 5.8 & 1.6e-06 & 4.8 & 4.4e-06 & 5.8 & 5.5e-03 & 4.1\\
1/160 & 1.6e-05 & 4.8 & 8.6e-07 & 5.1 & 3.5e-07 & 4.5 & 8.5e-07 & 5.2 & 1.4e-03 & 4.1\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_amp_rs_1000_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, AMP, t = .7, cfl = .9, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 7.4e-03 &  & 5.4e-04 &  & 7.3e-05 &  & 1.2e-04 &  & 1.6e-01 & \\
1/40 & 1.0e-03 & 7.4 & 2.9e-05 & 18.8 & 1.2e-05 & 6.2 & 9.8e-06 & 11.8 & 1.7e-02 & 9.0\\
1/80 & 5.3e-05 & 18.9 & 2.5e-06 & 11.5 & 2.3e-06 & 5.1 & 3.8e-06 & 2.6 & 6.7e-03 & 2.6\\
1/160 & 2.7e-05 & 2.0 & 2.5e-06 & 1.0 & 5.5e-07 & 4.2 & 2.0e-04 & 0.0 & 3.2e-02 & 0.2\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_1000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.1e-03 &  & 3.4e-04 &  & 9.3e-06 &  & 2.1e-05 &  & 1.8e-02 & \\
1/40 & 2.7e-04 & 4.0 & 9.2e-05 & 3.7 & 1.9e-06 & 4.9 & 2.6e-06 & 8.4 & 4.3e-03 & 4.3\\
1/80 & 7.0e-05 & 3.9 & 2.4e-05 & 3.9 & 4.1e-07 & 4.6 & 3.1e-07 & 8.2 & 1.1e-03 & 4.0\\
1/160 & 1.9e-05 & 3.6 & 6.0e-06 & 4.0 & 9.5e-08 & 4.3 & 4.0e-08 & 7.8 & 2.7e-04 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_1000_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.4e-04 &  & 3.6e-04 &  & 3.0e-05 &  & 1.1e-05 &  & 1.2e-02 & \\
1/40 & 5.1e-05 & 4.7 & 8.9e-05 & 4.1 & 8.2e-06 & 3.7 & 1.2e-06 & 8.9 & 4.7e-03 & 2.6\\
1/80 & 4.8e-06 & 10.6 & 2.1e-05 & 4.2 & 2.1e-06 & 3.9 & 1.9e-07 & 6.4 & 1.7e-03 & 2.7\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_1600_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 1600.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.1e-03 &  & 3.4e-04 &  & 9.2e-06 &  & 2.1e-05 &  & 3.0e-02 & \\
1/40 & 2.7e-04 & 4.0 & 9.2e-05 & 3.7 & 1.9e-06 & 4.9 & 2.5e-06 & 8.5 & 7.0e-03 & 4.3\\
1/80 & 6.8e-05 & 3.9 & 2.4e-05 & 3.9 & 4.0e-07 & 4.6 & 2.9e-07 & 8.6 & 1.8e-03 & 4.0\\
1/160 & 1.8e-05 & 3.8 & 6.0e-06 & 3.9 & 9.4e-08 & 4.3 & 3.2e-08 & 8.9 & 4.4e-04 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_1600_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 1600.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.6e-04 &  & 3.6e-04 &  & 3.0e-05 &  & 1.1e-05 &  & 2.0e-02 & \\
1/40 & 6.1e-05 & 4.2 & 9.0e-05 & 4.0 & 8.2e-06 & 3.7 & 1.2e-06 & 9.1 & 7.5e-03 & 2.7\\
1/80 & 1.1e-05 & 5.4 & 2.2e-05 & 4.1 & 2.1e-06 & 3.8 & 1.9e-07 & 6.1 & 2.8e-03 & 2.7\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_4000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 4000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.1e-03 &  & 3.4e-04 &  & 9.1e-06 &  & 2.1e-05 &  & 7.7e-02 & \\
1/40 & 2.7e-04 & 4.0 & 9.2e-05 & 3.7 & 1.8e-06 & 5.0 & 2.4e-06 & 8.6 & 1.8e-02 & 4.2\\
1/80 & 6.7e-05 & 4.0 & 2.4e-05 & 3.9 & 4.0e-07 & 4.6 & 2.7e-07 & 8.9 & 4.6e-03 & 4.0\\
1/160 & 1.7e-05 & 3.9 & 6.0e-06 & 3.9 & 9.2e-08 & 4.3 & 2.7e-08 & 10.0 & 1.1e-03 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_4000_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 4000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.7e-04 &  & 3.7e-04 &  & 3.0e-05 &  & 1.0e-05 &  & 5.1e-02 & \\
1/40 & 7.0e-05 & 3.9 & 9.2e-05 & 4.0 & 8.2e-06 & 3.7 & 1.1e-06 & 9.2 & 1.8e-02 & 2.8\\
1/80 & 1.7e-05 & 4.2 & 2.3e-05 & 4.0 & 2.1e-06 & 3.8 & 1.9e-07 & 5.9 & 6.8e-03 & 2.7\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_8000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 8000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.1e-03 &  & 3.4e-04 &  & 9.1e-06 &  & 2.1e-05 &  & 1.6e-01 & \\
1/40 & 2.6e-04 & 4.0 & 9.2e-05 & 3.7 & 1.8e-06 & 5.0 & 2.4e-06 & 8.7 & 3.7e-02 & 4.2\\
1/80 & 6.6e-05 & 4.0 & 2.4e-05 & 3.9 & 4.0e-07 & 4.6 & 2.6e-07 & 9.0 & 9.2e-03 & 4.0\\
1/160 & 1.7e-05 & 4.0 & 6.0e-06 & 3.9 & 9.2e-08 & 4.3 & 2.5e-08 & 10.4 & 2.3e-03 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_8000_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 8000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.8e-04 &  & 3.7e-04 &  & 3.0e-05 &  & 1.0e-05 &  & 1.0e-01 & \\
1/40 & 7.3e-05 & 3.8 & 9.2e-05 & 4.0 & 8.2e-06 & 3.7 & 1.1e-06 & 9.2 & 3.7e-02 & 2.8\\
1/80 & 1.8e-05 & 4.0 & 2.3e-05 & 4.0 & 2.1e-06 & 3.8 & 1.9e-07 & 5.8 & 1.4e-02 & 2.7\\
1/160 & 1.2e-02 & 0.0 & 4.8e-04 & 0.0 & 8.7e-07 & 2.4 & 4.8e-04 & 0.0 & 2.3e-01 & 0.1\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_800_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 800.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.1e-03 &  & 3.4e-04 &  & 9.3e-06 &  & 2.2e-05 &  & 1.4e-02 & \\
1/40 & 2.7e-04 & 3.9 & 9.2e-05 & 3.7 & 1.9e-06 & 4.9 & 2.6e-06 & 8.3 & 3.3e-03 & 4.3\\
1/80 & 7.2e-05 & 3.8 & 2.4e-05 & 3.9 & 4.1e-07 & 4.6 & 3.3e-07 & 8.0 & 8.3e-04 & 4.0\\
1/160 & 2.1e-05 & 3.4 & 5.9e-06 & 4.0 & 9.7e-08 & 4.3 & 4.7e-08 & 6.9 & 2.1e-04 & 4.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_b_rs_800_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 800.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 2.3e-04 &  & 3.6e-04 &  & 3.0e-05 &  & 1.1e-05 &  & 9.7e-03 & \\
1/40 & 4.3e-05 & 5.3 & 8.7e-05 & 4.1 & 8.2e-06 & 3.7 & 1.2e-06 & 8.8 & 3.8e-03 & 2.5\\
1/80 & 2.7e-07 & 163.0 & 2.0e-05 & 4.4 & 2.1e-06 & 3.9 & 1.8e-07 & 6.6 & 1.4e-03 & 2.8\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_1000_cfl_25_tf_3.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .3, cfl = .25, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 6.7e-03 &  & 1.9e-03 &  & 2.2e-05 &  & 1.3e-04 &  & 9.6e-02 & \\
1/40 & 1.7e-03 & 4.0 & 5.5e-04 & 3.6 & 5.0e-06 & 4.4 & 3.9e-05 & 3.3 & 1.3e-02 & 7.2\\
1/80 & 3.7e-04 & 4.6 & 1.4e-04 & 3.8 & 1.2e-06 & 4.2 & 1.1e-05 & 3.6 & 2.2e-03 & 6.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_1000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 3.7e-03 &  & 2.2e-03 &  & 1.6e-05 &  & 8.0e-05 &  & 6.1e-02 & \\
1/40 & 1.0e-03 & 3.7 & 5.5e-04 & 3.9 & 4.6e-06 & 3.5 & 1.3e-05 & 6.3 & 7.3e-03 & 8.3\\
1/80 & 2.4e-04 & 4.2 & 1.4e-04 & 3.9 & 1.2e-06 & 3.9 & 2.6e-06 & 5.0 & 3.4e-03 & 2.1\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_1000_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 1000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.8e-03 &  & 7.5e-04 &  & 5.2e-05 &  & 4.9e-05 &  & 5.3e-02 & \\
1/40 & 3.5e-04 & 5.1 & 2.0e-04 & 3.8 & 1.0e-05 & 5.2 & 7.1e-06 & 6.8 & 2.1e-02 & 2.5\\
1/80 & 6.5e-05 & 5.3 & 5.1e-05 & 3.9 & 2.1e-06 & 4.8 & 3.3e-06 & 2.2 & 8.1e-03 & 2.6\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_1600_cfl_25_tf_3.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .3, cfl = .25, scf = 1600.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 6.8e-03 &  & 1.9e-03 &  & 2.3e-05 &  & 1.3e-04 &  & 1.5e-01 & \\
1/40 & 1.8e-03 & 3.9 & 5.3e-04 & 3.6 & 5.1e-06 & 4.4 & 4.0e-05 & 3.3 & 2.1e-02 & 7.2\\
1/80 & 4.3e-04 & 4.1 & 1.4e-04 & 3.7 & 1.2e-06 & 4.2 & 1.1e-05 & 3.6 & 3.5e-03 & 6.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_1600_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 1600.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 3.7e-03 &  & 2.1e-03 &  & 1.6e-05 &  & 8.2e-05 &  & 9.2e-02 & \\
1/40 & 1.0e-03 & 3.6 & 5.4e-04 & 3.9 & 4.7e-06 & 3.5 & 1.3e-05 & 6.2 & 1.3e-02 & 7.1\\
1/80 & 2.6e-04 & 4.0 & 1.4e-04 & 3.9 & 1.2e-06 & 3.9 & 2.7e-06 & 5.0 & 5.7e-03 & 2.3\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_1600_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 1600.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.8e-03 &  & 7.5e-04 &  & 5.2e-05 &  & 5.0e-05 &  & 8.7e-02 & \\
1/40 & 3.6e-04 & 5.0 & 2.0e-04 & 3.8 & 1.0e-05 & 5.2 & 7.0e-06 & 7.1 & 3.4e-02 & 2.6\\
1/80 & 7.4e-05 & 4.9 & 5.1e-05 & 3.9 & 2.1e-06 & 4.8 & 3.3e-06 & 2.1 & 1.3e-02 & 2.6\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_4000_cfl_25_tf_3.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .3, cfl = .25, scf = 4000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 6.9e-03 &  & 1.9e-03 &  & 2.3e-05 &  & 1.3e-04 &  & 3.9e-01 & \\
1/40 & 1.8e-03 & 3.8 & 5.1e-04 & 3.6 & 5.2e-06 & 4.4 & 4.0e-05 & 3.3 & 5.3e-02 & 7.2\\
1/80 & 4.7e-04 & 3.9 & 1.4e-04 & 3.8 & 1.2e-06 & 4.2 & 1.1e-05 & 3.7 & 8.9e-03 & 6.0\\
1/160 & 1.2e-04 & 4.1 & 3.6e-05 & 3.8 & 3.0e-07 & 4.1 & 2.9e-06 & 3.8 & 1.7e-03 & 5.1\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_4000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 4000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 3.8e-03 &  & 2.1e-03 &  & 1.7e-05 &  & 8.4e-05 &  & 2.2e-01 & \\
1/40 & 1.0e-03 & 3.6 & 5.3e-04 & 4.0 & 4.7e-06 & 3.5 & 1.4e-05 & 6.1 & 3.6e-02 & 6.0\\
1/80 & 2.7e-04 & 3.8 & 1.3e-04 & 3.9 & 1.2e-06 & 3.9 & 2.8e-06 & 4.9 & 1.5e-02 & 2.4\\
1/160 & 6.8e-05 & 4.0 & 3.4e-05 & 3.9 & 3.1e-07 & 4.0 & 6.4e-07 & 4.4 & 4.5e-03 & 3.4\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_4000_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 4000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.8e-03 &  & 7.4e-04 &  & 5.3e-05 &  & 5.1e-05 &  & 2.2e-01 & \\
1/40 & 3.7e-04 & 4.9 & 2.0e-04 & 3.8 & 1.0e-05 & 5.2 & 6.8e-06 & 7.4 & 8.3e-02 & 2.7\\
1/80 & 8.0e-05 & 4.6 & 5.1e-05 & 3.9 & 2.1e-06 & 4.8 & 3.2e-06 & 2.1 & 3.2e-02 & 2.6\\
1/160 & 4.8e-03 & 0.0 & 2.2e-04 & 0.2 & 6.2e-07 & 3.4 & 2.2e-04 & 0.0 & 5.3e-02 & 0.6\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_8000_cfl_25_tf_3.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .3, cfl = .25, scf = 8000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 6.9e-03 &  & 1.9e-03 &  & 2.3e-05 &  & 1.3e-04 &  & 7.7e-01 & \\
1/40 & 1.8e-03 & 3.8 & 5.1e-04 & 3.7 & 5.2e-06 & 4.4 & 4.0e-05 & 3.3 & 1.1e-01 & 7.2\\
1/80 & 4.8e-04 & 3.8 & 1.3e-04 & 3.8 & 1.2e-06 & 4.2 & 1.1e-05 & 3.7 & 1.8e-02 & 6.0\\
1/160 & 1.2e-04 & 4.0 & 3.5e-05 & 3.7 & 3.0e-07 & 4.0 & 2.9e-06 & 3.8 & 3.5e-03 & 5.1\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_8000_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 8000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 3.8e-03 &  & 2.1e-03 &  & 1.7e-05 &  & 8.5e-05 &  & 4.2e-01 & \\
1/40 & 1.0e-03 & 3.6 & 5.2e-04 & 4.0 & 4.8e-06 & 3.5 & 1.4e-05 & 6.0 & 7.4e-02 & 5.7\\
1/80 & 2.7e-04 & 3.8 & 1.3e-04 & 4.0 & 1.2e-06 & 3.9 & 2.9e-06 & 4.9 & 3.1e-02 & 2.4\\
1/160 & 7.0e-05 & 3.9 & 3.3e-05 & 3.9 & 3.1e-07 & 4.0 & 6.5e-07 & 4.4 & 9.1e-03 & 3.4\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_8000_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 8000.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.8e-03 &  & 7.4e-04 &  & 5.3e-05 &  & 5.1e-05 &  & 4.5e-01 & \\
1/40 & 3.7e-04 & 4.9 & 2.0e-04 & 3.8 & 1.0e-05 & 5.2 & 6.8e-06 & 7.5 & 1.6e-01 & 2.7\\
1/80 & 8.2e-05 & 4.6 & 5.0e-05 & 3.9 & 2.1e-06 & 4.8 & 3.2e-06 & 2.1 & 6.3e-02 & 2.6\\
1/160 & 3.1e-03 & 0.0 & 1.4e-04 & 0.4 & 5.7e-07 & 3.7 & 1.4e-04 & 0.0 & 7.4e-02 & 0.9\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_800_cfl_25_tf_3.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .3, cfl = .25, scf = 800.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 6.6e-03 &  & 2.0e-03 &  & 2.2e-05 &  & 1.3e-04 &  & 7.7e-02 & \\
1/40 & 1.6e-03 & 4.1 & 5.5e-04 & 3.6 & 5.0e-06 & 4.4 & 3.9e-05 & 3.3 & 1.1e-02 & 7.2\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_800_cfl_5_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .5, scf = 800.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 3.7e-03 &  & 2.2e-03 &  & 1.6e-05 &  & 7.8e-05 &  & 5.1e-02 & \\
1/40 & 9.8e-04 & 3.7 & 5.6e-04 & 3.9 & 4.5e-06 & 3.5 & 1.2e-05 & 6.3 & 5.4e-03 & 9.3\\
1/80 & 2.2e-04 & 4.5 & 1.4e-04 & 3.9 & 1.2e-06 & 3.8 & 2.5e-06 & 5.0 & 2.7e-03 & 2.0\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/matlabOld/ep_mat_tp_rs_800_cfl_9_tf_7.tex <==
\begin{table}[H]
\caption{Matlab, TP, t = .7, cfl = .9, scf = 800.}
\begin{center}
\begin{tabular}{ccccccccccc}
\hline
$h$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/20 & 1.8e-03 &  & 7.6e-04 &  & 5.2e-05 &  & 4.8e-05 &  & 4.2e-02 & \\
1/40 & 3.4e-04 & 5.2 & 2.0e-04 & 3.8 & 1.0e-05 & 5.2 & 7.2e-06 & 6.6 & 1.7e-02 & 2.4\\
1/80 & 5.8e-05 & 5.8 & 5.0e-05 & 4.0 & 2.1e-06 & 4.8 & 3.3e-06 & 2.2 & 6.5e-03 & 2.7\\
\hline
\end{tabular}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpSCF0p01Imt0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{9.4}{-5} &      & \num{9.8}{-5} &      & \num{7.2}{-5} &      & \num{3.6}{-5} &      & \num{5.9}{-6} &       \\ \hline
                epg2 &     2 & \num{2.6}{-5} &  3.6 & \num{2.5}{-5} &  3.8 & \num{2.0}{-5} &  3.6 & \num{9.0}{-6} &  4.0 & \num{1.5}{-6} &  3.9  \\ \hline
                epg4 &     4 & \num{6.8}{-6} &  3.8 & \num{6.7}{-6} &  3.8 & \num{5.1}{-6} &  3.8 & \num{2.3}{-6} &  4.0 & \num{3.9}{-7} &  3.9  \\ \hline
    rate             &       &  $1.90$       &      &  $1.93$       &      &  $1.90$       &      &  $1.99$       &      &  $1.97$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF0p01Imt0p7, $t=0.7$, AM=1, cfl=.6, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.01, sm-diss=0.2  Tue Jul  4 11:25:00 2017}\label{table:insElasticPiston.epgp.AmpSCF0p01Imt0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpSCF0p1Imt0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{1.8}{-4} &      & \num{4.6}{-5} &      & \num{1.0}{-4} &      & \num{4.6}{-5} &      & \num{7.3}{-5} &       \\ \hline
                epg2 &     2 & \num{4.6}{-5} &  3.8 & \num{1.3}{-5} &  3.6 & \num{2.7}{-5} &  3.8 & \num{1.1}{-5} &  4.3 & \num{1.8}{-5} &  4.0  \\ \hline
                epg4 &     4 & \num{1.2}{-5} &  3.8 & \num{3.5}{-6} &  3.6 & \num{6.9}{-6} &  3.8 & \num{2.5}{-6} &  4.2 & \num{4.7}{-6} &  3.9  \\ \hline
    rate             &       &  $1.93$       &      &  $1.85$       &      &  $1.93$       &      &  $2.09$       &      &  $1.99$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF0p1Imt0p7, $t=0.7$, AM=1, cfl=.25, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.1, sm-diss=0.2  Tue Jul  4 11:19:44 2017}\label{table:insElasticPiston.epgp.AmpSCF0p1Imt0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpSCF1Imt0p3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{5.5}{-4} &      & \num{6.2}{-5} &      & \num{3.6}{-5} &      & \num{6.0}{-5} &      & \num{5.0}{-4} &       \\ \hline
                epg2 &     2 & \num{1.4}{-4} &  4.0 & \num{1.7}{-5} &  3.7 & \num{8.2}{-6} &  4.3 & \num{1.3}{-5} &  4.4 & \num{1.3}{-4} &  4.0  \\ \hline
                epg4 &     4 & \num{3.3}{-5} &  4.1 & \num{4.3}{-6} &  3.9 & \num{2.0}{-6} &  4.2 & \num{2.9}{-6} &  4.6 & \num{3.1}{-5} &  4.1  \\ \hline
    rate             &       &  $2.02$       &      &  $1.93$       &      &  $2.09$       &      &  $2.18$       &      &  $2.01$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1Imt0p3, $t=0.3$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, sm-diss=0.2  Tue Jul  4 10:04:23 2017}\label{table:insElasticPiston.epgp.AmpSCF1Imt0p3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpSCF1Imt0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{6.2}{-4} &      & \num{4.1}{-5} &      & \num{1.0}{-4} &      & \num{4.3}{-5} &      & \num{7.4}{-4} &       \\ \hline
                epg2 &     2 & \num{1.6}{-4} &  3.8 & \num{5.9}{-6} &  7.0 & \num{2.7}{-5} &  3.8 & \num{1.0}{-5} &  4.1 & \num{1.8}{-4} &  4.0  \\ \hline
                epg4 &     4 & \num{4.4}{-5} &  3.7 & \num{3.8}{-7} & 15.6 & \num{6.9}{-6} &  3.8 & \num{2.5}{-6} &  4.2 & \num{4.7}{-5} &  4.0  \\ \hline
    rate             &       &  $1.90$       &      &  $3.38$       &      &  $1.93$       &      &  $2.05$       &      &  $1.99$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpSCF1Imt0p7, $t=0.7$, AM=1, cfl=.25, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, sm-diss=0.2  Tue Jul  4 11:18:05 2017}\label{table:insElasticPiston.epgp.AmpSCF1Imt0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf0p001t0p3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{6.5}{-5} &      & \num{3.8}{-5} &      & \num{5.1}{-5} &      & \num{5.1}{-5} &      & \num{5.2}{-7} &       \\ \hline
                epg2 &     2 & \num{1.9}{-6} & 34.6 & \num{2.8}{-6} & 13.6 & \num{1.6}{-6} & 33.1 & \num{1.3}{-5} &  4.0 & \num{9.8}{-8} &  5.3  \\ \hline
                epg4 &     4 & \num{6.1}{-7} &  3.1 & \num{2.5}{-7} & 11.2 & \num{7.9}{-7} &  2.0 & \num{2.2}{-6} &  5.7 & \num{2.6}{-8} &  3.7  \\ \hline
                epg8 &     8 & \num{2.5}{-7} &  2.4 & \num{3.4}{-8} &  7.3 & \num{2.6}{-7} &  3.0 & \num{3.2}{-7} &  7.0 & \num{6.8}{-9} &  3.9  \\ \hline
    rate             &       &  $2.56$       &      &  $3.38$       &      &  $2.38$       &      &  $2.44$       &      &  $2.06$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf0p001t0p3, $t=.3$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=0.001, sm-diss=0.1  Mon Jul  3 06:53:56 2017}\label{table:insElasticPiston.epgp.AmpScf0p001t0p3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf0p001t0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{3.6}{-5} &      & \num{1.4}{-4} &      & \num{3.5}{-5} &      & \num{2.6}{-5} &      & \num{2.5}{-7} &       \\ \hline
                epg2 &     2 & \num{8.7}{-6} &  4.1 & \num{1.3}{-5} & 10.4 & \num{6.9}{-6} &  5.1 & \num{5.6}{-6} &  4.7 & \num{6.1}{-8} &  4.1  \\ \hline
                epg4 &     4 & \num{3.7}{-6} &  2.3 & \num{2.0}{-6} &  6.6 & \num{3.0}{-6} &  2.3 & \num{1.4}{-6} &  4.1 & \num{2.0}{-8} &  3.0  \\ \hline
                epg8 &     8 & \num{1.1}{-6} &  3.3 & \num{4.4}{-7} &  4.5 & \num{9.0}{-7} &  3.3 & \num{2.7}{-7} &  5.1 & \num{5.9}{-9} &  3.5  \\ \hline
    rate             &       &  $1.62$       &      &  $2.76$       &      &  $1.71$       &      &  $2.19$       &      &  $1.78$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf0p001t0p7, $t=.7$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=0.001, sm-diss=0.1  Mon Jul  3 06:59:59 2017}\label{table:insElasticPiston.epgp.AmpScf0p001t0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf0p1t0p3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{1.2}{-4} &      & \num{2.9}{-5} &      & \num{5.2}{-5} &      & \num{5.1}{-5} &      & \num{5.2}{-5} &       \\ \hline
                epg2 &     2 & \num{1.2}{-5} & 10.1 & \num{6.3}{-7} & 45.6 & \num{1.6}{-6} & 33.3 & \num{1.3}{-5} &  4.0 & \num{9.8}{-6} &  5.3  \\ \hline
                epg4 &     4 & \num{2.0}{-6} &  5.8 & \num{3.4}{-7} &  1.9 & \num{7.9}{-7} &  2.0 & \num{2.2}{-6} &  5.6 & \num{2.7}{-6} &  3.7  \\ \hline
                epg8 &     8 & \num{4.2}{-7} &  4.8 & \num{1.2}{-7} &  2.8 & \num{2.6}{-7} &  3.0 & \num{3.2}{-7} &  7.0 & \num{6.8}{-7} &  3.9  \\ \hline
    rate             &       &  $2.69$       &      &  $2.46$       &      &  $2.38$       &      &  $2.44$       &      &  $2.06$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf0p1t0p3, $t=.3$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=0.1, sm-diss=0.1  Mon Jul  3 06:51:03 2017}\label{table:insElasticPiston.epgp.AmpScf0p1t0p3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf1.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{5.6}{-4} &      & \num{5.1}{-5} &      & \num{5.1}{-5} &      & \num{4.6}{-5} &      & \num{5.0}{-4} &       \\ \hline
                epg2 &     2 & \num{9.8}{-5} &  5.7 & \num{1.9}{-5} &  2.7 & \num{1.5}{-6} & 34.2 & \num{1.2}{-5} &  3.8 & \num{9.7}{-5} &  5.1  \\ \hline
                epg4 &     4 & \num{2.6}{-5} &  3.8 & \num{5.7}{-6} &  3.3 & \num{7.9}{-7} &  1.9 & \num{2.2}{-6} &  5.6 & \num{2.6}{-5} &  3.7  \\ \hline
                epg8 &     8 & \num{6.5}{-6} &  3.9 & \num{1.5}{-6} &  3.7 & \num{2.6}{-7} &  3.0 & \num{3.2}{-7} &  7.0 & \num{6.8}{-6} &  3.9  \\ \hline
    rate             &       &  $2.12$       &      &  $1.69$       &      &  $2.37$       &      &  $2.40$       &      &  $2.04$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf1, $t=.3$, AM=1, cfl=.9, nu=0.1 CGSM=SM-Godunov, tz=none, scf=, sm-diss=0.1  Mon Jul  3 06:10:24 2017}\label{table:insElasticPiston.epgp.AmpScf1}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf1000t0p3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{4.1}{-3} &      & \num{1.2}{-3} &      & \num{3.5}{-5} &      & \num{6.2}{-5} &      & \num{1.8}{-1} &       \\ \hline
                epg2 &     2 & \num{4.3}{-3} &  1.0 & \num{2.7}{-4} &  4.5 & \num{2.2}{-6} & 15.9 & \num{4.8}{-6} & 12.8 & \num{5.2}{-2} &  3.5  \\ \hline
                epg4 &     4 & \num{2.8}{-3} &  1.5 & \num{7.2}{-5} &  3.8 & \num{1.1}{-6} &  2.0 & \num{9.6}{-7} &  5.0 & \num{1.8}{-2} &  2.9  \\ \hline
                epg8 &     8 & \num{1.2}{-3} &  2.3 & \num{2.8}{-5} &  2.6 & \num{3.2}{-7} &  3.5 & \num{2.7}{-7} &  3.6 & \num{4.7}{-3} &  3.8  \\ \hline
    rate             &       &  $0.58$       &      &  $1.82$       &      &  $2.14$       &      &  $2.59$       &      &  $1.73$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf1000t0p3, $t=.3$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=1000, sm-diss=0.1  Mon Jul  3 07:07:09 2017}\label{table:insElasticPiston.epgp.AmpScf1000t0p3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf1000t0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{4.2}{-3} &      & \num{1.0}{-3} &      & \num{1.8}{-5} &      & \num{5.9}{-5} &      & \num{1.7}{-1} &       \\ \hline
                epg2 &     2 & \num{3.9}{-4} & 10.8 & \num{4.0}{-5} & 26.3 & \num{1.1}{-5} &  1.6 & \num{1.7}{-5} &  3.5 & \num{8.6}{-2} &  1.9  \\ \hline
                epg4 &     4 & \num{7.8}{-5} &  5.0 & \num{2.1}{-6} & 18.6 & \num{3.8}{-6} &  3.1 & \num{2.9}{-6} &  5.8 & \num{2.5}{-2} &  3.4  \\ \hline
                epg8 &     8 & \num{3.2}{-4} &  0.2 & \num{5.2}{-6} &  0.4 & \num{1.0}{-6} &  3.7 & \num{4.2}{-7} &  6.9 & \num{6.5}{-3} &  3.9  \\ \hline
    rate             &       &  $1.36$       &      &  $2.72$       &      &  $1.40$       &      &  $2.39$       &      &  $1.58$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf1000t0p7, $t=.7$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=1000, sm-diss=0.1  Mon Jul  3 07:17:52 2017}\label{table:insElasticPiston.epgp.AmpScf1000t0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf1000t0p8.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{1.8}{-3} &      & \num{3.7}{-4} &      & \num{3.6}{-5} &      & \num{9.4}{-5} &      & \num{2.6}{-1} &       \\ \hline
                epg2 &     2 & \num{2.5}{-3} &  0.7 & \num{1.6}{-4} &  2.2 & \num{1.3}{-5} &  2.7 & \num{2.0}{-5} &  4.8 & \num{1.0}{-1} &  2.6  \\ \hline
                epg4 &     4 & \num{1.2}{-3} &  2.0 & \num{3.5}{-5} &  4.8 & \num{4.2}{-6} &  3.2 & \num{3.3}{-6} &  5.9 & \num{2.9}{-2} &  3.5  \\ \hline
                epg8 &     8 & \num{2.6}{-4} &  4.7 & \num{8.0}{-6} &  4.4 & \num{1.1}{-6} &  3.7 & \num{5.0}{-7} &  6.7 & \num{7.6}{-3} &  3.8  \\ \hline
    rate             &       &  $0.93$       &      &  $1.89$       &      &  $1.66$       &      &  $2.53$       &      &  $1.71$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf1000t0p8, $t=.8$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=1000, sm-diss=0.1  Mon Jul  3 07:21:58 2017}\label{table:insElasticPiston.epgp.AmpScf1000t0p8}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.AmpScf10t0p3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{3.0}{-3} &      & \num{5.9}{-4} &      & \num{4.5}{-5} &      & \num{1.2}{-5} &      & \num{2.9}{-3} &       \\ \hline
                epg2 &     2 & \num{7.4}{-4} &  4.0 & \num{1.7}{-4} &  3.4 & \num{1.1}{-6} & 41.4 & \num{8.8}{-6} &  1.3 & \num{7.4}{-4} &  3.9  \\ \hline
                epg4 &     4 & \num{2.4}{-4} &  3.1 & \num{5.4}{-5} &  3.2 & \num{8.1}{-7} &  1.3 & \num{2.0}{-6} &  4.4 & \num{2.4}{-4} &  3.1  \\ \hline
                epg8 &     8 & \num{6.6}{-5} &  3.6 & \num{1.5}{-5} &  3.6 & \num{2.6}{-7} &  3.1 & \num{3.1}{-7} &  6.4 & \num{6.6}{-5} &  3.6  \\ \hline
    rate             &       &  $1.81$       &      &  $1.76$       &      &  $2.27$       &      &  $1.79$       &      &  $1.80$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.AmpScf10t0p3, $t=.3$, AM=1, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=10, sm-diss=0.1  Mon Jul  3 06:48:38 2017}\label{table:insElasticPiston.epgp.AmpScf10t0p3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.TPSCF1600Imt0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{1.9}{-3} &      & \num{4.6}{-4} &      & \num{5.8}{-5} &      & \num{4.6}{-4} &      & \num{8.5}{-1} &       \\ \hline
                epg2 &     2 & \num{4.4}{-4} &  4.4 & \num{1.3}{-4} &  3.4 & \num{1.6}{-5} &  3.6 & \num{1.3}{-4} &  3.4 & \num{2.4}{-1} &  3.6  \\ \hline
                epg4 &     4 & \num{1.1}{-4} &  3.8 & \num{3.6}{-5} &  3.8 & \num{4.3}{-6} &  3.8 & \num{3.6}{-5} &  3.8 & \num{6.2}{-2} &  3.9  \\ \hline
    rate             &       &  $2.04$       &      &  $1.85$       &      &  $1.88$       &      &  $1.85$       &      &  $1.89$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.TPSCF1600Imt0p7, $t=0.7$, AM=0, cfl=.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1600, sm-diss=0.2  Tue Jul  4 10:14:56 2017}\label{table:insElasticPiston.epgp.TPSCF1600Imt0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.TPSCF8000Imt0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{1.9}{-3} &      & \num{4.6}{-4} &      & \num{5.8}{-5} &      & \num{4.6}{-4} &      & \num{4.2}{0} &       \\ \hline
                epg2 &     2 & \num{4.4}{-4} &  4.4 & \num{1.3}{-4} &  3.5 & \num{1.6}{-5} &  3.5 & \num{1.3}{-4} &  3.5 & \num{1.2}{0} &  3.6  \\ \hline
                epg4 &     4 & \num{1.1}{-4} &  3.8 & \num{3.6}{-5} &  3.7 & \num{4.3}{-6} &  3.8 & \num{3.6}{-5} &  3.7 & \num{3.1}{-1} &  3.8  \\ \hline
                epg8 &     8 & \num{2.9}{-5} &  3.9 & \num{9.2}{-6} &  3.9 & \num{1.1}{-6} &  3.8 & \num{9.2}{-6} &  3.9 & \num{8.1}{-2} &  3.8  \\ \hline
    rate             &       &  $2.00$       &      &  $1.89$       &      &  $1.91$       &      &  $1.89$       &      &  $1.91$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.TPSCF8000Imt0p7, $t=0.7$, AM=0, cfl=.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=8000, sm-diss=0.2  Tue Jul  4 10:13:35 2017}\label{table:insElasticPiston.epgp.TPSCF8000Imt0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.TPSc1600t0p7.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{1.9}{-3} &      & \num{4.6}{-4} &      & \num{5.8}{-5} &      & \num{4.6}{-4} &      & \num{8.5}{-1} &       \\ \hline
                epg2 &     2 & \num{3.0}{-4} &  6.5 & \num{1.6}{-4} &  3.0 & \num{1.0}{-5} &  5.7 & \num{1.6}{-4} &  3.0 & \num{1.7}{-1} &  5.1  \\ \hline
                epg4 &     4 & \num{7.2}{-5} &  4.1 & \num{3.9}{-5} &  4.0 & \num{3.0}{-6} &  3.5 & \num{3.9}{-5} &  4.0 & \num{4.7}{-2} &  3.5  \\ \hline
    rate             &       &  $2.38$       &      &  $1.78$       &      &  $2.15$       &      &  $1.78$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.TPSc1600t0p7, $t=.7$, AM=0, cfl=.9, nu=0.1 CgSm=SM-Godunov, tz=none, scf=1600, sm-diss=0.2  Mon Jul  3 18:44:42 2017}\label{table:insElasticPiston.epgp.TPSc1600t0p7}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.TPscf1600.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{8.3}{-4} &      & \num{3.4}{-4} &      & \num{3.0}{-5} &      & \num{3.5}{-4} &      & \num{5.6}{-1} &       \\ \hline
                epg2 &     2 & \num{2.1}{-4} &  4.0 & \num{8.1}{-5} &  4.3 & \num{9.2}{-6} &  3.3 & \num{8.1}{-5} &  4.3 & \num{1.5}{-1} &  3.7  \\ \hline
                epg4 &     4 & \num{5.2}{-5} &  3.9 & \num{1.9}{-5} &  4.1 & \num{2.5}{-6} &  3.7 & \num{1.9}{-5} &  4.1 & \num{4.0}{-2} &  3.8  \\ \hline
    rate             &       &  $1.99$       &      &  $2.07$       &      &  $1.79$       &      &  $2.08$       &      &  $1.91$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.TPscf1600, $t=.7$, AM=0, cfl=.25, nu=0.1 CGSM=SM-Godunoc, tz=none, scf=1600  Fri Jun 30 07:32:22 2017}\label{table:insElasticPiston.epgp.TPscf1600}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.TPscf1600SOSC.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r \\ \hline 
                epg1 &     1 & \num{4.4}{-3} &      & \num{1.2}{-4} &      & \num{2.8}{-4} &       \\ \hline
                epg2 &     2 & \num{1.1}{-3} &  4.2 & \num{1.6}{-5} &  7.3 & \num{7.3}{-5} &  3.8  \\ \hline
                epg4 &     4 & \num{2.8}{-4} &  3.8 & \num{3.9}{-6} &  4.2 & \num{1.9}{-5} &  3.9  \\ \hline
    rate             &       &  $2.00$       &      &  $2.46$       &      &  $1.96$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.TPscf1600SOSC, $t=.7$, AM=0, cfl=.9, nu=0.1 CGSM=SM-SOSC, tz=none, scf=1600  Fri Jun 30 07:30:14 2017}\label{table:insElasticPiston.epgp.TPscf1600SOSC}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e-3zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{2.7}{-9} &      & \num{6.5}{-9} &      & \num{1.1}{-7} &      & \num{6.4}{-11} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{6.6}{-10} &  4.1 & \num{6.4}{-10} & 10.1 & \num{2.0}{-8} &  5.4 & \num{1.1}{-11} &  5.7  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{1.7}{-10} &  4.0 & \num{7.9}{-11} &  8.1 & \num{1.5}{-9} & 13.4 & \num{1.6}{-12} &  7.0  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{4.2}{-11} &  4.0 & \num{1.9}{-11} &  4.1 & \num{2.4}{-10} &  6.3 & \num{2.1}{-13} &  7.6  \\ \hline
    rate             &       &  $-nan$       &      &  $2.01$       &      &  $2.82$       &      &  $3.02$       &      &  $2.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e-3zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 06:29:55 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e-3zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e-3zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{2.7}{-9} &      & \num{6.5}{-9} &      & \num{1.1}{-7} &      & \num{6.4}{-11} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{6.6}{-10} &  4.1 & \num{6.4}{-10} & 10.1 & \num{2.0}{-8} &  5.4 & \num{1.1}{-11} &  5.7  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{1.7}{-10} &  4.0 & \num{7.9}{-11} &  8.1 & \num{1.5}{-9} & 13.4 & \num{1.6}{-12} &  7.0  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{4.2}{-11} &  4.0 & \num{1.9}{-11} &  4.1 & \num{2.4}{-10} &  6.3 & \num{2.1}{-13} &  7.6  \\ \hline
    rate             &       &  $-nan$       &      &  $2.01$       &      &  $2.82$       &      &  $3.02$       &      &  $2.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e-3zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:06:20 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e-3zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e-3zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{2.6}{-9} &      & \num{3.0}{-9} &      & \num{5.0}{-8} &      & \num{3.2}{-11} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{6.6}{-10} &  3.9 & \num{3.8}{-10} &  7.9 & \num{9.4}{-9} &  5.3 & \num{5.3}{-12} &  6.0  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{1.7}{-10} &  4.0 & \num{5.9}{-11} &  6.5 & \num{6.1}{-10} & 15.4 & \num{6.8}{-13} &  7.8  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{4.2}{-11} &  4.0 & \num{1.7}{-11} &  3.5 & \num{8.8}{-11} &  6.9 & \num{1.4}{-13} &  4.7  \\ \hline
    rate             &       &  $-nan$       &      &  $1.99$       &      &  $2.52$       &      &  $3.14$       &      &  $2.64$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e-3zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 18:35:38 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e-3zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e-3zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{2.6}{-9} &      & \num{3.0}{-9} &      & \num{5.0}{-8} &      & \num{3.2}{-11} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{6.6}{-10} &  3.9 & \num{3.8}{-10} &  7.9 & \num{9.4}{-9} &  5.3 & \num{5.3}{-12} &  6.0  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{1.7}{-10} &  4.0 & \num{5.9}{-11} &  6.5 & \num{6.1}{-10} & 15.4 & \num{6.8}{-13} &  7.8  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{4.2}{-11} &  4.0 & \num{1.7}{-11} &  3.5 & \num{8.8}{-11} &  6.9 & \num{1.4}{-13} &  4.7  \\ \hline
    rate             &       &  $-nan$       &      &  $1.99$       &      &  $2.52$       &      &  $3.14$       &      &  $2.64$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e-3zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 16:12:57 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e-3zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e-3zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{2.7}{-9} &      & \num{6.5}{-9} &      & \num{1.1}{-7} &      & \num{6.4}{-11} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{6.6}{-10} &  4.1 & \num{6.4}{-10} & 10.1 & \num{2.0}{-8} &  5.4 & \num{1.1}{-11} &  5.7  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{1.7}{-10} &  4.0 & \num{7.9}{-11} &  8.1 & \num{1.5}{-9} & 13.4 & \num{1.6}{-12} &  7.0  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{4.2}{-11} &  4.0 & \num{1.9}{-11} &  4.1 & \num{2.4}{-10} &  6.3 & \num{2.1}{-13} &  7.6  \\ \hline
    rate             &       &  $-nan$       &      &  $2.01$       &      &  $2.82$       &      &  $3.02$       &      &  $2.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e-3zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 18:52:16 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e-3zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e3zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.1}{-4} &      & \num{1.3}{-5} &      & \num{1.1}{-4} &      & \num{5.2}{-2} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{2.2}{-5} &  5.0 & \num{2.5}{-6} &  5.3 & \num{2.2}{-5} &  5.0 & \num{8.3}{-3} &  6.2  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{5.1}{-6} &  4.3 & \num{5.0}{-7} &  5.0 & \num{5.2}{-6} &  4.3 & \num{1.5}{-3} &  5.6  \\ \hline
                epg8 &     8 & \num{6.2}{-13} &  0.0 & \num{1.2}{-6} &  4.2 & \num{1.0}{-7} &  4.8 & \num{1.3}{-6} &  4.0 & \num{2.9}{-4} &  5.1  \\ \hline
    rate             &       &  $-nan$       &      &  $2.16$       &      &  $2.33$       &      &  $2.13$       &      &  $2.49$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e3zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 06:29:17 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e3zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e3zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.0}{-4} &      & \num{1.5}{-5} &      & \num{1.0}{-4} &      & \num{5.2}{-2} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{2.2}{-5} &  4.7 & \num{2.5}{-6} &  5.9 & \num{2.2}{-5} &  4.7 & \num{8.2}{-3} &  6.4  \\ \hline
                epg4 &     4 & \num{1.4}{-13} &  0.0 & \num{5.1}{-6} &  4.3 & \num{5.0}{-7} &  5.0 & \num{5.2}{-6} &  4.2 & \num{1.5}{-3} &  5.6  \\ \hline
                epg8 &     8 & \num{2.2}{-7} &  0.0 & \num{1.2}{-6} &  4.1 & \num{1.0}{-7} &  4.8 & \num{1.3}{-6} &  4.0 & \num{2.9}{-4} &  5.1  \\ \hline
    rate             &       &  $-nan$       &      &  $2.12$       &      &  $2.38$       &      &  $2.09$       &      &  $2.49$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e3zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:05:42 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e3zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e3zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.1}{-4} &      & \num{1.3}{-5} &      & \num{1.1}{-4} &      & \num{5.2}{-2} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{2.2}{-5} &  5.0 & \num{2.5}{-6} &  5.4 & \num{2.2}{-5} &  5.0 & \num{8.4}{-3} &  6.2  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{5.1}{-6} &  4.3 & \num{5.0}{-7} &  5.0 & \num{5.2}{-6} &  4.3 & \num{1.5}{-3} &  5.6  \\ \hline
                epg8 &     8 & \num{1.6}{-13} &  0.0 & \num{1.2}{-6} &  4.2 & \num{1.0}{-7} &  4.8 & \num{1.3}{-6} &  4.0 & \num{3.0}{-4} &  5.1  \\ \hline
    rate             &       &  $-nan$       &      &  $2.16$       &      &  $2.33$       &      &  $2.13$       &      &  $2.49$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e3zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 18:34:57 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e3zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e3zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.1}{-4} &      & \num{1.4}{-5} &      & \num{1.1}{-4} &      & \num{5.2}{-2} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{2.2}{-5} &  5.0 & \num{2.5}{-6} &  5.5 & \num{2.2}{-5} &  4.9 & \num{8.4}{-3} &  6.2  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{5.1}{-6} &  4.3 & \num{5.0}{-7} &  5.0 & \num{5.2}{-6} &  4.2 & \num{1.5}{-3} &  5.6  \\ \hline
                epg8 &     8 & \num{0.0}{1} &  0.0 & \num{1.2}{-6} &  4.2 & \num{1.0}{-7} &  4.8 & \num{1.3}{-6} &  4.0 & \num{3.0}{-4} &  5.1  \\ \hline
    rate             &       &  $-nan$       &      &  $2.15$       &      &  $2.35$       &      &  $2.12$       &      &  $2.49$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e3zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 16:12:15 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e3zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgp.shearAmpSCF1e3zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                epg1 &     1 & \num{0.0}{1} &      & \num{1.1}{-4} &      & \num{1.3}{-5} &      & \num{1.1}{-4} &      & \num{5.2}{-2} &       \\ \hline
                epg2 &     2 & \num{0.0}{1} &  0.0 & \num{2.2}{-5} &  5.0 & \num{2.5}{-6} &  5.3 & \num{2.2}{-5} &  5.0 & \num{8.4}{-3} &  6.2  \\ \hline
                epg4 &     4 & \num{0.0}{1} &  0.0 & \num{5.1}{-6} &  4.3 & \num{5.0}{-7} &  5.0 & \num{5.2}{-6} &  4.2 & \num{1.5}{-3} &  5.6  \\ \hline
                epg8 &     8 & \num{2.3}{-12} &  0.0 & \num{1.2}{-6} &  4.2 & \num{1.0}{-7} &  4.8 & \num{1.3}{-6} &  4.0 & \num{3.0}{-4} &  5.1  \\ \hline
    rate             &       &  $-nan$       &      &  $2.16$       &      &  $2.33$       &      &  $2.13$       &      &  $2.49$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgp.shearAmpSCF1e3zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=10 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 18:51:39 2018}\label{table:insElasticPiston.epgp.shearAmpSCF1e3zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1Imtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.2}{-4} &      & \num{3.8}{-4} &      & \num{3.3}{-4} &      & \num{9.5}{-4} &      & \num{2.0}{-3} &       \\ \hline
               epgN2 &     2 & \num{2.1}{-5} &  5.7 & \num{6.9}{-5} &  5.5 & \num{6.7}{-5} &  5.0 & \num{1.2}{-4} &  8.2 & \num{7.4}{-4} &  2.7  \\ \hline
    rate             &       &  $2.51$       &      &  $2.46$       &      &  $2.31$       &      &  $3.03$       &      &  $1.44$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1Imtp3, $t=.3$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 13:22:32 2018}\label{table:insElasticPiston.epgpN.AmpSCF1Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{7.3}{-3} &      & \num{7.3}{-4} &      & \num{9.4}{-4} &      & \num{9.3}{-4} &      & \num{5.9}{-3} &       \\ \hline
               epgN2 &     2 & \num{1.8}{-3} &  4.1 & \num{2.4}{-4} &  3.1 & \num{2.3}{-4} &  4.0 & \num{2.4}{-4} &  3.9 & \num{1.5}{-3} &  4.0  \\ \hline
               epgN4 &     4 & \num{4.4}{-4} &  4.1 & \num{7.1}{-5} &  3.4 & \num{5.8}{-5} &  4.1 & \num{7.1}{-5} &  3.4 & \num{3.5}{-4} &  4.2  \\ \hline
               epgN8 &     8 & \num{1.1}{-4} &  4.1 & \num{1.9}{-5} &  3.7 & \num{1.4}{-5} &  4.0 & \num{1.9}{-5} &  3.7 & \num{8.8}{-5} &  4.0  \\ \hline
    rate             &       &  $2.03$       &      &  $1.75$       &      &  $2.01$       &      &  $1.86$       &      &  $2.03$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 13:41:30 2018}\label{table:insElasticPiston.epgpN.AmpSCF1Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e-3Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.1}{-3} &      & \num{4.4}{-4} &      & \num{7.5}{-4} &      & \num{4.4}{-4} &      & \num{8.6}{-6} &       \\ \hline
               epgN2 &     2 & \num{3.1}{-4} &  3.6 & \num{1.2}{-4} &  3.5 & \num{2.1}{-4} &  3.6 & \num{1.5}{-4} &  2.8 & \num{1.8}{-6} &  4.8  \\ \hline
               epgN4 &     4 & \num{8.0}{-5} &  3.9 & \num{3.2}{-5} &  3.8 & \num{5.4}{-5} &  3.9 & \num{3.2}{-5} &  4.7 & \num{4.2}{-7} &  4.2  \\ \hline
               epgN8 &     8 & \num{2.0}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.4}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $1.92$       &      &  $1.91$       &      &  $1.93$       &      &  $1.94$       &      &  $2.12$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e-3Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 13:41:55 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e-3Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e-3zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.1}{-3} &      & \num{4.4}{-4} &      & \num{7.4}{-4} &      & \num{4.4}{-4} &      & \num{8.6}{-6} &       \\ \hline
               epgN2 &     2 & \num{3.1}{-4} &  3.6 & \num{1.2}{-4} &  3.5 & \num{2.1}{-4} &  3.6 & \num{1.5}{-4} &  2.8 & \num{1.8}{-6} &  4.8  \\ \hline
               epgN4 &     4 & \num{8.0}{-5} &  3.9 & \num{3.2}{-5} &  3.8 & \num{5.4}{-5} &  3.9 & \num{3.2}{-5} &  4.7 & \num{4.2}{-7} &  4.2  \\ \hline
               epgN8 &     8 & \num{2.0}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.4}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $1.92$       &      &  $1.91$       &      &  $1.92$       &      &  $1.94$       &      &  $2.12$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e-3zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 06:19:57 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e-3zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e-3zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.1}{-3} &      & \num{4.4}{-4} &      & \num{7.5}{-4} &      & \num{4.4}{-4} &      & \num{8.6}{-6} &       \\ \hline
               epgN2 &     2 & \num{3.1}{-4} &  3.6 & \num{1.2}{-4} &  3.5 & \num{2.1}{-4} &  3.6 & \num{1.5}{-4} &  2.8 & \num{1.8}{-6} &  4.9  \\ \hline
               epgN4 &     4 & \num{8.0}{-5} &  3.9 & \num{3.2}{-5} &  3.8 & \num{5.4}{-5} &  3.9 & \num{3.2}{-5} &  4.7 & \num{4.2}{-7} &  4.2  \\ \hline
               epgN8 &     8 & \num{2.0}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.4}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $1.92$       &      &  $1.91$       &      &  $1.93$       &      &  $1.94$       &      &  $2.12$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e-3zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:05:08 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e-3zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e-3zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.1}{-3} &      & \num{4.4}{-4} &      & \num{7.4}{-4} &      & \num{4.4}{-4} &      & \num{8.6}{-6} &       \\ \hline
               epgN2 &     2 & \num{3.1}{-4} &  3.6 & \num{1.2}{-4} &  3.5 & \num{2.1}{-4} &  3.6 & \num{1.5}{-4} &  2.8 & \num{1.8}{-6} &  4.8  \\ \hline
               epgN4 &     4 & \num{8.0}{-5} &  3.9 & \num{3.2}{-5} &  3.8 & \num{5.4}{-5} &  3.9 & \num{3.2}{-5} &  4.7 & \num{4.2}{-7} &  4.2  \\ \hline
               epgN8 &     8 & \num{2.0}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.4}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $1.92$       &      &  $1.91$       &      &  $1.92$       &      &  $1.94$       &      &  $2.12$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e-3zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 15:46:40 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e-3zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e-3zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.1}{-3} &      & \num{4.4}{-4} &      & \num{7.5}{-4} &      & \num{4.4}{-4} &      & \num{8.6}{-6} &       \\ \hline
               epgN2 &     2 & \num{3.1}{-4} &  3.6 & \num{1.2}{-4} &  3.5 & \num{2.1}{-4} &  3.6 & \num{1.5}{-4} &  2.8 & \num{1.8}{-6} &  4.8  \\ \hline
               epgN4 &     4 & \num{8.0}{-5} &  3.9 & \num{3.2}{-5} &  3.8 & \num{5.4}{-5} &  3.9 & \num{3.2}{-5} &  4.7 & \num{4.2}{-7} &  4.2  \\ \hline
               epgN8 &     8 & \num{2.0}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.4}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $1.92$       &      &  $1.91$       &      &  $1.93$       &      &  $1.94$       &      &  $2.12$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e-3zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 15:44:05 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e-3zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e-3zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.1}{-3} &      & \num{4.4}{-4} &      & \num{7.5}{-4} &      & \num{4.4}{-4} &      & \num{8.6}{-6} &       \\ \hline
               epgN2 &     2 & \num{3.1}{-4} &  3.6 & \num{1.2}{-4} &  3.5 & \num{2.1}{-4} &  3.6 & \num{1.5}{-4} &  2.8 & \num{1.8}{-6} &  4.9  \\ \hline
               epgN4 &     4 & \num{8.0}{-5} &  3.9 & \num{3.2}{-5} &  3.8 & \num{5.4}{-5} &  3.9 & \num{3.2}{-5} &  4.7 & \num{4.2}{-7} &  4.2  \\ \hline
               epgN8 &     8 & \num{2.0}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.4}{-5} &  3.9 & \num{8.3}{-6} &  3.9 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $1.92$       &      &  $1.91$       &      &  $1.93$       &      &  $1.94$       &      &  $2.12$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e-3zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 18:51:14 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e-3zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e3Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{2.9}{-2} &      & \num{4.2}{-3} &      & \num{9.2}{-4} &      & \num{4.2}{-3} &      & \num{6.8}{0} &       \\ \hline
               epgN2 &     2 & \num{7.4}{-3} &  4.0 & \num{1.1}{-3} &  3.7 & \num{1.9}{-4} &  4.8 & \num{1.1}{-3} &  3.7 & \num{1.7}{0} &  4.1  \\ \hline
               epgN4 &     4 & \num{1.8}{-3} &  4.0 & \num{2.9}{-4} &  3.9 & \num{4.2}{-5} &  4.6 & \num{2.9}{-4} &  3.9 & \num{3.9}{-1} &  4.3  \\ \hline
               epgN8 &     8 & \num{4.5}{-4} &  4.1 & \num{7.4}{-5} &  4.0 & \num{9.6}{-6} &  4.3 & \num{7.4}{-5} &  4.0 & \num{9.1}{-2} &  4.3  \\ \hline
    rate             &       &  $2.01$       &      &  $1.94$       &      &  $2.20$       &      &  $1.94$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e3Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 13:41:43 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e3Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e3zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{2.9}{-2} &      & \num{4.2}{-3} &      & \num{9.2}{-4} &      & \num{4.2}{-3} &      & \num{6.8}{0} &       \\ \hline
               epgN2 &     2 & \num{7.3}{-3} &  4.0 & \num{1.1}{-3} &  3.7 & \num{1.9}{-4} &  4.8 & \num{1.1}{-3} &  3.7 & \num{1.7}{0} &  4.1  \\ \hline
               epgN4 &     4 & \num{1.8}{-3} &  4.1 & \num{3.0}{-4} &  3.9 & \num{4.2}{-5} &  4.6 & \num{3.0}{-4} &  3.9 & \num{3.9}{-1} &  4.3  \\ \hline
               epgN8 &     8 & \num{4.2}{-4} &  4.2 & \num{7.5}{-5} &  4.0 & \num{9.6}{-6} &  4.3 & \num{7.5}{-5} &  4.0 & \num{9.1}{-2} &  4.3  \\ \hline
    rate             &       &  $2.04$       &      &  $1.94$       &      &  $2.20$       &      &  $1.94$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e3zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 06:19:45 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e3zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e3zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{3.0}{-2} &      & \num{4.2}{-3} &      & \num{9.2}{-4} &      & \num{4.2}{-3} &      & \num{6.8}{0} &       \\ \hline
               epgN2 &     2 & \num{7.5}{-3} &  4.0 & \num{1.1}{-3} &  3.7 & \num{1.9}{-4} &  4.8 & \num{1.1}{-3} &  3.7 & \num{1.7}{0} &  4.1  \\ \hline
               epgN4 &     4 & \num{1.8}{-3} &  4.1 & \num{3.0}{-4} &  3.9 & \num{4.2}{-5} &  4.6 & \num{3.0}{-4} &  3.9 & \num{3.9}{-1} &  4.3  \\ \hline
               epgN8 &     8 & \num{4.4}{-4} &  4.1 & \num{7.4}{-5} &  4.0 & \num{9.6}{-6} &  4.3 & \num{7.5}{-5} &  4.0 & \num{9.1}{-2} &  4.3  \\ \hline
    rate             &       &  $2.02$       &      &  $1.94$       &      &  $2.20$       &      &  $1.94$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e3zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:04:56 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e3zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e3zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{2.9}{-2} &      & \num{4.2}{-3} &      & \num{9.2}{-4} &      & \num{4.2}{-3} &      & \num{6.8}{0} &       \\ \hline
               epgN2 &     2 & \num{7.4}{-3} &  4.0 & \num{1.1}{-3} &  3.7 & \num{1.9}{-4} &  4.8 & \num{1.1}{-3} &  3.7 & \num{1.7}{0} &  4.1  \\ \hline
               epgN4 &     4 & \num{1.8}{-3} &  4.0 & \num{2.9}{-4} &  3.9 & \num{4.2}{-5} &  4.6 & \num{2.9}{-4} &  3.9 & \num{3.9}{-1} &  4.3  \\ \hline
               epgN8 &     8 & \num{4.5}{-4} &  4.1 & \num{7.4}{-5} &  4.0 & \num{9.6}{-6} &  4.3 & \num{7.4}{-5} &  4.0 & \num{9.1}{-2} &  4.3  \\ \hline
    rate             &       &  $2.01$       &      &  $1.94$       &      &  $2.20$       &      &  $1.94$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e3zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 15:46:27 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e3zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e3zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{2.9}{-2} &      & \num{4.2}{-3} &      & \num{9.2}{-4} &      & \num{4.2}{-3} &      & \num{6.8}{0} &       \\ \hline
               epgN2 &     2 & \num{7.4}{-3} &  4.0 & \num{1.1}{-3} &  3.7 & \num{1.9}{-4} &  4.8 & \num{1.1}{-3} &  3.7 & \num{1.7}{0} &  4.1  \\ \hline
               epgN4 &     4 & \num{1.8}{-3} &  4.0 & \num{2.9}{-4} &  3.9 & \num{4.2}{-5} &  4.6 & \num{2.9}{-4} &  3.9 & \num{3.9}{-1} &  4.3  \\ \hline
               epgN8 &     8 & \num{4.5}{-4} &  4.1 & \num{7.4}{-5} &  4.0 & \num{9.6}{-6} &  4.3 & \num{7.4}{-5} &  4.0 & \num{9.1}{-2} &  4.3  \\ \hline
    rate             &       &  $2.01$       &      &  $1.94$       &      &  $2.20$       &      &  $1.94$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e3zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 15:43:52 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e3zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1e3zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{3.0}{-2} &      & \num{4.2}{-3} &      & \num{9.2}{-4} &      & \num{4.2}{-3} &      & \num{6.8}{0} &       \\ \hline
               epgN2 &     2 & \num{7.4}{-3} &  4.0 & \num{1.1}{-3} &  3.7 & \num{1.9}{-4} &  4.8 & \num{1.1}{-3} &  3.7 & \num{1.7}{0} &  4.1  \\ \hline
               epgN4 &     4 & \num{1.8}{-3} &  4.1 & \num{2.9}{-4} &  3.9 & \num{4.2}{-5} &  4.6 & \num{2.9}{-4} &  3.9 & \num{3.9}{-1} &  4.3  \\ \hline
               epgN8 &     8 & \num{4.4}{-4} &  4.1 & \num{7.4}{-5} &  4.0 & \num{9.6}{-6} &  4.3 & \num{7.4}{-5} &  4.0 & \num{9.1}{-2} &  4.3  \\ \hline
    rate             &       &  $2.02$       &      &  $1.94$       &      &  $2.20$       &      &  $1.94$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1e3zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 18:51:01 2018}\label{table:insElasticPiston.epgpN.AmpSCF1e3zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{3.4}{-3} &      & \num{2.2}{-3} &      & \num{1.0}{-3} &      & \num{3.2}{-3} &      & \num{8.7}{-3} &       \\ \hline
               epgN2 &     2 & \num{1.3}{-3} &  2.6 & \num{3.0}{-4} &  7.1 & \num{2.1}{-4} &  5.0 & \num{5.2}{-4} &  6.2 & \num{1.2}{-3} &  7.4  \\ \hline
               epgN4 &     4 & \num{4.3}{-4} &  3.0 & \num{6.8}{-5} &  4.5 & \num{5.7}{-5} &  3.7 & \num{7.2}{-5} &  7.2 & \num{3.5}{-4} &  3.4  \\ \hline
               epgN8 &     8 & \num{1.1}{-4} &  4.0 & \num{1.9}{-5} &  3.6 & \num{1.4}{-5} &  4.0 & \num{1.9}{-5} &  3.8 & \num{8.8}{-5} &  3.9  \\ \hline
    rate             &       &  $1.65$       &      &  $2.27$       &      &  $2.04$       &      &  $2.51$       &      &  $2.16$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 06:19:33 2018}\label{table:insElasticPiston.epgpN.AmpSCF1zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{1.0}{-2} &      & \num{5.8}{-4} &      & \num{9.9}{-4} &      & \num{4.0}{-4} &      & \num{8.8}{-3} &       \\ \hline
               epgN2 &     2 & \num{1.9}{-3} &  5.2 & \num{2.5}{-4} &  2.3 & \num{2.4}{-4} &  4.1 & \num{2.4}{-4} &  1.7 & \num{1.6}{-3} &  5.7  \\ \hline
               epgN4 &     4 & \num{4.4}{-4} &  4.4 & \num{7.3}{-5} &  3.5 & \num{5.8}{-5} &  4.1 & \num{7.2}{-5} &  3.3 & \num{3.5}{-4} &  4.4  \\ \hline
               epgN8 &     8 & \num{1.1}{-4} &  4.1 & \num{1.9}{-5} &  3.8 & \num{1.4}{-5} &  4.1 & \num{1.9}{-5} &  3.8 & \num{8.8}{-5} &  4.0  \\ \hline
    rate             &       &  $2.17$       &      &  $1.65$       &      &  $2.04$       &      &  $1.48$       &      &  $2.21$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:04:44 2018}\label{table:insElasticPiston.epgpN.AmpSCF1zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{3.5}{-3} &      & \num{1.5}{-3} &      & \num{8.9}{-4} &      & \num{2.6}{-3} &      & \num{5.8}{-3} &       \\ \hline
               epgN2 &     2 & \num{1.7}{-3} &  2.1 & \num{2.5}{-4} &  5.9 & \num{2.3}{-4} &  3.9 & \num{2.8}{-4} &  9.3 & \num{1.4}{-3} &  4.2  \\ \hline
               epgN4 &     4 & \num{4.4}{-4} &  3.9 & \num{7.0}{-5} &  3.6 & \num{5.8}{-5} &  4.0 & \num{7.1}{-5} &  3.9 & \num{3.5}{-4} &  4.0  \\ \hline
               epgN8 &     8 & \num{1.1}{-4} &  4.0 & \num{1.9}{-5} &  3.7 & \num{1.4}{-5} &  4.0 & \num{1.9}{-5} &  3.7 & \num{8.8}{-5} &  4.0  \\ \hline
    rate             &       &  $1.71$       &      &  $2.08$       &      &  $1.99$       &      &  $2.32$       &      &  $2.01$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 15:46:14 2018}\label{table:insElasticPiston.epgpN.AmpSCF1zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{7.3}{-3} &      & \num{7.3}{-4} &      & \num{9.4}{-4} &      & \num{9.3}{-4} &      & \num{5.9}{-3} &       \\ \hline
               epgN2 &     2 & \num{1.8}{-3} &  4.1 & \num{2.4}{-4} &  3.1 & \num{2.3}{-4} &  4.0 & \num{2.4}{-4} &  3.9 & \num{1.5}{-3} &  4.0  \\ \hline
               epgN4 &     4 & \num{4.4}{-4} &  4.1 & \num{7.1}{-5} &  3.4 & \num{5.8}{-5} &  4.1 & \num{7.1}{-5} &  3.4 & \num{3.5}{-4} &  4.2  \\ \hline
               epgN8 &     8 & \num{1.1}{-4} &  4.1 & \num{1.9}{-5} &  3.7 & \num{1.4}{-5} &  4.0 & \num{1.9}{-5} &  3.7 & \num{8.8}{-5} &  4.0  \\ \hline
    rate             &       &  $2.03$       &      &  $1.75$       &      &  $2.01$       &      &  $1.86$       &      &  $2.03$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 15:43:40 2018}\label{table:insElasticPiston.epgpN.AmpSCF1zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.epgpN.AmpSCF1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
               epgN1 &     1 & \num{9.9}{-3} &      & \num{5.7}{-4} &      & \num{9.9}{-4} &      & \num{3.3}{-4} &      & \num{8.7}{-3} &       \\ \hline
               epgN2 &     2 & \num{1.9}{-3} &  5.2 & \num{2.5}{-4} &  2.3 & \num{2.4}{-4} &  4.1 & \num{2.4}{-4} &  1.4 & \num{1.6}{-3} &  5.5  \\ \hline
               epgN4 &     4 & \num{4.4}{-4} &  4.4 & \num{7.2}{-5} &  3.5 & \num{5.8}{-5} &  4.1 & \num{7.2}{-5} &  3.3 & \num{3.5}{-4} &  4.4  \\ \hline
               epgN8 &     8 & \num{1.1}{-4} &  4.1 & \num{1.9}{-5} &  3.8 & \num{1.4}{-5} &  4.1 & \num{1.9}{-5} &  3.8 & \num{8.8}{-5} &  4.0  \\ \hline
    rate             &       &  $2.17$       &      &  $1.65$       &      &  $2.04$       &      &  $1.40$       &      &  $2.20$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.epgpN.AmpSCF1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=0 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 18:50:49 2018}\label{table:insElasticPiston.epgpN.AmpSCF1zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF0p1Imtp3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{4.2}{-3} &      & \num{2.1}{-3} &      & \num{1.0}{-4} &      & \num{8.3}{-4} &      & \num{2.7}{-4} &       \\ \hline
                rep2 &     2 & \num{9.6}{-4} &  4.4 & \num{5.3}{-4} &  4.1 & \num{1.5}{-5} &  6.7 & \num{1.4}{-4} &  5.7 & \num{4.4}{-5} &  6.1  \\ \hline
                rep4 &     4 & \num{2.1}{-4} &  4.5 & \num{1.5}{-4} &  3.4 & \num{3.6}{-6} &  4.2 & \num{3.4}{-5} &  4.2 & \num{1.2}{-5} &  3.7  \\ \hline
                rep8 &     8 & \num{4.8}{-5} &  4.4 & \num{3.9}{-5} &  4.0 & \num{1.1}{-6} &  3.3 & \num{9.0}{-6} &  3.8 & \num{3.6}{-6} &  3.3  \\ \hline
    rate             &       &  $2.15$       &      &  $1.92$       &      &  $2.17$       &      &  $2.17$       &      &  $2.05$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF0p1Imtp3, $t=.3$, AM=1, cfl=.9, nu=.01 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.1, sm-diss=0.2  Mon Jul 10 07:07:09 2017}\label{table:insElasticPiston.rep.AmpSCF0p1Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1Imtp3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{4.2}{-3} &      & \num{2.4}{-3} &      & \num{1.0}{-4} &      & \num{7.9}{-4} &      & \num{1.8}{-3} &       \\ \hline
                rep2 &     2 & \num{9.9}{-4} &  4.2 & \num{5.3}{-4} &  4.6 & \num{1.6}{-5} &  6.6 & \num{1.4}{-4} &  5.7 & \num{4.4}{-4} &  4.1  \\ \hline
                rep4 &     4 & \num{2.2}{-4} &  4.4 & \num{1.6}{-4} &  3.3 & \num{3.7}{-6} &  4.2 & \num{3.3}{-5} &  4.2 & \num{1.2}{-4} &  3.7  \\ \hline
                rep8 &     8 & \num{5.1}{-5} &  4.3 & \num{4.4}{-5} &  3.7 & \num{1.1}{-6} &  3.4 & \num{8.7}{-6} &  3.8 & \num{3.6}{-5} &  3.3  \\ \hline
    rate             &       &  $2.12$       &      &  $1.91$       &      &  $2.17$       &      &  $2.16$       &      &  $1.88$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1Imtp3, $t=.3$, AM=1, cfl=.9, nu=.01 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, sm-diss=0.2  Mon Jul 10 07:02:09 2017}\label{table:insElasticPiston.rep.AmpSCF1Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e-3zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.5}{-3} &      & \num{2.4}{-2} &      & \num{1.5}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  9.1 & \num{4.9}{-4} &  3.8 & \num{3.6}{-4} & 12.3 & \num{6.6}{-3} &  3.6 & \num{1.8}{-5} &  8.1  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.7}{-5} &  4.2 & \num{7.9}{-4} &  8.4 & \num{4.1}{-6} &  4.5  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  3.9 & \num{2.5}{-5} &  4.1 & \num{2.3}{-5} &  3.9 & \num{3.1}{-4} &  2.6 & \num{4.4}{-7} &  9.3  \\ \hline
    rate             &       &  $2.41$       &      &  $2.08$       &      &  $2.49$       &      &  $2.19$       &      &  $2.74$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 16:26:43 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e-3zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.5}{-3} &      & \num{2.4}{-2} &      & \num{1.5}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  9.1 & \num{4.9}{-4} &  3.8 & \num{3.6}{-4} & 12.3 & \num{6.7}{-3} &  3.5 & \num{1.8}{-5} &  8.2  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.7}{-5} &  4.2 & \num{7.9}{-4} &  8.4 & \num{4.1}{-6} &  4.5  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  3.9 & \num{2.5}{-5} &  4.1 & \num{2.3}{-5} &  3.9 & \num{3.1}{-4} &  2.6 & \num{4.4}{-7} &  9.3  \\ \hline
    rate             &       &  $2.41$       &      &  $2.08$       &      &  $2.49$       &      &  $2.19$       &      &  $2.74$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:10:44 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e-3zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{4.0}{-3} &      & \num{5.8}{-3} &      & \num{5.2}{-2} &      & \num{3.9}{-1} &      & \num{1.9}{-3} &       \\ \hline
                rep2 &     2 & \num{3.6}{-4} & 11.1 & \num{7.5}{-4} &  7.8 & \num{1.8}{-3} & 29.4 & \num{4.2}{-2} &  9.3 & \num{9.0}{-5} & 21.1  \\ \hline
                rep4 &     4 & \num{7.2}{-5} &  5.0 & \num{1.2}{-4} &  6.0 & \num{2.3}{-4} &  7.7 & \num{4.5}{-3} &  9.5 & \num{1.7}{-5} &  5.4  \\ \hline
                rep8 &     8 & \num{1.1}{-5} &  6.5 & \num{2.7}{-5} &  4.6 & \num{3.2}{-5} &  7.0 & \num{1.8}{-3} &  2.5 & \num{1.3}{-6} & 13.3  \\ \hline
    rate             &       &  $2.78$       &      &  $2.58$       &      &  $3.49$       &      &  $2.66$       &      &  $3.41$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 18:53:55 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e-3zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{4.0}{-3} &      & \num{5.8}{-3} &      & \num{5.2}{-2} &      & \num{3.9}{-1} &      & \num{1.9}{-3} &       \\ \hline
                rep2 &     2 & \num{3.6}{-4} & 11.1 & \num{7.5}{-4} &  7.8 & \num{1.8}{-3} & 29.4 & \num{4.2}{-2} &  9.3 & \num{9.0}{-5} & 21.1  \\ \hline
                rep4 &     4 & \num{7.2}{-5} &  5.0 & \num{1.2}{-4} &  6.0 & \num{2.3}{-4} &  7.7 & \num{4.5}{-3} &  9.5 & \num{1.7}{-5} &  5.4  \\ \hline
                rep8 &     8 & \num{1.1}{-5} &  6.5 & \num{2.7}{-5} &  4.6 & \num{3.2}{-5} &  7.0 & \num{1.8}{-3} &  2.5 & \num{1.3}{-6} & 13.3  \\ \hline
    rate             &       &  $2.78$       &      &  $2.58$       &      &  $3.49$       &      &  $2.66$       &      &  $3.41$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 18:45:18 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e-3zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.5}{-3} &      & \num{2.4}{-2} &      & \num{1.5}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  9.1 & \num{4.9}{-4} &  3.8 & \num{3.6}{-4} & 12.3 & \num{6.7}{-3} &  3.5 & \num{1.8}{-5} &  8.2  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.7}{-5} &  4.2 & \num{7.9}{-4} &  8.4 & \num{4.1}{-6} &  4.5  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  3.9 & \num{2.5}{-5} &  4.1 & \num{2.3}{-5} &  3.9 & \num{3.1}{-4} &  2.6 & \num{4.4}{-7} &  9.3  \\ \hline
    rate             &       &  $2.41$       &      &  $2.08$       &      &  $2.49$       &      &  $2.19$       &      &  $2.74$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 19:01:47 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e3zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.4}{-2} &      & \num{1.3}{-2} &      & \num{5.0}{-4} &      & \num{5.9}{-3} &      & \num{5.7}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.7 & \num{1.3}{-3} & 10.0 & \num{1.2}{-4} &  4.2 & \num{1.4}{-3} &  4.4 & \num{1.6}{0} &  3.7  \\ \hline
                rep4 &     4 & \num{6.4}{-4} &  2.8 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.7}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{1.1}{-5} & 58.5 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.6 & \num{9.7}{-5} &  3.8 & \num{9.9}{-2} &  3.7  \\ \hline
    rate             &       &  $3.24$       &      &  $2.32$       &      &  $2.02$       &      &  $1.97$       &      &  $1.96$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 16:24:54 2018}\label{table:insElasticPiston.rep.AmpSCF1e3zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e3zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.4}{-2} &      & \num{1.3}{-2} &      & \num{4.9}{-4} &      & \num{5.9}{-3} &      & \num{5.7}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.8 & \num{1.3}{-3} & 10.0 & \num{1.2}{-4} &  4.3 & \num{1.4}{-3} &  4.4 & \num{1.6}{0} &  3.7  \\ \hline
                rep4 &     4 & \num{6.5}{-4} &  2.8 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.7}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{2.0}{-5} & 31.9 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.6 & \num{9.7}{-5} &  3.8 & \num{9.8}{-2} &  3.8  \\ \hline
    rate             &       &  $2.97$       &      &  $2.32$       &      &  $2.03$       &      &  $1.97$       &      &  $1.97$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:08:56 2018}\label{table:insElasticPiston.rep.AmpSCF1e3zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e3zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.4}{-2} &      & \num{1.3}{-2} &      & \num{4.9}{-4} &      & \num{5.9}{-3} &      & \num{5.7}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.8 & \num{1.3}{-3} & 10.0 & \num{1.2}{-4} &  4.3 & \num{1.4}{-3} &  4.4 & \num{1.6}{0} &  3.7  \\ \hline
                rep4 &     4 & \num{6.5}{-4} &  2.8 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.7}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{2.0}{-5} & 31.9 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.6 & \num{9.7}{-5} &  3.8 & \num{9.8}{-2} &  3.8  \\ \hline
    rate             &       &  $2.97$       &      &  $2.32$       &      &  $2.03$       &      &  $1.97$       &      &  $1.97$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 18:52:01 2018}\label{table:insElasticPiston.rep.AmpSCF1e3zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e3zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.4}{-2} &      & \num{1.3}{-2} &      & \num{4.9}{-4} &      & \num{5.9}{-3} &      & \num{5.7}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.8 & \num{1.3}{-3} & 10.0 & \num{1.2}{-4} &  4.3 & \num{1.4}{-3} &  4.4 & \num{1.6}{0} &  3.7  \\ \hline
                rep4 &     4 & \num{6.5}{-4} &  2.8 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.7}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{2.0}{-5} & 31.9 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.6 & \num{9.7}{-5} &  3.8 & \num{9.8}{-2} &  3.8  \\ \hline
    rate             &       &  $2.97$       &      &  $2.32$       &      &  $2.03$       &      &  $1.97$       &      &  $1.97$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 18:43:24 2018}\label{table:insElasticPiston.rep.AmpSCF1e3zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1e3zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.4}{-2} &      & \num{1.3}{-2} &      & \num{4.9}{-4} &      & \num{5.9}{-3} &      & \num{5.7}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.8 & \num{1.3}{-3} & 10.0 & \num{1.2}{-4} &  4.3 & \num{1.4}{-3} &  4.4 & \num{1.6}{0} &  3.7  \\ \hline
                rep4 &     4 & \num{6.5}{-4} &  2.8 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.7}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{1.9}{-5} & 33.9 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.6 & \num{9.7}{-5} &  3.8 & \num{9.8}{-2} &  3.8  \\ \hline
    rate             &       &  $3.00$       &      &  $2.32$       &      &  $2.03$       &      &  $1.97$       &      &  $1.97$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 18:59:59 2018}\label{table:insElasticPiston.rep.AmpSCF1e3zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{2.0}{-2} &      & \num{1.4}{-2} &      & \num{2.6}{-3} &      & \num{4.4}{-3} &      & \num{2.5}{-2} &       \\ \hline
                rep2 &     2 & \num{7.4}{-4} & 27.5 & \num{1.7}{-3} &  8.5 & \num{7.4}{-5} & 34.6 & \num{1.6}{-3} &  2.7 & \num{1.0}{-3} & 24.2  \\ \hline
                rep4 &     4 & \num{2.3}{-4} &  3.2 & \num{4.0}{-4} &  4.2 & \num{1.7}{-5} &  4.3 & \num{3.9}{-4} &  4.2 & \num{3.2}{-4} &  3.3  \\ \hline
                rep8 &     8 & \num{6.4}{-5} &  3.6 & \num{1.0}{-4} &  4.0 & \num{4.8}{-6} &  3.6 & \num{9.9}{-5} &  4.0 & \num{8.8}{-5} &  3.6  \\ \hline
    rate             &       &  $2.66$       &      &  $2.35$       &      &  $2.93$       &      &  $1.85$       &      &  $2.62$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 16:23:08 2018}\label{table:insElasticPiston.rep.AmpSCF1zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1zf100+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{7.7}{-3} &      & \num{1.1}{-2} &      & \num{1.4}{-3} &      & \num{9.5}{-3} &      & \num{1.2}{-2} &       \\ \hline
                rep2 &     2 & \num{8.7}{-4} &  8.8 & \num{1.7}{-3} &  6.3 & \num{7.5}{-5} & 18.8 & \num{1.6}{-3} &  5.9 & \num{1.1}{-3} & 10.7  \\ \hline
                rep4 &     4 & \num{2.6}{-4} &  3.3 & \num{4.0}{-4} &  4.2 & \num{1.8}{-5} &  4.0 & \num{3.8}{-4} &  4.2 & \num{3.4}{-4} &  3.4  \\ \hline
                rep8 &     8 & \num{6.5}{-5} &  4.1 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.8 & \num{9.9}{-5} &  3.9 & \num{8.9}{-5} &  3.8  \\ \hline
    rate             &       &  $2.24$       &      &  $2.22$       &      &  $2.65$       &      &  $2.18$       &      &  $2.31$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1zf100+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=100 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Aug 11 20:07:10 2018}\label{table:insElasticPiston.rep.AmpSCF1zf100+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{5.9}{-3} &      & \num{1.1}{-2} &      & \num{1.4}{-3} &      & \num{9.5}{-3} &      & \num{1.3}{-2} &       \\ \hline
                rep2 &     2 & \num{7.9}{-4} &  7.4 & \num{1.7}{-3} &  6.3 & \num{7.7}{-5} & 18.5 & \num{1.6}{-3} &  5.8 & \num{1.1}{-3} & 11.8  \\ \hline
                rep4 &     4 & \num{2.5}{-4} &  3.1 & \num{4.0}{-4} &  4.2 & \num{1.9}{-5} &  4.1 & \num{3.8}{-4} &  4.2 & \num{3.3}{-4} &  3.3  \\ \hline
                rep8 &     8 & \num{6.6}{-5} &  3.8 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.8 & \num{9.9}{-5} &  3.9 & \num{9.0}{-5} &  3.7  \\ \hline
    rate             &       &  $2.11$       &      &  $2.22$       &      &  $2.66$       &      &  $2.18$       &      &  $2.33$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 18:50:08 2018}\label{table:insElasticPiston.rep.AmpSCF1zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{5.9}{-3} &      & \num{1.1}{-2} &      & \num{1.4}{-3} &      & \num{9.5}{-3} &      & \num{1.3}{-2} &       \\ \hline
                rep2 &     2 & \num{7.9}{-4} &  7.4 & \num{1.7}{-3} &  6.3 & \num{7.7}{-5} & 18.5 & \num{1.6}{-3} &  5.8 & \num{1.1}{-3} & 11.8  \\ \hline
                rep4 &     4 & \num{2.5}{-4} &  3.1 & \num{4.0}{-4} &  4.2 & \num{1.9}{-5} &  4.1 & \num{3.8}{-4} &  4.2 & \num{3.3}{-4} &  3.3  \\ \hline
                rep8 &     8 & \num{6.6}{-5} &  3.8 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.8 & \num{9.9}{-5} &  3.9 & \num{9.0}{-5} &  3.7  \\ \hline
    rate             &       &  $2.11$       &      &  $2.22$       &      &  $2.66$       &      &  $2.18$       &      &  $2.33$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline Mon Jul 23 18:41:30 2018}\label{table:insElasticPiston.rep.AmpSCF1zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{7.7}{-3} &      & \num{1.1}{-2} &      & \num{1.4}{-3} &      & \num{9.6}{-3} &      & \num{1.2}{-2} &       \\ \hline
                rep2 &     2 & \num{8.7}{-4} &  8.9 & \num{1.7}{-3} &  6.4 & \num{7.4}{-5} & 18.8 & \num{1.6}{-3} &  5.9 & \num{1.1}{-3} & 10.5  \\ \hline
                rep4 &     4 & \num{2.7}{-4} &  3.3 & \num{3.9}{-4} &  4.2 & \num{1.8}{-5} &  4.0 & \num{3.8}{-4} &  4.2 & \num{3.4}{-4} &  3.4  \\ \hline
                rep8 &     8 & \num{6.5}{-5} &  4.1 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.8 & \num{9.9}{-5} &  3.9 & \num{9.0}{-5} &  3.8  \\ \hline
    rate             &       &  $2.23$       &      &  $2.22$       &      &  $2.65$       &      &  $2.19$       &      &  $2.29$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 18:58:15 2018}\label{table:insElasticPiston.rep.AmpSCF1zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.AmpSCF8000Imtp3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.1}{-2} &      & \num{1.6}{-3} &      & \num{1.4}{-4} &      & \num{5.0}{-4} &      & \num{13.6}{0} &       \\ \hline
                rep2 &     2 & \num{1.6}{-3} &  6.8 & \num{3.0}{-4} &  5.3 & \num{1.8}{-5} &  7.5 & \num{1.0}{-4} &  4.9 & \num{3.0}{0} &  4.6  \\ \hline
                rep4 &     4 & \num{3.4}{-4} &  4.6 & \num{6.0}{-5} &  4.9 & \num{4.9}{-6} &  3.8 & \num{1.8}{-5} &  5.5 & \num{6.6}{-1} &  4.5  \\ \hline
                rep8 &     8 & \num{7.8}{-5} &  4.3 & \num{1.5}{-5} &  4.0 & \num{1.5}{-6} &  3.3 & \num{4.9}{-6} &  3.8 & \num{1.8}{-1} &  3.6  \\ \hline
    rate             &       &  $2.35$       &      &  $2.24$       &      &  $2.15$       &      &  $2.25$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF8000Imtp3, $t=.3$, AM=1, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=8000, sm-diss=0.2  Mon Jul 10 06:45:35 2017}\label{table:insElasticPiston.rep.AmpSCF8000Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.TPSCF1600Imtp3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{6.3}{-3} &      & \num{2.4}{-3} &      & \num{1.9}{-4} &      & \num{2.8}{-4} &      & \num{2.9}{0} &       \\ \hline
                rep2 &     2 & \num{1.0}{-3} &  6.1 & \num{4.1}{-4} &  5.7 & \num{2.6}{-5} &  7.4 & \num{5.7}{-5} &  4.9 & \num{6.8}{-1} &  4.3  \\ \hline
                rep4 &     4 & \num{2.4}{-4} &  4.3 & \num{8.4}{-5} &  4.9 & \num{7.7}{-6} &  3.4 & \num{1.6}{-5} &  3.4 & \num{1.8}{-1} &  3.8  \\ \hline
                rep8 &     8 & \num{5.9}{-5} &  4.1 & \num{2.0}{-5} &  4.1 & \num{2.3}{-6} &  3.4 & \num{5.4}{-6} &  3.1 & \num{5.1}{-2} &  3.5  \\ \hline
    rate             &       &  $2.23$       &      &  $2.28$       &      &  $2.10$       &      &  $1.88$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.TPSCF1600Imtp3, $t=.3$, AM=0, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1600, sm-diss=0.2  Sun Jul  9 16:34:26 2017}\label{table:insElasticPiston.rep.TPSCF1600Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.TPSCF8000Imtp3.ConvTable.tex <==
\begin{table}[hbt]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{6.3}{-3} &      & \num{2.4}{-3} &      & \num{1.9}{-4} &      & \num{2.8}{-4} &      & \num{14.6}{0} &       \\ \hline
                rep2 &     2 & \num{1.0}{-3} &  6.1 & \num{4.1}{-4} &  5.7 & \num{2.6}{-5} &  7.4 & \num{5.7}{-5} &  4.9 & \num{3.4}{0} &  4.3  \\ \hline
                rep4 &     4 & \num{2.4}{-4} &  4.3 & \num{8.4}{-5} &  4.9 & \num{7.6}{-6} &  3.4 & \num{1.6}{-5} &  3.4 & \num{9.0}{-1} &  3.7  \\ \hline
                rep8 &     8 & \num{5.9}{-5} &  4.1 & \num{2.0}{-5} &  4.1 & \num{2.3}{-6} &  3.4 & \num{5.4}{-6} &  3.1 & \num{2.6}{-1} &  3.5  \\ \hline
    rate             &       &  $2.23$       &      &  $2.28$       &      &  $2.11$       &      &  $1.89$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.TPSCF8000Imtp3, $t=.3$, AM=0, cfl=.9, nu=.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=8000, sm-diss=0.2  Sun Jul  9 16:36:07 2017}\label{table:insElasticPiston.rep.TPSCF8000Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF1000pNU10zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{5.5}{-7} &      & \num{1.1}{-7} &      & \num{1.6}{-8} &      & \num{2.0}{-7} &      & \num{1.2}{-4} &       \\ \hline
                rep2 &     2 & \num{8.7}{-8} &  6.3 & \num{2.7}{-8} &  4.1 & \num{3.5}{-9} &  4.5 & \num{4.5}{-8} &  4.4 & \num{3.3}{-5} &  3.5  \\ \hline
                rep4 &     4 & \num{3.7}{-8} &  2.3 & \num{6.1}{-9} &  4.4 & \num{8.8}{-10} &  4.0 & \num{1.0}{-8} &  4.5 & \num{8.3}{-6} &  4.0  \\ \hline
                rep8 &     8 & \num{2.1}{-8} &  1.8 & \num{1.4}{-9} &  4.3 & \num{2.2}{-10} &  4.0 & \num{2.3}{-9} &  4.5 & \num{2.1}{-6} &  4.0  \\ \hline
    rate             &       &  $1.53$       &      &  $2.10$       &      &  $2.05$       &      &  $2.15$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1000pNU10zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=10 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1000., rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 17 21:39:21 2018}\label{table:insElasticPiston.rep.shearAmpSCF1000pNU10zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF1000pNUp1zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.3}{-5} &      & \num{1.2}{-4} &      & \num{1.9}{-5} &      & \num{2.2}{-4} &      & \num{1.4}{-1} &       \\ \hline
                rep2 &     2 & \num{2.8}{-6} &  4.6 & \num{2.9}{-5} &  4.0 & \num{3.9}{-6} &  4.9 & \num{5.0}{-5} &  4.4 & \num{3.8}{-2} &  3.6  \\ \hline
                rep4 &     4 & \num{4.5}{-7} &  6.2 & \num{6.7}{-6} &  4.3 & \num{9.9}{-7} &  4.0 & \num{1.1}{-5} &  4.4 & \num{9.5}{-3} &  4.0  \\ \hline
                rep8 &     8 & \num{2.3}{-7} &  2.0 & \num{1.4}{-6} &  4.8 & \num{2.4}{-7} &  4.1 & \num{2.5}{-6} &  4.5 & \num{2.3}{-3} &  4.1  \\ \hline
    rate             &       &  $2.00$       &      &  $2.13$       &      &  $2.10$       &      &  $2.15$       &      &  $1.96$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1000pNUp1zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1000., rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 17 22:54:04 2018}\label{table:insElasticPiston.rep.shearAmpSCF1000pNUp1zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF10pNU10zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{7.9}{-8} &      & \num{2.2}{-9} &      & \num{10.0}{-10} &      & \num{4.6}{-8} &      & \num{1.2}{-7} &       \\ \hline
                rep2 &     2 & \num{2.7}{-9} & 28.9 & \num{6.2}{-10} &  3.6 & \num{3.5}{-10} &  2.9 & \num{1.5}{-8} &  3.1 & \num{3.2}{-8} &  3.8  \\ \hline
                rep4 &     4 & \num{2.0}{-10} & 13.8 & \num{1.4}{-10} &  4.5 & \num{7.9}{-11} &  4.4 & \num{3.7}{-9} &  4.0 & \num{6.7}{-9} &  4.8  \\ \hline
                rep8 &     8 & \num{5.6}{-11} &  3.5 & \num{3.1}{-11} &  4.5 & \num{2.0}{-11} &  4.0 & \num{9.3}{-10} &  4.0 & \num{1.4}{-9} &  4.7  \\ \hline
    rate             &       &  $3.52$       &      &  $2.07$       &      &  $1.91$       &      &  $1.89$       &      &  $2.15$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF10pNU10zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=10 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10., rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 17 21:33:12 2018}\label{table:insElasticPiston.rep.shearAmpSCF10pNU10zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF10pNUp1zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.0}{-5} &      & \num{8.9}{-5} &      & \num{1.1}{-5} &      & \num{1.6}{-4} &      & \num{1.0}{-3} &       \\ \hline
                rep2 &     2 & \num{1.9}{-6} &  5.5 & \num{2.1}{-5} &  4.2 & \num{3.4}{-6} &  3.2 & \num{3.5}{-5} &  4.5 & \num{3.0}{-4} &  3.5  \\ \hline
                rep4 &     4 & \num{3.9}{-7} &  4.8 & \num{4.9}{-6} &  4.4 & \num{8.6}{-7} &  4.0 & \num{7.8}{-6} &  4.5 & \num{7.7}{-5} &  3.9  \\ \hline
                rep8 &     8 & \num{1.6}{-7} &  2.4 & \num{1.1}{-6} &  4.6 & \num{2.1}{-7} &  4.2 & \num{1.8}{-6} &  4.5 & \num{1.8}{-5} &  4.2  \\ \hline
    rate             &       &  $2.02$       &      &  $2.13$       &      &  $1.92$       &      &  $2.16$       &      &  $1.95$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF10pNUp1zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10., rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 17 22:43:41 2018}\label{table:insElasticPiston.rep.shearAmpSCF10pNUp1zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF10zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.1}{-7} &      & \num{3.0}{-9} &      & \num{1.4}{-9} &      & \num{3.2}{-8} &      & \num{1.7}{-7} &       \\ \hline
                rep2 &     2 & \num{4.7}{-9} & 24.0 & \num{7.2}{-10} &  4.1 & \num{3.1}{-10} &  4.5 & \num{1.1}{-8} &  2.8 & \num{3.9}{-8} &  4.5  \\ \hline
                rep4 &     4 & \num{7.8}{-10} &  6.0 & \num{1.5}{-10} &  4.7 & \num{5.2}{-11} &  5.9 & \num{2.7}{-9} &  4.1 & \num{7.7}{-9} &  5.0  \\ \hline
                rep8 &     8 & \num{6.8}{-11} & 11.6 & \num{3.3}{-11} &  4.6 & \num{1.2}{-11} &  4.5 & \num{6.7}{-10} &  4.0 & \num{1.7}{-9} &  4.6  \\ \hline
    rate             &       &  $3.47$       &      &  $2.17$       &      &  $2.33$       &      &  $1.88$       &      &  $2.24$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF10zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 18:45:42 2018}\label{table:insElasticPiston.rep.shearAmpSCF10zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF10zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.9}{-8} &      & \num{2.8}{-9} &      & \num{1.3}{-9} &      & \num{3.2}{-8} &      & \num{1.6}{-7} &       \\ \hline
                rep2 &     2 & \num{5.1}{-9} & 17.5 & \num{7.2}{-10} &  3.9 & \num{3.0}{-10} &  4.2 & \num{1.1}{-8} &  2.9 & \num{3.9}{-8} &  4.2  \\ \hline
                rep4 &     4 & \num{7.7}{-10} &  6.6 & \num{1.5}{-10} &  4.8 & \num{5.2}{-11} &  5.8 & \num{2.7}{-9} &  4.1 & \num{7.7}{-9} &  5.1  \\ \hline
                rep8 &     8 & \num{6.7}{-11} & 11.5 & \num{3.3}{-11} &  4.6 & \num{1.1}{-11} &  4.5 & \num{6.7}{-10} &  4.0 & \num{1.7}{-9} &  4.6  \\ \hline
    rate             &       &  $3.39$       &      &  $2.15$       &      &  $2.30$       &      &  $1.87$       &      &  $2.21$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF10zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 19:11:22 2018}\label{table:insElasticPiston.rep.shearAmpSCF10zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF10zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.9}{-8} &      & \num{2.8}{-9} &      & \num{1.3}{-9} &      & \num{3.2}{-8} &      & \num{1.6}{-7} &       \\ \hline
                rep2 &     2 & \num{5.1}{-9} & 17.5 & \num{7.2}{-10} &  3.9 & \num{3.0}{-10} &  4.2 & \num{1.1}{-8} &  2.9 & \num{3.9}{-8} &  4.2  \\ \hline
                rep4 &     4 & \num{7.7}{-10} &  6.6 & \num{1.5}{-10} &  4.8 & \num{5.2}{-11} &  5.8 & \num{2.7}{-9} &  4.1 & \num{7.7}{-9} &  5.1  \\ \hline
                rep8 &     8 & \num{6.7}{-11} & 11.5 & \num{3.3}{-11} &  4.6 & \num{1.1}{-11} &  4.5 & \num{6.7}{-10} &  4.0 & \num{1.7}{-9} &  4.6  \\ \hline
    rate             &       &  $3.39$       &      &  $2.15$       &      &  $2.30$       &      &  $1.87$       &      &  $2.21$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF10zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 18:58:29 2018}\label{table:insElasticPiston.rep.shearAmpSCF10zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF10zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{6.5}{-8} &      & \num{2.9}{-9} &      & \num{1.3}{-9} &      & \num{3.3}{-8} &      & \num{1.7}{-7} &       \\ \hline
                rep2 &     2 & \num{5.5}{-9} & 11.7 & \num{7.4}{-10} &  4.0 & \num{3.1}{-10} &  4.3 & \num{1.1}{-8} &  2.9 & \num{3.9}{-8} &  4.4  \\ \hline
                rep4 &     4 & \num{7.8}{-10} &  7.1 & \num{1.5}{-10} &  4.8 & \num{5.2}{-11} &  5.9 & \num{2.7}{-9} &  4.1 & \num{7.7}{-9} &  5.1  \\ \hline
                rep8 &     8 & \num{6.8}{-11} & 11.5 & \num{3.3}{-11} &  4.6 & \num{1.2}{-11} &  4.5 & \num{6.7}{-10} &  4.0 & \num{1.7}{-9} &  4.6  \\ \hline
    rate             &       &  $3.25$       &      &  $2.17$       &      &  $2.30$       &      &  $1.89$       &      &  $2.24$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF10zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 19:04:11 2018}\label{table:insElasticPiston.rep.shearAmpSCF10zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF1e3zf1+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.9}{-7} &      & \num{1.1}{-8} &      & \num{1.7}{-8} &      & \num{1.3}{-8} &      & \num{1.5}{-4} &       \\ \hline
                rep2 &     2 & \num{4.2}{-8} & 21.2 & \num{2.5}{-9} &  4.2 & \num{3.8}{-9} &  4.5 & \num{5.4}{-9} &  2.5 & \num{3.4}{-5} &  4.3  \\ \hline
                rep4 &     4 & \num{3.0}{-8} &  1.4 & \num{8.1}{-10} &  3.1 & \num{8.5}{-10} &  4.4 & \num{1.7}{-9} &  3.2 & \num{7.5}{-6} &  4.5  \\ \hline
                rep8 &     8 & \num{5.7}{-9} &  5.3 & \num{2.3}{-10} &  3.5 & \num{2.0}{-10} &  4.2 & \num{4.9}{-10} &  3.4 & \num{1.7}{-6} &  4.3  \\ \hline
    rate             &       &  $2.23$       &      &  $1.82$       &      &  $2.14$       &      &  $1.60$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3zf1+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Wed Aug 15 18:50:01 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3zf1+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF1e3zf2+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.9}{-7} &      & \num{9.5}{-9} &      & \num{1.7}{-8} &      & \num{1.4}{-8} &      & \num{1.5}{-4} &       \\ \hline
                rep2 &     2 & \num{4.4}{-8} & 20.3 & \num{2.3}{-9} &  4.1 & \num{3.8}{-9} &  4.5 & \num{5.3}{-9} &  2.5 & \num{3.4}{-5} &  4.3  \\ \hline
                rep4 &     4 & \num{3.0}{-8} &  1.4 & \num{7.7}{-10} &  3.0 & \num{8.5}{-10} &  4.5 & \num{1.6}{-9} &  3.3 & \num{7.5}{-6} &  4.5  \\ \hline
                rep8 &     8 & \num{5.7}{-9} &  5.3 & \num{2.3}{-10} &  3.4 & \num{2.0}{-10} &  4.2 & \num{4.8}{-10} &  3.3 & \num{1.7}{-6} &  4.3  \\ \hline
    rate             &       &  $2.24$       &      &  $1.78$       &      &  $2.14$       &      &  $1.61$       &      &  $2.14$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3zf2+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=2 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 19:17:04 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3zf2+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF1e3zf5+0Imtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.9}{-7} &      & \num{9.5}{-9} &      & \num{1.7}{-8} &      & \num{1.4}{-8} &      & \num{1.5}{-4} &       \\ \hline
                rep2 &     2 & \num{4.4}{-8} & 20.3 & \num{2.3}{-9} &  4.1 & \num{3.8}{-9} &  4.5 & \num{5.3}{-9} &  2.5 & \num{3.4}{-5} &  4.3  \\ \hline
                rep4 &     4 & \num{3.0}{-8} &  1.4 & \num{7.7}{-10} &  3.0 & \num{8.5}{-10} &  4.5 & \num{1.6}{-9} &  3.3 & \num{7.5}{-6} &  4.5  \\ \hline
                rep8 &     8 & \num{5.7}{-9} &  5.3 & \num{2.3}{-10} &  3.4 & \num{2.0}{-10} &  4.2 & \num{4.8}{-10} &  3.3 & \num{1.7}{-6} &  4.3  \\ \hline
    rate             &       &  $2.24$       &      &  $1.78$       &      &  $2.14$       &      &  $1.61$       &      &  $2.14$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3zf5+0Imtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline Mon Jul 23 19:04:03 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3zf5+0Imtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF1e3zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{9.4}{-7} &      & \num{6.4}{-9} &      & \num{1.8}{-8} &      & \num{1.3}{-8} &      & \num{1.5}{-4} &       \\ \hline
                rep2 &     2 & \num{4.4}{-8} & 21.4 & \num{2.1}{-9} &  3.0 & \num{3.8}{-9} &  4.6 & \num{5.1}{-9} &  2.6 & \num{3.4}{-5} &  4.4  \\ \hline
                rep4 &     4 & \num{2.9}{-8} &  1.5 & \num{7.3}{-10} &  2.9 & \num{8.5}{-10} &  4.5 & \num{1.6}{-9} &  3.3 & \num{7.5}{-6} &  4.6  \\ \hline
                rep8 &     8 & \num{5.6}{-9} &  5.1 & \num{2.3}{-10} &  3.2 & \num{2.0}{-10} &  4.2 & \num{4.9}{-10} &  3.2 & \num{1.7}{-6} &  4.3  \\ \hline
    rate             &       &  $2.27$       &      &  $1.60$       &      &  $2.15$       &      &  $1.60$       &      &  $2.14$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=10. CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 dtMax=2.e-2 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 10 19:08:31 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3zfmImtp6}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCF1pNUp1zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.8}{-6} &      & \num{1.4}{-5} &      & \num{5.9}{-6} &      & \num{2.0}{-5} &      & \num{3.8}{-5} &       \\ \hline
                rep2 &     2 & \num{1.7}{-7} & 10.5 & \num{1.6}{-6} &  8.6 & \num{1.6}{-6} &  3.8 & \num{6.3}{-6} &  3.3 & \num{1.1}{-5} &  3.6  \\ \hline
                rep4 &     4 & \num{4.6}{-8} &  3.7 & \num{4.0}{-7} &  4.0 & \num{3.8}{-7} &  4.2 & \num{1.7}{-6} &  3.7 & \num{2.6}{-6} &  4.2  \\ \hline
                rep8 &     8 & \num{4.6}{-9} & 10.0 & \num{9.8}{-8} &  4.1 & \num{8.8}{-8} &  4.3 & \num{4.0}{-7} &  4.2 & \num{6.0}{-7} &  4.3  \\ \hline
    rate             &       &  $2.78$       &      &  $2.34$       &      &  $2.03$       &      &  $1.89$       &      &  $2.00$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1pNUp1zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1., rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 17 22:32:46 2018}\label{table:insElasticPiston.rep.shearAmpSCF1pNUp1zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCFp001NUp1zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{5.4}{-9} &      & \num{2.5}{-8} &      & \num{2.5}{-6} &      & \num{6.7}{-5} &      & \num{2.5}{-8} &       \\ \hline
                rep2 &     2 & \num{4.1}{-10} & 13.1 & \num{7.3}{-9} &  3.3 & \num{9.2}{-7} &  2.7 & \num{2.0}{-5} &  3.4 & \num{6.5}{-9} &  3.8  \\ \hline
                rep4 &     4 & \num{3.0}{-11} & 13.5 & \num{1.7}{-9} &  4.2 & \num{2.2}{-7} &  4.2 & \num{4.9}{-6} &  4.1 & \num{1.5}{-9} &  4.3  \\ \hline
                rep8 &     8 & \num{8.2}{-12} &  3.7 & \num{4.4}{-10} &  3.9 & \num{5.1}{-8} &  4.2 & \num{1.3}{-6} &  3.9 & \num{3.6}{-10} &  4.2  \\ \hline
    rate             &       &  $3.18$       &      &  $1.95$       &      &  $1.88$       &      &  $1.92$       &      &  $2.05$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCFp001NUp1zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=.001, rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 17 22:07:07 2018}\label{table:insElasticPiston.rep.shearAmpSCFp001NUp1zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rep.shearAmpSCFp1NUp1zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{5.0}{-7} &      & \num{2.0}{-6} &      & \num{1.2}{-6} &      & \num{5.7}{-5} &      & \num{2.0}{-6} &       \\ \hline
                rep2 &     2 & \num{3.8}{-8} & 13.0 & \num{6.1}{-7} &  3.4 & \num{5.0}{-7} &  2.3 & \num{1.8}{-5} &  3.1 & \num{5.0}{-7} &  4.1  \\ \hline
                rep4 &     4 & \num{3.1}{-9} & 12.5 & \num{1.4}{-7} &  4.2 & \num{1.2}{-7} &  4.2 & \num{4.5}{-6} &  4.0 & \num{1.0}{-7} &  4.8  \\ \hline
                rep8 &     8 & \num{7.3}{-10} &  4.2 & \num{3.6}{-8} &  4.0 & \num{2.9}{-8} &  4.2 & \num{1.1}{-6} &  4.0 & \num{2.2}{-8} &  4.7  \\ \hline
    rate             &       &  $3.19$       &      &  $1.96$       &      &  $1.80$       &      &  $1.89$       &      &  $2.19$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCFp1NUp1zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=.1, rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Aug 17 22:22:28 2018}\label{table:insElasticPiston.rep.shearAmpSCFp1NUp1zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.AmpCaseid7SCF200NUp1zf1+0Imt1p.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{2.6}{-7} &      & \num{1.7}{-7} &      & \num{1.9}{-7} &      & \num{1.6}{-6} &      & \num{2.2}{-7} &       \\ \hline
                rtw4 &     2 & \num{5.7}{-8} &  4.6 & \num{5.5}{-8} &  3.1 & \num{2.3}{-8} &  7.9 & \num{3.2}{-7} &  5.1 & \num{3.8}{-8} &  5.9  \\ \hline
    rate             &       &  $2.19$       &      &  $1.63$       &      &  $2.99$       &      &  $2.35$       &      &  $2.55$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.AmpCaseid7SCF200NUp1zf1+0Imt1p, $t=1.$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=200, rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=7 -amp=1e-05 Sun Aug 19 14:57:26 2018}\label{table:insElasticPiston.rtw.AmpCaseid7SCF200NUp1zf1+0Imt1p}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.AmpCaseid7SCF200NUp1zf1+0Imtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{4.2}{-7} &      & \num{2.3}{-7} &      & \num{3.2}{-7} &      & \num{2.5}{-6} &      & \num{3.4}{-7} &       \\ \hline
                rtw4 &     2 & \num{6.6}{-8} &  6.3 & \num{6.8}{-8} &  3.4 & \num{4.5}{-8} &  7.1 & \num{5.0}{-7} &  5.0 & \num{6.4}{-8} &  5.3  \\ \hline
                rtw8 &     4 & \num{1.5}{-8} &  4.3 & \num{1.8}{-8} &  3.8 & \num{9.7}{-9} &  4.6 & \num{1.2}{-7} &  4.2 & \num{1.6}{-8} &  4.1  \\ \hline
               rtw16 &     8 & \num{3.8}{-9} &  4.0 & \num{5.0}{-9} &  3.6 & \num{2.3}{-9} &  4.3 & \num{3.0}{-8} &  4.1 & \num{4.2}{-9} &  3.8  \\ \hline
    rate             &       &  $2.24$       &      &  $1.85$       &      &  $2.36$       &      &  $2.13$       &      &  $2.11$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.AmpCaseid7SCF200NUp1zf1+0Imtp3, $t=.3$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=200, rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=7 -amp=1e-05 Sun Aug 19 15:00:12 2018}\label{table:insElasticPiston.rtw.AmpCaseid7SCF200NUp1zf1+0Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.AmpCaseid8SCF200NUp1zf1+0Imtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{4.7}{-8} &      & \num{3.5}{-8} &      & \num{2.3}{-9} &      & \num{1.6}{-8} &      & \num{2.2}{-7} &       \\ \hline
                rtw4 &     2 & \num{3.7}{-8} &  1.3 & \num{9.3}{-9} &  3.7 & \num{6.3}{-10} &  3.7 & \num{5.0}{-9} &  3.2 & \num{8.0}{-8} &  2.8  \\ \hline
                rtw8 &     4 & \num{8.0}{-9} &  4.5 & \num{2.2}{-9} &  4.2 & \num{1.4}{-10} &  4.4 & \num{1.3}{-9} &  3.9 & \num{2.2}{-8} &  3.7  \\ \hline
               rtw16 &     8 & \num{2.0}{-9} &  4.0 & \num{5.7}{-10} &  3.9 & \num{3.3}{-11} &  4.4 & \num{3.4}{-10} &  3.8 & \num{5.6}{-9} &  3.9  \\ \hline
    rate             &       &  $1.58$       &      &  $1.99$       &      &  $2.06$       &      &  $1.86$       &      &  $1.78$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.AmpCaseid8SCF200NUp1zf1+0Imtp3, $t=.3$, AM=1, cfl=0.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=200, rhoSolid=1 sm-diss=.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=8 -amp=1e-05 Sun Aug 19 15:38:35 2018}\label{table:insElasticPiston.rtw.AmpCaseid8SCF200NUp1zf1+0Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1zf1+0Imtp2.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{1.8}{-7} &      & \num{7.4}{-8} &      & \num{1.2}{-8} &      & \num{8.6}{-8} &      & \num{1.5}{-7} &       \\ \hline
                rtw4 &     2 & \num{2.9}{-8} &  6.2 & \num{1.3}{-8} &  5.7 & \num{2.6}{-9} &  4.8 & \num{1.6}{-8} &  5.4 & \num{4.2}{-8} &  3.5  \\ \hline
                rtw8 &     4 & \num{6.1}{-9} &  4.7 & \num{2.7}{-9} &  4.7 & \num{6.0}{-10} &  4.4 & \num{3.4}{-9} &  4.6 & \num{10.0}{-9} &  4.2  \\ \hline
               rtw16 &     8 & \num{1.5}{-9} &  4.1 & \num{6.5}{-10} &  4.2 & \num{1.4}{-10} &  4.2 & \num{8.2}{-10} &  4.2 & \num{2.5}{-9} &  4.0  \\ \hline
    rate             &       &  $2.30$       &      &  $2.27$       &      &  $2.15$       &      &  $2.24$       &      &  $1.98$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1zf1+0Imtp2, $t=.2$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-5 Wed Aug 15 18:55:02 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1zf1+0Imtp2}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1zf5+0Imtp2.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw1 &     1 & \num{3.6}{-6} &      & \num{1.4}{-6} &      & \num{1.0}{-7} &      & \num{1.4}{-6} &      & \num{3.1}{-6} &       \\ \hline
                rtw2 &     2 & \num{1.5}{-7} & 24.7 & \num{6.2}{-8} & 22.3 & \num{1.3}{-8} &  7.9 & \num{8.3}{-8} & 16.7 & \num{1.4}{-7} & 21.4  \\ \hline
                rtw4 &     4 & \num{2.9}{-8} &  5.0 & \num{1.2}{-8} &  5.0 & \num{2.6}{-9} &  4.9 & \num{1.5}{-8} &  5.4 & \num{4.2}{-8} &  3.5  \\ \hline
                rtw8 &     8 & \num{6.2}{-9} &  4.7 & \num{2.7}{-9} &  4.6 & \num{6.0}{-10} &  4.4 & \num{3.4}{-9} &  4.5 & \num{1.0}{-8} &  4.2  \\ \hline
    rate             &       &  $2.99$       &      &  $2.93$       &      &  $2.45$       &      &  $2.84$       &      &  $2.66$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1zf5+0Imtp2, $t=.2$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-5 Fri Jul 27 07:46:11 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1zf5+0Imtp2}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{4.6}{-7} &      & \num{2.6}{-7} &      & \num{2.7}{-5} &      & \num{1.8}{-4} &      & \num{3.3}{-7} &       \\ \hline
                rtw4 &     2 & \num{7.0}{-8} &  6.5 & \num{7.4}{-8} &  3.5 & \num{3.3}{-6} &  8.0 & \num{4.3}{-5} &  4.2 & \num{5.8}{-8} &  5.6  \\ \hline
                rtw8 &     4 & \num{1.6}{-8} &  4.5 & \num{1.9}{-8} &  3.9 & \num{7.3}{-7} &  4.6 & \num{1.2}{-5} &  3.5 & \num{1.4}{-8} &  4.1  \\ \hline
               rtw16 &     8 & \num{3.8}{-9} &  4.1 & \num{5.7}{-9} &  3.4 & \num{2.0}{-7} &  3.7 & \num{6.9}{-6} &  1.8 & \num{5.4}{-9} &  2.6  \\ \hline
    rate             &       &  $2.30$       &      &  $1.85$       &      &  $2.34$       &      &  $1.59$       &      &  $1.98$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=2 -amp=1e-5 Wed Aug 15 19:25:42 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp5.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{4.7}{-7} &      & \num{2.7}{-7} &      & \num{1.7}{-5} &      & \num{1.8}{-4} &      & \num{3.5}{-7} &       \\ \hline
                rtw4 &     2 & \num{8.7}{-8} &  5.5 & \num{9.1}{-8} &  3.0 & \num{2.8}{-6} &  6.0 & \num{4.7}{-5} &  3.9 & \num{6.3}{-8} &  5.6  \\ \hline
                rtw8 &     4 & \num{1.9}{-8} &  4.5 & \num{2.0}{-8} &  4.5 & \num{6.1}{-7} &  4.6 & \num{1.1}{-5} &  4.1 & \num{1.4}{-8} &  4.4  \\ \hline
               rtw16 &     8 & \num{4.8}{-9} &  4.0 & \num{5.5}{-9} &  3.7 & \num{2.1}{-7} &  3.0 & \num{5.0}{-6} &  2.3 & \num{4.7}{-9} &  3.1  \\ \hline
    rate             &       &  $2.21$       &      &  $1.91$       &      &  $2.13$       &      &  $1.77$       &      &  $2.08$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp5, $t=.5$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=2 -amp=1e-5 Wed Aug 15 09:30:31 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp5}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf5+0Imtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw1 &     1 & \num{7.5}{-6} &      & \num{4.4}{-6} &      & \num{1.0}{-4} &      & \num{4.4}{-6} &      & \num{5.9}{-6} &       \\ \hline
                rtw2 &     2 & \num{4.3}{-7} & 17.3 & \num{2.8}{-7} & 16.0 & \num{2.7}{-5} &  3.8 & \num{1.5}{-4} &  0.0 & \num{2.9}{-7} & 20.6  \\ \hline
                rtw4 &     4 & \num{7.1}{-8} &  6.1 & \num{7.3}{-8} &  3.8 & \num{3.3}{-6} &  8.3 & \num{4.4}{-5} &  3.5 & \num{5.7}{-8} &  5.0  \\ \hline
                rtw8 &     8 & \num{1.6}{-8} &  4.6 & \num{1.9}{-8} &  3.9 & \num{7.0}{-7} &  4.7 & \num{1.0}{-5} &  4.3 & \num{1.4}{-8} &  4.2  \\ \hline
    rate             &       &  $2.93$       &      &  $2.56$       &      &  $2.47$       &      &  $-0.18$       &      &  $2.85$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf5+0Imtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=2 -amp=1e-5 Fri Jul 27 09:45:26 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf5+0Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf5+0Imtp4.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw1 &     1 & \num{6.8}{-6} &      & \num{4.8}{-6} &      & \num{1.1}{-4} &      & \num{4.7}{-6} &      & \num{5.7}{-6} &       \\ \hline
                rtw2 &     2 & \num{4.5}{-7} & 15.1 & \num{2.9}{-7} & 16.6 & \num{2.1}{-5} &  5.4 & \num{1.8}{-4} &  0.0 & \num{3.2}{-7} & 18.2  \\ \hline
                rtw4 &     4 & \num{8.2}{-8} &  5.4 & \num{8.6}{-8} &  3.3 & \num{3.2}{-6} &  6.5 & \num{5.1}{-5} &  3.5 & \num{5.7}{-8} &  5.5  \\ \hline
                rtw8 &     8 & \num{1.8}{-8} &  4.6 & \num{2.0}{-8} &  4.3 & \num{6.5}{-7} &  5.0 & \num{1.2}{-5} &  4.2 & \num{1.3}{-8} &  4.3  \\ \hline
    rate             &       &  $2.81$       &      &  $2.53$       &      &  $2.50$       &      &  $-0.23$       &      &  $2.88$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf5+0Imtp4, $t=.4$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=2 -amp=1e-5 Fri Jul 27 09:58:16 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf5+0Imtp4}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid4SCF10zf1+0Imtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{4.2}{-9} &      & \num{1.8}{-9} &      & \num{2.8}{-10} &      & \num{1.3}{-9} &      & \num{2.1}{-8} &       \\ \hline
                rtw4 &     2 & \num{4.7}{-9} &  0.9 & \num{6.9}{-10} &  2.6 & \num{7.2}{-11} &  3.9 & \num{5.3}{-10} &  2.5 & \num{7.9}{-9} &  2.7  \\ \hline
                rtw8 &     4 & \num{7.7}{-10} &  6.1 & \num{1.9}{-10} &  3.7 & \num{1.6}{-11} &  4.6 & \num{1.3}{-10} &  4.0 & \num{2.2}{-9} &  3.7  \\ \hline
               rtw16 &     8 & \num{1.7}{-10} &  4.5 & \num{6.3}{-11} &  3.0 & \num{3.4}{-12} &  4.6 & \num{3.6}{-11} &  3.7 & \num{5.6}{-10} &  3.8  \\ \hline
    rate             &       &  $1.65$       &      &  $1.65$       &      &  $2.13$       &      &  $1.75$       &      &  $1.76$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid4SCF10zf1+0Imtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption= zfMuByH=1 zfRhoHByDt=0 zfMono=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=4 -amp=1e-5 Wed Aug 15 20:13:25 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid4SCF10zf1+0Imtp3}
\end{center}
\end{table}


==> tables/old/insElasticPiston.rtw.radialTravelingWaveAmpCaseid4SCF10zf5+0Imtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw1 &     1 & \num{1.5}{-7} &      & \num{5.1}{-8} &      & \num{9.7}{-9} &      & \num{3.8}{-8} &      & \num{1.2}{-7} &       \\ \hline
                rtw2 &     2 & \num{5.0}{-9} & 29.7 & \num{1.8}{-9} & 27.8 & \num{2.8}{-10} & 34.3 & \num{1.4}{-9} & 27.9 & \num{2.2}{-8} &  5.4  \\ \hline
                rtw4 &     4 & \num{4.6}{-9} &  1.1 & \num{6.9}{-10} &  2.7 & \num{7.0}{-11} &  4.0 & \num{5.3}{-10} &  2.5 & \num{7.8}{-9} &  2.8  \\ \hline
                rtw8 &     8 & \num{7.7}{-10} &  6.0 & \num{1.9}{-10} &  3.7 & \num{1.6}{-11} &  4.5 & \num{1.3}{-10} &  4.0 & \num{2.2}{-9} &  3.6  \\ \hline
    rate             &       &  $2.30$       &      &  $2.57$       &      &  $2.99$       &      &  $2.58$       &      &  $1.88$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid4SCF10zf5+0Imtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfMuByH=5 zfRhoHByDt=0 dtMax=5.e-2 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=4 -amp=1e-5 Fri Jul 27 10:05:15 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid4SCF10zf5+0Imtp3}
\end{center}
\end{table}


==> tables/old_8_23/insElasticPiston.rep.shearAmpSCF1NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{5.2}{-6} &      & \num{1.5}{-5} &      & \num{7.7}{-6} &      & \num{2.6}{-5} &      & \num{3.5}{-5} &       \\ \hline
                rep2 &     2 & \num{3.7}{-7} & 14.1 & \num{3.1}{-6} &  4.9 & \num{1.3}{-6} &  5.7 & \num{8.7}{-6} &  3.0 & \num{8.5}{-6} &  4.1  \\ \hline
                rep4 &     4 & \num{8.7}{-8} &  4.3 & \num{7.0}{-7} &  4.4 & \num{3.0}{-7} &  4.5 & \num{2.1}{-6} &  4.1 & \num{1.8}{-6} &  4.7  \\ \hline
                rep8 &     8 & \num{1.2}{-8} &  7.5 & \num{1.7}{-7} &  4.1 & \num{7.2}{-8} &  4.1 & \num{5.1}{-7} &  4.2 & \num{4.3}{-7} &  4.2  \\ \hline
    rate             &       &  $2.85$       &      &  $2.14$       &      &  $2.24$       &      &  $1.92$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 22:01:05 2018}\label{table:insElasticPiston.rep.shearAmpSCF1NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/old_8_23/insElasticPiston.rep.shearAmpSCF1e-3NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{4.9}{-9} &      & \num{2.5}{-8} &      & \num{2.4}{-6} &      & \num{4.3}{-5} &      & \num{3.1}{-8} &       \\ \hline
                rep2 &     2 & \num{4.2}{-10} & 11.8 & \num{4.7}{-9} &  5.5 & \num{4.9}{-7} &  4.8 & \num{1.3}{-5} &  3.4 & \num{5.9}{-9} &  5.2  \\ \hline
                rep4 &     4 & \num{6.1}{-11} &  6.9 & \num{1.1}{-9} &  4.4 & \num{9.5}{-8} &  5.2 & \num{3.1}{-6} &  4.2 & \num{1.2}{-9} &  4.9  \\ \hline
                rep8 &     8 & \num{6.9}{-12} &  8.9 & \num{2.7}{-10} &  3.9 & \num{2.3}{-8} &  4.1 & \num{7.8}{-7} &  3.9 & \num{2.5}{-10} &  4.7  \\ \hline
    rate             &       &  $3.13$       &      &  $2.18$       &      &  $2.24$       &      &  $1.94$       &      &  $2.31$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e-3NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 21:48:22 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e-3NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/old_8_23/insElasticPiston.rep.shearAmpSCF1e3NUp1zfmImtp6.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{2.8}{-5} &      & \num{3.3}{-5} &      & \num{1.8}{-5} &      & \num{2.1}{-5} &      & \num{1.6}{-1} &       \\ \hline
                rep2 &     2 & \num{2.1}{-6} & 13.3 & \num{8.5}{-6} &  3.9 & \num{4.1}{-6} &  4.4 & \num{7.4}{-6} &  2.9 & \num{3.6}{-2} &  4.3  \\ \hline
                rep4 &     4 & \num{1.2}{-6} &  1.7 & \num{2.0}{-6} &  4.3 & \num{9.3}{-7} &  4.4 & \num{2.1}{-6} &  3.5 & \num{8.0}{-3} &  4.5  \\ \hline
                rep8 &     8 & \num{3.3}{-7} &  3.7 & \num{4.6}{-7} &  4.2 & \num{2.2}{-7} &  4.3 & \num{5.8}{-7} &  3.6 & \num{1.9}{-3} &  4.3  \\ \hline
    rate             &       &  $2.00$       &      &  $2.06$       &      &  $2.12$       &      &  $1.74$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3NUp1zfmImtp6, $t=.6$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Tue Aug 21 22:13:22 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3NUp1zfmImtp6}
\end{center}
\end{table}


==> tables/old_8_23/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NUp1zfmImtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{1.0}{-7} &      & \num{4.8}{-8} &      & \num{1.7}{-8} &      & \num{5.7}{-8} &      & \num{1.6}{-7} &       \\ \hline
                rtw4 &     2 & \num{4.7}{-8} &  2.2 & \num{1.4}{-8} &  3.5 & \num{3.5}{-9} &  4.9 & \num{1.4}{-8} &  4.1 & \num{4.2}{-8} &  3.9  \\ \hline
                rtw8 &     4 & \num{9.7}{-9} &  4.9 & \num{3.2}{-9} &  4.4 & \num{7.6}{-10} &  4.6 & \num{3.1}{-9} &  4.4 & \num{1.3}{-8} &  3.3  \\ \hline
               rtw16 &     8 & \num{2.4}{-9} &  4.0 & \num{8.0}{-10} &  3.9 & \num{1.8}{-10} &  4.3 & \num{7.7}{-10} &  4.1 & \num{2.8}{-9} &  4.5  \\ \hline
    rate             &       &  $1.86$       &      &  $1.99$       &      &  $2.19$       &      &  $2.07$       &      &  $1.92$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NUp1zfmImtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-5 Tue Aug 21 21:47:23 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NUp1zfmImtp3}
\end{center}
\end{table}


==> tables/old_8_23/insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCFp1NUp1zfmImtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{4.2}{-7} &      & \num{2.3}{-7} &      & \num{3.2}{-7} &      & \num{2.5}{-6} &      & \num{3.4}{-7} &       \\ \hline
                rtw4 &     2 & \num{6.6}{-8} &  6.3 & \num{6.8}{-8} &  3.4 & \num{4.5}{-8} &  7.1 & \num{5.0}{-7} &  5.0 & \num{6.4}{-8} &  5.3  \\ \hline
                rtw8 &     4 & \num{1.5}{-8} &  4.3 & \num{1.8}{-8} &  3.8 & \num{9.7}{-9} &  4.6 & \num{1.2}{-7} &  4.2 & \num{1.7}{-8} &  3.8  \\ \hline
               rtw16 &     8 & \num{3.8}{-9} &  4.0 & \num{5.0}{-9} &  3.6 & \num{2.3}{-9} &  4.3 & \num{3.0}{-8} &  4.1 & \num{4.2}{-9} &  4.1  \\ \hline
    rate             &       &  $2.24$       &      &  $1.85$       &      &  $2.36$       &      &  $2.13$       &      &  $2.10$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCFp1NUp1zfmImtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=.1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=7 -amp=1e-5 Tue Aug 21 21:46:37 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCFp1NUp1zfmImtp3}
\end{center}
\end{table}


==> tables/old_8_23/insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NUp1zfmImtp3.ConvTable.tex <==
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{4.7}{-8} &      & \num{3.5}{-8} &      & \num{2.3}{-9} &      & \num{1.6}{-8} &      & \num{2.2}{-7} &       \\ \hline
                rtw4 &     2 & \num{3.6}{-8} &  1.3 & \num{9.3}{-9} &  3.7 & \num{6.3}{-10} &  3.7 & \num{5.0}{-9} &  3.2 & \num{8.0}{-8} &  2.8  \\ \hline
                rtw8 &     4 & \num{8.3}{-9} &  4.4 & \num{2.2}{-9} &  4.2 & \num{1.4}{-10} &  4.4 & \num{1.3}{-9} &  3.8 & \num{2.6}{-8} &  3.0  \\ \hline
               rtw16 &     8 & \num{2.0}{-9} &  4.1 & \num{5.7}{-10} &  3.9 & \num{3.3}{-11} &  4.4 & \num{3.4}{-10} &  3.9 & \num{5.7}{-9} &  4.7  \\ \hline
    rate             &       &  $1.57$       &      &  $1.99$       &      &  $2.06$       &      &  $1.85$       &      &  $1.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NUp1zfmImtp3, $t=.3$, AM=1, cfl=.9, nu=.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 zfMono=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=8 -amp=1e-5 Tue Aug 21 21:47:51 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NUp1zfmImtp3}
\end{center}
\end{table}


==> texFiles/ElasticPistonRigidWalls.tex <==
\subsection{Elastic piston with rigid walls}

\begin{figure}[h]
\centering
\def\H{3}
\def\L{3}
\def\gap{.1}
\begin{tikzpicture}
  \draw[fill=blue!20,draw=blue,line width=2pt] 
  (0,\gap) -- (0,\H+\gap) -- (\L,\H+\gap) -- (\L,\gap) -- (0,\gap);
  \draw[fill=red!20,draw=red,line width=2pt] 
  (0,-\gap) -- (0,-\H-\gap) -- (\L,-\H-\gap) -- (\L,-\gap) -- (0,-\gap);
  \draw (-\gap,\H/2) node[anchor=east] {no-slip wall};
  \draw (-\gap,-\H/2) node[anchor=east] {zero-displacement wall};
  \draw (\L/2,\H/2) node[] {fluid};
  \draw (\L/2,-\H/2) node[] {solid};
  \draw (-\gap,0) node[anchor=east] {$y=0$};
\end{tikzpicture}
\end{figure}

\textbf{Test case}: a pressure ramp is applied as the top boundary condition, defined by
\begin{align}
p_{\text{top}}(t) &= p_0 \xi(t) \\
\xi(t) &= 
\begin{cases}
\sin^4(2 \pi t), & t<\frac{1}{4} \\
1, & t\ge \frac{1}{4}
\end{cases}.
\end{align}
%
See figures \ref{fig:cornerFix1} and \ref{fig:cornerFix2}.

\begin{figure}[h]
\centering
\includegraphics[width=.49\textwidth]{fig/cornerFixN20}
\includegraphics[width=.49\textwidth]{fig/cornerFixN40}
\includegraphics[width=.49\textwidth]{fig/cornerFixN80}
\caption{
Results of test case with 
$p_0 = 0.03,\,
\gamma = 0.01 / h^2,\,
\rho = 1,\,
\rhos = .001,\,
\mu = .1, \,
\lambdas = \mus = 1.$
The plot shows the pressure in the top domain (fluid) and vertical component in the bottom
domain (solid).
Top left: $N=20.$ Top right: $N=40.$ Bottom: $N=80.$
No wiggles near the corner are present. Any corner effects seam to disappear 
as the grid is refined. 
\label{fig:cornerFix1}}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=.49\textwidth]{fig/cornerNoFixN20DifferentView}
\includegraphics[width=.49\textwidth]{fig/cornerFixN20DifferentView}
\caption{
Results of test case with 
$p_0 = 0.03,\,
\gamma = 0.01 / h^2,\,
\rho = 1,\,
\rhos = .001,\,
\mu = .1, \,
\lambdas = \mus = 1.$
The plot shows the pressure in the top domain (fluid) and vertical component in the bottom
domain (solid).
Left: no corner fix-up, $N=20.$ Right: corner fix-up, $N=20.$ 
\label{fig:cornerFix2}}
\end{figure}


==> texFiles/GoverningEquationsInPolar.tex <==
\section{Governing equations in polar coordinates}

An incompressible fluid and elastic solid 
are considered in polar coordinates.
Let $v_r$ and $v_\theta$ be the radial and circumferential components
of the fluid velocity, respectively.
The fluid continuity equation is given by
\begin{align}
\frac{1}{r} \frac{\partial (r v_r)}{\partial r} + 
\frac{1}{r} \frac{\partial v_\theta}{\partial \theta} = 0.
\end{align}
%
The fluid momentum equations are given by
\begin{align}
\rho \frac{\partial v_r}{\partial t}
+ \rho \left(v_r \frac{\partial v_r}{\partial r} 
+ \frac{v_\theta}{r} \frac{\partial v_r}{\partial \theta}
- \frac{1}{r} v_\theta^2 \right)
+ \frac{\partial p}{\partial r} &= 
\mu \left( \frac{1}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_r}{\partial r}\right) 
+ \frac{1}{r^2} \frac{\partial^2 v_r}{\partial \theta^2}
- \frac{v_r}{r^2} 
- \frac{2}{r^2} \frac{\partial v_\theta}{\partial \theta}
\right) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rho \frac{\partial v_\theta}{\partial t}
+ \rho \left(v_r \frac{\partial v_\theta}{\partial r} 
+ \frac{v_\theta}{r} \frac{\partial v_\theta}{\partial \theta}
- \frac{1}{r} v_r v_\theta \right)
+ \frac{1}{r} \frac{\partial p}{\partial \theta} &= 
\mu \left( \frac{1}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_\theta}{\partial r}\right) 
+ \frac{1}{r^2} \frac{\partial^2 v_\theta}{\partial \theta^2}
+ \frac{2}{r^2} \frac{\partial v_r}{\partial \theta}
- \frac{v_\theta}{r^2}
\right).
\end{align}
%
The fluid stress tensor components are
\begin{align}
\sigma_{rr} &= -p + 2 \mu \frac{\partial v_r}{\partial r} \\
\sigma_{r\theta} &= \mu \left(\frac{1}{r} \frac{\partial v_r}{\partial \theta} + 
  \frac{\partial v_\theta}{\partial r}
  - \frac{v_\theta}{r} \right)\\
\sigma_{\theta\theta} &= -p + \frac{2\mu }{r} \left( \frac{\partial v_\theta}{\partial \theta} + v_r \right).
\end{align}
%
Let $\us_r$ and $\us_\theta$ be the radial and circumferential 
components of the solid displacement.
The solid momentum equations are
\begin{align}
\rhos \frac{\partial^2 \us_r}{\partial t^2} &= \frac{\partial \sigmas_{rr}}{\partial r} 
+ \frac{1}{r} \frac{\partial \sigmas_{r\theta}}{\partial \theta} 
+ \frac{1}{r} \left(\sigmas_{rr} - \sigmas_{\theta\theta} \right)
+ \bs_r \\
\rhos \frac{\partial^2 \us_\theta}{\partial t^2} &= \frac{\partial \sigmas_{r\theta}}{\partial r}
+ \frac{1}{r} \frac{\partial \sigmas_{\theta\theta}}{\partial \theta} 
+ \frac{2}{r} \sigmas_{r \theta} 
+ b_\theta.
\end{align}
% 
% The terms of the stress tensor are computed
% \begin{align}
% \grad \cdot \usv &= \frac{1}{r} \frac{\partial (r \us_r)}{ \partial r}
% + \frac{1}{r} \frac{\partial \us_\theta}{\partial \theta}.
% \end{align}
% %
% \begin{align}
% \epsilonsv = 
% \frac{1}{2} \left( \grad \usv + \left(\grad \usv \right)^T\right) &= 
% \left[\begin{array}{cc}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{\partial \us_r}{\partial r} &
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{1}{2} \left( \frac{1}{r} \frac{\partial \us_r}{\partial \theta} 
% + \frac{\partial \us_\theta}{\partial r}
% - \frac{\us_\theta}{r} \right) \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{1}{2} \left( \frac{1}{r} \frac{\partial \us_r}{\partial \theta} 
% + \frac{\partial \us_\theta}{\partial r}
% - \frac{\us_\theta}{r} \right) &
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{1}{r} \left(\frac{\partial \us_\theta}{\partial \theta} + \us_r  \right)
% \end{array}\right]
% \end{align}
%
The solid stress components are
\begin{align}
\sigmas_{rr} &= \lambdas \left(\frac{1}{r} \frac{\partial (r \us_r)}{ \partial r}
+ \frac{1}{r} \frac{\partial \us_\theta}{\partial \theta} \right) 
+ 2 \mus \frac{\partial \us_r}{\partial r} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{r\theta} &= \mus \left( \frac{1}{r} \frac{\partial \us_r}{\partial \theta} 
+ \frac{\partial \us_\theta}{\partial r}
- \frac{\us_\theta}{r} \right) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{\theta\theta} &= \lambdas \left(\frac{1}{r} \frac{\partial (r \us_r)}{ \partial r}
+ \frac{1}{r} \frac{\partial \us_\theta}{\partial \theta} \right) 
+ \frac{2 \mus }{r} \left(\frac{\partial \us_\theta}{\partial \theta} + \us_r  \right).
\end{align}



\subsection{Axial symmetry}

We look for solutions in which derivatives with respect to $\theta$
are zero.
The fluid continuity equation simplifies to
\begin{align}
\frac{\partial (r v_r)}{\partial r} &= 0 \nonumber 
\end{align}
%
Using this, an expression for $v_r$ can be obtained in terms of a
single function of time, $f(t)$.
\begin{align}
r v_r &= f(t) \nonumber \\
v_r(r,t) &= \frac{1}{r} f(t).
\end{align}
%
A boundary condition is required to find $f(t).$
The momentum equations simplify to
\begin{align}
\rho \frac{\partial v_r}{\partial t}
+ \rho \left(v_r \frac{\partial v_r}{\partial r} 
- \frac{1}{r} v_\theta^2 \right)
+ \frac{\partial p}{\partial r} &= 
\frac{\mu}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_r}{\partial r}\right) 
- \frac{\mu}{r^2} v_r \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rho \frac{\partial v_\theta}{\partial t}
+ \rho \left(v_r \frac{\partial v_\theta}{\partial r} 
- \frac{1}{r} v_r v_\theta \right)
\phantom{\;\frac{\partial p}{\partial r}}
 &= 
 \frac{\mu}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_\theta}{\partial r}\right) 
- \frac{\mu}{r^2} v_\theta
\end{align}
%
These equations are used to determine $p$ and $v_\theta.$ 
The solid momentum equations simplify to
\begin{align}
\rhos \frac{\partial^2 \us_r}{\partial t^2} &= \frac{\partial \sigmas_{rr}}{\partial r} 
+ \frac{1}{r} \left(\sigmas_{rr} - \sigmas_{\theta\theta} \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rhos \frac{\partial^2 \us_\theta}{\partial t^2} &= \frac{\partial \sigmas_{r\theta}}{\partial r}
+ \frac{2}{r} \sigmas_{r \theta}.
\end{align}
%
The solid stress tensor simplifies to
\begin{align}
\sigmas_{rr} &=  \frac{\lambdas}{r} \frac{\partial (r \us_r)}{ \partial r}
+ 2 \mus \frac{\partial \us_r}{\partial r} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{r\theta} &= \mus \left( 
\frac{\partial \us_\theta}{\partial r}
- \frac{\us_\theta}{r} \right) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{\theta\theta} &= \frac{\lambdas}{r} \frac{\partial (r \us_r)}{ \partial r}
+ \frac{2 \mus }{r} \us_r  .
\end{align}
%
The solid equations simplify to wave equations.
\begin{align}
 \frac{\partial^2 \us_r}{\partial t^2} &=
\cp^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_r)}{\partial r} \right) \\
\frac{\partial^2 \us_\theta}{\partial t^2} &=
\cs^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_\theta)}{\partial r} \right).
\end{align}


==> texFiles/algorithm-7-17-18.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{FSI algorithms} \label{sec:algorithm}

In this section, we describe the AMP algorithm, and we also discuss the traditional partitioned (TP) algorithm and the anti-traditional partitioned (ATP) algorithm for comparative purposes.  All three partitioned schemes use the same fluid and solid domain solvers.  For the fluid domain, we integrate the governing equations in velocity-pressure form using a fractional-step scheme in which the fluid velocity is advanaced in one step and the pressure-Poisson equation is solved to update the fluid pressure in the other step (see~\cite{splitStep2003}).  An explicit upwind Godunov method is used to advance the velocity and stress of the solid in its reference domain following approach described in~\cite{smog}, while a Lax-Wendroff scheme is used to advance the solid displacement.  These two domain solvers, both second-order accurate in space and time, are embedded in the FSI algorithms using a predictor-corrector approach.  The first step of the FSI time-stepping loop involves advancing the solid variables to the next time level.  The solid displacement predicts the new position of the fluid-solid interface and this information is used to deform the fluid grid and compute its {\em grid velocity}.  The fluid-domain solver is then called to advance the fluid velocity to the next time level and update the fluid pressure.  In the fluid solver, the diffusion terms of the momentum equations are treated implicitly, while the convection and pressure-gradient terms are approximated explicitly.  Following this fluid-domain step, the solid interface data is updated using fluid data at the new time level.  The steps outlined above are essentially repeated in the corrector step.  Depending on the densities of the fluid and solid (and on the grid spacing), the TP and ATP schemes may require addition sub-iterations for stability, in which case the corrector step is repeated.

The AMP algorithm differs from that of the TP and ATP schemes in the implementation of the fluid-solid interface conditions.  To this end, we begin in Section~\ref{sec:interfaceConditions} by describing the various treatments of the interface conditions, including compatability conditions, at a continuous level.  This discussion is then followed in Section~\ref{sec:partitionedAlgorithms} by a detailed description of the various FSI algorithms at a discrete level.


% ================================ ALGORITHM ============================================
{
    \def\alignspace{\hspace{1.2em}}
\begin{algorithm}\caption{\rm Added-mass partitioned (AMP) scheme}\scriptsize
\medskip
\[
\begin{array}{l}
\hbox{// \textsl{comment}}\smallskip\\
1.\text{ Predict the solid:}\\ 
\alignspace \vsv^{(p)} = \vsv^{n}
\end{array}
\]
\label{alg:ampRB}
\end{algorithm}
}


\subsection{Continuous interface conditions} \label{sec:interfaceConditions}

Using the formulas for the fluid stress tensor in~\eqref{eq:fluidStressTensor} and~\eqref{eq:fluidViscousStressTensor}, the AMP interface conditions in~\eqref{eq:BCharacteristicBC} for the fluid become
\begin{align}
-p + \nv^T \tauv \nv + \zp \nv^T \vv = \nv^T \sigmasv \nv + \zp \nv^T \vsv, \quad \phantom{m = 1,2,}\qquad \xv \in \GammaIf(t),
\label{eq:AMPNormalCharacteristic} \\
\tnv_m^T \tauv \nv + \zs \tnv_m^T \vv = \tnv_m^T \sigmasv \nv + \zs \tnv_m^T \vsv,  \quad m = 1,2, \qquad \xv \in \GammaIf(t),\label{eq:AMPTangentialCharacteristic}
\end{align}
with the $(p)$ superscipt on the solid variables suppressed.  These conditions, along with $\grad \cdot \vv = 0$ applied on the boundary, are a sufficient set of conditions for the fluid equations in velocity-pressure form.  The left-hand side of the interface conditions in~\eqref{eq:AMPTangentialCharacteristic} only involve the fluid velocity (and its derivatives), and these conditions with the divergence-free constraint are used as boundary conditions for the momentum equation in~\eqref{eq:fluidMomentum} to advance the fluid velocity.  The stress and velocity of the solid appearing on the right-hand side of~\eqref{eq:AMPTangentialCharacteristic} are obtained from an explicit time step of the hyperbolic system of equations for the solid.  Once the fluid velocity is advanced to the next time step, a Poisson problem is solved to update the fluid pressure.  Following the approach in~\cite{fib2014}, the interface condition in~\eqref{eq:AMPNormalCharacteristic} is used with the momentum equation in~\eqref{eq:fluidMomentum} to derive a Robin condition for the pressure-Poisson problem.  The momentum equation involves the acceleration of the fluid, and this quantity may be obtained on the moving fluid-solid interface using the Taylor approximation
\newcommand{\fluidPoint}{{\mathcal P}}
\newcommand{\solidPoint}{{\bar{\mathcal P}}_0}
\begin{align}
\Bigl.\vv(\xv,t-\dt)\Bigr\vert_{\xv=\fluidPoint(t-\dt)}\approx\Bigl.\bigl(\vv(\xv,t)-\dt D_t\vv(\xv,t)\bigr)\Bigr\vert_{\xv=\fluidPoint(t)},
\label{eq:fluidTaylorApprox}
\end{align}
where $D_t=\partial_t+\vv\cdot\grad$ is the material derivative and $\fluidPoint(t)$ is a point on the moving interface.  The corresponding approximation for the solid is
\begin{align}
\Bigl.\vsv(\xsv,t-\dt)\Bigr\vert_{\xsv=\solidPoint}\approx\Bigl.\bigl(\vsv(\xsv,t)-\dt\vsv_t(\xsv,t)\bigr)\Bigr\vert_{\xsv=\solidPoint},
\label{eq:solidTaylorApprox}
\end{align}
where $\solidPoint$ is the Lagrangian position associated with $\fluidPoint(t)$.  Using~\eqref{eq:fluidTaylorApprox} and~\eqref{eq:solidTaylorApprox} in~\eqref{eq:AMPNormalCharacteristic}, and assuming the fluid and solid velocities match on the interface at times $t-\dt$ and $t$, we obtain
\begin{align}
-p + \nv^T \tauv \nv + \zp \dt \nv^T D_t\vv = \nv^T \sigmasv \nv + \zp \dt \nv^T \vsv_t, \qquad \xv \in \GammaIf(t).
\label{eq:pressureBCtemp}
\end{align}
We may now eliminate the fluid acceleration using~\eqref{eq:fluidMomentum} to obtain the following Robin condition for the fluid pressure:
\begin{align}
-p - {\zp \dt\over\rho} \partial_n p =  -\nv^T \tauv \nv + \nu\zp \dt\nv^T\bigl(\grad\times\grad\times\vv\bigr) +\nv^T \sigmasv \nv + \zp \dt \nv^T\vsv_t, \qquad \xv \in \GammaIf(t),
\label{eq:AMPpressureBC}
\end{align}
where $\partial_n=\nv\cdot\grad$ is the normal derivative and $\nu=\mu/\rho$ is the kinematic viscosity of the fluid.  Following~\cite{splitStep2003}, we have used the identity, $\Delta \vv = - \grad \curl \grad \curl \vv$, noting that $\grad \cdot \vv = 0$, to replace $\Delta \vv$ on the right-hand side of~\eqref{eq:AMPpressureBC} in favor of the curl-curl operator.  This is done for improved stability of the fractional-step scheme.  The condition in~\eqref{eq:AMPpressureBC}, along with suitable conditions for $\xv\in\partial\OmegaF(t)\backslash\GammaIf(t)$, is used for the Poisson equation in~\eqref{eq:pressurePoissonEquation} for the pressure.

\wdh{ \textbf{Alternative to~\eqref{eq:AMPTangentialCharacteristic}}. We could use the same approach used
to obtain~\eqref{eq:AMPpressureBC} to also match accelerations in~\eqref{eq:AMPTangentialCharacteristic}. This would
lead to (*check me*)
\ba
\tnv_m^T \tauv \nv + \f{\zs\dt}{\rho} \tnv_m^T(-\grad p + \mu\Delta\vv) =
        \tnv_m^T \sigmasv \nv + \zs \dt \tnv_m^T \vsv_t,  \quad m = 1,2, \qquad \xv \in \GammaIf(t),\label{eq:AMPTangentialCharacteristicII}
\ea
This has a different behaviour from~\eqref{eq:AMPTangentialCharacteristic} since now the solid looks {\em light}
when $\f{\zs\dt}{\rho}$ is small.
}% end wdh 



The traction along the interface is taken to be that given by the fluid, namely,
\newcommand{\vf}{{v_f}}
\begin{align}
(\sigmav\nv)^I=-p\nv+\tauv\nv,\qquad \xv\in\GammaIf(t),
\label{eq:AMPinterfaceTraction}
\end{align}
while the normal and tangential components of the velocity along the interface are defined by the following impedance-weighted averages:
\begin{align}
\nv^T\vv^I={\zf\over\zf+\zp}\nv^T\vv+{\zp\over\zf+\zp}\nv^T\vsv+{1\over\zf+\zp}\nv^T\bigl(\sigmasv\nv-(\sigmav\nv)^I\bigr), \quad \phantom{m = 1,2,}\qquad \xv \in \GammaIf(t),
\label{eq:AMPinterfaceNormalVelocity} \\
\tnv_m^T\vv^I={\zf\over\zf+\zs}\tnv_m^T\vv+{\zs\over\zf+\zs}\tnv_m^T\vsv+{1\over\zf+\zs}\tnv_m^T\bigl(\sigmasv\nv-(\sigmav\nv)^I\bigr) ,  \quad m = 1,2, \qquad \xv \in \GammaIf(t).
\label{eq:AMPinterfaceTangentialVelocity}
\end{align}
Here, $\zf=\rho\vf$ is a fluid impedance where $\vf$ is a suitable measure of the fluid velocity. 
In practice, we take $\vf = H/\dt$ where $H$ is an appropriate length scale for the problem.
This choice naturally appears in the non-dimensionalization of the stability analysis in Section \ref{sec:analysis}.
However, in \cite{fib2014}, it was shown that the AMP algorithm is insensitive to the choice of $\vf.$ 
The impedance-weighted averages are defined to ensure that the correct behaviors of the interface conditions are obtained in the limits of a heavy and light solids as we discuss next.

\das{I still think \eqref{eq:AMPinterfaceTangentialVelocity} is redundant. In the limit of a heavy solid, both
\eqref{eq:AMPTangentialCharacteristic} and \eqref{eq:AMPinterfaceTangentialVelocity} set the fluid velocity as the solid velocity.
We should discuss further...}

%It is instructive to consider the behaviors of the AMP interface conditions in the limits of heavy and light solids.
In the limit of a heavy solid, i.e.~$\rhos\rightarrow\infty$ ($\zp$, $\zs\rightarrow\infty$), the interface conditions for the fluid should approach those of a (moving) no-slip wall.  For $\zs\rightarrow\infty$, \eqref{eq:AMPTangentialCharacteristic} reduces to
\begin{align}
\tnv_m^T\vv=\tnv_m^T\vsv,\quad m=1,2,\qquad \xv \in \GammaIf(t),
\label{eq:tangentialVelocityHeavySolid}
\end{align}
so that the tangential components of the fluid velocity match those of the solid wall.  We note that the tangential components of the interface velocity defined in~\eqref{eq:AMPinterfaceTangentialVelocity} agree with those given in~\eqref{eq:tangentialVelocityHeavySolid} in this limit.  The normal component of the fluid is given by the normal component of the interface velocity, defined in~\eqref{eq:AMPinterfaceNormalVelocity}, which becomes
\begin{align}
\nv^T\vv=\nv^T\vv^I=\nv^T\vsv,\qquad \xv \in \GammaIf(t),
\label{eq:normalVelocityHeavySolid}
\end{align}
so that the normal component of the velocity of the fluid also matches that of the solid wall.  In this heavy-solid limit, the divergence-free constraint applied on the boundary becomes a compatibility condition used to specify values of the normal component of the fluid velocity at ghost points.  The Robin condition for the pressure given in~\eqref{eq:AMPpressureBC} in the limit $\zp\rightarrow\infty$ reduces to
\begin{align}
- {1\over\rho} \partial_n p =  \nu\nv^T\bigl(\grad\times\grad\times\vv\bigr) + \nv^T\vsv_t, \qquad \xv \in \GammaIf(t).
\label{eq:pressureBCHeavySolid}
\end{align}
This Neumann condition for the pressure is often used for the pressure-Poisson problem at a no-slip wall.

In the limit of a light solid, i.e.~$\rhos\rightarrow0$ ($\zp$, $\zs\rightarrow0$), the interface conditions for the fluid should approach those of a free surface.  With $\zs\rightarrow0$, \eqref{eq:AMPTangentialCharacteristic} becomes
\begin{align}
\tnv_m^T\sigmav\nv=\tnv_m^T\sigmasv\nv,\quad m=1,2,\qquad \xv \in \GammaIf(t),
\label{eq:tangentialStressLightSolid}
\end{align}
and thus the tangential components of the fluid stress match those of the light solid.  In this limit, the conditions in~\eqref{eq:tangentialStressLightSolid} and the divergence-free constraint on the fluid velocity provide the boundary conditions needed to advance the velocity using~\eqref{eq:fluidMomentum}, along with suitable boundary conditions for $\xv\in\partial\OmegaF(t)\backslash\GammaIf(t)$ which we do not discuss.  The interface condition in~\eqref{eq:AMPNormalCharacteristic} or the derived Robin condition in~\eqref{eq:AMPpressureBC} both reduce to
\begin{align}
-p = - \nv^T \tauv \nv + \nv^T \sigmasv \nv, \qquad \xv \in \GammaIf(t),
\label{eq:normalStressLightSolid}
\end{align}
in the limit $\zp\rightarrow0$, and this Dirichlet condition on pressure is used for the pressure-Poisson problem.  Essentially, the solid traction sets the fluid traction along the interface in the light-solid limit, and the definition of the interface traction in~\eqref{eq:AMPinterfaceTraction} only confirms this assignment.  Finally, the impedance-weighted averages in~\eqref{eq:AMPinterfaceNormalVelocity} and~\eqref{eq:AMPinterfaceTangentialVelocity} reduce to
\begin{align}
\vv^I=\vv, \qquad \xv \in \GammaIf(t),
\label{eq:fluidVelocityLightSolid}
\end{align}
so that the velocity of the interface is specified by the fluid velocity, as expected, which then prescribes the velocity of the solid as a boundary condition.

%\vspace{1in}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In the TP algorithm, the velocity of the solid provides a no-slip boundary for the fluid, while the stress of the fluid sets a traction condition for the solid.  In this approach, the interface conditions in~\eqref{eq:velocityMatching} and~\eqref{eq:tractionMatching} are implemented as
%\begin{alignat}{2}
%\vv &= \vsv^{(p)}, \qquad &&\xv \in \GammaIf(t),
%\label{eq:TPVelocity}\\
%\sigmasv \nsv &= (\sigmav \nv)^{(p)}, \qquad &&\xsv \in \GammaIs.
%\label{eq:TPTraction}
%\end{alignat}
%%
%In a fractional-step scheme for the fluid, the pressure-Poisson problem requires a boundary condition for the fluid pressure.  Since the interface is considered to be a no-slip boundary in the TP scheme, a compatability condition involving the normal derivative of the pressure can be derived from the normal component of the momentum equation.  Such a condition requires the calculation of the acceleration at the interface, which is given by
%\begin{align}
%\dot{\vv}_I = \frac{1}{\rhos} \left[\left(\grads \cdot \sigmasv\right)^{(p)} + \bsv \right],
%\qquad \xv \in \GammaIf(t).
%\label{eq:interfaceAcceleration}
%\end{align}
%%
%This acceleration is then used in the normal component of the momentum equation to give
%\begin{align}
%\nv^T \grad p = - \nv^T \bigl[\mu \grad \curl \grad \curl \vv 
%  + \rho \dot{\vv}_I + \rho (\vv \cdot \grad) \vv \bigr],
%\qquad \xv \in \GammaIf(t).
%\label{eq:TPCompatibilityCondition}
%\end{align}
%%
%Following~\cite{??}, we have used the identity, $\Delta \vv = - \grad \curl \grad \curl \vv$, noting that $\grad \cdot \vv = 0$, to replace $\Delta \vv$ on the right-hand side of~\eqref{eq:TPCompatibilityCondition} in favor of the curl-curl operator.  This is done for improved stability of the fractional-step scheme.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In the ATP algorithm, the roles of the fluid and solid are reversed in the treatment of the interface conditions.  For this case, the fluid provides a no-slip wall for the solid, while the solid traction sets a boundary condition for the fluid stress.  Thus, the interface conditions give
%\begin{alignat}{2}
%\vsv &= \vv^{(p)} , \qquad &&\xsv \in \GammaIs,
%\label{eq:ATPVelocity}
%\\
%\sigmav \nv &= (\sigmasv \nsv)^{(p)}, \qquad &&\xv \in \GammaIf(t).
%\label{eq:ATPTraction}
%\end{alignat}
%%
%For the fractional-step scheme, the tangential components of~\eqref{eq:ATPTraction}, along with $\grad \cdot \vv = 0$ \textcolor{red}{(Is this true?)}, are used as a mixed-type boundary condition to advance the fluid velocity, while the normal component of~\eqref{eq:ATPTraction} is employed as a boundary condition on the fluid pressure for the pressure-Poisson problem.
%%The traction condition is broken up into two components. 
%%The tangential component is used as a mixed boundary condition for the 
%%fluid velocity and the normal component is used as a condition for
%%the pressure.
%%\begin{alignat}{2}
%%-p \esv_m^T \nv + \esv_m^T \tauv\nv &= \esv_m^T \sigmasv \nsv, 
%%\quad m = 1,2 , \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
%%\label{eq:ATPTangentialTraction}
%%\\
%%-p \nsv^T \nv + \nsv^T \tauv\nv &= \nsv^T \sigmasv \nsv
%%, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
%%\label{eq:ATPNormalTraction}
%%\end{alignat}
%%%
%%Since the velocity step comes before the pressure elliptic solve, an extrapolated
%%value for $p$ is used during the predictor, and the predicted value for $p$ is
%%used during the corrector.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The \textit{added-mass} algorithm approaches the traditional algorithm in the heavy solid limit
%($\rho/\rhos \rightarrow 0$)
%and approaches the anti-traditional algorithm in the light solid limit
%($\rhos/\rho \rightarrow 0$).
%Equation \eqref{eq:AmCharacteristicBC} is used to set the 
%tangential fluid velocity from the
%outgoing solid characteristic.
%\begin{align}
%-p \esv_m^T \nv + \esv_m^T \tauv \nv
%- \zs \esv_m^T \vv
%=
%\esv_m^T (\sigmasv \nsv)^{(p)}
%- \zs \esv_m^T \vsv^{(p)}
%,  \quad m = 1,2 
%, \quad \xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
%%\label{eq:AMPTangentialCharacteristic}
%\end{align}
%%
%The normal velocity must approach the solid velocity for heavy solids. 
%In the light solid case, the numerical scheme is used to update the normal velocity.
%In order to accommodate both limits, 
%the normal velocity is set using an impedance weighted average of the fluid and solid velocity.
%\begin{align}
%\nsv^T \vv &= \nsv^T 
%\frac{\zf \vv_f + \zp \vsv^{(p)} 
%+ \beta ((\sigmasv \nsv)^{(p)} - \sigmav \nv)}{\zf + \zp} 
%, \quad \xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
%\label{eq:AMPImpedanceWeightedAverage}
%\end{align}
%%
%As in \cite{fib2014}, we define $\zf = \rho H/\dt$ because this quantity naturally
%follows from the stability analysis.
%%
%$\vv_f$ is determined by the interior scheme for the fluid velocity. 
%If the viscous terms are treated implicitly, this condition will also be implicit.
%This is because the update for $\vv_f$ depends on the discrete Laplacian.
%%
%We choose $\beta = 0$ during the predictor step since this condition comes before 
%the pressure update. During the corrector, we choose $\beta = 1$ 
%and use predicted values for the traction jump terms.
%%
%The pressure Robin condition is a linear combination of the pressure conditions in the 
%traditional and anti-traditional scheme. This condition is obtained by matching
%the first two terms of the Taylor series for the solid and fluid velocity, given by
%\begin{align}
%\vv - \dt \vv_t = \vsv - \dt \vsv_t.
%\end{align}
%%
%Equation \eqref{eq:ACharacteristicBC} for the outgoing normal solid characteristic is used
%to eliminate $\vv$ from the equation.
%\begin{align}
%\frac{1}{\zp} \nsv^T (\sigmav \nv - \sigmasv \nsv)
%+ \dt \nsv^T \vv_t = -\dt \nsv^T \vsv_t
%\end{align}
%%
%Next the fluid momentum equation is used to eliminate $\vv_t$ and the definition of
%the fluid stress tensor is used to reveal the dependence on $p$.
%The Robin condition becomes
%\begin{align}
%-p \nsv^T \nv 
%+\frac{\zp \dt}{\rho} \nsv^T \grad p
%= 
%\nsv^T \left( \sigmasv \nsv - \tauv \nv\right)
%- \zp \dt
% \nsv^T (\nu \grad \curl \grad \curl \vv 
%  + \dot{\vv}_I +  (\vv \cdot \grad) \vv )
%\label{eq:AMPRobinCondition},
%\end{align}
%%
%for $\xv \in \GammaIf(t), \xsv \in \GammaIs.$
%Here we used $\vsv = \dot{\vv}_I.$
%The interface acceleration is calculated from equation
%\eqref{eq:interfaceAcceleration}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discrete partitioned algorithms} \label{sec:partitionedAlgorithms}

In this section, the details of the AMP algorithm are presented, along with the special cases of the TP and ATP schemes for comparison.  The description of the AMP algorithm here extends the framework of the original scheme given in~\cite{fib2014} to moving grids and deforming interfaces.  A semi-implicit predictor-corrector scheme is used to solve the fluid equations following the work in~\cite{splitStep2003}, while a second-order accurate upwind scheme is used to advance the solid equations.  The evolving fluid domain is discretized on a moving overlapping grid (see Section ???).  Let $\xv_\iv^n$ for $\iv \in \OmegaFh$ denote the time-dependent grid points belonging to the fluid domain (including grid points on the boundaries and the interface), and let $\dot{\xv}_\iv^n$ denote the velocity of the grid points at the $n\sp{{\rm th}}$ time step, $t_n$.  The indices of grid points on the interface of the fluid grid are denoted by $\iv \in \GammaIfh$.  The solid equations are discretized on its reference domain using a static overlapping grid with grid points, $\xsv_\isv$ for $\isv \in \OmegaSh$ (including boundaries and the interface), while $\isv \in \GammaIsh$ are the indicies associated with grid points on the interface of the solid grid.

In the description of the algorithm, we assume that all quantities belonging to the fluid and solid are known at $t=t_n$, and the task is to advance the solution to $t_{n+1}=t_n+\dt$.  The first five stages of the algorithm form the {\em predictor} step.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent
\textbf{Stage 1 (predict solid)}: 
Predicted values for the solid displacement are obtained by integrating~\eqref{eq:solidDisplacement} using a Lax-Wendroff scheme, i.e.
\begin{align}
\Usv_\isv^{(p)} = \Usv_\isv^n
+ \dt \Vsv_\isv^n
+ \frac{\dt^2}{2} \left(\Grads \cdot \Sigmasv_\isv^n - \bsv_\isv^n \right), 
\qquad \isv \in \OmegaSh.
\label{eq:LaxWendroffSolidDisplacement}
\end{align}
%
Predicted values for the solid velocity and stress, contained in the vector $\Qsv_\isv=(\vsv_\isv,\sigmasv_\isv)$, are obtained using a Godunov upwind scheme of the form
\begin{align}
\frac{\Qsv_\isv^{(p)} - \Qsv_\isv^n }{\dt} = 
- \sum_{m=1}^3 \frac{1}{\dxs_m} 
\left( \Fsv_{m, \; \isv}^+ - \Fsv_{m, \; \isv}^- \right)
+ \Hsv_{\isv}^n, \qquad \isv \in \OmegaSh,
\label{eq:GodunovSolidVariables}
\end{align}
%
where $\Fsv_{m, \; \isv}^\pm$ represents the upwind fluxes corresponding to the $\xs_m$ coordinate direction, and $\Hsv_{\isv}^n$ represents the contribution from the body force.  Boundary conditions are applied to the predicted values along the grid boundaries corresponding to $\xsv\in\partial\OmegaS\backslash\GammaIs$, and the ghost cells along the fluid-solid interface are extrapolated.  Note that the predicted solid quantities, $\Usv_\isv^{(p)}$ and $\Qsv_\isv^{(p)}$, can be assigned to their final values, $\Usv_\isv^{n+1}$ and $\Qsv_\isv^{n+1}$, respectively, for interior grid points and for grid points associated with the boundary $\xsv\in\partial\OmegaS\backslash\GammaIs$.  The values at grid points along the interface (and their associated ghost points) are subject to later adjustments and are considered to be predicted values at this stage.

%\textcolor{red}{(I need to re-think this.  If the solution for the solid is known everywhere at $t_n$, then the solution at $t_{n+1}$ can be computed in the interior of the solid grid and on its boundary.  Ghost points associated with non-interface boundaries can be computed as usual.  The values of the solid on the interface should be considered as predicted values at this point as they are subject to later adjustments.  Just confirm with Bill that all of this is true.  If this is true, then the stage label should be (advance solid), or something, $(p)$ should become $n+1$ probably as Dan had done originally.)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 2 (predict fluid grid motion)}: 
The computed solid displacement, $\Usv_\isv^{(p)}$, is used to predict the position, $\xv_\iv^{(p)}$ for $\iv \in \GammaIfh$, of the fluid-solid interface at $t_{n+1}$.  The overlapping-grid generator is called to move the fluid grid to match the predicted interface position, and to determine the grid velocity $\dot{\xv}_\iv^{(p)}$.  \textcolor{red}{Might point to the Overlapping Grid section for more details, or just point to the moving grid paper.  Also, Bill mentioned that there might be not be a corrector for the grid motion computed.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 3 (predict fluid velocity)}: 
The fluid velocity at $t_{n+1}$ is predicted using an explicit Adams-Bashforth scheme for the convection and pressure-gradient terms and an implicit Crank-Nicholson scheme for the viscous terms. The scheme takes the form
\begin{align}
%\frac{\vv_\iv^{(p)} - \vv_\iv^n}{\dt} = \frac{1}{2}\left(3\Lvh_E^n - \Lvh_E^{n-1}\right)
%+ \frac{1}{2}\left(\Lvh_I^{(p)} + \Lvh_I^{n}\right),
\frac{\vv_\iv^{(p)} - \vv_\iv^n}{\dt} = \frac{1}{2}\left(3\Nvh(\vv_\iv\sp n,p_\iv\sp n) - \Nvh(\vv_\iv\sp{n-1},p_\iv\sp{n-1})\right)
+ \frac{1}{2}\left(\Lvh(\vv_\iv\sp{(p)}) + \Lvh(\vv_\iv\sp n)\right),
\qquad    \iv \in \OmegaFh\backslash\GammaIfh,
\label{eq:VelocityPredictorUpdate}
\end{align}
%
%where $\Lvh_E$ and $\Lvh_I$ represent grid operators for the explicit and implicit terms, respectively, given by
where $\Nvh$ and $\Lvh$ represent grid operators associated with the explicit and implicit terms in~\eqref{eq:VelocityPredictorUpdate}, respectively, given by
\[
%\Lvh_E = - \bigl( (\vv_\iv - \dot{\xv}_\iv) \cdot \Grad \bigr) \vv_\iv 
%- \frac{1}{\rho} \Grad \,p_\iv ,\qquad
%\Lvh_I = \nu \Grad \vv_\iv.
\Nvh(\vv_\iv,p_\iv) = - \bigl( (\vv_\iv - \dot{\xv}_\iv) \cdot \Grad \bigr) \vv_\iv 
- \frac{1}{\rho} \Grad \,p_\iv ,\qquad
\Lvh(\vv_\iv) = \nu \Delta_h \vv_\iv.
\]
%
Since $\vv_\iv\sp{(p)}$ is determined implicitly in~\eqref{eq:VelocityPredictorUpdate}, boundary conditions are required for $\iv\in\partial\OmegaFh$.  Standard conditions are used for the portion of the boundary away from the interface, while care must be used in the application of the AMP interface conditions for the velocity as described in Section~\ref{sec:interfaceConditions} so that the correct limiting behaviors are obtained.  On the interface, the characteristic condition in~\eqref{eq:AMPTangentialCharacteristic} and the divergence-free constraint give
\begin{align}
 \tnv_m^T \tauv_{\iv}^{(p)} \nv + \zs \tnv_m^T \vv_\iv^{(p)} =
 \tnv_m^T \Sigmasv_\isv^{(p)} \nv
+ \zs \tnv_m^T \Vsv_{\isv}^{(p)}
,  \quad m = 1,2,
\qquad &\iv \in \GammaIfh, \; \isv \in \GammaIsh, \label{eq:AMPVelocityDiscrete} \\
\Grad\cdot\vv_\iv\sp{(p)}=0,\qquad\qquad\qquad\qquad\qquad\qquad\quad\;  % this could be handled better
\qquad &\iv \in \GammaIfh,
\label{eq:DivergenceFreeDiscrete}
\end{align}
where the interface normal, $\nv$, and tangent vectors, $\tnv_m$, are evaluated at grids points $\iv\in\GammaIfh$ along the predicted interface at $t_{n+1}$.
Since~\eqref{eq:VelocityPredictorUpdate} excludes the grids points on the interface, another set of equations are required to complete the system for the implicit time step.  Following the interface conditions in~\eqref{eq:AMPinterfaceNormalVelocity} and~\eqref{eq:AMPinterfaceTangentialVelocity}, we set
\begin{align}
 \nv^T\vv_\iv^{(p)}=\f{\zf}{\zf+\zp}\nv^T\vv_\iv^{(e)}+ \f{\zp}{\zf+\zp}\nv^T\vsv_\isv^{(p)}, \quad \phantom{m = 1,2,}\qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh,
        \label{eq:AMPinterfaceNormalVelocityDiscrete} \\
%
  \wdh{\tnv_m^T\vv_\iv^{(p)}=\tnv_m^T\vv_\iv^{(e)},  \quad m = 1,2, \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh,}
             \label{eq:AMPinterfaceTangentialVelocityDiscrete} \\
%
  \old{\tnv_m^T\vv_\iv^{(p)}={\zf\over\zf+\zs}\tnv_m^T\vv_\iv^{(e)}+{\zs\over\zf+\zs}\tnv_m^T\vsv_\isv^{(p)},  \quad m = 1,2, \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh,}
     \label{eq:AMPinterfaceTangentialVelocityDiscreteOld}
\end{align}
where $\vv_\iv^{(e)}$ is defined by
\ba
\vv_\iv^{(e)} \eqdef \vv_\iv^n + \frac{\dt}{2}\left(3\Nvh(\vv_\iv^ n,p_\iv^ n) - \Nvh(\vv_\iv^{n-1},p_\iv^{n-1})\right)
+ \frac{\dt}{2}\Big(\Lvh(\vv_\iv^{(p)}) + \Lvh(\vv_\iv^ n)\Big),
\qquad    \iv \in \GammaIfh . \label{eq:veDef}
\ea
\wdh{Note that $\vv_\iv^{(e)}$ depends on $\vv_\iv^{(p)}$ so that combining~\eqref{eq:AMPinterfaceNormalVelocityDiscrete}
and~\eqref{eq:AMPinterfaceTangentialVelocityDiscrete} with~\eqref{eq:veDef} leads to the
generalized {\em mixed-type} boundary conditions
\bas
    \nv^T\vv_\iv^{(p)} - \f{\zf}{\zf+\zp} \f{\dt}{2}\nv^T \Lvh(\vv_\iv^{(p)}) &= \f{\zf}{\zf+\zp} \nv^T\rv_\iv + \f{\zp}{\zf+\zp}\nv^T\vsv_\isv^{(p)} , \\
%
   \tnv_m^T\vv_\iv^{(p)} - \f{\dt}{2} \tnv_m^T\, \Lvh(\vv_\iv^{(p)}) &= \tnv_m^T\rv_i, 
%
\eas
where
\bas
& \rv_\iv \eqdef \vv_\iv^n + \frac{\dt}{2}\Big(3\Nvh(\vv_\iv^ n,p_\iv^ n) - \Nvh(\vv_\iv^{n-1},p_\iv^{n-1})\Big)
      + \frac{\dt}{2} \Lvh(\vv_\iv^ n).
\eas
}
%
%
%
\das{DAS: Something to discuss: I think we can replace \eqref{eq:AMPinterfaceTangentialVelocityDiscrete} with 
$\tnv_m^T \vv_\iv^{(p)} = \tnv_m^T \vv_\iv^{(e)}$ and still achieve the heavy and light solid limits.} \wdh{WDH: I agree.}
We note that the difference in the fluid and solid tractions have been omitted from the interface conditions in~\eqref{eq:AMPinterfaceNormalVelocityDiscrete}
% and~\eqref{eq:AMPinterfaceTangentialVelocityDiscrete}
since suitable approximations are not available at this stage of the algorithm.  (These terms are used in the analogous corrector step.) \textcolor{red}{Note $\zf$ is yet to be defined.}
%
%\begin{align}
%\nv^T \vv_\iv^{(p)} &= \nv^T
%\frac{\zf \vv_f^{(p)} + \zp \Vsv_\isv^{n+1} 
%+ \beta \left(\Sigmav_\iv^{(p)} \nsv - \Sigmasv_\isv^{n+1} \nv \right)}{\zf + \zp} ,
%\quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh


\wdh{\color{purple} WDH: ALTERNATIVE velocity BC's: (June 2018) 
Use conditions we had before
\ba
&  \tnv_m^T \tauv_{\iv}^{(p)} \nv + \zs \tnv_m^T \vv_\iv^{(p)} =
 \tnv_m^T \Sigmasv_\isv^{(p)} \nv
+ \zs \tnv_m^T \Vsv_{\isv}^{(p)}
,  \quad m = 1,2,
\qquad &\iv \in \GammaIfh, \; \isv \in \GammaIsh,  \\
& \grad\cdot\vv_\iv\sp{(p)}=0,\qquad\qquad\qquad\qquad\qquad\qquad\quad\;  
\qquad &\iv \in \GammaIfh,  
\ea
and add an equation that combines the normal component of characteristic equation with the interior equation 
** maybe something like this -- or scale first term by $1/\zp$ ?**
\ba
& \alpha\Big( -p^* + \nv^T\tauv^{(p)}\nv + \zp \nv^T\vv_\iv^{(p)} \Big) + (1-\alpha) \nv^T(\vv_\iv^{(p)}-\vv_\iv^{(e)}) = \alpha\Big( \nv^T\sigmasv\nv + \zp\nv^T\vvs \Big) , \\
& \alpha =\f{\zp}{\zf+\zp}.
\ea
This last condition has the limits
\bas
  & \zp\rightarrow \infty,\quad \alpha\rightarrow 1, \implies  \vv_\iv^{(p)} =  \vvs^{(p)}, \quad\text{(heavy solid)}, \\
  & \zp\rightarrow 0     ,\quad \alpha\rightarrow 0  \implies  \vv_\iv^{(p)} = \text{interior eqn}, \quad\text{(light solid)}.
\eas
}

\das{\color{orange} DAS: (6/19/18)
The AMP condition for the normal component of the velocity is
\begin{align}
-p + \nv^T \tauv \nv + \zp \nv^T \vv = \nv^T \sigmasv \nv + \zp \nv^T \vsv.
\end{align}
%
We define
\begin{align}
\tilde{\tauv} = \tauv - 2 \mu (\grad \cdot \vv) \Iv.
\end{align}
%
Since $\grad \cdot \vv = 0,$ $\tilde{\tauv}$ is equivalent to $\tauv,$
but takes a slightly different form.
\begin{align}
\tauv = 
\mu \left[\begin{array}{cc}
2 v_{1x} & v_{1y} + v_{2x} \\
v_{1y} + v_{2x} & 2v_{2y} \\
\end{array}\right],
\quad
\tilde{\tauv} = 
\mu \left[\begin{array}{cc}
- 2 v_{2y} & v_{1y} + v_{2x} \\
v_{1y} + v_{2x} & -2v_{1x} \\
\end{array}\right]
\end{align}
%
The AMP condition we apply is
\begin{align}
-p^{*} + \nv^T \tilde{\tauv}^* \nv + 2 \mu (\grad \cdot \vv) 
+ \zp \nv^T \vv = \nv^T \sigmasv \nv + \zp \nv^T \vsv.
\label{eq:newAmpCondition}
\end{align}
%
The $-p^*+\nv^T \tilde{\tauv}^* \nv$ term will not be treated implicitly and
will have a different role for the predictor and corrector.
\begin{align}
-p^{*} + \nv^T \tilde{\tauv}^* \nv
= \begin{cases}
\nv^T \sigmasv \nv, & \text{predictor} \\
-p^{(p)} + \nv^T \tilde{\tauv}^{(p)} \nv, & \text{corrector}
\end{cases}
\end{align}
%
In the pressure condition, we now replace the $\nv^T \tauv \nv$ term
with $\nv^T \tilde{\tauv} \nv.$
\begin{align}
-p - \frac{\zp \dt}{\rho} \frac{\partial p}{\partial n}
=
\nv^T \sigmasv \nv - {\blue \nv^T \tilde{\tauv} \nv}
+ \zp \dt \nv^T \partial_t \vsv + \zp \dt \nu \nv^T (\grad \times \grad \times \vv)
\end{align}
%
The velocity condition has the following limits.
\begin{align}
\begin{cases}
\nv^T \vv = \nv^T \vsv, & \zp \rightarrow \infty \\
-p^* + \nv^T \tilde{\tauv}^* \nv + 2 \mu (\grad \cdot \vv) = 
\nv^T \sigmasv \nv, & \zp \rightarrow 0
\end{cases}
\end{align}
%
The heavy solid condition sets the interface velocity.
We would typically use $\grad \cdot \vv = 0$ to set the ghost point.
The light solid condition sets the interface ghost points. The numerical scheme 
would be used to set the interface velocity.
We apply the following numerical condition. (NEW: note the minus sign)
\begin{align}
\nv^T (\vv - \vv^{(e)}) {\blue- \frac{\zp \dt}{\rho}} (\grad \cdot \vv) = 0, \label{eq:compatibility}
\end{align}
%
This condition achieves the following limits:
\begin{align}
\begin{cases}
\grad \cdot \vv = 0, & \zp \rightarrow \infty \\
\nv^T \vv = \nv^T \vv^{(e)}, & \zp \rightarrow 0
\end{cases}
\end{align}%

We can eliminate $\grad \cdot \vv$ from \eqref{eq:compatibility} and \eqref{eq:newAmpCondition}
to obtain
\begin{align}
-p^{*} + \nv^T \tilde{\tauv}^* \nv + \frac{2 \mu \rho}{\zp \dt} \nv^T (\vv-\vv^{(e)})
+ \zp \nv^T \vv = \nv^T \sigmasv \nv + \zp \nv^T \vsv.
\end{align}
%
We can solve for $\nv^T \vv$ to obtain
\begin{align}
\nv^T \vv = \frac{2 \zf \nv^T \vv^{(e)} + \zp \nv^T \vsv
+ \nv^T \sigmasv \nv - (-p^* + \nv^T \tilde{\tauv}^* \nv)}{2 \zf + \zp},
\end{align}
%
where
\begin{align}
\zf = \frac{\mu \rho}{\zp \dt}
\end{align}
This is an impedance weighted average. The stress jump terms turn on during the corrector.
This is equivalent to
\begin{align}
\nv^T \vv = \frac{2 z_\mu z_\rho \nv^T \vv^{(e)} + \zp^2 \nv^T \vsv
+ \zp (\nv^T \sigmasv \nv - (-p^* + \nv^T \tilde{\tauv}^* \nv))}
{2 z_\mu z_\rho + \zp^2},
\end{align}
%
where
\begin{align}
z_\mu = \frac{\mu}{H}, \quad z_\rho = \frac{\rho H}{\dt}
\end{align}
}



\wdh{wdh: We could simply say the TP scheme is defined by taking the limit of a heavy solid, $\zp\rightarrow\infty$ and $\zs\rightarrow\infty$
  in the above interface conditions (in practice we often
  use extrapolation for $\tv_m^T\vv_\iv$ on the ghost points for the TP scheme instead of~\eqref{eq:AMPinterfaceTangentialVelocityDiscrete}), while
  the ATP scheme takes $\zp\rightarrow 0$ and $\zs\rightarrow 0$.}
The TP scheme sets the fluid velocity on the interface to equal that of the solid, so that the interface conditions in~\eqref{eq:AMPinterfaceNormalVelocityDiscrete} and~\eqref{eq:AMPinterfaceTangentialVelocityDiscrete} are replaced by
\begin{align}
\vv_\iv^{(p)} = \Vsv_\isv^{(p)}, \quad \iv \in \GammaIfh, \; \isv \in \GammaIsh.
\label{eq:TPVelocityDiscrete}
\end{align}
\textcolor{red}{Do we also say that the divergence-free constraint is applied to specify the normal component of the fluid velocity in the ghost points, and that the tangential components of the velocity in the ghost points are extrapolated?}
The ATP scheme applies a tangential stress boundary condition on the fluid along with the divergence-free constraint.  These conditions are equivalent to the conditions in~\eqref{eq:AMPVelocityDiscrete} and~\eqref{eq:DivergenceFreeDiscrete}, but with the terms in~\eqref{eq:AMPVelocityDiscrete} involving the fluid and solid velocity dropped (effectively setting $\zs=0$), and then replacing the interface conditions in~\eqref{eq:AMPinterfaceNormalVelocityDiscrete} and~\eqref{eq:AMPinterfaceTangentialVelocityDiscrete} with $\vv_\iv^{(p)}=\vv_\iv^{(e)}$ for $\iv\in\GammaIfh$.  We note that these limiting cases for the discrete equations correspond to the limits of the continuous conditions discussed above in Section~\ref{sec:interfaceConditions}.

%++++++++++++++++




%The \textit{traditional algorithm} assigns the fluid velocity as the solid 
%velocity \eqref{eq:TPVelocity}.
%\begin{align}
%\vv_\iv^{(p)} = \Vsv_\isv^{n+1}, \quad \iv \in \GammaIfh, \; \isv \in \GammaIsh 
%\label{eq:TPVelocityDiscrete}
%\end{align}
%%
%The \textit{anti-traditional algorithm} applies a tangential stress boundary condition
%on the fluid \eqref{eq:ATPTangentialTraction}. This can be interpreted 
%as a Neumann boundary condition for the tangential velocity. 
%The scheme is used to update the normal velocity.
%\begin{alignat}{2}
%-p^{(e)}_\iv \esv_m^T \nv 
%+ \esv_m^T \tauv_\iv^{(p)} \nv 
%&= \esv_m^T \Sigmasv^{n+1}_\isv \nsv, 
%\quad m = 1,2, \quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
%\label{eq:ATPTangentialTractionDiscrete}
% \\
%\nv^T \frac{\vv_\iv^{(p)} - \vv_\iv^n}{\dt} &= 
%\nv^T \left(\frac{3}{2} \Lvh_E^n - \frac{1}{2} \Lvh_E^{n-1}
%+ \frac{1}{2} \Lvh_I^{(p)} + \frac{1}{2} \Lvh_I^{n} \right),
%\quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
%\label{eq:ATPNormalScheme}
%\end{alignat}
%%
%\wdh{
%%   I guess we also need an extrapolation condition for the ghost value of $\nv^T\vv_\iv$ to eval~\eqref{eq:ATPNormalScheme}.
%The second BC should probably be $\grad\cdot\vv=0$ instead of~\eqref{eq:ATPNormalScheme}
%}
%Since $\esv_m^T \nv$ may be nonzero, the pressure is extrapolated in time 
%to predict $p^{(e)}_\iv.$
%The \textit{added-mass partitioned algorithm} applies a characteristic 
%condition from
%the outgoing tangential solid characteristic \eqref{eq:AMPTangentialCharacteristic} 
%and sets the normal velocity using an impedance weighted average.
%\eqref{eq:AMPImpedanceWeightedAverage}.
%\begin{alignat}{2}
%-p^{(e)}_\iv \esv_m^T \nv + \esv_m^T \tauv_{\iv}^{(p)} \nv
%- \zs \esv_m^T \vv_\iv^{(p)}
%&=
%\esv_m^T \Sigmasv_\isv^{n+1} \nsv
%- \zs \esv_m^T \Vsv_{\isv}^{n+1}
%,  \quad m = 1,2,
%\quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
%\label{eq:AMPTangentialCharacteristicDiscrete}
%\\
%\nsv^T \vv_\iv^{(p)} &= \nsv^T
%\frac{\zf \vv_f^{(p)} + \zp \Vsv_\isv^{n+1} 
%+ \beta \left(\Sigmav_\iv^{(p)} \nsv - \Sigmasv_\isv^{n+1} \nv \right)}{\zf + \zp} ,
%\quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
%\label{eq:AMPImpedanceWeightedAverageDiscrete}
%\end{alignat}
%%
%The traction jump terms are turned off for the predictor ($\beta=0$).
%Here, $\vv_f$ is defined from the scheme to ensure viscous terms are taken 
%implicitly.
%\begin{align}
%\vv_f^{(p)} = \vv_\iv^{n} + 
%\dt \left(\frac{3}{2} \Lvh_E^n - \frac{1}{2} \Lvh_E^{n-1}
%+ \frac{1}{2}  \Lvh_I^{n} + \frac{1}{2} \Lvh_I^{(p)} \right)
%\label{eq:AMPVfDefinition}
%\end{align}
%%
%For all schemes, we enforce that the velocity is divergence free on the
%boundary.
%\begin{align}
%\Grad \cdot \vv_\iv^{(p)} = 0, \quad \iv \in \GammaIFh
%\label{eq:DivergenceConditionDiscrete}
%\end{align} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 4 (predict fluid pressure):}
Predicted values for the fluid pressure are obtained by solving the discrete Poisson problem
\begin{align}
\Delta_h p_\iv^{(p)} = -\rho \Grad \vv_\iv^{(p)} : \left(\Grad \vv_\iv^{(p)}  \right)^T,
\qquad \iv \in \OmegaFh,
\label{eq:predictPressure}
\end{align}
with the predicted fluid velocity from the previous stage used to determine the right-hand side of~\eqref{eq:predictPressure}.  The discrete approximation of the Robin condition in~\eqref{eq:AMPpressureBC} is
\begin{align}
-p_\iv^{(p)}
-\frac{\zp \dt}{\rho} (\nv\cdot\Grad) p_\iv^{(p)}
&= 
\nv^T \left(\Sigmasv_\isv^{(p)} \nv - \tauv_\iv^{(p)} \nv\right) 
\nonumber \\
&\qquad + \zp \dt
 \nv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} + (\vsv_t)_\isv^{(p)}\right), \qquad \iv \in \GammaIFh,
\label{eq:discreteAMPpressureBC}
\end{align}
% \wdh{wdh: change sign to match code:}
% \begin{align}
%  p_\iv^{(p)}
%  + \frac{\zp \dt}{\rho} (\nv\cdot\Grad) p_\iv^{(p)}
% &= 
% \nv^T \left(\tauv_\iv^{(p)} \nv - \Sigmasv_\isv^{(p)} \nv  \right) 
% \nonumber \\
% &\qquad - \zp \dt
%  \nv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} + (\vsv_t)_\isv^{(p)}\right), \qquad \iv \in \GammaIFh,
% \label{eq:discreteAMPpressureBC}
% \end{align}
where the acceleration of the solid along the interface appearing on the right-hand side of~\eqref{eq:discreteAMPpressureBC} is given by \wdh{wdh: The CG code may predict the solid acceleration by extrapolation in time (?)}
\[
(\vsv_t)_\isv^{(p)} = \frac{1}{\rhos} \left(\Grads \cdot \Sigmasv_\isv^{(p)} 
  -\bsv_\isv^{n+1} \right), \qquad \iv \in \GammaIFh.
\]
As before, the normal, $\nv$, in~\eqref{eq:discreteAMPpressureBC} is evaluated at grid points along the predicted interface.

\wdh{wdh: Again we could simply say the TP scheme is defined by taking the liimit of a heavy solid, $\zp\rightarrow\infty$ and $\zs\rightarrow\infty$
  in the above interface conditions, while
  the ATP scheme takes $\zp\rightarrow 0$ and $\zs\rightarrow 0$.}
In the TP scheme, the Robin condition in~\eqref{eq:discreteAMPpressureBC} is replaced by a discrete approximate of~\eqref{eq:pressureBCHeavySolid} given by
\[
-(\nv\cdot\Grad) p_\iv^{(p)} = \nsv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} + (\vsv_t)_\isv^{(p)}\right), \qquad \iv \in \GammaIFh,
\]
whereas the ATP scheme uses an approximation of~\eqref{eq:normalStressLightSolid} given by
\[
-p_\iv^{(p)} = \nv^T \left(\Sigmasv_\isv^{(p)} \nv - \tauv_\iv^{(p)} \nv\right), \qquad \iv \in \GammaIFh.
\]

%The \textit{traditional algorithm} applies a compatibility condition for 
%the pressure gradient using the normal component of the momentum equation
%\eqref{eq:TPCompatibilityCondition}.
%\begin{align}
%\nv^T \Grad p_\iv^{(p)} = - \nv^T (\mu \Grad \curl \Grad \curl \vv_\iv^{(p)} 
%  + \rho \dot{\vv}_{\iv}^{(p)} + \rho (\vv_\iv^{(p)} \cdot \Grad) \vv_\iv^{(p)} ),
%\quad \iv \in \GammaIFh
%\end{align}
%%
%The interface acceleration is
%calculated from the solid equations \eqref{eq:interfaceAcceleration}.
%\begin{align}
%\dot{\vv}_{\iv}^{(p)} = \frac{1}{\rhos} \left(\Grads \cdot \Sigmasv_\isv^{n+1} 
%  -\bsv_\isv^{n+1} \right), 
%\quad 
%\iv \in \GammaIfh, \; \isv \in \GammaIsh.
%\end{align}
%%
%The \textit{anti-traditional algorithm} applies a normal traction boundary condition
%to set the pressure \eqref{eq:ATPNormalTraction}.
%\begin{align}
%-p_\iv^{(p)} \nsv^T \nv + \nsv^T \tauv_\iv^{(p)} \nv &= \nsv^T \Sigmasv_\isv^{n+1} \nsv,
%\quad \iv \in \GammaIFh, \; \isv \in \GammaIsh
%\end{align}
%%
%The \textit{added-mass algorithm} applies a Robin condition for the
%pressure \eqref{eq:AMPRobinCondition}.
%\begin{align}
%-p_\iv^{(p)} \nsv^T \nv 
%+\frac{\zp \dt}{\rho} \nsv^T \Grad p_\iv^{(p)}
%=\;& 
%\nsv^T \left(\Sigmasv_\isv^{n+1} \nsv - \tauv_\iv^{(p)} \nv\right) 
%\nonumber \\
%&- \zp \dt
% \nsv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} 
%  + \dot{\vv}_\iv^{(p)} +  (\vv_\iv^{(p)} \cdot \Grad) \vv_\iv^{(p)} \right),
%\end{align}
%%
%for $\iv \in \GammaIFh, \isv \in \GammaISh.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 5 (predict solid interface):}
Having obtained predicted values for the fluid velocity and stress on the interface, we now specify the anologous quantities for the solid in the AMP algorithm using
\begin{alignat}{2}
\Vsv_\isv^{(p)} &= \vv_\iv^{(p)}, \qquad &&\isv \in \GammaIsh,\quad \iv \in \GammaIfh,
\label{eq:predictSolidInterfaceVelocity}\\
\Sigmasv^{(p)}_{\isv} \nv &= \Sigmav^{(p)}_\iv \nv, \qquad &&\isv \in \GammaIsh,\quad \iv \in \GammaIfh.
\label{eq:predictSolidInterfaceStress}
\end{alignat}

\wdh{WDH: June 27, 2018: We could also maybe add the jump in sigma and jump in v to these projections (*check signs below*)?}
\das{DAS: 6/19/18
We now apply a projection to get interface values.
\begin{alignat}{2}
\nv^T \Vsv_\isv^I &= \frac{\zf}{\zf+\zp} \nv^T \vv_\iv^{(p)}
     + \frac{\zp}{\zf+\zp} \nv^T \Vsv_\isv^{(p)}
     + {\blue \f{1}{\zf+\zp}\Big( \nv^T\Sigmasv^{(p)}_\iv\nv - \nv^T\Sigmav^{(p)}_\iv\nv \Big)},
      \qquad &&\isv \in \GammaIsh,\quad \iv \in \GammaIfh,\\
% 
\tv_m^T \Vsv_\isv^I &= \frac{\zf}{\zf+\zs} \tv_m^T \vv_\iv^{(p)}
     + \frac{\zs}{\zf+\zs} \tv_m^T \Vsv_\isv^{(p)}
     + {\blue \f{1}{\zf+\zs}\Big( \tv_m^T\Sigmasv^{(p)}_\iv\nv - \tv_m^T\Sigmav^{(p)}_\iv\nv \Big)},
     \qquad &&\isv \in \GammaIsh,\quad \iv \in \GammaIfh,\\
%
\nv^T \Sigmasv^I_{\isv} \nv &= \frac{\zf^{-1}}{\zf^{-1}+\zp^{-1}}\nv^T\Sigmav^{(p)}_\iv \nv
+ \frac{\zp^{-1}}{\zf^{-1}+\zp^{-1}} \nv^T\Sigmasv^{(p)} \nv
    + {\blue \f{1}{\zf^{-1}+\zp^{-1}}\Big( \nv^T\vsv^{(p)}_\iv - \nv^T\vv^{(p)}_\iv \Big)},
     \qquad &&\isv \in \GammaIsh,\quad \iv \in \GammaIfh. \\
% 
\tv_m^T \Sigmasv^I_{\isv} \nv &= \frac{\zf^{-1}}{\zf^{-1}+\zs^{-1}}\tv_m^T\Sigmav^{(p)}_\iv \nv
    + \frac{\zs^{-1}}{\zf^{-1}+\zs^{-1}} \tv_m^T\Sigmasv^{(p)} \nv
    + {\blue \f{1}{\zf^{-1}+\zs^{-1}}\Big( \tv_m^T\vsv^{(p)}_\iv - \tv_m^T\vv^{(p)}_\iv \Big)},
        \qquad &&\isv \in \GammaIsh,\quad \iv \in \GammaIfh.
\label{eq:predictSolidInterfaceStress}
\end{alignat}
%
The stability analysis suggests
\begin{align}
\zf = \frac{\rho \nu}{h},
\end{align}
%
where $h$ is the characteristic grid spacing.
}


\wdh{WDH: Conditions~\eqref{eq:predictedSolidInterfaceVelocityCompatibility} and~\eqref{eq:predictedSolidStressGhostBC} below 
are now always used to get the ghost values for the solid I think.
}

In the TP scheme, we use~\eqref{eq:predictSolidInterfaceStress} to set the predicted solid stress on the interface,
but then compute the solid velocity on the interface using the compatibility condition
\begin{align}
\lambdas \left(\Grads \cdot \Vsv_\isv^{(p)} \right) \nsv
+ \mus \left(\Grads \Vsv_\isv^{(p)} + \left(\Grads \Vsv_\isv^{(p)} \right)^T  \right) \nsv
 &= \dot{\Sigmasv}_{\isv} \nsv,
\qquad \isv \in \GammaIsh 
\label{eq:predictedSolidInterfaceVelocityCompatibility}
\end{align}
which can be interpreted as a set of discrete Neumann conditions for the components of $\Vsv_\isv^{(p)}$.  The time-derivative of the solid stress on the right-hand side of~\eqref{eq:predictedSolidInterfaceVelocityCompatibility} is obtained using a second-order accurate approximation involving $\Sigmasv_{\isv}^{(p)}$ and the solid stress at $t_n$ and $t_{n-1}$.  \textcolor{red}{(Is this correct?)}.  The ATP scheme, on the other hand, sets the solid velocity using~\eqref{eq:predictSolidInterfaceVelocity}, but then computes the predicted solid stress on the interface using the compability condition
\begin{align}
\Grads \cdot \Sigmasv_\isv^{(p)} = \rho \dot{\Vsv}_\isv - \bsv_\isv^{n+1},
\qquad \isv \in \GammaIsh, \label{eq:predictedSolidStressGhostBC}
\end{align}
which can be interpreted as a set of discrete Neumann conditions for the components of $\Sigmasv_\isv^{(p)}$.  \textcolor{red}{(Double check here, but this appears to be only 3 conditions for the 6 components of stress in 3D, noting symmetry of the stress tensor.  I don't recall offhand how the remaining components are set.)}  The acceleration of the solid on the interface is computed using a finite-difference approximation similar to that described to compute the stress for the TP scheme.

%In the continuous case, either a displacement, traction, or 
%mixed boundary condition is required for the solid problem to be well posed.
%However in the discrete case, 
%a numerical boundary condition is required for each variable. 
%The \textit{traditional algorithm} applies a traction boundary condition.
%\begin{align}
%\Sigmasv^{n+1}_{\isv} \nsv = \Sigmav^{(p)}_\iv \nv, 
%\quad \iv \in \GammaIfh, \; \isv \in \GammaIsh
%\end{align}
%% 
%The compatibility condition enforces
%compatibility of the velocity with the time derivative of the
%stress tensor at the interface. 
%This can be interpreted as a Neumann condition.
%\begin{align}
%\lambdas \left(\Grads \cdot \Vsv_\isv^{n+1} \right) \nsv
%+ \mus \left(\Grads \Vsv_\isv^{n+1} + \left(\Grads \Vsv_\isv^{n+1} \right)^T  \right) \nsv
% &= \dot{\Sigmasv}^{n+1}_{\isv} \nsv,
%\quad \isv \in \GammaIsh 
%\end{align}
%%
%For the \textit{anti-traditional algorithm}, a velocity boundary condition is applied.
%\begin{align}
%\Vsv_\isv^{n+1} = \vv_\iv^{(p)},
%\quad \iv \in \GammaIfh, \; \isv \in \GammaIsh
%\end{align}
%%
%The momentum equation is used as a compatibility condition for solid stress. 
%Similar to the previous compatibility condition, this is a Neumann type condition.
%\begin{align}
%\Grads \cdot \Sigmasv_\isv^{n+1} = \rho \dot{\Vsv}_\isv^{n+1} - \bsv_\isv^{n+1},
%\quad \isv \in \GammaIsh
%\end{align}
%%
%The \textit{added-mass algorithm} applies both the velocity and stress.
%\begin{alignat}{2}
%\Vsv_\isv^{n+1} &= \vv_\iv^{(p)},
%\quad &&\iv \in \GammaIfh, \; \isv \in \GammaIsh \\
%\Sigmasv^{n+1}_{\isv} \nsv &= \Sigmav^{(p)}_\iv \nv, 
%\quad &&\iv \in \GammaIfh, \; \isv \in \GammaIsh
%\end{alignat}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\medskip
This completes the set of stages used for the predictor step of the algorithm.  The remaining ??? stages form the {\em corrector} step.  \textcolor{red}{(Will wait to get clarification of earlier comments before finishing the editing of this section.)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 6 (correct fluid grid motion):}  \textcolor{red}{It may be that the current value for the solid displacement is not used to corrent the grid as Bill mentioned.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 7 (correct fluid velocity):}
The corrected fluid velocity, $\vv_\iv^{n+1}$, is obtained by solving the implicit equations
\begin{align}
\frac{\vv_\iv^{n+1} - \vv_\iv^n}{\dt} = \frac{1}{2}\left(\Nvh(\vv_\iv^{(p)},p_\iv^{(p)}) + \Nvh(\vv_\iv^{n},p_\iv^{n})\right)
+ \frac{1}{2}\left(\Lvh(\vv_\iv^{n+1}) + \Lvh(\vv_\iv^ n)\right),
\qquad    \iv \in \OmegaFh\backslash\GammaIfh,
\label{eq:VelocityCorrectorUpdate}
\end{align}
together with the AMP interface conditions 
\begin{align}
 \tnv_m^T \tauv_{\iv}^{n+1} \nv + \zs \tnv_m^T \vv_\iv^{n+1} =
 \tnv_m^T \Sigmasv_\isv^{n+1} \nv
+ \zs \tnv_m^T \Vsv_{\isv}^{n+1}
,  \quad m = 1,2,
\qquad &\iv \in \GammaIfh, \; \isv \in \GammaIsh, \label{eq:AMPVelocityDiscreteCorrect} \\
\Grad\cdot\vv_\iv^{n+1}=0,\qquad\qquad\qquad\qquad\qquad\qquad\quad\;  % this could be handled better
\qquad &\iv \in \GammaIfh,
\label{eq:DivergenceFreeDiscreteCorrect}
\end{align}
\wdh{and 
\begin{align}
\nv^T\vv_\iv^{n+1}=&{\zf\over\zf+\zp}\nv^T\vv_\iv^{(e)}+{\zp\over\zf+\zp}\nv^T\vsv_\isv^{n+1} \nonumber\\
&\qquad+{1\over\zf+\zp}\nv^T\bigl((\sigmasv\nv)_\isv^{n+1}-(\sigmav\nv)_\iv^{(p)}\bigr), \quad \phantom{m = 1,2,}\qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh,
\label{eq:AMPinterfaceNormalVelocityDiscreteC} \\
\tnv_m^T\vv_\iv^{n+1}=&\tnv_m^T\vv_\iv^{(e)} ,  \quad m = 1,2, \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh,
\label{eq:AMPinterfaceTangentialVelocityDiscreteC}
\end{align}
}
\old{
\begin{align}
\nv^T\vv_\iv^{n+1}=&{\zf\over\zf+\zp}\nv^T\vv_\iv^{(e)}+{\zp\over\zf+\zp}\nv^T\vsv_\isv^{n+1} \nonumber\\
&\qquad+{1\over\zf+\zp}\nv^T\bigl((\sigmasv\nv)_\isv^{n+1}-(\sigmav\nv)_\iv^{(p)}\bigr), \quad \phantom{m = 1,2,}\qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh,
\label{eq:AMPinterfaceNormalVelocityDiscreteC} \\
\tnv_m^T\vv_\iv^{n+1}=&{\zf\over\zf+\zs}\tnv_m^T\vv_\iv^{(e)}+{\zs\over\zf+\zs}\tnv_m^T\vsv_\isv^{n+1} \nonumber\\
&\qquad+{1\over\zf+\zs}\tnv_m^T\bigl((\sigmasv\nv)_\isv^{n+1}-(\sigmav\nv)_\iv^{(p)}\bigr),  \quad m = 1,2, \qquad \iv \in \GammaIfh, \; \isv \in \GammaIsh,
\label{eq:AMPinterfaceTangentialVelocityDiscreteC}
\end{align}
}
where $\vv_\iv^{(e)}$ is now defined by
\[
\vv_\iv^{(e)} = \vv_\iv^n + \frac{\dt}{2}\left(\Nvh(\vv_\iv^{(p)},p_\iv^{(p)}) + \Nvh(\vv_\iv^{n},p_\iv^{n})\right)
+ \frac{\dt}{2}\left(\Lvh(\vv_\iv^{n+1}) + \Lvh(\vv_\iv^n)\right),
\qquad    \iv \in \GammaIfh.
\]

The boundary conditions for the TP and ATP scheme are handled in an analogous fashion following the discussion of these schemes in Stage~3.

%\begin{align}
%\nv^T\vv^I={\zf\over\zf+\zp}\nv^T\vv+{\zp\over\zf+\zp}\nv^T\vsv+{1\over\zf+\zp}\nv^T\bigl(\sigmasv\nv-(\sigmav\nv)^I\bigr), \quad \phantom{m = 1,2,}\qquad \xv \in \GammaIf(t),
%\label{eq:AMPinterfaceNormalVelocity} \\
%\tnv_m^T\vv^I={\zf\over\zf+\zs}\tnv_m^T\vv+{\zs\over\zf+\zs}\tnv_m^T\vsv+{1\over\zf+\zs}\tnv_m^T\bigl(\sigmasv\nv-(\sigmav\nv)^I\bigr) ,  \quad m = 1,2, \qquad \xv \in \GammaIf(t).
%\label{eq:AMPinterfaceTangentialVelocity}
%\end{align}



%Apply an Adams-Moulton corrector to the explicit terms \eqref{eq:ExplicitTerms} 
%and Crank-Nicholson to the implicit terms \eqref{eq:ImplicitTerms}. 
%Since the implicit scheme is the same for the predictor and corrector, the 
%left-hand-side matrix does not need to be rebuilt for the corrector.
%The corrector scheme is given by
%\begin{align}
%\frac{\vv_\iv^{n+1} - \vv_\iv^n}{\dt} = \frac{1}{2} 
%\left(\Lvh_E^{(p)} + \Lvh_E^{n}
%+  \Lvh_I^{n+1} + \Lvh_I^{n}  \right),
%\quad    \iv \in \OmegaFh.
%\end{align}
%%
%For the \textit{traditional algorithm}, the fluid velocity is set as the solid 
%velocity. This condition is equation \eqref{eq:TPVelocityDiscrete}, but with
%$\vv^{(p)}_\iv$ replaced with $\vv^{n+1}_\iv.$
%%
%For the \textit{anti-traditional algorithm},
%a boundary condition is applied on the fluid tangential stress 
%and the normal velocity is updated using the scheme.
%In the corrector version of equation \eqref{eq:ATPTangentialTractionDiscrete},
%$p_\iv^{(e)}$ is replaced by $p_\iv^{(p)}$ and $\tauv_\iv^{(p)}$ is replaced
%by $\tauv_\iv^{n+1}.$ The condition on the normal velocity now mimics the corrector scheme,
%given by
%\begin{align}
%\nv^T \frac{\vv_\iv^{n+1} - \vv_\iv^n}{\dt} = 
%\nv^T \left(\frac{1}{2} \Lvh_E^{(p)} + \frac{1}{2} \Lvh_E^{n}
%+ \frac{1}{2} \Lvh_I^{n+1} + \frac{1}{2} \Lvh_I^{n} \right),
%\quad \iv \in \GammaIfh, \; \isv \in \GammaIsh.
%\end{align}
%%
%For the \textit{added-mass algorithm}, the tangential characteristic and the
%impedance weighted average conditions are set.
%The conditions are equivalent to \eqref{eq:AMPTangentialCharacteristicDiscrete}
%and \eqref{eq:AMPImpedanceWeightedAverageDiscrete}, but with 
%$\vv^{(p)}_\iv$, $p_\iv^{(e)}$, $\tauv_\iv^{(p)}$, and $\vv_f^{(p)}$
%replaced with $\vv^{n+1}_\iv$, $p_\iv^{(p)}$, $\tauv_\iv^{n+1}$,
%and $\vv_f^{n+1},$ respectively. For the corrector, the traction jump turns are switched on
%($\beta = 1$). $\vv_f^{n+1}$ is defined from using the corrector scheme,
%\begin{align}
%\vv_f^{(p)} = \vv_\iv^{n} + 
%\dt \left(\frac{1}{2} \Lvh_E^{(p)} + \frac{1}{2} \Lvh_E^{n}
%+ \frac{1}{2}  \Lvh_I^{n} + \frac{1}{2} \Lvh_I^{n+1} \right).
%\end{align}
%%
%As in the predictor, the divergence of the velocity is set to $0$ on the boundary,
%\eqref{eq:DivergenceConditionDiscrete}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 8 (correct fluid pressure):}
Corrected values for the pressure corrector are determined using the equations in Stage~4, but with predicted values replaced with corrected values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\medskip\noindent
\textbf{Stage 9 (correct solid interface):}
The solid interface boundary conditions during this stage are determined using the 
equations in Stage~5, but with predicted values replaced with corrected values.

\medskip
We note that the AMP scheme is stable without the corrector step. The corrector will 
improve the stability region when convection terms are dominant over the viscous terms.
The corrector comes at a low computational cost because the matrices formed for the velocity
and pressure in the predictor stages are the same ones used in the corresponding corrector stages.
%
On the other hand, the traditional scheme may need additional sub-iterations 
to stabilize the approximation. The algorithm for under-relaxed sub-iterations
is presented and analyzed in the stability section.  \textcolor{red}{May need to re-visit this statement depending on what is ultimately written for the next section}.



==> texFiles/algorithm-orig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Algorithm} \label{sec:algorithm}

In this section, the AMP algorithm and two fundamental partitioned algorithms will
be discussed.
In a time stepping loop, the first step is advancing the solid displacement to
the next time level. The solid displacement is used to deform the fluid grid.
%
Following this, the fluid and solid solvers are called. 
%
An upwind Godunov scheme is used to update the solid velocity and stress.
Since this scheme is explicit, the interface and boundary data is predicted 
and will be overwritten in a later step.
%
A semi-implicit solver is used to update the fluid velocity.
The diffusion terms are taken implicitly
and the convection and pressure terms are taken explicitly 
using a predictor-corrector scheme.
%
The pressure Poisson equation is solved with an elliptic solver. 
The key ingredient for stability lies in the boundary condition for pressure at the interface.
%
After this step, the solid interface data is updated with fluid data.
%
If a corrector or sub-iteration is required, this process is repeated.

\subsection{Continuous Interface Conditions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the \textit{traditional} algorithm, the fluid sees the solid as
a no-slip wall and applies a traction on the solid. 
\begin{alignat}{2}
\vv &= \vsv^{(p)}, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:TPVelocity}\\
\sigmasv \nsv &= (\sigmav \nv)^{(p)}, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:TPTraction}
\end{alignat}
%
During the pressure solve,
a compatibility boundary condition for the normal pressure gradient is given using 
the normal component of the momentum equation. This requires computation 
of the interface acceleration, given by
\begin{align}
\dot{\vv}_I = \frac{1}{\rhos} \left( \grads \cdot \sigmasv + \bsv \right),
\quad \xsv \in \GammaIs 
.
\label{eq:interfaceAcceleration}
\end{align}
%
The compatibility condition is 
\begin{align}
\nv^T \grad p = - \nv^T (\mu \grad \curl \grad \curl \vv 
  + \rho \dot{\vv}_I + \rho (\vv \cdot \grad) \vv ),
\quad \xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:TPCompatibilityCondition},
\end{align}
%
where we used $\Delta \vv = - \grad \curl \grad \curl \vv$, 
which is true because $\grad \cdot \vv = 0.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the \textit{anti-traditional} algorithm, the roles of the 
fluid and solid are reversed
The solid sees the fluid as a no slip wall
and applies a traction on the fluid.
\begin{alignat}{2}
\vsv &= \vv^{(p)} , \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:ATPVelocity}
\\
\sigmav \nv &= (\sigmasv \nsv)^{(p)}, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:ATPTraction}
\end{alignat}
%
The traction condition is broken up into two components. 
The tangential component is used as a mixed boundary condition for the 
fluid velocity and the normal component is used as a condition for
the pressure.
\begin{alignat}{2}
-p \esv_m^T \nv + \esv_m^T \tauv\nv &= \esv_m^T \sigmasv \nsv, 
\quad m = 1,2 , \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:ATPTangentialTraction}
\\
-p \nsv^T \nv + \nsv^T \tauv\nv &= \nsv^T \sigmasv \nsv
, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:ATPNormalTraction}
\end{alignat}
%
Since the velocity step comes before the pressure elliptic solve, an extrapolated
value for $p$ is used during the predictor, and the predicted value for $p$ is
used during the corrector.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The \textit{added-mass} algorithm approaches the traditional algorithm in the heavy solid limit
($\rho/\rhos \rightarrow 0$)
and approaches the anti-traditional algorithm in the light solid limit
($\rhos/\rho \rightarrow 0$).
Equation \eqref{eq:AmCharacteristicBC} is used to set the 
tangential fluid velocity from the
outgoing solid characteristic.
\begin{align}
-p \esv_m^T \nv + \esv_m^T \tauv \nv
- \zs \esv_m^T \vv
=
\esv_m^T (\sigmasv \nsv)^{(p)}
- \zs \esv_m^T \vsv^{(p)}
,  \quad m = 1,2 
, \quad \xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:AMPTangentialCharacteristic}
\end{align}
%
The normal velocity must approach the solid velocity for heavy solids. 
In the light solid case, the numerical scheme is used to update the normal velocity.
In order to accommodate both limits, 
the normal velocity is set using an impedance weighted average of the fluid and solid velocity.
\begin{align}
\nsv^T \vv &= \nsv^T 
\frac{\zf \vv_f + \zp \vsv^{(p)} 
+ \beta ((\sigmasv \nsv)^{(p)} - \sigmav \nv)}{\zf + \zp} 
, \quad \xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:AMPImpedanceWeightedAverage}
\end{align}
%
As in \cite{fib2014}, we define $\zf = \rho H/\dt$ because this quantity naturally
follows from the stability analysis.
%
$\vv_f$ is determined by the interior scheme for the fluid velocity. 
If the viscous terms are treated implicitly, this condition will also be implicit.
This is because the update for $\vv_f$ depends on the discrete Laplacian.
%
We choose $\beta = 0$ during the predictor step since this condition comes before 
the pressure update. During the corrector, we choose $\beta = 1$ 
and use predicted values for the traction jump terms.
%
The pressure Robin condition is a linear combination of the pressure conditions in the 
traditional and anti-traditional scheme. This condition is obtained by matching
the first two terms of the Taylor series for the solid and fluid velocity, given by
\begin{align}
\vv - \dt \vv_t = \vsv - \dt \vsv_t.
\end{align}
%
Equation \eqref{eq:ACharacteristicBC} for the outgoing normal solid characteristic is used
to eliminate $\vv$ from the equation.
\begin{align}
\frac{1}{\zp} \nsv^T (\sigmav \nv - \sigmasv \nsv)
+ \dt \nsv^T \vv_t = -\dt \nsv^T \vsv_t
\end{align}
%
Next the fluid momentum equation is used to eliminate $\vv_t$ and the definition of
the fluid stress tensor is used to reveal the dependence on $p$.
The Robin condition becomes
\begin{align}
-p \nsv^T \nv 
+\frac{\zp \dt}{\rho} \nsv^T \grad p
= 
\nsv^T \left( \sigmasv \nsv - \tauv \nv\right)
- \zp \dt
 \nsv^T (\nu \grad \curl \grad \curl \vv 
  + \dot{\vv}_I +  (\vv \cdot \grad) \vv )
\label{eq:AMPRobinCondition},
\end{align}
%
for $\xv \in \GammaIf(t), \xsv \in \GammaIs.$
Here we used $\vsv = \dot{\vv}_I.$
The interface acceleration is calculated from equation
\eqref{eq:interfaceAcceleration}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discrete Numerical Algorithm}

In this section, the details of the numerical implementation 
for each FSI algorithm will be presented. 
This description also
extends the framework of \cite{fib2014} to moving grids and deforming interfaces.
A semi-implicit predictor-corrector 
scheme \cite{splitStep2003} is used to solve the fluid equations. 
The fluid grid is defined on grid points $\iv \in \OmegaFh$ 
and is allowed to deform in time. The grid-point location at time
$t^n$ is denoted by $\xv_\iv^n.$ The velocity is
denoted by $\dot{\xv}_\iv^n$ and is used in the calculation of
the convective acceleration.
An upwind finite volume scheme is used to solve the solid equations
which are discretized on grid points $\isv \in \OmegaSh.$
The following is the numerical algorithm. \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Begin predictor.} 

\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 1 - solid update}: 
Equation \eqref{eq:solidDisplacement} for the solid displacement 
is integrated using a Lax-Wendroff scheme.
\begin{align}
\Usv_\isv^{n+1} = \Usv_\isv^n
+ \dt \Vsv_\isv^n
+ \frac{\dt^2}{2} \left(\Grads \cdot \Sigmasv_\isv^n - \bsv_\isv^n \right), 
\quad \isv \in \OmegaSh
\label{eq:LaxWendroffSolidDisplacement}
\end{align}
%
The solid velocity and stress components, contained in vector $\Qsv,$
are updated using a Godunov upwind scheme
of the form
\begin{align}
\frac{\Qsv_\isv^{n+1} - \Qsv_\isv^n }{\dt} = 
- \sum_{m=1}^3 \frac{1}{\dxs_m} 
\left( \Fsv_{m, \; \isv}^+ - \Fsv_{m, \; \isv}^- \right)
+ \Hsv_{\isv}^n, \quad \isv \in \OmegaSh
\label{eq:GodunovSolidVariables}
\end{align}
%
where $\Fsv_m$ represents the upwind flux corresponding to the $\xs_m$ coordinate
and $\Hsv$ represents the contribution from body forces.
Boundary conditions are applied to non-interface boundaries and the 
interface ghost cells are extrapolated.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 2 - grid deformation}: 
The fluid grid is then deformed to match the solid deformation at the interface
\eqref{eq:geometryMatching}. Many grid generation strategies can be used including 
trans-finite interpolation and overlapping grids. \todo{more details.} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 3 - fluid velocity}: 
The fluid velocity is then predicted using an Adams-Bashforth scheme for the convective and 
pressure terms and a Crank-Nicholson scheme for the viscous terms. The 
scheme is
\begin{align}
\frac{\vv_\iv^{(p)} - \vv_\iv^n}{\dt} = \frac{3}{2} \Lv_E^n - \frac{1}{2} \Lv_E^{n-1}
+ \frac{1}{2}  \Lv_I^{(p)} + \frac{1}{2} \Lv_I^{n},
\quad    \iv \in \OmegaFh
\label{eq:VelocityPredictorUpdate}
\end{align}
%
where $\Lv_E$ and $\Lv_I$ represent grid operators for the explicit and implicit terms,
respectively, given by
\begin{align}
\Lv_E &= - \left( \left(\vv_\iv - \dot{\xv}_\iv\right) \cdot \Grad \right) \vv_\iv 
- \frac{1}{\rho} \Grad p_\iv 
\label{eq:ExplicitTerms}
\\
\Lv_I &= \nu \Grad \vv_\iv
\label{eq:ImplicitTerms}.
\end{align}
%
The \textit{traditional algorithm} assigns the fluid velocity as the solid 
velocity \eqref{eq:TPVelocity}.
\begin{align}
\vv_\iv^{(p)} = \Vsv_\isv^{n+1}, \quad \iv \in \GammaIfh, \; \isv \in \GammaIsh 
\label{eq:TPVelocityDiscrete}
\end{align}
%
The \textit{anti-traditional algorithm} applies a tangential stress boundary condition
on the fluid \eqref{eq:ATPTangentialTraction}. This can be interpreted 
as a Neumann boundary condition for the tangential velocity. 
The scheme is used to update the normal velocity.
\begin{alignat}{2}
-p^{(e)}_\iv \esv_m^T \nv 
+ \esv_m^T \tauv_\iv^{(p)} \nv 
&= \esv_m^T \Sigmasv^{n+1}_\isv \nsv, 
\quad m = 1,2, \quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
\label{eq:ATPTangentialTractionDiscrete}
 \\
\nv^T \frac{\vv_\iv^{(p)} - \vv_\iv^n}{\dt} &= 
\nv^T \left(\frac{3}{2} \Lv_E^n - \frac{1}{2} \Lv_E^{n-1}
+ \frac{1}{2} \Lv_I^{(p)} + \frac{1}{2} \Lv_I^{n} \right),
\quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
\label{eq:ATPNormalScheme}
\end{alignat}
%
\wdh{
%   I guess we also need an extrapolation condition for the ghost value of $\nv^T\vv_\iv$ to eval~\eqref{eq:ATPNormalScheme}.
The second BC should probably be $\grad\cdot\vv=0$ instead of~\eqref{eq:ATPNormalScheme}
}
Since $\esv_m^T \nv$ may be nonzero, the pressure is extrapolated in time 
to predict $p^{(e)}_\iv.$
The \textit{added-mass partitioned algorithm} applies a characteristic 
condition from
the outgoing tangential solid characteristic \eqref{eq:AMPTangentialCharacteristic} 
and sets the normal velocity using an impedance weighted average.
\eqref{eq:AMPImpedanceWeightedAverage}.
\begin{alignat}{2}
-p^{(e)}_\iv \esv_m^T \nv + \esv_m^T \tauv_{\iv}^{(p)} \nv
- \zs \esv_m^T \vv_\iv^{(p)}
&=
\esv_m^T \Sigmasv_\isv^{n+1} \nsv
- \zs \esv_m^T \Vsv_{\isv}^{n+1}
,  \quad m = 1,2,
\quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
\label{eq:AMPTangentialCharacteristicDiscrete}
\\
\nsv^T \vv_\iv^{(p)} &= \nsv^T
\frac{\zf \vv_f^{(p)} + \zp \Vsv_\isv^{n+1} 
+ \beta \left(\Sigmav_\iv^{(p)} \nsv - \Sigmasv_\isv^{n+1} \nv \right)}{\zf + \zp} ,
\quad &\iv \in \GammaIfh, \; \isv \in \GammaIsh
\label{eq:AMPImpedanceWeightedAverageDiscrete}
\end{alignat}
%
The traction jump terms are turned off for the predictor ($\beta=0$).
Here, $\vv_f$ is defined from the scheme to ensure viscous terms are taken 
implicitly.
\begin{align}
\vv_f^{(p)} = \vv_\iv^{n} + 
\dt \left(\frac{3}{2} \Lv_E^n - \frac{1}{2} \Lv_E^{n-1}
+ \frac{1}{2}  \Lv_I^{n} + \frac{1}{2} \Lv_I^{(p)} \right)
\label{eq:AMPVfDefinition}
\end{align}
%
For all schemes, we enforce that the velocity is divergence free on the
boundary.
\begin{align}
\Grad \cdot \vv_\iv^{(p)} = 0, \quad \iv \in \GammaIFh
\label{eq:DivergenceConditionDiscrete}
\end{align} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 4 - fluid pressure:}
During the next stage, the fluid pressure equation is solved.
\begin{align}
\Delta_h p_\iv^{(p)} = -\rho \Grad \vv_\iv^{(p)} : \left(\Grad \vv_\iv^{(p)}  \right)^T,
\quad \iv \in \OmegaFh
\end{align}
%
The \textit{traditional algorithm} applies a compatibility condition for 
the pressure gradient using the normal component of the momentum equation
\eqref{eq:TPCompatibilityCondition}.
\begin{align}
\nv^T \Grad p_\iv^{(p)} = - \nv^T (\mu \Grad \curl \Grad \curl \vv_\iv^{(p)} 
  + \rho \dot{\vv}_{\iv}^{(p)} + \rho (\vv_\iv^{(p)} \cdot \Grad) \vv_\iv^{(p)} ),
\quad \iv \in \GammaIFh
\end{align}
%
The interface acceleration is
calculated from the solid equations \eqref{eq:interfaceAcceleration}.
\begin{align}
\dot{\vv}_{\iv}^{(p)} = \frac{1}{\rhos} \left(\Grads \cdot \Sigmasv_\isv^{n+1} 
  -\bsv_\isv^{n+1} \right), 
\quad 
\iv \in \GammaIfh, \; \isv \in \GammaIsh.
\end{align}
%
The \textit{anti-traditional algorithm} applies a normal traction boundary condition
to set the pressure \eqref{eq:ATPNormalTraction}.
\begin{align}
-p_\iv^{(p)} \nsv^T \nv + \nsv^T \tauv_\iv^{(p)} \nv &= \nsv^T \Sigmasv_\isv^{n+1} \nsv,
\quad \iv \in \GammaIFh, \; \isv \in \GammaIsh
\end{align}
%
The \textit{added-mass algorithm} applies a Robin condition for the
pressure \eqref{eq:AMPRobinCondition}.
\begin{align}
-p_\iv^{(p)} \nsv^T \nv 
+\frac{\zp \dt}{\rho} \nsv^T \Grad p_\iv^{(p)}
=\;& 
\nsv^T \left(\Sigmasv_\isv^{n+1} \nsv - \tauv_\iv^{(p)} \nv\right) 
\nonumber \\
&- \zp \dt
 \nsv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} 
  + \dot{\vv}_\iv^{(p)} +  (\vv_\iv^{(p)} \cdot \Grad) \vv_\iv^{(p)} \right),
\end{align}
%
for $\iv \in \GammaIFh, \isv \in \GammaISh.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 5 - solid interface:}
In the continuous case, either a displacement, traction, or 
mixed boundary condition is required for the solid problem to be well posed.
However in the discrete case, 
a numerical boundary condition is required for each variable. 
The \textit{traditional algorithm} applies a traction boundary condition.
\begin{align}
\Sigmasv^{n+1}_{\isv} \nsv = \Sigmav^{(p)}_\iv \nv, 
\quad \iv \in \GammaIfh, \; \isv \in \GammaIsh
\end{align}
% 
The compatibility condition enforces
compatibility of the velocity with the time derivative of the
stress tensor at the interface. 
This can be interpreted as a Neumann condition.
\begin{align}
\lambdas \left(\Grads \cdot \Vsv_\isv^{n+1} \right) \nsv
+ \mus \left(\Grads \Vsv_\isv^{n+1} + \left(\Grads \Vsv_\isv^{n+1} \right)^T  \right) \nsv
 &= \dot{\Sigmasv}^{n+1}_{\isv} \nsv,
\quad \isv \in \GammaIsh 
\end{align}
%
For the \textit{anti-traditional algorithm}, a velocity boundary condition is applied.
\begin{align}
\Vsv_\isv^{n+1} = \vv_\iv^{(p)},
\quad \iv \in \GammaIfh, \; \isv \in \GammaIsh
\end{align}
%
The momentum equation is used as a compatibility condition for solid stress. 
Similar to the previous compatibility condition, this is a Neumann type condition.
\begin{align}
\Grads \cdot \Sigmasv_\isv^{n+1} = \rho \dot{\Vsv}_\isv^{n+1} - \bsv_\isv^{n+1},
\quad \isv \in \GammaIsh
\end{align}
%
The \textit{added-mass algorithm} applies both the velocity and stress.
\begin{alignat}{2}
\Vsv_\isv^{n+1} &= \vv_\iv^{(p)},
\quad &&\iv \in \GammaIfh, \; \isv \in \GammaIsh \\
\Sigmasv^{n+1}_{\isv} \nsv &= \Sigmav^{(p)}_\iv \nv, 
\quad &&\iv \in \GammaIfh, \; \isv \in \GammaIsh
\end{alignat}

\end{itemize}
\noindent \textbf{End predictor.}\\ \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Begin corrector.}

\begin{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 6 - velocity corrector:}
Apply an Adams-Moulton corrector to the explicit terms \eqref{eq:ExplicitTerms} 
and Crank-Nicholson to the implicit terms \eqref{eq:ImplicitTerms}. 
Since the implicit scheme is the same for the predictor and corrector, the 
left-hand-side matrix does not need to be rebuilt for the corrector.
The corrector scheme is given by
\begin{align}
\frac{\vv_\iv^{n+1} - \vv_\iv^n}{\dt} = \frac{1}{2} 
\left(\Lv_E^{(p)} + \Lv_E^{n}
+  \Lv_I^{n+1} + \Lv_I^{n}  \right),
\quad    \iv \in \OmegaFh.
\end{align}
%
For the \textit{traditional algorithm}, the fluid velocity is set as the solid 
velocity. This condition is equation \eqref{eq:TPVelocityDiscrete}, but with
$\vv^{(p)}_\iv$ replaced with $\vv^{n+1}_\iv.$
%
For the \textit{anti-traditional algorithm},
a boundary condition is applied on the fluid tangential stress 
and the normal velocity is updated using the scheme.
In the corrector version of equation \eqref{eq:ATPTangentialTractionDiscrete},
$p_\iv^{(e)}$ is replaced by $p_\iv^{(p)}$ and $\tauv_\iv^{(p)}$ is replaced
by $\tauv_\iv^{n+1}.$ The condition on the normal velocity now mimics the corrector scheme,
given by
\begin{align}
\nv^T \frac{\vv_\iv^{n+1} - \vv_\iv^n}{\dt} = 
\nv^T \left(\frac{1}{2} \Lv_E^{(p)} + \frac{1}{2} \Lv_E^{n}
+ \frac{1}{2} \Lv_I^{n+1} + \frac{1}{2} \Lv_I^{n} \right),
\quad \iv \in \GammaIfh, \; \isv \in \GammaIsh.
\end{align}
%
For the \textit{added-mass algorithm}, the tangential characteristic and the
impedance weighted average conditions are set.
The conditions are equivalent to \eqref{eq:AMPTangentialCharacteristicDiscrete}
and \eqref{eq:AMPImpedanceWeightedAverageDiscrete}, but with 
$\vv^{(p)}_\iv$, $p_\iv^{(e)}$, $\tauv_\iv^{(p)}$, and $\vv_f^{(p)}$
replaced with $\vv^{n+1}_\iv$, $p_\iv^{(p)}$, $\tauv_\iv^{n+1}$,
and $\vv_f^{n+1},$ respectively. For the corrector, the traction jump turns are switched on
($\beta = 1$). $\vv_f^{n+1}$ is defined from using the corrector scheme,
\begin{align}
\vv_f^{(p)} = \vv_\iv^{n} + 
\dt \left(\frac{1}{2} \Lv_E^{(p)} + \frac{1}{2} \Lv_E^{n}
+ \frac{1}{2}  \Lv_I^{n} + \frac{1}{2} \Lv_I^{n+1} \right).
\end{align}
%
As in the predictor, the divergence of the velocity is set to $0$ on the boundary,
\eqref{eq:DivergenceConditionDiscrete}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 7 - pressure corrector}:
Corrected values for the pressure corrector are determined using the equations in 
\textbf{stage 4}, but with predicted values replaced with corrected values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\item[] \textbf{Stage 8 - solid interface}:
The solid interface boundary conditions during this stage are determined using the 
equations in \textbf{stage 5}, but with predicted values replaced with corrected values.

\end{itemize}
\noindent \textbf{End Corrector} \\

We note that the AMP scheme is stable without the corrector step. The corrector will 
improve the stability region when convection terms are dominant over the viscous terms.
The corrector comes at a low computational cost because the matrices formed for the velocity
and pressure predictor are the same for the corrector.
%
On the other hand, the traditional scheme may need additional sub-iterations 
to stabilize the approximation. The algorithm for under-relaxed sub-iterations
is presented and analyzed in the stability section.


==> texFiles/analysis-2-16-18.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Stability analysis of a FSI model problem} \label{sec:analysis}

% todo
%
% replace \lambda_y with \ly etc.
%
\noindent
\textcolor{red}{(Current thoughts on editing this section: (1) Describe the model problem at a continuous level.  Simplify the notation by $v_2\rightarrow v$, $\sigma_{21}\rightarrow\sigma_1$, etc., basically dropping the 2 since everything is in the vertical direction anyway.  BTW: I wonder if it is too much to say that the solid velocity and stress tend to zero as $y\rightarrow-\infty$.  I think this would only be true if this property also holds for the initial data.  Requiring that the solution is bounded at infinity should be enough.  I wonder if this issue was discussed during the writing of FIB???  (2) Describe how the equations are approximated.  (3) Describe the AMP algorithm for the approximation of the model equations.  Here I think it is helpful to point back to the previously discussed algorithm so that the mapping between the general algorithm and the one in the model problem analysis is clear.  (4) Perform the analysis for the AMP scheme and give the results.  (5) State the corresponding results for the TP and ATP schemes, but leave any details to an appendix.)}

\input texFiles/rectangularModelProblemCartoon

% \wdh{\bf This is from fib:
% In this section, we perform a stability analysis of the AMP algorithm applied to
% the two-dimensional FSI model problem MP-IA.  In this problem, the fluid is
% taken as inviscid and the solid is treated as an acoustic solid that only
% supports motion in the vertical direction. The governing equations for the model
% are given by~\eqref{eq:MP-IA}.
% % We are interested in the stability of different frequencies in the $x$ direction and thus consider a periodic problem in $x$. 
% We consider a semi-infinite solid domain ($\Hs=\infty$) and look for solutions in the solid that have finite $L_2$-norm (which implies the solutions decay to zero as $y\rightarrow\infty$).  The bottom boundary condition on the fluid at $y=-H$ is chosen as $\sigma=0$ (i.e. $p=0$).
% }

In this section, the stability of the second order accurate
AMP, TP, and ATP algorithms are explored for a simplified two-dimensional 
model problem. This extends the stability results of first order 
accurate schemes in \cite{fib2014}.
In this analysis, the TP scheme is considered 
without under-relaxed sub-iterations. 
To supplement this, an analysis of the TP scheme with sub-iterations is performed.
In the model problem, we assume the fluid is inviscid and the solid 
is acoustic with motion constrained to vertical direction. 
We are interested in the stability of different frequencies 
in the $x$ direction and thus consider a periodic problem in $x$. 
The solid domain is semi-infinite ($\Hs \rightarrow \infty)$ and we require solutions
to decay to zero as $y \rightarrow -\infty.$ The fluid pressure is given to be 
$p=0$ at the top boundary. The interface conditions enforce matching of the 
velocity and traction at $y=0.$
The governing equations and boundary conditions are given by
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t \vfy + \partial_y p = 0, & \xv\in\OmegaF \\
(\partial_x^2 + \partial_y^2) p =0, & \xv\in\OmegaF \\
p = 0, & x\in(0,L), \quad y=H
\end{cases} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsy = \partial_x \ssx + \partial_y \ssy, & \xv\in\OmegaS \\
\partial_t \ssx = \rhos\cp^2 \partial_x \vsy, & \xv\in\OmegaS \\
\partial_t \ssy = \rhos\cp^2 \partial_y \vsy, & \xv\in\OmegaS \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 < \infty, & y\rightarrow - \infty
\end{cases} \\
\text{Interface: } &\begin{cases}
\vfy = \vsy, & x\in(0,L), \quad y = 0 \\
p = -\ssy, & x\in(0,L), \quad y = 0.
\end{cases}
\end{align}

% governing equations
% ------------------------------------------------------------------------------------------------
\subsection{Discretization}

The fluid and the solid are discretized in the $x$ direction by a uniform grid defined by
grid spacing $\dx = L/N_x$ and grid points $x_\ell = \ell \Delta x$ for 
$\ell = 0, 1,\ldots N_x.$ 
Since the problem is periodic in the $x$ direction, each
variable can be represented as a discrete Fourier series, e.g.
\begin{align}
q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2}  e^{2 \pi i k x_\ell/ L} \hat{q}_k (y,t), 
\qquad \ell=0,1,2,\ldots,N_x. \label{eq:discreteFourier}
\end{align}
%
Here, $q_\ell(y,t) \approx q(x_\ell,y,t)$ and $\hat{q}_k$ are Fourier coefficients.
For convenience, $N_x$ is assumed to be an even integer. Let
$k_x = 2 \pi k /L$ be the normalized wave number for each 
$k = -N_x/2,-N_x/2+1, \ldots, N_x/2.$ The governing equations are now transformed
to obtain equations for the Fourier coefficients. The transformed
equations for the fluid and solid become
\begin{alignat}{2}
\rho \partial_t \vfyh + \partial_y \ph &= 0, \quad && y\in(0,H), \\
\partial_y^2 \ph - k_x^2 \ph &=0, \quad && y\in(0,H),
\label{eq:phEqn} \\
% \end{alignat}
% %
% The transformed equations for the solid are
% \begin{alignat}{2}
\rhos \partial_t \vsyh &= i k_x \ssxh + \partial_y \ssyh, \quad && y\in(-\infty,0) ,
\label{eq:vsyhEqn} \\
\partial_t \ssxh &= i k_x \rhos\cp^2 \vsyh, && y\in(-\infty,0), 
\label{eq:ssxhEqn} \\
\partial_t \ssyh &= \rhos\cp^2 \partial_y \vsyh, && y\in(-\infty,0)
\label{eq:ssyhEqn}.
\end{alignat}
%
For notational convenience, the hats and subscripts 
on the Fourier coefficients are suppressed.
It is convenient to consider the solid equations in characteristic form. 
Equations \eqref{eq:vsyhEqn}--\eqref{eq:ssyhEqn} are diagonalized to derive the
following characteristic variables
\begin{align}
\ac = \ssyh - \rhos\cp\vsyh, \quad
\bc = \ssyh + \rhos\cp\vsyh, \quad
\dc = \ssxh.
\end{align}
%
$\bc$ and $\ac$ are the incoming and outgoing characteristics, respectively,
and are obtained by substituting $\nv=[0,-1]^T$ in equations \eqref{eq:ACharacteristic}
and \eqref{eq:BCharacteristic}.
These characteristics satisfy
\begin{alignat}{2}
\partial_t \ac + \cp \partial_y \ac &= -i k_x \cp \dc, \quad && y\in(-\infty,0), 
\label{eq:advSrcA} \\
\partial_t \bc - \cp \partial_y \bc &= i k_x \cp \dc, \quad && y\in(-\infty,0),
\label{eq:advSrcB} \\
\partial_t \dc &= \frac{i k_x \cp}{2} (\bc - \ac), \quad && y\in(-\infty,0),
\label{eq:SrcD}
\end{alignat}
%
which is a system of advection equations with a source. $\ac$ corresponds to the
$\cp^+$ characteristic and $\bc$ corresponds to the $\cp^-$ characteristic.

The solid characteristic variables are discretized in the $y$ direction using a
uniform collocated grid with grid spacing $\dy$ and grid points
$y_j = j\dy,$ for $j = 1, 0, -1, -2 \ldots$. 
Although staggered grids are used for the analysis in 
\cite{BanksSjogreen2011,lrb2013,fib2014}, the analysis for second order interface
conditions is significantly simpler on a collocated grid. 
Let $\Delta t$ be the time step and let $t^n = n \Delta t.$
The solid equations are solved with a dissipative scheme to in order to exploit 
some useful properties in the analysis.
A second order centered scheme was chosen to minimize the stencil to 
three grid points (a second order upwind scheme requires a five point stencil).
The schemes for equations \eqref{eq:advSrcA}--\eqref{eq:advSrcB}
are derived by taking a Taylor series in time and replacing time derivatives
with spacial derivatives. 
Define the grid functions
$\ac^n_j \approx \ac(y_j, t^n), \bc^n_j \approx \bc(y_j, t^n),$ and
$\dc^n_j \approx \dc(y_j,t^n),$
then the Taylor series for $\ac$ is given by
\begin{align}
\ac(y_j,t^{n+1}) =\;& \ac(y_j,t^{n}) + 
\dt \partial_t \ac(y_j,t^{n}) + 
\frac{\dt^2}{2} \partial_t^2 \ac(y_j,t^{n}) + O(\dt^3)\\
=\;& \ac(y_j,t^{n}) - 
\cp \dt \partial_y \ac(y_j,t^{n}) + 
\frac{\cp^2 \dt^2}{2} \partial_y^2 \ac(y_j,t^{n}) \nonumber \\
&- i k_x \cp \dt \dc(y_j,t^n)
+ \frac{i k_x \cp^2 \dt^2}{2} \partial_y \dc(y_j,t^n) \nonumber \\
&+ \frac{k_x^2 \cp^2 \dt^2}{4} \left(\bc(y_j,t^{n}) - \ac(y_j,t^{n}) \right) + O(\dt^3).
\end{align}
% \begin{align}
% \ac^{n+1}_j &= \ac^{n}_j + 
% \dt \partial_t \ac^{n}_j + 
% \frac{\dt^2}{2} \partial_t^2 \ac^{n}_j + O(\dt^3)\\
% \ac^{n+1}_j &= \ac^{n}_j - 
% \cp \dt \partial_y \ac^{n}_j + 
% \frac{\cp^2 \dt^2}{2} \partial_y^2 \ac^{n}_j 
% + i k_x \cp \dt \dc^n_j
% - \frac{k_x^2 \cp^2 \dt^2}{4} (\bc^{n}_{j} - \ac^{n}_{j}) + O(\dt^3).
% \end{align}
%
A similar series can be derived for $\bc.$
The spacial derivatives are approximated by centered second order finite
difference formulas. Define the undivided difference operators
$\delta_+ u_j = u_{j+1} - u_j,$ 
$\delta_- u_j = u_j - u_{j-1},$ and $\delta_0 u_j = u_{j+1} - u_{j-1}$ 
for an arbitrary grid function $u_j.$ The scheme for $\ac$ and $\bc$
can be written as 
\begin{align}
\ac^{n+1}_{j} &= \ac^{n}_j - 
\frac{\lambda_y}{2} \delta_0 \ac^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \ac^{n}_j 
- i \lambda_x \dc^n_j
+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
+ \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j)  \label{eq:aLax} \\
\bc^{n+1}_{j} &= \bc^{n}_j + 
\frac{\lambda_y}{2} \delta_0 \bc^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \bc^{n}_j 
+ i \lambda_x \dc^n_j
+ \frac{i \lambda_x \lambda_y}{4} \delta_0 \dc^{n}_j
- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j) \label{eq:bLax}
\end{align}
%
where $\lambda_x = k_x \cp \dt$ and $\lambda_y = \cp \dt / \dy.$
This is a Lax-Wendroff scheme for an advection equation with a source.
After advancing $\ac$ and $\bc$ to the next time level, $\dc$ can be
advanced with a simple quadrature. Since a non-dissipative pseudo-spectral approximation
is used in the $x$ direction, 
% the trapezoidal rule 
a BDF scheme
is used to stabilize the approximation.
% \begin{align}
% \dc^{n+1}_j &= \dc^{n}_j + \frac{i \lambda_x}{4}
% \left(\bc^{n+1}_j - \ac^{n+1}_j + \bc^n_j - \ac^n_j \right). \label{eq:dTrap}
% \end{align}
\begin{align}
\dc^{n+1}_j &= \frac{4}{3}\dc^{n}_j - \frac{1}{3} \dc^{n-1}+ \frac{i \lambda_x}{3}
\left(\bc^{n+1}_j - \ac^{n+1}_j \right). \label{eq:dTrap}
\end{align}
%
The $\cp^+$ characteristic, $\ac,$ will be extrapolated to the interface ghost point.
Additionally, the solution must be bounded as $y \rightarrow -\infty.$
\begin{alignat}{2}
\ac^n_{1} &= 2 \ac^n_{0} - \ac^n_{-1}, \quad && \\
\vert \ac^n_j \vert^2 +
\vert \bc^n_j \vert^2 +
\vert \dc^n_j \vert^2 &< \infty, \quad &&\text{as } j \rightarrow -\infty
\label{eq:bcInf}
\end{alignat}
%
The interface condition will determine $b_{1}^n,$ and the initial conditions will 
define $a_j^0, b_j^0,$ and $d_j^0$ for $j = 0,1,2,3,\ldots$.
For reference, the Fourier 
coefficients of the solid velocity and stress components are related to the characteristic 
variables by
\begin{align}
(\vsyh)_j^n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \quad
(\ssyh)_j^n = \frac{1}{2} (\bc^n_j+\ac^n_j), \quad
(\ssxh)_j^n = \dc^n_j.
\end{align}

The fluid variables are kept continuous in $y$ but discrete in time.
The pressure sub-problem solves
\begin{align}
p_{yy}^{n}(y) - k_x^2 p^{n}(y) &= 0, \label{eq:pressureSubProblem}\\
p^{n}(H) &= 0, \label{eq:pressureTopBoundary}
\end{align}
% 
with an additional algorithm dependent interface condition at $y=0.$ The
general solution to \eqref{eq:pressureSubProblem}--\eqref{eq:pressureTopBoundary}
is
\begin{align}
p^n(y) = p_I^n \frac{\sinh(k_x(H-y))}{\sinh(k_x H)}, \label{eq:pressureSubProblemSolution}
\end{align}
%
where $p_I^n$ is the interface pressure at time $t^n$, determined by the interface condition.
The pressure gradient at the interface, needed to advance the fluid interface velocity,
is given by
\begin{align}
\partial_y p^n(0) = - \frac{p_I^n}{\Heff},
\end{align}
%
where
\begin{align}
\Heff = \frac{\tanh(k_x H)}{k_x}.
\end{align}
%
For the 1D problem ($k_x = 0$), $\Heff = H.$ When $k_x \rightarrow \infty,$ 
$\Heff \rightarrow 0.$
For this simplified model problem analysis, only the fluid velocity at the interface
is needed, which will be denoted as $v_f^n$ at time $t^n.$

\subsubsection{AMP interface conditions}

Following section \ref{sec:partitionedAlgorithms}, the AMP algorithm is applied
to the simplified model problem.
In the limit of a heavy solid, the AMP conditions approach a 
no-slip condition for the fluid and a traction condition for the solid.
In the light solid limit, the conditions approach a traction condition for 
the fluid and a no-slip condition for the solid.
Only the fluid solution at the interface is necessary to advance the solid in time.
The AMP algorithm is given by the following.

\listAlgorithm{AMP Algorithm (added-mass partitioned)}{
\item Advance the solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
$j = 0,\, -1, \, -2, \, -3, \, \ldots$.

\item Obtain the predicted velocity and traction from the solid.
\begin{align}
v_s^{n+1} &= \frac{1}{2 \zp} \left(\bc^{n+1}_0 - \ac^{n+1}_0 \right) \\
\sigma_s^{n+1} &= \frac{1}{2} \left(\bc^{n+1}_0 + \ac^{n+1}_0 \right)
\end{align}

\item Advance the fluid interface velocity using a BDF scheme on
the fluid momentum equation.
\begin{align}
v_f^{n+1} = \frac{4}{3} v_I^n - \frac{1}{3} v_I^{n-1} 
+ \frac{2\dt}{3 \rho \Heff} 
 p_I^{n+1} 
\end{align}
%

\item Set the interface velocity as the impedance weighted average
of the fluid and solid velocities using $\zf = \rho H/\dt$. 
\begin{align}
v_I^{n+1} = \frac{\zf v_f + \zp v_s}{\zf + \zp} 
\end{align}

\item Calculate the interface acceleration using a second order accurate
backward difference formula.
\begin{align}
\dot{v}_I^{n+1} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{n+1} 
  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
\end{align}

\item Solve the Poisson equation for the fluid pressure with
the following AMP Robin condition specified at $y=0.$
\begin{alignat}{2}
-\ph^{n+1}+\frac{\zp \dt}{\rho} \ph_y^{n+1} &= 
\sigma_s^{n+1} - \zp \dt \dot{v}_I^{n+1}, \quad && y = 0, 
\end{alignat}

Given the general solution in equation \eqref{eq:pressureSubProblemSolution},
the interface pressure is 
\begin{align}
p_I^{n+1} &= \frac{1}{M \eta+1} 
\rho \dot{v}_I \Heff
 - \frac{M \eta}{M \eta+1} \sigma_s,
\end{align}
%
where
\begin{align}
M &= \frac{\rho H}{\zp \dt} = \frac{\rho H}{\rhos \cp \dt}, \label{eq:AcousticMassRatio} \\
\eta &= \frac{\Heff}{H} = \frac{\tanh(k_x H)}{k_x H} \label{eq:Eta}
\end{align}

\item 
%Set the interface traction $\sigma_I^{n+1} = -p_I^{n+1}.$
Set the incoming $\cp^-$ characteristic, $\bc,$ using the interface velocity and stress.
%$\delta = \rho/\rhos.$
\begin{align}
\bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right).
% \bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 
% \left[\frac{1}{1+\delta} 
% \left(2 \sigma_I^{n+1} - \frac{\ac^{n+1}_{1} + \ac^{n+1}_{-1}}{2} \right)
% +\frac{\delta}{1+\delta} \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right) \right].
\end{align}

\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$
\begin{align}
\ac^{n+1}_1 = 2 \ac^{n+1}_0 - \ac^{n+1}_{-1}
\end{align}

} \\

% The solid is advanced on the interior and the boundary in the first two steps.
% Next the fluid velocity is obtained in step 3. 
% The interface velocity is projected using an impedance weighted average of the
% fluid and solid values. 
% This is used to determine the interface acceleration, which is used in
% the pressure solution for step 7.
% Afterwards, the solid boundary conditions are applied to obtain the ghost points.

The acoustic mass ratio, $M$, defined in \eqref{eq:AcousticMassRatio},
is the ratio of the mass of the fluid in a column of height 
$H$ over the mass of a solid with the same cross section
of height $\cp \dt,$ or the distance a p-wave travels in a single time step.
The mass ratio is a measure of the prevalence of the added mass effect.
For a heavy solid, the mass ratio is small and therefore added mass effects are small. 
The mass ratio is inversely proportional to $\rhos$ and $\dt,$ therefore
added mass effects can arise both in light solids and solids with a fine mesh.
$\eta$ is the ratio between the effective fluid column height and the true fluid column height.

The key behavior of the AMP algorithm is observed by taking the heavy and
light solid limits. When $\zp \rightarrow \infty,$ the interface velocity
and pressure approach the following limits.
\begin{align}
v_I^{n+1} &= 
\begin{cases}
v_s, & \zp \rightarrow \infty \\
v_f, & \zp \rightarrow 0 
\end{cases} \\
p_I^{n+1} &= 
\begin{cases}
-\sigma_s, & \zp \rightarrow \infty \\
\rho \dot{v}_I \Heff, & \zp \rightarrow 0 
\end{cases}
\end{align}
%
Corresponding algorithms for the TP (traditional partitioned) and the
ATP (anti-traditional partitioned) schemes can be applied to the simplified model 
problem following section \ref{sec:partitionedAlgorithms}.


\subsection{Stability analysis of AMP, TP, and ATP schemes}

We will now look for normal mode solutions to the discretization in terms of an
amplification factor, $\amp.$ Let
\begin{align}
\ac^{n}_j = \amp^n \tac_j, \quad 
\bc^{n}_j = \amp^n \tbc_j, \quad 
\dc^{n}_j = \amp^n \tdc_j,
\end{align}
%
where tilde variables are spacial grid functions. The scheme is said to be weakly
stable if there are no non-trivial solutions where $|\amp| > 1.$ Our strategy for
determining the stability region will be to search only for unstable modes, $|A| > 1.$ 
First, the analysis is split into a spacial and temporal problem. The tilde variables 
will be determined from the interior discretization and boundary condition as 
$y \rightarrow -\infty.$ Solutions for the amplification factor will be found by
finding non-trivial solutions when the normal mode anzatz is
substituted into the interface conditions.

Let $\tacv = [\tac,\tbc,\tdc]^T,$ then equations \eqref{eq:aLax}--\eqref{eq:dTrap}
can be written as a system of linear second order difference equations.
\begin{align}
(H_0 + H_1 \delta_0 + H_2 \delta_+ \delta_-) \tacv_j = 0
\label{eq:DifferenceEquation}
\end{align}
%
where
% \begin{align}
% H_{0} &= 
% \left[\begin{array}{ccc}
% -\frac{\lx^2}{4}& \frac{\lx^2}{4}&-i \lx \\
% \frac{\lx^2}{4}&-\frac{\lx^2}{4}&i \lx \\
% - \frac{i \lx}{4} & \frac{i \lx}{4}&0 
% \end{array}\right], \\
% H_{1} &= 
% \left[\begin{array}{ccc}
% -\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
% 0&\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
% 0 & 0&0 
% \end{array}\right], \\
% H_{2} &= 
% \left[\begin{array}{ccc}
% \frac{\ly^2}{2} &0&0 \\
% 0&\frac{\ly^2}{2}&0 \\
% 0 & 0&0 
% \end{array}\right].
% \end{align}
\begin{align}
H_{0} &= 
-A^2 
\left[\begin{array}{ccc}
1&0&0\\
0&1&0 \\
\frac{i \lx}{3}&-\frac{i \lx}{3}&1
\end{array}\right] 
+A 
\left[\begin{array}{ccc}
1- \frac{\lx^2}{4}&\frac{\lx^2}{4}&-i \lx\\
\frac{\lx^2}{4}&1-\frac{\lx^2}{4}&i \lx \\
0&0&\frac{4}{3}
\end{array}\right] 
-
\left[\begin{array}{ccc}
0&0&0\\
0&0&0\\
0&0&\frac{1}{3}
\end{array}\right] \\
H_{1} &= 
A \left[\begin{array}{ccc}
-\frac{\ly}{2} &0&\frac{i \lx \ly}{4} \\
0&\frac{\ly}{2}&\frac{i \lx \ly}{4} \\
0 & 0&0 
\end{array}\right], \\
H_{2} &= 
A \left[\begin{array}{ccc}
\frac{\ly^2}{2} &0&0 \\
0&\frac{\ly^2}{2}&0 \\
0 & 0&0 
\end{array}\right].
\end{align}
%
Solutions are sought of the form $\tacv_j = \rev \p^j.$ This is substituted into 
equation \eqref{eq:DifferenceEquation} to obtain
\begin{align}
\left( H_0 + H_1 \left(\p - \frac{1}{\p}\right)
+ H_2 \left(\p - 2 + \frac{1}{\p} \right) \right) \rev = 0 \label{eq:evProblem}
\end{align}
%
Non trivial solutions for $\p$ are found when the above problem is singular,
therefore we search for $\p$ that satisfies
\begin{align}
\det\bigg{(}H_0 + H_1 \left(\p - \frac{1}{\p}\right)
+ H_2 \left(\p - 2 + \frac{1}{\p} \right) \bigg{)} = 0. \label{eq:quarticPhi}
\end{align}
%
There are four roots for $\p.$ Since we require the solid variables to 
be bounded as
$y \rightarrow -\infty,$ \eqref{eq:bcInf}, we are only interested in solutions 
where $|\p|^j \le 1$ as $j \rightarrow -\infty.$ Therefore, only roots where
$|\p| \ge 1$ are solutions to the boundary condition.

\textbf{Lemma}: \textit{when $|A| > 1$ and the CFL condition is satisfied,
the roots satisfy}
\begin{align}
|\phi_1| > 1, \quad |\phi_2| > 1, \quad |\phi_3| < 1, \quad |\phi_4| < 1.
\label{eq:SizeOfEigenvalues}
\end{align}
%
This result follows using a similar argument to that of
\cite{DifferenceApproximationsForTheInitialBoundary}.
First, we will show that the scheme applied to the Cauchy problem is stable
(Fourier stability). Let $\phi = e^{i \omega}$. 
% Noting that 
% $(I+H_{-1})^{-1} = I-H_{-1},$ the solution for the amplification factor reduces 
% to the following eigenvalue problem for $A$.
% \begin{align}
% A \rv = (I - H_{-1})
% \left( I + H_0 + H_1 \left(e^{i \omega} - e^{-i \omega}\right)
% + H_2 \left(e^{i \omega} - 2 + e^{-i \omega} \right) \right) \rev.
% \end{align}
The solution for the amplification factor reduces to the following eigenvalue problem for $A$.
\begin{align}
\left( H_0 + H_1 \left(e^{i \omega} - e^{-i \omega}\right)
+ H_2 \left(e^{i \omega} - 2 + e^{-i \omega} \right) 
 \right) \rev = 0 \label{eq:evProblem}
\end{align}
%
For a reasonable CFL restriction on $\lx$ and $\ly$, $|A| \le 1$
for $0 \le \omega \le 2 \pi$ and therefore the Cauchy scheme is stable.
Since $|A| \le 1$ when $|\phi| = 1,$ 
we have that $|\phi| \ne 1$ when $|A| > 1.$
This proves that as long as $|A| > 1$
and $\lx$ and $\ly$ are within the CFL restriction,
a change in parameters will not cause $\phi$ to cross the unit circle, $|\phi|=1.$
Due to this, it is only necessary to prove that the conditions in \eqref{eq:SizeOfEigenvalues}
hold for one set of parameters. For $\lx=0,$ the difference scheme reduces to 
a Lax-Wendroff scheme, where it is well known (e.g. \cite{GKSII}) that 
the condition in equation \eqref{eq:SizeOfEigenvalues} holds.

Due to the above Lemma, we can now write the general solution as
\begin{align}
\acv^n_j = \amp^n \left(k_1 \rev_1 \p_1^j + 
k_2 \rev_2 \p_2^j \right). \label{eq:EigenvectorExpansion}
\end{align}
%
Let $\rev_n = [\qn{n},\rn{n},\sn{n}]^T$ for $n = 1,2.$
Using the third component of equation \eqref{eq:DifferenceEquation}, 
$\sn{n}$ can be found in terms of $\qn{n}$ and $\rn{n}$.
\begin{align}
% \sn{n} = \frac{i \lx}{4} \frac{A+1}{A-1} (\rn{n} - \qn{n}) 
\sn{n} = \frac{A^2 i \lx}{3 A^2- 4 A + 1} (\rn{n} - \qn{n})
\end{align}
%
When $\acv_j$ is plugged into the interface conditions, a system of equations arise.
\begin{align}
\dMat \kv= \left[\begin{array}{cc}
\dComp_{11} & \dComp_{12} \\
\dComp_{21} & \dComp_{22}
\end{array}\right] 
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right] = 0
\label{eq:StabilitySystem}
\end{align}
%
The coefficients of the matrix $\dMat$ are provided in
\ref{sec:StabilityAnalysisDetails}.
For non-trivial solutions, we look for solutions of $\amp$ such that
\begin{align}
\det(\dMat) = \dComp_{11} \dComp_{22} - \dComp_{12} \dComp_{21} = 0.
\end{align}
%
We first proceed with an analysis of the 1D case ($\lx \rightarrow 0$). After finding 
1D solutions for $\amp,$ numerical continuation in $\lx$ is used to follow the 
evolution of $\amp$ as the wave number in the $x$ direction increases.

\subsubsection{1D scheme}

When $\lx \rightarrow 0,$ the equations in the solid become two uncoupled advection 
equations for the $\cp^+$ characteristic, $\ac,$ and the $\cp^-$ characteristic, $\bc.$
The solid scheme is Lax-Wendroff without source corrections. 
Equation \eqref{eq:DifferenceEquation}
simplifies to 
\begin{align}
A \tac_j = \left( 1 - \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tac_j, \quad
A \tbc_j = \left( 1 + \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tbc_j
\end{align}
%
The solutions to the eigenvalues, $\p,$ are given by
\begin{align}
\p_{\bc,\pm} = {\frac {{\lambda_{{y}}}^{2}+A-1 \pm \sqrt {2\,A{\lambda_{{y}}}^{2}+{A}^{2}-{
\lambda_{{y}}}^{2}-2\,A+1}}{\lambda_{{y}} \left( \lambda_{{y}}-1
 \right) }}, \quad 
\p_{\ac,\pm} =  \frac{\lambda_y - 1}{\lambda_y + 1} \p_{\bc,\pm}
\end{align}
%
Following the properties in equation \eqref{eq:SizeOfEigenvalues},
let the corresponding spacial eigenvalues be $\phi_1$ and $\phi_3$ for $\tbc$
and $\phi_2$ and $\phi_4$ for $\tac.$
%Due to the branch cut of the square root, $\phi_1$ must be piece-wise defined
%to take either the value of $\p_{\bc,+}$ or $\p_{\bc,-}$ to ensure that $|\phi_1| > 1.$
$\phi_j$ for $j=1,\,2,\,3,\,4$ 
must be piece-wise defined
to take either the plus or minus branch 
to ensure the correct sign of $|\phi_j| - 1.$


Since $\ac$ and $\bc$ are decoupled, the corresponding eigenvectors in equation
\eqref{eq:EigenvectorExpansion} 
are 
unit vectors,
$\rev_{1} = [0,1,0]^{T}$ and $\rev_{2} = [1,0,0]^{T}$ 
(i.e. $\qn{1} = \rn{2} = \sn{1} = \sn{2} = 0$). 
The remaining nonzero components of $\dMat$ are $\dComp_{12}$ and $\dComp_{21},$ which leaves
\begin{align}
\det(\dMat_{\text{1D}})= -\dComp_{12} \dComp_{21} = 0
\end{align}
% 
$\dComp_{12}$ is a standard extrapolation operator with repeated roots of $\p_2 = 1.$ 
Since an eigenvalue of magnitude one does not satisfy the boundary conditions, these roots
will be ignored. Upon substituting $\p_1$ as a function of $\amp$ into $\dComp_{21},$
a polynomial can be formed for $\amp$ with coefficients that depend on $\lambda_y$
and $M = \rho H / (\zp \dt).$ 
Maple was used to generate the polynomials for the TP, ATP, and AMP
schemes. The polynomial degrees for the TP, ATP, and AMP schemes are 
6, 4, and 6, respectively. Due to the large size, the coefficients of the 
polynomials are omitted from this paper.

All solutions to $\det(\dMat_{\text{1D}}) = 0$ are roots of the characteristic 
polynomials, but some spurious roots were introduced in deriving these polynomials.
These spurious roots can be easily identified by checking $\det(\dMat_{\text{1D}}).$

We evaluate the roots numerically for an array of equally spaced parameters in
the $\ly-\Mr$ plane. $\Mr$ is the grid mass ratio defined as
\begin{align}
\Mr = \frac{\rho H}{\rhos \dy}.
\end{align}
%
This dimensionless quantity represents the ratio of mass of a fluid column of height $H$
to the mass of a solid with the same cross section of height $\dy$. The grid mass ratio
is related to the acoustic mass ratio through $\Mr = \ly \Mra.$

The roots of the AMP polynomial were found at an array of $800$ points in 
$10^{-6} \le \lambda_y \le 1$ and $800$ points in $10^{-6} \le \Mr \le 10^{7}.$ 
No unstable roots, $|A| > 1,$ were found. The same process was repeated for the 
TP and ATP schemes for a range $10^{-6} \le \Mr \le 10.$ The stability region
was plotted in figure \ref{fig:acousticSolidStokesStabilityTP}. 
Since $\Mr \propto \dy^{-1},$ grid refinement will increase the mass ratio.
The TP scheme will become unstable for sufficiently large $\Mr,$ therefore the 
scheme is formally unconditionally unstable. On the other hand, the ATP scheme will 
eventually become stable for a sufficiently large $\Mr.$ This scheme is weakly
stable. Despite this, there is a significant
region in parameter space where only the AMP scheme is stable.
A 1D FSI numerical solver was used to verify the stability regions for the TP and ATP
schemes. In figure \ref{fig:acousticSolidStokesStabilityTPNumerical}, points in
$\Mr$-$\ly$ space were sampled to test for numerical instability. 
It was found that the numerical results confirm that the stability region holds.

{
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMPStability1D}
  \includegraphics[width=\figWidth]{fig/FSIStabilityRegion}
  \caption{Left: plot of the maximum amplification factor 
    for the AMP scheme. The stability region for the AMP scheme spans 
    $0 < \ly < 1,$ $0 < \Mr < \infty.$
    Right: Stability region for the 1D TP and ATP schemes. 
    For reference, 
    $\lambda_y = \cp \dt / \dy$ and $\Mr = \rho H / (\rhos \dy).$
    Grid refinement corresponds to increasing $\Mr,$ therefore the
    TP scheme will become unstable and the ATP scheme will become stable.
  }  \label{fig:acousticSolidStokesStabilityTP}
\end{center}
\end{figure}
}


{
% ---- from codes/analysis/numerical/b4_runTP1DStability ---- $
% ---- from codes/analysis/numerical/b5_runATP1DStability ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityTP1DNumerical}
  \includegraphics[width=\figWidth]{fig/FSIStabilityATP1DNumerical}
  \caption{Verification of the stability regions for the TP scheme (left)
    and the ATP scheme (right) using a 1D FSI numerical solver. Green markers 
    correspond to the numerical solution approximately close to the exact solution
    and red markers correspond to a numerical instability.
  }  \label{fig:acousticSolidStokesStabilityTPNumerical}
\end{center}
\end{figure}
}


% talk about numerical results

% Numerical Results:
%  - convergence for each scheme
%  - confirm stability region for each scheme
%
%   TP:
%     - heavy solid convergence study
%     - show stability region
%   ATP: 
%     - light solid convergence study
%     - show stability region
%   AMP:
%     - heavy/light solid convergence study
%     - really heavy/really light

\subsubsection{Continuation into 2D}

% derive eigenvectors with the idea that lx is small
% Now we approach the 2D model problem by considering $\lx$ to be a small 
% perturbation to the 1D problem. The main motivation for this is
% that the stability limit for the Cauchy problem requires $\lx < .3,$ (\todo{show this})
% and only $\lx^2$ appears in the discretization. 
%Additionally, the 2D added mass ratio
%$\Mr = (\rho \tanh(k_x H))/(k_x \rhos \dy)$ will only decrease as $k_x$ increases
The strategy for finding roots for $\lx \ne 0$ is to use the 1D roots as a starting point
for a numerical root solver that performs a continuation for $\lx > 0.$ The first step
is finding a suitable expression for the eigenvectors $\rev_1$ and $\rev_2$ so that
$\rev_1 / \| \rev_1 \| \rightarrow [0,1,0]^T, 
 \rev_2 / \| \rev_2 \| \rightarrow [1,0,0]^T$ as $\lx \rightarrow 0.$
The first and second components of equation \eqref{eq:evProblem} are used to define
$\rev_1$ and $\rev_2,$ respectively.
In 2D, the three dimensionless parameters needed are 
$\lx,\, \ly,$ and $\Mr_{\text{2D}} = \Mr \eta = \rho \tanh(k_x H) / (\rhos k_x \dy).$
Given these parameters, a nonlinear equation solver can be used to find 
solutions for the amplification factor, $A$, which solve $\det(\dMat)=0.$
Though there are multiple roots for a given set of parameters, 
we are only interested in the amplification factor with the maximum modulus.
Define $A_{\max}(\lx,\,\ly\,\Mr \eta)$ to be the maximum amplification factor 
given $\lx,\,\ly,$ and $\Mr \eta.$ 
%
In order to ensure stability of the pseudo-spectral approximation, 
all Fourier modes must be stable.
Both $\lx$ and $\eta$ are dependent on the transverse wavenumber, $k_x$. Therefore,
for a given $\ly$ and $\Mr,$ we search for the worst possible amplification factor,
$\mathcal{A}_{\Mr},$ for all possible $\lx$ and $\eta$. 
\begin{align}
\mathcal{A}_{\Mr}(\Mr,\ly) = 
\max_{\lx \in \mathcal{D}(\ly),\, \eta \in (0,1]} A_{\max}(\lx,\,\ly,\,\Mr \eta) 
\end{align}
%
where $\mathcal{D}(\ly)$ is the Cauchy stability bound for $\lx$.
Since the 1D amplification factor must be less than or equal to $\mathcal{A}_{\Mr},$
we are effectively seeing how the stability worsens when 
increasing the wave number, $\kx.$ 
Figure \ref{fig:lysmAMP2D} shows a surface plot of $\mathcal{A}_{\Mr}$
and the stability region, $|A| \le 1$ in the $\Mr$-$\ly$ plane.
There is a finite range of $\ly$ for which the AMP scheme is stable for all 
$\lx,\,\Mr,$ and $\eta$.

We can also search for a maximum amplification factor over all mass ratios,
$\mathcal{A}_{\text{CFL}},$ to see the CFL region for the AMP scheme in $\lx$-$\ly$ plane. 
Define
\begin{align}
\mathcal{A}_{\text{CFL}}(\lx,\ly) = 
\max_{0 < \Mr \eta < \infty} A_{\max}(\lx,\,\ly,\,\Mr \eta) .
\end{align}
%
This definition allows us to find a time step restriction regardless of the
mass ratio of the problem.
Figure \ref{fig:lylxAMP2D} shows a surface plot of $\mathcal{A}_{\text{CFL}}$
and the stability region, $|A| \le 1$ in the $\lx$-$\ly$ plane.

\textbf{Theorem}: \textit{By numerical evaluation of $\ACFL(\lx,\ly)$,
we have found that the AMP algorithm is weakly stable ($|\ACFL| \le 1$)
provided that $\lx^2 + \ly^2 \le 1$, i.e.}
\begin{align}
\dt \le \frac{1}{\cp} \left[\frac{1}{\dy^2} + k_x^2 \right]^{-1/2}.
\end{align}
%
\textit{This is a sufficient but not a necessary condition.}

%
% {
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
% \newcommand{\figWidth}{8cm}
% \begin{figure}[H]
% \begin{center}
%   \includegraphics[width=\figWidth]{fig/FSIStabilityRegion2D}
%   \caption{Stability region for the 1D and 2D TP and ATP schemes. 
%     $\bar{\Mr}$ is defined from 
%     equations \eqref{eq:MrbarTP}--\eqref{eq:MrbarATP} and is the worst
%     case mass ratio for all Fourier modes.
%     $\lambda_y = \bar{c} \dt / \dy$ is the CFL number.
%     The stability region for the AMP scheme spans 
%     $0 < \ly < 1,$ $0 < \bar{\Mr} < \infty.$ 
%     An increase in $\bar{\Mr}$ corresponds to grid refinement,
%     therefore TP scheme will become unstable and the ATP scheme will become stable.
%   }  \label{fig:acousticSolidStokesStabilityTP2D}
% \end{center}
% \end{figure}
% }
{
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_sm_surf}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_sm_cont}
  \caption{Left: surface plot of maximum $|A|$ over $\lx \in [0,1]$
    and $\eta \in (0,1]$ for the AMP scheme.
    Right: The green fill indicates the stability region $|A| \le 1.$
    For reference, 
    $\ly = \cp \dt / \dy,\, \Mr = \rho H / (\rhos \dy),\, \lx = \cp k_x \dt,\, 
    \eta = \tanh(k_x H)/ (k_x H).$
  } \label{fig:lysmAMP2D}
\end{center}
\end{figure}
}
{
\newcommand{\figWidth}{8cm}
\begin{figure}[h]
\begin{center}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_lx_surf}
  \includegraphics[width=\figWidth]{fig/AMP_continuation_02_15_N50_LargeRange_newer_ly_lx_cont}
  \caption{
    Left: surface plot of maximum $|A|$ over $\Mr \eta \in [10^{-6},10^{6}]$
    for the AMP scheme.
    The green fill indicates the stability region $|A| \le 1.$
    The dotted line is a plot of
    $\lx^2 + \ly^2 = 1$. 
    For reference, 
    $\ly = \cp \dt / \dy,\, \Mr = \rho H / (\rhos \dy),\, \lx = \cp k_x \dt,\, 
    \eta = \tanh(k_x H)/ (k_x H).$
  } \label{fig:lylxAMP2D}
\end{center}
\end{figure}
}

\subsection{Stability analysis of TP scheme with iterations}

\das{Should this be in this paper?}
\das{Put iterations scheme here. Also want to note that there are better iterative
schemes such as Aitken acceleration.}
The TP scheme is more commonly used with iterations to avoid the added mass instability
when refining grids. We perform an analysis of the TP iteration to understand
how to choose the under-relaxation factor and how many iterations to take.
Define the error between iterations to be the difference in interface velocities
\begin{align}
e^{(k)} = v_I^{(k+1)} - v_I^{(k)}.
\end{align}
%
By taking the difference between the current and previous iteration variable for
each step of the TP iteration, one can derive that
\begin{align}
e^{(k)} &= \left(1 - \omega \left(\frac{3}{2} \Mra + 1 \right)\right) e^{(k-1)}.
\end{align}
%
Define the amplification factor, $\ampI = 1 - \omega \left(\frac{3}{2} \Mra + 1 \right)$
where $e^{(k)} = A^{k} e^{(0)}.$
$\Mra$ is dependent on the wave number, $k_x.$ In order to optimize the convergence rate,
$\ampI$ needs to be optimized for all wave numbers.
\begin{align}
\Mra = \frac{\rho \tanh(k_x H)}{\zp \dt k_x} 
= \frac{\rho H}{\zp \dt} \frac{\tanh(k_x H)}{k_x H} 
= \Mra_0 \eta
\end{align}
%
where $\Mra_0 = (\rho H) / (\zp \dt)$ is the 1D acoustic mass ratio and 
$\eta = \tanh(k_x H) / (k_x H)$ is the 2D scale factor. To accommodate all
potential wave numbers in the $x$ direction, we consider $\eta \in [0,1].$
Let $\Mra = \Mra(\eta) = \Mra_0 \eta.$ The amplification factor for a given
$\omega$ and $\eta$ is
\begin{align}
\ampI(\eta,\omega) = a - \omega \left(\frac{3}{2} M_0 \eta + 1 \right).
\end{align}
%
We pose the following optimization problem to find the optimal 
under-relaxation parameter, $\omega^*$.
\begin{align}
\omega^* = \argmin_{\omega} \max_{0 \le \eta \le 1} |A(\eta,\omega)|
\end{align}
%
Since $\ampI$ is linear in $\eta$ and $\omega$ and $|\ampI| > 0,$ the maximum 
amplification factor for a 
given $\omega$ will occur on the boundary, $\eta = 0$ or $\eta = 1.$ 
\begin{align}
\ampI(\eta=0,\omega) = |1-\omega|, \quad 
\ampI(\eta=1,\omega) = \left| 1 - \omega \left(\frac{3}{2} M_0 + 1 \right) \right|
\end{align}
%
The choice of $\omega$ that minimizes both expressions corresponds to solving
$\ampI(\eta=0,\omega^*) = \ampI(\eta=1,\omega^*).$ It can be shown that
\begin{align}
\omega^* = \frac{4}{3 \Mra_0 + 4}, \quad \ampI^* = \frac{3 M_0}{3 M_0 + 4}.
\end{align}
%
This is a sensible result. The TP scheme suffers from added mass instability
for fine grids and light solids, which correspond to large acoustic mass ratios.
The under-relaxation parameter scales with $\Mra_0^{-1}$ to stabilize the added mass
effects. As a penalty, the amplification factor approaches $1$ for large $\Mra_0.$
To get a sense of computational cost for using TP iterations, we look at the number
of iterations needed for the relative error, $|e^{(k)}/e^{(0)}|,$ to converge to 
a desired tolerance, $\tau.$  It is easy to show that if $|A^*|^k < \tau,$ $k$ must 
satisfy
\begin{align}
k &> \frac{\log (\tau) }
{\log \left(\frac{3 M_0}{3 M_0 + 4} \right)} .
\end{align}
% 
We are interested in the asymptotic behavior for $\Mra_0 \gg 1.$ The denominator
of the above expression is asymptotically equivalent to
\begin{align}
\log \left(\frac{3 \Mra_0}{3 \Mra_0 + 4} \right) =
 \log \left(\frac{1}{1 + \frac{4}{3 \Mra_0} } \right)
\sim  \log \left(1 - \frac{4}{3 \Mra_0} + ... \right) 
\sim -\frac{4}{3 \Mra_0} + ...
\end{align}
%
Therefore 
\begin{align}
k > -\frac{3}{4} M_0 \log(\tau) = 
-\frac{3 }{4} \frac{\rho H }{ \bar{\rho} \bar{c} \Delta t} \log(\tau).
\end{align}
% 
The required number of iterations is proportional to $\dt^{-1}.$ 
For a viscous fluid simulation, the viscous terms can be treated as
implicitly or explicitly.
When an implicit solver is chosen, the time step will be proportional to
the grid spacing and the number of iterations will double when the grid is refined 
by a factor of $2$. 
When an explicit solver is chosen, the time step will be proportional to the 
square of the grid spacing and the number of iterations will quadruple when the grid
is refined by a factor of $2.$


% numerical results 



%%%%%%%%%%%%% old paper
% \subsection{Discretization}

% talk about fluid and solid discretization in x. 
% discrete fourier series on grid 
% % \wdh{We discretize the fluid and solid variables in the $x$~direction using a uniform
% % grid with spacing $\dx=L/(N_x+1)$. The grid points are given by $x_\ell=\ell\dx$,
% % $\ell=0,1,\ldots,N_x$.  The choice of discrete approximations to the
% % $x$~derivatives in the equations plays little role in the analysis.  Therefore, it is
% % convenient to use a pseudo-spectral approximation by expanding
% % each component $q$ of the solution $(\qv,\qsv)$ in a discrete Fourier series of
% % the form
% % % which gives a formally {\em exact} approximation,  $i\kx$, to an $x$-derivative.
% % % After discretizing in the $x$~direction we will expand the solution in a discrete Fourier series of the form
% % \begin{align}
% %    q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_\ell/L} \qHat_{k}(y,t), \qquad \ell=0,1,2,\ldots,N_x, \label{eq:discreteFourier}
% % \end{align}
% % where $q_\ell(y,t)\approx q(x_\ell,y,t)$ and $\qHat_{k}(y,t)$ are Fourier coefficients, 
% % and where $N_x$ is assumed to be even for convenience.
% % Transforming the governing equations to Fourier space leads to the following equations for the Fourier coefficients of the solution variables:
% % \begin{alignat}{3}
% % &   \rhos \partial_t \vs = i\kx \sigmas_{21} + \partial_y \sigmas_{22} , \quad&& y\in(0,\infty), \label{eq:vEqn} \\
% % &   \partial_t \sigmas_{22} = \rhos \cp^2 \partial_y\vs , \quad&&y\in(0,\infty), \label{eq:s22Eqn} \\
% % &   \partial_t \sigmas_{21} = i\kx \rhos \cp^2 \vs , \quad&&y\in(0,\infty) , \label{eq:s21Eqn} \\
% % & \rho \partial_t v_1 = i\kx      \sigma, \quad &&y\in(-H,0), \label{eq:v1HatEqn} \\
% % & \rho \partial_t v_2 = \partial_y\sigma, \quad && y\in(-H,0), \label{eq:v2HatEqn} \\
% % &  i\kx v_1 + \partial_y v_2 =0 ,                  \quad&&y\in(-H,0) , \label{eq:divHatEqn}
% % \end{alignat}
% % where $\kx = 2\pi k/L$ is a normalized wave number in the $x$~direction and the
% % equations hold for each $k=-N_x/2,-N_x/2+1,\ldots,N_x/2$. The hats on the
% % Fourier coefficients, along with the $k$ subscripts, have been dropped for
% % notational convenience.  Note that the horizontal component of the fluid
% % velocity, $v_1$, is decoupled from the other equations and boundary conditions, 
% % and can be determined once $v_2$ is known. Equations~\eqref{eq:v1HatEqn}--\eqref{eq:divHatEqn} are used to obtain
% % \[
% % \partial_y^2 \sigma - \kx^2 \sigma =0,      \qquad y\in(-H,0) ,
% % \]
% % which is a Laplace equation for pressure (in Fourier space).  The equations for the Fourier coefficients of the solid variables will be discretized using an upwind scheme.  In preparation for this, it is convenient to define the characteristic variables
% % \[
% % a=\sigmas_{22}-\rhos\cp\vs,\qquad b=\sigmas_{22}+\rhos\cp\vs,\qquad d=\sigmas_{21},
% % \]
% % which, from~\eqref{eq:vEqn}--\eqref{eq:s21Eqn}, satisfy
% % \begin{alignat}{3}
% % &   \partial_t a + \cp \partial_y a =  i\kx\cp\, d , \qquad&& y\in(0,\infty),  \label{eq:aHatEqnII}\\
% % &   \partial_t b - \cp \partial_y b = -i\kx\cp\, d , \qquad&& y\in(0,\infty),  \\
% % &   \partial_t d = \frac{i\kx\cp}{2}(b-a) , \qquad&& y\in(0,\infty).  \label{eq:dHatEqnII} 
% % \end{alignat}}
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% The solid variables are discretized in the $y$~direction using a uniform grid with
% spacing $\dy$.  The grid points for the solid domain are defined as $y_j=
% (j-\half)\dy$, $j=0,1,2,\ldots$. 
% Following the analysis in~\cite{BanksSjogreen2011,lrb2013}, the grid is staggered with respect to the
% interface at $y=0$ and has a ghost point at $j=0$; use of a non-staggered grid leads to similar results.
% %  This staggering simplifies the analysis but is not critical {\bf (I'm not convinced of this ?!?!)}.  
% Let  $\dt$ be the time step and let $t^n=n\dt$.  The
% equations~\eqref{eq:aHatEqnII}--\eqref{eq:dHatEqnII} are discretized using the
% first-order upwind scheme,
% \begin{alignat}{3}
% &   \frac{ a_j^{n+1}- a_j^n}{\dt} + \cp\frac{( a_j^n - a_{j-1}^n)}{\dy} =   i\kx\cp\, d_j^{n}, \label{eq:aEqnIII} \\
% &   \frac{ b_j^{n+1}- b_j^n}{\dt} - \cp\frac{( b_{j+1}^n - b_j^n)}{\dy} = - i\kx\cp\, d_j^{n}, \label{eq:bEqnIII} \\
% &   \frac{ d_j^{n+1}- d_j^n}{\dt} = \frac{i\kx\cp}{2}(b_j^{n+1} - a_j^{n+1}), \label{eq:dEqnIII}
% \end{alignat}
% where $a_j^{n}\approx a(y_j,t^n)$, $b_j^{n}\approx b(y_j,t^n)$ and
% $d_j^{n}\approx d(y_j,t^n)$. 
% Since we have used a non-dissipative pseudo-spectral approximation, rather than a two-dimensional upwind scheme, 
% the right-hand side terms in~\eqref{eq:dEqnIII} are taken at time $t^{n+1}$ in order to stabilize the approximation.
% A von Neumann stability analysis of equations~\eqref{eq:aEqnIII} and~\eqref{eq:bEqnIII} (for a
% periodic problem in $y$) shows that this time-stepping scheme is stable under
% reasonable conditions on the constants $\ly=\cp\dt/\dy$ and $\lx=\cp\kx\dt$.
% The fluid variables are kept continuous in $y$ in order to simplify the
% presentation; a discrete version can be introduced but this makes only
% insignificant changes to the fundamental results.  We are thus led to the
% following semi-discrete approximation for the solid and fluid equations,
% \begin{alignat}{3}
% &   a_j^{n+1} = a_j^n -\ly( a_j^n - a_{j-1}^n) - i \lx d_j^{n} , \quad&& j=1,2,3,\ldots\;, \label{eq:aEqn} \\
% &   b_j^{n+1} = b_j^n +\ly( b_{j+1}^n - b_j^n) + i \lx d_j^{n},  \quad&& j=0,1,2,\ldots\;, \label{eq:bEqn}  \\
% &   d_j^{n+1} = d_j^n +  \frac{i\lx}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=0,1,2,\ldots\;,  \\
% % 
% &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0), \\
% &  0=\partial_y^2 \sigma^{n+1}- \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), \label{eq:sigmaEqn}
% \end{alignat}
% where $v^n(y)=v(y,t^n)$ and $\sigma^n(y)=\sigma(y,t^n)$.  For reference, the discrete values for the (Fourier coefficients of the) velocity and components of stress in the solid are related to the characteristic variables by
% \[
% \vs_j^n=\frac{1}{2\zp}(b_j^n-a_j^n),\qquad\sigmas_{22,j}^n=\frac{1}{2}(b_j^n+a_j^n),\qquad \sigmas_{21,j}^n=d_j^n.
% \]
% The conditions at the top and bottom boundaries are 
% \begin{align}
% &   \vert a_j^{n}\vert^2 + \vert b_j^{n}\vert^2 + \vert d_j^{n}\vert^2 \rightarrow 0, 
%          \quad\text{as $j\rightarrow \infty$} ,  \label{eq:BCtop}\\
% &   \sigma^n(-H)=0. \label{eq:BCbottom}
% \end{align}
% Initial conditions are required to define $a_j^{0}$, $b_j^{0}$ and $d_j^{0}$ for $j=0,1,2,3,\ldots$, as well as $v^0(y)$ for  $y\in(-H,0)$, but these conditions are of no significance in the subsequent stability analysis.

% Approximations to the interface conditions are needed to complete the discrete
% formulation of the FSI model problem, and various choices are possible depending
% on the algorithm used.  
% For the AMP algorithm, the pressure Robin
% condition~\eqref{eq:AddedMassPressureBC} is imposed on the fluid; this is derived from the
% outgoing characteristic variables~\eqref{eq:AMPoutgoing}. In addition, the 
% incoming characteristic variable~\eqref{eq:AMPincoming} is used to specify a condition
% on the solid.  The latter condition uses an interface velocity defined
% in~\eqref{eq:ImpedenceWeightedVn} based on an impedance-weighted average.  
% First-order accurate approximations of these conditions are
% \begin{alignat}{3}
% &  \sigma^{n+1}(0) + \frac{\zp\dt}{\rho} \sigma_y^{n+1}(0) = \sigmas_{22,1}^{n+1} + \zp(\vs_1^{n+1} - v^{I,n})
%                                            = b_1^{n+1} -\zp v^{I,n}, && \label{eq:1dSigmaBC}\\
% &  a_0^{n+1} = \sigma^{I,n+1} - \zp v^{I,n+1}, &&\label{eq:1dSolidBC}
% \end{alignat}
% where $\sigma^{I,n}\equiv\sigma^n(0)$ and $v^{I,n}$ are the interface traction and velocity, respectively.  The latter is given by the impedance-weighted average
% \begin{alignat}{3}
% &   v^{I,n+1} = \frac{\zf}{\zf+\zp} v^{n+1}(0) + \frac{\zp}{\zf+\zp}\vs_1^{n+1} + \frac{1}{\zf+\zp}(\sigma_{22,1}^{n+1} - \sigma^{I,n+1} ) && \nonumber\\
% & \hphantom{v^{I,n+1}} = \gamma v^{n+1}(0) + \frac{1-\gamma}{\zp}( b_1^{n+1} - \sigma^{I,n+1} ), && \label{eq:1dVelocityBC}\end{alignat}
% where
% \[
% \gamma=\frac{\zf}{\zf+\zp},
% \]
% and where $\zf$ is a measure of the fluid impedance as introduced in Section~\ref{sec:partitionedAlgorithms}.

% The traditional partitioned (TP) algorithm uses the velocity from the solid as a boundary condition for the fluid and the traction from the fluid as a boundary condition for the solid.  First-order accurate approximations of these conditions are
% \begin{alignat}{3}
%  &   v^{n+1}(0)=\vs_1^{n+1}  
%         , &&   \label{eq:1dTradv} \\
%  &   \sigmas^{n+1}_{22,0} = \sigma^{n+1}(0). &&\label{eq:1dTradsigma}
% \end{alignat}
% It is also instructive to consider an anti-traditional algorithm in which
% the roles of the fluid and solid are reversed in the application of the
% partitioned interface conditions.  Approximations of these conditions are
% \begin{alignat}{3}
% &   \sigma^{n+1}(0) = \sigmas^{n+1}_{22,1}\,,  &&  \label{eq:1dAntiTradsigma} \\
% &   a_0^{n+1} = \sigma^{n+1}(0) - \zp v^{n+1}(0) .&& \label{eq:1dAntiTradv} 
% \end{alignat}
% The condition in~\eqref{eq:1dAntiTradv} is equivalent to setting the velocity of solid at the interface equal to the velocity in the fluid since the stresses have already been equilibrated in~\eqref{eq:1dAntiTradsigma}. 

% % 
% % 
% % % On the interface we assign the out-going characteristic variable by imposing~\eqref{eq:bEqn} at $j=0$.
% % The boundary conditions for the fluid are $\sigma^n(-H)=0$, while the solid solution should decay to zero 
% % as $j\rightarrow\infty$. 
% % The solution for $\sigma^n$ satisfying the boundary condition $\sigma^n(-H)=0$ can be written as
% % \begin{alignat}{3}
% % &  \sigma^{n}= \sigma^{I,n} \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \quad&& y\in(-H,0), 
% % \end{alignat}
% % where $\sigma^{I,n}=\sigma^n(0)$. 



% %- \vskip3\baselineskip
% %- 
% %- 
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- Let $\dt$ be the time step and let $t^n=n\dt$. 
% %- Introduce fully discrete approximations for the solid variables of the form $\qs_j^n \approx \qsHat(y_j,t^n)$ and
% %- semi-discrete approximations for the fluid variables of the form $q^n(y) \approx \qHat(y,t^n)$. 
% %- 
% %- This leads to the approximation
% %- \begin{alignat}{3}
% %- &   a_j^{n+1} = a_j^n -\lambda( a_j^n - a_{j-1}^n) - i \lambdax d_j^{n} , \quad&& j=1,2,3,\ldots \\
% %- &   b_j^{n+1} = b_j^n +\lambda( b_{j+1}^n - b_j^n) + i \lambdax d_j^{n},  \quad&& j=1,2,\ldots  \\
% %- &   d_j^{n+1} = d_j^n + i \frac{\lambdax}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=1,2,\ldots  \\
% %- % 
% %- &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0) \\
% %- &  \partial_y^2 \sigma^{n+1}= \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), 
% %- \end{alignat}
% %- where $\lambday=\frac{\cb\dt}{\dy}$ and $\lambdax=\cb\dt\kx$ and where $a_j^{n}$, $b_j^{n}$ and $d_j^n$
% %- are the characteristic variables in the solid given by 
% %- \begin{alignat}{3}
% %-    a_j^{n} = \sigmas_j^n -\zb \vs_j^n, \quad&& \vs_j^n &=\frac{1}{2\zb}(b_j^n-a_j^n), \\
% %-    b_j^{n} = \sigmas_j^n +\zb \vs_j^n, \quad&& \sigmas_j^n &=\frac{1}{2}(b_j^n+a_j^n), \\
% %-    d_j^n = \sigma^n_{21,j}
% %- \end{alignat}
% %- The boundary conditions for the fluid are $\sigma^n(-H)=0$, while for the solid the solution should remain bounded
% %- as $j\rightarrow\infty$. Initial conditions are needed for $a_j^{0}$, $b_j^{0}$, $d_j^{0}$, $j=0,1,2,3,\ldots$, 
% %- and $v^0(y)$, $y\in(-H,0)$.
% %- Approximations to the interface conditions are needed; various choices for these will be specified later. 
% %- 
% %- 
% %- 
% %- \vskip3\baselineskip
% %- 
% %- Introduce the fully discrete approximations $\vs_{ij}^n \approx \vs(x_i, y_j, t^n)$, 
% %- $\sigmas_{22,ij}^n \approx \sigmas^{22}(x_i, y_j, t^n)$, 
% %- $\sigmas_{21,ij}^n \approx \sigmas^{21}(x_i, y_j, t^n)$, 
% %- in the solid, 
% %- and the semi-discrete approximations $\vv_i^n(y)\approx \vv(x_i,y,t^n)$, $\sigma_i^n(y)\approx \sigma(x_i,y,t^n)$ in the fluid.
% %- We 
% %- expand the solution in a Fourier series in $x$,
% %- \begin{align}
% %-    \vs_{ij}^n = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat_{k,j}^n, \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}


% %- 
% %- 
% %- 
% %- We 
% %- expand the solution in a Fourier series in $x$. 
% %- We introduce the approximations $\vs_j(y,t) \approx \vs(x_j,y,t)$, $\sigma_{22,j}(y,t) \approx \sigmas_{22}(x_j,y,t)$, 
% %- $\sigma_{21,j}(y,t) \approx \sigmas_{21}(x_j,y,t)$, for the solid and 
% %- $\vv_j(y,t) \approx \vv(x_j,y,t)$, and $\sigma_{j}(y,t) \approx \sigma(x_j,y,t)$ for the fluid. 
% %- where 
% %- \begin{align}
% %-    \vs_j(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat(k,y,t), \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}
% %- We let $\kx = 2\pi k/L$ be the normalized wave number.
% %- 
% %- 
% %- 
% %- We discretize the solid in the $y$~direction with a grid spacing $\dy$.
% %- The grid for the solid is defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$. This grid is staggered
% %- with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- simplies the analysis but is not critical.
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- 
% %- % with grid spacing $\dy$ and use 
% %- % a first-order upwind scheme (in the $y$~direction) for the resulting solid equations. 
% %- % The grid for the solid, defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$, is staggered
% %- % with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- % simplies the analysis but is not critical.
% %- 
% %- In the solid we introduce grid functions $\vs_j^n\approx \vsHat(\kx,y_j,t^n)$, etc. 
% %- For the fluid we form approximations that are continuous in $y$ but discerete in time denoted by  
% %- $\sigma^n(y) \approx \sigmaHat(\kx,y,t^n)$,  and 
% %- $v^n(y) \approx \vHat_2(\kx,y,t^n)$. The horizontal component of the fluid velocity, $\vHat_1^n$, plays no role 
% %- in the analysis and can be determined from $v^n(y)$ using  $i\kx \vHat_1^n + \partial_y v^n(y)=0$, if needed.
% %- 
% %- 
% %- 


% % ------------------------------------------------------------------------------------------------
% \subsection{Stability analysis}

% \renewcommand{\aHat}{{\tilde a}}
% \renewcommand{\bHat}{{\tilde b}}
% \renewcommand{\dHat}{{\tilde d}}
% \renewcommand{\vHat}{{\tilde v}}
% \renewcommand{\sigmaHat}{{\tilde\sigma}}
% % \renewcommand{\aTilde}{{\bar a}}
% % \renewcommand{\bTilde}{{\bar b}}
% \renewcommand{\aTilde}{\alpha}
% \renewcommand{\bTilde}{\beta}

% To analyze the stability of the approximation
% in~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn}, we look for solutions of the form \[
% a_j^n=\amp^n\aHat_j, \qquad b_j^n=\amp^n\bHat_j, \qquad d_j^n=\amp^n\dHat_j,
% \qquad v^n(y)=\amp^n\vHat(y), \qquad \sigma^n(y)=\amp^n\sigmaHat(y),
% \] 
% where $\amp\in\Complex$ is the amplification factor,
% $(\aHat_j,\bHat_j,\dHat_j)$ are grid functions, and $(\vHat(y),\sigmaHat(y))$
% are functions for $y\in[-H,0]$. 
%  Substituting these forms
% into~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} results in the following system of
% equations
% \begin{alignat}{3}
% &  \amp \aHat_j = \aHat_j -\ly( \aHat_j - \aHat_{j-1}) - i \lx \dHat_j , \qquad&& j=1,2,3,\ldots\,, \label{eq:aHatEqn} \\
% &  \amp  \bHat_j = \bHat_j +\ly( \bHat_{j+1} - \bHat_j) + i \lx \dHat_j,  \qquad&& j=0,1,2,\ldots\,, \label{eq:bHatEqn}  \\
% &  \amp  \dHat_j = \dHat_j + \frac{i\lx}{2}\amp  ( \bHat_j - \aHat_j),    \qquad&& j=0,1,2,\ldots\,,  \label{eq:dHatEqn} \\
% % 
% &  \amp  \vHat(y) = \vHat(y) + \amp\dt\,\sigmaHat^I\,\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},  \qquad&& y\in[-H,0], \label{eq:vHatEqn} \\
% &  \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \qquad&& y\in[-H,0].\label{eq:sigmaHatEqn}
% \end{alignat}
% To obtain~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn},  the
% ODE in~\eqref{eq:sigmaEqn} was integrated using the boundary conditions $\sigmaHat(-H)=0$
% and $\sigmaHat(0)=\sigmaHat^I$, where the fluid stress at the interface, $\sigmaHat^I$, is as
% yet unspecified.  Note that the solution in the one-dimensional case,
% $\kk=0$, is a special case that can be found by taking the limit $\kk\rightarrow
% 0$ in~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn}. 
% Together with the interface
% conditions, equations~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} define
% a homogeneous set of difference equations. These equations have
% non-trivial solutions (i.e. eigenfunctions) only for particular values of $\amp$ (i.e. eigenvalues).
% The scheme is said to be weakly stable, or stable in the sense of
% Godunov-Ryabenkii, for given values of the parameters $\dt$, $\dy$, $\kx$, $H$, etc., 
% if there are no solutions (i.e.~eigenfunctions) to this
% eigenvalue problem with $\vert \amp\vert>1$. 
% The {\em region of stability} of the scheme is the region in parameter space where there are no roots with $\vert \amp\vert>1$. 
% In order to delineate the stability region 
% it is generally easier to look for regions where the scheme is {\em not} stable. Therefore, we 
% assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % we look for regions in the space of parameters where $\vert \amp\vert>1$  and the scheme is unstable.
% % We thus 
% % assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % If no such solutions exist for some given values of the parameters, then the scheme is (weakly) stable there. 
% % The stability domain is defined to be the region in parameter space where there are no roots with $\amp>1$.


% Equations~\eqref{eq:aHatEqn}--\eqref{eq:dHatEqn} are a system of
% constant-coefficient difference equations for the solid characteristic
% variables.  After solving for $\dHat_j$ from~\eqref{eq:dHatEqn} and substituting
% into~\eqref{eq:aHatEqn} and~\eqref{eq:bHatEqn}, $\aHat_j$ and
% $\bHat_j$ are found to satisfy the recursion
% \begin{equation}
%  \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = K \begin{bmatrix} \aHat_{j-1} \\ \bHat_{j-1} \end{bmatrix}, \qquad K =\begin{bmatrix}  ( 1 - \theta^2)/R & -\theta \\ \theta & R \end{bmatrix} ,
% \label{eq:recursion}
% \end{equation}
% where
% \begin{equation}
% R = r-\theta, \qquad r = \frac{\amp-1+\ly}{\ly}, \qquad \theta = -\frac{\amp\lx^2}{2\ly(\amp-1)} . 
% \label{eq:RandTheta}
% \end{equation}
% The eigenvalues, $\phi_-$ and $\phi_+$, of
% the $2\times2$ matrix $K$ in~\eqref{eq:recursion}
% %  \old{are the roots of a quadratic polynomial, and are given by} 
% are given by
% % \old{
% % We are interested in solutions for $\aHat_j$ and $\bHat_j$ that decay as
% % $j\rightarrow\infty$ so that the boundary condition in~\eqref{eq:BCtop} is
% % satisfied.  This leads us to consider the eigenvalues, $\phi_-$ and $\phi_+$, of
% % the $2\times2$ matrix $K$ in~\eqref{eq:recursion}, which are found by finding
% % the roots of a quadratic polynomial.  The result is
% % }
% \begin{equation}
% \phim = B - \sqrt{ B^2 - 1}, \qquad \phip=1/\phim, \qquad B = \frac{1}{2}\left(R + \frac{1 - \thetaj^2}{R}\right).
% \label{eq:phipm}
% \end{equation}
% Note that the product of the eigenvalues is one.  
% If both eigenvalues 
% % \old{were to have magnitude one} 
% had magnitude equal to one, then there would be no solution of the recursion
% in~\eqref{eq:recursion} satisfying the boundary condition~\eqref{eq:BCtop}.
% Therefore, for a valid solution, there is one eigenvalue (either $\phi_-$ or $\phi_+$),
% denoted by $\phis$ (for {\em small} $\phi$), that has magnitude strictly less
% than one, i.e.~$\vert\phis\vert<1$.  Let $\phib=1/\phis$ (for {\em big} $\phi$)
% be the other eigenvalue with $\vert\phib\vert>1$.  Note that when $\theta=0$,
% $0<\ly\le 1$, and $\vert\amp\vert>1$, then $\phis=\phim=1/r$ (but in general
% $\phis$ is not always equal to $\phim$).  Given that the eigenvalues are
% distinct, $K$ can be diagonalized as 
% \[
% K = S^{-1} \Phi S , \qquad
% \Phi =\begin{bmatrix}  \phis &  0 \\
%                            0 & \phib \end{bmatrix}, \qquad
% S =\begin{bmatrix}  R-\phis & \thetaj \\
%                     R-\phib & \theta \end{bmatrix}.
% \]
% By setting 
% \begin{align}
% &   \begin{bmatrix} \aTilde_j \\ \bTilde_j \end{bmatrix}
%    =  S \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = 
%    \begin{bmatrix} (R-\phis)\aHat_j + \theta \bHat_j \\
%                    (R-\phib)\aHat_j + \theta \bHat_j
%    \end{bmatrix}, \label{eq:abTildeEqn}
% \end{align}
% the general solution of the recursion in~\eqref{eq:recursion} is given by 
% \begin{equation}
% \begin{array}{l}
%    \aTilde_j = \phis^j \aTilde_0, \smallskip\\
%    \bTilde_j = \phib^j \bTilde_0.
% \end{array}
% \label{eq:abBarEqn}
% \end{equation}
% Since the solution must decay to zero as $j\rightarrow \infty$ and since $\vert\phib\vert>1$, it follows that $\bTilde_0=0$ and thus $\bTilde_j=0$ for all $j=0,1,2,\ldots$.  Since $\bTilde_j=0$, it follows from~\eqref{eq:abTildeEqn} that
% \begin{equation}
% \bHat_j = Q \aHat_j,\qquad \aTilde_j=(\phib-\phis)\aHat_j,\qquad Q = \frac{\phib-R}{\theta},
% \label{eq:Qdef}
% \end{equation}
% and thus from~\eqref{eq:abBarEqn}, 
% \[
% \aHat_j=\phi_s^j\aHat_0\,.
% \]
% Whence,
% % ------------------------------------------- PROP -------------------------------------------------
% \begin{proposition}
% Solutions to the system in~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} with $\vert\amp\vert>1$ satisfying the boundary conditions in~\eqref{eq:BCtop} and~\eqref{eq:BCbottom} are given by
% \[
% \begin{array}{c}
% \displaystyle{
% \aHat_j=\phi_s^j\aHat_0,\qquad \bHat_j=Q\aHat_j,\qquad \dHat_j=\frac{i\lx(Q-1)\amp}{2(\amp-1)}\aHat_j,\qquad j=0,1,2,\ldots\,,
% } \bigskip\\
% \displaystyle{
% \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},\qquad \vHat(y)=\sigmaHat^I\,\frac{\amp\dt}{\amp-1}\;\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},\qquad y\in[-H,0],
% }
% \end{array}
% \]
% % \old{where the two free constants, $\aHat_0$ and $\sigmaHat^I$, will be determined by two interface conditions.} 
% where $\aHat_0$ and $\sigmaHat^I$ are free constants.
% \end{proposition}

% The remaining constraints needed to complete the eigenvalue problem, which then determines the amplification factor $\amp$, are provided by two interface conditions.  Choices for these interface conditions are discussed in the subsections below.

% % \bigskip\noindent
% % \textcolor{green}{Note: I have chosen the wording above since the two interface conditions don't actually determine the two free constants, but rather they determine $\amp$ and a relationship between the constants.  I believe the constants would still be arbitrary to within a multiplicative constant.}

% % --------------------------------------------------------------------------------------------------------
% \subsection{AMP interface conditions} 
% Imposing the AMP interface conditions in~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC} with the formula for the interface velocity in~\eqref{eq:1dVelocityBC} gives
% % The AMP Robin boundary condition for $\sigma$ is~\eqref{eq:1dSigmaBC} which gives
% % follows from~\eqref{eq:AddedMassPressureBC}.
% % A first-order approximation is 
% % \begin{align}
% %   \sigma^{n+1} + \frac{\zb\dt}{\rho} \sigma_y^{n+1} &= \sigmas_{22,1}^{n+1} + \zb\vs_1^{n+1} - \zb v^{I,n}
% %                                            = b_1^{n+1} -\zb v^{I,n}, \qquad\text{for $y=0$}, \label{eq:1dSigmaBC}
% % \end{align}
% % where we have introduced the interface velocity $v^{I,n}$.
% % This gives,
% % \begin{align}
% % &  \sigma^{I,n+1} = \eta\Big( b_1^{n+1} - \zb v^{I,n}\Big), \\
% % & v^{I,n+1}  = \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \\
% % &  a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}, 
% % \end{align}
% \begin{align}
% &  \amp\sigmaHat^{I} = \eta\left( \amp\bHat_1 - \zp \vHat^{I}\right), \label{eq:AmpSigmaHat} \\
% &  \aHat_0 = \sigmaHat^{I} - \zp \vHat^{I} , \label{eq:AmpaHat} \\
% &  \vHat^{I}  = \gamma \vHat(0) + \frac{1-\gamma}{\zp}( \bHat_1 - \sigmaHat^{I} ), \label{eq:AmpvHatI}
% \end{align}
% where
% \begin{align*}
%  & \eta \equiv \frac{1}{1 + \frac{\zp\kk\dt}{\rho}\coth(\kk H)}  = \frac{1}{1 + \frac{\rhos\lx}{\rho}\coth(\kk H)}. 
% \end{align*}
% From~\eqref{eq:vHatEqn} and~\eqref{eq:AmpSigmaHat} we also have
% \begin{align}
%   (\amp-1) \vHat(0) = \frac{1-\eta}{\zb}(\amp \bHat_1 - \zb\vHat^I). \label{eq:AmpvHat} 
% \end{align}
% Using $\bHat_1=Q\phis \aHat_0$ to eliminate $\bHat_1$ in terms of $\aHat_0$ and using~\eqref{eq:AmpSigmaHat} to
% eliminate $\sigmaHat^{I}$, equations~\eqref{eq:AmpaHat}, \eqref{eq:AmpvHat} and~\eqref{eq:AmpvHatI} can be written
% in the form 
% %- The interface velocity follows from~\eqref{eq:1dVelocityBC}, giving 
% %- \begin{align}
% %- %    v^{I,n+1} &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( \zb\vs_1^{n+1} + \sigma_{22,1}^{n+1} - \sigma^{I,n+1} ), \\
% %- v^{I,n+1}   &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \label{eq:1dVelocityBCb}
% %- \end{align}
% %- where $\gamma=\zf/(\zf+\zb)$.
% %- For the final interface condition we set the incoming characteristic variable in the solid using the interface
% %- stress and velocity, 
% %- \begin{align}
% %-   a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}. \label{eq:1dSolidBCb}
% %- \end{align}
% % addedMass.mample : 
% % M := Matrix( [ [ A*(1-eta*Q*phim) , 0   , eta+A] , 
% %                [ (1-eta)*A*Q*phim , 1-A , -(1-eta) ], 
% %                [ -(1-g)*(1-eta)*Q*phim    , -g   , 1-(1-g)*eta/A ] ] );
% %
% %-The equations defining the AMP approximation can thus be written in the form
% \begin{align}
% \begin{bmatrix}
%    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
%    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
%   -(1-\gamma)(1-\eta)Q\phis  & -\gamma &  1-(1-\gamma)\eta \amp^{-1} 
% \end{bmatrix} 
% \begin{bmatrix} \aHat_0 \\ \zb \vHat(0) \\ \zb\vHat^I \end{bmatrix} =0 .  \label{eq:AMPmatrix}
% \end{align}
% The determinant of the matrix in~\eqref{eq:AMPmatrix} must be zero for non-trivial solutions to exist, and this leads to the following equation for $\amp$:
% \begin{align*}
% %    \tilde{f(\amp) :=& 
%    \big(\amp-(1-\gamma)\big) \left(\amp-\eta - \big( (2\eta-1)\amp -\eta \big)Q \phis\right) =0.
% \end{align*}
% % For $0\le \gamma\le 2$ the root $A=1-\gamma$ has magnitude less than or equal to one.
% Since $\amp-(1-\gamma)\ne0$ when $\vert\amp\vert>1$ and $0\le \gamma\le 2$, we have the following result.
% % --------------------------------------------------------------------------------------------------
% \begin{theorem} \label{th:amp1d}
% The AMP interface approximation to the
% scheme~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary
% conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, interface
% conditions~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC}, and interface
% velocity~\eqref{eq:1dVelocityBC} is weakly stable if and only if $0\le \gamma\le 2$ and there are no roots $\amp$ with $\vert \amp\vert>1$ to the equation
% \begin{align}
%    f(\amp) \equiv& \amp -\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis =0. \label{eq:fAMP}
% \end{align}
% \end{theorem}
% \noindent Note that $f(\amp)$ does not depend on $\gamma$, i.e.~the weighting in the definition of the interface velocity, and thus the stability of the scheme is independent of $\gamma$ provided $0\le \gamma\le 2$.  From a numerical conditioning point of view, however, we recommend the choice $\gamma=\zf/(\zf+\zp)$ as used in~\eqref{eq:1dVelocityBC}.


% %
% %- 
% %- \begin{align}
% %- &  A \sigma^{I} = \eta\Big( A \bHat_1 - \zb v^{I}\Big), \label{eq:AddedMassSigmaI} \\
% %- % &  \aHat_0 = \sigmasHat_0 - \zb \vsHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- &  \aHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- & (A-1)\vHat(0)= \frac{1-\eta}{\eta\zb} A \sigma^{I}, \\
% %- & v^{I} = \gamma \vHat(0) + (1-\gamma)\frac{1}{\zb}( \bHat_1 - \sigma^{I} )
% %- % &  b^{I,n+1}= b_1^{n+1},  ~~\text{(first order approximations)}, 
% %- \end{align}
% %- Using the expressions for $b_1^n$, etc. 
% %- lead to the conditions
% %- \begin{align}
% %- &  A(1-\eta Q\phis)\aHat_0 + (\eta+A) (\zb\vHat^I) =0 ,   \\
% %- & (A-1)(\zb\vHat(0)) -(1-\eta) A Q \phis \aHat_0 + (1-\eta) (\zb \vHat^I) = 0, \\
% %- & (1 - (1-\gamma)\eta A^{-1}) (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(1-\eta) Q \phis\aHat_0 = 0. 
% %- % & (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(Q-1)\half\phis \aHat_0=0. 
% %- \end{align}
% %- This is an eigenvalue problem for $\amp$. 
% %- Taking the determinant of the associated matrix leads to 
% %- \begin{align}
% %- & f(\amp) \equiv
% %- \det
% %- \begin{bmatrix}
% %-    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
% %-    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
% %-    \half(1-\gamma)(Q-1) \phis  & \gamma & -1 
% %- \end{bmatrix} =0,\\
% %- & f(\amp)=  \amp(1-\eta Q\phis) \Big( 1-\amp +\gamma(1-\eta)\Big) + 
% %-          (\amp+\eta)\phis\Big(  \gamma(1-\eta)\amp Q - \half(1-\amp)(1-\gamma)(Q-1)   \Big) .
% %- \end{align}
% %-The scheme is unstable if there are solutions to $f(\amp)=0$ with $\vert\amp\vert>1$. 
% %-The scheme is said to be (weakly stable) at particular values of $\lambdax,\lambday,\gamma$
% %-if there are no roots with $\vert\amp\vert>1$. Given a choice for $\gamma$ we can plot the
% %-region of stability in the $(\lambdax,\lambday)$ plane. 


% \paragraph{Reduction to a polynomial equation for $\amp$} To examine the stability of the AMP algorithm we must consider all solutions of $f(\amp)=0$.  The function $f(\amp)$ in~\eqref{eq:fAMP} involves square roots of $\amp$ through the eigenvalues, $\phis$ and $\phib$, of the matrix $K$ in~\eqref{eq:recursion} and the definition of $Q$ in~\eqref{eq:Qdef}.  
% To ensure that all possible solutions are found, 
% a polynomial $P(\amp)$ can be derived whose roots include
% all the roots of $f(\amp)$.  To this end, 
% note that from the definition for $Q$ and $\phis\phib=1$ it follows that 
% \begin{align*}
%   Q\phis = \frac{1-R\phis}{\theta}.
% \end{align*}
% Thus $f$ is a linear function of $\phis$ since $f$ only depends on the product $Q\phis$. 
% Note 
% also that $Q\phis$ is a rational function of $\amp$ according the definitions of $R$ and $\theta$ in~\eqref{eq:RandTheta}.  
% Thus, $f(\amp)=0$ can be written in the form
% \begin{align*}
%     \phis = F(\amp) ,
% \end{align*}
% where $F$ is a rational function of $\amp$. 
% Since $\phis$ is equal to one of the two eigenvalues, $\phi_\pm$, defined in~\eqref{eq:phipm}, it follows that 
% \begin{equation}
%   \pm \sqrt{ B^2 - 1} = F(\amp)-B,
% \label{eq:Fratio}
% \end{equation}
% where the sign in front of the square root is chosen to be consistent with $\vert\phis\vert<1$.
% % \old{where the sign in front of the square root is chosen based on the assignment of $\phis$ so that $\vert\phis\vert<1$.}
% Upon squaring both sides of~\eqref{eq:Fratio}, which introduces new roots, one obtains
% %  
% %  Since $\phis$ also satisfies a quadradic equation
% %  with coefficients that are polynomials of $A$, 
% %  \begin{align}
% %   (\amp-1)^2 R \phis^2 - (\amp-1)^2 R B \phis + (\amp-1)^2 R=0,
% %  \end{align}
% % we can eliminate $\phis$ to derive a higher degree polynomial satisfied by $A$,
% \begin{equation}
%    P(\amp)=0,
% \label{eq:PAMP}
% \end{equation}
% where $P(\amp)$ is a polynomial (as described below).  We have thus shown the following:
% \begin{proposition}
%   Any solution of $f(\amp)=0$ is also a root of the polynomial $P(\amp)$. 
% \end{proposition}
% All of the roots of $P(\amp)$ can be found numerically using well-developed
% algorithms (e.g.~solving the eigenvalue problem for the companion matrix).  
% In
% deriving $P(\amp)$, however, new roots have been introduced. Therefore, each
% root $\amp^*$ of $P(\amp)$ must be checked to ensure that it is also solution of
% $f(\amp)=0$.
% % To do this we set $\phis=\phi_-(\amp_0)$ if $\vert\phi_-(\amp_0)\vert<1 $ otherwise we set $\phis=\phi_+(\amp_0)$,
% % and then check that $f(\amp_0)=0$. 
% \begin{proposition}
%   A root, $\amp^*$, of $P(\amp)$ is also a root of $f(\amp)$, if $\phis$ in the definition of $f$ satisfies
% \begin{equation*}
%     \phis = \begin{cases}
%                 \phi_-(\amp^*) & \text{if $\vert\phi_-(\amp^*)\vert<1 $}, \\
%                 \phi_+(\amp^*) & \text{otherwise} ,
%             \end{cases}
% \end{equation*}
% and if $f(\amp^*)=0$.
% \end{proposition}
% % \begin{align}
% %    P(\amp)=0, \quad f(\amp)=0, \quad \vert\phis(\amp)\vert<1. 
% % \end{align}
% % {\bf Scheme 1:} Taking $\gamma=1$ (interface velocity from the fluid), gives (removing a factor of $2\amp$)
% % ff := phim Q A - eta - 2 eta Q phim A + eta Q phim + A
% % 
% \newcommand{\Pamp}{P_{\rm AMP}}
% The polynomial in~\eqref{eq:PAMP} is (after removing uninteresting factors of $\amp-1$) a polynomial of degree 5 given by 
% \[
% \Pamp(\amp)=\alpha_5\amp^5+\alpha_4\amp^4+\alpha_3\amp^3+\alpha_2\amp^2+\alpha_1\amp+\alpha_0,
% \]
% where the coefficients in the polynomial are
% \[
% \begin{array}{l}
% \alpha_0=-\eta^2+2 \eta^2 \ly, \smallskip\\
% \alpha_1=-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2, \smallskip\\
% \alpha_2=10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly, \smallskip\\
% \alpha_3=-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2, \smallskip\\
% \alpha_4=3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2, \smallskip\\
% \alpha_5=-1+2 \eta.
% \end{array}
% \]
% %\begin{align*}
% %%  f_1(\amp) :=&  A-\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis, \\
% % \Pamp(\amp) =&  (-1+2 \eta) A^5+(3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2) A^4+\\
% %&    (-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2) A^3+\\
% %&    (10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly) A^2+(-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2) A\\
% %&    -\eta^2+2 \eta^2 \ly .
% %\end{align*}
% It turns out that $\Pamp(\amp)$ is the same polynomial generated by the Maple symbolic algebra program when asked to solve $f(\amp)=0$.

% To determine if there are any roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$, we
% evaluate the roots numerically for an array of parameter values in the region
% $0<\lx<1.2$, $0<\ly<1.2$ and $0\le \eta \le 1$ with $N_\amp$ equally spaced
% points in each parameter direction.  The stability region of the scheme is the
% region in the space of $(\lx,\ly,\eta)$ where the magnitude of the largest
% valid root satisfies $\vert\amp\vert\le 1$.  This region is computed on a grid with
% $N_\amp=800$ points for each parameter.  In
% Figure~\ref{fig:acousticSolidStokestability}, we plot the curve in the
% $(\lx,\ly)$ plane for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  (The
% curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is also plotted for
% reference.)  Observe that the region of stability contains the region
% $0\le\eta\le1$ and $\lx^2 + \ly^2 \le \kappa^2$
% (for $\lx\ge0$ and $\ly\ge 0$) where the maximum value for $\kappa$ appears to be $\kappa=1$. 
% Further evidence for $\kappa=1$ being the upper bound is provided by the restriction of the analysis to one dimension given below.
% % \old{, where $\kappa$ is a positive constant strictly less than 1.  }
% The curve $\lx^2 + \ly^2 = (.99)^2$
% is shown in the figure as an example.  Since $\lx=\cp\kx\dt$ and $\ly=\cp\dt/\dy$,
% the condition $\lx^2+\ly^2\le 1$ implies the following result.

% % To determine if there are any roots of $\Pamp(\amp)=0$ with $\vert\amp\vert>1$ we evaluate the roots numerically for 
% % values of $\lambda$, $\lambdax$ and $\eta$ in the ranges $0<\lambda<1$, $0<\lambdax<1$, and $0\le \eta \le 1$.
% % We choose $M$ equally spaced values of each of $\lambda$, $\lambdax$ and $\eta$ over their ranges, resulting
% % in finding the roots for $M^3$ points. Using Maple we computed roots with $M=50$ and $M=100$ and using $20$ digits of precision.
% \begin{theorem}
% By numerical evaluation of the stability polynomial, $\Pamp(\amp)$,
% we have found that the AMP algorithm is weakly stable (i.e.~there are no valid roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$) 
% provided $\lx^2+\ly^2\le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{1}{\cp}\left[ \frac{1}{\dy^2} + \kx^2 \right]^{-1/2}. 
%  \end{align*}
% % where $0\le\kappa<1$. 
% This is a sufficient but not a necessary condition. 
% \end{theorem}
% Note that the time step $\dt$ satisfies a typical CFL constraint arising from the fastest wave speed in the solid.
% In the incompressible limit when $\cp \rightarrow \infty$, the maximum stable $\dt$ would go to zero,
% as it would for the solid in isolation. For incompressible solids, alternative formulations should be considered.
% Developing AMP algorithms for incompressible solids is a subject for future work. 

% % \noindent{\bf Note 1:} There are generally four valid roots to $\Pamp(\amp)=0$.
% % Figure~\ref{fig:acousticSolidStokestability} shows a plot of the computed stability region.

% {
% % ---- from codes/cauchy.m  (and cauchy.maple) ----
% \newcommand{\figWidth}{8cm}
% \begin{figure}
% \begin{center}
% %   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP_num50}
%   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP}
%   \caption{Stability region for the two-dimensional model problem using the AMP algorithm.  The curve marked 1 is the curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  The curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is shown for reference.  The dashed curve shows the curve $\lx^2+\ly^2=(.99)^2$.}
%   \label{fig:acousticSolidStokestability}
% \end{center}
% \end{figure}
% }


% % \noindent{\bf Note 2:} The scheme is found to be unstable for $\lambda>1$. Note, however, that the stability bound
% % derived in Section~\ref{} for a periodic strip in $y$ is somewhat more restrictive than the bound found here
% % for the seimi-infinite strip. For example, the periodic strip is unstable for $(\lambda,\lambdax)=(.9,9.)$.

% % {\bf TO-DO: Check the $\eta=0$ limit -- decoupled solid -- we should get von-Neumann stability bound.}

% % --------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% The stability of the one-dimensional version of the AMP algorithm 
% % \old{(described previously in Section~{\bf ?????})}
% may be examined by considering the special case of the two-dimensional algorithm with $\lx=0$ and $Q=0$.  In this case there are two solutions of $f(\amp)=0$ given by
% \begin{align*}
%    \amp = 1-2\ly \qquad\text{or}\qquad \amp =\eta. % \label{eq:fAMP1D}
% \end{align*}
% We are interested in whether there are solutions with $\vert\amp\vert>1$.  Since $0\le \eta\le 1$ we have the result.
% \begin{theorem}
% The one-dimensional AMP algorithm is weakly stable provided  $0\le\gamma\le 2$ and $0 \le \ly \le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{\dy}{\cp}. 
%  \end{align*}
% \end{theorem}

% % \noindent{\bf Note 2:} Even though there are no roots $\vert\amp\vert>1$ to $\Pamp$ for even larger values of $\lambda$ and $\lambdax$,
% %   the orginial scheme should respect the time step restriction from the solid scheme 
% % {\bf But why? Does some assumption go bad? e.g. $\vert\phis\vert<1$?}


% For comparison, we now discuss briefly the corresponding stability results for the scheme given by~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, and with interface conditions given by either the 
% traditional (TP) algorithm or the anti-traditional algorithm.



% % ==========================================================================================================
% \subsection{TP interface conditions} \label{sec:TPanalysis}
% % \newcommand{\Mr}{\Mc}% mass ratio

% The interface conditions for the TP algorithm are given by~\eqref{eq:1dTradv} and~\eqref{eq:1dTradsigma}.  
% Following the previous analysis, $\amp$ is found to satisfy 
% \begin{align}
% &   f_{{\rm TP}}(\amp) \equiv \amp(Q+1) - \frac{\eta-1}{\eta} (\amp-1)(Q-1)\phis =0 . \label{eq:traditionalSchemeF}
% % &   \mr \equiv \frac{\zb\dt\kx}{\rho\tanh(\kx H)} = \frac{\eta-1}{\eta} ...
% \end{align}

% % {\bf TO-DO} The stability region for this scheme is computed numerically and shown in Fig.~\ref{??}.
% % We could plot the stability regions for fixed values of $\eta$ and show that as $\eta\rightarrow 1$ the
% % stability region shrinks to nothing. This shows that as $\dt\rightarrow 0$ ($\eta\rightarrow 1$) the
% % scheme is unstable. 


% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 

% In one dimension, the condition in~\eqref{eq:traditionalSchemeF} reduces to the polynomial equation
% \begin{align*}
% P_{{\rm TP}}(\amp) = \amp^2 + (\Mr + \ly-1) \amp - \Mr = 0, \quad\text{where}~~
%   \Mr = \frac{\rho H}{\rhos \dy}.
% \end{align*}
% (Here, all of the roots of this quadratic are valid since no spurious roots were introduced in deriving the equation.)  The product of the roots is $-\Mr$ and thus a necessary condition for stability is that $\vert \Mr\vert\le 1$.
% Thus the mass of the solid in a thin strip one grid cell wide, $\rhos\dy L$, 
% must be larger than the mass of the entire fluid domain $\rho H L$. 
% Using the theory of von Neumann polynomials~\cite{Miller1971,Strikwerda89} one can show the following necessary and
% sufficient condition.  
% % {\bf (It is a little unclear to me how $\Delta y$ appears.) WDH: Multiply the expression below with $\cp/\dy$ and $\lambda$ and $\Mr$ appear. }
% % ---------------------------------- THEOREM -------------------------------------------------
% \begin{theorem} \label{lemma:traditional}
% The one-dimensional TP algorithm is weakly stable if and only if 
% \begin{align*}
% %      \Mr = \frac{\rho H}{\rhos \dy} <1, \\
%      \dt \le \frac{2}{\cp}\Big( \dy - \frac{\rho H}{\rhos} \Big). 
% %      \lambda < 2(1-\Mr). 
% \end{align*}
% \end{theorem}
% This is a curious result.  For a given {\em large} value of $\dy$ the one-dimensional scheme may be stable, but it will eventually become unstable as the mesh is refined and $\dy$ becomes less than $(\rho H)/\rhos$.  The one-dimensional TP algorithm is thus formally {\em unconditionally unstable}.  
% The numerical results in Section~\ref{sec:travelingWaveResults} show that this behaviour also holds for 
% the second-order accurate discretization of the two-dimensional model problem MP-VE.
% % This behaviour of the traditional scheme is also found to hold in the two-dimensional
% %  since as the mesh is refined eventually $\dy$ will be less than $\frac{\rho H}{\rhos}$. 


% % --------------------------------------------------------------------------------------------------------
% \subsection{Anti-traditional interface conditions} \label{sec:ATPanalysis}

% The interface conditions for the anti-traditional algorithm are given by~\eqref{eq:1dAntiTradsigma} and~\eqref{eq:1dAntiTradv}.  The analysis for this choice leads to the constraint
% %These can be written as 
% %\begin{align*}
% %&  \sigmaHat^I = \sigmasHat_{22,1}= \half(Q+1)\phis\aHat_0, \\
% %&  \aHat_0 = \sigmaHat^I -\zb\Big( \frac{\kk\dt}{\rho}\coth(\kk H)\frac{\amp}{\amp-1} \Big)\sigmaHat^I, 
% %\end{align*}
% % The anti-traditional scheme takes the interface velocity from the fluid and the interface
% % stress from the solid,
% % \begin{align}
% % &   \vHat^I = \vHat(0) = \frac{1-\eta}{\eta}\frac{1}{\zb} \frac{\amp}{\amp-1} \sigmaHat^I, \\
% % &   \sigmaHat^I = \sigmasHat_1 = \half(Q+1) \aHat_0, \\
% % &   \aHat_0 = \sigmaHat^I - \zb \vHat^I = (1- \frac{1-\eta}{\eta}\frac{\amp}{\amp-1}) \half(Q+1) \aHat_0.
% % \end{align}
% % ese interface conditions lead to the eigenvalue equation for $\amp$ of 
% %which leads to the eigenvalue equation for $\amp$ of 
% \begin{align}
% &   f_{{\rm AT}}(\amp) = 1- \amp + \half\left( \frac{2\eta-1}{\eta} \amp -1 \right) (Q+1)\phis=0 .  \label{eq:antiTraditional2d}
% \end{align}

% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% In one dimension, \eqref{eq:antiTraditional2d} reduces to the polynomial constraint
% \begin{align*}
% %      \amp^2 + ( \frac{\lambda}{2\eta} -2)\amp + 1-\frac{\lambda}{2} = 0.  \\
%      P_{{\rm AT}}(\amp) = \amp^2 + \left( \frac{\ly}{2}\left(1+\frac{\ly}{\Mr}\right) -2\right)\amp + 1-\frac{\ly}{2} = 0.  
% %     \amp^2 + (  \frac{\lambda}{2} + \frac{\lambda^2}{2\Mr} -2)\amp + 1-\frac{\lambda}{2} = 0. 
% \end{align*}
% % The anti-traditional scheme is weakly stable in one-dimension if and only if the following conditions
% %  are satisfied (**CHECK ME**)
% %  \begin{align}
% %  &    \lambda < 4, \\
% %  &    \frac{\lambda^2}{2\Mr} < 4-\lambda. 
% %  \end{align}
% %  where $\Mr = \frac{\rho H}{\rhos \dy}$. {\bf TO-DO:} $\Mr$ depends on $\dy$ so we really need to find the condition on $\dt$ in terms of $\dy$.
% An analysis of the roots of $P_{{\rm AT}}(\amp)$ leads us to the following result:
% \begin{theorem}
%   The one-dimensional anti-traditional algorithm is weakly stable if and only if $\ly\le 4$ and 
% % \begin{align}
% % %    \lambda \le \sqrt{ 8\Mr + \Mr^2  } -       \Mr     =       \Mr     \Big( \sqrt{ 1+\frac{8 }{\Mr}} -1 \Big). \\
% %     \half G \dt^2 + \dt < \frac{4\dy}{\cb}, \qquad G=\frac{\rhos\cb}{\rho H}
% % \end{align}
% % or 
% \begin{align}
% %    \dt  < \frac{ \sqrt{1+\frac{8\rhos}{\rho H} \dy} -1 }{G}, \qquad G=\frac{\rhos\cb}{\rho H} . \\
%    \dt  \le \frac{\dy}{\cp}\left( \sqrt{\Mr^2+8\Mr}-\Mr \right).   \label{eq:ATStability}
% \end{align}
% \end{theorem}

% We observe that the one-dimensional anti-traditional scheme is (weakly) stable for any value of the added-mass ratio $\Mr=(\rho H)/(\rhos \dy)$ provided that $\dt$ is taken sufficiently small. 
% The anti-traditional scheme is thus a stable alternative to the AMP scheme. However, in the {\em heavy solid} regime 
% when $\Mr$ is small, the anti-traditional requires a smaller $\dt$ than the AMP scheme, scaling
% like $\sqrt{8\Mr}$ for $\Mr\ll 1$,  as can be seen from~\eqref{eq:ATStability}.



==> texFiles/analysis-orig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TODO:
% - fix taylor series derivation of LW. can't do time derivative of discrete var

\section{Analysis of a two-dimensional acoustic solid and an inviscid incompressible fluid} \label{sec:analysis}

% todo
%
% replace \lambda_y with \ly etc.
%

\input texFiles/rectangularModelProblemCartoon

% \wdh{\bf This is from fib:
% In this section, we perform a stability analysis of the AMP algorithm applied to
% the two-dimensional FSI model problem MP-IA.  In this problem, the fluid is
% taken as inviscid and the solid is treated as an acoustic solid that only
% supports motion in the vertical direction. The governing equations for the model
% are given by~\eqref{eq:MP-IA}.
% % We are interested in the stability of different frequencies in the $x$ direction and thus consider a periodic problem in $x$. 
% We consider a semi-infinite solid domain ($\Hs=\infty$) and look for solutions in the solid that have finite $L_2$-norm (which implies the solutions decay to zero as $y\rightarrow\infty$).  The bottom boundary condition on the fluid at $y=-H$ is chosen as $\sigma=0$ (i.e. $p=0$).
% }

In this section, the stability of the second order accurate
AMP, TP, and ATP algorithms are explored for a simplified two-dimensional 
model problem. This extends the stability results of first order 
accurate schemes in \cite{fib2014}.
In this analysis, the TP scheme is considered 
without under-relaxed sub-iterations. 
To supplement this, an analysis of the TP scheme with sub-iterations is performed.
In the model problem, we assume the fluid is inviscid and the solid 
is acoustic with motion constrained to vertical direction. 
We are interested in the stability of different frequencies 
in the $x$ direction and thus consider a periodic problem in $x$. 
The solid domain is semi-infinite ($\Hs \rightarrow \infty)$ and we require solutions
to decay to zero as $y \rightarrow -\infty.$ The fluid pressure is given to be 
$p=0$ at the top boundary. The interface conditions enforce matching of the 
velocity and traction at $y=0.$
The governing equations and boundary conditions are given by
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t \vfy + \partial_y p = 0, & \xv\in\OmegaF \\
(\partial_x^2 + \partial_y^2) p =0, & \xv\in\OmegaF \\
p = 0, & x\in(0,L), \quad y=H
\end{cases} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsy = \partial_x \ssx + \partial_y \ssy, & \xv\in\OmegaS \\
\partial_t \ssx = \rhos\cp^2 \partial_x \vsy, & \xv\in\OmegaS \\
\partial_t \ssy = \rhos\cp^2 \partial_y \vsy, & \xv\in\OmegaS \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 \rightarrow 0, & y\rightarrow - \infty
\end{cases} \\
\text{Interface: } &\begin{cases}
\vfy = \vsy, & x\in(0,L), \quad y = 0 \\
p = -\ssy, & x\in(0,L), \quad y = 0.
\end{cases}
\end{align}

% governing equations
% ------------------------------------------------------------------------------------------------
\subsection{Discretization}

The fluid and the solid are discretized in the $x$ direction by a uniform grid defined by
grid spacing $\dx = L/N_x$ and grid points $x_l = l \Delta x$ for 
$\ell = 0, 1,\ldots N_x.$ 
Since the problem is periodic in the $x$ direction, each
variable can be represented as a discrete Fourier series, e.g.
\begin{align}
q_l(y,t) = \sum_{k=-N_x/2}^{N_x/2-1}  e^{2 \pi i k x_l/ L} \hat{q}_k (y,t), 
\qquad \ell=0,1,2,\ldots,N_x. \label{eq:discreteFourier}
\end{align}
%
Here, $q_l(y,t) \approx q(x_l,y,t)$ and $\hat{q}_k$ are Fourier coefficients.
For convenience, $N_x$ is assumed to be an even integer. Let
$k_x = 2 \pi k /L$ be the normalized wave number for each 
$k = -N_x/2,-N_x/2+1, \ldots, N_x/2-1.$ The governing equations are now transformed
to obtain equations for the Fourier coefficients. The equations for the fluid become
\begin{alignat}{2}
\rho \partial_t \vfyh + \partial_y \ph &= 0, \quad && y\in(0,H) \\
\partial_y^2 \ph - k_x^2 \ph &=0, \quad && y\in(0,H).
\end{alignat}
%
% todo, we dropped the subscript k for the fourier coefficients. explain this?
The transformed equations for the solid are
\begin{alignat}{2}
\rhos \partial_t \vsyh &= i k_x \ssxh + \partial_y \ssyh, \quad && y\in(-\infty,0) ,
\label{eq:vsyhEqn} \\
\partial_t \ssxh &= i k_x \rhos\cp^2 \vsyh, && y\in(-\infty,0), 
\label{eq:ssxhEqn} \\
\partial_t \ssyh &= \rhos\cp^2 \partial_y \vsyh, && y\in(-\infty,0)
\label{eq:ssyhEqn}.
\end{alignat}
%
It is convenient to consider the solid equations in characteristic form. 
Equations \eqref{eq:vsyhEqn}--\eqref{eq:ssyhEqn} are diagonalized to derive the
following characteristic variables
\begin{align}
\ac = \ssyh - \rhos\cp\vsyh, \quad
\bc = \ssyh + \rhos\cp\vsyh, \quad
\dc = \ssxh,
\end{align}
%
which satisfy
\begin{alignat}{2}
\partial_t \ac + \cp \partial_y \ac &= i k_x \cp \dc, \quad && y\in(-\infty,0), 
\label{eq:advSrcA} \\
\partial_t \bc - \cp \partial_y \bc &= -i k_x \cp \dc, \quad && y\in(-\infty,0),
\label{eq:advSrcB} \\
\partial_t \dc &= \frac{i k_x \cp}{2} (\bc - \ac), \quad && y\in(-\infty,0). 
\label{eq:SrcD}
\end{alignat}
%
This is a system of advection equations with a source. $\ac$ corresponds to the
$\cp^+$ characteristic and $\bc$ corresponds to the $\cp^-$ characteristic.

The solid characteristic variables are discretized in the $y$ direction using a
uniform collocated grid with grid spacing $\dy$ and grid points
$y_j = j\dy,$ for $j = 1, 0, -1, -2 \ldots$. 
Although staggered grids are used for the analysis in 
\cite{BanksSjogreen2011,lrb2013,fib2014}, the analysis for second order interface
conditions is significantly simpler on a collocated grid. 
Let $\Delta t$ be the time step and let $t^n = n \Delta t.$
The solid equations are solved with a dissipative scheme to in order to exploit 
some useful properties in the analysis.
A second order centered scheme was chosen to minimize the stencil to 
three grid points (a second order upwind scheme requires a five point stencil).
The schemes for equations \eqref{eq:advSrcA}--\eqref{eq:advSrcB}
are derived by taking a Taylor series in time and replacing time derivatives
with spacial derivatives. 
Define the grid functions
$\ac^n_j \approx \ac(y_j, t^n), \bc^n_j \approx \bc(y_j, t^n),$ and
$\dc^n_j \approx \dc(y_j,t^n),$
then the Taylor series for $\ac$ is given by
\begin{align}
\ac(y_j,t^{n+1}) =\;& \ac(y_j,t^{n}) + 
\dt \partial_t \ac(y_j,t^{n}) + 
\frac{\dt^2}{2} \partial_t^2 \ac(y_j,t^{n}) + O(\dt^3)\\
=\;& \ac(y_j,t^{n}) - 
\cp \dt \partial_y \ac(y_j,t^{n}) + 
\frac{\cp^2 \dt^2}{2} \partial_y^2 \ac(y_j,t^{n}) \nonumber \\
&+ i k_x \cp \dt \dc(y_j,t^n)
- \frac{k_x^2 \cp^2 \dt^2}{4} \left(\bc(y_j,t^{n}) - \ac(y_j,t^{n}) \right) + O(\dt^3).
\end{align}
% \begin{align}
% \ac^{n+1}_j &= \ac^{n}_j + 
% \dt \partial_t \ac^{n}_j + 
% \frac{\dt^2}{2} \partial_t^2 \ac^{n}_j + O(\dt^3)\\
% \ac^{n+1}_j &= \ac^{n}_j - 
% \cp \dt \partial_y \ac^{n}_j + 
% \frac{\cp^2 \dt^2}{2} \partial_y^2 \ac^{n}_j 
% + i k_x \cp \dt \dc^n_j
% - \frac{k_x^2 \cp^2 \dt^2}{4} (\bc^{n}_{j} - \ac^{n}_{j}) + O(\dt^3).
% \end{align}
%
A similar series can be derived for $\bc.$
The spacial derivatives are approximated by centered second order finite
difference formulas. Define the undivided difference operators
$\delta_+ u_j = u_{j+1} - u_j,$ 
$\delta_- u_j = u_j - u_{j-1},$ and $\delta_0 = (\delta_+ + \delta_-)/2$ 
for an arbitrary grid function $u_j.$ The scheme for $\ac$ and $\bc$
can be written as
\begin{align}
\ac^{n+1}_{j} &= \ac^{n}_j - 
\frac{\lambda_y}{2} \delta_0 \ac^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \ac^{n}_j 
+ i \lambda_x \dc^n_j
- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j)  \label{eq:aLax} \\
\bc^{n+1}_{j} &= \bc^{n}_j + 
\frac{\lambda_y}{2} \delta_0 \bc^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \bc^{n}_j 
- i \lambda_x \dc^n_j
- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j) \label{eq:bLax}
\end{align}
%
where $\lambda_x = k_x \cp \dt$ and $\lambda_y = \cp \dt / \dy.$
This is a Lax-Wendroff scheme for an advection equation with a source.
After advancing $\ac$ and $\bc$ to the next time level, $\dc$ can be
advanced with a simple quadrature. Since a non-dissipative pseudo-spectral approximation
is used in the $x$ direction, the trapezoidal rule is used to stabilize the approximation.
\begin{align}
\dc^{n+1}_j &= \dc^{n}_j + \frac{i \lambda_x}{4}
\left(\bc^{n+1}_j - \ac^{n+1}_j + \bc^n_j - \ac^n_j \right). \label{eq:dTrap}
\end{align}
%
The $\cp^+$ characteristic, $\ac,$ will be extrapolated to the interface ghost point.
Additionally, the solution must decay to zero at $y \rightarrow -\infty.$
\begin{alignat}{2}
\ac^n_{1} &= 2 \ac^n_{0} - \ac^n_{-1}, \quad && \\
\vert \ac^n_j \vert^2 +
\vert \bc^n_j \vert^2 +
\vert \dc^n_j \vert^2 &\rightarrow 0, \quad &&\text{as } j \rightarrow -\infty
\label{eq:bcInf}
\end{alignat}
%
The interface condition will determine $b_{1}^n,$ and the initial conditions will 
define $a_j^0, b_j^0,$ and $d_j^0$ for $j = 0,1,2,3,\ldots$.

The fluid variables are kept continuous in $y$ but discrete in time.
For this simplified model analysis, the interface conditions determine 
how the fluid variables are updated. For reference, the Fourier 
coefficients of the velocity and stress components are related to the characteristic 
variables by
\begin{align}
(\vsyh)_j^n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \quad
(\ssyh)_j^n = \frac{1}{2} (\bc^n_j+\ac^n_j), \quad
(\ssxh)_j^n = \dc^n_j.
\end{align}

\subsubsection{TP (traditional partitioned) interface conditions}

The TP algorithm is designed to treat the interface as a no-slip velocity 
boundary condition for the fluid and a no-slip traction boundary condition 
for the solid. For this model problem, the time-stepping scheme for the fluid
velocity does not play a role in the analysis. This is because the fluid pressure 
solution only depends on the interface acceleration, which is computed using the
solid solution. The interface acceleration is computed 
using a second order backward difference formula. 

\listAlgorithm{TP Algorithm (without iterations)}{
\item Advance solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
$j = 0,\, -1, \, -2, \, -3, \, \ldots$.

\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$

\item Set the interface velocity as the solid velocity.
\begin{align}
v_I^{n+1} = \frac{1}{2 \zp} \left(\bc_0^{n+1} 
- \ac_{0}^{n+1} \right)
\end{align}

\item Calculate the interface acceleration using a second order accurate
backward difference formula.
\begin{align}
\dot{v}_I^{n+1} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{n+1} 
  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
\end{align}

\item Solve the Poisson equation for the fluid pressure. 
The fluid momentum equation is used to obtain a compatibility 
condition on the pressure gradient at $y=0.$
\begin{alignat}{2}
\ph_{yy}^{n+1} - k_x^2 \ph^{n+1} &= 0, \quad && y \in (0,H), \\
\ph_y^{n+1} &= -\rho \dot{v}_I^{n+1}, \quad && y = 0, \\
\ph^{n+1} &= 0, \quad && y=H
\end{alignat}
%
The solution is
\begin{align}
\ph^{n+1}(y) &= \frac{\rho \dot{v}_I^{n+1} \sinh(k_x (H - y) )}{k_x \cosh(k_x H)} 
\end{align}

\item Set the fluid traction as the solid traction at the interface.
Let $p_I^{n+1} = \ph^{n+1}(0) = \rho \dot{v}_I^{n+1} \tanh(k_x H)/k_x.$
Use an average of the solid cells to obtain $\bc_{1}^{n+1}.$
\begin{align}
b^{n+1}_1 = -b^{n+1}_{-1} - a^{n+1}_1 - a^{n+1}_{-1} - 4 p_I^{n+1}
\end{align}
} \\

It will be shown that the TP algorithm without iterations is unconditionally unstable.
The TP iteration is also analyzed to supplement the results from the zero iteration
algorithm. Under-relaxed iterations are performed on the interface velocity with
under-relaxation parameter, $\omega.$ At the end of the iteration, the $\cp^-$ 
characteristic on the interface, $\bc_0,$ is updated. 

\listAlgorithm{TP Iteration}{
\item Set the interface velocity as the solid velocity.
\begin{align}
v_I^{(k+1)} = \frac{\omega}{2 \zp} \left(\bc_0^{(k)} 
- \ac_{0}^{n+1} \right) + (1-\omega) v_I^{(k)}
\end{align}

\item Calculate the interface acceleration using a second order accurate
backward difference formula.
\begin{align}
\dot{v}_I^{(k+1)} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{(k+1)} 
  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
\end{align}

\item Solve for the interface pressure
\begin{align}
p^{(k+1)}_I &= \frac{\rho \dot{v}_I^{(k+1)} \tanh(k_x H)}{k_x} 
\end{align}

\item Update the $\cp^-$ characteristic, $\bc_{0}^{(k+1)},$ at the interface.
\begin{align}
b^{(k+1)}_0 = -a^{n+1}_0 - 2 p_I^{(k+1)}
\end{align}
} \\

Define $\Heff = \tanh(k_x H)/k_x$ as the effective height of the fluid column. 
This quantity is present in each interface algorithm. For the 1D model problem
($k_x \rightarrow 0$), $\Heff \rightarrow H.$ As the wave number in the $x$ 
direction increases, $\Heff$ will decrease to $0.$ Define the mass ratio
\begin{align}
\Mra = \frac{\rho \Heff}{\zp \dt} = \frac{\rho \Heff}{\rhos \cp \dt}
= \frac{\rho \Heff}{\rhos \ly \dy}.
\end{align}
%
Consider boxes with a cross section of length $L$ in the $x$ direction 
and unit depth out of the $x-y$ plane.
$\Mra$ is the ratio of the fluid mass enclosed in the box of height $\Heff$ to 
the solid mass enclosed in the box of height $\cp \dt,$ or the distance that
a p-wave propagates in time $\dt.$  Additionally define
\begin{align}
\Mr = \ly \Mra = \frac{\rho \Heff}{\rhos \dy}.
\end{align}
%
$\Mr$ is a mass ratio which does not depend on the solid CFL number, $\ly.$
Both $\Mra$ and $\Mr$ decrease as $k_x$ increases.


\subsubsection{ATP (anti-traditional partitioned) interface conditions}

The anti-traditional algorithm reverses the role of the interface in the
traditional scheme. The fluid treats the interface as a no-slip 
traction boundary while the solid treats the interface as a no-slip
velocity boundary. For this algorithm, the fluid velocity is advanced after the
pressure step with trapezoidal rule integration.

\listAlgorithm{ATP Algorithm}{
\item Advance solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
$j = 0,\, -1, \, -2, \, -3, \, \ldots$.

\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$

\item Set the solid traction as the fluid traction at the interface.
\begin{align}
p_I^{n+1} = -\frac{1}{2} \left(b^{n+1}_0 + a^{n+1}_0 \right)
\end{align}

\item Solve the Poisson equation for the fluid pressure. The interface pressure
is used as a Dirichlet condition at $y=0.$
\begin{alignat}{2}
\ph_{yy}^{n+1} - k_x^2 \ph^{n+1} &= 0, \quad && y \in (0,H), \\
\ph^{n+1} &= p_I^{n+1}, \quad && y = 0, \\
\ph^{n+1} &= 0, \quad && y=H
\end{alignat}
%
The solution is
\begin{align}
\ph^{n+1}(y) &= \frac{p_I^{n+1} \sinh(k_x (H - y) )}{\sinh(k_x H)} 
\end{align}

\item Advance the interface velocity using trapezoidal rule on the fluid momentum
equation.
\begin{align}
v^{n+1}_I = v^{n}_I + \frac{k_x \dt}{2 \rho \tanh(k_x H)} 
\left(p_I^{n+1} + p_I^{n}\right)
\end{align}

\item Set the fluid velocity as the solid velocity. Use an average of the solid cells
to obtain $\bc_1^{n+1}.$
\begin{align}
b_{1}^{n+1} = -b_{-1}^{n+1} + a^{n+1}_{1} + a^{n+1}_{-1}
+ 4 \zp v_I^{n+1}
\end{align}
}

\subsubsection{AMP interface conditions}

The AMP algorithm has features from both the TP and ATP scheme. The
interface velocity is taken to be an impedance-weighted average of the 
fluid and solid velocities.
The crucial ingredient is the Robin condition for the pressure in the fluid.
For a large mass ratio, this approximates the Dirichlet problem for 
pressure in the ATP scheme while for a small mass ratio, this approximates the
Neumann problem for pressure in the TP Scheme.

\listAlgorithm{AMP Algorithm (added-mass partitioned)}{
\item Advance solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
$j = 0,\, -1, \, -2, \, -3, \, \ldots$.

\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$

\item Advance the fluid interface velocity using Adams Bashforth on 
the fluid momentum equation.
\begin{align}
v_f^{n+1} = v_I^n + \frac{k_x \dt}{2 \rho \tanh(k_x H)} 
\left( 3 p_I^n - p_I^{n-1} \right)
\end{align}

\item Get the interface velocity and traction from the solid.
\begin{align}
v_s^{n+1} &= \frac{1}{2 \bar{z}} \left(b^{n+1}_0 - a^{n+1}_0 \right) \\
\sigma_s^{n+1} &= \frac{1}{2} \left(b^{n+1}_0 + a^{n+1}_0 \right)
\end{align}

\item Set the interface velocity as the impedance weighted average
of the fluid and solid velocities.
\begin{align}
v_I^{n+1} = \frac{\zf v_f + \zp v_s}{\zf + \zp} 
\end{align}

\item Calculate the interface acceleration using a second order accurate
backward difference formula.
\begin{align}
\dot{v}_I^{n+1} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{n+1} 
  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
\end{align}

\item Solve the Poisson equation for the fluid pressure with
the AMP Robin condition specified at $y=0.$
\begin{alignat}{2}
\ph_{yy}^{n+1} - k_x^2 \ph^{n+1} &= 0, \quad && y \in (0,H), \\
-\ph^{n+1}+\frac{\zp \dt}{\rho} \ph_y^{n+1} &= 
\sigma_s^{n+1} - \zp \dt \dot{v}_I^{n+1}, \quad && y = 0, \\
\ph^{n+1} &= 0, \quad && y=H
\end{alignat}

The solution is
\begin{align}
\ph^{n+1}(y) &= p_I^{n+1} \frac{\sinh(k_x (H-y) )}{\sinh(k_x H)} \\
p_I^{n+1} &= \frac{1}{M+1} 
\frac{\rho \dot{v}_I \tanh{(k_x H)}}{ k_x }
 - \frac{M}{M+1} \sigma_s
\end{align}

\item Set the interface traction $\sigma_I^{n+1} = -p_I^{n+1}.$
Set the $\cp^-$ characteristic, $\bc,$ using the interface velocity and stress.
$\delta = \rho/\rhos.$
\begin{align}
%b^{n+1}_1 = -b^{n+1}_{-1} + 2 \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right).
\bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 
\left[\frac{1}{1+\delta} 
\left(2 \sigma_I^{n+1} - \frac{\ac^{n+1}_{1} + \ac^{n+1}_{-1}}{2} \right)
+\frac{\delta}{1+\delta} \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right) \right].
\end{align}
}


\subsection{Stability analysis of AMP, TP, and ATP schemes}

We will now look for normal mode solutions to the discretizations in terms of an
amplification factor, $\amp.$ Let
\begin{align}
\ac^{n}_j = \amp^n \tac_j, \quad 
\bc^{n}_j = \amp^n \tbc_j, \quad 
\dc^{n}_j = \amp^n \tdc_j,
\end{align}
%
where tilde variables are spacial grid functions. The scheme is said to be weakly
stable if there are no non-trivial solutions where $|\amp| > 1.$ Our strategy for
determining the stability region will be to search only for unstable modes, $|A| > 1.$ 
First, the analysis is split into a spacial and temporal problem. The tilde variables 
will be determined from the interior discretization and boundary condition as 
$y \rightarrow -\infty.$ Solutions for the amplification factor will be found by
finding non-trivial solutions when the normal mode anzatz is
substituted into the interface conditions.

First we reduce the size of the problem by using equation \eqref{eq:dTrap}
to find $\tdc$ in terms of $\tac$ and $\tbc.$ 
\begin{align}
\tdc_j = i \lx D(\amp) (\tbc_j - \tac_j)
\end{align}
%
where
\begin{align}
D(\amp) = \frac{1}{4} \frac{\amp+1}{\amp-1}.
\end{align}
%
Equations \eqref{eq:aLax}--\eqref{eq:bLax} can be written as a system of 
linear second order difference equations. 
Let $\tacv_j = [\tilde{\ac}_j,\tilde{\bc}_j]^T,$ then
\begin{align}
\amp \tacv_j &= 
(I + H_0 + H_1 \delta_0 + H_2 \delta_+ \delta_-) 
\tacv_j \label{eq:diffScheme}
\end{align}
%
where
\begin{align}
H_0 &= \left[ \begin{array}{cc}
-\lambda_x^2 D(\amp) - \frac{\lambda_x^2}{4}
& \lambda_x^2 D(\amp) + \frac{\lambda_x^2}{4} \\
\lambda_x^2 D(\amp) + \frac{\lambda_x^2}{4} & 
-\lambda_x^2 D(\amp) - \frac{\lambda_x^2}{4}
\end{array} \right], \\
H_1 &= \left[ \begin{array}{cc}
-\frac{\lambda_y}{2} + \frac{\lambda_x^2 \lambda_y}{4} D(\amp)
& - \frac{\lambda_x^2 \lambda_y}{4} D(\amp) \\
\frac{\lambda_x^2 \lambda_y}{4} D(\amp) &
\frac{\lambda_y}{2} - \frac{\lambda_x^2 \lambda_y}{4} D(\amp)
\end{array} \right], \\
H_2 &= \left[ \begin{array}{cc}
\frac{\lambda_y^2}{2} & 0 \\ 0 & \frac{\lambda_y^2}{2}
\end{array} \right].
\end{align}
%
Solutions are sought of the form $\tacv_j = \rev \p^j.$ This is substituted into 
equation \eqref{eq:diffScheme} to obtain
\begin{align}
A \rev &= \left( I + H_0 + H_1 \left(\p - \frac{1}{\p}\right)
+ H_2 \left(\p - 2 + \frac{1}{\p} \right) \right) \rev  \label{eq:evProblem}
\end{align}
%
Non trivial solutions for $\p$ are found when the above problem is singular,
therefore
\begin{align}
0 &= \det\bigg{(}I(1-A) + H_0 + H_1 \left(\p - \frac{1}{\p}\right)
+ H_2 \left(\p - 2 + \frac{1}{\p} \right) \bigg{)}. \label{eq:quarticPhi}
\end{align}
%
This results in a quartic polynomial for $\p.$ Due to the boundary condition as
$y \rightarrow -\infty,$ \eqref{eq:bcInf}, we are only interested in solutions 
where $|\p|^j \rightarrow 0$ as $j \rightarrow -\infty.$ Therefore, only $|\p| > 1$ is
a valid solution. Since $|A| > 1$ and the scheme is dissipative, we have
$|\p_1| > 1, |\p_2| > 1, |\p_3| < 1, |\p_4| < 1.$ \todo{ cite Kreiss, explain further.}
We can now write the general solution as
\begin{align}
\acv^n_j = \amp^n \left(k_1 \rev_1 \p_1^j + 
k_2 \rev_2 \p_2^j \right).
\end{align}
%
Let $\rev_n = [\qn{n},\rn{n}]^T$ for $n = 1,2.$
When this is plugged into the interface conditions, a system of equations arise.
\begin{align}
\dMat \kv= \left[\begin{array}{cc}
\dComp_{11} & \dComp_{12} \\
\dComp_{21} & \dComp_{22}
\end{array}\right] 
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right] = 0.
\end{align}
%
The first row represents extrapolation of the $\cp^+$ characteristic into the interface
ghost point and is the same for each algorithm.
\begin{align}
\dComp_{1n} = \qn{n} \left(\p_n - 2 + \frac{1}{\p_n} \right), \quad n = 1,2
\end{align}
%
% \begin{align}
% \dComp_{2n} = \begin{cases}
% (\rn{n}+\qn{n}) \left(\p_n + \frac{1}{\p_n} \right)
% + (\rn{n}-\qn{n}) \frac{ M (3 A - 1) (A-1) }{A^2}, & \text{TP} \\
% %%%%%%%%%%%%%%%%%%%%
% (\rn{n}-\qn{n}) \left(\p_n + \frac{1}{\p_n} \right)
% + (\rn{n}+\qn{n}) \frac{(A + 1)}{M (A-1)}, & \text{ATP} \\
% %%%%%%%%%%%%%%%%%%%%
% \rn{n} \left(\p_n + \frac{1}{\p_n} \right)
% \Big(- \left( M+1 \right)^{2} {A}^{4} +\frac{1}{4} \left( 4{M}^{2}+13M
%  \right) {A}^{3} \\
% \phantom{\rn{n} \left(\p_n + \frac{1}{\p_n} \right) \Big{(} }
% -{\frac {15M}{4}}A^2 +\frac{7}{4}M A-\frac{M}{4} \Big{)} \\
% %
% + \qn{n} \left(  \left( {M}^{2}+3/2M-1 \right) {A}^{2}+ \left( -{M}^{2}-7/2
% M \right) A+M \right) {A}^{2} \\
% %
% + \rn{n} 1/2 \left( 2{M}^{2}+M+2 \right) {A}^{4}+1/2 \left( -2{M}^{2}+M
%  \right) {A}^{3}, & \text{AMP}
% \end{cases}
% \end{align}
%
The second row is given by
\begin{align}
\dComp_{2n,\text{TP}} = \;&
 (\rn{n}-\qn{n}) \frac{ M (3 A - 1) (A-1) }{A^2}
+(\rn{n}+\qn{n}) \left(\p_n + \frac{1}{\p_n} \right), \\
% \end{align}
%
% \begin{align}
\dComp_{2n,\text{ATP}} = \;&
 (\rn{n}+\qn{n}) \frac{(A + 1)}{M (A-1)}
+ (\rn{n}-\qn{n}) \left(\p_n + \frac{1}{\p_n} \right), \\
% \end{align}
%
% \begin{align}
\dComp_{2n,\text{AMP}} =\;& 
 \frac{1}{2} \rn{n} \left(\left( 2{M}^{2}+M+2 \right) {A}^{4}+ \left( -2{M}^{2}+M
 \right) {A}^{3} \right),  \nonumber \\
%
&+ \qn{n} \left(  \left( {M}^{2}+\frac{3}{2}M-1 \right) {A}^{2}- \left( {M}^{2}
+\frac{7}{2}
M \right) A+M \right) {A}^{2} \\
%
& \rn{n} \left( \p_n + \frac{1}{\p_n} \right)
\left(- \left( M+1 \right)^{2} {A}^{4} +\frac{1}{4} \left( 4{M}^{2}+13M
 \right) {A}^{3} -{\frac {15M}{4}}A^2 +\frac{7}{4}M A-\frac{M}{4} \right) \nonumber 
\end{align}
%
for $n = 1,2.$ For non-trivial solutions, we look for solutions of $\amp$ such that
\begin{align}
\det(\dMat) = \dComp_{11} \dComp_{22} - \dComp_{12} \dComp_{21} = 0.
\end{align}
%
We first proceed with an analysis of the 1D case ($\lx \rightarrow 0$). After finding 
1D solutions for $\amp,$ numerical continuation in $\lx$ is used to follow the 
evolution of $\amp$ as the wave number in the $x$ direction increases.


%\subsubsection{Stability for Cauchy problem in the solid}

% phi's are now exponentials
% plot stability region
% talk about dissipation

\subsubsection{1D scheme}

When $\lx \rightarrow 0,$ the equations in the solid become two uncoupled advection 
equations for the $\cp^+$ characteristic, $\ac,$ and the $\cp^-$ characteristic, $\bc.$
The solid scheme is Lax-Wendroff without source corrections. 
Equation \eqref{eq:diffScheme}
simplifies to 
\begin{align}
A \tac_j = \left( 1 - \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tac_j, \quad
A \tbc_j = \left( 1 + \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tbc_j
\end{align}
%
The solutions to the eigenvalues, $\p,$ are given by
\begin{align}
\p_{\bc,\pm} = {\frac {{\lambda_{{y}}}^{2}+A-1 \pm \sqrt {2\,A{\lambda_{{y}}}^{2}+{A}^{2}-{
\lambda_{{y}}}^{2}-2\,A+1}}{\lambda_{{y}} \left( \lambda_{{y}}-1
 \right) }}, \quad 
\p_{\ac,\pm} =  \frac{\lambda_y - 1}{\lambda_y + 1} \p_{\bc,\pm}
\end{align}
%
It is well known (e.g. \cite{GKSII}) that when $|A| > 1,$ either
$|\phi_{a,+}| > 1 > |\phi_{a,-}|$ or 
$|\phi_{a,-}| > 1 > |\phi_{a,+}|.$ Define $\phi_1$ and $\phi_2$ to be piecewise, 
so that their magnitudes are strictly greater than one.
\begin{align}
\phi_{1} = \begin{cases}
\phi_{b,+}, & |\phi_{b,+}| > 1 > |\phi_{b,-}| \\
\phi_{b,-}, & |\phi_{b,-}| > 1 > |\phi_{b,+}| \\
\end{cases}, \quad
\phi_{2} = \begin{cases}
\phi_{a,+}, & |\phi_{a,+}| > 1 > |\phi_{a,-}| \\
\phi_{a,-}, & |\phi_{a,-}| > 1 > |\phi_{a,+}| \\
\end{cases}
\end{align}
%
Since $\ac$ and $\bc$ are decoupled, the corresponding eigenvectors are unit vectors,
$\rev_{1} = [0,1]^{T}$ and $\rev_{2} = [1,0]^{T}$ (i.e. $\qn{1} = \rn{2} = 0$). 
The remaining nonzero components of $\dMat$ are $\dComp_{12}$ and $\dComp_{21},$ which leaves
\begin{align}
\det(\dMat_{\text{1D}})= -\dComp_{12} \dComp_{21} = 0
\end{align}
% 
$\dComp_{12}$ is a standard extrapolation operator with repeated roots of $\p_2 = 1.$ 
Since an eigenvalue of magnitude one does not satisfy the boundary conditions, these roots
will be ignored. Upon substituting $\p_1$ as a function of $\amp$ into $\dComp_{21},$
a polynomial can be formed for $\amp$ with coefficients that depend on $\lambda_y$
and $M.$ Maple was used to generate the polynomials for the TP, ATP, and AMP
schemes.
\begin{align}
P_{\text{TP}} =\;& 
 4 {\amp}^{6}
%
+ \left( 12 M{\lambda_{{y}}}^{2
}+8 {\lambda_{{y}}}^{2}-8 \right) {\amp}^{5} \nonumber \\
% 
&+ \left( 9 {M}^{2}{
\lambda_{{y}}}^{4}+12 M{\lambda_{{y}}}^{4}-9 {M}^{2}{\lambda_{{y}}}^
{2}+4 {\lambda_{{y}}}^{4}-28 M{\lambda_{{y}}}^{2}-4 {\lambda_{{y}}}
^{2}+4 \right) {\amp}^{4}\nonumber \\
%
&+ \left( -24 {M}^{2}{\lambda_{{y}}}^{4}
-16 M{\lambda_{{y}}}^{4}+24 {M}^{2}{\lambda_{{y}}}^{2}+20 M{\lambda
_{{y}}}^{2} \right) {\amp}^{3}\nonumber \\
%
&+ \left( 22 {M}^{2}{\lambda_{{y}}}
^{4}+4 M{\lambda_{{y}}}^{4}-22 {M}^{2}{\lambda_{{y}}}^{2}-4 M{
\lambda_{{y}}}^{2} \right) {\amp}^{2}\nonumber \\
%
&+ \left( -8 {M}^{2}{\lambda
_{{y}}}^{4}+8 {M}^{2}{\lambda_{{y}}}^{2} \right) {\amp}
%
+{M}^{2}{
\lambda_{{y}}}^{4}-{M}^{2}{\lambda_{{y}}}^{2} \nonumber\\
% \end{align}
% %
% \begin{align}
P_{\text{ATP}} =\;& 4 {M}^{2}{\amp}^{4}
%
+ \left( 8 {M}^{2}{
\lambda_{{y}}}^{2}+4 {\lambda_{{y}}}^{2}M-16 {M}^{2} \right) {\amp}^{3}\nonumber \\
%
&+ \left( 4 {M}^{2}{\lambda_{{y}}}^{4}+4 M{\lambda_{{y}}}^{4
}-20 {M}^{2}{\lambda_{{y}}}^{2}+{\lambda_{{y}}}^{4}-4 {\lambda_{{y}}
}^{2}M+24 {M}^{2}-{\lambda_{{y}}}^{2} \right) {\amp}^{2}\nonumber \\
%
&+ \left( -8 {M}^{2}{\lambda_{{y}}}^{4}+16 {M}^{2}{\lambda_{{y}}}^{2}+
2 {\lambda_{{y}}}^{4}-4 {\lambda_{{y}}}^{2}M-16 {M}^{2}-2 {\lambda
_{{y}}}^{2} \right) {\amp} \nonumber \\
%
&+4 {M}^{2}{\lambda_{{y}}}^{4}-4 M{
\lambda_{{y}}}^{4}-4 {M}^{2}{\lambda_{{y}}}^{2}+{\lambda_{{y}}}^{4}+4
 {\lambda_{{y}}}^{2}M+4 {M}^{2}-{\lambda_{{y}}}^{2} \nonumber \\
% \end{align}
% %
% \begin{align}
P_{\text{\text{AMP}}} =\;& \big{(} 16 {M}^{4}+64 {M}^{3}+96 {M}^{2}+64 M+
16 \big{)} {\amp}^{10}\nonumber \\
%
&+ \big{(} 16 {M}^{4}{\lambda_{{y}}}^{2}+88
 {M}^{3}{\lambda_{{y}}}^{2}-64 {M}^{4}+144 {M}^{2}{\lambda_{{y}}}^{
2}-296 {M}^{3}\nonumber \\
& \phantom{(+)}+88 M{\lambda_{{y}}}^{2}-432 {M}^{2}+16 {\lambda_{{y
}}}^{2}-232 M-32 \big{)} {\amp}^{9}\nonumber \\
%
&+ \big{(} 4 {M}^{4}{\lambda_{
{y}}}^{4}+28 {M}^{3}{\lambda_{{y}}}^{4}-36 {M}^{4}{\lambda_{{y}}}^{2
}+57 {M}^{2}{\lambda_{{y}}}^{4}-280 {M}^{3}{\lambda_{{y}}}^{2}\nonumber \\
& \phantom{(+)} +28 M
{\lambda_{{y}}}^{4}+96 {M}^{4}-495 {M}^{2}{\lambda_{{y}}}^{2}+4 {
\lambda_{{y}}}^{4}+624 {M}^{3}\nonumber \\
& \phantom{(+)} -192 M{\lambda_{{y}}}^{2}+985 {M}^{2}
-4 {\lambda_{{y}}}^{2}+392 M+16 \big{)} {\amp}^{8}\nonumber \\
% 
&+ \big{(} -8 
{M}^{4}{\lambda_{{y}}}^{4}-84 {M}^{3}{\lambda_{{y}}}^{4}+24 {M}^{4}{
\lambda_{{y}}}^{2}-204 {M}^{2}{\lambda_{{y}}}^{4}+428 {M}^{3}{
\lambda_{{y}}}^{2}-56 M{\lambda_{{y}}}^{4} \nonumber \\
% 
& \phantom{(+)} -64 {M}^{4}+1018 {M}^{2}{
\lambda_{{y}}}^{2}-792 {M}^{3}+236 M{\lambda_{{y}}}^{2}-1560 {M}^{2
}-400 M \big{)} {\amp}^{7} \nonumber \\
%
&+ \big{(} 4 {M}^{4}{\lambda_{{y}}}^{4}
+116 {M}^{3}{\lambda_{{y}}}^{4}-4 {M}^{4}{\lambda_{{y}}}^{2}+406 {M
}^{2}{\lambda_{{y}}}^{4}-380 {M}^{3}{\lambda_{{y}}}^{2}+60 M{\lambda
_{{y}}}^{4} \nonumber \\
&\phantom{(+)} +16 {M}^{4}-1426 {M}^{2}{\lambda_{{y}}}^{2}+640 {M}^{3}-
144 M{\lambda_{{y}}}^{2}+1836 {M}^{2}+240 M \big{)} {\amp}^{6} \nonumber \\
%
&+ \big{(} -88 {M}^{3}{\lambda_{{y}}}^{4}-518 {M}^{2}{\lambda_{{y}}}^{
4}+184 {M}^{3}{\lambda_{{y}}}^{2}-28 M{\lambda_{{y}}}^{4}+1376 {M}^
{2}{\lambda_{{y}}}^{2} \nonumber \\
&\phantom{(+)} -312 {M}^{3}+40 M{\lambda_{{y}}}^{2}-1584 {M}
^{2}-72 M \big{)} {\amp}^{5} \nonumber \\
%
&+ \big{(} 32 {M}^{3}{\lambda_{{y}}}^
{4}+435 {M}^{2}{\lambda_{{y}}}^{4}-44 {M}^{3}{\lambda_{{y}}}^{2}+4 
M{\lambda_{{y}}}^{4} \nonumber \\
&\phantom{(+)} -909 {M}^{2}{\lambda_{{y}}}^{2}+80 {M}^{3}-4 M{
\lambda_{{y}}}^{2}+974 {M}^{2}+8 M \big{)} {\amp}^{4}\nonumber \\
%
&+ \big{(} -
4 {M}^{3}{\lambda_{{y}}}^{4}-238 {M}^{2}{\lambda_{{y}}}^{4}+4 {M}^{
3}{\lambda_{{y}}}^{2}+396 {M}^{2}{\lambda_{{y}}}^{2}-8 {M}^{3}-408 
{M}^{2} \big{)} {\amp}^{3}\nonumber \\
%
&+ \big{(} 79 {M}^{2}{\lambda_{{y}}}^{4}
-107 {M}^{2}{\lambda_{{y}}}^{2}+108 {M}^{2} \big{)} {\amp}^{2}\nonumber \\
%
&+ \big{(} -14 {M}^{2}{\lambda_{{y}}}^{4}+16 {M}^{2}{\lambda_{{y}}}^{2}
-16 {M}^{2} \big{)} {\amp}
%
+{M}^{2}{\lambda_{{y}}}^{4}-{M}^{2}{
\lambda_{{y}}}^{2}+{M}^{2}  \nonumber
\end{align}
%
All solutions to $\det(\dMat_{\text{1D}}) = 0$ are roots of the characteristic 
polynomials, but some spurious roots were introduced in deriving these polynomials.
These spurious roots are easily identified by evaluating $\det(\dMat_{\text{1D}}).$
We evaluate the roots numerically for an array of equally spaced parameters in
the $\ly-\Mr$ plane. 
The roots of the AMP polynomial were found at an array of $800$ points in 
$10^{-6} \le \lambda_y \le 1$ and $800$ points in $10^{-6} \le \Mr \le 10^{7}.$ 
No unstable roots, $|A| > 1,$ were found. The same process was repeated for the 
TP and ATP schemes for a range $10^{-6} \le \Mr \le 10.$ The stability region
was plotted in figure \ref{fig:acousticSolidStokesStabilityTP}. 
Since $\Mr \propto \dy^{-1},$ grid refinement will increase the mass ratio.
The TP scheme will become unstable for sufficiently large $\Mr,$ therefore the 
scheme is formally unconditionally unstable. On the other hand, the ATP scheme will 
eventually become stable for a sufficiently large $\Mr.$ This scheme is weakly
stable. Despite this, there is a significant
region in parameter space where only the AMP scheme is stable.

{
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityRegion}
  \caption{Stability region for the 1D TP and ATP schemes. 
    The stability region for the AMP scheme spans 
    $0 < \ly < 1,$ $0 < \Mr < \infty.$ For reference, 
    $\lambda_y = \bar{c} \dt / \dy$ and $\Mr = \rho H / (\rhos \dy).$
    Grid refinement corresponds to increasing $\Mr,$ therefore the
    TP scheme will become unstable and the ATP scheme will become stable.
  }  \label{fig:acousticSolidStokesStabilityTP}
\end{center}
\end{figure}
}

% talk about numerical results

% Numerical Results:
%  - convergence for each scheme
%  - confirm stability region for each scheme
%
%   TP:
%     - heavy solid convergence study
%     - show stability region
%   ATP: 
%     - light solid convergence study
%     - show stability region
%   AMP:
%     - heavy/light solid convergence study
%     - really heavy/really light

\subsubsection{Continuation into 2D}

% derive eigenvectors with the idea that lx is small
% Now we approach the 2D model problem by considering $\lx$ to be a small 
% perturbation to the 1D problem. The main motivation for this is
% that the stability limit for the Cauchy problem requires $\lx < .3,$ (\todo{show this})
% and only $\lx^2$ appears in the discretization. 
%Additionally, the 2D added mass ratio
%$\Mr = (\rho \tanh(k_x H))/(k_x \rhos \dy)$ will only decrease as $k_x$ increases
The strategy for finding roots for $\lx \ne 0$ is to use the 1D roots as a starting point
for a numerical root solver that performs a continuation for $\lx > 0.$ The first step
is finding a suitable expression for the eigenvectors $\rev_1$ and $\rev_2$ so that
$\rev_1 / \| \rev_1 \| \rightarrow [0,1]^T, 
 \rev_2 / \| \rev_2 \| \rightarrow [1,0]^T$ as $\lx \rightarrow 0.$
The first and second components of equation \eqref{eq:evProblem} are used to define
$\rev_1$ and $\rev_2,$ respectively.
\begin{align*}
\qn{1} =\;& -{\lambda_{{x}}}^{2} \left( A{\p_1}^{2}\lambda_{{y}}+{\p_1}^{2}\lambda
_{{y}}-8A\p_1-A\lambda_{{y}}-\lambda_{{y}} \right) \\
%
\rn{1} =\;& -A{\p_1}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}-8A{\p_1}^{2}{\lambda_{{
y}}}^{2}-{\p_1}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}+8A{\p_1}^{2}
\lambda_{{y}}+8A\p_1{\lambda_{{x}}}^{2}+16A\p_1{\lambda_{{y}}}
^{2} \nonumber \\
& +A{\lambda_{{x}}}^{2}\lambda_{{y}}+8{\p_1}^{2}{\lambda_{{y}}}^{2
}+16{A}^{2}\p_1-8A{\lambda_{{y}}}^{2}-8{\p_1}^{2}\lambda_{{y}}-
16\p_1{\lambda_{{y}}}^{2}+{\lambda_{{x}}}^{2}\lambda_{{y}} \nonumber\\
& -32A \p_1-8A\lambda_{{y}}+8{\lambda_{{y}}}^{2}+16\p_1+8\lambda_{{y}
}\\
%
\qn{2} =\;& A{\p_2}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}-8A{\p_2}^{2}{\lambda_{{y
}}}^{2}+{\p_2}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}-8A{\p_2}^{2}
\lambda_{{y}}+8A\p_2{\lambda_{{x}}}^{2}+16A\p_2{\lambda_{{y}}}
^{2} \nonumber\\
& -A{\lambda_{{x}}}^{2}\lambda_{{y}}+8{\p_2}^{2}{\lambda_{{y}}}^{2
}+16{A}^{2}\p_2-8A{\lambda_{{y}}}^{2}+8{\p_2}^{2}\lambda_{{y}}-
16\p_2{\lambda_{{y}}}^{2}-{\lambda_{{x}}}^{2}\lambda_{{y}} \nonumber\\
& -32A \p_2+8A\lambda_{{y}}+8{\lambda_{{y}}}^{2}+16\p_2-8\lambda_{{y}
} \\
%
\rn{2} =\;& {\lambda_{{x}}}^{2} \left( A{\p_2}^{2}\lambda_{{y}}+{\p_2}^{2}\lambda_
{{y}}+8A\p_2-A\lambda_{{y}}-\lambda_{{y}} \right) .
\end{align*}
%
It is easy to see that $\qn{1} = \rn{2} = 0$ when $\lambda_x = 0.$ In order to solve for 
roots numerically, a black box residual function was created to evaluate $\det(\dMat)$
given $A, \ly, \lx,$ and $\Mra.$ The eigenvalues and eigenvectors can be determined from
these inputs.

% residual function for root solver
\listAlgorithm{Compute Residual of $\det(\dMat)$}{
\item Given $A, \ly,$ and $\lx,$
solve the quartic polynomial for $\p,$ equation \eqref{eq:quarticPhi}, with
ordering $|\p_1| > |\p_2| > |\p_3| > |\p_4|.$ Only $\p_1$ and $\p_2$ are
kept.
\item Calculate the corresponding eigenvectors, $\rev_1$ and $\rev_2.$
\item Given $\Mra,$ form components of $\dMat$ and take the determinant.
} \\

Now that a residual function is introduced, a nonlinear equation solver can be
employed to obtain roots near an initial guess. For this paper, a Newton solver
was used with a Jacobian approximated by finite differences. 
The continuation procedure is outlined as follows.
$\lx$ is discretized 
according to $(\lx^2)_k = k \Delta \lx^2,$ for $k = 0,1,\ldots N$, 
where $\Delta \lx^2 = (\lx^2)_f / N.$ 
Define $A^{(k)}_j$ as the $j$th root corresponding to $\lx = (\lx)_k.$
The 1D root, $A^{(0)}_j$ is used as an initial guess to the 2D problem 
for $k=1$ with $\lx^2 = (\lx^2)_1 = \Delta \lx^2$ to obtain a solution $A^{(1)}_j.$
From here on, the solution $A^{(k-1)}_j$ is used as an initial guess to the 
$\lx^2 = (\lx^2)_{k}$ problem to obtain $A^{(k)}.$

% continuation algorithm
% \listAlgorithm{Continuation in $\lx$}{
% \item Calculate 
% \item $\Delta \lx^2 = (\lx^2)_f/N$
% }
\begin{algorithm}[h]
\caption{Continuation in $\lx$}\label{contour}
\begin{algorithmic}[1]
\Procedure{continuationTP}{$(\lx)_{f},\ly,\Mr,N$}
\State $\Delta \lx^2 \gets (\lx^2)_f/N$ 
% calculate 1D roots
\State Calculate roots, $A_{j}^{(0)},$ 
for $j = 1,\, ...,\, N_{\text{roots}}.$
\For{$j = 1,\, ...,\, N_{\text{roots}}$}
\For{$k = 1,\, ...,\, N$}
\State $(\lx)_k = \sqrt{k \Delta \lx^2}$
\State $A_j^{(k)} \gets$ 
{\tt solveDeterminant}$\left((\lx)_k,\ly,\Mr,A_j^{(k-1)}\right) $
%\Comment{use previous solution as an initial guess}
\EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

For both the TP and ATP schemes,
there exists a surface $\Mr^*(\lx,\ly)$ such that $|A| = 1.$ 
Given $\lx$ and $\ly,$ a point on this surface can be computed using a root solving 
algorithm for $|A|=1.$ Since $|A|$ may not be smooth over the search region, the
bisection algorithm was used for it's robustness. 

%%%%%%%%%%%%%%%%%%
In order to ensure stability of the pseudo-spectral approximation, 
all Fourier modes must be stable.
Therefore for a given $\ly,$ we are interested 
the worst case mass ratio for $\lx \in \mathcal{D}(\ly),$ where 
$\mathcal{D}(\ly)$ is the Cauchy stability bound for $\lx.$
Recall $k_x = \frac{2 \pi k}{L},$ for $k = 0, \pm 1, \dots, \pm \frac{N_x}{2}$
The wave number will be bounded by
\begin{align}
0 \le |k_x| \le \frac{\pi N_x}{L} = \frac{\pi}{\dx},
\end{align}
%
which implies the CFL number in the $x$ direction will be bounded by
\begin{align}
0 \le \lx \le \pi \frac{\cp \dt}{\dx}.
\end{align}
%
Since there will be a finite number of wave numbers, there will be a CFL number and mass ratio
corresponding to each wave number.
\begin{align}
0 &= (\lx)_0 < (\lx)_1 < ... < (\lx)_{N_x/2} =
    \pi \frac{\bar{c} \Delta t}{\Delta x}, \\
\frac{\rho H}{\bar{\rho} \dy} 
  &= \Mr_0 > \Mr_1 > ... > \Mr_{N_x/2} = 
    \frac{\rho H}{\bar{\rho} \dy} \frac{\tanh(\pi H/ \dx) }{\pi H/\dx}.
\end{align}
%
For stability of the TP and ATP schemes, we must have
\begin{align}
  (\Mr_{\text{TP}})_j &\le \Mr^*_{\text{TP}}((\lx)_j,\ly) \\
  (\Mr_{\text{ATP}})_j &\ge \Mr^*_{\text{ATP}}((\lx)_j,\ly).
\end{align}
%
Define $\bar{\Mr}$ to be the worst case mass ratio.
\begin{align}
  \bar{\Mr}_{\text{TP}}(\ly) &= \min_{\lx \in \mathcal{D}(\ly)} \Mr^*_{\text{TP}} (\lx,\ly) 
\label{eq:MrbarTP}\\
  \bar{\Mr}_{\text{ATP}}(\ly) &= \max_{\lx \in \mathcal{D}(\ly)} \Mr^*_{\text{ATP}} (\lx,\ly)
\label{eq:MrbarATP}
\end{align}
%
A conservative bound can be placed by taking the 
extreme ends of the inequalities.
\begin{align}
  (\Mr_{\text{TP}})_0 &\le \bar{\Mr}_{\text{TP}}(\ly) \\
  (\Mr_{\text{ATP}})_{N_x/2} &\ge \bar{\Mr}_{\text{ATP}}(\ly)
\end{align}
%
{
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}[H]
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityRegion2D}
  \caption{Stability region for the 1D and 2D TP and ATP schemes. 
    $\bar{\Mr}$ is defined from 
    equations \eqref{eq:MrbarTP}--\eqref{eq:MrbarATP} and is the worst
    case mass ratio for all Fourier modes.
    $\lambda_y = \bar{c} \dt / \dy$ is the CFL number.
    The stability region for the AMP scheme spans 
    $0 < \ly < 1,$ $0 < \bar{\Mr} < \infty.$ 
    An increase in $\bar{\Mr}$ corresponds to grid refinement,
    therefore TP scheme will become unstable and the ATP scheme will become stable.
  }  \label{fig:acousticSolidStokesStabilityTP2D}
\end{center}
\end{figure}
}

The time step restriction for the TP scheme is given by
\begin{align}
  \dt &\ge \frac{\ly}{\bar{\Mr}_{\text{TP}}(\ly)} \frac{\rho}{\bar{\rho}} \frac{H}{\cp}.
\label{eq:TPTimeStep2D}
\end{align}
%
For a fixed $\ly,$ the right hand side of equation \eqref{eq:TPTimeStep2D} is 
a constant independent of the grid spacing. Therefore the scheme will eventually become
unstable when the time step is sufficiently small. When the solid density is much larger 
than the fluid density, this condition is less restrictive.
%
The time step restriction for the ATP scheme is given by
\begin{align}
  \dt &\le \frac{\ly \tanh(\pi H/ \dx)}{ \pi \bar{\Mr}_{\text{ATP}}(\ly)} 
        \frac{\rho}{\bar{\rho}} \frac{\dx}{\cp}.
\label{eq:AntiTPTimeStep2D}
\end{align}
%
The right hand side of equation \eqref{eq:AntiTPTimeStep2D} scales 
like $\dx,$ therefore a stable time step can always be chosen. 
% Figure \ref{fig:acousticSolidStokesStabilityTP2D} shows that $\bar{\Mr}_{\text{ATP}}$
% can be quite large comparted to $\bar{\Mr}_{\text{TP}}.$ As a result the 
% time step must be tiny.
Although this algorithm is formally stable, it is not practical for all problems.
When the solid is much heavier than the fluid (large $\rhos/\rho$), a tiny time
step is needed. For this case, the traditional algorithm may be more suitable.
As seen in figure \ref{fig:acousticSolidStokesStabilityTP2D}, there is a region
where neither algorithm is stable, which motivates the necessity for the AMP algorithm.

For the AMP algorithm, roots were calculated for $N$ equally spaced points
in the solid stability region and $N$ equally spaced points in 
$10^{-4} < \Mr < 10^{4}$ to verify that no unstable roots were found.

\subsection{Stability analysis of TP scheme with iterations}

The TP scheme is more commonly used with iterations to avoid the added mass instability
when refining grids. We perform an analysis of the TP iteration to understand
how to choose the under-relaxation factor and how many iterations to take.
Define the error between iterations to be the difference in interface velocities
\begin{align}
e^{(k)} = v_I^{(k+1)} - v_I^{(k)}.
\end{align}
%
By taking the difference between the current and previous iteration variable for
each step of the TP iteration, one can derive that
\begin{align}
e^{(k)} &= \left(1 - \omega \left(\frac{3}{2} \Mra + 1 \right)\right) e^{(k-1)}.
\end{align}
%
Define the amplification factor, $\ampI = 1 - \omega \left(\frac{3}{2} \Mra + 1 \right)$
where $e^{(k)} = A^{k} e^{(0)}.$
$\Mra$ is dependent on the wave number, $k_x.$ In order to optimize the convergence rate,
$\ampI$ needs to be optimized for all wave numbers.
\begin{align}
\Mra = \frac{\rho \tanh(k_x H)}{\zp \dt k_x} 
= \frac{\rho H}{\zp \dt} \frac{\tanh(k_x H)}{k_x H} 
= \Mra_0 \eta
\end{align}
%
where $\Mra_0 = (\rho H) / (\zp \dt)$ is the 1D acoustic mass ratio and 
$\eta = \tanh(k_x H) / (k_x H)$ is the 2D scale factor. To accommodate all
potential wave numbers in the $x$ direction, we consider $\eta \in [0,1].$
Let $\Mra = \Mra(\eta) = \Mra_0 \eta.$ The amplification factor for a given
$\omega$ and $\eta$ is
\begin{align}
\ampI(\eta,\omega) = a - \omega \left(\frac{3}{2} M_0 \eta + 1 \right).
\end{align}
%
We pose the following optimization problem to find the optimal 
under-relaxation parameter, $\omega^*$.
\begin{align}
\omega^* = \argmin_{\omega} \max_{0 \le \eta \le 1} |A(\eta,\omega)|
\end{align}
%
Since $\ampI$ is linear in $\eta$ and $\omega$ and $|\ampI| > 0,$ the maximum 
amplification factor for a 
given $\omega$ will occur on the boundary, $\eta = 0$ or $\eta = 1.$ 
\begin{align}
\ampI(\eta=0,\omega) = |1-\omega|, \quad 
\ampI(\eta=1,\omega) = \left| 1 - \omega \left(\frac{3}{2} M_0 + 1 \right) \right|
\end{align}
%
The choice of $\omega$ that minimizes both expressions corresponds to solving
$\ampI(\eta=0,\omega^*) = \ampI(\eta=1,\omega^*).$ It can be shown that
\begin{align}
\omega^* = \frac{4}{3 \Mra_0 + 4}, \quad \ampI^* = \frac{3 M_0}{3 M_0 + 4}.
\end{align}
%
This is a sensible result. The TP scheme suffers from added mass instability
for fine grids and light solids, which correspond to large acoustic mass ratios.
The under-relaxation parameter scales with $\Mra_0^{-1}$ to stabilize the added mass
effects. As a penalty, the amplification factor approaches $1$ for large $\Mra_0.$
To get a sense of computational cost for using TP iterations, we look at the number
of iterations needed for the relative error, $|e^{(k)}/e^{(0)}|,$ to converge to 
a desired tolerance, $\tau.$  It is easy to show that if $|A^*|^k < \tau,$ $k$ must 
satisfy
\begin{align}
k &> \frac{\log (\tau) }
{\log \left(\frac{3 M_0}{3 M_0 + 4} \right)} .
\end{align}
% 
We are interested in the asymptotic behavior for $\Mra_0 \gg 1.$ The denominator
of the above expression is asymptotically equivalent to
\begin{align}
\log \left(\frac{3 \Mra_0}{3 \Mra_0 + 4} \right) =
 \log \left(\frac{1}{1 + \frac{4}{3 \Mra_0} } \right)
\sim  \log \left(1 - \frac{4}{3 \Mra_0} + ... \right) 
\sim -\frac{4}{3 \Mra_0} + ...
\end{align}
%
Therefore 
\begin{align}
k > -\frac{3}{4} M_0 \log(\tau) = 
-\frac{3 }{4} \frac{\rho H }{ \bar{\rho} \bar{c} \Delta t} \log(\tau).
\end{align}
% 
The required number of iterations is proportional to $\dt^{-1}.$ 
For a viscous fluid simulation, the viscous terms can be treated as
implicitly or explicitly.
When an implicit solver is chosen, the time step will be proportional to
the grid spacing and the number of iterations will double when the grid is refined 
by a factor of $2$. 
When an explicit solver is chosen, the time step will be proportional to the 
square of the grid spacing and the number of iterations will quadruple when the grid
is refined by a factor of $2.$


% numerical results 



%%%%%%%%%%%%% old paper
% \subsection{Discretization}

% talk about fluid and solid discretization in x. 
% discrete fourier series on grid 
% % \wdh{We discretize the fluid and solid variables in the $x$~direction using a uniform
% % grid with spacing $\dx=L/(N_x+1)$. The grid points are given by $x_\ell=\ell\dx$,
% % $\ell=0,1,\ldots,N_x$.  The choice of discrete approximations to the
% % $x$~derivatives in the equations plays little role in the analysis.  Therefore, it is
% % convenient to use a pseudo-spectral approximation by expanding
% % each component $q$ of the solution $(\qv,\qsv)$ in a discrete Fourier series of
% % the form
% % % which gives a formally {\em exact} approximation,  $i\kx$, to an $x$-derivative.
% % % After discretizing in the $x$~direction we will expand the solution in a discrete Fourier series of the form
% % \begin{align}
% %    q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_\ell/L} \qHat_{k}(y,t), \qquad \ell=0,1,2,\ldots,N_x, \label{eq:discreteFourier}
% % \end{align}
% % where $q_\ell(y,t)\approx q(x_\ell,y,t)$ and $\qHat_{k}(y,t)$ are Fourier coefficients, 
% % and where $N_x$ is assumed to be even for convenience.
% % Transforming the governing equations to Fourier space leads to the following equations for the Fourier coefficients of the solution variables:
% % \begin{alignat}{3}
% % &   \rhos \partial_t \vs = i\kx \sigmas_{21} + \partial_y \sigmas_{22} , \quad&& y\in(0,\infty), \label{eq:vEqn} \\
% % &   \partial_t \sigmas_{22} = \rhos \cp^2 \partial_y\vs , \quad&&y\in(0,\infty), \label{eq:s22Eqn} \\
% % &   \partial_t \sigmas_{21} = i\kx \rhos \cp^2 \vs , \quad&&y\in(0,\infty) , \label{eq:s21Eqn} \\
% % & \rho \partial_t v_1 = i\kx      \sigma, \quad &&y\in(-H,0), \label{eq:v1HatEqn} \\
% % & \rho \partial_t v_2 = \partial_y\sigma, \quad && y\in(-H,0), \label{eq:v2HatEqn} \\
% % &  i\kx v_1 + \partial_y v_2 =0 ,                  \quad&&y\in(-H,0) , \label{eq:divHatEqn}
% % \end{alignat}
% % where $\kx = 2\pi k/L$ is a normalized wave number in the $x$~direction and the
% % equations hold for each $k=-N_x/2,-N_x/2+1,\ldots,N_x/2$. The hats on the
% % Fourier coefficients, along with the $k$ subscripts, have been dropped for
% % notational convenience.  Note that the horizontal component of the fluid
% % velocity, $v_1$, is decoupled from the other equations and boundary conditions, 
% % and can be determined once $v_2$ is known. Equations~\eqref{eq:v1HatEqn}--\eqref{eq:divHatEqn} are used to obtain
% % \[
% % \partial_y^2 \sigma - \kx^2 \sigma =0,      \qquad y\in(-H,0) ,
% % \]
% % which is a Laplace equation for pressure (in Fourier space).  The equations for the Fourier coefficients of the solid variables will be discretized using an upwind scheme.  In preparation for this, it is convenient to define the characteristic variables
% % \[
% % a=\sigmas_{22}-\rhos\cp\vs,\qquad b=\sigmas_{22}+\rhos\cp\vs,\qquad d=\sigmas_{21},
% % \]
% % which, from~\eqref{eq:vEqn}--\eqref{eq:s21Eqn}, satisfy
% % \begin{alignat}{3}
% % &   \partial_t a + \cp \partial_y a =  i\kx\cp\, d , \qquad&& y\in(0,\infty),  \label{eq:aHatEqnII}\\
% % &   \partial_t b - \cp \partial_y b = -i\kx\cp\, d , \qquad&& y\in(0,\infty),  \\
% % &   \partial_t d = \frac{i\kx\cp}{2}(b-a) , \qquad&& y\in(0,\infty).  \label{eq:dHatEqnII} 
% % \end{alignat}}
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% The solid variables are discretized in the $y$~direction using a uniform grid with
% spacing $\dy$.  The grid points for the solid domain are defined as $y_j=
% (j-\half)\dy$, $j=0,1,2,\ldots$. 
% Following the analysis in~\cite{BanksSjogreen2011,lrb2013}, the grid is staggered with respect to the
% interface at $y=0$ and has a ghost point at $j=0$; use of a non-staggered grid leads to similar results.
% %  This staggering simplifies the analysis but is not critical {\bf (I'm not convinced of this ?!?!)}.  
% Let  $\dt$ be the time step and let $t^n=n\dt$.  The
% equations~\eqref{eq:aHatEqnII}--\eqref{eq:dHatEqnII} are discretized using the
% first-order upwind scheme,
% \begin{alignat}{3}
% &   \frac{ a_j^{n+1}- a_j^n}{\dt} + \cp\frac{( a_j^n - a_{j-1}^n)}{\dy} =   i\kx\cp\, d_j^{n}, \label{eq:aEqnIII} \\
% &   \frac{ b_j^{n+1}- b_j^n}{\dt} - \cp\frac{( b_{j+1}^n - b_j^n)}{\dy} = - i\kx\cp\, d_j^{n}, \label{eq:bEqnIII} \\
% &   \frac{ d_j^{n+1}- d_j^n}{\dt} = \frac{i\kx\cp}{2}(b_j^{n+1} - a_j^{n+1}), \label{eq:dEqnIII}
% \end{alignat}
% where $a_j^{n}\approx a(y_j,t^n)$, $b_j^{n}\approx b(y_j,t^n)$ and
% $d_j^{n}\approx d(y_j,t^n)$. 
% Since we have used a non-dissipative pseudo-spectral approximation, rather than a two-dimensional upwind scheme, 
% the right-hand side terms in~\eqref{eq:dEqnIII} are taken at time $t^{n+1}$ in order to stabilize the approximation.
% A von Neumann stability analysis of equations~\eqref{eq:aEqnIII} and~\eqref{eq:bEqnIII} (for a
% periodic problem in $y$) shows that this time-stepping scheme is stable under
% reasonable conditions on the constants $\ly=\cp\dt/\dy$ and $\lx=\cp\kx\dt$.
% The fluid variables are kept continuous in $y$ in order to simplify the
% presentation; a discrete version can be introduced but this makes only
% insignificant changes to the fundamental results.  We are thus led to the
% following semi-discrete approximation for the solid and fluid equations,
% \begin{alignat}{3}
% &   a_j^{n+1} = a_j^n -\ly( a_j^n - a_{j-1}^n) - i \lx d_j^{n} , \quad&& j=1,2,3,\ldots\;, \label{eq:aEqn} \\
% &   b_j^{n+1} = b_j^n +\ly( b_{j+1}^n - b_j^n) + i \lx d_j^{n},  \quad&& j=0,1,2,\ldots\;, \label{eq:bEqn}  \\
% &   d_j^{n+1} = d_j^n +  \frac{i\lx}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=0,1,2,\ldots\;,  \\
% % 
% &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0), \\
% &  0=\partial_y^2 \sigma^{n+1}- \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), \label{eq:sigmaEqn}
% \end{alignat}
% where $v^n(y)=v(y,t^n)$ and $\sigma^n(y)=\sigma(y,t^n)$.  For reference, the discrete values for the (Fourier coefficients of the) velocity and components of stress in the solid are related to the characteristic variables by
% \[
% \vs_j^n=\frac{1}{2\zp}(b_j^n-a_j^n),\qquad\sigmas_{22,j}^n=\frac{1}{2}(b_j^n+a_j^n),\qquad \sigmas_{21,j}^n=d_j^n.
% \]
% The conditions at the top and bottom boundaries are 
% \begin{align}
% &   \vert a_j^{n}\vert^2 + \vert b_j^{n}\vert^2 + \vert d_j^{n}\vert^2 \rightarrow 0, 
%          \quad\text{as $j\rightarrow \infty$} ,  \label{eq:BCtop}\\
% &   \sigma^n(-H)=0. \label{eq:BCbottom}
% \end{align}
% Initial conditions are required to define $a_j^{0}$, $b_j^{0}$ and $d_j^{0}$ for $j=0,1,2,3,\ldots$, as well as $v^0(y)$ for  $y\in(-H,0)$, but these conditions are of no significance in the subsequent stability analysis.

% Approximations to the interface conditions are needed to complete the discrete
% formulation of the FSI model problem, and various choices are possible depending
% on the algorithm used.  
% For the AMP algorithm, the pressure Robin
% condition~\eqref{eq:AddedMassPressureBC} is imposed on the fluid; this is derived from the
% outgoing characteristic variables~\eqref{eq:AMPoutgoing}. In addition, the 
% incoming characteristic variable~\eqref{eq:AMPincoming} is used to specify a condition
% on the solid.  The latter condition uses an interface velocity defined
% in~\eqref{eq:ImpedenceWeightedVn} based on an impedance-weighted average.  
% First-order accurate approximations of these conditions are
% \begin{alignat}{3}
% &  \sigma^{n+1}(0) + \frac{\zp\dt}{\rho} \sigma_y^{n+1}(0) = \sigmas_{22,1}^{n+1} + \zp(\vs_1^{n+1} - v^{I,n})
%                                            = b_1^{n+1} -\zp v^{I,n}, && \label{eq:1dSigmaBC}\\
% &  a_0^{n+1} = \sigma^{I,n+1} - \zp v^{I,n+1}, &&\label{eq:1dSolidBC}
% \end{alignat}
% where $\sigma^{I,n}\equiv\sigma^n(0)$ and $v^{I,n}$ are the interface traction and velocity, respectively.  The latter is given by the impedance-weighted average
% \begin{alignat}{3}
% &   v^{I,n+1} = \frac{\zf}{\zf+\zp} v^{n+1}(0) + \frac{\zp}{\zf+\zp}\vs_1^{n+1} + \frac{1}{\zf+\zp}(\sigma_{22,1}^{n+1} - \sigma^{I,n+1} ) && \nonumber\\
% & \hphantom{v^{I,n+1}} = \gamma v^{n+1}(0) + \frac{1-\gamma}{\zp}( b_1^{n+1} - \sigma^{I,n+1} ), && \label{eq:1dVelocityBC}\end{alignat}
% where
% \[
% \gamma=\frac{\zf}{\zf+\zp},
% \]
% and where $\zf$ is a measure of the fluid impedance as introduced in Section~\ref{sec:partitionedAlgorithms}.

% The traditional partitioned (TP) algorithm uses the velocity from the solid as a boundary condition for the fluid and the traction from the fluid as a boundary condition for the solid.  First-order accurate approximations of these conditions are
% \begin{alignat}{3}
%  &   v^{n+1}(0)=\vs_1^{n+1}  
%         , &&   \label{eq:1dTradv} \\
%  &   \sigmas^{n+1}_{22,0} = \sigma^{n+1}(0). &&\label{eq:1dTradsigma}
% \end{alignat}
% It is also instructive to consider an anti-traditional algorithm in which
% the roles of the fluid and solid are reversed in the application of the
% partitioned interface conditions.  Approximations of these conditions are
% \begin{alignat}{3}
% &   \sigma^{n+1}(0) = \sigmas^{n+1}_{22,1}\,,  &&  \label{eq:1dAntiTradsigma} \\
% &   a_0^{n+1} = \sigma^{n+1}(0) - \zp v^{n+1}(0) .&& \label{eq:1dAntiTradv} 
% \end{alignat}
% The condition in~\eqref{eq:1dAntiTradv} is equivalent to setting the velocity of solid at the interface equal to the velocity in the fluid since the stresses have already been equilibrated in~\eqref{eq:1dAntiTradsigma}. 

% % 
% % 
% % % On the interface we assign the out-going characteristic variable by imposing~\eqref{eq:bEqn} at $j=0$.
% % The boundary conditions for the fluid are $\sigma^n(-H)=0$, while the solid solution should decay to zero 
% % as $j\rightarrow\infty$. 
% % The solution for $\sigma^n$ satisfying the boundary condition $\sigma^n(-H)=0$ can be written as
% % \begin{alignat}{3}
% % &  \sigma^{n}= \sigma^{I,n} \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \quad&& y\in(-H,0), 
% % \end{alignat}
% % where $\sigma^{I,n}=\sigma^n(0)$. 



% %- \vskip3\baselineskip
% %- 
% %- 
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- Let $\dt$ be the time step and let $t^n=n\dt$. 
% %- Introduce fully discrete approximations for the solid variables of the form $\qs_j^n \approx \qsHat(y_j,t^n)$ and
% %- semi-discrete approximations for the fluid variables of the form $q^n(y) \approx \qHat(y,t^n)$. 
% %- 
% %- This leads to the approximation
% %- \begin{alignat}{3}
% %- &   a_j^{n+1} = a_j^n -\lambda( a_j^n - a_{j-1}^n) - i \lambdax d_j^{n} , \quad&& j=1,2,3,\ldots \\
% %- &   b_j^{n+1} = b_j^n +\lambda( b_{j+1}^n - b_j^n) + i \lambdax d_j^{n},  \quad&& j=1,2,\ldots  \\
% %- &   d_j^{n+1} = d_j^n + i \frac{\lambdax}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=1,2,\ldots  \\
% %- % 
% %- &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0) \\
% %- &  \partial_y^2 \sigma^{n+1}= \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), 
% %- \end{alignat}
% %- where $\lambday=\frac{\cb\dt}{\dy}$ and $\lambdax=\cb\dt\kx$ and where $a_j^{n}$, $b_j^{n}$ and $d_j^n$
% %- are the characteristic variables in the solid given by 
% %- \begin{alignat}{3}
% %-    a_j^{n} = \sigmas_j^n -\zb \vs_j^n, \quad&& \vs_j^n &=\frac{1}{2\zb}(b_j^n-a_j^n), \\
% %-    b_j^{n} = \sigmas_j^n +\zb \vs_j^n, \quad&& \sigmas_j^n &=\frac{1}{2}(b_j^n+a_j^n), \\
% %-    d_j^n = \sigma^n_{21,j}
% %- \end{alignat}
% %- The boundary conditions for the fluid are $\sigma^n(-H)=0$, while for the solid the solution should remain bounded
% %- as $j\rightarrow\infty$. Initial conditions are needed for $a_j^{0}$, $b_j^{0}$, $d_j^{0}$, $j=0,1,2,3,\ldots$, 
% %- and $v^0(y)$, $y\in(-H,0)$.
% %- Approximations to the interface conditions are needed; various choices for these will be specified later. 
% %- 
% %- 
% %- 
% %- \vskip3\baselineskip
% %- 
% %- Introduce the fully discrete approximations $\vs_{ij}^n \approx \vs(x_i, y_j, t^n)$, 
% %- $\sigmas_{22,ij}^n \approx \sigmas^{22}(x_i, y_j, t^n)$, 
% %- $\sigmas_{21,ij}^n \approx \sigmas^{21}(x_i, y_j, t^n)$, 
% %- in the solid, 
% %- and the semi-discrete approximations $\vv_i^n(y)\approx \vv(x_i,y,t^n)$, $\sigma_i^n(y)\approx \sigma(x_i,y,t^n)$ in the fluid.
% %- We 
% %- expand the solution in a Fourier series in $x$,
% %- \begin{align}
% %-    \vs_{ij}^n = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat_{k,j}^n, \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}


% %- 
% %- 
% %- 
% %- We 
% %- expand the solution in a Fourier series in $x$. 
% %- We introduce the approximations $\vs_j(y,t) \approx \vs(x_j,y,t)$, $\sigma_{22,j}(y,t) \approx \sigmas_{22}(x_j,y,t)$, 
% %- $\sigma_{21,j}(y,t) \approx \sigmas_{21}(x_j,y,t)$, for the solid and 
% %- $\vv_j(y,t) \approx \vv(x_j,y,t)$, and $\sigma_{j}(y,t) \approx \sigma(x_j,y,t)$ for the fluid. 
% %- where 
% %- \begin{align}
% %-    \vs_j(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat(k,y,t), \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}
% %- We let $\kx = 2\pi k/L$ be the normalized wave number.
% %- 
% %- 
% %- 
% %- We discretize the solid in the $y$~direction with a grid spacing $\dy$.
% %- The grid for the solid is defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$. This grid is staggered
% %- with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- simplies the analysis but is not critical.
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- 
% %- % with grid spacing $\dy$ and use 
% %- % a first-order upwind scheme (in the $y$~direction) for the resulting solid equations. 
% %- % The grid for the solid, defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$, is staggered
% %- % with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- % simplies the analysis but is not critical.
% %- 
% %- In the solid we introduce grid functions $\vs_j^n\approx \vsHat(\kx,y_j,t^n)$, etc. 
% %- For the fluid we form approximations that are continuous in $y$ but discerete in time denoted by  
% %- $\sigma^n(y) \approx \sigmaHat(\kx,y,t^n)$,  and 
% %- $v^n(y) \approx \vHat_2(\kx,y,t^n)$. The horizontal component of the fluid velocity, $\vHat_1^n$, plays no role 
% %- in the analysis and can be determined from $v^n(y)$ using  $i\kx \vHat_1^n + \partial_y v^n(y)=0$, if needed.
% %- 
% %- 
% %- 


% % ------------------------------------------------------------------------------------------------
% \subsection{Stability analysis}

% \renewcommand{\aHat}{{\tilde a}}
% \renewcommand{\bHat}{{\tilde b}}
% \renewcommand{\dHat}{{\tilde d}}
% \renewcommand{\vHat}{{\tilde v}}
% \renewcommand{\sigmaHat}{{\tilde\sigma}}
% % \renewcommand{\aTilde}{{\bar a}}
% % \renewcommand{\bTilde}{{\bar b}}
% \renewcommand{\aTilde}{\alpha}
% \renewcommand{\bTilde}{\beta}

% To analyze the stability of the approximation
% in~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn}, we look for solutions of the form \[
% a_j^n=\amp^n\aHat_j, \qquad b_j^n=\amp^n\bHat_j, \qquad d_j^n=\amp^n\dHat_j,
% \qquad v^n(y)=\amp^n\vHat(y), \qquad \sigma^n(y)=\amp^n\sigmaHat(y),
% \] 
% where $\amp\in\Complex$ is the amplification factor,
% $(\aHat_j,\bHat_j,\dHat_j)$ are grid functions, and $(\vHat(y),\sigmaHat(y))$
% are functions for $y\in[-H,0]$. 
%  Substituting these forms
% into~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} results in the following system of
% equations
% \begin{alignat}{3}
% &  \amp \aHat_j = \aHat_j -\ly( \aHat_j - \aHat_{j-1}) - i \lx \dHat_j , \qquad&& j=1,2,3,\ldots\,, \label{eq:aHatEqn} \\
% &  \amp  \bHat_j = \bHat_j +\ly( \bHat_{j+1} - \bHat_j) + i \lx \dHat_j,  \qquad&& j=0,1,2,\ldots\,, \label{eq:bHatEqn}  \\
% &  \amp  \dHat_j = \dHat_j + \frac{i\lx}{2}\amp  ( \bHat_j - \aHat_j),    \qquad&& j=0,1,2,\ldots\,,  \label{eq:dHatEqn} \\
% % 
% &  \amp  \vHat(y) = \vHat(y) + \amp\dt\,\sigmaHat^I\,\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},  \qquad&& y\in[-H,0], \label{eq:vHatEqn} \\
% &  \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \qquad&& y\in[-H,0].\label{eq:sigmaHatEqn}
% \end{alignat}
% To obtain~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn},  the
% ODE in~\eqref{eq:sigmaEqn} was integrated using the boundary conditions $\sigmaHat(-H)=0$
% and $\sigmaHat(0)=\sigmaHat^I$, where the fluid stress at the interface, $\sigmaHat^I$, is as
% yet unspecified.  Note that the solution in the one-dimensional case,
% $\kk=0$, is a special case that can be found by taking the limit $\kk\rightarrow
% 0$ in~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn}. 
% Together with the interface
% conditions, equations~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} define
% a homogeneous set of difference equations. These equations have
% non-trivial solutions (i.e. eigenfunctions) only for particular values of $\amp$ (i.e. eigenvalues).
% The scheme is said to be weakly stable, or stable in the sense of
% Godunov-Ryabenkii, for given values of the parameters $\dt$, $\dy$, $\kx$, $H$, etc., 
% if there are no solutions (i.e.~eigenfunctions) to this
% eigenvalue problem with $\vert \amp\vert>1$. 
% The {\em region of stability} of the scheme is the region in parameter space where there are no roots with $\vert \amp\vert>1$. 
% In order to delineate the stability region 
% it is generally easier to look for regions where the scheme is {\em not} stable. Therefore, we 
% assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % we look for regions in the space of parameters where $\vert \amp\vert>1$  and the scheme is unstable.
% % We thus 
% % assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % If no such solutions exist for some given values of the parameters, then the scheme is (weakly) stable there. 
% % The stability domain is defined to be the region in parameter space where there are no roots with $\amp>1$.


% Equations~\eqref{eq:aHatEqn}--\eqref{eq:dHatEqn} are a system of
% constant-coefficient difference equations for the solid characteristic
% variables.  After solving for $\dHat_j$ from~\eqref{eq:dHatEqn} and substituting
% into~\eqref{eq:aHatEqn} and~\eqref{eq:bHatEqn}, $\aHat_j$ and
% $\bHat_j$ are found to satisfy the recursion
% \begin{equation}
%  \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = K \begin{bmatrix} \aHat_{j-1} \\ \bHat_{j-1} \end{bmatrix}, \qquad K =\begin{bmatrix}  ( 1 - \theta^2)/R & -\theta \\ \theta & R \end{bmatrix} ,
% \label{eq:recursion}
% \end{equation}
% where
% \begin{equation}
% R = r-\theta, \qquad r = \frac{\amp-1+\ly}{\ly}, \qquad \theta = -\frac{\amp\lx^2}{2\ly(\amp-1)} . 
% \label{eq:RandTheta}
% \end{equation}
% The eigenvalues, $\phi_-$ and $\phi_+$, of
% the $2\times2$ matrix $K$ in~\eqref{eq:recursion}
% %  \old{are the roots of a quadratic polynomial, and are given by} 
% are given by
% % \old{
% % We are interested in solutions for $\aHat_j$ and $\bHat_j$ that decay as
% % $j\rightarrow\infty$ so that the boundary condition in~\eqref{eq:BCtop} is
% % satisfied.  This leads us to consider the eigenvalues, $\phi_-$ and $\phi_+$, of
% % the $2\times2$ matrix $K$ in~\eqref{eq:recursion}, which are found by finding
% % the roots of a quadratic polynomial.  The result is
% % }
% \begin{equation}
% \phim = B - \sqrt{ B^2 - 1}, \qquad \phip=1/\phim, \qquad B = \frac{1}{2}\left(R + \frac{1 - \thetaj^2}{R}\right).
% \label{eq:phipm}
% \end{equation}
% Note that the product of the eigenvalues is one.  
% If both eigenvalues 
% % \old{were to have magnitude one} 
% had magnitude equal to one, then there would be no solution of the recursion
% in~\eqref{eq:recursion} satisfying the boundary condition~\eqref{eq:BCtop}.
% Therefore, for a valid solution, there is one eigenvalue (either $\phi_-$ or $\phi_+$),
% denoted by $\phis$ (for {\em small} $\phi$), that has magnitude strictly less
% than one, i.e.~$\vert\phis\vert<1$.  Let $\phib=1/\phis$ (for {\em big} $\phi$)
% be the other eigenvalue with $\vert\phib\vert>1$.  Note that when $\theta=0$,
% $0<\ly\le 1$, and $\vert\amp\vert>1$, then $\phis=\phim=1/r$ (but in general
% $\phis$ is not always equal to $\phim$).  Given that the eigenvalues are
% distinct, $K$ can be diagonalized as 
% \[
% K = S^{-1} \Phi S , \qquad
% \Phi =\begin{bmatrix}  \phis &  0 \\
%                            0 & \phib \end{bmatrix}, \qquad
% S =\begin{bmatrix}  R-\phis & \thetaj \\
%                     R-\phib & \theta \end{bmatrix}.
% \]
% By setting 
% \begin{align}
% &   \begin{bmatrix} \aTilde_j \\ \bTilde_j \end{bmatrix}
%    =  S \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = 
%    \begin{bmatrix} (R-\phis)\aHat_j + \theta \bHat_j \\
%                    (R-\phib)\aHat_j + \theta \bHat_j
%    \end{bmatrix}, \label{eq:abTildeEqn}
% \end{align}
% the general solution of the recursion in~\eqref{eq:recursion} is given by 
% \begin{equation}
% \begin{array}{l}
%    \aTilde_j = \phis^j \aTilde_0, \smallskip\\
%    \bTilde_j = \phib^j \bTilde_0.
% \end{array}
% \label{eq:abBarEqn}
% \end{equation}
% Since the solution must decay to zero as $j\rightarrow \infty$ and since $\vert\phib\vert>1$, it follows that $\bTilde_0=0$ and thus $\bTilde_j=0$ for all $j=0,1,2,\ldots$.  Since $\bTilde_j=0$, it follows from~\eqref{eq:abTildeEqn} that
% \begin{equation}
% \bHat_j = Q \aHat_j,\qquad \aTilde_j=(\phib-\phis)\aHat_j,\qquad Q = \frac{\phib-R}{\theta},
% \label{eq:Qdef}
% \end{equation}
% and thus from~\eqref{eq:abBarEqn}, 
% \[
% \aHat_j=\phi_s^j\aHat_0\,.
% \]
% Whence,
% % ------------------------------------------- PROP -------------------------------------------------
% \begin{proposition}
% Solutions to the system in~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} with $\vert\amp\vert>1$ satisfying the boundary conditions in~\eqref{eq:BCtop} and~\eqref{eq:BCbottom} are given by
% \[
% \begin{array}{c}
% \displaystyle{
% \aHat_j=\phi_s^j\aHat_0,\qquad \bHat_j=Q\aHat_j,\qquad \dHat_j=\frac{i\lx(Q-1)\amp}{2(\amp-1)}\aHat_j,\qquad j=0,1,2,\ldots\,,
% } \bigskip\\
% \displaystyle{
% \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},\qquad \vHat(y)=\sigmaHat^I\,\frac{\amp\dt}{\amp-1}\;\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},\qquad y\in[-H,0],
% }
% \end{array}
% \]
% % \old{where the two free constants, $\aHat_0$ and $\sigmaHat^I$, will be determined by two interface conditions.} 
% where $\aHat_0$ and $\sigmaHat^I$ are free constants.
% \end{proposition}

% The remaining constraints needed to complete the eigenvalue problem, which then determines the amplification factor $\amp$, are provided by two interface conditions.  Choices for these interface conditions are discussed in the subsections below.

% % \bigskip\noindent
% % \textcolor{green}{Note: I have chosen the wording above since the two interface conditions don't actually determine the two free constants, but rather they determine $\amp$ and a relationship between the constants.  I believe the constants would still be arbitrary to within a multiplicative constant.}

% % --------------------------------------------------------------------------------------------------------
% \subsection{AMP interface conditions} 
% Imposing the AMP interface conditions in~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC} with the formula for the interface velocity in~\eqref{eq:1dVelocityBC} gives
% % The AMP Robin boundary condition for $\sigma$ is~\eqref{eq:1dSigmaBC} which gives
% % follows from~\eqref{eq:AddedMassPressureBC}.
% % A first-order approximation is 
% % \begin{align}
% %   \sigma^{n+1} + \frac{\zb\dt}{\rho} \sigma_y^{n+1} &= \sigmas_{22,1}^{n+1} + \zb\vs_1^{n+1} - \zb v^{I,n}
% %                                            = b_1^{n+1} -\zb v^{I,n}, \qquad\text{for $y=0$}, \label{eq:1dSigmaBC}
% % \end{align}
% % where we have introduced the interface velocity $v^{I,n}$.
% % This gives,
% % \begin{align}
% % &  \sigma^{I,n+1} = \eta\Big( b_1^{n+1} - \zb v^{I,n}\Big), \\
% % & v^{I,n+1}  = \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \\
% % &  a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}, 
% % \end{align}
% \begin{align}
% &  \amp\sigmaHat^{I} = \eta\left( \amp\bHat_1 - \zp \vHat^{I}\right), \label{eq:AmpSigmaHat} \\
% &  \aHat_0 = \sigmaHat^{I} - \zp \vHat^{I} , \label{eq:AmpaHat} \\
% &  \vHat^{I}  = \gamma \vHat(0) + \frac{1-\gamma}{\zp}( \bHat_1 - \sigmaHat^{I} ), \label{eq:AmpvHatI}
% \end{align}
% where
% \begin{align*}
%  & \eta \equiv \frac{1}{1 + \frac{\zp\kk\dt}{\rho}\coth(\kk H)}  = \frac{1}{1 + \frac{\rhos\lx}{\rho}\coth(\kk H)}. 
% \end{align*}
% From~\eqref{eq:vHatEqn} and~\eqref{eq:AmpSigmaHat} we also have
% \begin{align}
%   (\amp-1) \vHat(0) = \frac{1-\eta}{\zb}(\amp \bHat_1 - \zb\vHat^I). \label{eq:AmpvHat} 
% \end{align}
% Using $\bHat_1=Q\phis \aHat_0$ to eliminate $\bHat_1$ in terms of $\aHat_0$ and using~\eqref{eq:AmpSigmaHat} to
% eliminate $\sigmaHat^{I}$, equations~\eqref{eq:AmpaHat}, \eqref{eq:AmpvHat} and~\eqref{eq:AmpvHatI} can be written
% in the form 
% %- The interface velocity follows from~\eqref{eq:1dVelocityBC}, giving 
% %- \begin{align}
% %- %    v^{I,n+1} &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( \zb\vs_1^{n+1} + \sigma_{22,1}^{n+1} - \sigma^{I,n+1} ), \\
% %- v^{I,n+1}   &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \label{eq:1dVelocityBCb}
% %- \end{align}
% %- where $\gamma=\zf/(\zf+\zb)$.
% %- For the final interface condition we set the incoming characteristic variable in the solid using the interface
% %- stress and velocity, 
% %- \begin{align}
% %-   a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}. \label{eq:1dSolidBCb}
% %- \end{align}
% % addedMass.mample : 
% % M := Matrix( [ [ A*(1-eta*Q*phim) , 0   , eta+A] , 
% %                [ (1-eta)*A*Q*phim , 1-A , -(1-eta) ], 
% %                [ -(1-g)*(1-eta)*Q*phim    , -g   , 1-(1-g)*eta/A ] ] );
% %
% %-The equations defining the AMP approximation can thus be written in the form
% \begin{align}
% \begin{bmatrix}
%    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
%    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
%   -(1-\gamma)(1-\eta)Q\phis  & -\gamma &  1-(1-\gamma)\eta \amp^{-1} 
% \end{bmatrix} 
% \begin{bmatrix} \aHat_0 \\ \zb \vHat(0) \\ \zb\vHat^I \end{bmatrix} =0 .  \label{eq:AMPmatrix}
% \end{align}
% The determinant of the matrix in~\eqref{eq:AMPmatrix} must be zero for non-trivial solutions to exist, and this leads to the following equation for $\amp$:
% \begin{align*}
% %    \tilde{f(\amp) :=& 
%    \big(\amp-(1-\gamma)\big) \left(\amp-\eta - \big( (2\eta-1)\amp -\eta \big)Q \phis\right) =0.
% \end{align*}
% % For $0\le \gamma\le 2$ the root $A=1-\gamma$ has magnitude less than or equal to one.
% Since $\amp-(1-\gamma)\ne0$ when $\vert\amp\vert>1$ and $0\le \gamma\le 2$, we have the following result.
% % --------------------------------------------------------------------------------------------------
% \begin{theorem} \label{th:amp1d}
% The AMP interface approximation to the
% scheme~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary
% conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, interface
% conditions~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC}, and interface
% velocity~\eqref{eq:1dVelocityBC} is weakly stable if and only if $0\le \gamma\le 2$ and there are no roots $\amp$ with $\vert \amp\vert>1$ to the equation
% \begin{align}
%    f(\amp) \equiv& \amp -\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis =0. \label{eq:fAMP}
% \end{align}
% \end{theorem}
% \noindent Note that $f(\amp)$ does not depend on $\gamma$, i.e.~the weighting in the definition of the interface velocity, and thus the stability of the scheme is independent of $\gamma$ provided $0\le \gamma\le 2$.  From a numerical conditioning point of view, however, we recommend the choice $\gamma=\zf/(\zf+\zp)$ as used in~\eqref{eq:1dVelocityBC}.


% %
% %- 
% %- \begin{align}
% %- &  A \sigma^{I} = \eta\Big( A \bHat_1 - \zb v^{I}\Big), \label{eq:AddedMassSigmaI} \\
% %- % &  \aHat_0 = \sigmasHat_0 - \zb \vsHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- &  \aHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- & (A-1)\vHat(0)= \frac{1-\eta}{\eta\zb} A \sigma^{I}, \\
% %- & v^{I} = \gamma \vHat(0) + (1-\gamma)\frac{1}{\zb}( \bHat_1 - \sigma^{I} )
% %- % &  b^{I,n+1}= b_1^{n+1},  ~~\text{(first order approximations)}, 
% %- \end{align}
% %- Using the expressions for $b_1^n$, etc. 
% %- lead to the conditions
% %- \begin{align}
% %- &  A(1-\eta Q\phis)\aHat_0 + (\eta+A) (\zb\vHat^I) =0 ,   \\
% %- & (A-1)(\zb\vHat(0)) -(1-\eta) A Q \phis \aHat_0 + (1-\eta) (\zb \vHat^I) = 0, \\
% %- & (1 - (1-\gamma)\eta A^{-1}) (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(1-\eta) Q \phis\aHat_0 = 0. 
% %- % & (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(Q-1)\half\phis \aHat_0=0. 
% %- \end{align}
% %- This is an eigenvalue problem for $\amp$. 
% %- Taking the determinant of the associated matrix leads to 
% %- \begin{align}
% %- & f(\amp) \equiv
% %- \det
% %- \begin{bmatrix}
% %-    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
% %-    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
% %-    \half(1-\gamma)(Q-1) \phis  & \gamma & -1 
% %- \end{bmatrix} =0,\\
% %- & f(\amp)=  \amp(1-\eta Q\phis) \Big( 1-\amp +\gamma(1-\eta)\Big) + 
% %-          (\amp+\eta)\phis\Big(  \gamma(1-\eta)\amp Q - \half(1-\amp)(1-\gamma)(Q-1)   \Big) .
% %- \end{align}
% %-The scheme is unstable if there are solutions to $f(\amp)=0$ with $\vert\amp\vert>1$. 
% %-The scheme is said to be (weakly stable) at particular values of $\lambdax,\lambday,\gamma$
% %-if there are no roots with $\vert\amp\vert>1$. Given a choice for $\gamma$ we can plot the
% %-region of stability in the $(\lambdax,\lambday)$ plane. 


% \paragraph{Reduction to a polynomial equation for $\amp$} To examine the stability of the AMP algorithm we must consider all solutions of $f(\amp)=0$.  The function $f(\amp)$ in~\eqref{eq:fAMP} involves square roots of $\amp$ through the eigenvalues, $\phis$ and $\phib$, of the matrix $K$ in~\eqref{eq:recursion} and the definition of $Q$ in~\eqref{eq:Qdef}.  
% To ensure that all possible solutions are found, 
% a polynomial $P(\amp)$ can be derived whose roots include
% all the roots of $f(\amp)$.  To this end, 
% note that from the definition for $Q$ and $\phis\phib=1$ it follows that 
% \begin{align*}
%   Q\phis = \frac{1-R\phis}{\theta}.
% \end{align*}
% Thus $f$ is a linear function of $\phis$ since $f$ only depends on the product $Q\phis$. 
% Note 
% also that $Q\phis$ is a rational function of $\amp$ according the definitions of $R$ and $\theta$ in~\eqref{eq:RandTheta}.  
% Thus, $f(\amp)=0$ can be written in the form
% \begin{align*}
%     \phis = F(\amp) ,
% \end{align*}
% where $F$ is a rational function of $\amp$. 
% Since $\phis$ is equal to one of the two eigenvalues, $\phi_\pm$, defined in~\eqref{eq:phipm}, it follows that 
% \begin{equation}
%   \pm \sqrt{ B^2 - 1} = F(\amp)-B,
% \label{eq:Fratio}
% \end{equation}
% where the sign in front of the square root is chosen to be consistent with $\vert\phis\vert<1$.
% % \old{where the sign in front of the square root is chosen based on the assignment of $\phis$ so that $\vert\phis\vert<1$.}
% Upon squaring both sides of~\eqref{eq:Fratio}, which introduces new roots, one obtains
% %  
% %  Since $\phis$ also satisfies a quadradic equation
% %  with coefficients that are polynomials of $A$, 
% %  \begin{align}
% %   (\amp-1)^2 R \phis^2 - (\amp-1)^2 R B \phis + (\amp-1)^2 R=0,
% %  \end{align}
% % we can eliminate $\phis$ to derive a higher degree polynomial satisfied by $A$,
% \begin{equation}
%    P(\amp)=0,
% \label{eq:PAMP}
% \end{equation}
% where $P(\amp)$ is a polynomial (as described below).  We have thus shown the following:
% \begin{proposition}
%   Any solution of $f(\amp)=0$ is also a root of the polynomial $P(\amp)$. 
% \end{proposition}
% All of the roots of $P(\amp)$ can be found numerically using well-developed
% algorithms (e.g.~solving the eigenvalue problem for the companion matrix).  
% In
% deriving $P(\amp)$, however, new roots have been introduced. Therefore, each
% root $\amp^*$ of $P(\amp)$ must be checked to ensure that it is also solution of
% $f(\amp)=0$.
% % To do this we set $\phis=\phi_-(\amp_0)$ if $\vert\phi_-(\amp_0)\vert<1 $ otherwise we set $\phis=\phi_+(\amp_0)$,
% % and then check that $f(\amp_0)=0$. 
% \begin{proposition}
%   A root, $\amp^*$, of $P(\amp)$ is also a root of $f(\amp)$, if $\phis$ in the definition of $f$ satisfies
% \begin{equation*}
%     \phis = \begin{cases}
%                 \phi_-(\amp^*) & \text{if $\vert\phi_-(\amp^*)\vert<1 $}, \\
%                 \phi_+(\amp^*) & \text{otherwise} ,
%             \end{cases}
% \end{equation*}
% and if $f(\amp^*)=0$.
% \end{proposition}
% % \begin{align}
% %    P(\amp)=0, \quad f(\amp)=0, \quad \vert\phis(\amp)\vert<1. 
% % \end{align}
% % {\bf Scheme 1:} Taking $\gamma=1$ (interface velocity from the fluid), gives (removing a factor of $2\amp$)
% % ff := phim Q A - eta - 2 eta Q phim A + eta Q phim + A
% % 
% \newcommand{\Pamp}{P_{\rm AMP}}
% The polynomial in~\eqref{eq:PAMP} is (after removing uninteresting factors of $\amp-1$) a polynomial of degree 5 given by 
% \[
% \Pamp(\amp)=\alpha_5\amp^5+\alpha_4\amp^4+\alpha_3\amp^3+\alpha_2\amp^2+\alpha_1\amp+\alpha_0,
% \]
% where the coefficients in the polynomial are
% \[
% \begin{array}{l}
% \alpha_0=-\eta^2+2 \eta^2 \ly, \smallskip\\
% \alpha_1=-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2, \smallskip\\
% \alpha_2=10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly, \smallskip\\
% \alpha_3=-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2, \smallskip\\
% \alpha_4=3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2, \smallskip\\
% \alpha_5=-1+2 \eta.
% \end{array}
% \]
% %\begin{align*}
% %%  f_1(\amp) :=&  A-\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis, \\
% % \Pamp(\amp) =&  (-1+2 \eta) A^5+(3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2) A^4+\\
% %&    (-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2) A^3+\\
% %&    (10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly) A^2+(-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2) A\\
% %&    -\eta^2+2 \eta^2 \ly .
% %\end{align*}
% It turns out that $\Pamp(\amp)$ is the same polynomial generated by the Maple symbolic algebra program when asked to solve $f(\amp)=0$.

% To determine if there are any roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$, we
% evaluate the roots numerically for an array of parameter values in the region
% $0<\lx<1.2$, $0<\ly<1.2$ and $0\le \eta \le 1$ with $N_\amp$ equally spaced
% points in each parameter direction.  The stability region of the scheme is the
% region in the space of $(\lx,\ly,\eta)$ where the magnitude of the largest
% valid root satisfies $\vert\amp\vert\le 1$.  This region is computed on a grid with
% $N_\amp=800$ points for each parameter.  In
% Figure~\ref{fig:acousticSolidStokestability}, we plot the curve in the
% $(\lx,\ly)$ plane for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  (The
% curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is also plotted for
% reference.)  Observe that the region of stability contains the region
% $0\le\eta\le1$ and $\lx^2 + \ly^2 \le \kappa^2$
% (for $\lx\ge0$ and $\ly\ge 0$) where the maximum value for $\kappa$ appears to be $\kappa=1$. 
% Further evidence for $\kappa=1$ being the upper bound is provided by the restriction of the analysis to one dimension given below.
% % \old{, where $\kappa$ is a positive constant strictly less than 1.  }
% The curve $\lx^2 + \ly^2 = (.99)^2$
% is shown in the figure as an example.  Since $\lx=\cp\kx\dt$ and $\ly=\cp\dt/\dy$,
% the condition $\lx^2+\ly^2\le 1$ implies the following result.

% % To determine if there are any roots of $\Pamp(\amp)=0$ with $\vert\amp\vert>1$ we evaluate the roots numerically for 
% % values of $\lambda$, $\lambdax$ and $\eta$ in the ranges $0<\lambda<1$, $0<\lambdax<1$, and $0\le \eta \le 1$.
% % We choose $M$ equally spaced values of each of $\lambda$, $\lambdax$ and $\eta$ over their ranges, resulting
% % in finding the roots for $M^3$ points. Using Maple we computed roots with $M=50$ and $M=100$ and using $20$ digits of precision.
% \begin{theorem}
% By numerical evaluation of the stability polynomial, $\Pamp(\amp)$,
% we have found that the AMP algorithm is weakly stable (i.e.~there are no valid roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$) 
% provided $\lx^2+\ly^2\le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{1}{\cp}\left[ \frac{1}{\dy^2} + \kx^2 \right]^{-1/2}. 
%  \end{align*}
% % where $0\le\kappa<1$. 
% This is a sufficient but not a necessary condition. 
% \end{theorem}
% Note that the time step $\dt$ satisfies a typical CFL constraint arising from the fastest wave speed in the solid.
% In the incompressible limit when $\cp \rightarrow \infty$, the maximum stable $\dt$ would go to zero,
% as it would for the solid in isolation. For incompressible solids, alternative formulations should be considered.
% Developing AMP algorithms for incompressible solids is a subject for future work. 

% % \noindent{\bf Note 1:} There are generally four valid roots to $\Pamp(\amp)=0$.
% % Figure~\ref{fig:acousticSolidStokestability} shows a plot of the computed stability region.

% {
% % ---- from codes/cauchy.m  (and cauchy.maple) ----
% \newcommand{\figWidth}{8cm}
% \begin{figure}
% \begin{center}
% %   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP_num50}
%   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP}
%   \caption{Stability region for the two-dimensional model problem using the AMP algorithm.  The curve marked 1 is the curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  The curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is shown for reference.  The dashed curve shows the curve $\lx^2+\ly^2=(.99)^2$.}
%   \label{fig:acousticSolidStokestability}
% \end{center}
% \end{figure}
% }


% % \noindent{\bf Note 2:} The scheme is found to be unstable for $\lambda>1$. Note, however, that the stability bound
% % derived in Section~\ref{} for a periodic strip in $y$ is somewhat more restrictive than the bound found here
% % for the seimi-infinite strip. For example, the periodic strip is unstable for $(\lambda,\lambdax)=(.9,9.)$.

% % {\bf TO-DO: Check the $\eta=0$ limit -- decoupled solid -- we should get von-Neumann stability bound.}

% % --------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% The stability of the one-dimensional version of the AMP algorithm 
% % \old{(described previously in Section~{\bf ?????})}
% may be examined by considering the special case of the two-dimensional algorithm with $\lx=0$ and $Q=0$.  In this case there are two solutions of $f(\amp)=0$ given by
% \begin{align*}
%    \amp = 1-2\ly \qquad\text{or}\qquad \amp =\eta. % \label{eq:fAMP1D}
% \end{align*}
% We are interested in whether there are solutions with $\vert\amp\vert>1$.  Since $0\le \eta\le 1$ we have the result.
% \begin{theorem}
% The one-dimensional AMP algorithm is weakly stable provided  $0\le\gamma\le 2$ and $0 \le \ly \le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{\dy}{\cp}. 
%  \end{align*}
% \end{theorem}

% % \noindent{\bf Note 2:} Even though there are no roots $\vert\amp\vert>1$ to $\Pamp$ for even larger values of $\lambda$ and $\lambdax$,
% %   the orginial scheme should respect the time step restriction from the solid scheme 
% % {\bf But why? Does some assumption go bad? e.g. $\vert\phis\vert<1$?}


% For comparison, we now discuss briefly the corresponding stability results for the scheme given by~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, and with interface conditions given by either the 
% traditional (TP) algorithm or the anti-traditional algorithm.



% % ==========================================================================================================
% \subsection{TP interface conditions} \label{sec:TPanalysis}
% % \newcommand{\Mr}{\Mc}% mass ratio

% The interface conditions for the TP algorithm are given by~\eqref{eq:1dTradv} and~\eqref{eq:1dTradsigma}.  
% Following the previous analysis, $\amp$ is found to satisfy 
% \begin{align}
% &   f_{{\rm TP}}(\amp) \equiv \amp(Q+1) - \frac{\eta-1}{\eta} (\amp-1)(Q-1)\phis =0 . \label{eq:traditionalSchemeF}
% % &   \mr \equiv \frac{\zb\dt\kx}{\rho\tanh(\kx H)} = \frac{\eta-1}{\eta} ...
% \end{align}

% % {\bf TO-DO} The stability region for this scheme is computed numerically and shown in Fig.~\ref{??}.
% % We could plot the stability regions for fixed values of $\eta$ and show that as $\eta\rightarrow 1$ the
% % stability region shrinks to nothing. This shows that as $\dt\rightarrow 0$ ($\eta\rightarrow 1$) the
% % scheme is unstable. 


% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 

% In one dimension, the condition in~\eqref{eq:traditionalSchemeF} reduces to the polynomial equation
% \begin{align*}
% P_{{\rm TP}}(\amp) = \amp^2 + (\Mr + \ly-1) \amp - \Mr = 0, \quad\text{where}~~
%   \Mr = \frac{\rho H}{\rhos \dy}.
% \end{align*}
% (Here, all of the roots of this quadratic are valid since no spurious roots were introduced in deriving the equation.)  The product of the roots is $-\Mr$ and thus a necessary condition for stability is that $\vert \Mr\vert\le 1$.
% Thus the mass of the solid in a thin strip one grid cell wide, $\rhos\dy L$, 
% must be larger than the mass of the entire fluid domain $\rho H L$. 
% Using the theory of von Neumann polynomials~\cite{Miller1971,Strikwerda89} one can show the following necessary and
% sufficient condition.  
% % {\bf (It is a little unclear to me how $\Delta y$ appears.) WDH: Multiply the expression below with $\cp/\dy$ and $\lambda$ and $\Mr$ appear. }
% % ---------------------------------- THEOREM -------------------------------------------------
% \begin{theorem} \label{lemma:traditional}
% The one-dimensional TP algorithm is weakly stable if and only if 
% \begin{align*}
% %      \Mr = \frac{\rho H}{\rhos \dy} <1, \\
%      \dt \le \frac{2}{\cp}\Big( \dy - \frac{\rho H}{\rhos} \Big). 
% %      \lambda < 2(1-\Mr). 
% \end{align*}
% \end{theorem}
% This is a curious result.  For a given {\em large} value of $\dy$ the one-dimensional scheme may be stable, but it will eventually become unstable as the mesh is refined and $\dy$ becomes less than $(\rho H)/\rhos$.  The one-dimensional TP algorithm is thus formally {\em unconditionally unstable}.  
% The numerical results in Section~\ref{sec:travelingWaveResults} show that this behaviour also holds for 
% the second-order accurate discretization of the two-dimensional model problem MP-VE.
% % This behaviour of the traditional scheme is also found to hold in the two-dimensional
% %  since as the mesh is refined eventually $\dy$ will be less than $\frac{\rho H}{\rhos}$. 


% % --------------------------------------------------------------------------------------------------------
% \subsection{Anti-traditional interface conditions} \label{sec:ATPanalysis}

% The interface conditions for the anti-traditional algorithm are given by~\eqref{eq:1dAntiTradsigma} and~\eqref{eq:1dAntiTradv}.  The analysis for this choice leads to the constraint
% %These can be written as 
% %\begin{align*}
% %&  \sigmaHat^I = \sigmasHat_{22,1}= \half(Q+1)\phis\aHat_0, \\
% %&  \aHat_0 = \sigmaHat^I -\zb\Big( \frac{\kk\dt}{\rho}\coth(\kk H)\frac{\amp}{\amp-1} \Big)\sigmaHat^I, 
% %\end{align*}
% % The anti-traditional scheme takes the interface velocity from the fluid and the interface
% % stress from the solid,
% % \begin{align}
% % &   \vHat^I = \vHat(0) = \frac{1-\eta}{\eta}\frac{1}{\zb} \frac{\amp}{\amp-1} \sigmaHat^I, \\
% % &   \sigmaHat^I = \sigmasHat_1 = \half(Q+1) \aHat_0, \\
% % &   \aHat_0 = \sigmaHat^I - \zb \vHat^I = (1- \frac{1-\eta}{\eta}\frac{\amp}{\amp-1}) \half(Q+1) \aHat_0.
% % \end{align}
% % ese interface conditions lead to the eigenvalue equation for $\amp$ of 
% %which leads to the eigenvalue equation for $\amp$ of 
% \begin{align}
% &   f_{{\rm AT}}(\amp) = 1- \amp + \half\left( \frac{2\eta-1}{\eta} \amp -1 \right) (Q+1)\phis=0 .  \label{eq:antiTraditional2d}
% \end{align}

% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% In one dimension, \eqref{eq:antiTraditional2d} reduces to the polynomial constraint
% \begin{align*}
% %      \amp^2 + ( \frac{\lambda}{2\eta} -2)\amp + 1-\frac{\lambda}{2} = 0.  \\
%      P_{{\rm AT}}(\amp) = \amp^2 + \left( \frac{\ly}{2}\left(1+\frac{\ly}{\Mr}\right) -2\right)\amp + 1-\frac{\ly}{2} = 0.  
% %     \amp^2 + (  \frac{\lambda}{2} + \frac{\lambda^2}{2\Mr} -2)\amp + 1-\frac{\lambda}{2} = 0. 
% \end{align*}
% % The anti-traditional scheme is weakly stable in one-dimension if and only if the following conditions
% %  are satisfied (**CHECK ME**)
% %  \begin{align}
% %  &    \lambda < 4, \\
% %  &    \frac{\lambda^2}{2\Mr} < 4-\lambda. 
% %  \end{align}
% %  where $\Mr = \frac{\rho H}{\rhos \dy}$. {\bf TO-DO:} $\Mr$ depends on $\dy$ so we really need to find the condition on $\dt$ in terms of $\dy$.
% An analysis of the roots of $P_{{\rm AT}}(\amp)$ leads us to the following result:
% \begin{theorem}
%   The one-dimensional anti-traditional algorithm is weakly stable if and only if $\ly\le 4$ and 
% % \begin{align}
% % %    \lambda \le \sqrt{ 8\Mr + \Mr^2  } -       \Mr     =       \Mr     \Big( \sqrt{ 1+\frac{8 }{\Mr}} -1 \Big). \\
% %     \half G \dt^2 + \dt < \frac{4\dy}{\cb}, \qquad G=\frac{\rhos\cb}{\rho H}
% % \end{align}
% % or 
% \begin{align}
% %    \dt  < \frac{ \sqrt{1+\frac{8\rhos}{\rho H} \dy} -1 }{G}, \qquad G=\frac{\rhos\cb}{\rho H} . \\
%    \dt  \le \frac{\dy}{\cp}\left( \sqrt{\Mr^2+8\Mr}-\Mr \right).   \label{eq:ATStability}
% \end{align}
% \end{theorem}

% We observe that the one-dimensional anti-traditional scheme is (weakly) stable for any value of the added-mass ratio $\Mr=(\rho H)/(\rhos \dy)$ provided that $\dt$ is taken sufficiently small. 
% The anti-traditional scheme is thus a stable alternative to the AMP scheme. However, in the {\em heavy solid} regime 
% when $\Mr$ is small, the anti-traditional requires a smaller $\dt$ than the AMP scheme, scaling
% like $\sqrt{8\Mr}$ for $\Mr\ll 1$,  as can be seen from~\eqref{eq:ATStability}.



==> texFiles/backup/algorithm.tex <==
\section{Algorithm} \label{sec:algorithm}


==> texFiles/backup/analysis.tex <==
\section{Analysis of a two-dimensional acoustic solid and an inviscid incompressible fluid} \label{sec:analysis}

% todo
%
% replace \lambda_y with \ly etc.
%

\input texFiles/rectangularModelProblemCartoon

% \wdh{\bf This is from fib:
% In this section, we perform a stability analysis of the AMP algorithm applied to
% the two-dimensional FSI model problem MP-IA.  In this problem, the fluid is
% taken as inviscid and the solid is treated as an acoustic solid that only
% supports motion in the vertical direction. The governing equations for the model
% are given by~\eqref{eq:MP-IA}.
% % We are interested in the stability of different frequencies in the $x$ direction and thus consider a periodic problem in $x$. 
% We consider a semi-infinite solid domain ($\Hs=\infty$) and look for solutions in the solid that have finite $L_2$-norm (which implies the solutions decay to zero as $y\rightarrow\infty$).  The bottom boundary condition on the fluid at $y=-H$ is chosen as $\sigma=0$ (i.e. $p=0$).
% }

In this section, the stability of the second order accurate
AMP, TP, and ATP algorithms are explored for the two-dimensional 
FSI model problem MP-IA. This extends the stability results of first order 
accurate schemes by Banks, Henshaw, and Schwendeman \cite{fib2014}.
In this analysis, the TP scheme is considered 
without under-relaxed sub-iterations. 
To supplement this, an analysis on the TP scheme with sub-iterations is performed.
In the model problem, we assume the fluid is inviscid and the solid 
is acoustic with motion constrained to vertical direction. 
We are interested in the stability of different frequencies 
in the $x$ direction and thus consider a periodic problem in $x$. 
The solid domain is semi-infinite ($\Hs \rightarrow \infty)$ and we require solutions
to decay to zero as $y \rightarrow -\infty.$ The fluid pressure is given to be 
$p=0$ at the top boundary. The interface conditions enforces matching of the 
velocity and traction at $y=0.$
The governing equations and boundary conditions are given by
\begin{align}
\text{Fluid: } &\begin{cases}
\rho \partial_t \vfy + \partial_y p = 0, & \xv\in\OmegaF \\
(\partial_x^2 + \partial_y^2) p =0, & \xv\in\OmegaF \\
p = 0, & x\in(0,L), \quad y=H
\end{cases} \\
\text{Solid: } &\begin{cases}
\rhos \partial_t \vsy = \partial_x \ssx + \partial_y \ssy, & \xv\in\OmegaS \\
\partial_t \ssx = \rhos\cp^2 \partial_x \vsy, & \xv\in\OmegaS \\
\partial_t \ssy = \rhos\cp^2 \partial_y \vsy, & \xv\in\OmegaS \\
|\vsy|^2+|\ssx|^2+|\ssy|^2 \rightarrow 0, & y\rightarrow - \infty
\end{cases} \\
\text{Interface: } &\begin{cases}
\vfy = \vsy, & x\in(0,L), \quad y = 0 \\
p = -\ssy, & x\in(0,L), \quad y = 0.
\end{cases}
\end{align}

% governing equations
% ------------------------------------------------------------------------------------------------
\subsection{Discretization}

The fluid and the solid are discretized in the $x$ direction by a uniform grid defined by
grid spacing $\dx = L/N_x$ and grid points $x_l = l \Delta x$ for 
$\ell = 0, 1,\ldots N_x.$ 
Since the problem is periodic in the $x$ direction, each
variable can be represented as a discrete Fourier series, e.g.
\begin{align}
q_l(y,t) = \sum_{k=-N_x/2}^{N_x/2-1}  e^{2 \pi i k x_l/ L} \hat{q}_k (y,t), 
\qquad \ell=0,1,2,\ldots,N_x. \label{eq:discreteFourier}
\end{align}
%
Here, $q_l(y,t) \approx q(x_l,y,t)$ and $\hat{q}_k$ are Fourier coefficients.
For convenience, $N_x$ is assumed to be an even integer. Let
$k_x = 2 \pi k /L$ be the normalized wave number for each 
$k = -N_x/2,-N_x/2+1, \ldots, N_x/2-1.$ The governing equations are now transformed
to obtain equations for the Fourier coefficients. The equations for the fluid become
\begin{alignat}{2}
\rho \partial_t \vfyh + \partial_y \ph &= 0, \quad && y\in(0,H) \\
\partial_y^2 \ph - k_x^2 \ph &=0, \quad && y\in(0,H).
\end{alignat}
%
% todo, we dropped the subscript k for the fourier coefficients. explain this?
The transformed equations for the solid are
\begin{alignat}{2}
\rhos \partial_t \vsyh &= i k_x \ssxh + \partial_y \ssyh, \quad && y\in(-\infty,0) ,
\label{eq:vsyhEqn} \\
\partial_t \ssxh &= i k_x \rhos\cp^2 \vsyh, && y\in(-\infty,0), 
\label{eq:ssxhEqn} \\
\partial_t \ssyh &= \rhos\cp^2 \partial_y \vsyh, && y\in(-\infty,0)
\label{eq:ssyhEqn}.
\end{alignat}
%
It is convenient to consider the solid equations in characteristic form. 
Equations \eqref{eq:vsyhEqn}--\eqref{eq:ssyhEqn} are diagonalized to derive the
following characteristic variables
\begin{align}
\ac = \ssyh - \rhos\cp\vsyh, \quad
\bc = \ssyh + \rhos\cp\vsyh, \quad
\dc = \ssxh,
\end{align}
%
which satisfy
\begin{alignat}{2}
\partial_t \ac + \cp \partial_y \ac &= i k_x \cp \dc, \quad && y\in(-\infty,0), 
\label{eq:advSrcA} \\
\partial_t \bc - \cp \partial_y \bc &= -i k_x \cp \dc, \quad && y\in(-\infty,0),
\label{eq:advSrcB} \\
\partial_t \dc &= \frac{i k_x \cp}{2} (\bc - \ac), \quad && y\in(-\infty,0). 
\label{eq:SrcD}
\end{alignat}
%
This is a system of advection equations with a source. $\ac$ corresponds to the
$\cp^+$ characteristic and $\bc$ corresponds to the $\cp^-$ characteristic.

The solid characteristic variables are discretized in the $y$ direction using a
uniform collocated grid with grid spacing $\dy$ and grid points
$y_j = j\dy,$ for $j = 1, 0, -1, -2 \ldots$. 
Although staggered grids are used for the analysis in 
\cite{BanksSjogreen2011,lrb2013,fib2014}, the analysis for second order interface
conditions is significantly simpler on a collocated grid. 
Let $\Delta t$ be the time step and let $t^n = n \Delta t.$
The solid equations are solved with a dissipative scheme to in order to exploit 
some useful properties in the analysis.
A second order centered scheme was chosen to minimize the stencil to 
three grid points (a second order upwind scheme requires a five point stencil).
The schemes for equations \eqref{eq:advSrcA}--\eqref{eq:advSrcB}
are derived by taking a Taylor series in time and replacing time derivatives
with spacial derivatives. 
Define the grid functions
$\ac^n_j \approx \ac(y_j, t^n), \bc^n_j \approx \bc(y_j, t^n),$ and
$\dc^n_j \approx \dc(y_j,t^n),$
then the Taylor series for $\ac$ is given by
\begin{align}
\ac^{n+1}_j &= \ac^{n}_j + 
\dt \partial_t \ac^{n}_j + 
\frac{\dt^2}{2} \partial_t^2 \ac^{n}_j + O(\dt^3)\\
\ac^{n+1}_j &= \ac^{n}_j - 
\cp \dt \partial_y \ac^{n}_j + 
\frac{\cp^2 \dt^2}{2} \partial_y^2 \ac^{n}_j 
+ i k_x \cp \dt \dc^n_j
- \frac{k_x^2 \cp^2 \dt^2}{4} (\bc^{n}_{j} - \ac^{n}_{j}) + O(\dt^3).
\end{align}
%
A similar series can be derived for $\bc.$
The spacial derivatives are approximated by centered second order finite
difference formulas. Define the undivided difference operators
$\delta_+ u_j = u_{j+1} - u_j,$ 
$\delta_- u_j = u_j - u_{j-1},$ and $\delta_0 = (\delta_+ + \delta_-)/2$ 
for an arbitrary grid function $u_j.$ The scheme for $\ac$ and $\bc$
can be written as
\begin{align}
\ac^{n+1}_{j} &= \ac^{n}_j - 
\frac{\lambda_y}{2} \delta_0 \ac^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \ac^{n}_j 
+ i \lambda_x \dc^n_j
- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j)  \label{eq:aLax} \\
\bc^{n+1}_{j} &= \bc^{n}_j + 
\frac{\lambda_y}{2} \delta_0 \bc^{n}_j + 
\frac{\lambda_y^2}{2} \delta_+ \delta_- \bc^{n}_j 
- i \lambda_x \dc^n_j
- \frac{\lambda_x^2}{4} (\bc^n_j - \ac^n_j) \label{eq:bLax}
\end{align}
%
where $\lambda_x = k_x \cp \dt$ and $\lambda_y = \cp \dt / \dy.$
This is a Lax-Wendroff scheme for an advection equation with a source.
After advancing $\ac$ and $\bc$ to the next time level, $\dc$ can be
advanced with a simple quadrature. Since a non-dissipative pseudo-spectral approximation
is used in the $x$ direction, the trapezoidal rule is used to stabilize the approximation.
\begin{align}
\dc^{n+1}_j &= \dc^{n}_j + \frac{i \lambda_x}{4}
\left(\bc^{n+1}_j - \ac^{n+1}_j + \bc^n_j - \ac^n_j \right). \label{eq:dTrap}
\end{align}
%
The $\cp^+$ characteristic, $\ac,$ will be extrapolated to the interface ghost point.
Additionally, the solution must decay to zero at $y \rightarrow -\infty.$
\begin{alignat}{2}
\ac^n_{1} &= 2 \ac^n_{0} - \ac^n_{-1}, \quad && \\
\vert \ac^n_j \vert^2 +
\vert \bc^n_j \vert^2 +
\vert \dc^n_j \vert^2 &\rightarrow 0, \quad &&\text{as } j \rightarrow -\infty
\label{eq:bcInf}
\end{alignat}
%
The interface condition will determine $b_{1}^n,$ and the initial conditions will 
define $a_j^0, b_j^0,$ and $d_j^0$ for $j = 0,1,2,3,\ldots$.

The fluid variables are kept continuous in $y$ but discrete in time.
For this simplified model analysis, the interface conditions determine 
how the fluid variables are updated. For reference, the Fourier 
coefficients of the velocity and stress components are related to the characteristic 
variables by
\begin{align}
(\vsyh)_j^n = \frac{1}{2\zp} (\bc^n_j-\ac^n_j), \quad
(\ssyh)_j^n = \frac{1}{2} (\bc^n_j+\ac^n_j), \quad
(\ssxh)_j^n = \dc^n_j.
\end{align}

\subsubsection{TP (traditional partitioned) interface conditions}

The TP algorithm is designed to treat the interface as a no-slip velocity 
boundary condition for the fluid and a no-slip traction boundary condition 
for the solid. For this model problem, the time-stepping scheme for the fluid
velocity does not play a role in the analysis. This is because the fluid pressure 
solution only depends on the interface acceleration, which is computed using the
solid solution. The interface acceleration is computed 
using a second order backward difference formula. 

\listAlgorithm{TP Algorithm (without iterations)}{
\item Advance solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
$j = 0,\, -1, \, -2, \, -3, \, \ldots$.

\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$

\item Set the interface velocity as the solid velocity.
\begin{align}
v_I^{n+1} = \frac{1}{2 \zp} \left(\bc_0^{n+1} 
- \ac_{0}^{n+1} \right)
\end{align}

\item Calculate the interface acceleration using a second order accurate
backward difference formula.
\begin{align}
\dot{v}_I^{n+1} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{n+1} 
  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
\end{align}

\item Solve the Poisson equation for the fluid pressure. 
The fluid momentum equation is used to obtain a compatibility 
condition on the pressure gradient at $y=0.$
\begin{alignat}{2}
\ph_{yy}^{n+1} - k_x^2 \ph^{n+1} &= 0, \quad && y \in (0,H), \\
\ph_y^{n+1} &= -\rho \dot{v}_I^{n+1}, \quad && y = 0, \\
\ph^{n+1} &= 0, \quad && y=H
\end{alignat}
%
The solution is
\begin{align}
\ph^{n+1}(y) &= \frac{\rho \dot{v}_I^{n+1} \sinh(k_x (H - y) )}{k_x \cosh(k_x H)} 
\end{align}

\item Set the fluid traction as the solid traction at the interface.
Let $p_I^{n+1} = \ph^{n+1}(0) = \rho \dot{v}_I^{n+1} \tanh(k_x H)/k_x.$
Use an average of the solid cells to obtain $\bc_{1}^{n+1}.$
\begin{align}
b^{n+1}_1 = -b^{n+1}_{-1} - a^{n+1}_1 - a^{n+1}_{-1} - 4 p_I^{n+1}
\end{align}
} \\

It will be shown that the TP algorithm without iterations is unconditionally unstable.
The TP iteration is also analyzed to supplement the results from the zero iteration
algorithm. Under-relaxed iterations are performed on the interface velocity with
under-relaxation parameter, $\omega.$ At the end of the iteration, the $\cp^-$ 
characteristic on the interface, $\bc_0,$ is updated. 

\listAlgorithm{TP Iteration}{
\item Set the interface velocity as the solid velocity.
\begin{align}
v_I^{(k+1)} = \frac{\omega}{2 \zp} \left(\bc_0^{(k)} 
- \ac_{0}^{n+1} \right) + (1-\omega) v_I^{(k)}
\end{align}

\item Calculate the interface acceleration using a second order accurate
backward difference formula.
\begin{align}
\dot{v}_I^{(k+1)} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{(k+1)} 
  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
\end{align}

\item Solve for the interface pressure
\begin{align}
p^{(k+1)}_I &= \frac{\rho \dot{v}_I^{(k+1)} \tanh(k_x H)}{k_x} 
\end{align}

\item Update the $\cp^-$ characteristic, $\bc_{0}^{(k+1)},$ at the interface.
\begin{align}
b^{(k+1)}_0 = -a^{n+1}_0 - 2 p_I^{(k+1)}
\end{align}
} \\

Define $\Heff = \tanh(k_x H)/k_x$ as the effective height of the fluid column. 
This quantity is present in each interface algorithm. For the 1D model problem
($k_x \rightarrow 0$), $\Heff \rightarrow H.$ As the wave number in the $x$ 
direction increases, $\Heff$ will decrease to $0.$ Define the mass ratio
\begin{align}
\Mra = \frac{\rho \Heff}{\zp \dt} = \frac{\rho \Heff}{\rhos \cp \dt}
= \frac{\rho \Heff}{\rhos \ly \dy}.
\end{align}
%
Consider boxes with a cross section of length $L$ in the $x$ direction 
and unit depth out of the $x-y$ plane.
$\Mra$ is the ratio of the fluid mass enclosed in the box of height $\Heff$ to 
the solid mass enclosed in the box of height $\cp \dt,$ or the distance that
a p-wave propagates in time $\dt.$  Additionally define
\begin{align}
\Mr = \ly \Mra = \frac{\rho \Heff}{\rhos \dy}.
\end{align}
%
$\Mr$ is a mass ratio which does not depend on the solid CFL number, $\ly.$
Both $\Mra$ and $\Mr$ decrease as $k_x$ increases.


\subsubsection{ATP (anti-traditional partitioned) interface conditions}

The anti-traditional algorithm reverses the role of the interface in the
traditional scheme. The fluid treats the interface as a no-slip 
traction boundary while the solid treats the interface as a no-slip
velocity boundary. For this algorithm, the fluid velocity is advanced after the
pressure step with trapezoidal rule integration.

\listAlgorithm{ATP Algorithm}{
\item Advance solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
$j = 0,\, -1, \, -2, \, -3, \, \ldots$.

\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$

\item Set the solid traction as the fluid traction at the interface.
\begin{align}
p_I^{n+1} = -\frac{1}{2} \left(b^{n+1}_0 + a^{n+1}_0 \right)
\end{align}

\item Solve the Poisson equation for the fluid pressure. The interface pressure
is used as a Dirichlet condition at $y=0.$
\begin{alignat}{2}
\ph_{yy}^{n+1} - k_x^2 \ph^{n+1} &= 0, \quad && y \in (0,H), \\
\ph^{n+1} &= p_I^{n+1}, \quad && y = 0, \\
\ph^{n+1} &= 0, \quad && y=H
\end{alignat}
%
The solution is
\begin{align}
\ph^{n+1}(y) &= \frac{p_I^{n+1} \sinh(k_x (H - y) )}{\sinh(k_x H)} 
\end{align}

\item Advance the interface velocity using trapezoidal rule on the fluid momentum
equation.
\begin{align}
v^{n+1}_I = v^{n}_I + \frac{k_x \dt}{2 \rho \tanh(k_x H)} 
\left(p_I^{n+1} + p_I^{n}\right)
\end{align}

\item Set the fluid velocity as the solid velocity. Use an average of the solid cells
to obtain $\bc_1^{n+1}.$
\begin{align}
b_{1}^{n+1} = -b_{-1}^{n+1} + a^{n+1}_{1} + a^{n+1}_{-1}
+ 4 \zp v_I^{n+1}
\end{align}
}

\subsubsection{AMP interface conditions}

The AMP algorithm has features from both the TP and ATP scheme. The
interface velocity is taken to be an impedance-weighted average of the 
fluid and solid velocities.
The crucial ingredient is the Robin condition for the pressure in the fluid.
For a large mass ratio, this approximates the Dirichlet problem for 
pressure in the ATP scheme while for a small mass ratio, this approximates the
Neumann problem for pressure in the TP Scheme.

\listAlgorithm{AMP Algorithm (added-mass partitioned)}{
\item Advance solid using equations \eqref{eq:aLax}, \eqref{eq:bLax}, and 
\eqref{eq:dTrap} to obtain $\ac^{n+1}_j, \bc^{n+1}_j,$ and $\dc^{n+1}_j$ for 
$j = 0,\, -1, \, -2, \, -3, \, \ldots$.

\item Extrapolate outgoing $\cp^+$ characteristic, $\ac,$ to $j=1.$

\item Advance the fluid interface velocity using Adams Bashforth on 
the fluid momentum equation.
\begin{align}
v_f^{n+1} = v_I^n + \frac{k_x \dt}{2 \rho \tanh(k_x H)} 
\left( 3 p_I^n - p_I^{n-1} \right)
\end{align}

\item Get the interface velocity and traction from the solid.
\begin{align}
v_s^{n+1} &= \frac{1}{2 \bar{z}} \left(b^{n+1}_0 - a^{n+1}_0 \right) \\
\sigma_s^{n+1} &= \frac{1}{2} \left(b^{n+1}_0 + a^{n+1}_0 \right)
\end{align}

\item Set the interface velocity as the impedance weighted average
of the fluid and solid velocities.
\begin{align}
v_I^{n+1} = \frac{\zf v_f + \zp v_s}{\zf + \zp} 
\end{align}

\item Calculate the interface acceleration using a second order accurate
backward difference formula.
\begin{align}
\dot{v}_I^{n+1} = \frac{1}{\Delta t} \left(\frac{3}{2} v_{I}^{n+1} 
  - 2 v_{I}^{n} + \frac{1}{2} v_{I}^{n-1}  \right)
\end{align}

\item Solve the Poisson equation for the fluid pressure with
the AMP Robin condition specified at $y=0.$
\begin{alignat}{2}
\ph_{yy}^{n+1} - k_x^2 \ph^{n+1} &= 0, \quad && y \in (0,H), \\
-\ph^{n+1}+\frac{\zp \dt}{\rho} \ph_y^{n+1} &= 
\sigma_s^{n+1} - \zp \dt \dot{v}_I^{n+1}, \quad && y = 0, \\
\ph^{n+1} &= 0, \quad && y=H
\end{alignat}

The solution is
\begin{align}
\ph^{n+1}(y) &= p_I^{n+1} \frac{\sinh(k_x (H-y) )}{\sinh(k_x H)} \\
p_I^{n+1} &= \frac{1}{M+1} 
\frac{\rho \dot{v}_I \tanh{(k_x H)}}{ k_x }
 - \frac{M}{M+1} \sigma_s
\end{align}

\item Set the interface traction $\sigma_I^{n+1} = -p_I^{n+1}.$
Set the $\cp^-$ characteristic, $\bc,$ using the interface velocity and stress.
$\delta = \rho/\rhos.$
\begin{align}
%b^{n+1}_1 = -b^{n+1}_{-1} + 2 \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right).
\bc^{n+1}_1 = -\bc^{n+1}_{-1} + 2 
\left[\frac{1}{1+\delta} 
\left(2 \sigma_I^{n+1} - \frac{\ac^{n+1}_{1} + \ac^{n+1}_{-1}}{2} \right)
+\frac{\delta}{1+\delta} \left(\sigma_I^{n+1} + \zp v_I^{n+1} \right) \right].
\end{align}
}


\subsection{Stability analysis of AMP, TP, and ATP schemes}

We will now look for normal mode solutions to the discretizations in terms of an
amplification factor, $\amp.$ Let
\begin{align}
\ac^{n}_j = \amp^n \tac_j, \quad 
\bc^{n}_j = \amp^n \tbc_j, \quad 
\dc^{n}_j = \amp^n \tdc_j,
\end{align}
%
where tilde variables are spacial grid functions. The scheme is said to be weakly
stable if there are no non-trivial solutions where $|\amp| > 1.$ Our strategy for
determining the stability region will be to search only for unstable modes, $|A| > 1.$ 
First, the analysis is split into a spacial and temporal problem. The tilde variables 
will be determined from the interior discretization and boundary condition as 
$y \rightarrow -\infty.$ Solutions for the amplification factor will be found by
finding non-trivial solutions when the normal mode anzatz is
substituted into the interface conditions.

First we reduce the size of the problem by using equation \eqref{eq:dTrap}
to find $\tdc$ in terms of $\tac$ and $\tbc.$ 
\begin{align}
\tdc_j = i \lx D(\amp) (\tbc_j - \tac_j)
\end{align}
%
where
\begin{align}
D(\amp) = \frac{1}{4} \frac{\amp+1}{\amp-1}.
\end{align}
%
Equations \eqref{eq:aLax}--\eqref{eq:bLax} can be written as a system of 
linear second order difference equations. 
Let $\tacv_j = [\tilde{\ac}_j,\tilde{\bc}_j]^T,$ then
\begin{align}
\amp \tacv_j &= 
(I + H_0 + H_1 \delta_0 + H_2 \delta_+ \delta_-) 
\tacv_j \label{eq:diffScheme}
\end{align}
%
where
\begin{align}
H_0 &= \left[ \begin{array}{cc}
-\lambda_x^2 D(\amp) - \frac{\lambda_x^2}{4}
& \lambda_x^2 D(\amp) + \frac{\lambda_x^2}{4} \\
\lambda_x^2 D(\amp) + \frac{\lambda_x^2}{4} & 
-\lambda_x^2 D(\amp) - \frac{\lambda_x^2}{4}
\end{array} \right], \\
H_1 &= \left[ \begin{array}{cc}
-\frac{\lambda_y}{2} + \frac{\lambda_x^2 \lambda_y}{4} D(\amp)
& - \frac{\lambda_x^2 \lambda_y}{4} D(\amp) \\
\frac{\lambda_x^2 \lambda_y}{4} D(\amp) &
\frac{\lambda_y}{2} - \frac{\lambda_x^2 \lambda_y}{4} D(\amp)
\end{array} \right], \\
H_2 &= \left[ \begin{array}{cc}
\frac{\lambda_y^2}{2} & 0 \\ 0 & \frac{\lambda_y^2}{2}
\end{array} \right].
\end{align}
%
Solutions are sought of the form $\tacv_j = \rev \p^j.$ This is substituted into 
equation \eqref{eq:diffScheme} to obtain
\begin{align}
A \rev &= \left( I + H_0 + H_1 \left(\p - \frac{1}{\p}\right)
+ H_2 \left(\p - 2 + \frac{1}{\p} \right) \right) \rev  \label{eq:evProblem}
\end{align}
%
Non trivial solutions for $\p$ are found when the above problem is singular,
therefore
\begin{align}
0 &= \det\bigg{(}I(1-A) + H_0 + H_1 \left(\p - \frac{1}{\p}\right)
+ H_2 \left(\p - 2 + \frac{1}{\p} \right) \bigg{)}. \label{eq:quarticPhi}
\end{align}
%
This results in a quartic polynomial for $\p.$ Due to the boundary condition as
$y \rightarrow -\infty,$ \eqref{eq:bcInf}, we are only interested in solutions 
where $|\p|^j \rightarrow 0$ as $j \rightarrow -\infty.$ Therefore, only $|\p| > 1$ is
a valid solution. Since $|A| > 1$ and the scheme is dissipative, we have
$|\p_1| > 1, |\p_2| > 1, |\p_3| < 1, |\p_4| < 1.$ \todo{ cite Kreiss, explain further.}
We can now write the general solution as
\begin{align}
\acv^n_j = \amp^n \left(k_1 \rev_1 \p_1^j + 
k_2 \rev_2 \p_2^j \right).
\end{align}
%
Let $\rev_n = [\qn{n},\rn{n}]^T$ for $n = 1,2.$
When this is plugged into the interface conditions, a system of equations arise.
\begin{align}
\dMat \kv= \left[\begin{array}{cc}
\dComp_{11} & \dComp_{12} \\
\dComp_{21} & \dComp_{22}
\end{array}\right] 
\left[\begin{array}{c}
k_1 \\ k_2
\end{array}\right] = 0.
\end{align}
%
The first row represents extrapolation of the $\cp^+$ characteristic into the interface
ghost point and is the same for each algorithm.
\begin{align}
\dComp_{1n} = \qn{n} \left(\p_n - 2 + \frac{1}{\p_n} \right), \quad n = 1,2
\end{align}
%
% \begin{align}
% \dComp_{2n} = \begin{cases}
% (\rn{n}+\qn{n}) \left(\p_n + \frac{1}{\p_n} \right)
% + (\rn{n}-\qn{n}) \frac{ M (3 A - 1) (A-1) }{A^2}, & \text{TP} \\
% %%%%%%%%%%%%%%%%%%%%
% (\rn{n}-\qn{n}) \left(\p_n + \frac{1}{\p_n} \right)
% + (\rn{n}+\qn{n}) \frac{(A + 1)}{M (A-1)}, & \text{ATP} \\
% %%%%%%%%%%%%%%%%%%%%
% \rn{n} \left(\p_n + \frac{1}{\p_n} \right)
% \Big(- \left( M+1 \right)^{2} {A}^{4} +\frac{1}{4} \left( 4{M}^{2}+13M
%  \right) {A}^{3} \\
% \phantom{\rn{n} \left(\p_n + \frac{1}{\p_n} \right) \Big{(} }
% -{\frac {15M}{4}}A^2 +\frac{7}{4}M A-\frac{M}{4} \Big{)} \\
% %
% + \qn{n} \left(  \left( {M}^{2}+3/2M-1 \right) {A}^{2}+ \left( -{M}^{2}-7/2
% M \right) A+M \right) {A}^{2} \\
% %
% + \rn{n} 1/2 \left( 2{M}^{2}+M+2 \right) {A}^{4}+1/2 \left( -2{M}^{2}+M
%  \right) {A}^{3}, & \text{AMP}
% \end{cases}
% \end{align}
%
The second row is given by
\begin{align}
\dComp_{2n,\text{TP}} = \;&
 (\rn{n}-\qn{n}) \frac{ M (3 A - 1) (A-1) }{A^2}
+(\rn{n}+\qn{n}) \left(\p_n + \frac{1}{\p_n} \right), \\
% \end{align}
%
% \begin{align}
\dComp_{2n,\text{ATP}} = \;&
 (\rn{n}+\qn{n}) \frac{(A + 1)}{M (A-1)}
+ (\rn{n}-\qn{n}) \left(\p_n + \frac{1}{\p_n} \right), \\
% \end{align}
%
% \begin{align}
\dComp_{2n,\text{AMP}} =\;& 
 \frac{1}{2} \rn{n} \left(\left( 2{M}^{2}+M+2 \right) {A}^{4}+ \left( -2{M}^{2}+M
 \right) {A}^{3} \right),  \nonumber \\
%
&+ \qn{n} \left(  \left( {M}^{2}+\frac{3}{2}M-1 \right) {A}^{2}- \left( {M}^{2}
+\frac{7}{2}
M \right) A+M \right) {A}^{2} \\
%
& \rn{n} \left( \p_n + \frac{1}{\p_n} \right)
\left(- \left( M+1 \right)^{2} {A}^{4} +\frac{1}{4} \left( 4{M}^{2}+13M
 \right) {A}^{3} -{\frac {15M}{4}}A^2 +\frac{7}{4}M A-\frac{M}{4} \right) \nonumber 
\end{align}
%
for $n = 1,2.$ For non-trivial solutions, we look for solutions of $\amp$ such that
\begin{align}
\det(\dMat) = \dComp_{11} \dComp_{22} - \dComp_{12} \dComp_{21} = 0.
\end{align}
%
We first proceed with an analysis of the 1D case ($\lx \rightarrow 0$). After finding 
1D solutions for $\amp,$ numerical continuation in $\lx$ is used to follow the 
evolution of $\amp$ as the wave number in the $x$ direction increases.

\subsubsection{Stability for Cauchy problem in the solid}

% phi's are now exponentials
% plot stability region
% talk about dissipation

\subsubsection{1D scheme}

When $\lx \rightarrow 0,$ the equations in the solid become two uncoupled advection 
equations for the $\cp^+$ characteristic, $\ac,$ and the $\cp^-$ characteristic, $\bc.$
The solid scheme is Lax-Wendroff without source corrections. 
Equation \eqref{eq:diffScheme}
simplifies to 
\begin{align}
A \tac_j = \left( 1 - \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tac_j, \quad
A \tbc_j = \left( 1 + \frac{\lambda_y}{2} \delta_0 
+ \frac{\lambda_y^2}{2} \delta_+ \delta_- \right) \tbc_j
\end{align}
%
The solutions to the eigenvalues, $\p,$ are given by
\begin{align}
\p_{\bc,\pm} = {\frac {{\lambda_{{y}}}^{2}+A-1 \pm \sqrt {2\,A{\lambda_{{y}}}^{2}+{A}^{2}-{
\lambda_{{y}}}^{2}-2\,A+1}}{\lambda_{{y}} \left( \lambda_{{y}}-1
 \right) }}, \quad 
\p_{\ac,\pm} =  \frac{\lambda_y - 1}{\lambda_y + 1} \p_{\bc,\pm}
\end{align}
%
It is well known (e.g. \cite{GKSII}) that when $|A| > 1,$ either
$|\phi_{a,+}| > 1 > |\phi_{a,-}|$ or 
$|\phi_{a,-}| > 1 > |\phi_{a,+}|.$ Define $\phi_1$ and $\phi_2$ to be piecewise, 
so that their magnitudes are strictly greater than one.
\begin{align}
\phi_{1} = \begin{cases}
\phi_{b,+}, & |\phi_{b,+}| > 1 > |\phi_{b,-}| \\
\phi_{b,-}, & |\phi_{b,-}| > 1 > |\phi_{b,+}| \\
\end{cases}, \quad
\phi_{2} = \begin{cases}
\phi_{a,+}, & |\phi_{a,+}| > 1 > |\phi_{a,-}| \\
\phi_{a,-}, & |\phi_{a,-}| > 1 > |\phi_{a,+}| \\
\end{cases}
\end{align}
%
Since $\ac$ and $\bc$ are decoupled, the corresponding eigenvectors are unit vectors,
$\rev_{1} = [0,1]^{T}$ and $\rev_{2} = [1,0]^{T}$ (i.e. $\qn{1} = \rn{2} = 0$). 
The remaining nonzero components of $\dMat$ are $\dComp_{12}$ and $\dComp_{21},$ which leaves
\begin{align}
\det(\dMat_{\text{1D}})= -\dComp_{12} \dComp_{21} = 0
\end{align}
% 
$\dComp_{12}$ is a standard extrapolation operator with repeated roots of $\p_2 = 1.$ 
Since an eigenvalue of magnitude one does not satisfy the boundary conditions, these roots
will be ignored. Upon substituting $\p_1$ as a function of $\amp$ into $\dComp_{21},$
a polynomial can be formed for $\amp$ with coefficients that depend on $\lambda_y$
and $M.$ Maple was used to generate the polynomials for the TP, ATP, and AMP
schemes.
\begin{align}
P_{\text{TP}} =\;& 
 4 {\amp}^{6}
%
+ \left( 12 M{\lambda_{{y}}}^{2
}+8 {\lambda_{{y}}}^{2}-8 \right) {\amp}^{5} \nonumber \\
% 
&+ \left( 9 {M}^{2}{
\lambda_{{y}}}^{4}+12 M{\lambda_{{y}}}^{4}-9 {M}^{2}{\lambda_{{y}}}^
{2}+4 {\lambda_{{y}}}^{4}-28 M{\lambda_{{y}}}^{2}-4 {\lambda_{{y}}}
^{2}+4 \right) {\amp}^{4}\nonumber \\
%
&+ \left( -24 {M}^{2}{\lambda_{{y}}}^{4}
-16 M{\lambda_{{y}}}^{4}+24 {M}^{2}{\lambda_{{y}}}^{2}+20 M{\lambda
_{{y}}}^{2} \right) {\amp}^{3}\nonumber \\
%
&+ \left( 22 {M}^{2}{\lambda_{{y}}}
^{4}+4 M{\lambda_{{y}}}^{4}-22 {M}^{2}{\lambda_{{y}}}^{2}-4 M{
\lambda_{{y}}}^{2} \right) {\amp}^{2}\nonumber \\
%
&+ \left( -8 {M}^{2}{\lambda
_{{y}}}^{4}+8 {M}^{2}{\lambda_{{y}}}^{2} \right) {\amp}
%
+{M}^{2}{
\lambda_{{y}}}^{4}-{M}^{2}{\lambda_{{y}}}^{2} \nonumber\\
% \end{align}
% %
% \begin{align}
P_{\text{ATP}} =\;& 4 {M}^{2}{\amp}^{4}
%
+ \left( 8 {M}^{2}{
\lambda_{{y}}}^{2}+4 {\lambda_{{y}}}^{2}M-16 {M}^{2} \right) {\amp}^{3}\nonumber \\
%
&+ \left( 4 {M}^{2}{\lambda_{{y}}}^{4}+4 M{\lambda_{{y}}}^{4
}-20 {M}^{2}{\lambda_{{y}}}^{2}+{\lambda_{{y}}}^{4}-4 {\lambda_{{y}}
}^{2}M+24 {M}^{2}-{\lambda_{{y}}}^{2} \right) {\amp}^{2}\nonumber \\
%
&+ \left( -8 {M}^{2}{\lambda_{{y}}}^{4}+16 {M}^{2}{\lambda_{{y}}}^{2}+
2 {\lambda_{{y}}}^{4}-4 {\lambda_{{y}}}^{2}M-16 {M}^{2}-2 {\lambda
_{{y}}}^{2} \right) {\amp} \nonumber \\
%
&+4 {M}^{2}{\lambda_{{y}}}^{4}-4 M{
\lambda_{{y}}}^{4}-4 {M}^{2}{\lambda_{{y}}}^{2}+{\lambda_{{y}}}^{4}+4
 {\lambda_{{y}}}^{2}M+4 {M}^{2}-{\lambda_{{y}}}^{2} \nonumber \\
% \end{align}
% %
% \begin{align}
P_{\text{\text{AMP}}} =\;& \big{(} 16 {M}^{4}+64 {M}^{3}+96 {M}^{2}+64 M+
16 \big{)} {\amp}^{10}\nonumber \\
%
&+ \big{(} 16 {M}^{4}{\lambda_{{y}}}^{2}+88
 {M}^{3}{\lambda_{{y}}}^{2}-64 {M}^{4}+144 {M}^{2}{\lambda_{{y}}}^{
2}-296 {M}^{3}\nonumber \\
& \phantom{(+)}+88 M{\lambda_{{y}}}^{2}-432 {M}^{2}+16 {\lambda_{{y
}}}^{2}-232 M-32 \big{)} {\amp}^{9}\nonumber \\
%
&+ \big{(} 4 {M}^{4}{\lambda_{
{y}}}^{4}+28 {M}^{3}{\lambda_{{y}}}^{4}-36 {M}^{4}{\lambda_{{y}}}^{2
}+57 {M}^{2}{\lambda_{{y}}}^{4}-280 {M}^{3}{\lambda_{{y}}}^{2}\nonumber \\
& \phantom{(+)} +28 M
{\lambda_{{y}}}^{4}+96 {M}^{4}-495 {M}^{2}{\lambda_{{y}}}^{2}+4 {
\lambda_{{y}}}^{4}+624 {M}^{3}\nonumber \\
& \phantom{(+)} -192 M{\lambda_{{y}}}^{2}+985 {M}^{2}
-4 {\lambda_{{y}}}^{2}+392 M+16 \big{)} {\amp}^{8}\nonumber \\
% 
&+ \big{(} -8 
{M}^{4}{\lambda_{{y}}}^{4}-84 {M}^{3}{\lambda_{{y}}}^{4}+24 {M}^{4}{
\lambda_{{y}}}^{2}-204 {M}^{2}{\lambda_{{y}}}^{4}+428 {M}^{3}{
\lambda_{{y}}}^{2}-56 M{\lambda_{{y}}}^{4} \nonumber \\
% 
& \phantom{(+)} -64 {M}^{4}+1018 {M}^{2}{
\lambda_{{y}}}^{2}-792 {M}^{3}+236 M{\lambda_{{y}}}^{2}-1560 {M}^{2
}-400 M \big{)} {\amp}^{7} \nonumber \\
%
&+ \big{(} 4 {M}^{4}{\lambda_{{y}}}^{4}
+116 {M}^{3}{\lambda_{{y}}}^{4}-4 {M}^{4}{\lambda_{{y}}}^{2}+406 {M
}^{2}{\lambda_{{y}}}^{4}-380 {M}^{3}{\lambda_{{y}}}^{2}+60 M{\lambda
_{{y}}}^{4} \nonumber \\
&\phantom{(+)} +16 {M}^{4}-1426 {M}^{2}{\lambda_{{y}}}^{2}+640 {M}^{3}-
144 M{\lambda_{{y}}}^{2}+1836 {M}^{2}+240 M \big{)} {\amp}^{6} \nonumber \\
%
&+ \big{(} -88 {M}^{3}{\lambda_{{y}}}^{4}-518 {M}^{2}{\lambda_{{y}}}^{
4}+184 {M}^{3}{\lambda_{{y}}}^{2}-28 M{\lambda_{{y}}}^{4}+1376 {M}^
{2}{\lambda_{{y}}}^{2} \nonumber \\
&\phantom{(+)} -312 {M}^{3}+40 M{\lambda_{{y}}}^{2}-1584 {M}
^{2}-72 M \big{)} {\amp}^{5} \nonumber \\
%
&+ \big{(} 32 {M}^{3}{\lambda_{{y}}}^
{4}+435 {M}^{2}{\lambda_{{y}}}^{4}-44 {M}^{3}{\lambda_{{y}}}^{2}+4 
M{\lambda_{{y}}}^{4} \nonumber \\
&\phantom{(+)} -909 {M}^{2}{\lambda_{{y}}}^{2}+80 {M}^{3}-4 M{
\lambda_{{y}}}^{2}+974 {M}^{2}+8 M \big{)} {\amp}^{4}\nonumber \\
%
&+ \big{(} -
4 {M}^{3}{\lambda_{{y}}}^{4}-238 {M}^{2}{\lambda_{{y}}}^{4}+4 {M}^{
3}{\lambda_{{y}}}^{2}+396 {M}^{2}{\lambda_{{y}}}^{2}-8 {M}^{3}-408 
{M}^{2} \big{)} {\amp}^{3}\nonumber \\
%
&+ \big{(} 79 {M}^{2}{\lambda_{{y}}}^{4}
-107 {M}^{2}{\lambda_{{y}}}^{2}+108 {M}^{2} \big{)} {\amp}^{2}\nonumber \\
%
&+ \big{(} -14 {M}^{2}{\lambda_{{y}}}^{4}+16 {M}^{2}{\lambda_{{y}}}^{2}
-16 {M}^{2} \big{)} {\amp}
%
+{M}^{2}{\lambda_{{y}}}^{4}-{M}^{2}{
\lambda_{{y}}}^{2}+{M}^{2}  \nonumber
\end{align}
%
All solutions to $\det(\dMat_{\text{1D}}) = 0$ are roots of the characteristic 
polynomials, but some spurious roots were introduced in deriving these polynomials.
We evaluate the roots numerically for an array of equally spaced parameters in
the $\ly-\Mr$ plane. 
The roots of the AMP polynomial were found at an array of $800$ points in 
$10^{-6} \le \lambda_y \le 1$ and $800$ points in $10^{-6} \le \Mr \le 10^{7}.$ 
No unstable roots, $|A| > 1,$ were found. The same process was repeated for the 
TP and ATP schemes for a range $10^{-6} \le \Mr \le 10.$ The stability region
was plotted in figure \ref{fig:acousticSolidStokesStabilityTP}. 
Since $\Mr \propto \dy^{-1},$ grid refinement will increase the mass ratio.
The TP scheme will become unstable for sufficiently large $\Mr,$ therefore the 
scheme is formally unconditionally unstable. On the other hand, the ATP scheme will 
eventually become stable for a sufficiently large $\Mr.$ This scheme is weakly
stable. Despite this, there is a significant
region in parameter space where only the AMP scheme is stable.

{
% ---- from codes/analysis/rootFinding/p_1D/b1_genPlots.m ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityRegion}
  \caption{Stability region for the 1D TP and ATP schemes. 
    The stability region for the AMP scheme spans 
    $0 < \ly < 1,$ $0 < \Mr < \infty.$ For reference, 
    $\lambda_y = \bar{c} \dt / \dy$ and $\Mr = \rho H / (\rhos \dy).$
    Grid refinement corresponds to increasing $\Mr,$ therefore the
    TP scheme will become unstable and the ATP scheme will become stable.
  }  \label{fig:acousticSolidStokesStabilityTP}
\end{center}
\end{figure}
}

% talk about numerical results

% Numerical Results:
%  - convergence for each scheme
%  - confirm stability region for each scheme
%
%   TP:
%     - heavy solid convergence study
%     - show stability region
%   ATP: 
%     - light solid convergence study
%     - show stability region
%   AMP:
%     - heavy/light solid convergence study
%     - really heavy/really light

\subsubsection{Continuation into 2D}

% derive eigenvectors with the idea that lx is small
Now we approach the 2D model problem by considering $\lx$ to be a small 
perturbation to the 1D problem. The main motivation for this is
that the stability limit for the Cauchy problem requires $\lx < .3,$ (\todo{show this})
and only $\lx^2$ appears in the discretization. 
%Additionally, the 2D added mass ratio
%$\Mr = (\rho \tanh(k_x H))/(k_x \rhos \dy)$ will only decrease as $k_x$ increases
The strategy for finding roots for $\lx \ne 0$ is to use the 1D roots as a starting point
for a numerical root solver that performs a continuation in $\lx > 0.$ The first step
is finding a suitable expression for the eigenvectors $\rev_1$ and $\rev_2$ so that
$\rev_1 / \| \rev_1 \| \rightarrow [0,1]^T, 
 \rev_2 / \| \rev_2 \| \rightarrow [1,0]^T$ as $\lx \rightarrow 0.$
The first and second components of equation \eqref{eq:evProblem} are used to define
$\rev_1$ and $\rev_2,$ respectively.
\begin{align*}
\qn{1} =\;& -{\lambda_{{x}}}^{2} \left( A{\p_1}^{2}\lambda_{{y}}+{\p_1}^{2}\lambda
_{{y}}-8A\p_1-A\lambda_{{y}}-\lambda_{{y}} \right) \\
%
\rn{1} =\;& -A{\p_1}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}-8A{\p_1}^{2}{\lambda_{{
y}}}^{2}-{\p_1}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}+8A{\p_1}^{2}
\lambda_{{y}}+8A\p_1{\lambda_{{x}}}^{2}+16A\p_1{\lambda_{{y}}}
^{2} \nonumber \\
& +A{\lambda_{{x}}}^{2}\lambda_{{y}}+8{\p_1}^{2}{\lambda_{{y}}}^{2
}+16{A}^{2}\p_1-8A{\lambda_{{y}}}^{2}-8{\p_1}^{2}\lambda_{{y}}-
16\p_1{\lambda_{{y}}}^{2}+{\lambda_{{x}}}^{2}\lambda_{{y}} \nonumber\\
& -32A \p_1-8A\lambda_{{y}}+8{\lambda_{{y}}}^{2}+16\p_1+8\lambda_{{y}
}\\
%
\qn{2} =\;& A{\p_2}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}-8A{\p_2}^{2}{\lambda_{{y
}}}^{2}+{\p_2}^{2}{\lambda_{{x}}}^{2}\lambda_{{y}}-8A{\p_2}^{2}
\lambda_{{y}}+8A\p_2{\lambda_{{x}}}^{2}+16A\p_2{\lambda_{{y}}}
^{2} \nonumber\\
& -A{\lambda_{{x}}}^{2}\lambda_{{y}}+8{\p_2}^{2}{\lambda_{{y}}}^{2
}+16{A}^{2}\p_2-8A{\lambda_{{y}}}^{2}+8{\p_2}^{2}\lambda_{{y}}-
16\p_2{\lambda_{{y}}}^{2}-{\lambda_{{x}}}^{2}\lambda_{{y}} \nonumber\\
& -32A \p_2+8A\lambda_{{y}}+8{\lambda_{{y}}}^{2}+16\p_2-8\lambda_{{y}
} \\
%
\rn{2} =\;& {\lambda_{{x}}}^{2} \left( A{\p_2}^{2}\lambda_{{y}}+{\p_2}^{2}\lambda_
{{y}}+8A\p_2-A\lambda_{{y}}-\lambda_{{y}} \right) .
\end{align*}
%
It is easy to see that $\qn{1} = \rn{2} = 0$ when $\lambda_x = 0.$ In order to solve for 
roots numerically, a black box residual function was created to evaluate $\det(\dMat)$
given $A, \ly, \lx,$ and $\Mra.$ The eigenvalues and eigenvectors can be determined from
these inputs.

% residual function for root solver
\listAlgorithm{Compute Residual of $\det(\dMat)$}{
\item Given $A, \ly,$ and $\lx,$
solve the quartic polynomial for $\p,$ equation \eqref{eq:quarticPhi}, with
ordering $|\p_1| > |\p_2| > |\p_3| > |\p_4|.$ Only $\p_1$ and $\p_2$ are
kept.
\item Calculate the corresponding eigenvectors, $\rev_1$ and $\rev_2.$
\item Given $\Mra,$ form components of $\dMat$ and take the determinant.
} \\

Now that a residual function is introduced, a nonlinear equation solver can be
employed to obtain roots near an initial guess. For this paper, a Newton solver
was used with a Jacobian approximated by finite differences. 
The continuation procedure is outlined as follows.
$\lx$ is discretized 
according to $(\lx^2)_k = k \Delta \lx^2,$ for $k = 0,1,\ldots N$, 
where $\Delta \lx^2 = (\lx^2)_f / N.$ 
Define $A^{(k)}_j$ as the $j$th root corresponding to $\lx = (\lx)_k.$
The 1D root, $A^{(0)}_j$ is used as an initial guess to the 2D problem 
for $k=1$ with $\lx^2 = (\lx^2)_1 = \Delta \lx^2$ to obtain a solution $A^{(1)}_j.$
From here on, the solution $A^{(k-1)}_j$ is used as an initial guess to the 
$\lx^2 = (\lx^2)_{k}$ problem to obtain $A^{(k)}.$

% continuation algorithm
% \listAlgorithm{Continuation in $\lx$}{
% \item Calculate 
% \item $\Delta \lx^2 = (\lx^2)_f/N$
% }
\begin{algorithm}[h]
\caption{Continuation in $\lx$}\label{contour}
\begin{algorithmic}[1]
\Procedure{continuationTP}{$(\lx)_{f},\ly,\Mr,N$}
\State $\Delta \lx^2 \gets (\lx^2)_f/N$ 
% calculate 1D roots
\State Calculate roots, $A_{j}^{(0)},$ 
for $j = 1,\, ...,\, N_{\text{roots}}.$
\For{$j = 1,\, ...,\, N_{\text{roots}}$}
\For{$k = 1,\, ...,\, N$}
\State $(\lx)_k = \sqrt{k \Delta \lx^2}$
\State $A_j^{(k)} \gets$ 
{\tt solveDeterminant}$\left((\lx)_k,\ly,\Mr,A_j^{(k-1)}\right) $
%\Comment{use previous solution as an initial guess}
\EndFor
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

Now consider a fixed $\lx.$ For both the TP and ATP schemes,
there exists a curve $\Mr^*(\ly)$ such that $|A| = 1.$ We are interested in
how this curve evolves when changing $\lx.$ For a given $\lx$ and range
for $\ly,$ points on this curve can be computed using a root solving 
algorithm for $|A|=1.$ Since $|A|$ may not be smooth over the search region, the
bisection algorithm was used for it's robustness. 

% show results
% interpret and account for definition of \Mr

For the AMP algorithm, roots were calculated for $N$ equally spaced points
in the solid stability region and $N$ equally spaced points in 
$10^{-4} < \Mr < 10^{4}$ to verify that no unstable roots were found.

\subsection{Stability analysis of TP scheme with iterations}

The TP scheme is more commonly used with iterations to avoid the added mass instability
when refining grids. We perform an analysis of the TP iteration to understand
how to choose the under-relaxation factor and how many iterations to take.
Define the error between iterations to be the difference in interface velocities
\begin{align}
e^{(k)} = v_I^{(k+1)} - v_I^{(k)}.
\end{align}
%
By taking the difference between the current and previous iteration variable for
each step of the TP iteration, one can derive that
\begin{align}
e^{(k)} &= \left(1 - \omega \left(\frac{3}{2} \Mra + 1 \right)\right) e^{(k-1)}.
\end{align}
%
Define the amplification factor, $\ampI = 1 - \omega \left(\frac{3}{2} \Mra + 1 \right)$
where $e^{(k)} = A^{k} e^{(0)}.$
$\Mra$ is dependent on the wave number, $k_x.$ In order to optimize the convergence rate,
$\ampI$ needs to be optimized for all wave numbers.
\begin{align}
\Mra = \frac{\rho \tanh(k_x H)}{\zp \dt k_x} 
= \frac{\rho H}{\zp \dt} \frac{\tanh(k_x H)}{k_x H} 
= \Mra_0 \eta
\end{align}
%
where $\Mra_0 = (\rho H) / (\zp \dt)$ is the 1D acoustic mass ratio and 
$\eta = \tanh(k_x H) / (k_x H)$ is the 2D scale factor. To accommodate all
potential wave numbers in the $x$ direction, we consider $\eta \in [0,1].$
Let $\Mra = \Mra(\eta) = \Mra_0 \eta.$ The amplification factor for a given
$\omega$ and $\eta$ is
\begin{align}
\ampI(\eta,\omega) = a - \omega \left(\frac{3}{2} M_0 \eta + 1 \right).
\end{align}
%
We pose the following optimization problem to find the optimal 
under-relaxation parameter, $\omega^*$.
\begin{align}
\omega^* = \argmin_{\omega} \max_{0 \le \eta \le 1} |A(\eta,\omega)|
\end{align}
%
Since $\ampI$ is linear in $\eta$ and $\omega$ and $|\ampI| > 0,$ the maximum 
amplification factor for a 
given $\omega$ will occur on the boundary, $\eta = 0$ or $\eta = 1.$ 
\begin{align}
\ampI(\eta=0,\omega) = |1-\omega|, \quad 
\ampI(\eta=1,\omega) = \left| 1 - \omega \left(\frac{3}{2} M_0 + 1 \right) \right|
\end{align}
%
The choice of $\omega$ that minimizes both expressions corresponds to solving
$\ampI(\eta=0,\omega^*) = \ampI(\eta=1,\omega^*).$ It can be shown that
\begin{align}
\omega^* = \frac{4}{3 \Mra_0 + 4}, \quad \ampI^* = \frac{3 M_0}{3 M_0 + 4}.
\end{align}
%
This is a sensible result. The TP scheme suffers from added mass instability
for fine grids and light solids, which correspond to large acoustic mass ratios.
The under-relaxation parameter scales with $\Mra_0^{-1}$ to stabilize the added mass
effects. As a penalty, the amplification factor approaches $1$ for large $\Mra_0.$
To get a sense of computational cost for using TP iterations, we look at the number
of iterations needed for the relative error, $|e^{(k)}/e^{(0)}|,$ to converge to 
a desired tolerance, $\tau.$  It is easy to show that if $|A^*|^k < \tau,$ $k$ must 
satisfy
\begin{align}
k &> \frac{\log (\tau) }
{\log \left(\frac{3 M_0}{3 M_0 + 4} \right)} .
\end{align}
% 
We are interested in the asymptotic behavior for $\Mra_0 \gg 1.$ The denominator
of the above expression is asymptotically equivalent to
\begin{align}
\log \left(\frac{3 \Mra_0}{3 \Mra_0 + 4} \right) =
 \log \left(\frac{1}{1 + \frac{4}{3 \Mra_0} } \right)
\sim  \log \left(1 - \frac{4}{3 \Mra_0} + ... \right) 
\sim -\frac{4}{3 \Mra_0} + ...
\end{align}
%
Therefore 
\begin{align}
k > -\frac{3}{4} M_0 \log(\tau) = 
-\frac{3 }{4} \frac{\rho H }{ \bar{\rho} \bar{c} \Delta t} \log(\tau).
\end{align}
% 
The required number of iterations is proportional to $\dt^{-1}.$ 
For a viscous fluid simulation, the viscous terms can be treated as
implicitly or explicitly.
When an implicit solver is chosen, the time step will be proportional to
the grid spacing and the number of iterations will double when the grid is refined 
by a factor of $2$. 
When an explicit solver is chosen, the time step will be proportional to the 
square of the grid spacing and the number of iterations will quadruple when the grid
is refined by a factor of $2.$


% numerical results 



%%%%%%%%%%%%% old paper
% \subsection{Discretization}

% talk about fluid and solid discretization in x. 
% discrete fourier series on grid 
% % \wdh{We discretize the fluid and solid variables in the $x$~direction using a uniform
% % grid with spacing $\dx=L/(N_x+1)$. The grid points are given by $x_\ell=\ell\dx$,
% % $\ell=0,1,\ldots,N_x$.  The choice of discrete approximations to the
% % $x$~derivatives in the equations plays little role in the analysis.  Therefore, it is
% % convenient to use a pseudo-spectral approximation by expanding
% % each component $q$ of the solution $(\qv,\qsv)$ in a discrete Fourier series of
% % the form
% % % which gives a formally {\em exact} approximation,  $i\kx$, to an $x$-derivative.
% % % After discretizing in the $x$~direction we will expand the solution in a discrete Fourier series of the form
% % \begin{align}
% %    q_\ell(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_\ell/L} \qHat_{k}(y,t), \qquad \ell=0,1,2,\ldots,N_x, \label{eq:discreteFourier}
% % \end{align}
% % where $q_\ell(y,t)\approx q(x_\ell,y,t)$ and $\qHat_{k}(y,t)$ are Fourier coefficients, 
% % and where $N_x$ is assumed to be even for convenience.
% % Transforming the governing equations to Fourier space leads to the following equations for the Fourier coefficients of the solution variables:
% % \begin{alignat}{3}
% % &   \rhos \partial_t \vs = i\kx \sigmas_{21} + \partial_y \sigmas_{22} , \quad&& y\in(0,\infty), \label{eq:vEqn} \\
% % &   \partial_t \sigmas_{22} = \rhos \cp^2 \partial_y\vs , \quad&&y\in(0,\infty), \label{eq:s22Eqn} \\
% % &   \partial_t \sigmas_{21} = i\kx \rhos \cp^2 \vs , \quad&&y\in(0,\infty) , \label{eq:s21Eqn} \\
% % & \rho \partial_t v_1 = i\kx      \sigma, \quad &&y\in(-H,0), \label{eq:v1HatEqn} \\
% % & \rho \partial_t v_2 = \partial_y\sigma, \quad && y\in(-H,0), \label{eq:v2HatEqn} \\
% % &  i\kx v_1 + \partial_y v_2 =0 ,                  \quad&&y\in(-H,0) , \label{eq:divHatEqn}
% % \end{alignat}
% % where $\kx = 2\pi k/L$ is a normalized wave number in the $x$~direction and the
% % equations hold for each $k=-N_x/2,-N_x/2+1,\ldots,N_x/2$. The hats on the
% % Fourier coefficients, along with the $k$ subscripts, have been dropped for
% % notational convenience.  Note that the horizontal component of the fluid
% % velocity, $v_1$, is decoupled from the other equations and boundary conditions, 
% % and can be determined once $v_2$ is known. Equations~\eqref{eq:v1HatEqn}--\eqref{eq:divHatEqn} are used to obtain
% % \[
% % \partial_y^2 \sigma - \kx^2 \sigma =0,      \qquad y\in(-H,0) ,
% % \]
% % which is a Laplace equation for pressure (in Fourier space).  The equations for the Fourier coefficients of the solid variables will be discretized using an upwind scheme.  In preparation for this, it is convenient to define the characteristic variables
% % \[
% % a=\sigmas_{22}-\rhos\cp\vs,\qquad b=\sigmas_{22}+\rhos\cp\vs,\qquad d=\sigmas_{21},
% % \]
% % which, from~\eqref{eq:vEqn}--\eqref{eq:s21Eqn}, satisfy
% % \begin{alignat}{3}
% % &   \partial_t a + \cp \partial_y a =  i\kx\cp\, d , \qquad&& y\in(0,\infty),  \label{eq:aHatEqnII}\\
% % &   \partial_t b - \cp \partial_y b = -i\kx\cp\, d , \qquad&& y\in(0,\infty),  \\
% % &   \partial_t d = \frac{i\kx\cp}{2}(b-a) , \qquad&& y\in(0,\infty).  \label{eq:dHatEqnII} 
% % \end{alignat}}
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%
% The solid variables are discretized in the $y$~direction using a uniform grid with
% spacing $\dy$.  The grid points for the solid domain are defined as $y_j=
% (j-\half)\dy$, $j=0,1,2,\ldots$. 
% Following the analysis in~\cite{BanksSjogreen2011,lrb2013}, the grid is staggered with respect to the
% interface at $y=0$ and has a ghost point at $j=0$; use of a non-staggered grid leads to similar results.
% %  This staggering simplifies the analysis but is not critical {\bf (I'm not convinced of this ?!?!)}.  
% Let  $\dt$ be the time step and let $t^n=n\dt$.  The
% equations~\eqref{eq:aHatEqnII}--\eqref{eq:dHatEqnII} are discretized using the
% first-order upwind scheme,
% \begin{alignat}{3}
% &   \frac{ a_j^{n+1}- a_j^n}{\dt} + \cp\frac{( a_j^n - a_{j-1}^n)}{\dy} =   i\kx\cp\, d_j^{n}, \label{eq:aEqnIII} \\
% &   \frac{ b_j^{n+1}- b_j^n}{\dt} - \cp\frac{( b_{j+1}^n - b_j^n)}{\dy} = - i\kx\cp\, d_j^{n}, \label{eq:bEqnIII} \\
% &   \frac{ d_j^{n+1}- d_j^n}{\dt} = \frac{i\kx\cp}{2}(b_j^{n+1} - a_j^{n+1}), \label{eq:dEqnIII}
% \end{alignat}
% where $a_j^{n}\approx a(y_j,t^n)$, $b_j^{n}\approx b(y_j,t^n)$ and
% $d_j^{n}\approx d(y_j,t^n)$. 
% Since we have used a non-dissipative pseudo-spectral approximation, rather than a two-dimensional upwind scheme, 
% the right-hand side terms in~\eqref{eq:dEqnIII} are taken at time $t^{n+1}$ in order to stabilize the approximation.
% A von Neumann stability analysis of equations~\eqref{eq:aEqnIII} and~\eqref{eq:bEqnIII} (for a
% periodic problem in $y$) shows that this time-stepping scheme is stable under
% reasonable conditions on the constants $\ly=\cp\dt/\dy$ and $\lx=\cp\kx\dt$.
% The fluid variables are kept continuous in $y$ in order to simplify the
% presentation; a discrete version can be introduced but this makes only
% insignificant changes to the fundamental results.  We are thus led to the
% following semi-discrete approximation for the solid and fluid equations,
% \begin{alignat}{3}
% &   a_j^{n+1} = a_j^n -\ly( a_j^n - a_{j-1}^n) - i \lx d_j^{n} , \quad&& j=1,2,3,\ldots\;, \label{eq:aEqn} \\
% &   b_j^{n+1} = b_j^n +\ly( b_{j+1}^n - b_j^n) + i \lx d_j^{n},  \quad&& j=0,1,2,\ldots\;, \label{eq:bEqn}  \\
% &   d_j^{n+1} = d_j^n +  \frac{i\lx}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=0,1,2,\ldots\;,  \\
% % 
% &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0), \\
% &  0=\partial_y^2 \sigma^{n+1}- \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), \label{eq:sigmaEqn}
% \end{alignat}
% where $v^n(y)=v(y,t^n)$ and $\sigma^n(y)=\sigma(y,t^n)$.  For reference, the discrete values for the (Fourier coefficients of the) velocity and components of stress in the solid are related to the characteristic variables by
% \[
% \vs_j^n=\frac{1}{2\zp}(b_j^n-a_j^n),\qquad\sigmas_{22,j}^n=\frac{1}{2}(b_j^n+a_j^n),\qquad \sigmas_{21,j}^n=d_j^n.
% \]
% The conditions at the top and bottom boundaries are 
% \begin{align}
% &   \vert a_j^{n}\vert^2 + \vert b_j^{n}\vert^2 + \vert d_j^{n}\vert^2 \rightarrow 0, 
%          \quad\text{as $j\rightarrow \infty$} ,  \label{eq:BCtop}\\
% &   \sigma^n(-H)=0. \label{eq:BCbottom}
% \end{align}
% Initial conditions are required to define $a_j^{0}$, $b_j^{0}$ and $d_j^{0}$ for $j=0,1,2,3,\ldots$, as well as $v^0(y)$ for  $y\in(-H,0)$, but these conditions are of no significance in the subsequent stability analysis.

% Approximations to the interface conditions are needed to complete the discrete
% formulation of the FSI model problem, and various choices are possible depending
% on the algorithm used.  
% For the AMP algorithm, the pressure Robin
% condition~\eqref{eq:AddedMassPressureBC} is imposed on the fluid; this is derived from the
% outgoing characteristic variables~\eqref{eq:AMPoutgoing}. In addition, the 
% incoming characteristic variable~\eqref{eq:AMPincoming} is used to specify a condition
% on the solid.  The latter condition uses an interface velocity defined
% in~\eqref{eq:ImpedenceWeightedVn} based on an impedance-weighted average.  
% First-order accurate approximations of these conditions are
% \begin{alignat}{3}
% &  \sigma^{n+1}(0) + \frac{\zp\dt}{\rho} \sigma_y^{n+1}(0) = \sigmas_{22,1}^{n+1} + \zp(\vs_1^{n+1} - v^{I,n})
%                                            = b_1^{n+1} -\zp v^{I,n}, && \label{eq:1dSigmaBC}\\
% &  a_0^{n+1} = \sigma^{I,n+1} - \zp v^{I,n+1}, &&\label{eq:1dSolidBC}
% \end{alignat}
% where $\sigma^{I,n}\equiv\sigma^n(0)$ and $v^{I,n}$ are the interface traction and velocity, respectively.  The latter is given by the impedance-weighted average
% \begin{alignat}{3}
% &   v^{I,n+1} = \frac{\zf}{\zf+\zp} v^{n+1}(0) + \frac{\zp}{\zf+\zp}\vs_1^{n+1} + \frac{1}{\zf+\zp}(\sigma_{22,1}^{n+1} - \sigma^{I,n+1} ) && \nonumber\\
% & \hphantom{v^{I,n+1}} = \gamma v^{n+1}(0) + \frac{1-\gamma}{\zp}( b_1^{n+1} - \sigma^{I,n+1} ), && \label{eq:1dVelocityBC}\end{alignat}
% where
% \[
% \gamma=\frac{\zf}{\zf+\zp},
% \]
% and where $\zf$ is a measure of the fluid impedance as introduced in Section~\ref{sec:partitionedAlgorithms}.

% The traditional partitioned (TP) algorithm uses the velocity from the solid as a boundary condition for the fluid and the traction from the fluid as a boundary condition for the solid.  First-order accurate approximations of these conditions are
% \begin{alignat}{3}
%  &   v^{n+1}(0)=\vs_1^{n+1}  
%         , &&   \label{eq:1dTradv} \\
%  &   \sigmas^{n+1}_{22,0} = \sigma^{n+1}(0). &&\label{eq:1dTradsigma}
% \end{alignat}
% It is also instructive to consider an anti-traditional algorithm in which
% the roles of the fluid and solid are reversed in the application of the
% partitioned interface conditions.  Approximations of these conditions are
% \begin{alignat}{3}
% &   \sigma^{n+1}(0) = \sigmas^{n+1}_{22,1}\,,  &&  \label{eq:1dAntiTradsigma} \\
% &   a_0^{n+1} = \sigma^{n+1}(0) - \zp v^{n+1}(0) .&& \label{eq:1dAntiTradv} 
% \end{alignat}
% The condition in~\eqref{eq:1dAntiTradv} is equivalent to setting the velocity of solid at the interface equal to the velocity in the fluid since the stresses have already been equilibrated in~\eqref{eq:1dAntiTradsigma}. 

% % 
% % 
% % % On the interface we assign the out-going characteristic variable by imposing~\eqref{eq:bEqn} at $j=0$.
% % The boundary conditions for the fluid are $\sigma^n(-H)=0$, while the solid solution should decay to zero 
% % as $j\rightarrow\infty$. 
% % The solution for $\sigma^n$ satisfying the boundary condition $\sigma^n(-H)=0$ can be written as
% % \begin{alignat}{3}
% % &  \sigma^{n}= \sigma^{I,n} \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \quad&& y\in(-H,0), 
% % \end{alignat}
% % where $\sigma^{I,n}=\sigma^n(0)$. 



% %- \vskip3\baselineskip
% %- 
% %- 
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- Let $\dt$ be the time step and let $t^n=n\dt$. 
% %- Introduce fully discrete approximations for the solid variables of the form $\qs_j^n \approx \qsHat(y_j,t^n)$ and
% %- semi-discrete approximations for the fluid variables of the form $q^n(y) \approx \qHat(y,t^n)$. 
% %- 
% %- This leads to the approximation
% %- \begin{alignat}{3}
% %- &   a_j^{n+1} = a_j^n -\lambda( a_j^n - a_{j-1}^n) - i \lambdax d_j^{n} , \quad&& j=1,2,3,\ldots \\
% %- &   b_j^{n+1} = b_j^n +\lambda( b_{j+1}^n - b_j^n) + i \lambdax d_j^{n},  \quad&& j=1,2,\ldots  \\
% %- &   d_j^{n+1} = d_j^n + i \frac{\lambdax}{2} ( b_j^{n+1} - a_j^{n+1}),    \quad&& j=1,2,\ldots  \\
% %- % 
% %- &   v^{n+1} = v^n + \frac{\dt}{\rho} \partial_y \sigma^{n+1},             \quad&& y\in(-H,0) \\
% %- &  \partial_y^2 \sigma^{n+1}= \kk^2 \sigma^{n+1},                             \quad&& y\in(-H,0), 
% %- \end{alignat}
% %- where $\lambday=\frac{\cb\dt}{\dy}$ and $\lambdax=\cb\dt\kx$ and where $a_j^{n}$, $b_j^{n}$ and $d_j^n$
% %- are the characteristic variables in the solid given by 
% %- \begin{alignat}{3}
% %-    a_j^{n} = \sigmas_j^n -\zb \vs_j^n, \quad&& \vs_j^n &=\frac{1}{2\zb}(b_j^n-a_j^n), \\
% %-    b_j^{n} = \sigmas_j^n +\zb \vs_j^n, \quad&& \sigmas_j^n &=\frac{1}{2}(b_j^n+a_j^n), \\
% %-    d_j^n = \sigma^n_{21,j}
% %- \end{alignat}
% %- The boundary conditions for the fluid are $\sigma^n(-H)=0$, while for the solid the solution should remain bounded
% %- as $j\rightarrow\infty$. Initial conditions are needed for $a_j^{0}$, $b_j^{0}$, $d_j^{0}$, $j=0,1,2,3,\ldots$, 
% %- and $v^0(y)$, $y\in(-H,0)$.
% %- Approximations to the interface conditions are needed; various choices for these will be specified later. 
% %- 
% %- 
% %- 
% %- \vskip3\baselineskip
% %- 
% %- Introduce the fully discrete approximations $\vs_{ij}^n \approx \vs(x_i, y_j, t^n)$, 
% %- $\sigmas_{22,ij}^n \approx \sigmas^{22}(x_i, y_j, t^n)$, 
% %- $\sigmas_{21,ij}^n \approx \sigmas^{21}(x_i, y_j, t^n)$, 
% %- in the solid, 
% %- and the semi-discrete approximations $\vv_i^n(y)\approx \vv(x_i,y,t^n)$, $\sigma_i^n(y)\approx \sigma(x_i,y,t^n)$ in the fluid.
% %- We 
% %- expand the solution in a Fourier series in $x$,
% %- \begin{align}
% %-    \vs_{ij}^n = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat_{k,j}^n, \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}


% %- 
% %- 
% %- 
% %- We 
% %- expand the solution in a Fourier series in $x$. 
% %- We introduce the approximations $\vs_j(y,t) \approx \vs(x_j,y,t)$, $\sigma_{22,j}(y,t) \approx \sigmas_{22}(x_j,y,t)$, 
% %- $\sigma_{21,j}(y,t) \approx \sigmas_{21}(x_j,y,t)$, for the solid and 
% %- $\vv_j(y,t) \approx \vv(x_j,y,t)$, and $\sigma_{j}(y,t) \approx \sigma(x_j,y,t)$ for the fluid. 
% %- where 
% %- \begin{align}
% %-    \vs_j(y,t) = \sum_{k=-N_x/2}^{N_x/2} e^{2\pi i k x_j/L} \vsHat(k,y,t), \quad j=0,1,2,\ldots,N_x-1.
% %- \end{align}
% %- We let $\kx = 2\pi k/L$ be the normalized wave number.
% %- 
% %- 
% %- 
% %- We discretize the solid in the $y$~direction with a grid spacing $\dy$.
% %- The grid for the solid is defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$. This grid is staggered
% %- with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- simplies the analysis but is not critical.
% %- The fluid variables are kept continuous in $y$ in order to simplify the presentation; the discrete version
% %- can be easily handled and makes only insignificant changes to the fundamental results.
% %- 
% %- % with grid spacing $\dy$ and use 
% %- % a first-order upwind scheme (in the $y$~direction) for the resulting solid equations. 
% %- % The grid for the solid, defined as $y_j= (j-\half)\dy$, $j=0,1,2,\ldots$, is staggered
% %- % with respect to the boundary at $y=0$ (see Figure ??) and has a ghost point at $j=0$. This staggering 
% %- % simplies the analysis but is not critical.
% %- 
% %- In the solid we introduce grid functions $\vs_j^n\approx \vsHat(\kx,y_j,t^n)$, etc. 
% %- For the fluid we form approximations that are continuous in $y$ but discerete in time denoted by  
% %- $\sigma^n(y) \approx \sigmaHat(\kx,y,t^n)$,  and 
% %- $v^n(y) \approx \vHat_2(\kx,y,t^n)$. The horizontal component of the fluid velocity, $\vHat_1^n$, plays no role 
% %- in the analysis and can be determined from $v^n(y)$ using  $i\kx \vHat_1^n + \partial_y v^n(y)=0$, if needed.
% %- 
% %- 
% %- 


% % ------------------------------------------------------------------------------------------------
% \subsection{Stability analysis}

% \renewcommand{\aHat}{{\tilde a}}
% \renewcommand{\bHat}{{\tilde b}}
% \renewcommand{\dHat}{{\tilde d}}
% \renewcommand{\vHat}{{\tilde v}}
% \renewcommand{\sigmaHat}{{\tilde\sigma}}
% % \renewcommand{\aTilde}{{\bar a}}
% % \renewcommand{\bTilde}{{\bar b}}
% \renewcommand{\aTilde}{\alpha}
% \renewcommand{\bTilde}{\beta}

% To analyze the stability of the approximation
% in~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn}, we look for solutions of the form \[
% a_j^n=\amp^n\aHat_j, \qquad b_j^n=\amp^n\bHat_j, \qquad d_j^n=\amp^n\dHat_j,
% \qquad v^n(y)=\amp^n\vHat(y), \qquad \sigma^n(y)=\amp^n\sigmaHat(y),
% \] 
% where $\amp\in\Complex$ is the amplification factor,
% $(\aHat_j,\bHat_j,\dHat_j)$ are grid functions, and $(\vHat(y),\sigmaHat(y))$
% are functions for $y\in[-H,0]$. 
%  Substituting these forms
% into~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} results in the following system of
% equations
% \begin{alignat}{3}
% &  \amp \aHat_j = \aHat_j -\ly( \aHat_j - \aHat_{j-1}) - i \lx \dHat_j , \qquad&& j=1,2,3,\ldots\,, \label{eq:aHatEqn} \\
% &  \amp  \bHat_j = \bHat_j +\ly( \bHat_{j+1} - \bHat_j) + i \lx \dHat_j,  \qquad&& j=0,1,2,\ldots\,, \label{eq:bHatEqn}  \\
% &  \amp  \dHat_j = \dHat_j + \frac{i\lx}{2}\amp  ( \bHat_j - \aHat_j),    \qquad&& j=0,1,2,\ldots\,,  \label{eq:dHatEqn} \\
% % 
% &  \amp  \vHat(y) = \vHat(y) + \amp\dt\,\sigmaHat^I\,\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},  \qquad&& y\in[-H,0], \label{eq:vHatEqn} \\
% &  \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},          \qquad&& y\in[-H,0].\label{eq:sigmaHatEqn}
% \end{alignat}
% To obtain~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn},  the
% ODE in~\eqref{eq:sigmaEqn} was integrated using the boundary conditions $\sigmaHat(-H)=0$
% and $\sigmaHat(0)=\sigmaHat^I$, where the fluid stress at the interface, $\sigmaHat^I$, is as
% yet unspecified.  Note that the solution in the one-dimensional case,
% $\kk=0$, is a special case that can be found by taking the limit $\kk\rightarrow
% 0$ in~\eqref{eq:vHatEqn} and~\eqref{eq:sigmaHatEqn}. 
% Together with the interface
% conditions, equations~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} define
% a homogeneous set of difference equations. These equations have
% non-trivial solutions (i.e. eigenfunctions) only for particular values of $\amp$ (i.e. eigenvalues).
% The scheme is said to be weakly stable, or stable in the sense of
% Godunov-Ryabenkii, for given values of the parameters $\dt$, $\dy$, $\kx$, $H$, etc., 
% if there are no solutions (i.e.~eigenfunctions) to this
% eigenvalue problem with $\vert \amp\vert>1$. 
% The {\em region of stability} of the scheme is the region in parameter space where there are no roots with $\vert \amp\vert>1$. 
% In order to delineate the stability region 
% it is generally easier to look for regions where the scheme is {\em not} stable. Therefore, we 
% assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % we look for regions in the space of parameters where $\vert \amp\vert>1$  and the scheme is unstable.
% % We thus 
% % assume that $\vert \amp\vert>1$ and look for solutions to the eigenvalue problem.  
% % If no such solutions exist for some given values of the parameters, then the scheme is (weakly) stable there. 
% % The stability domain is defined to be the region in parameter space where there are no roots with $\amp>1$.


% Equations~\eqref{eq:aHatEqn}--\eqref{eq:dHatEqn} are a system of
% constant-coefficient difference equations for the solid characteristic
% variables.  After solving for $\dHat_j$ from~\eqref{eq:dHatEqn} and substituting
% into~\eqref{eq:aHatEqn} and~\eqref{eq:bHatEqn}, $\aHat_j$ and
% $\bHat_j$ are found to satisfy the recursion
% \begin{equation}
%  \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = K \begin{bmatrix} \aHat_{j-1} \\ \bHat_{j-1} \end{bmatrix}, \qquad K =\begin{bmatrix}  ( 1 - \theta^2)/R & -\theta \\ \theta & R \end{bmatrix} ,
% \label{eq:recursion}
% \end{equation}
% where
% \begin{equation}
% R = r-\theta, \qquad r = \frac{\amp-1+\ly}{\ly}, \qquad \theta = -\frac{\amp\lx^2}{2\ly(\amp-1)} . 
% \label{eq:RandTheta}
% \end{equation}
% The eigenvalues, $\phi_-$ and $\phi_+$, of
% the $2\times2$ matrix $K$ in~\eqref{eq:recursion}
% %  \old{are the roots of a quadratic polynomial, and are given by} 
% are given by
% % \old{
% % We are interested in solutions for $\aHat_j$ and $\bHat_j$ that decay as
% % $j\rightarrow\infty$ so that the boundary condition in~\eqref{eq:BCtop} is
% % satisfied.  This leads us to consider the eigenvalues, $\phi_-$ and $\phi_+$, of
% % the $2\times2$ matrix $K$ in~\eqref{eq:recursion}, which are found by finding
% % the roots of a quadratic polynomial.  The result is
% % }
% \begin{equation}
% \phim = B - \sqrt{ B^2 - 1}, \qquad \phip=1/\phim, \qquad B = \frac{1}{2}\left(R + \frac{1 - \thetaj^2}{R}\right).
% \label{eq:phipm}
% \end{equation}
% Note that the product of the eigenvalues is one.  
% If both eigenvalues 
% % \old{were to have magnitude one} 
% had magnitude equal to one, then there would be no solution of the recursion
% in~\eqref{eq:recursion} satisfying the boundary condition~\eqref{eq:BCtop}.
% Therefore, for a valid solution, there is one eigenvalue (either $\phi_-$ or $\phi_+$),
% denoted by $\phis$ (for {\em small} $\phi$), that has magnitude strictly less
% than one, i.e.~$\vert\phis\vert<1$.  Let $\phib=1/\phis$ (for {\em big} $\phi$)
% be the other eigenvalue with $\vert\phib\vert>1$.  Note that when $\theta=0$,
% $0<\ly\le 1$, and $\vert\amp\vert>1$, then $\phis=\phim=1/r$ (but in general
% $\phis$ is not always equal to $\phim$).  Given that the eigenvalues are
% distinct, $K$ can be diagonalized as 
% \[
% K = S^{-1} \Phi S , \qquad
% \Phi =\begin{bmatrix}  \phis &  0 \\
%                            0 & \phib \end{bmatrix}, \qquad
% S =\begin{bmatrix}  R-\phis & \thetaj \\
%                     R-\phib & \theta \end{bmatrix}.
% \]
% By setting 
% \begin{align}
% &   \begin{bmatrix} \aTilde_j \\ \bTilde_j \end{bmatrix}
%    =  S \begin{bmatrix} \aHat_j \\ \bHat_j \end{bmatrix} = 
%    \begin{bmatrix} (R-\phis)\aHat_j + \theta \bHat_j \\
%                    (R-\phib)\aHat_j + \theta \bHat_j
%    \end{bmatrix}, \label{eq:abTildeEqn}
% \end{align}
% the general solution of the recursion in~\eqref{eq:recursion} is given by 
% \begin{equation}
% \begin{array}{l}
%    \aTilde_j = \phis^j \aTilde_0, \smallskip\\
%    \bTilde_j = \phib^j \bTilde_0.
% \end{array}
% \label{eq:abBarEqn}
% \end{equation}
% Since the solution must decay to zero as $j\rightarrow \infty$ and since $\vert\phib\vert>1$, it follows that $\bTilde_0=0$ and thus $\bTilde_j=0$ for all $j=0,1,2,\ldots$.  Since $\bTilde_j=0$, it follows from~\eqref{eq:abTildeEqn} that
% \begin{equation}
% \bHat_j = Q \aHat_j,\qquad \aTilde_j=(\phib-\phis)\aHat_j,\qquad Q = \frac{\phib-R}{\theta},
% \label{eq:Qdef}
% \end{equation}
% and thus from~\eqref{eq:abBarEqn}, 
% \[
% \aHat_j=\phi_s^j\aHat_0\,.
% \]
% Whence,
% % ------------------------------------------- PROP -------------------------------------------------
% \begin{proposition}
% Solutions to the system in~\eqref{eq:aHatEqn}--\eqref{eq:sigmaHatEqn} with $\vert\amp\vert>1$ satisfying the boundary conditions in~\eqref{eq:BCtop} and~\eqref{eq:BCbottom} are given by
% \[
% \begin{array}{c}
% \displaystyle{
% \aHat_j=\phi_s^j\aHat_0,\qquad \bHat_j=Q\aHat_j,\qquad \dHat_j=\frac{i\lx(Q-1)\amp}{2(\amp-1)}\aHat_j,\qquad j=0,1,2,\ldots\,,
% } \bigskip\\
% \displaystyle{
% \sigmaHat(y)= \sigmaHat^I\, \frac{\sinh(\kk (y+H))}{\sinh(\kk H)},\qquad \vHat(y)=\sigmaHat^I\,\frac{\amp\dt}{\amp-1}\;\frac{\kk\cosh(\kk (y+H))}{\rho\sinh(\kk H)},\qquad y\in[-H,0],
% }
% \end{array}
% \]
% % \old{where the two free constants, $\aHat_0$ and $\sigmaHat^I$, will be determined by two interface conditions.} 
% where $\aHat_0$ and $\sigmaHat^I$ are free constants.
% \end{proposition}

% The remaining constraints needed to complete the eigenvalue problem, which then determines the amplification factor $\amp$, are provided by two interface conditions.  Choices for these interface conditions are discussed in the subsections below.

% % \bigskip\noindent
% % \textcolor{green}{Note: I have chosen the wording above since the two interface conditions don't actually determine the two free constants, but rather they determine $\amp$ and a relationship between the constants.  I believe the constants would still be arbitrary to within a multiplicative constant.}

% % --------------------------------------------------------------------------------------------------------
% \subsection{AMP interface conditions} 
% Imposing the AMP interface conditions in~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC} with the formula for the interface velocity in~\eqref{eq:1dVelocityBC} gives
% % The AMP Robin boundary condition for $\sigma$ is~\eqref{eq:1dSigmaBC} which gives
% % follows from~\eqref{eq:AddedMassPressureBC}.
% % A first-order approximation is 
% % \begin{align}
% %   \sigma^{n+1} + \frac{\zb\dt}{\rho} \sigma_y^{n+1} &= \sigmas_{22,1}^{n+1} + \zb\vs_1^{n+1} - \zb v^{I,n}
% %                                            = b_1^{n+1} -\zb v^{I,n}, \qquad\text{for $y=0$}, \label{eq:1dSigmaBC}
% % \end{align}
% % where we have introduced the interface velocity $v^{I,n}$.
% % This gives,
% % \begin{align}
% % &  \sigma^{I,n+1} = \eta\Big( b_1^{n+1} - \zb v^{I,n}\Big), \\
% % & v^{I,n+1}  = \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \\
% % &  a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}, 
% % \end{align}
% \begin{align}
% &  \amp\sigmaHat^{I} = \eta\left( \amp\bHat_1 - \zp \vHat^{I}\right), \label{eq:AmpSigmaHat} \\
% &  \aHat_0 = \sigmaHat^{I} - \zp \vHat^{I} , \label{eq:AmpaHat} \\
% &  \vHat^{I}  = \gamma \vHat(0) + \frac{1-\gamma}{\zp}( \bHat_1 - \sigmaHat^{I} ), \label{eq:AmpvHatI}
% \end{align}
% where
% \begin{align*}
%  & \eta \equiv \frac{1}{1 + \frac{\zp\kk\dt}{\rho}\coth(\kk H)}  = \frac{1}{1 + \frac{\rhos\lx}{\rho}\coth(\kk H)}. 
% \end{align*}
% From~\eqref{eq:vHatEqn} and~\eqref{eq:AmpSigmaHat} we also have
% \begin{align}
%   (\amp-1) \vHat(0) = \frac{1-\eta}{\zb}(\amp \bHat_1 - \zb\vHat^I). \label{eq:AmpvHat} 
% \end{align}
% Using $\bHat_1=Q\phis \aHat_0$ to eliminate $\bHat_1$ in terms of $\aHat_0$ and using~\eqref{eq:AmpSigmaHat} to
% eliminate $\sigmaHat^{I}$, equations~\eqref{eq:AmpaHat}, \eqref{eq:AmpvHat} and~\eqref{eq:AmpvHatI} can be written
% in the form 
% %- The interface velocity follows from~\eqref{eq:1dVelocityBC}, giving 
% %- \begin{align}
% %- %    v^{I,n+1} &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( \zb\vs_1^{n+1} + \sigma_{22,1}^{n+1} - \sigma^{I,n+1} ), \\
% %- v^{I,n+1}   &= \gamma v^{n+1}(0) + (1-\gamma)\frac{1}{\zb}( b_1^{n+1} - \sigma^{I,n+1} ), \label{eq:1dVelocityBCb}
% %- \end{align}
% %- where $\gamma=\zf/(\zf+\zb)$.
% %- For the final interface condition we set the incoming characteristic variable in the solid using the interface
% %- stress and velocity, 
% %- \begin{align}
% %-   a_0^{n+1} = \sigma^{I,n+1} - \zb v^{I,n+1}. \label{eq:1dSolidBCb}
% %- \end{align}
% % addedMass.mample : 
% % M := Matrix( [ [ A*(1-eta*Q*phim) , 0   , eta+A] , 
% %                [ (1-eta)*A*Q*phim , 1-A , -(1-eta) ], 
% %                [ -(1-g)*(1-eta)*Q*phim    , -g   , 1-(1-g)*eta/A ] ] );
% %
% %-The equations defining the AMP approximation can thus be written in the form
% \begin{align}
% \begin{bmatrix}
%    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
%    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
%   -(1-\gamma)(1-\eta)Q\phis  & -\gamma &  1-(1-\gamma)\eta \amp^{-1} 
% \end{bmatrix} 
% \begin{bmatrix} \aHat_0 \\ \zb \vHat(0) \\ \zb\vHat^I \end{bmatrix} =0 .  \label{eq:AMPmatrix}
% \end{align}
% The determinant of the matrix in~\eqref{eq:AMPmatrix} must be zero for non-trivial solutions to exist, and this leads to the following equation for $\amp$:
% \begin{align*}
% %    \tilde{f(\amp) :=& 
%    \big(\amp-(1-\gamma)\big) \left(\amp-\eta - \big( (2\eta-1)\amp -\eta \big)Q \phis\right) =0.
% \end{align*}
% % For $0\le \gamma\le 2$ the root $A=1-\gamma$ has magnitude less than or equal to one.
% Since $\amp-(1-\gamma)\ne0$ when $\vert\amp\vert>1$ and $0\le \gamma\le 2$, we have the following result.
% % --------------------------------------------------------------------------------------------------
% \begin{theorem} \label{th:amp1d}
% The AMP interface approximation to the
% scheme~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary
% conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, interface
% conditions~\eqref{eq:1dSigmaBC} and~\eqref{eq:1dSolidBC}, and interface
% velocity~\eqref{eq:1dVelocityBC} is weakly stable if and only if $0\le \gamma\le 2$ and there are no roots $\amp$ with $\vert \amp\vert>1$ to the equation
% \begin{align}
%    f(\amp) \equiv& \amp -\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis =0. \label{eq:fAMP}
% \end{align}
% \end{theorem}
% \noindent Note that $f(\amp)$ does not depend on $\gamma$, i.e.~the weighting in the definition of the interface velocity, and thus the stability of the scheme is independent of $\gamma$ provided $0\le \gamma\le 2$.  From a numerical conditioning point of view, however, we recommend the choice $\gamma=\zf/(\zf+\zp)$ as used in~\eqref{eq:1dVelocityBC}.


% %
% %- 
% %- \begin{align}
% %- &  A \sigma^{I} = \eta\Big( A \bHat_1 - \zb v^{I}\Big), \label{eq:AddedMassSigmaI} \\
% %- % &  \aHat_0 = \sigmasHat_0 - \zb \vsHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- &  \aHat_0 = \sigma^{I} -\zb v^{I}, \\
% %- & (A-1)\vHat(0)= \frac{1-\eta}{\eta\zb} A \sigma^{I}, \\
% %- & v^{I} = \gamma \vHat(0) + (1-\gamma)\frac{1}{\zb}( \bHat_1 - \sigma^{I} )
% %- % &  b^{I,n+1}= b_1^{n+1},  ~~\text{(first order approximations)}, 
% %- \end{align}
% %- Using the expressions for $b_1^n$, etc. 
% %- lead to the conditions
% %- \begin{align}
% %- &  A(1-\eta Q\phis)\aHat_0 + (\eta+A) (\zb\vHat^I) =0 ,   \\
% %- & (A-1)(\zb\vHat(0)) -(1-\eta) A Q \phis \aHat_0 + (1-\eta) (\zb \vHat^I) = 0, \\
% %- & (1 - (1-\gamma)\eta A^{-1}) (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(1-\eta) Q \phis\aHat_0 = 0. 
% %- % & (\zb\vHat^I) - \gamma (\zb\vHat(0)) - (1-\gamma)(Q-1)\half\phis \aHat_0=0. 
% %- \end{align}
% %- This is an eigenvalue problem for $\amp$. 
% %- Taking the determinant of the associated matrix leads to 
% %- \begin{align}
% %- & f(\amp) \equiv
% %- \det
% %- \begin{bmatrix}
% %-    \amp(1-\eta Q\phis)            & 0      & \amp+\eta \\
% %-    (1-\eta)\amp Q \phis           & 1-\amp    & \eta-1 \\
% %-    \half(1-\gamma)(Q-1) \phis  & \gamma & -1 
% %- \end{bmatrix} =0,\\
% %- & f(\amp)=  \amp(1-\eta Q\phis) \Big( 1-\amp +\gamma(1-\eta)\Big) + 
% %-          (\amp+\eta)\phis\Big(  \gamma(1-\eta)\amp Q - \half(1-\amp)(1-\gamma)(Q-1)   \Big) .
% %- \end{align}
% %-The scheme is unstable if there are solutions to $f(\amp)=0$ with $\vert\amp\vert>1$. 
% %-The scheme is said to be (weakly stable) at particular values of $\lambdax,\lambday,\gamma$
% %-if there are no roots with $\vert\amp\vert>1$. Given a choice for $\gamma$ we can plot the
% %-region of stability in the $(\lambdax,\lambday)$ plane. 


% \paragraph{Reduction to a polynomial equation for $\amp$} To examine the stability of the AMP algorithm we must consider all solutions of $f(\amp)=0$.  The function $f(\amp)$ in~\eqref{eq:fAMP} involves square roots of $\amp$ through the eigenvalues, $\phis$ and $\phib$, of the matrix $K$ in~\eqref{eq:recursion} and the definition of $Q$ in~\eqref{eq:Qdef}.  
% To ensure that all possible solutions are found, 
% a polynomial $P(\amp)$ can be derived whose roots include
% all the roots of $f(\amp)$.  To this end, 
% note that from the definition for $Q$ and $\phis\phib=1$ it follows that 
% \begin{align*}
%   Q\phis = \frac{1-R\phis}{\theta}.
% \end{align*}
% Thus $f$ is a linear function of $\phis$ since $f$ only depends on the product $Q\phis$. 
% Note 
% also that $Q\phis$ is a rational function of $\amp$ according the definitions of $R$ and $\theta$ in~\eqref{eq:RandTheta}.  
% Thus, $f(\amp)=0$ can be written in the form
% \begin{align*}
%     \phis = F(\amp) ,
% \end{align*}
% where $F$ is a rational function of $\amp$. 
% Since $\phis$ is equal to one of the two eigenvalues, $\phi_\pm$, defined in~\eqref{eq:phipm}, it follows that 
% \begin{equation}
%   \pm \sqrt{ B^2 - 1} = F(\amp)-B,
% \label{eq:Fratio}
% \end{equation}
% where the sign in front of the square root is chosen to be consistent with $\vert\phis\vert<1$.
% % \old{where the sign in front of the square root is chosen based on the assignment of $\phis$ so that $\vert\phis\vert<1$.}
% Upon squaring both sides of~\eqref{eq:Fratio}, which introduces new roots, one obtains
% %  
% %  Since $\phis$ also satisfies a quadradic equation
% %  with coefficients that are polynomials of $A$, 
% %  \begin{align}
% %   (\amp-1)^2 R \phis^2 - (\amp-1)^2 R B \phis + (\amp-1)^2 R=0,
% %  \end{align}
% % we can eliminate $\phis$ to derive a higher degree polynomial satisfied by $A$,
% \begin{equation}
%    P(\amp)=0,
% \label{eq:PAMP}
% \end{equation}
% where $P(\amp)$ is a polynomial (as described below).  We have thus shown the following:
% \begin{proposition}
%   Any solution of $f(\amp)=0$ is also a root of the polynomial $P(\amp)$. 
% \end{proposition}
% All of the roots of $P(\amp)$ can be found numerically using well-developed
% algorithms (e.g.~solving the eigenvalue problem for the companion matrix).  
% In
% deriving $P(\amp)$, however, new roots have been introduced. Therefore, each
% root $\amp^*$ of $P(\amp)$ must be checked to ensure that it is also solution of
% $f(\amp)=0$.
% % To do this we set $\phis=\phi_-(\amp_0)$ if $\vert\phi_-(\amp_0)\vert<1 $ otherwise we set $\phis=\phi_+(\amp_0)$,
% % and then check that $f(\amp_0)=0$. 
% \begin{proposition}
%   A root, $\amp^*$, of $P(\amp)$ is also a root of $f(\amp)$, if $\phis$ in the definition of $f$ satisfies
% \begin{equation*}
%     \phis = \begin{cases}
%                 \phi_-(\amp^*) & \text{if $\vert\phi_-(\amp^*)\vert<1 $}, \\
%                 \phi_+(\amp^*) & \text{otherwise} ,
%             \end{cases}
% \end{equation*}
% and if $f(\amp^*)=0$.
% \end{proposition}
% % \begin{align}
% %    P(\amp)=0, \quad f(\amp)=0, \quad \vert\phis(\amp)\vert<1. 
% % \end{align}
% % {\bf Scheme 1:} Taking $\gamma=1$ (interface velocity from the fluid), gives (removing a factor of $2\amp$)
% % ff := phim Q A - eta - 2 eta Q phim A + eta Q phim + A
% % 
% \newcommand{\Pamp}{P_{\rm AMP}}
% The polynomial in~\eqref{eq:PAMP} is (after removing uninteresting factors of $\amp-1$) a polynomial of degree 5 given by 
% \[
% \Pamp(\amp)=\alpha_5\amp^5+\alpha_4\amp^4+\alpha_3\amp^3+\alpha_2\amp^2+\alpha_1\amp+\alpha_0,
% \]
% where the coefficients in the polynomial are
% \[
% \begin{array}{l}
% \alpha_0=-\eta^2+2 \eta^2 \ly, \smallskip\\
% \alpha_1=-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2, \smallskip\\
% \alpha_2=10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly, \smallskip\\
% \alpha_3=-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2, \smallskip\\
% \alpha_4=3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2, \smallskip\\
% \alpha_5=-1+2 \eta.
% \end{array}
% \]
% %\begin{align*}
% %%  f_1(\amp) :=&  A-\eta - \Big( (2\eta-1)\amp -\eta \Big)Q \phis, \\
% % \Pamp(\amp) =&  (-1+2 \eta) A^5+(3-2 \ly-2 \eta^2-\lx^2+4 \eta \ly-6 \eta+2 \eta \lx^2) A^4+\\
% %&    (-2 \ly \lx^2-2 \eta \lx^2+4 \ly+\lx^2+4 \eta \ly \lx^2+7 \eta^2-3+6 \eta-4 \eta^2 \ly-8 \eta \ly-2 \eta^2 \ly \lx^2-2 \lx^2 \eta^2) A^3+\\
% %&    (10 \eta^2 \ly-9 \eta^2+1+3 \lx^2 \eta^2+4 \eta \ly-2 \eta-2 \ly) A^2+(-8 \eta^2 \ly+5 \eta^2-\lx^2 \eta^2) A\\
% %&    -\eta^2+2 \eta^2 \ly .
% %\end{align*}
% It turns out that $\Pamp(\amp)$ is the same polynomial generated by the Maple symbolic algebra program when asked to solve $f(\amp)=0$.

% To determine if there are any roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$, we
% evaluate the roots numerically for an array of parameter values in the region
% $0<\lx<1.2$, $0<\ly<1.2$ and $0\le \eta \le 1$ with $N_\amp$ equally spaced
% points in each parameter direction.  The stability region of the scheme is the
% region in the space of $(\lx,\ly,\eta)$ where the magnitude of the largest
% valid root satisfies $\vert\amp\vert\le 1$.  This region is computed on a grid with
% $N_\amp=800$ points for each parameter.  In
% Figure~\ref{fig:acousticSolidStokestability}, we plot the curve in the
% $(\lx,\ly)$ plane for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  (The
% curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is also plotted for
% reference.)  Observe that the region of stability contains the region
% $0\le\eta\le1$ and $\lx^2 + \ly^2 \le \kappa^2$
% (for $\lx\ge0$ and $\ly\ge 0$) where the maximum value for $\kappa$ appears to be $\kappa=1$. 
% Further evidence for $\kappa=1$ being the upper bound is provided by the restriction of the analysis to one dimension given below.
% % \old{, where $\kappa$ is a positive constant strictly less than 1.  }
% The curve $\lx^2 + \ly^2 = (.99)^2$
% is shown in the figure as an example.  Since $\lx=\cp\kx\dt$ and $\ly=\cp\dt/\dy$,
% the condition $\lx^2+\ly^2\le 1$ implies the following result.

% % To determine if there are any roots of $\Pamp(\amp)=0$ with $\vert\amp\vert>1$ we evaluate the roots numerically for 
% % values of $\lambda$, $\lambdax$ and $\eta$ in the ranges $0<\lambda<1$, $0<\lambdax<1$, and $0\le \eta \le 1$.
% % We choose $M$ equally spaced values of each of $\lambda$, $\lambdax$ and $\eta$ over their ranges, resulting
% % in finding the roots for $M^3$ points. Using Maple we computed roots with $M=50$ and $M=100$ and using $20$ digits of precision.
% \begin{theorem}
% By numerical evaluation of the stability polynomial, $\Pamp(\amp)$,
% we have found that the AMP algorithm is weakly stable (i.e.~there are no valid roots of $\Pamp(\amp)$ with $\vert\amp\vert>1$) 
% provided $\lx^2+\ly^2\le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{1}{\cp}\left[ \frac{1}{\dy^2} + \kx^2 \right]^{-1/2}. 
%  \end{align*}
% % where $0\le\kappa<1$. 
% This is a sufficient but not a necessary condition. 
% \end{theorem}
% Note that the time step $\dt$ satisfies a typical CFL constraint arising from the fastest wave speed in the solid.
% In the incompressible limit when $\cp \rightarrow \infty$, the maximum stable $\dt$ would go to zero,
% as it would for the solid in isolation. For incompressible solids, alternative formulations should be considered.
% Developing AMP algorithms for incompressible solids is a subject for future work. 

% % \noindent{\bf Note 1:} There are generally four valid roots to $\Pamp(\amp)=0$.
% % Figure~\ref{fig:acousticSolidStokestability} shows a plot of the computed stability region.

% {
% % ---- from codes/cauchy.m  (and cauchy.maple) ----
% \newcommand{\figWidth}{8cm}
% \begin{figure}
% \begin{center}
% %   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP_num50}
%   \includegraphics[width=\figWidth]{fig/FSI_Stability_AMP}
%   \caption{Stability region for the two-dimensional model problem using the AMP algorithm.  The curve marked 1 is the curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1$.  The curve for which $\max_{0\le\eta\le1}\vert\amp\vert=1.1$ is shown for reference.  The dashed curve shows the curve $\lx^2+\ly^2=(.99)^2$.}
%   \label{fig:acousticSolidStokestability}
% \end{center}
% \end{figure}
% }


% % \noindent{\bf Note 2:} The scheme is found to be unstable for $\lambda>1$. Note, however, that the stability bound
% % derived in Section~\ref{} for a periodic strip in $y$ is somewhat more restrictive than the bound found here
% % for the seimi-infinite strip. For example, the periodic strip is unstable for $(\lambda,\lambdax)=(.9,9.)$.

% % {\bf TO-DO: Check the $\eta=0$ limit -- decoupled solid -- we should get von-Neumann stability bound.}

% % --------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% The stability of the one-dimensional version of the AMP algorithm 
% % \old{(described previously in Section~{\bf ?????})}
% may be examined by considering the special case of the two-dimensional algorithm with $\lx=0$ and $Q=0$.  In this case there are two solutions of $f(\amp)=0$ given by
% \begin{align*}
%    \amp = 1-2\ly \qquad\text{or}\qquad \amp =\eta. % \label{eq:fAMP1D}
% \end{align*}
% We are interested in whether there are solutions with $\vert\amp\vert>1$.  Since $0\le \eta\le 1$ we have the result.
% \begin{theorem}
% The one-dimensional AMP algorithm is weakly stable provided  $0\le\gamma\le 2$ and $0 \le \ly \le 1$, i.e.
%  \begin{align*}
%     \dt \le \frac{\dy}{\cp}. 
%  \end{align*}
% \end{theorem}

% % \noindent{\bf Note 2:} Even though there are no roots $\vert\amp\vert>1$ to $\Pamp$ for even larger values of $\lambda$ and $\lambdax$,
% %   the orginial scheme should respect the time step restriction from the solid scheme 
% % {\bf But why? Does some assumption go bad? e.g. $\vert\phis\vert<1$?}


% For comparison, we now discuss briefly the corresponding stability results for the scheme given by~\eqref{eq:aEqn}--\eqref{eq:sigmaEqn} with boundary conditions~\eqref{eq:BCtop} and~\eqref{eq:BCbottom}, and with interface conditions given by either the 
% traditional (TP) algorithm or the anti-traditional algorithm.



% % ==========================================================================================================
% \subsection{TP interface conditions} \label{sec:TPanalysis}
% % \newcommand{\Mr}{\Mc}% mass ratio

% The interface conditions for the TP algorithm are given by~\eqref{eq:1dTradv} and~\eqref{eq:1dTradsigma}.  
% Following the previous analysis, $\amp$ is found to satisfy 
% \begin{align}
% &   f_{{\rm TP}}(\amp) \equiv \amp(Q+1) - \frac{\eta-1}{\eta} (\amp-1)(Q-1)\phis =0 . \label{eq:traditionalSchemeF}
% % &   \mr \equiv \frac{\zb\dt\kx}{\rho\tanh(\kx H)} = \frac{\eta-1}{\eta} ...
% \end{align}

% % {\bf TO-DO} The stability region for this scheme is computed numerically and shown in Fig.~\ref{??}.
% % We could plot the stability regions for fixed values of $\eta$ and show that as $\eta\rightarrow 1$ the
% % stability region shrinks to nothing. This shows that as $\dt\rightarrow 0$ ($\eta\rightarrow 1$) the
% % scheme is unstable. 


% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 

% In one dimension, the condition in~\eqref{eq:traditionalSchemeF} reduces to the polynomial equation
% \begin{align*}
% P_{{\rm TP}}(\amp) = \amp^2 + (\Mr + \ly-1) \amp - \Mr = 0, \quad\text{where}~~
%   \Mr = \frac{\rho H}{\rhos \dy}.
% \end{align*}
% (Here, all of the roots of this quadratic are valid since no spurious roots were introduced in deriving the equation.)  The product of the roots is $-\Mr$ and thus a necessary condition for stability is that $\vert \Mr\vert\le 1$.
% Thus the mass of the solid in a thin strip one grid cell wide, $\rhos\dy L$, 
% must be larger than the mass of the entire fluid domain $\rho H L$. 
% Using the theory of von Neumann polynomials~\cite{Miller1971,Strikwerda89} one can show the following necessary and
% sufficient condition.  
% % {\bf (It is a little unclear to me how $\Delta y$ appears.) WDH: Multiply the expression below with $\cp/\dy$ and $\lambda$ and $\Mr$ appear. }
% % ---------------------------------- THEOREM -------------------------------------------------
% \begin{theorem} \label{lemma:traditional}
% The one-dimensional TP algorithm is weakly stable if and only if 
% \begin{align*}
% %      \Mr = \frac{\rho H}{\rhos \dy} <1, \\
%      \dt \le \frac{2}{\cp}\Big( \dy - \frac{\rho H}{\rhos} \Big). 
% %      \lambda < 2(1-\Mr). 
% \end{align*}
% \end{theorem}
% This is a curious result.  For a given {\em large} value of $\dy$ the one-dimensional scheme may be stable, but it will eventually become unstable as the mesh is refined and $\dy$ becomes less than $(\rho H)/\rhos$.  The one-dimensional TP algorithm is thus formally {\em unconditionally unstable}.  
% The numerical results in Section~\ref{sec:travelingWaveResults} show that this behaviour also holds for 
% the second-order accurate discretization of the two-dimensional model problem MP-VE.
% % This behaviour of the traditional scheme is also found to hold in the two-dimensional
% %  since as the mesh is refined eventually $\dy$ will be less than $\frac{\rho H}{\rhos}$. 


% % --------------------------------------------------------------------------------------------------------
% \subsection{Anti-traditional interface conditions} \label{sec:ATPanalysis}

% The interface conditions for the anti-traditional algorithm are given by~\eqref{eq:1dAntiTradsigma} and~\eqref{eq:1dAntiTradv}.  The analysis for this choice leads to the constraint
% %These can be written as 
% %\begin{align*}
% %&  \sigmaHat^I = \sigmasHat_{22,1}= \half(Q+1)\phis\aHat_0, \\
% %&  \aHat_0 = \sigmaHat^I -\zb\Big( \frac{\kk\dt}{\rho}\coth(\kk H)\frac{\amp}{\amp-1} \Big)\sigmaHat^I, 
% %\end{align*}
% % The anti-traditional scheme takes the interface velocity from the fluid and the interface
% % stress from the solid,
% % \begin{align}
% % &   \vHat^I = \vHat(0) = \frac{1-\eta}{\eta}\frac{1}{\zb} \frac{\amp}{\amp-1} \sigmaHat^I, \\
% % &   \sigmaHat^I = \sigmasHat_1 = \half(Q+1) \aHat_0, \\
% % &   \aHat_0 = \sigmaHat^I - \zb \vHat^I = (1- \frac{1-\eta}{\eta}\frac{\amp}{\amp-1}) \half(Q+1) \aHat_0.
% % \end{align}
% % ese interface conditions lead to the eigenvalue equation for $\amp$ of 
% %which leads to the eigenvalue equation for $\amp$ of 
% \begin{align}
% &   f_{{\rm AT}}(\amp) = 1- \amp + \half\left( \frac{2\eta-1}{\eta} \amp -1 \right) (Q+1)\phis=0 .  \label{eq:antiTraditional2d}
% \end{align}

% % --------------------------------------------------------------------------------------------------------
% \paragraph{Restriction to one space dimension} 
% In one dimension, \eqref{eq:antiTraditional2d} reduces to the polynomial constraint
% \begin{align*}
% %      \amp^2 + ( \frac{\lambda}{2\eta} -2)\amp + 1-\frac{\lambda}{2} = 0.  \\
%      P_{{\rm AT}}(\amp) = \amp^2 + \left( \frac{\ly}{2}\left(1+\frac{\ly}{\Mr}\right) -2\right)\amp + 1-\frac{\ly}{2} = 0.  
% %     \amp^2 + (  \frac{\lambda}{2} + \frac{\lambda^2}{2\Mr} -2)\amp + 1-\frac{\lambda}{2} = 0. 
% \end{align*}
% % The anti-traditional scheme is weakly stable in one-dimension if and only if the following conditions
% %  are satisfied (**CHECK ME**)
% %  \begin{align}
% %  &    \lambda < 4, \\
% %  &    \frac{\lambda^2}{2\Mr} < 4-\lambda. 
% %  \end{align}
% %  where $\Mr = \frac{\rho H}{\rhos \dy}$. {\bf TO-DO:} $\Mr$ depends on $\dy$ so we really need to find the condition on $\dt$ in terms of $\dy$.
% An analysis of the roots of $P_{{\rm AT}}(\amp)$ leads us to the following result:
% \begin{theorem}
%   The one-dimensional anti-traditional algorithm is weakly stable if and only if $\ly\le 4$ and 
% % \begin{align}
% % %    \lambda \le \sqrt{ 8\Mr + \Mr^2  } -       \Mr     =       \Mr     \Big( \sqrt{ 1+\frac{8 }{\Mr}} -1 \Big). \\
% %     \half G \dt^2 + \dt < \frac{4\dy}{\cb}, \qquad G=\frac{\rhos\cb}{\rho H}
% % \end{align}
% % or 
% \begin{align}
% %    \dt  < \frac{ \sqrt{1+\frac{8\rhos}{\rho H} \dy} -1 }{G}, \qquad G=\frac{\rhos\cb}{\rho H} . \\
%    \dt  \le \frac{\dy}{\cp}\left( \sqrt{\Mr^2+8\Mr}-\Mr \right).   \label{eq:ATStability}
% \end{align}
% \end{theorem}

% We observe that the one-dimensional anti-traditional scheme is (weakly) stable for any value of the added-mass ratio $\Mr=(\rho H)/(\rhos \dy)$ provided that $\dt$ is taken sufficiently small. 
% The anti-traditional scheme is thus a stable alternative to the AMP scheme. However, in the {\em heavy solid} regime 
% when $\Mr$ is small, the anti-traditional requires a smaller $\dt$ than the AMP scheme, scaling
% like $\sqrt{8\Mr}$ for $\Mr\ll 1$,  as can be seen from~\eqref{eq:ATStability}.



==> texFiles/backup/beamInAChannel.tex <==
\section{Results for solid beam in a channel}

Consider the flow of an incompressible fluid past a solid deformable beam.


{% ------------------------------------------
\newcommand{\figWidth}{8.cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.25}{.25}}
\newcommand{\figWidtha}{6.5cm}
\newcommand{\trimfiga}[2]{\trimw{#1}{#2}{.0}{.0}{.1}{.0}}
\begin{figure}[htb]
\begin{center}
\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.5) rectangle (16.,6.);  % set the bounding box (so we have less surrounding white space)
%
%   \draw(8.0,7) node[anchor=south,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/risingBodyCompareYb}{\figWidthA}};
%%  \draw(8.0,7) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/fallingBodyAnimation1}{\figWidth}};
%
  \draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{beamInAChannel/bilcInsSmt5p5Grid}{\figWidtha}};
  \draw(7.5,1) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{beamInAChannel/bilcInsSmt5p5streamLines}{\figWidth}};

%
% grid:
%  \draw[step=1cm,gray] (0,.5) grid (16,6);
\end{tikzpicture}
}% END resize box
\end{center}
  \caption{Incompressible flow past an elastic solid beam.
 }
  \label{fig:beamInAChannel}
\end{figure}
}


{% ------------------------------------------
\newcommand{\figWidth}{8.cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.25}{.25}}
\newcommand{\figWidtha}{6.5cm}
\newcommand{\trimfiga}[2]{\trimw{#1}{#2}{.0}{.0}{.05}{.0}}
\begin{figure}[htb]
\begin{center}
\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.5) rectangle (16.,6.);  % set the bounding box (so we have less surrounding white space)
%
%   \draw(8.0,7) node[anchor=south,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/risingBodyCompareYb}{\figWidthA}};
%%  \draw(8.0,7) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/fallingBodyAnimation1}{\figWidth}};
%
%  \draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{beamInAChannel/bilcInsSmt5p5Grid}{\figWidtha}};
  \draw(7.5,1) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{beamInAChannel/thinBeamInAChannelStreamlines}{\figWidth}};

%
% grid:
%  \draw[step=1cm,gray] (0,.5) grid (16,6);
\end{tikzpicture}
}% END resize box
\end{center}
  \caption{Incompressible flow past a thin elastic solid beam.
 }
  \label{fig:thinBeamInAChannel}
\end{figure}
}


==> texFiles/backup/conclusions.tex <==
\section{Conclusions} \label{sec:conclusions}


==> texFiles/backup/deformingChannel.tex <==
\section{Results for a deforming channel}


% ----------------------------------------------------------------------------------
\subsection{Elastic-piston: slipWalls}

We consider a initially rectangular shaped elastic solid on top of a rectangular fluid channel.

\medskip
\noindent Notes
\begin{enumerate}
  \item Fluid: slip walls on left and right.
  \item Solid: slip walls on left and right.
  \item Solid: $\rhos=100$, $\lambda=\mu=1$. 
  \item Ramped pressure at bottom.
  \item Solid undergoes a repeating compression and expansion that slowly decays
\end{enumerate}


\input texFiles/deformingChannelSlipWallsGridsFig.tex




% ----------------------------------------------------------------------------------
\clearpage
\subsection{Fixed ends}

In this example the side walls are no-slip for the fluid and zero-displacement for the solid.


\input texFiles/deformingChannelNoSlipWallsGridsFig.tex


==> texFiles/backup/deformingChannelNoSlipWallsGridsFig.tex <==
{% ------ DEFORMING CHANNEL - SLIP WALLS   ------
% 
% --------- START drawContour -----------
\newcommand{\drawContour}[7]{%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{deformingChannel/#2}{\figWidth}};
  % \draw(.5,.5) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #3};
  % \draw(0,0.0) node[draw,fill=white,anchor=south west,xshift=12pt,yshift=12pt] {\scriptsize #4};
  \draw(.75,.25) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #5};
 % colour bar:
%- \begin{scope}[xshift=9pt]
%-   \draw (\xcb,\ycb) node[anchor=south west,xshift=0.cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
%-   \draw (.8,0) node[anchor=north,xshift=+3pt,yshift=+2pt] {\scriptsize $#6$};
%-   \draw (4.4,0) node[anchor=north,xshift=+0pt,yshift=+2pt] {\scriptsize $#7$};
%- \end{scope}
% \draw (\xcb,\ycb) node[anchor=south west,xshift= +8pt,yshift=+1pt] {\scriptsize $#6$};
% \draw (\xcb,\ycbTop) node[anchor=south west,xshift= +8pt,yshift=-6pt] {\scriptsize $#7$};
\end{scope}
}
% --------- END drawContour -----------
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{4cm}% colour bar height
\newcommand{\xcb}{.5cm}% colour bar lower left corner
\newcommand{\ycb}{-.2cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*\real{.5}}% colour bar top label position
% \newcommand{\xLabel}{6.5cm}% label position
% \newcommand{\yLabel}{6.5cm}% label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
% ========================= DRAW ================
%
\newcommand{\figWidth}{5cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.095}{.0975}{.175}{.175}}
\begin{figure}[htb]
\begin{center}
\resizebox{14cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.4,.5) rectangle (16.,9);  % set the bounding box (so we have less surrounding white space)
%  top row: 
 \begin{scope}[yshift=4.5cm]
   \drawContour{xshift= 0.0cm}{deformingChannelPinnedG4t0p0Grids}{$p$}{$p$}{$t=0.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelPinnedG4t2p0Grids}{$p$}{$p$}{$t=2.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelPinnedG4t4p0Grids}{$p$}{$p$}{$t=4.0$}{-.026}{.719};
 \end{scope}
 \begin{scope}
   \drawContour{xshift= 0.0cm}{deformingChannelPinnedG4t5p0Grids}{$p$}{$p$}{$t=5.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelPinnedG4t6p0Grids}{$p$}{$p$}{$t=6.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelPinnedG4t9p0Grids}{$p$}{$p$}{$t=9.0$}{-.026}{.719};
 \end{scope}
% 
% grid:
% \draw[step=1cm,gray] (0,0) grid (16,9);
\end{tikzpicture}
}% end resize box
\end{center}
  \caption{Deforming channel: elastic solid on top of an incompressible fluid.}
  \label{fig:deformingChannelPinnedGrids}
\end{figure}
}


==> texFiles/backup/deformingChannelSlipWallsGridsFig.tex <==
{% ------ DEFORMING CHANNEL - SLIP WALLS   ------
% 
% --------- START drawContour -----------
\newcommand{\drawContour}[7]{%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{deformingChannel/#2}{\figWidth}};
  % \draw(.5,.5) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #3};
  % \draw(0,0.0) node[draw,fill=white,anchor=south west,xshift=12pt,yshift=12pt] {\scriptsize #4};
  \draw(.75,.25) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #5};
 % colour bar:
%- \begin{scope}[xshift=9pt]
%-   \draw (\xcb,\ycb) node[anchor=south west,xshift=0.cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
%-   \draw (.8,0) node[anchor=north,xshift=+3pt,yshift=+2pt] {\scriptsize $#6$};
%-   \draw (4.4,0) node[anchor=north,xshift=+0pt,yshift=+2pt] {\scriptsize $#7$};
%- \end{scope}
% \draw (\xcb,\ycb) node[anchor=south west,xshift= +8pt,yshift=+1pt] {\scriptsize $#6$};
% \draw (\xcb,\ycbTop) node[anchor=south west,xshift= +8pt,yshift=-6pt] {\scriptsize $#7$};
\end{scope}
}
% --------- END drawContour -----------
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{4cm}% colour bar height
\newcommand{\xcb}{.5cm}% colour bar lower left corner
\newcommand{\ycb}{-.2cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*\real{.5}}% colour bar top label position
% \newcommand{\xLabel}{6.5cm}% label position
% \newcommand{\yLabel}{6.5cm}% label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
% ========================= DRAW ================
%
\newcommand{\figWidth}{5cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.095}{.0975}{.175}{.175}}
\begin{figure}[htb]
\begin{center}
\resizebox{14cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.4,.5) rectangle (16.,9);  % set the bounding box (so we have less surrounding white space)
%  top row: 
 \begin{scope}[yshift=4.5cm]
   \drawContour{xshift= 0.0cm}{deformingChannelG4t0p0Grids}{$p$}{$p$}{$t=0.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelG4t2p0Grids}{$p$}{$p$}{$t=2.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelG4t4p0Grids}{$p$}{$p$}{$t=4.0$}{-.026}{.719};
 \end{scope}
 \begin{scope}
   \drawContour{xshift= 0.0cm}{deformingChannelG4t5p0Grids}{$p$}{$p$}{$t=5.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelG4t6p0Grids}{$p$}{$p$}{$t=6.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelG4t9p0Grids}{$p$}{$p$}{$t=9.0$}{-.026}{.719};
 \end{scope}
% 
% grid:
% \draw[step=1cm,gray] (0,0) grid (16,9);
\end{tikzpicture}
}% end resize box
\end{center}
  \caption{Deforming channel: elastic solid on top of an incompressible fluid.}
  \label{fig:deformingChannelGrids}
\end{figure}
}


==> texFiles/backup/defs.tex <==
\renewcommand{\url}[1]{}% ******** Remove URL's from bibtex entries ********
\newcommand{\citeCount}[1]{}% for citation counts papers for WDH citations
% 
\newtheorem{theorem}{Theorem}
\newtheorem{Algorithm}{Algorithm}
\newtheorem{procedure}{Procedure}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{condition}{Condition}
% \newtheorem{AMPInterfaceCondition}{AMP Interface Condition}
\newtheorem{AMPInterfaceCondition}{Interface Condition}
\newtheorem{modelProblem}{Model Problem}
\newtheorem{travelingWave}{Traveling Wave Exact Solution}

\newtheorem*{algorithmAMP}{AMP Algorithm (added-mass partitioned)}
\newtheorem*{algorithmTP}{TP Algorithm (traditional partitioned)}

\newtheorem*{ModelProblemIA}{Model Problem MP-IA}
\newtheorem*{ModelProblemVA}{Model Problem MP-VA}
\newtheorem*{ModelProblemVE}{Model Problem MP-VE}

\newcommand{\dx}{\Delta x}
\newcommand{\dy}{\Delta y}
\newcommand{\dt}{\Delta t}


% \newcommand{\kappaR}{{\rhoR\cR^2}}

\newcommand{\Dp}{D_{+}}
\newcommand{\Dm}{D_{-}}
\newcommand{\Dpx}{D_{+x}}
\newcommand{\Dmx}{D_{-x}}
\newcommand{\Dpy}{D_{+y}}
\newcommand{\Dmy}{D_{-y}}

\newcommand{\erf}{\operatorname{erf}}

    
\newcommand{\bogus}[1]{{}}

% -----Bill's common definitions-----

\newcommand{\av}{\mathbf{ a}}
\newcommand{\bv}{\mathbf{ b}}
\newcommand{\cv}{\mathbf{ c}}
\newcommand{\dv}{\mathbf{ d}}
\newcommand{\ev}{\mathbf{ e}}
\newcommand{\fv}{\mathbf{ f}}
\newcommand{\gv}{\mathbf{ g}}
\newcommand{\hv}{\mathbf{ h}}
\newcommand{\iv}{\mathbf{ i}}
\newcommand{\jv}{\mathbf{ j}}
\newcommand{\kv}{\mathbf{ k}}
\newcommand{\lv}{\mathbf{ l}}
\newcommand{\mv}{\mathbf{ m}}
\newcommand{\nv}{\mathbf{ n}}
\newcommand{\ov}{\mathbf{ o}}
\newcommand{\pv}{\mathbf{ p}}
\newcommand{\qv}{\mathbf{ q}}
\newcommand{\rv}{\mathbf{ r}}
\newcommand{\sv}{\mathbf{ s}}
\newcommand{\tv}{\mathbf{ t}}
\newcommand{\uv}{\mathbf{ u}}
\newcommand{\vv}{\mathbf{ v}}
\newcommand{\wv}{\mathbf{ w}}
\newcommand{\xv}{\mathbf{ x}}
\newcommand{\yv}{\mathbf{ y}}
\newcommand{\zv}{\mathbf{ z}}
% 
\newcommand{\Av}{\mathbf{ A}}
\newcommand{\Bv}{\mathbf{ B}}
\newcommand{\Cv}{\mathbf{ C}}
\newcommand{\Dv}{\mathbf{ D}}
\newcommand{\Ev}{\mathbf{ E}}
\newcommand{\Fv}{\mathbf{ F}}
\newcommand{\Gv}{\mathbf{ G}}
\newcommand{\Hv}{\mathbf{ H}}
\newcommand{\Iv}{\mathbf{ I}}
\newcommand{\Jv}{\mathbf{ J}}
\newcommand{\Kv}{\mathbf{ K}}
\newcommand{\Lv}{\mathbf{ L}}
\newcommand{\Mv}{\mathbf{ M}}
\newcommand{\Nv}{\mathbf{ N}}
\newcommand{\Ov}{\mathbf{ O}}
\newcommand{\Pv}{\mathbf{ P}}
\newcommand{\Qv}{\mathbf{ Q}}
\newcommand{\Rv}{\mathbf{ R}}
\newcommand{\Sv}{\mathbf{ S}}
\newcommand{\Tv}{\mathbf{ T}}
\newcommand{\Uv}{\mathbf{ U}}
\newcommand{\Vv}{\mathbf{ V}}
\newcommand{\Wv}{\mathbf{ W}}
\newcommand{\Xv}{\mathbf{ X}}
\newcommand{\Yv}{\mathbf{ Y}}
\newcommand{\Zv}{\mathbf{ Z}}

\newcommand{\collon}{:}  % note \colon already defined by someone.
\newcommand{\ff}{\tt}

% \newcommand{\lt}{{<}}
% \newcommand{\grad}{\nabla}
% \newcommand{\comma}{~~~,~~}
% \newcommand{\calo}{{\cal O}}

\newcommand{\half}{{1\over2}}

\newcommand{\Real}{{\mathbb R}}
\newcommand{\Complex}{{\mathbb C}}

\newcommand{\zerov}{\mathbf{0}}


\newcommand{\Ac}{{\mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Dc}{{\mathcal D}}
\newcommand{\Ec}{{\mathcal E}}
\newcommand{\Ic}{{\mathcal I}}
\newcommand{\Rc}{{\mathcal R}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Lc}{{\mathcal L}}
\newcommand{\Nc}{{\mathcal N}}
\newcommand{\Oc}{{\mathcal O}}

\newcommand{\deltav}{\boldsymbol{\delta}}
\newcommand{\omegav}{\boldsymbol{\omega}}
\newcommand{\tauv}{\boldsymbol{\tau}}
\newcommand{\phiv}{\boldsymbol{\phi}}
\newcommand{\psiv}{\boldsymbol{\psi}}
\newcommand{\sigmav}{\boldsymbol{\sigma}}
\newcommand{\chiv}{\boldsymbol{\chi}}


\newcommand{\grad}{\nabla}

\newcommand{\tableFont}{\scriptsize}
\newcommand{\tableFontSize}{\small}
\newcommand{\num}[2]{#1e#2} % Use this macro to define the format of the numbers in the table
\newcommand{\eem}{e^{(j)}}
\newcommand{\rateLabel}{rate}

\clearpage
\newcommand{\dtau}{\delta_\tau}
\newcommand{\Gb}{G}


\newcommand{\rhos}{\bar{\rho}}
\newcommand{\cp}{\bar{c}_p}
\newcommand{\cs}{\bar{c}_s}
\newcommand{\kappas}{{\rhos\cs^2}}
\newcommand{\zs}{{\bar {z}}}  % solid impedance based on c_p
\newcommand{\zp}{z_p}  % solid impedance based on c_s
\newcommand{\us}{\bar{u}}
\newcommand{\qs}{\bar{q}}
\newcommand{\vs}{\bar{v}}
\newcommand{\sigmas}{\bar{\sigma}}
\newcommand{\xs}{\bar{x}}
\newcommand{\xsv}{\bar{\xv}}
\newcommand{\xf}{{x}}
\newcommand{\dxs}{\Delta{\bar x}}
\newcommand{\dxf}{{\Delta x}}
\newcommand{\Ns}{\bar{N}}
\newcommand{\Nf}{{N}}
\newcommand{\zf}{z_f}

% ---- DAS definitions ---- $
% solid definition in analysis
\newcommand{\ssy}{\bar{\sigma}_{22}}
\newcommand{\ssx}{\bar{\sigma}_{21}}
\newcommand{\vsy}{\vs_{2}}
\newcommand{\vfy}{v_{2}}

% hat variables in fluid and solid (Fourier)
\newcommand{\ssyh}{\hat{\bar{\sigma}}_{22}}
\newcommand{\ssxh}{\hat{\bar{\sigma}}_{21}}
\newcommand{\vsyh}{\hat{\bar{v}}_2}
\newcommand{\vfyh}{\hat{v}_2}
% \newcommand{\ph}{\hat{p}}

% characteristic variables
% \newcommand{\ac}{\bar{a}}
% \newcommand{\bc}{\bar{b}}
% \newcommand{\dc}{\bar{d}}
\newcommand{\ac}{a}
\newcommand{\bc}{b}
\newcommand{\dc}{d}
\newcommand{\acv}{\mathbf{\ac}}

% effective fluid height
\newcommand{\Heff}{H_{\text{eff}}}

% analysis
\newcommand{\p}{\phi} % spacial eigenvalue
\newcommand{\rev}{\mathbf{r}} % spacial eigenvector
\newcommand{\qn}[1]{q_{#1}}
\newcommand{\rn}[1]{r_{#1}}

% tilde variables
\newcommand{\tac}{\tilde{\ac}}
\newcommand{\tbc}{\tilde{\bc}}
\newcommand{\tdc}{\tilde{\dc}}
\newcommand{\tacv}{\tilde{\acv}}

% determinant condition
\newcommand{\dComp}{g}
\newcommand{\dMat}{\mathcal{G}}

% environment for algorithm
\newcommand{\listAlgorithm}[2]{
\noindent \hrulefill \\
\noindent \textit{#1:}
\begin{enumerate}
#2
\end{enumerate}
\noindent \hrulefill
}

% arg min definition
\DeclareMathOperator*{\argmin}{arg\,min}



% ---------------- $


\newcommand{\usv}{\bar{\uv}}
\newcommand{\vsv}{\bar{\vv}}
\newcommand{\wsv}{\bar{\wv}}

\newcommand{\ush}{\hat{\us}}
\newcommand{\usvh}{\hat{\usv}}
\newcommand{\vvh}{\hat{\vv}}
\newcommand{\vh}{\hat{v}}
\newcommand{\ph}{\hat{p}}

\newcommand{\nsv}{\bar{\nv}}
\newcommand{\vvs}{\bar{\vv}}
\newcommand{\uvs}{\bar{\uv}}
\newcommand{\xvs}{\bar{\xv}}
\newcommand{\sigmavs}{\bar{\sigmav}}
\newcommand{\sigmasv}{\bar{\sigmav}}
\newcommand{\fsv}{\bar{\fv}}
\newcommand{\qsv}{\bar{\qv}}

\newcommand{\qsvp}{\qsv^p}
\newcommand{\qsvI}{\qsv^I}
\newcommand{\qvI}{\qv^I}

\newcommand{\vvI}{\vv^I}
\newcommand{\tauvI}{\tauv^I}
\newcommand{\vvIf}{\vv^f}
\newcommand{\tauvIf}{\tauv^f}
% \newcommand{\vvIf}{\vv^{I,f}}
\newcommand{\sigmavI}{\sigmav^I}
\newcommand{\vsvIs}{\vsv^s}
\newcommand{\sigmavIs}{\sigmav^s}

\newcommand{\dvel}{{\delta_v}}
\newcommand{\vDot}{\dot{v}}
\newcommand{\vsDot}{\dot{\vs}}
\newcommand{\vvDot}{\dot{\vv}}
\newcommand{\vsvDot}{\dot{\vsv}}

% \newcommand{\rb}{r_b} % a point on the body surface

% \newcommand{\amp}{{\mathcal{A}}}
\newcommand{\amp}{A}
\newcommand{\ampI}{A} % amplification factor for iterations



% \newcommand{\Energy}{\mathcal{E}}% Energy of the fluid
% \newcommand{\Area}{\mathcal{A}_b}
% \newcommand{\Area}{A_b}
% \newcommand{\width}{\mathcal{W}}
% \newcommand{\width}{w_b}


\newcommand{\charSpeed}{s}% Char. speed
\newcommand{\charVar}{\chi}% Char. variable


\newcommand{\largess}{\sffamily\large}
\newcommand{\Largess}{\sffamily\Large}
\newcommand{\bfss}{\sffamily\bfseries}
\newcommand{\smallss}{\sffamily\small}
\newcommand{\normalss}{\sffamily}
\newcommand{\scriptsizess}{\sffamily\scriptsize}

\newcommand{\hs}{h_s}
% \newcommand{\Hs}{H_s}
\newcommand{\Hs}{\bar{H}}

\newcommand{\kxHat}{\hat{k}_x}
\newcommand{\kyHat}{\hat{k}_y}
\newcommand{\omegaHat}{\hat{\omega}}
\newcommand{\aHat}{\hat{a}}
\newcommand{\bHat}{\hat{b}}

\newcommand{\aTilde}{\tilde{a}}
\newcommand{\bTilde}{\tilde{b}}

\newcommand{\qsHat}{\hat{\qs}}
\newcommand{\phase}{x_0}
\newcommand{\phaset}{t_0}

\newcommand{\as}{\bar{a}}
\newcommand{\bs}{\bar{b}}
\newcommand{\ds}{\bar{d}}
\newcommand{\asHat}{\hat{\as}}
\newcommand{\bsHat}{\hat{\bs}}
\newcommand{\dsHat}{\hat{\ds}}

\newcommand{\dHat}{\hat{d}}
\newcommand{\pHat}{\hat{p}}
\newcommand{\qHat}{\hat{q}}
\newcommand{\vHat}{\hat{v}}
\newcommand{\vvHat}{\hat{\vv}}
\newcommand{\vsHat}{\hat{\vs}}
\newcommand{\sigmaHat}{\hat{\sigma}}
\newcommand{\sigmasHat}{\hat{\sigmas}}

\newcommand{\lambdas}{\bar{\lambda}}% solid Lame' parameter
\newcommand{\mus}{\bar{\mu}}% solid Lame' parameter

\newcommand{\OmegaF}{\Omega^F}% fluid domain
\newcommand{\OmegaS}{\Omega^S}% solid domain

\newcommand{\OmegaFh}{\Omega^F_h}% fluid domain
\newcommand{\OmegaSh}{\Omega^S_h}% solid domain

\newcommand{\GammaI}{\Gamma}% Fluid-Solid Interface
\newcommand{\GammaIh}{\Gamma_h}% Fluid-Solid Interface

\renewcommand{\zp}{\bar{z}_p}
\renewcommand{\zs}{\bar{z}_s}
\newcommand{\zb}{\bar{z}}
\newcommand{\Lt}{\tilde{L}}

\newcommand{\MR}{M_r}% added mass ratio
\newcommand{\Mr}{\mathcal{M}}% another added mass ratio
\newcommand{\Mra}{M}%acoustic mass ratio

\newcommand{\phis}{\phi_s}
\newcommand{\phib}{\phi_b}
% \newcommand{\phit}{\tilde{\phi}}
% \newcommand{\phit}{\phi_<}

\newcommand{\phim}{\phi_-}
\newcommand{\phip}{\phi_+}


\newcommand{\lambday}{\lambda}% 
\newcommand{\lambdax}{\lambda_x}% 

\newcommand{\cb}{\bar{c}}
\newcommand{\kk}{k_x} % wave number of 2d analysis
\newcommand{\kx}{k_x} % wave number of 2d analysis
\newcommand{\ax}{\alpha \amp^{m+1}}
\newcommand{\thetaj}{\theta} % Jeff's theta


% Predicted states:
\newcommand{\vvp}{\vv^p}
\newcommand{\vp}{v^p}
\newcommand{\sigmavp}{\sigmav^p}
\newcommand{\sigmap}{\sigma^p}
\newcommand{\tauvp}{\tauv^p}
\newcommand{\taup}{\tau^p}
\newcommand{\vsvp}{\vsv^p}
\newcommand{\vsp}{\vs^p}
\newcommand{\sigmasvp}{\sigmasv^p}
\newcommand{\sigmasp}{\sigmas^p}


\newcommand{\Achar}{\Ac}% incoming characteristic variable
\newcommand{\Bchar}{\Bc}% characteristic BC operator
\newcommand{\Bcharp}{\Bc_p}% characteristic BC operator

\newcommand{\Af}{A_f}
\newcommand{\Bf}{B_f}
\newcommand{\Df}{\Dc}
\newcommand{\As}{A_s}
\newcommand{\Bs}{B_s}
\newcommand{\Ds}{\bar{\Dc}}


\newcommand{\Ck}{C_k}
\newcommand{\Sk}{S_k}
\newcommand{\Ca}{C_\alpha}
\newcommand{\Sa}{S_\alpha}

\newcommand{\Sas}{S_a}
\newcommand{\Cas}{C_a}
\newcommand{\Sbs}{S_b}
\newcommand{\Cbs}{C_b}

\newcommand{\dsf}{\delta}


\newcommand{\expkw}{e^{i(k x -\omega t)}}
% \newcommand{\ampe}{\Ac_0}% amplitude of exact solution
\newcommand{\ampe}{{\bar u_{{\rm max}}}}


% \newcommand{\nus}{\bar\nu}
% \newcommand{\betas}{\bar\beta}
% \newcommand{\ly}{\ell_y}
% \newcommand{\lx}{\ell_x}
% \newcommand{\ly}{\beta_y}
% \newcommand{\lx}{\beta_x}
% \newcommand{\ly}{\alpha_y}
% \newcommand{\lx}{\alpha_x}
\newcommand{\ly}{\lambda_y}
\newcommand{\lx}{\lambda_x}
% \newcommand{\ly}{\gamma_y}
% \newcommand{\lx}{\gamma_x}

\newcommand{\tanv}{\ev}% tangent 
\newcommand{\blue}{\color{blue}}

\newcommand{\strutt}{\rule{0pt}{10pt}}% strutt to make table height bigger


==> texFiles/backup/elasticPiston.tex <==
% \newcommand{\cp}{c_p}
% \newcommand{\xI}{x_I}
\newcommand{\pH}{p_0}
\section{An exact solution for an elastic piston}

We derive an exact solution for a one-dimensional elastic piston by posing a
given motion of the interface $x=\Gb(t)$ and then determining the pressure boundary
condition on the fluid that will result in that motion.

First consider the solution to the one-dimensional IBVP for the wave equation
on strip $x\in[a,b]$,
\begin{align*}
 & \left\{
  \begin{aligned}
   \partial_t \us - \vs &=0 \\
   \rhos\partial_t \vs - \partial_{\xs} \sigmas &=0 \\
  \partial_t \sigmas - \rhos\as^2 \partial_{\xs}\vs  &=0 
 \end{aligned} 
 \right.
, ~~\text{for $\xs\in[a,b]$},  \\
& \us(a,t)=\alpha(t), \quad \us(b,t)=\beta(t), \qquad\text{(boundary conditions)}, \\
& \us(x,t)=\us_0(x), \quad \vs(x,t)=\vs_0(x), \qquad\text{(initial conditions)}.
\end{align*}
\begin{figure}[hbt]
\begin{center}
\begin{tikzpicture}[scale=1]
 \useasboundingbox (-3,-.25) rectangle (3,6);  % set the bounding box (so we have less surrounding white space)
%
  \draw[very thick] (-2,0) -- (-2,5);
  \draw[very thick] (2,0) -- (2,5);
  \draw (-2,0) node[anchor=north] {$a$};
  \draw ( 2,0) node[anchor=north] {$b$};
  \draw (-2,3) node[rotate=90,yshift=+8pt] {$\us=\alpha(t)$};
  \draw ( 2,3) node[rotate=90,yshift=-8pt] {$\us=\beta(t)$};
%
  \draw[->] (-3.5,0)--(2.5,0) node[anchor=north] {$x$};
  \draw[->] (-3.,-.2)--(-3.,6) node[anchor=east] {$t$};
% characteristics
  \draw[blue] (-2,0) -- (2,2) -- (-2,4) -- (2,6);
  \draw[red ] (2,0) -- (-2,2) -- (2,4) -- (-2,6);
%
  \draw (0,.5) node {$A$};
  \draw (-1.25,1.25) node {$B$};
%
%  \draw (-.5,2) node[anchor=south] {$(x,t)$}; 
%  \draw (-.5,2) -- (2,.75) -- (.5,0);
%  \draw (-.5,2) -- (-2,1.25) -- (.5,0);
% grid:
   \draw[step=1cm,gray] (-3,0) grid (3,.);
\end{tikzpicture}
\end{center}
\caption{Wave equation in a strip...}
\label{fig:elasticPistonCartoon}
\end{figure}
%
The solution at a point $P=(x,t)$ can be determined by tracing characteristics.
The characteristic conditions are
\begin{align*}
    w_\pm = \sigmas \mp \zp \vs = \text{const} \quad \text{along $\frac{d x}{d t}=\pm\as$},
\end{align*}
For a point $A$ in region I, the solution is determined from the two conditions
\begin{align*}
  &  w_+(x,t) = w_+(x-\as t,0) = \sigma_0(x-\as t) -\zp \vs_0(x-\as t), \\
  &  w_-(x,t) = w_-(x-\as t,0) = \sigma_0(x+\as t) +\zp \vs_0(x+\as t),
\end{align*}
which gives 
\begin{align*}
    v(x,t) = \half( \vs_0(x-\as t) + \vs_0(x+\as t)) + \frac{1}{2\as}( \sigma_0(x+\as t)-\sigma_0(x-\as t))
\end{align*}
For a point $B$ in region II, the solution is determined from the three equations
\begin{align*}
 &   w_+(x,t) = w_+(x-\as (t-\tau),\tau ) = \sigma+(x-\as (t-\tau),\tau ) -\zp \alpha(\tau), \\
 &   w_-(x,t) = w_-(x-\as t,0) = \sigma_0(x+\as t) +\zp \vs_0(x+\as t), \\
 &   w_-(x-\as (t-\tau),\tau ) = w_-(\xi,0) = \sigma_0(\xi) +\zp \vs_0(\xi)
\end{align*}

Consider a one-dimensional fluid domain $\Omega_F=[\Gb(t),H]$ adjacent to an elastic solid 
on the domain $\Omega_S=[-\Hs,\Gb(t)]$. The governing equations are
\begin{equation}
  \left\{
  \begin{aligned}
   \partial_t \us - \vs &=0 \\
   \rhos\partial_t \vs - \partial_{\xs} \sigmas &=0 \\
  \partial_t \sigmas - \rhos\as^2 \partial_{\xs}\vs  &=0 
 \end{aligned} 
 \right.
, ~~\text{for $\xs\in[-\Hs,0]$}, 
\qquad 
  \left\{
  \begin{aligned}
  \rho (\partial_t v + v \p_x v) + \p_x p &= \mu \p_x^2 v \\
  \p_x v  &=0 \\
 \end{aligned} 
 \right.
, ~~\text{for $x\in[\Gb(t),H]$} , \label{eq:elasticPiston}
\end{equation}




%
% Cartoon showing the grid for the elastic piston
%
\begin{figure}[hbt]
\begin{center}
\begin{tikzpicture}[scale=1]
 \useasboundingbox (-5.,-.5) rectangle (5,1);  % set the bounding box (so we have less surrounding white space)
%
  \filldraw[fill=red!20,line width=2pt] (-5,-.5) -- (0,-.5) -- (0,.5) -- (-5,.5) -- (-5,-.5) ;
  \draw (-2,0) node {solid};
  \filldraw[fill=blue!20,line width=2pt] ( 5,-.5) -- (0,-.5) -- (0,.5) -- (5,.5) -- ( 5,-.5);
  \draw (2,0) node {fluid};
  \draw[color=green,line width=2pt] (0,-.5) -- (0,.5);
%
  \draw (0,-.5) node[anchor=north] {$x=\Gb(t)$};
  \draw (-5,-.5) node[anchor=north] {$x=-\Hs$};
  \draw ( 5,-.5) node[anchor=north] {$x=H$};
% 
  \draw ( 5,0) node[anchor=west] {$p=\pH(t)$};
  \draw (-5,0) node[anchor=east] {$\us=0$};
% grid:
%   \draw[step=1cm,gray] (-5,-1) grid (5,1.);
\end{tikzpicture}
\end{center}
\caption{Elastic piston...}
\label{fig:elasticPistonCartoon}
\end{figure}


The solution for the pressure in the fluid domain subject to a specified pressure boundary condition at $x=H$
and the compatibility condition at $x=\Gb(t)$ together with $[v]=0$, 
\begin{align}
    p(H,t)=\pH(t), \qquad p_x(\Gb(t),t) = -\rho v_t(\Gb(t),t) = -\rho \vs_t(0,t),
\end{align}
is
\begin{align}
    p(x)= \pH(t)  -\rho \vs_t(0,t)\, ( x-H)
\end{align}


The solution to the elasticity equations with
initial conditions $\us(\xs,0)=\us_0(\xs)$ and $\partial_t \us(\xs,0) = \vs_0(\xs)$ and boundary
condition $\us(0,t)=\Gb(t)$ follows from the d'Alembert solution, ({\bf *fix me*} for BC at $\xs=-\Hs$)
\begin{align}
  \us(\xs,t) &= f(\xs-\cp t) + g( \xs+ \cp t ),  \label{eq:dAlembert}  \\
  f(\xi) &= \half\big[ \us_0(\xi)- \cp^{-1}\int_0^\xi \vs_0(s) d s\big]  ~~\text{for $\xi<0$}, \label{eq:f-solution} \\
  g(\xi) &= \begin{cases}
           \half\big[ \us_0(\xi)+ \cp^{-1}\int_0^\xi \vs_0(s) d s\big]  & \text{for $\xi<0$},  \\
           \Gb(\xi/\cp) - f(-\xi)  & \text{for $\xi>0$} .
          \end{cases} \label{eq:g-solution} 
\end{align}
% where $c_p^2 = (\lambda+2\mu)/\rhos$.
The interface traction condition, 
\begin{align*}
  \rhos\cp^2\partial_{\xs}\us(0,t) &= -p(\Gb(t),t) , \\
                                  &= -\pH(t)  + \rho \vs_t(0,t)\, ( \Gb(t) -H)
\end{align*}
determines $\pH$ as a function of the interface position $\Gb$, 
\begin{align}
  \pH(t) =  \rho \vs_t(0,t)\, ( \Gb(t) -H) - \rhos\cp^2\partial_{\xs}\us(0,t) . \label{eq:pH}
\end{align}
Thus, by choosing $\pH$ according to~\eqref{eq:pH} the interface wll undergo the motion $x=\Gb(t)$.


==> texFiles/backup/governing.tex <==
\section{Governing equations and interface conditions} \label{sec:governingEquations}

\wdh{\bf This is from fib:}

We consider a fluid-structure interaction problem in which an incompressible
fluid in a domain $\OmegaF$ is coupled to a compressible elastic solid in
a domain $\OmegaS$.  The interface where the two domains meet is assumed to be
smooth and is denoted by $\Gamma$.  For the purposes of this paper, we consider
an FSI problem consisting of small perturbations about an equilibrium state.
Thus, we assume that the nonlinear convection terms in the fluid are negligible and
the solid is linearly elastic, and we consider the problem to be linearized
about a fixed interface position.  We also neglect the effects of gravity or other body forces.
Under these assumptions, the flow in the
% \old{(fixed)}
fluid domain is governed by the linear Stokes equations
\begin{alignat}{3}
  &  \rho\frac{\partial\vv}{\partial t} 
                 =  \grad\cdot\sigmav  , \quad&& \xv\in\OmegaF ,  \label{eq:stokes3d} \\
  & \grad\cdot\vv =0,  \quad&& \xv\in\OmegaF ,  \label{eq:fluidDiv3d}
\end{alignat}
where $\xv$ is position, $t$ is time, $\rho$ is the (constant) fluid density, and $\vv=\vv(\xv,t)$ is the fluid velocity.
% \old{and $\fv=\fv(\xv,t)$ is a (given) body force.}  
In the linearized approximation, the Eulerian fluid domain $\OmegaF$ does not deform and remains fixed in time.
The fluid stress tensor, $\sigmav=\sigmav(\xv,t)$, is given by 
\begin{equation}
  \sigmav = -p \Iv + \tauv,\qquad \tauv = \mu \left[ \grad\vv + (\grad\vv)^T \right],
  \label{eq:fluidStress}
\end{equation}
where $p$ is the pressure, $\Iv$ is the identity tensor, $\tauv$ is the viscous stress tensor, and $\mu$ is the (constant) fluid viscosity. 
For future reference, 
the components of a vector, such as $\vv$ will be denoted by $v_m$, $m=1,2,3$, (i.e. $\vv=[v_1, v_2, v_3]^T$), while components
of a tensor such as $\sigmav$, will be denoted by $\sigma_{mn}$, $m,n=1,2,3$.
In the 
%\old{(fixed)} 
solid domain, the solid displacement $\usv=\usv(\xv,t)$ and velocity $\vsv=\vsv(\xv,t)$ are governed by 
\begin{alignat}{3}
  \frac{\partial\usv}{\partial t} &= \vsv,  \quad&& \xv\in\OmegaS , \label{eq:usFromvs} \\
  \rhos \frac{\partial\vsv}{\partial t} &= \grad \cdot\sigmasv  , \quad&& \xv\in\OmegaS , \label{eq:elasticWave}
\end{alignat}
where $\rhos$ is the (constant) solid density and $\sigmasv=\sigmasv(\xv,t)$ is the 
Cauchy stress tensor\footnote{
Over-bars on symbols are used throughout the paper to denote quantities belonging to the solid.}.
In the linearized approximation,
the Lagrangian reference coordinates for the solid are the same as the Eulerian coordinates~$\xv$.
The stress tensor is given by
\begin{align*}
  \sigmasv &= \lambdas(\grad\cdot\usv)\Iv + \mus\left[ \grad\usv + \grad\usv^T \right],
\end{align*}
where $\lambdas$ and $\mus$ are (constant) Lam\'e parameters.  The matching conditions at the fluid-solid interface $\Gamma$ are
\begin{alignat}{3}
  \vv(\xv,t) &= \vvs(\xv,t), \quad && \xv\in\Gamma,                    \label{eq:interfaceV} \\
  \sigmav(\xv,t)\nv &= \sigmavs(\xv,t)\nv, \quad && \xv\in\Gamma, \label{eq:interfaceStress}
\end{alignat}
where $\nv$ is the outward unit normal to the fluid domain.  The problem is closed by specifying initial conditions for $\vv$ in $\OmegaF$ and for $\usv$ and $\vsv$ in $\OmegaS$, and by specifying suitable conditions on the boundaries of the fluid and solid domains not included in $\Gamma$.

The elastic wave equations in~\eqref{eq:usFromvs} and~\eqref{eq:elasticWave} form a hyperbolic system with a characteristic structure and finite wave speeds.  These wave speeds, given by
\[
\bar c_p=\sqrt{\frac{\lambdas+2\mus}{\rhos}},\qquad \bar c_s=\sqrt{\frac{\mus}{\rhos}},
\]
are the propagation speeds of p-waves and s-waves, respectively, in the elastic
solid.  At the interface the equations can be locally transformed into normal
and tangential coordinates. 
By considering the 
components of the equations in the normal direction, one can define characteristics
and characteristic variables~\cite{Whitham74} that indicate the propagation of information in the direction normal to the interface.
The {\em incoming} and {\em outgoing} characteristic variables
normal to the interface are given by
\begin{alignat}{3}
 \Achar(\sigmasv,\vsv)  &  = \nv^T\sigmasv\nv  - \zp \nv^T\vsv,  \qquad&& \xv\in\GammaI \quad\text{(incoming)},  \label{eq:charA} \\
 \Achar_m(\sigmasv,\vsv)&  = \ev_m^T\sigmasv\nv - \zs \ev_m ^T\vsv, \quad m=1,2,  \qquad&& \xv\in\GammaI \quad\text{(incoming)},\\
 \Bchar(\sigmasv,\vsv)  &  = \nv^T\sigmasv\nv  + \zp \nv^T\vsv,  \qquad&& \xv\in\GammaI  \quad\text{(outgoing)}, \label{eq:charB} \\
 \Bchar_m(\sigmasv,\vsv)&  = \ev_m^T\sigmasv\nv   + \zs \ev_m ^T\vsv, \quad m=1,2, \qquad&& \xv\in\GammaI\quad\text{(outgoing)}.       \label{eq:charBm}
\end{alignat}
Here, $\zp=\rhos\bar c_p$ and $\zs=\rhos\bar c_s$ are the solid impedances for
p-waves and s-waves, respectively, and $\ev_m$, $m=1,2$ denote mutually
orthogonal unit vectors tangent to the interface.  By {\em outgoing} we mean the
characteristics that leave the solid domain through the interface, and vice versa for the {\em incoming} characteristics.


Partitioned algorithms impose the interface conditions~\eqref{eq:interfaceV} and~\eqref{eq:interfaceStress}
by defining segregated conditions for the fluid and solid domains. 
In the traditional partitioned algorithm, the interface condition
in~\eqref{eq:interfaceV} is taken to be the (Dirichlet) boundary condition for the fluid
(velocity from solid), while~\eqref{eq:interfaceStress} is taken to be the (Neumann)
boundary condition for the solid (traction from fluid).  
Alternatively, the approach we develop in this article is
based on using the incoming and outgoing solid characteristic variables
normal to the interface given in~\eqref{eq:charA}--\eqref{eq:charBm}. 
In this approach a Robin interface condition for the fluid
is defined in terms of the outgoing solid characteristic variables, namely
\begin{equation}
\Bchar(\sigmav,\vv) =\Bchar(\sigmasv,\vsv), \qquad \Bchar_m(\sigmav,\vv) =\Bchar_m(\sigmasv,\vsv), \quad m=1,2,\qquad \xv\in\Gamma,
\label{eq:AMPoutgoing}
\end{equation}
while a Robin interface condition for the solid is defined in terms of the fluid variables using the incoming characteristic variables
\begin{equation}
\Achar(\sigmasv,\vsv) = \Achar(\sigmav,\vv), \qquad \Achar_m(\sigmasv,\vsv) = \Achar_m(\sigmav,\vv), \quad m=1,2,\qquad \xv\in\Gamma.
\label{eq:AMPincoming}
\end{equation}
This, in a nutshell, is the key ingredient of the added-mass partitioned (AMP)
algorithm.  These conditions are linearly independent combinations of the
interface conditions in~\eqref{eq:interfaceV} and~\eqref{eq:interfaceStress}, and
are thus equivalent to the original conditions.


In practice, numerical computations, including those presented in Section~\ref{sec:numericalResults}, are often based on alternative forms of the governing equations.
For the case of the fluid, the equations may be written in the velocity-pressure form
\begin{alignat}{3}
  &  \rho\frac{\partial\vv}{\partial t} + \nabla p
                 =  \mu\Delta\vv  , \quad&& \xv\in\OmegaF ,  \label{eq:NS3dv} \\
  & \Delta p = 0,  \quad&& \xv\in\OmegaF . \label{eq:pressurePoisson}
\end{alignat}
We use a numerical approximation of this form of the equations to advance the fluid variables following the fractional-step method described in~\cite{ICNS}.  
As discussed in~\cite{ICNS},
an additional boundary condition is required for this form of the equations, and a suitable choice is given by
\begin{align}
  & \grad\cdot\vv =0,  \qquad \xv\in\partial\OmegaF.
\label{eq:NS3dDiv}
\end{align}
For the solid domain, we consider the equations of linear elasticity written as the first-order system
\begin{alignat}{3}
  \frac{\partial\usv}{\partial t} &= \vsv,  \quad&& \xv\in\OmegaS , \label{eq:solidDisplacement} \\
  \rhos \frac{\partial\vsv}{\partial t} &= \grad \cdot\sigmasv  , && \xv\in\OmegaS ,\label{eq:solidMomemtum}\\
  \frac{\partial\sigmasv}{\partial t} &= \lambdas(\grad\cdot\vsv)\Iv + \mus\left[ \grad\vsv + \grad\vsv^T \right],\quad && \xv\in\OmegaS , \label{eq:solidStress}
\end{alignat}
and use a numerical approximation of this form of the equations to advance the solid variables following the second-order upwind (Godunov) method discussed in~\cite{smog2012}.  


==> texFiles/backup/intro.tex <==
\section{Introduction} \label{sec:intro}



\wdh{\bf This is from fib:}

The coupled evolution of fluids and structures is of great interest in a wide range of applications
including, for example, structural engineering and biomedicine.  Such fluid-structure interaction
(FSI) problems are often modeled mathematically by suitable partial differential equations for the
fluids and structures in their respective domains, together with conditions at the boundaries of the
domains where the solutions of the equations interact.  Numerical algorithms used to solve these FSI
problems can be classified into two main categories.  Algorithms belonging to one category, called
monolithic schemes, treat the equations for the domains of the fluids and structures along with
interface conditions as a large system of evolution equations, and then advance the solutions
together.  The other category of algorithms are partitioned schemes (also known as modular or
sequential schemes), and these algorithms employ separate solvers for the fluids and structures
which are coupled at the interface.  Typically, sub-iterations are performed at each time step of a
partitioned algorithm for stability.  Strongly-coupled partitioned schemes perform multiple
iterations per time step to solve the coupled equations, while loosely coupled schemes use only one
or a few iterations.  Even though many existing partitioned schemes suffer from serious stability
issues in certain problem regimes, they are often preferred since they can make use of existing
solvers and can be more efficient than monolithic schemes.

In this paper we consider an important class of FSI problems where partitioned schemes often have
difficulty.  This class involves the coupling of incompressible fluids and relatively {\em light}
structures where {\em added-mass} effects are large.  Added-mass effects arise from the fact that
the force required to accelerate a solid structure immersed in a fluid must also account for the
acceleration of the surrounding fluid.  Partitioned schemes for this class of problem generally
suffer from poor convergence, requiring many sub-iterations per time step, or are unstable, when
added-mass effects are large.  The instabilities in partitioned schemes can be traced to the
application of the interface conditions which must also be partitioned between the fluid and solid
solvers.  The traditional partitioned algorithm uses the velocity of the solid as a boundary
condition on the fluid and the traction from the fluid as a forcing on the solid.  This is sometimes
referred to as Dirichlet-Neumann coupling with the Dirichlet condition being the assignment of the
velocity and the Neumann condition the assignment of the traction.  More generally, practitioners
have considered Robin-Robin coupling (i.e.~{\em mixed} boundary conditions for the fluid and solid)
to impose the interface conditions~\cite{BadiaNobileVergara2008}.

The central aim of the present work is to describe an added-mass partitioned (AMP) algorithm for FSI
problems involving an incompressible fluid coupled to an elastic structure.  A key feature of our
new AMP algorithm is that it is stable, even when added-mass effects are large, and it retains full
accuracy with no sub-iterations.  We discuss the algorithm and analyze its stability for two types
of structures.  In Part I of this paper, we describe the algorithm for FSI problems involving
compressible bulk solids, while in Part II, we consider problems involving elastic shells.  A common
feature of the algorithms for both types of structures is the derivation of an AMP Robin interface
condition for the fluid involving the velocity or acceleration of the interface and the stress on
it.  The version of the Robin interface condition involving the velocity, which applies for the bulk
solid case only, may be used as a boundary condition for the partitioned solver for the fluid in
velocity-divergence form.  The version of the interface condition involving the acceleration applies
for both cases, and can be used for the fluid solver in velocity-pressure form.  In the latter case,
a further manipulation of the Robin condition is carried out so that it provides a suitable boundary
condition for the pressure in a fractional-step fluid solver.  The details of the derivation of the
AMP Robin condition depends on the type of structure, whether it be an elastic solid or an elastic
shell, and this is principally where the discussion of the algorithms in the two parts of the paper,
and the corresponding stability analyses and results, differ.  For the case of a compressible bulk
solid, the AMP interface condition is obtained based on characteristic equations for the solid
applied at the interface, while for the case of the elastic shell, the interface condition is
obtained from the evolution equation for the shell itself.  This latter case is described in detail
in Part II of the paper~\cite{fis2014}.

For the present work, we focus primarily on an analysis of the stability of the AMP algorithm, and
therefore consider (linear) Stokes flow for the incompressible fluid coupled to a linearly elastic
solid.  Subsequent work will extend the AMP algorithm to fully nonlinear incompressible flow and
elastic solids with large deformation, and will be based on the foundation laid in this paper.  We
introduce various two-dimensional model problems, each with a fluid-solid interface that is
linearized about its initial position, and use these to study the behavior of the new algorithm and
compare it with existing algorithms.  A normal-mode analysis of the algorithm applied to one of the
model problems is used to show that the AMP algorithm is stable for any ratio of the fluid to solid
densities, and in particular for the case of light solids where added-mass effects are large.  In
contrast, a stability analysis of a scheme based on the traditional Dirichlet-Neumann coupling is
shown to be {\em formally} unconditionally unstable for any density ratio in the sense that the
scheme may be stable on a coarse grid but becomes unstable for a sufficiently fine
mesh\footnote{Formally, a scheme is said to be stable, if for a given time interval, the numerical
  solutions can be bounded, independent of the mesh spacing, for all mesh spacings sufficiently
  small~\cite{GustafssonKreissOliger95}.  We will sometimes informally refer to a scheme being
  stable for some particular values of the mesh spacing and time step.}.  The Stokes equations in
our implementation of the AMP algorithm are solved with a fractional-step method based on a
velocity-pressure formulation~\cite{ICNS,splitStep2003} that can be made fully second-order (or
higher-order) accurate.  A key ingredient to this scheme is the proper specification of boundary
conditions for the pressure.  The elastic wave equation is solved with a second-order accurate
upwind scheme for the equations written as a first-order system following the approach developed for
overlapping grids in~\cite{smog2012}.  Together with the AMP interface condition, the partitioned
algorithm is fully second-order accurate.  The stability and accuracy is verified by comparing
numerical solutions with exact traveling-wave solutions to three FSI model problems.

In previous work~\cite{fsi2012}, a stable partitioned algorithm for {\em compressible} flows and
compressible elastic solids was developed that overcomes the added-mass effect and uses deforming
composite grids to treat large solid motions.  FSI problems involving compressible flows are
somewhat easier to deal with than incompressible flows since the added-mass effects are localized
due to the finite speeds of wave propagation in the fluid~\cite{vanBrummelen2009}.  The scheme
in~\cite{fsi2012}, which is based on the analysis in~\cite{BanksSjogreen2011}, uses a local
characteristic analysis of a fluid-structure Riemann problem to define an impedance weighted
averaging of the fluid and solid interface values (i.e.~a Robin-Robin coupling).  This algorithm was
extended to the case of rigid bodies in~\cite{lrb2013} where it was shown that the scheme remains
stable even for rigid bodies of zero mass.

The development and study of numerical algorithms for FSI problems is an active area of research, see for example, the papers~\cite{Farhat2006,SchaferHeckYigit2006,HronTurekMonolithic2006,TezduyarSathe2007,BorazjaniGeSotiropolous2008,DegrooteVierendeels2011,GretarssonKwatraFedkiw2011,HouWangLayton2012} and the references cited therein.
%, see for example~\cite{DoneaGiulianiHalleux1982,CebralLohner1997,Lohner99,LeTallecMouro2001,PipernoFarhat2001,SchaferTeschauer2001,GlowinskiPanHelsaJosephPeriaux2001,Guruswamy2002,MillerColella2002,KuhlHulshoffBorst2003,ArientiHungMoranoShepherd2003,Farhat2006,HronTurekMonolithic2006,Tezduyar2006,SchaferHeckYigit2006,AhnKallinderis2006,CirakDeiterdingMauch2007,vanLoon2007,TezduyarSathe2007,BorazjaniGeSotiropolous2008,Wilcox2010,BartonObadiaDrikakis2011,DegrooteVierendeels2011,TezduyarTakizawaBrummerChen2011,CrosettoDeparisFouresteyQuarteroni2011,Degroote2011,GretarssonKwatraFedkiw2011,HouWangLayton2012}.
In particular, there has been much work concerning partitioned algorithms and the added-mass effect.  For the case of incompressible fluids coupled to thin structural shells, there has been some success in treating the added-mass instability.  The kinematically-coupled scheme of Guidoboni et~al.~\cite{GuidoboniGlowinskiCavalliniCanic2009}, later extended to the $\beta$-scheme by \v{C}ani\'c, Muha and Buka\v{c}~\cite{CanicMuhaBukac2012}, is a stable partitioned scheme that uses operator splitting.  Nobile and Vergara~\cite{NobileVergara2008}, among others, have developed stable semi-monolithic schemes for the case of thin shells.  Even fully monolithic schemes for thin-shells~\cite{FigueroaVignonClementelJansenHughesTaylor2006} are not overly expensive since the number of degrees of freedom for the structural shell is usually small compared to those in the fluid.  For bulk solids, however, apparently all previous partitioned approaches for coupling incompressible flows and light solids are either unstable or require multiple sub-iterations per time step to converge (tens or hundreds of iterations are typical) with the number of iterations generally increasing as the solid gets lighter.  Indeed, it is common to resort to fully monolithic schemes~\cite{BatheZhang2004,Heil2004,HronTurekMonolithic2006,GeeKuttlerWall2011} or semi-monolithic schemes~\cite{FernandezGerbeauGrandmont2007,AstorinoChoulyFernandez2009,GretarssonKwatraFedkiw2011}.

A number of authors have analyzed the added-mass effect and the stability of FSI algorithms~\cite{Conca1997,LeTallecMani2000,MokWallRamm2001,ForsterWallRamm2007,AstorinoChoulyFernandez2009,vanBrummelen2009,Gerardo_GiordaNobileVergara2010}.  Causin, Gerbeau and Nobile~\cite{CausinGerbeauNobile2005}, for example, analyze a model problem of a structural shell coupled to an incompressible fluid and show that the traditional scheme can be unconditionally unstable over a certain range of parameters.  There are numerous approaches that have been developed to reduce the number of iterations required per time step in partitioned schemes~\cite{MokWallRamm2001}.  Robin-Robin interface conditions are used to stabilize partitioned schemes by, for example, Nobile, Vergara and co-workers~\cite{NobileVergara2008,BadiaNobileVergara2008,BadiaNobileVergara2009,Gerardo_GiordaNobileVergara2010,NobileVergara2012} and Astorino, Chouly and Fernandez~\cite{AstorinoChoulyFernandez2009}.  Yu, Baek and Karniadakis~\cite{YuBaekKarniadakis2013} and Baek and Karniadakis~\cite{BaekKarniadakis2012} have developed fictitious-pressure and fictitious-mass algorithms which incorporate additional terms into the governing equations to account for added-mass effects.  The optimal values for parameters are estimated from analysis and computation, and the number of sub-iterations required using Aitken acceleration (tens of iterations) is similar to optimal Robin-Robin approaches.  To stabilize the FSI algorithm and reduce the number of sub-iterations, Riemslagh, Virendeels and Dick~\cite{RiemslaghVierendeelsDick2000}, Degroote et~al.~\cite{DegrooteSwillensBruggemanHaeltermanSegersVierendeels2010}, and Raback, Ruokolainen, and Lyly~\cite{RabackRuokolainenLyly2001} have developed an interface artificial compressibility method that adds a source term to the fluid continuity equation near the interface; the effect of the source term goes away as the sub-iterations converge.  Idelsohn et~al.~\cite{IdelsohnDelPinRossiOnate2012} and Badia, Quaini and Quarteroni~\cite{BadiaQuainiQuarteroni2008} form approximate factorizations of the fully monolithic scheme to construct partitioned schemes but these still may require many iterations to converge.  Degroote et~al.~\cite{DegrooteBruggemanHaeltermanVierendeels2008,DegrooteBatheVierendeels2009} use reduced-order models and Aitken acceleration methods to decrease the number of iterations in partitioned schemes.

The remainder of the manuscript is organized as follows. In Section~\ref{sec:governingEquations} we define the governing equations and present the essential form of the AMP interface conditions.  In Section~\ref{sec:partitionedAlgorithms} there is a discussion of partitioned algorithms and how the AMP interface conditions are incorporated into the fluid and solid solution schemes.  Three model problems are defined in Section~\ref{sec:modelProblems} and these are used later for the analysis and numerical results.  In Section~\ref{sec:AMP1D} the form of the AMP algorithm for a one-dimensional model problem is discussed.  A normal mode stability analysis of the AMP scheme as well as the traditional (Dirichlet-Neumann) and anti-traditional (Neumann-Dirichlet) schemes are presented in Section~\ref{sec:analysis}.  The FSI time-stepping algorithm for the AMP scheme is outlined in Section~\ref{sec:timeSteppingAlgorithm}.  Section~\ref{sec:numericalResults} provides numerical results confirming the stability and accuracy of the scheme.  Conclusions are given in Section~\ref{sec:conclusions}.  A summary comparison of the algorithm discussed here for bulk solids with the one for structural shells is provided at the end of Part II of this paper~\cite{fis2014}.


==> texFiles/backup/numericalResults.tex <==
\section{Numerical results} \label{sec:numericalResults}


% ---- from codes/analysis/numerical/b1_runTP1D.m ---- $
\input tables/analysisTP1D

% ---- from codes/analysis/numerical/b2_runATP1D.m ---- $
\input tables/analysisATP1D

% ---- from codes/analysis/numerical/b3_runAMP1D.m ---- $
\input tables/analysisAMP1DLight

% ---- from codes/analysis/numerical/b4_runAMP1D.m ---- $
\input tables/analysisAMP1DHeavy

{
% ---- from codes/analysis/numerical/b4_runTP1DStability ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityTP1DNumerical}
  \caption{
  }  \label{fig:acousticSolidStokesStabilityTPNumerical}
\end{center}
\end{figure}
}

{
% ---- from codes/analysis/numerical/b5_runATP1DStability ---- $
\newcommand{\figWidth}{8cm}
\begin{figure}
\begin{center}
  \includegraphics[width=\figWidth]{fig/FSIStabilityATP1DNumerical}
  \caption{
  }  \label{fig:acousticSolidStokesStabilityATPNumerical}
\end{center}
\end{figure}
}


==> texFiles/backup/rectangularModelProblemCartoon.tex <==
{
\newcommand{\lbfont}{\small}
\def\ysb{-.15} % bottom of rigid body 
\def\ysa{-2}   % top of rigid body 
\def\ya{0} % bottom of fluid domain 
\def\yb{3} % top of fluid domain
\def\xL{8}
\begin{figure}[hbt]
	\newcommand{\textFont}{\normalss}
	\begin{center}
		\begin{tikzpicture}[scale=.9]
		%
		\useasboundingbox (0,\ysa) rectangle (\xL,3.2);  % set the bounding box (so we have less surrounding white space)
		%
		\draw[thick,fill=red!20,draw=red,line width=2pt] (0,\ysa) rectangle (\xL,\ysb);
		% \draw[thick,black] (0,\ysa) rectangle (\xL,\ysb);
		\draw[thick,black] (4,-1.2) node {solid: $\OmegaS$};
		%
		\draw[thick,fill=blue!20,draw=blue,line width=2pt] (0,\ya) rectangle (\xL,\yb);
		\draw[thick,blue] (0,\ya) rectangle (\xL,\yb);
		\draw[thick,black] (4,1.75) node {fluid: $\OmegaF$};
		%
		\draw[thick,black] (4,\ya) node[anchor=south] {interface: $\Gamma$};

		% -- solid
		\draw[-,thick,red] (0  ,\ysa) -- (\xL,\ysa);
		\draw[-,thick,red] (0  ,\ysb) -- (\xL,\ysb);
		\draw[-,thick,red] (0  ,\ya) -- (0  ,\ya) node[anchor=east,black,yshift=-4pt] {\lbfont$y=0$};
		\draw[-,thick,red] (\xL,\ysa) -- (\xL,\ysb);
		%
		%
		\draw[-,thick,blue] (0,\yb) -- (\xL,\yb);
		\draw[-,thick,blue] (\xL,0) -- (\xL,\yb);
		\draw (0  ,\ysa) node[anchor=north,black,yshift=-4pt] {\lbfont$x=0$};
		\draw (\xL,\ysa) node[anchor=north,black,yshift=-4pt] {\lbfont$x=L$};
		\draw (0,  \ysa) node[anchor=east,black] {\lbfont$y=-\Hs$};
		\draw (0,   \yb) node[anchor=east,black] {\lbfont$y=H$};
		%
		%\draw[thick,blue,yshift=\yH cm] (0,0) sin (2,0.25) cos (4,0) sin (6,-.25) cos (8,0); %  cos (4,-1) sin (6,1) cos (8,-1);
		%\draw[blue] (4,\yH) node[anchor=south,yshift=5pt] {\textFont $y=\eta(x,t)$};
		% grid:
		% \draw[step=1cm,gray] (0,\ysa) grid (8,\yb);
		%
		\end{tikzpicture}
	\end{center}
	\caption{The geometry for the rectangular geometry FSI model problems.} \label{fig:rectangularModelProblem}
\end{figure}
}


==> texFiles/backup/trimFig.tex <==
% -------------------------------------------------------------------------------------
%
% Trim a figure: **NEW VERSION**
%  In this new version we hard code the original width of the plot to match an Overture figure.
%  The clipping parameters then denote fractions of this width (width=7.5 in = 19.05 cm)
%
%  \trimPlot{file}{width}{xa}{xb}{ya}{yb}
% Trim a figure and show the bounding box:
%  \trimPlotb{file}{width}{xa}{xb}{ya}{yb}
% 
%  file = name of the graphics file for includegraphics : .eps or pdf or ...
%  width : final width (after trimming) of the figure e.g. 5cm
%  xa,xb,ya,yb : trim this fraction of the width from the left, right, bottom and top
% 
% -----------------------------------------------------------------------------------------
\newlength{\tfwidth}
\newlength{\tfheight}
\newlength{\tfxa}
\newlength{\tfxb}
\newlength{\tfya}
\newlength{\tfyb}
% 
\newcommand{\trimPlotWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
\newcommand{\trimPlotNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% Trim a figure and draw the bounding box 
% Overture figures are 7.5 inches wide (8.5 - .5 -.5) = 19.05 cm
\newcommand{\trimPlotb}[6]{%
\setlength{\tfwidth}{19.05cm}%   % width of un-clipped fig
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfwidth*\real{#5}}%
\setlength{\tfyb}{\tfwidth*\real{#6}}%
% trim=l b r t
\trimPlotWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
% \trimPlotWithBox{#1}{#2}{#3}{#4}{#5}{#6}%
}
% Trim a figure 
% 
\newcommand{\trimPlot}[6]{%
\setlength{\tfwidth}{19.05cm}%   % width of un-clipped fig
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfwidth*\real{#5}}%
\setlength{\tfyb}{\tfwidth*\real{#6}}%
% trim=l b r t
\trimPlotNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% ----------------------------------------------------------------------------------------------
% -------------------------------------------------------------------------------------
%
% Trim a figure: 
%  \trimFig{file}{width}{xa}{xb}{ya}{yb}
% Trim a figure and show the bounding box:
%  \trimFigb{file}{width}{xa}{xb}{ya}{yb}
% 
%  file = name of the graphics file for includegraphics : .eps or pdf or ...
%  width : final width (after trimming) of the figure e.g. 5cm
%  xa,xb,ya,yb : trim this fraction of the width from the left, right, bottom and top
% 
% -----------------------------------------------------------------------------------------
\newcommand{\trimFigWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
% -----------------------------------------------------------------------------------------
\newcommand{\trimFigNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% ---------- Set height -----
\newcommand{\trimFigHeightWithBox}[6]{%
\setlength\fboxsep{0pt}%
\setlength\fboxrule{1.0pt}% border thickness
\fbox{\includegraphics[height=#2, clip, trim=#3 #4 #5 #6]{#1}}%
}
% ---------- Set height -----
\newcommand{\trimFigHeightNoBox}[6]{%
\setlength\fboxsep{1pt}% note: make this 1pt and rule thickness zero so box size matches that below
\setlength\fboxrule{0.0pt}% border thickness
\fbox{\includegraphics[height=#2, clip, trim=#3 #4 #5 #6]{#1}}%
% \includegraphics[width=#2, clip, trim=#3 #4 #5 #6]{#1}
}
% Trim a figure and draw the bounding box 
\newcommand{\trimFigb}[6]{%
\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
% trim=l b r t
\trimFigWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% Trim a figure 
% 
\newcommand{\trimFig}[6]{%
\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
% trim=l b r t
\trimFigNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

%%%%%%%%%%%%%% TRIMW : trim and set width %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% THIS VERSION WORKS PROPERLY %%%%%%%%%%%%%%%%%%
%  Thanks to Longfei Li
% New:
% Trim a figure (working) 
%  trims #3 #4 #5 #6 percent of left, right, bottom, top of the original figure
\newsavebox\figBox

\newcommand{\trimw}[6]{%
%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMWB : trim and set width %%%%%%%%%%%%%%%%%%
%%%%%%%%%%   Version of trim that also draws the bounding box %%%%%%%%%%%%
\newcommand{\trimwb}[6]{%
%old: 
%\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
%\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
%new: Longfei 20160727: we should get the size of the original picture:
%\settowidth\tfwidth{\includegraphics{#1}}
%\settoheight\tfheight{\includegraphics{#1}}

%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMH : trim and set height %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% THIS VERSION WORKS PROPERLY %%%%%%%%%%%%%%%%%%
%  Thanks to Longfei Li
% New:
% Trim a figure (working) 
%  trims #3 #4 #5 #6 percent of left, right, bottom, top of the original figure
\newcommand{\trimh}[6]{%
%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigHeightNoBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}

% ----------------------------------------------------------------------------------------------
%%%%%%%%%%%%%% TRIMWB : trim and set height %%%%%%%%%%%%%%%%%%
%%%%%%%%%%   Version of trim that also draws the bounding box %%%%%%%%%%%%
\newcommand{\trimhb}[6]{%
%old: 
%\setlength{\tfwidth}{(#2+#2*\real{#3})+#2*\real{#4}}%   % width of un-clipped fig
%\setlength{\tfheight}{(#2+#2*\real{#5})+#2*\real{#6}}%
%new: Longfei 20160727: we should get the size of the original picture:
%\settowidth\tfwidth{\includegraphics{#1}}
%\settoheight\tfheight{\includegraphics{#1}}

%20160728 use \sbox to save one include graphics
\sbox\figBox{\includegraphics{#1}}
\setlength{\tfwidth}{\the\wd\figBox}
\setlength{\tfheight}{\the\ht\figBox}
\setlength{\tfxa}{\tfwidth*\real{#3}}%
\setlength{\tfxb}{\tfwidth*\real{#4}}%
\setlength{\tfya}{\tfheight*\real{#5}}%
\setlength{\tfyb}{\tfheight*\real{#6}}%
\trimFigHeightWithBox{#1}{#2}{\tfxa}{\tfya}{\tfxb}{\tfyb}%
}
% ----------------------------------------------------------------------------------------------
% 


==> texFiles/balloon.tex <==
\clearpage
\subsection{An elastic balloon} \label{sec:elasticBalloon}

Here is a potentially nice example showing an elastic balloon. Same
geometry as the radial travelling wave but with a larger deformation.
Could do a grid convergence study. 

An annular shaped region of an elastic solid surrounds an enclosed disk of an incompressible fluid.

The grid along with some computed solutions are shown in Figure~\ref{fig:elasticBallonGrid}. 

\wdh{Could plot stress in fluid as well?}

\newcommand{\Gcb}{\Gc_b}
\input texFiles/balloonFig.tex


==> texFiles/balloonFig.tex <==
{% ----------- BALLOON ------  
%
\newcommand{\figWidth}{5cm}% width
\newcommand{\trimfig}[2]{\trimwb{#1}{#2}{.1}{.1}{.11}{.11}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (15,5);  % set the bounding box (so we have less surrounding white space)

   \draw( 0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/elasticBalloonGride2}{\figWidth}};
% 
   \draw( 5.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/balloonG8t2p0stress}{\figWidth}};
   \draw(10.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/balloonG8t9p0stress}{\figWidth}};
   % grid:
 \draw[step=1cm,gray] (0,0) grid (15,5);
\end{tikzpicture}
\end{center}
  \caption{Left: composite grid $\Gcb^{(2)}$ for the elastic balloon.
    The green fluid grid adjacent to the interface moves over time while the blue fluid background grid remains fixed.
    The red grid for the solid reference domain also remains fixed over time.
    Middle and right: fluid pressure and $\| \sigmavs\|$ at times $t=2$ and $t=9$, computed
      on grid $\Gcb^{(8)}$. \wdh{wdh: add colour bars}
}
  \label{fig:elasticBallonGrid}
\end{figure}
}


==> texFiles/beamInAChannel.tex <==
\subsection{Results for solid beam in a channel}


Consider the flow of an incompressible fluid past a solid deformable beam.

Figure~\ref{fig:beamInAChannelScf100} shows results for SCF=100. NOTE: I had to use $z_f = 20 \mu/h$ for this case
($z_f = 10 \mu/h$ was not stable).

{% ------------------------------------------
\newcommand{\figWidth}{8.cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.25}{.25}}
\newcommand{\figWidtha}{6.5cm}
\newcommand{\trimfiga}[2]{\trimw{#1}{#2}{.0}{.0}{.1}{.0}}
\begin{figure}[H]
\begin{center}
\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.5) rectangle (16.,6.);  % set the bounding box (so we have less surrounding white space)
%
%  \draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{beamInAChannel/bilcInsSmt5p5Grid}{\figWidtha}};
  \draw(7.5,1) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{beamInAChannel/bicG8Scf100StreamLinesSpeedt6p0}{\figWidth}};

%
% grid:
%  \draw[step=1cm,gray] (0,.5) grid (16,6);
\end{tikzpicture}
}% END resize box
\end{center}
\caption{Incompressible flow past an elastic solid beam. SCF=100 $t=4$. Note beam expansion at top due
  to linear elastic approximation.
 }
  \label{fig:beamInAChannelScf100}
\end{figure}
}


{% ------------------------------------------
\newcommand{\figWidth}{8.cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.25}{.25}}
\newcommand{\figWidtha}{6.5cm}
\newcommand{\trimfiga}[2]{\trimw{#1}{#2}{.0}{.0}{.1}{.0}}
\begin{figure}[htb]
\begin{center}
\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.5) rectangle (16.,6.);  % set the bounding box (so we have less surrounding white space)
%
%   \draw(8.0,7) node[anchor=south,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/risingBodyCompareYb}{\figWidthA}};
%%  \draw(8.0,7) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/fallingBodyAnimation1}{\figWidth}};
%
  \draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{beamInAChannel/bilcInsSmt5p5Grid}{\figWidtha}};
  \draw(7.5,1) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{beamInAChannel/bilcInsSmt5p5streamLines}{\figWidth}};

%
% grid:
%  \draw[step=1cm,gray] (0,.5) grid (16,6);
\end{tikzpicture}
}% END resize box
\end{center}
  \caption{Incompressible flow past an elastic solid beam. HEAVY 
 }
  \label{fig:beamInAChannel}
\end{figure}
}


{% ------------------------------------------
\newcommand{\figWidth}{8.cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.0}{.0}{.25}{.25}}
\newcommand{\figWidtha}{6.5cm}
\newcommand{\trimfiga}[2]{\trimw{#1}{#2}{.0}{.0}{.05}{.0}}
\begin{figure}[htb]
\begin{center}
\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.5) rectangle (16.,6.);  % set the bounding box (so we have less surrounding white space)
%
%   \draw(8.0,7) node[anchor=south,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/risingBodyCompareYb}{\figWidthA}};
%%  \draw(8.0,7) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fallingBody/fallingBodyAnimation1}{\figWidth}};
%
%  \draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{beamInAChannel/bilcInsSmt5p5Grid}{\figWidtha}};
  \draw(7.5,1) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{beamInAChannel/thinBeamInAChannelStreamlines}{\figWidth}};

%
% grid:
%  \draw[step=1cm,gray] (0,.5) grid (16,6);
\end{tikzpicture}
}% END resize box
\end{center}
  \caption{Incompressible flow past a thin elastic solid beam. HEAVY 
 }
  \label{fig:thinBeamInAChannel}
\end{figure}
}


==> texFiles/boundaryConditionsNotes.tex <==


Here we will show the AMP boundary conditions and how they reduce to 
heavy solid and light solid conditions in the proper limits.\\

\noindent \textbf{Heavy solid} (no-slip wall): 
For $\xv \in \Gamma,$
\begin{align}
\tv_m^T \vv &= \tv_m^T \vvs \label{eq:heavySolidVelocityTangential}, \quad m=1,2\\
\nv^T \vv &= \nv^T \vvs \label{eq:heavySolidVelocityNormal}
\end{align}
%
\textbf{Light solid} (free surface):
For $\xv \in \Gamma,$
\begin{align}
\tv_m^T \tauv \nv &= \tv_m^T \sigmavs \nv, \quad m=1,2 \label{eq:lightSolidVelocityTangential}\\
-p + \nv^T \tauv \nv &= \nv^T \sigmavs \nv \label{eq:lightSolidPressure}
\end{align}
%
\textbf{AMP}: 
The outgoing solid characteristics are used as boundary conditions for the fluid.
For $\xv \in \Gamma,$
\begin{align}
-p + \nv^T \tauv \nv + \zp \nv^T \vv &= \nv^T \sigmasv \nv + \zp \nv^T \vvs 
\label{eq:normalCharacteristic} \\
\tv_m^T \tauv \nv + \zs \tv_m^T \vv &= \tv_m^T \sigmasv \nv + \zs \tv_m^T \vvs, \quad m=1,2
\label{eq:tangentialCharacteristic}
\end{align}
%
Equation \eqref{eq:normalCharacteristic} is manipulated to form a Robin condition
for the pressure. Consider the Taylor expansion of a point moving with the interface, 
$\mathcal{P}(t)$ in the fluid Eulerian frame and $\mathcal{P}_0$ in the solid Lagrangian frame,
\begin{align*}
\vv(\xv, t-\dt) \big{|}_{\xv = \mathcal{P}(t-\dt)} &= \left( \vv(\xv,t) - \dt D_t \vv(\xv,t) + \hdots  \right) \big{|}_{\xv = \mathcal{P}(t)} \\
\vvs(\xvs, t-\dt) \big{|}_{\xvs= \mathcal{P}_0} &=  \left( \vvs(\xvs,t) - \dt \vvs_t(\xvs,t) + \hdots \right) \big{|}_{\xvs = \mathcal{P}_0}
\end{align*}
%
We equate the first two terms of the expansion.
Bring the velocity terms to one side and pre-multiply by 
$\zp \nv^T$
\begin{align*}
\zp \nv^T (\vv - \vvs) &= \zp \dt \nv^T \left( D_t \vv - \vvs_t \right).
\end{align*}
%
Use the solid characteristic to eliminate the velocity terms and use the 
fluid equation to eliminate $D_t \vv.$
By rearranging terms, a Robin condition for the pressure is revealed.
\begin{align}
-p - \frac{\zp \dt}{\rho} \frac{\partial p}{\partial n} &= 
\nv^T (\sigmavs - \tauv) \nv 
+ \zp \dt \nv^T \left(\nu \grad \times \grad \times \vv + \vvs_t \right)
\end{align}
%
In the light and heavy solid limits, this condition approaches
\begin{alignat*}{2}
-p  &= \nv^T (\sigmavs - \tauv) \nv, \quad &&\zp \rightarrow 0  \\
- \frac{1}{\rho} \frac{\partial p}{\partial n} &= 
\nv^T \left(\nu \grad \times \grad \times \vv + \vvs_t \right),
\quad &&\zp \rightarrow \infty.
\end{alignat*}
%
The latter condition is equivalent to the compatibility condition used in 
the heavy solid limit.
In the light and heavy solid limits, equation \ref{eq:tangentialCharacteristic}
approaches
\begin{alignat*}{6}
\tv_m^T \tauv \nv &= \tv_m^T \sigmasv \nv , &&\quad m=1,2, \quad &&\zp \rightarrow 0 \\
\tv_m^T \vv &=  \tv_m^T \vvs, &&\quad m=1,2,
\quad &&\zp \rightarrow \infty.
\end{alignat*}
%
Note that the heavy solid condition $\nv^T \vv = \nv^T \vvs$ is not 
satisfied when $\zp \rightarrow \infty.$ That is why we impose the 
following compatibility condition
\begin{align}
\nv^T \vv = \nv^T \frac{\zf \vv_f + \zp \vvs}{\zf + \zp}.
\end{align}
%
In the corresponding limits,
\begin{alignat*}{2}
\nv^T \vv &= \nv^T \vv_f \quad &&\zp \rightarrow 0 \\
\nv^T \vv &= \nv^T \vvs, \quad &&\zp \rightarrow \infty
\end{alignat*}
%
In the discrete algorithm, $\vv_f$ would correspond to using interior update scheme, 
\begin{align}
\vv_f = \vv^n 
+ \frac{\dt}{2} \left(-\frac{1}{\rho} \grad p^{n+1} + \Delta \vv 
-\frac{1}{\rho} \grad p^{n} + \Delta \vv^n \right).
\end{align}
%
Note that since the RHS contains $\Delta \vv,$ the impedance weighted average 
condition is implicit.

% \subsection{traditional scheme (heavy solid): explicit}

% cgmp elasticShear -g=elasticPistonGride2.order2p.hdf -addedMass=1 -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -muFluid=10. -muSolid=1000. -rhoSolid=1000. -nu=10. -lambdaSolid=1000. -useTP=1 -amp=.001

% \begin{table}[h]
% \begin{tabular}{c}
% \begin{lstlisting}
%  err(u)     r   err(v1s)   r  err(s12s)   r   err(u1s)   r    Nt
% 3.99e-11        1.19e-08       1.45e-05       3.08e-09        76
% 3.23e-12  12.4  3.06e-09  3.9  2.87e-06  5.0  7.73e-10  4.0  226
% 6.86e-13   4.7  7.72e-10  4.0  6.71e-07  4.3  1.93e-10  4.0  901
% 1.72e-13   4.0  1.99e-10  3.9  1.64e-07  4.1  4.84e-11  4.0 3576
% \end{lstlisting}
% \end{tabular}
% \end{table}



% \subsection{traditional scheme (heavy solid): implicit}

% cgmp elasticShear -g=elasticPistonGride2.order2p.hdf -addedMass=1 -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=im -go=halt -cfl=.9 -muFluid=10. -muSolid=1000. -rhoSolid=1000. -nu=10. -lambdaSolid=1000. -useTP=1 -amp=.001

% \begin{table}[h]
% \begin{tabular}{c}
% \begin{lstlisting}
%  err(u)    r   err(v1s)   r  err(s12s)   r   err(u1s)   r    Nt
% 1.09e-11       1.18e-08       1.45e-05       3.08e-09        26
% 2.72e-12  4.0  3.04e-09  3.9  2.87e-06  5.0  7.71e-10  4.0   51
% 6.81e-13  4.0  7.67e-10  4.0  6.69e-07  4.3  1.93e-10  4.0  101
% 1.70e-13  4.0  1.95e-10  3.9  1.64e-07  4.1  4.83e-11  4.0  201
% \end{lstlisting}
% \end{tabular}
% \end{table}







\subsection{AMP: 2D, explicit, linearized interface}

Consider $\nv = [0,-1]^T,\; \tv = [1,0]^T.$
The velocity is advanced using the scheme on the interior and boundary points.
The normal component of velocity is updated using an impedance weighted average,
\begin{align*}
v_2 &= \frac{\zf v_2^{(p)} + \zp \vs_2}{\zf + \zp}.
\end{align*}
%
The Robin condition and the scheme couple for $v_1$ on
the boundary and ghost point, so these are solved together.
The Robin condition is
\begin{align*}
\mu (v_{1,y} + v_{2,x}) - \zs v_1 &= \sigmas_{12} - \zs \vs_1 .
\end{align*}
%
The scheme is
\begin{align*}
v_1^n &= v_1^{n-1}
+ \frac{\theta \dt}{\rho} \left( -p_x^n + \mu (v_{1,xx}^n + v_{1,yy}^n) \right)
+ \frac{(1-\theta) \dt}{\rho} \left( -p_x^{n-1} + \mu (v_{1,xx}^{n-1} + v_{1,yy}^{n-1} ) \right) .
\end{align*}
%
There are two options to handle the $v_{1,xx}$ term. 
The substitution, $v_{1,xx} = -v_{2,xy}$, can be made.
Alternatively we can use
\begin{align*}
v_{1,xx} \approx \frac{v_{1, i+1,j}^{(p)} - 2 v_{1, i,j} + v_{1, i-1,j}^{(p)}}{\dx^2}.
\end{align*}
%
The condition (for $v_{1,i,j}$ and $v_{1,i,j-1}$) becomes
\begin{align*}
-\zs v_{1,i,j} + \mu \frac{v_{1,i,j+1}-v_{1,i,j-1}}{2 \dy} &= G_1 \\
 v_{1,i,j} - \theta \nu \dt 
\left(
\frac{v_{1, i+1,j}^{(p)} - 2 v_{1, i,j} + v_{1, i-1,j}^{(p)}}{\dx^2} 
+ \frac{v_{1, i,j+1} - 2 v_{1, i,j} + v_{1, i,j-1}}{\dy^2}
\right) &= G_2 .
\end{align*}
%
The ghost point $v_{2,i,j-1}$ can be found by applying the divergence free condition.
\begin{align*}
\frac{v_{1,i+1,j}-v_{1,i-1,j}}{2 \dx} + \frac{v_{2,i,j+1}-v_{2,i,j-1}}{2 \dy} = 0
\end{align*}

\bigskip
cgmp elasticShear -g=elasticPistonGride2.order2p.hdf -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -muFluid=10. -muSolid=10. -rhoSolid=10. -nu=10. -lambdaSolid=10. -useTP=0 -addedMass=1 -amp=.001

\FloatBarrier
\begin{table}[h]
\caption{Elastic shear, light solid}
\centering
\begin{tabular}{cccccccccc}
$g$ & $N_t$ & $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
1 & 76 &  6.6e-07 &   &  1.1e-09 &   &  1.0e-06 &   &  4.8e-05 &   \\ 
2 & 226 &  2.5e-07 & 2.6  &  5.8e-10 & 1.8  &  1.6e-07 & 6.3  &  1.2e-05 & 3.9  \\ 
3 & 901 &  5.4e-08 & 4.7  &  9.3e-11 & 6.3  &  4.3e-08 & 3.7  &  2.1e-06 & 5.7  \\ 
4 & 3576 &  1.3e-08 & 4.0  &  2.1e-11 & 4.5  &  1.4e-08 & 3.1  &  5.3e-07 & 4.0  \\ 
\end{tabular}
\end{table}
\FloatBarrier

cgmp elasticShear -g=elasticPistonGride2.order2p.hdf -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -muFluid=10. -muSolid=1000. -rhoSolid=1000. -nu=10. -lambdaSolid=1000. -useTP=0 -addedMass=1 -amp=.001

\FloatBarrier
\begin{table}[h]
\caption{Elastic shear, heavy solid}
\centering
\begin{tabular}{cccccccccc}
$g$ & $N_t$ & $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
1 & 76 &  3.0e-08 &   &  3.1e-09 &   &  1.2e-08 &   &  1.4e-05 &   \\ 
2 & 226 &  7.5e-09 & 4.0  &  7.7e-10 & 4.0  &  3.1e-09 & 3.9  &  2.9e-06 & 5.0  \\ 
3 & 901 &  1.8e-09 & 4.1  &  1.9e-10 & 4.0  &  8.1e-10 & 3.8  &  6.7e-07 & 4.3  \\ 
4 & 3576 &  4.5e-10 & 4.1  &  4.8e-11 & 4.0  &  2.1e-10 & 3.9  &  1.6e-07 & 4.1  \\ 
\end{tabular}
\end{table}
\FloatBarrier


\subsection{Curvilinear interface}

For implementation in curvilinear coordinates, we take the scalar conditions above and assign a direction 
in the interface coordinate basis ($\nv,\, \tv_1,\, \tv_2$). The divergence and Robin conditions are
combined to give
\begin{align}
\nv \nv^T (\grad \cdot \vv) 
+ \frac{1}{\mu} \left(I - \nv \nv^T \right)
\left(\tauv \nv + \zs \vv \right)
 &= \frac{1}{\mu} \left(I - \nv \nv^T \right)
\left(\sigmasv \nv + \zs \vvs \right).
\end{align}
%
The normal component of the velocity is assigned using the impedance weighted average
and the tangential component of the velocity is assigned using the fluid scheme.
\begin{align*}
\vv &= 
\nv \nv^T \left( \alpha \vv_f + (1-\alpha) \vvs \right)
+ (I- \nv \nv^T) \vv_f \\
&= \left(I + (\alpha-1) \nv \nv^T \right) \vv_f
+ (1 - \alpha )\nv \nv^T \vvs .
\end{align*}
%
Let $\mathcal{P} = (1-\alpha) \nv \nv^T$, then
\begin{align}
\vv &= \left( I - \mathcal{P} \right) \vv_f
+ \mathcal{P} \vvs.
\end{align}
%
Here,
\begin{align}
\vv_f = \vv^{n-1} 
+ \frac{\theta \dt}{\rho} \left(- (\grad p)^n + \mu \Delta \vv \right)
+ \frac{(1-\theta) \dt}{\rho} \left(- (\grad p)^{n-1} + \mu \Delta \vv^{n-1} \right).
\end{align}
%
The conditions look like
\begin{align}
\nv (\grad \cdot \vv) 
+ \frac{1}{\mu} (I-\nv\nv^T) (\tauv \nv - \zs \vv) &= \fv \\
\vv - \theta \dt \nu \left(I - \mathcal{P} \right) \Delta \vv &= \gv.
\end{align}
%

\subsection{Explicit curvilinear}
In implementation, we use predicted values to decouple 
these conditions in the `tangential' direction.
When we are applying the boundary condition on a constant $s$ wall,
the derivatives look like
\begin{align*}
u_{rr} = \frac{u_{i+1,j}^{(p)} - 2 u_{i,j} + u_{i-1,j}^{(p)}}{\Delta r^2},
\quad
u_{ss} = \frac{u_{i,j+1} - 2 u_{i,j} + u_{i,j-1}}{\Delta s^2}.
\end{align*}

\bigskip
cgmp elasticShear -g=elasticPistonGride2.order2p.hdf -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -muFluid=10. -muSolid=10. -rhoSolid=10. -nu=10. -lambdaSolid=10. -useTP=0 -addedMass=1 -amp=.001
\FloatBarrier
\begin{table}[h]
\caption{Elastic shear, light solid}
\centering
\begin{tabular}{cccccccccc}
$g$ & $N_t$ & $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
1 & 76 &  6.3e-07 &   &  1.1e-09 &   &  9.4e-07 &   &  4.5e-05 &   \\ 
2 & 226 &  2.1e-07 & 3.0  &  4.9e-10 & 2.2  &  1.1e-07 & 8.5  &  9.5e-06 & 4.7  \\ 
3 & 901 &  4.6e-08 & 4.5  &  7.5e-11 & 6.5  &  3.7e-08 & 3.0  &  1.9e-06 & 5.0  \\ 
4 & 3576 &  1.2e-08 & 4.0  &  1.7e-11 & 4.4  &  1.2e-08 & 3.1  &  4.6e-07 & 4.1  \\ 
\end{tabular}
\end{table}
\FloatBarrier

cgmp elasticShear -g=elasticPistonGride2.order2p.hdf -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -muFluid=10. -muSolid=1000. -rhoSolid=1000. -nu=10. -lambdaSolid=1000. -useTP=0 -addedMass=1 -amp=.001

\FloatBarrier
\begin{table}[h]
\caption{Elastic shear, heavy solid}
\centering
\begin{tabular}{cccccccccc}
$g$ & $N_t$ & $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
1 & 76 &  2.7e-08 &   &  3.1e-09 &   &  1.2e-08 &   &  1.4e-05 &   \\ 
2 & 226 &  6.5e-09 & 4.1  &  7.7e-10 & 4.0  &  3.1e-09 & 3.9  &  2.9e-06 & 5.0  \\ 
3 & 901 &  1.6e-09 & 4.1  &  1.9e-10 & 4.0  &  8.1e-10 & 3.8  &  6.7e-07 & 4.3  \\ 
\end{tabular}
\end{table}
\FloatBarrier

% cgmp elasticPiston -g=elasticPistonGride2.order2p.hdf -addedMass=1 -scf=.1 -nu=.01 -tp=.01 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -tf=.25 -cfl=.9

% \FloatBarrier
% \begin{table}[h]
% \caption{Elastic piston, light solid}
% \centering
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 1 & 51 &  3.0e-05 &   &  3.4e-05 &   &  1.1e-05 &   &  8.4e-06 &   &  6.5e-06 &   \\ 
% 2 & 76 &  7.2e-06 & 4.2  &  7.3e-06 & 4.6  &  2.4e-06 & 4.3  &  3.0e-06 & 2.8  &  1.7e-06 & 3.9  \\ 
% 3 & 126 &  2.7e-06 & 2.6  &  6.1e-06 & 1.2  &  5.9e-07 & 4.2  &  1.3e-06 & 2.4  &  4.6e-07 & 3.6  \\ 
% 4 & 376 &  9.3e-07 & 2.9  &  1.1e-06 & 5.7  &  1.2e-07 & 5.0  &  2.2e-07 & 5.8  &  9.1e-08 & 5.1  \\ 
% \end{tabular}
% \end{table}
% \FloatBarrier

% cgmp travelingWave -g=elasticPistonGride2.order2p.hdf -tp=.01 -tf=.25 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -rhoSolid=1. -muSolid=1. -lambdaSolid=1. -nu=.02 -addedMass=1 -useTP=0 -amp=.000001

% \FloatBarrier
% \begin{table}[h]
% \caption{Traveling wave, light solid}
% \centering
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 1 & 51 &  2.1e-07 &   &  5.9e-07 &   &  8.6e-08 &   &  6.9e-08 &   &  4.2e-07 &   \\ 
% 2 & 76 &  6.3e-08 & 3.3  &  1.7e-07 & 3.4  &  2.8e-08 & 3.1  &  2.8e-08 & 2.4  &  1.3e-07 & 3.2  \\ 
% 3 & 201 &  1.5e-08 & 4.1  &  4.6e-08 & 3.8  &  6.3e-09 & 4.4  &  1.1e-08 & 2.7  &  3.7e-08 & 3.6  \\ 
% 4 & 726 &  3.4e-09 & 4.5  &  1.2e-08 & 3.9  &  1.2e-09 & 5.2  &  2.8e-09 & 3.7  &  9.7e-09 & 3.8  \\ 
% \end{tabular}
% \end{table}
% \FloatBarrier

% cgmp radialElasticPiston -g=radialElasticPistonGride2.order2.hdf -addedMass=1 -scf=1 -nu=.05 -tp=.01 -tf=.25 -smVariation=g -debug=1 -tsINS=pc -cdv=1 -smoothInterface=0 -go=halt

% \FloatBarrier
% \begin{table}[h]
% \caption{Radial elastic piston, light solid}
% \centering
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 1 & 76 &  8.9e-04 &   &  3.7e-04 &   &  6.6e-04 &   &  7.5e-05 &   &  6.6e-04 &   \\ 
% 2 & 176 &  2.1e-04 & 4.3  &  1.2e-04 & 3.1  &  1.5e-04 & 4.3  &  1.6e-05 & 4.7  &  1.6e-04 & 4.2  \\ 
% 3 & 538 &  4.9e-05 & 4.2  &  4.4e-05 & 2.8  &  4.3e-05 & 3.6  &  4.5e-06 & 3.6  &  4.3e-05 & 3.6  \\ 
% 4 & 1910 &  1.2e-05 & 4.0  &  1.5e-05 & 2.8  &  1.1e-05 & 3.8  &  1.3e-06 & 3.4  &  1.1e-05 & 3.8  \\ 
% \end{tabular}
% \end{table}
% \FloatBarrier

% \subsection{Debug Radial Traveling Wave and Shear Solution- 12/17/17 benchmark}

% cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -rhoSolid=.001 -muSolid=.001 -lambdaSolid=.001 -nu=.1 -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=2

% \FloatBarrier
% \begin{table}[h]
% \caption{Exact interface transfer + set velocity}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 64 &  1.7e-07 &   &  1.4e-07 &   &  1.2e-05 &   &  1.2e-04 &   &  1.7e-07 &   \\ 
% 1 & 154 &  6.1e-08 & 2.8  &  4.4e-08 & 3.2  &  3.9e-06 & 3.1  &  4.3e-05 & 2.7  &  6.7e-08 & 2.5  \\ 
% 2 & 463 &  2.9e-08 & 2.1  &  1.6e-08 & 2.8  &  1.3e-06 & 3.1  &  1.6e-05 & 2.7  &  2.6e-08 & 2.5  \\ 
% 3 & 1669 &  1.1e-08 & 2.6  &  4.7e-09 & 3.3  &  4.1e-07 & 3.2  &  5.4e-06 & 3.0  &  9.1e-09 & 2.9  \\ 
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{AMP}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 64 &  9.8e-06 &   &  1.6e-05 &   &  4.7e-04 &   &  2.9e-03 &   &  1.3e-05 &   \\ 
% 1 & 154 &  9.2e-06 & 1.1  &  1.5e-05 & 1.0  &  3.8e-04 & 1.2  &  2.2e-03 & 1.3  &  1.2e-05 & 1.1  \\ 
% 2 & 463 &  7.4e-06 & 1.2  &  1.2e-05 & 1.2  &  2.6e-04 & 1.5  &  1.5e-03 & 1.5  &  9.4e-06 & 1.3  \\ 
% 3 & 1669 &  5.0e-06 & 1.5  &  6.1e-06 & 2.0  &  1.0e-04 & 2.5  &  8.0e-04 & 1.9  &  5.6e-06 & 1.7  \\ 
% \end{tabular}
% \end{table}

% \FloatBarrier

% cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -rhoSolid=1 -muSolid=1 -lambdaSolid=1 -nu=.1 -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=0
% \FloatBarrier

% \begin{table}[h]
% \caption{Exact interface transfer + set velocity}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 64 &  9.9e-08 &   &  9.1e-08 &   &  1.2e-07 &   &  6.2e-08 &   &  1.2e-07 &   \\ 
% 1 & 154 &  2.9e-08 & 3.4  &  2.6e-08 & 3.5  &  3.4e-08 & 3.6  &  1.5e-08 & 4.1  &  3.3e-08 & 3.8  \\ 
% 2 & 463 &  9.0e-09 & 3.2  &  8.0e-09 & 3.3  &  9.4e-09 & 3.6  &  4.2e-09 & 3.6  &  8.5e-09 & 3.9  \\ 
% 3 & 1669 &  3.1e-09 & 2.9  &  2.4e-09 & 3.3  &  2.6e-09 & 3.7  &  1.2e-09 & 3.5  &  2.3e-09 & 3.8  \\ 
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{AMP}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 64 &  2.9e-07 &   &  3.3e-07 &   &  3.3e-07 &   &  1.0e-07 &   &  3.5e-07 &   \\ 
% 1 & 154 &  1.2e-07 & 2.4  &  1.7e-07 & 1.9  &  1.7e-07 & 2.0  &  3.3e-08 & 3.1  &  1.7e-07 & 2.0  \\ 
% 2 & 463 &  4.4e-08 & 2.7  &  6.8e-08 & 2.5  &  6.7e-08 & 2.5  &  1.2e-08 & 2.8  &  6.9e-08 & 2.5  \\ 
% 3 & 1669 &  1.5e-08 & 3.0  &  2.3e-08 & 3.0  &  2.2e-08 & 3.0  &  4.1e-09 & 2.9  &  2.3e-08 & 3.0  \\ 
% \end{tabular}
% \end{table}

% \FloatBarrier

% cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -rhoSolid=1000 -muSolid=1000 -lambdaSolid=1000 -nu=.1 -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=1
% \FloatBarrier
% \begin{table}[h]
% \caption{Exact interface transfer + set velocity}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 64 &  9.6e-08 &   &  4.0e-08 &   &  4.7e-05 &   &  2.8e-08 &   &  4.8e-05 &   \\ 
% 1 & 154 &  3.1e-08 & 3.1  &  1.3e-08 & 3.1  &  1.3e-05 & 3.7  &  7.2e-09 & 4.0  &  1.2e-05 & 4.1  \\ 
% 2 & 463 &  1.1e-08 & 2.9  &  3.8e-09 & 3.3  &  4.1e-06 & 3.1  &  2.0e-09 & 3.5  &  3.3e-06 & 3.6  \\ 
% 3 & 1669 &  2.7e-09 & 3.9  &  1.1e-09 & 3.4  &  1.3e-06 & 3.2  &  5.8e-10 & 3.5  &  1.1e-06 & 3.1  \\ 
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{AMP}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 64 &  4.3e-07 &   &  1.0e-07 &   &  4.7e-05 &   &  2.8e-08 &   &  4.8e-05 &   \\ 
% 1 & 154 &  2.0e-07 & 2.2  &  2.6e-08 & 3.9  &  1.3e-05 & 3.7  &  7.2e-09 & 4.0  &  1.2e-05 & 4.1  \\ 
% 2 & 463 &  1.1e-07 & 1.7  &  8.0e-09 & 3.3  &  4.1e-06 & 3.1  &  2.0e-09 & 3.5  &  3.3e-06 & 3.6  \\ 
% 3 & 1669 &  5.8e-08 & 2.0  &  3.1e-09 & 2.6  &  1.3e-06 & 3.2  &  5.8e-10 & 3.5  &  1.1e-06 & 3.2  \\ 
% \end{tabular}
% \end{table}

% \FloatBarrier

% cgmp radialShearFlow -g=radialElasticPistonGride1.order2.hdf -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -muFluid=10. -muSolid=10. -rhoSolid=10. -nu=10. -lambdaSolid=10. -useTP=0 -addedMass=1 -amp=.001
% \FloatBarrier
% \begin{table}[h]
% \caption{Exact interface transfer + set velocity}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 76 &  2.6e-09 &   &  4.9e-10 &   &  2.5e-07 &   &  1.2e-09 &   &  2.3e-07 &   \\ 
% 1 & 126 &  4.8e-10 & 5.5  &  1.3e-10 & 3.7  &  1.8e-08 & 14.1  &  9.9e-11 & 12.3  &  2.2e-08 & 10.2  \\ 
% 2 & 351 &  2.4e-10 & 2.0  &  4.5e-11 & 2.9  &  6.9e-09 & 2.6  &  5.9e-11 & 1.7  &  5.4e-09 & 4.2  \\ 
% 3 & 1101 &  1.2e-10 & 2.0  &  1.7e-11 & 2.6  &  2.1e-09 & 3.2  &  3.4e-11 & 1.8  &  1.8e-09 & 3.1  \\ 
% \end{tabular}
% \end{table}
% % \begin{table}[h]
% % \caption{Exact interface transfer + set velocity}
% % \begin{tabular}{cccccccccccc}
% % $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% % \hline
% % 0 & 76 &  4.9e-10 &   &  1.8e-08 &   &  6.2e-06 &   &  1.4e-08 &   &  6.2e-06 &   \\ 
% % 1 & 126 &  1.3e-10 & 3.7  &  2.1e-09 & 8.3  &  6.2e-06 & 1.0  &  1.7e-08 & 0.8  &  6.2e-06 & 1.0  \\ 
% % 2 & 351 &  4.5e-11 & 2.9  &  2.6e-10 & 8.0  &  6.2e-06 & 1.0  &  2.7e-08 & 0.6  &  6.2e-06 & 1.0  \\ 
% % 3 & 1101 &  1.7e-11 & 2.6  &  1.2e-10 & 2.2  &  6.2e-06 & 1.0  &  4.4e-08 & 0.6  &  6.2e-06 & 1.0  \\ 
% % \end{tabular}
% % \end{table}

% \begin{table}[h]
% \caption{AMP}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $\vv$ & ratio  &  $p$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 76 &  2.7e-09 &   &  4.0e-09 &   &  3.7e-07 &   &  7.9e-09 &   &  3.7e-07 &   \\ 
% 1 & 126 &  5.1e-10 & 5.3  &  2.6e-09 & 1.6  &  2.1e-07 & 1.7  &  4.2e-09 & 1.9  &  2.1e-07 & 1.7  \\ 
% 2 & 351 &  2.3e-10 & 2.2  &  1.2e-09 & 2.2  &  8.4e-08 & 2.5  &  1.2e-09 & 3.4  &  8.4e-08 & 2.5  \\ 
% 3 & 1101 &  1.2e-10 & 2.0  &  4.2e-10 & 2.8  &  3.1e-08 & 2.7  &  2.9e-10 & 4.2  &  3.1e-08 & 2.7  \\ 
% \end{tabular}
% \end{table}

% \FloatBarrier

% \textbf{Note}:
% See cg/mp/runs/elasticPiston/memo for coupled runs
% and cg/ins/runs/elasticPiston/memo and 
% cg/sm/runs/elasticPiston/memo for decoupled runs.
% For debugging, the AMP velocity conditions can be turned off in
% projectInterfaceVelocity.C. Change this to true:
% \begin{lstlisting}
% if( false ) // set this to true for debugging
% {
%   // ** do this for now****
%   // --- set the gridVelocity to the solid velocity
%   gridVelocityLocal(Ib1,Ib2,Ib3,Rx)= vSolidLocal(Ib1,Ib2,Ib3,Rx);
%   uLocal(Ib1,Ib2,Ib3,Rx) = vSolidLocal(Ib1,Ib2,Ib3,Rx);
% }
% \end{lstlisting}
% %
% and change the section that looks like this to false:
% \begin{lstlisting}
% if ( true ) {
% assert( axis == 1 && side == 0);
% assert( numberOfDimensions == 2 );

% // solve the system:
% // n (div.u) + 1/mu (I-n.n') (tau n + zs v) = 1/mu (I-n.n') ( Ts + zs vs )
% // v - (I + (alpha - 1) n.n') theta dt nu Delta v
% //      = (I + (alpha - 1) n.n') (vp + theta dt / rho (- grad p)
% //                   +(1-theta) dt / rho (-grad pp + mu Delta vp))
% //        (1 - alpha) n.n' vs
% //
% // *** See Dropbox/CG/fibr/codes/curvilinearBC/* for maple file ***
% ...
% }
% \end{lstlisting}

% \subsection{Predicted pressure fix}

% Third order extrapolation is used for the pressure during the predictor stage.
% \begin{table}[h]
% \caption{Elastic piston with predicted pressure}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 30 &  2.3e-05 &   &  5.4e-06 &   &  1.3e-05 &   &  7.8e-06 &   &  7.8e-06 &   \\ 
% 1 & 59 &  5.7e-06 & 4.1  &  1.4e-06 & 4.0  &  3.2e-06 & 4.1  &  1.9e-06 & 4.1  &  1.9e-06 & 4.2  \\ 
% 2 & 117 &  1.4e-06 & 4.1  &  3.4e-07 & 4.0  &  7.9e-07 & 4.1  &  4.8e-07 & 4.0  &  4.5e-07 & 4.2  \\ 
% 3 & 357 &  1.5e-07 & 9.4  &  2.9e-08 & 11.8  &  1.4e-07 & 5.7  &  1.0e-07 & 4.6  &  8.0e-08 & 5.6  \\ 
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{Elastic piston without predicted pressure}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 30 &  8.1e-05 &   &  1.0e-04 &   &  1.2e-05 &   &  1.7e-05 &   &  7.8e-06 &   \\ 
% 1 & 59 &  1.1e-05 & 7.2  &  1.3e-05 & 7.9  &  2.7e-06 & 4.5  &  4.9e-06 & 3.4  &  1.9e-06 & 4.1  \\ 
% 2 & 117 &  3.0e-06 & 3.7  &  6.9e-06 & 1.8  &  6.4e-07 & 4.3  &  1.5e-06 & 3.2  &  5.0e-07 & 3.8  \\ 
% \end{tabular}
% \end{table}



% \begin{table}[h]
% \caption{radial elastic piston with predicted pressure}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 51 &  3.4e-03 &   &  2.0e-03 &   &  2.4e-03 &   &  6.0e-04 &   &  2.4e-03 &   \\ 
% 1 & 76 &  8.8e-04 & 3.9  &  4.4e-04 & 4.5  &  6.6e-04 & 3.7  &  7.9e-05 & 7.6  &  6.6e-04 & 3.7  \\ 
% 2 & 176 &  2.0e-04 & 4.3  &  1.4e-04 & 3.1  &  1.5e-04 & 4.3  &  1.6e-05 & 4.9  &  1.6e-04 & 4.2  \\ 
% 3 & 538 &  4.9e-05 & 4.2  &  4.7e-05 & 3.0  &  4.3e-05 & 3.6  &  4.4e-06 & 3.7  &  4.3e-05 & 3.6  \\ 
% 4 & 1910 &  1.2e-05 & 4.0  &  1.6e-05 & 3.0  &  1.1e-05 & 3.8  &  1.3e-06 & 3.3  &  1.1e-05 & 3.8  \\ 
% \end{tabular}
% \end{table}

% \begin{table}[h]
% \caption{radial elastic piston without predicted pressure}
% \begin{tabular}{cccccccccccc}
% $g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
% \hline
% 0 & 51 &  3.4e-03 &   &  1.9e-03 &   &  2.5e-03 &   &  5.9e-04 &   &  2.4e-03 &   \\ 
% 1 & 76 &  8.9e-04 & 3.9  &  3.7e-04 & 5.0  &  6.6e-04 & 3.7  &  7.5e-05 & 7.9  &  6.6e-04 & 3.7  \\ 
% 2 & 176 &  2.1e-04 & 4.3  &  1.2e-04 & 3.1  &  1.5e-04 & 4.3  &  1.6e-05 & 4.7  &  1.6e-04 & 4.2  \\ 
% \end{tabular}
% \end{table}

\FloatBarrier
\subsection{1/6/17 benchmark}

New: enforce exact divergence and robin condition for ghost. 
$\rho = 1, \rhos = \mus = \lambdas = \delta$
\bigskip

cgmp elasticPiston -g=elasticPistonGride2.order2p.hdf -addedMass=1 -scf=.1 -nu=.01 -tp=.25 -tf=.25 -smVariation=g -debug=1 -debug=3 -tsINS=pc -cfl=.9 

\FloatBarrier
\begin{table}[h]
\caption{elastic piston, $\delta = .1$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 30 &  2.3e-05 &   &  5.4e-06 &   &  1.3e-05 &   &  7.8e-06 &   &  7.8e-06 &   \\ 
1 & 59 &  5.7e-06 & 4.1  &  1.4e-06 & 4.0  &  3.2e-06 & 4.1  &  1.9e-06 & 4.1  &  1.9e-06 & 4.2  \\ 
2 & 117 &  1.4e-06 & 4.1  &  3.4e-07 & 4.0  &  7.9e-07 & 4.1  &  4.8e-07 & 4.0  &  4.5e-07 & 4.2  \\ 
3 & 357 &  1.5e-07 & 9.4  &  2.9e-08 & 11.8  &  1.4e-07 & 5.7  &  1.0e-07 & 4.6  &  8.0e-08 & 5.6  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialElasticPiston -g=radialElasticPistonGride1.order2.hdf -addedMass=1 -scf=1 -nu=.05 -tp=.01 -tf=.25 -smVariation=g -debug=1 -tsINS=pc -cdv=1 -smoothInterface=0 -go=halt
\FloatBarrier
\begin{table}[h]
\caption{radial elastic piston, $\delta = 1$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 51 &  3.5e-03 &   &  2.0e-03 &   &  2.4e-03 &   &  5.9e-04 &   &  2.4e-03 &   \\ 
1 & 76 &  8.8e-04 & 4.0  &  4.4e-04 & 4.5  &  6.6e-04 & 3.7  &  7.9e-05 & 7.5  &  6.6e-04 & 3.7  \\ 
2 & 176 &  2.0e-04 & 4.3  &  1.4e-04 & 3.1  &  1.5e-04 & 4.3  &  1.6e-05 & 4.9  &  1.6e-04 & 4.2  \\ 
3 & 538 &  4.9e-05 & 4.2  &  4.7e-05 & 3.0  &  4.3e-05 & 3.6  &  4.4e-06 & 3.7  &  4.3e-05 & 3.6  \\ 
4 & 1910 &  1.2e-05 & 4.0  &  1.6e-05 & 3.0  &  1.1e-05 & 3.8  &  1.3e-06 & 3.3  &  1.1e-05 & 3.8  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=2
\begin{table}[h]
\caption{radial traveling wave, light solid, $\delta = .001$, $n=3$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 64 &  2.4e-07 &   &  2.8e-07 &   &  1.1e-05 &   &  8.7e-05 &   &  1.5e-07 &   \\ 
1 & 154 &  9.1e-08 & 2.7  &  1.1e-07 & 2.6  &  4.0e-06 & 2.7  &  3.8e-05 & 2.3  &  1.2e-07 & 1.2  \\ 
2 & 463 &  5.7e-08 & 1.6  &  4.3e-08 & 2.4  &  1.6e-06 & 2.5  &  1.6e-05 & 2.3  &  8.0e-08 & 1.5  \\ 
3 & 1669 &  2.3e-08 & 2.5  &  1.7e-08 & 2.5  &  5.4e-07 & 3.0  &  7.8e-06 & 2.1  &  3.3e-08 & 2.4  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=0
\FloatBarrier
\begin{table}[h]
\caption{radial traveling wave, medium solid, $\delta = 1$, $n=3$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 64 &  1.8e-07 &   &  1.1e-07 &   &  1.3e-07 &   &  6.9e-08 &   &  1.1e-07 &   \\ 
1 & 154 &  4.5e-08 & 4.1  &  2.9e-08 & 3.9  &  3.9e-08 & 3.3  &  1.7e-08 & 4.1  &  3.9e-08 & 2.9  \\ 
2 & 463 &  1.2e-08 & 3.9  &  8.4e-09 & 3.5  &  1.2e-08 & 3.3  &  4.7e-09 & 3.6  &  1.3e-08 & 3.1  \\ 
3 & 1669 &  2.7e-09 & 4.2  &  2.1e-09 & 4.0  &  2.8e-09 & 4.2  &  1.3e-09 & 3.5  &  3.3e-09 & 3.8  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=1
\FloatBarrier
\begin{table}[h]
\caption{radial traveling wave, heavy solid, $\delta =1000$, $n=3$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 64 &  4.1e-07 &   &  1.0e-07 &   &  4.7e-05 &   &  2.8e-08 &   &  4.8e-05 &   \\ 
1 & 154 &  1.9e-07 & 2.2  &  2.5e-08 & 4.1  &  1.3e-05 & 3.7  &  7.2e-09 & 4.0  &  1.2e-05 & 4.1  \\ 
2 & 463 &  1.1e-07 & 1.7  &  7.6e-09 & 3.3  &  4.1e-06 & 3.1  &  2.0e-09 & 3.5  &  3.3e-06 & 3.6  \\ 
3 & 1669 &  5.6e-08 & 2.0  &  3.0e-09 & 2.5  &  1.3e-06 & 3.2  &  5.8e-10 & 3.5  &  1.1e-06 & 3.2  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialShearFlow -g=radialElasticPistonGride1.order2.hdf -tp=.0001 -tf=.0025 -smVariation=g -debug=1 -debug=3 -tsINS=pc -go=halt -cfl=.9 -muFluid=10. -muSolid=10. -rhoSolid=10. -nu=10. -lambdaSolid=10. -useTP=0 -addedMass=1 -amp=.001
\FloatBarrier
\begin{table}[h]
\caption{radial shear flow, $\delta=10$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 76 &  4.9e-09 &   &  3.5e-10 &   &  2.5e-07 &   &  1.2e-09 &   &  2.3e-07 &   \\ 
1 & 126 &  8.1e-10 & 6.1  &  1.2e-10 & 2.9  &  1.8e-08 & 14.1  &  6.1e-10 & 2.0  &  2.2e-08 & 10.2  \\ 
2 & 351 &  2.4e-10 & 3.4  &  4.7e-11 & 2.6  &  7.3e-09 & 2.5  &  2.4e-10 & 2.5  &  7.3e-09 & 3.1  \\ 
3 & 1101 &  1.2e-10 & 2.0  &  1.5e-11 & 3.2  &  2.6e-09 & 2.8  &  7.3e-11 & 3.3  &  2.6e-09 & 2.8  \\ 
\end{tabular}
\end{table}
\FloatBarrier

\subsection{1/10/18}

cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=3

\FloatBarrier
\begin{table}[h]
\caption{$\delta = 1000, n = 1$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 64 &  1.5e-07 &   &  1.1e-08 &   &  5.5e-06 &   &  2.1e-09 &   &  6.1e-06 &   \\ 
1 & 154 &  6.2e-08 & 2.5  &  2.9e-09 & 3.8  &  1.6e-06 & 3.5  &  6.2e-10 & 3.4  &  1.9e-06 & 3.3  \\ 
2 & 463 &  2.9e-08 & 2.1  &  9.3e-10 & 3.1  &  4.5e-07 & 3.5  &  1.8e-10 & 3.5  &  5.7e-07 & 3.2  \\ 
3 & 1669 &  1.2e-08 & 2.4  &  4.4e-10 & 2.1  &  1.2e-07 & 3.6  &  5.0e-11 & 3.5  &  1.7e-07 & 3.4  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=4
\FloatBarrier
\begin{table}[h]
\caption{$\delta = 10, n = 1$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 64 &  4.0e-08 &   &  8.8e-09 &   &  6.7e-08 &   &  2.4e-09 &   &  7.8e-08 &   \\ 
1 & 154 &  1.2e-08 & 3.3  &  2.9e-09 & 3.0  &  1.9e-08 & 3.5  &  7.1e-10 & 3.4  &  2.3e-08 & 3.3  \\ 
2 & 463 &  3.7e-09 & 3.3  &  1.0e-09 & 2.9  &  5.4e-09 & 3.5  &  2.0e-10 & 3.6  &  7.0e-09 & 3.4  \\ 
3 & 1669 &  1.0e-09 & 3.6  &  3.3e-10 & 3.1  &  1.5e-09 & 3.7  &  5.5e-11 & 3.6  &  2.0e-09 & 3.6  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=5
\begin{table}[h]
\caption{$\delta = .1, n = 1$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 64 &  9.5e-08 &   &  1.9e-07 &   &  1.2e-07 &   &  7.5e-07 &   &  1.3e-07 &   \\ 
1 & 154 &  3.1e-08 & 3.1  &  7.3e-08 & 2.6  &  8.0e-08 & 1.6  &  3.9e-07 & 1.9  &  7.8e-08 & 1.6  \\ 
2 & 463 &  9.1e-09 & 3.4  &  2.7e-08 & 2.7  &  3.6e-08 & 2.2  &  1.9e-07 & 2.1  &  3.5e-08 & 2.2  \\ 
3 & 1669 &  3.2e-09 & 2.8  &  1.1e-08 & 2.6  &  1.3e-08 & 2.8  &  7.4e-08 & 2.6  &  1.3e-08 & 2.7  \\ 
\end{tabular}
\end{table}
\FloatBarrier
cgmp radialTravelingWave -g=radialTravelingWaveGride1.order2.hdf -addedMass=1 -tf=.3 -tp=.1 -amp=.00001 -caseid=6
\FloatBarrier
\begin{table}[h]
\caption{$\delta = 1$, $n=1$}
\begin{tabular}{cccccccccccc}
$g$ & $N_t$ & $p$ & ratio  &  $\vv$ & ratio  &  $\usv$ & ratio  &  $\vsv$ & ratio  &  $\sigmasv$ & ratio  \\ 
\hline
0 & 64 &  1.4e-08 &   &  7.1e-09 &   &  1.7e-08 &   &  5.6e-09 &   &  2.0e-08 &   \\ 
1 & 154 &  3.6e-09 & 3.8  &  1.7e-09 & 4.3  &  4.6e-09 & 3.6  &  1.5e-09 & 3.7  &  5.7e-09 & 3.5  \\ 
2 & 463 &  9.9e-10 & 3.6  &  6.2e-10 & 2.7  &  1.2e-09 & 3.7  &  4.0e-10 & 3.8  &  1.6e-09 & 3.6  \\ 
3 & 1669 &  2.3e-10 & 4.2  &  2.1e-10 & 2.9  &  3.1e-10 & 4.0  &  1.1e-10 & 3.7  &  4.1e-10 & 3.9  \\ 
\end{tabular}
\end{table}
\FloatBarrier

==> texFiles/cornerRegularization.tex <==
\subsection{Regularization at a fluid-solid corner}


% For the velocity, the amp conditions are applied to obtain the ghost point on the interface line.
% this may not be necessary...
% \begin{align}
% \tv^T_m \tauv_\iv^{n+1} \nv + \zs \tv^T_m \vv_{\tilde{\iv}}^{n+1}
% &=
% \tv^T_m \sigmasv_\iv^{n+1} \nv + \zs \tv^T_m \vsv_{\tilde{\iv}}^{n+1} \\
% \grad_h \cdot \vv_\iv^{n+1} &= 0
% \end{align}
% \begin{align}
% \mu (D_{0,x} (v_2)_{0,0}^{n+1} + D_{0,y} (v_1)_{0,0}^{n+1}) - \zs (v_2)_{-1,0}^{n+1}
% &= \dots \\
% D_{0,x} (v_1)_{0,0} + D_{0,y} (v_2)_{0,0} &= 0
% \end{align}

In the solid, the zero-displacement and interface boundary conditions are incompatible 
if there is a non-zero traction at the corner. 
We can apply a numerical fix-up in two places to avoid wiggles.
The approach is to treat the fluid and solid interfaces as free surfaces near the corners.
The modified pressure condition \wdh{at the predictor stage} is
\begin{align}
-p_\iv^{(p)}
-\frac{\zp \dt}{\rho} (\nv\cdot\Grad) p_\iv^{(p)}
&= 
{ \eta_\iv}\, \nv^T \left(  \Sigmasv_\isv^{(p)} \nv - \tauv_\iv^{(p)} \nv\right)
\nonumber \\
&\qquad + \zp \dt
 \nv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} + (\vsv_t)_\isv^{(p)}\right), \qquad \iv \in \GammaIFh,
\end{align}
%
and the modified solid stress condition \wdh{sets the solid traction at the predictor stage using }
\begin{align}
\nv^T \sigmasv_\isv^{(p)} \nv \leftarrow  {\eta_\isv} \, \nv^T (\sigmav^I)_\isv \nv .
\end{align}
%
\wdh{Similar alterations are made at the corrector stage.}
In the regularized interface conditions, a ramp function is introduced which goes to zero near the fluid-solid corner
and goes to one away from the corner, 
\old{
\begin{align}
\eta_\iv = 1 - \sum_{corners} \exp(-\gamma \|\xv_\iv - \xv_{\text{corner}}\|^2) .
\end{align}
}
\wdh{wdh: I think what you have is the same as using a distance in index space. I like a slower decay from
  the corner so as to be a bit smoother (use distance as opposed to square-distance):
\begin{align}
\eta_\iv = 1 - \sum_{corners} \exp(- \beta |\iv - \iv_{\text{corner}}| ) .
\end{align}
}


\input texFiles/cornerFixFig

\wdh{
It also seems more robust to also modify the solid velocity and displacement,
\begin{align}
 & \sigmasv_\isv^{I} \nv \leftarrow  {\eta_\isv} \, \sigmav^I_\isv \nv , \\
 & \vsv_\isv^{I} \leftarrow  {\eta_\isv} \, \vsv^I_\isv,  \\
 & \usv_\isv^{(p)} \leftarrow  {\eta_\isv} \, \usv^{(p)}_\isv , 
\end{align}
as this will keep fixed the angle at which the interface meets the wall.
}
%

\wdh{With no regularization, numerical wiggles occur in only a few grid points near the corners.}
Therefore, we choose $\gamma$ to be proportional to $\frac{1}{h^2}.$ 
Due to this choice, $\eta_\iv$ only affects a fixed number of grid points near the corner
as the grid is refined.  \wdh{The regularization will thus affect a smaller and smaller region near the
  fluid-solid corner as the mesh is refined.}




==> texFiles/deformingChannel.tex <==
\section{Results for a deforming channel}


% ----------------------------------------------------------------------------------
\subsection{Elastic-piston: slipWalls}

We consider a initially rectangular shaped elastic solid on top of a rectangular fluid channel.

\medskip
\noindent Notes
\begin{enumerate}
  \item Fluid: slip walls on left and right.
  \item Solid: slip walls on left and right.
  \item Solid: $\rhos=100$, $\lambda=\mu=1$. 
  \item Ramped pressure at bottom.
  \item Solid undergoes a repeating compression and expansion that slowly decays
\end{enumerate}


\input texFiles/deformingChannelSlipWallsGridsFig.tex




% ----------------------------------------------------------------------------------
\clearpage
\subsection{Fixed ends}

In this example the side walls are no-slip for the fluid and zero-displacement for the solid.


\input texFiles/deformingChannelNoSlipWallsGridsFig.tex


==> texFiles/deformingChannelNoSlipWallsGridsFig.tex <==
{% ------ DEFORMING CHANNEL - SLIP WALLS   ------
% 
% --------- START drawContour -----------
\newcommand{\drawContour}[7]{%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{deformingChannel/#2}{\figWidth}};
  % \draw(.5,.5) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #3};
  % \draw(0,0.0) node[draw,fill=white,anchor=south west,xshift=12pt,yshift=12pt] {\scriptsize #4};
  \draw(.75,.25) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #5};
 % colour bar:
%- \begin{scope}[xshift=9pt]
%-   \draw (\xcb,\ycb) node[anchor=south west,xshift=0.cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
%-   \draw (.8,0) node[anchor=north,xshift=+3pt,yshift=+2pt] {\scriptsize $#6$};
%-   \draw (4.4,0) node[anchor=north,xshift=+0pt,yshift=+2pt] {\scriptsize $#7$};
%- \end{scope}
% \draw (\xcb,\ycb) node[anchor=south west,xshift= +8pt,yshift=+1pt] {\scriptsize $#6$};
% \draw (\xcb,\ycbTop) node[anchor=south west,xshift= +8pt,yshift=-6pt] {\scriptsize $#7$};
\end{scope}
}
% --------- END drawContour -----------
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{4cm}% colour bar height
\newcommand{\xcb}{.5cm}% colour bar lower left corner
\newcommand{\ycb}{-.2cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*\real{.5}}% colour bar top label position
% \newcommand{\xLabel}{6.5cm}% label position
% \newcommand{\yLabel}{6.5cm}% label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
% ========================= DRAW ================
%
\newcommand{\figWidth}{5cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.095}{.0975}{.175}{.175}}
\begin{figure}[htb]
\begin{center}
\resizebox{14cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.4,.5) rectangle (16.,9);  % set the bounding box (so we have less surrounding white space)
%  top row: 
 \begin{scope}[yshift=4.5cm]
   \drawContour{xshift= 0.0cm}{deformingChannelPinnedG4t0p0Grids}{$p$}{$p$}{$t=0.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelPinnedG4t2p0Grids}{$p$}{$p$}{$t=2.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelPinnedG4t4p0Grids}{$p$}{$p$}{$t=4.0$}{-.026}{.719};
 \end{scope}
 \begin{scope}
   \drawContour{xshift= 0.0cm}{deformingChannelPinnedG4t5p0Grids}{$p$}{$p$}{$t=5.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelPinnedG4t6p0Grids}{$p$}{$p$}{$t=6.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelPinnedG4t9p0Grids}{$p$}{$p$}{$t=9.0$}{-.026}{.719};
 \end{scope}
% 
% grid:
% \draw[step=1cm,gray] (0,0) grid (16,9);
\end{tikzpicture}
}% end resize box
\end{center}
  \caption{Deforming channel: elastic solid on top of an incompressible fluid.}
  \label{fig:deformingChannelPinnedGrids}
\end{figure}
}


==> texFiles/deformingChannelSlipWallsGridsFig.tex <==
{% ------ DEFORMING CHANNEL - SLIP WALLS   ------
% 
% --------- START drawContour -----------
\newcommand{\drawContour}[7]{%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{deformingChannel/#2}{\figWidth}};
  % \draw(.5,.5) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #3};
  % \draw(0,0.0) node[draw,fill=white,anchor=south west,xshift=12pt,yshift=12pt] {\scriptsize #4};
  \draw(.75,.25) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #5};
 % colour bar:
%- \begin{scope}[xshift=9pt]
%-   \draw (\xcb,\ycb) node[anchor=south west,xshift=0.cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
%-   \draw (.8,0) node[anchor=north,xshift=+3pt,yshift=+2pt] {\scriptsize $#6$};
%-   \draw (4.4,0) node[anchor=north,xshift=+0pt,yshift=+2pt] {\scriptsize $#7$};
%- \end{scope}
% \draw (\xcb,\ycb) node[anchor=south west,xshift= +8pt,yshift=+1pt] {\scriptsize $#6$};
% \draw (\xcb,\ycbTop) node[anchor=south west,xshift= +8pt,yshift=-6pt] {\scriptsize $#7$};
\end{scope}
}
% --------- END drawContour -----------
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{4cm}% colour bar height
\newcommand{\xcb}{.5cm}% colour bar lower left corner
\newcommand{\ycb}{-.2cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*real{0.5}}% colour bar top label position
% \newcommand{\xLabel}{6.5cm}% label position
% \newcommand{\yLabel}{6.5cm}% label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
% ========================= DRAW ================
%
\newcommand{\figWidth}{5cm}
\newcommand{\trimfig}[2]{\trimw{#1}{#2}{.095}{.0975}{.175}{.175}}
\begin{figure}[htb]
\begin{center}
\resizebox{14cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.4,.5) rectangle (16.,9);  % set the bounding box (so we have less surrounding white space)
%  top row: 
 \begin{scope}[yshift=4.5cm]
   \drawContour{xshift= 0.0cm}{deformingChannelG4t0p0Grids}{$p$}{$p$}{$t=0.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelG4t2p0Grids}{$p$}{$p$}{$t=2.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelG4t4p0Grids}{$p$}{$p$}{$t=4.0$}{-.026}{.719};
 \end{scope}
 \begin{scope}
   \drawContour{xshift= 0.0cm}{deformingChannelG4t5p0Grids}{$p$}{$p$}{$t=5.0$}{-.223}{.242};
   \drawContour{xshift=5.25cm}{deformingChannelG4t6p0Grids}{$p$}{$p$}{$t=6.0$}{-.141}{.444};
   \drawContour{xshift=10.5cm}{deformingChannelG4t9p0Grids}{$p$}{$p$}{$t=9.0$}{-.026}{.719};
 \end{scope}
% 
% grid:
% \draw[step=1cm,gray] (0,0) grid (16,9);
\end{tikzpicture}
}% end resize box
\end{center}
  \caption{Deforming channel: elastic solid on top of an incompressible fluid.}
  \label{fig:deformingChannelGrids}
\end{figure}
}


==> texFiles/defs-orig.tex <==
\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green}}
% 
\renewcommand{\url}[1]{}% ******** Remove URL's from bibtex entries ********
\newcommand{\citeCount}[1]{}% for citation counts papers for WDH citations
% 
% 
\newcommand{\f}[2]{\frac{#1}{#2}}% \frac short form
\newcommand{\pr}{\partial} % short for partial
%
\newtheorem{theorem}{Theorem}
\newtheorem{Algorithm}{Algorithm}
\newtheorem{procedure}{Procedure}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
\newtheorem{condition}{Condition}
% \newtheorem{AMPInterfaceCondition}{AMP Interface Condition}
\newtheorem{AMPInterfaceCondition}{Interface Condition}
\newtheorem{modelProblem}{Model Problem}
\newtheorem{travelingWave}{Traveling Wave Exact Solution}

\newtheorem*{algorithmAMP}{AMP Algorithm (added-mass partitioned)}
\newtheorem*{algorithmTP}{TP Algorithm (traditional partitioned)}

\newtheorem*{ModelProblemIA}{Model Problem MP-IA}
\newtheorem*{ModelProblemVA}{Model Problem MP-VA}
\newtheorem*{ModelProblemVE}{Model Problem MP-VE}

\newcommand{\dx}{\Delta x}
\newcommand{\dxs}{{\Delta \bar{x}}}
\newcommand{\dy}{\Delta y}
\newcommand{\dt}{\Delta t}

\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}

% \newcommand{\kappaR}{{\rhoR\cR^2}}

\newcommand{\Dp}{D_{+}}
\newcommand{\Dm}{D_{-}}
\newcommand{\Dpx}{D_{+x}}
\newcommand{\Dmx}{D_{-x}}
\newcommand{\Dpy}{D_{+y}}
\newcommand{\Dmy}{D_{-y}}

\newcommand{\erf}{\operatorname{erf}}

    
\newcommand{\bogus}[1]{{}}

% -----Bill's common definitions-----

\newcommand{\av}{\mathbf{ a}}
\newcommand{\bv}{\mathbf{ b}}
\newcommand{\cv}{\mathbf{ c}}
\newcommand{\dv}{\mathbf{ d}}
\newcommand{\ev}{\mathbf{ e}}
\newcommand{\fv}{\mathbf{ f}}
\newcommand{\gv}{\mathbf{ g}}
\newcommand{\hv}{\mathbf{ h}}
\newcommand{\iv}{\mathbf{ i}}
\newcommand{\jv}{\mathbf{ j}}
\newcommand{\kv}{\mathbf{ k}}
\newcommand{\lv}{\mathbf{ l}}
\newcommand{\mv}{\mathbf{ m}}
\newcommand{\nv}{\mathbf{ n}}
\newcommand{\ov}{\mathbf{ o}}
\newcommand{\pv}{\mathbf{ p}}
\newcommand{\qv}{\mathbf{ q}}
\newcommand{\rv}{\mathbf{ r}}
\newcommand{\sv}{\mathbf{ s}}
\newcommand{\tv}{\mathbf{ t}}
\newcommand{\uv}{\mathbf{ u}}
\newcommand{\vv}{\mathbf{ v}}
\newcommand{\wv}{\mathbf{ w}}
\newcommand{\xv}{\mathbf{ x}}
\newcommand{\yv}{\mathbf{ y}}
\newcommand{\zv}{\mathbf{ z}}
% 
\newcommand{\Av}{\mathbf{ A}}
\newcommand{\Bv}{\mathbf{ B}}
\newcommand{\Cv}{\mathbf{ C}}
\newcommand{\Dv}{\mathbf{ D}}
\newcommand{\Ev}{\mathbf{ E}}
\newcommand{\Fv}{\mathbf{ F}}
\newcommand{\Gv}{\mathbf{ G}}
\newcommand{\Hv}{\mathbf{ H}}
\newcommand{\Iv}{\mathbf{ I}}
\newcommand{\Jv}{\mathbf{ J}}
\newcommand{\Kv}{\mathbf{ K}}
\newcommand{\Lv}{\mathbf{ L}}
\newcommand{\Mv}{\mathbf{ M}}
\newcommand{\Nv}{\mathbf{ N}}
\newcommand{\Ov}{\mathbf{ O}}
\newcommand{\Pv}{\mathbf{ P}}
\newcommand{\Qv}{\mathbf{ Q}}
\newcommand{\Rv}{\mathbf{ R}}
\newcommand{\Sv}{\mathbf{ S}}
\newcommand{\Tv}{\mathbf{ T}}
\newcommand{\Uv}{\mathbf{ U}}
\newcommand{\Vv}{\mathbf{ V}}
\newcommand{\Wv}{\mathbf{ W}}
\newcommand{\Xv}{\mathbf{ X}}
\newcommand{\Yv}{\mathbf{ Y}}
\newcommand{\Zv}{\mathbf{ Z}}

\newcommand{\collon}{:}  % note \colon already defined by someone.
\newcommand{\ff}{\tt}

% \newcommand{\lt}{{<}}
% \newcommand{\grad}{\nabla}
% \newcommand{\comma}{~~~,~~}
% \newcommand{\calo}{{\cal O}}

\newcommand{\half}{{1\over2}}

\newcommand{\Real}{{\mathbb R}}
\newcommand{\Complex}{{\mathbb C}}

\newcommand{\zerov}{\mathbf{0}}


\newcommand{\Ac}{{\mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Dc}{{\mathcal D}}
\newcommand{\Ec}{{\mathcal E}}
\newcommand{\Ic}{{\mathcal I}}
\newcommand{\Rc}{{\mathcal R}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Lc}{{\mathcal L}}
\newcommand{\Nc}{{\mathcal N}}
\newcommand{\Oc}{{\mathcal O}}

\newcommand{\deltav}{\boldsymbol{\delta}}
\newcommand{\omegav}{\boldsymbol{\omega}}
\newcommand{\tauv}{\boldsymbol{\tau}}
\newcommand{\phiv}{\boldsymbol{\phi}}
\newcommand{\thetav}{\boldsymbol{\theta}}
\newcommand{\psiv}{\boldsymbol{\psi}}
\newcommand{\sigmav}{\boldsymbol{\sigma}}
\newcommand{\chiv}{\boldsymbol{\chi}}
\newcommand{\epsilonv}{\boldsymbol{\varepsilon}}
\newcommand{\epsilonsv}{\bar{\boldsymbol{\varepsilon}}}

\newcommand{\grad}{\nabla}
\newcommand{\curl}{\times}
\newcommand{\grads}{\nabla_{\xsv}}

\newcommand{\tableFont}{\scriptsize}
\newcommand{\tableFontSize}{\small}
\newcommand{\num}[2]{#1e#2} % Use this macro to define the format of the numbers in the table
\newcommand{\eem}{e^{(j)}}
\newcommand{\rateLabel}{rate}

\clearpage
\newcommand{\dtau}{\delta_\tau}
\newcommand{\Gb}{G}


\newcommand{\rhos}{\bar{\rho}}
\newcommand{\cp}{\bar{c}_p}
\newcommand{\cs}{\bar{c}_s}
\newcommand{\kappas}{{\rhos\cs^2}}
\newcommand{\zs}{{\bar {z}}}  % solid impedance based on c_p
\newcommand{\zp}{z_p}  % solid impedance based on c_s
\newcommand{\us}{\bar{u}}
\newcommand{\rs}{\bar{r}}
\newcommand{\qs}{\bar{q}}
\newcommand{\vs}{\bar{v}}
\newcommand{\sigmas}{\bar{\sigma}}
\newcommand{\bsv}{\bar{\bv}}
\newcommand{\xs}{\bar{x}}
\newcommand{\xsv}{\bar{\xv}}
\newcommand{\ys}{{\bar{y}}}
\newcommand{\ysv}{\bar{\yv}}
\newcommand{\xf}{{x}}
% \newcommand{\dxs}{\Delta{\bar x}}
\newcommand{\dxf}{{\Delta x}}
\newcommand{\Ns}{\bar{N}}
\newcommand{\Nf}{{N}}
\newcommand{\zf}{z_f}

% ---- DAS definitions ---- $
% solid definition in analysis
\newcommand{\ssy}{\bar{\sigma}_{22}}
\newcommand{\ssx}{\bar{\sigma}_{21}}
\newcommand{\vsy}{\vs_{2}}
\newcommand{\vfy}{v_{2}}

% hat variables in fluid and solid (Fourier)
\newcommand{\ssyh}{\hat{\bar{\sigma}}_{22}}
\newcommand{\ssxh}{\hat{\bar{\sigma}}_{21}}
\newcommand{\vsyh}{\hat{\bar{v}}_2}
\newcommand{\vfyh}{\hat{v}_2}
% \newcommand{\ph}{\hat{p}}

% characteristic variables
% \newcommand{\ac}{\bar{a}}
% \newcommand{\bc}{\bar{b}}
% \newcommand{\dc}{\bar{d}}
\newcommand{\ac}{a}
\newcommand{\bc}{b}
\newcommand{\dc}{d}
\newcommand{\acv}{\mathbf{\ac}}

% effective fluid height
\newcommand{\Heff}{H_{\text{eff}}}

% analysis
\newcommand{\p}{\phi} % spacial eigenvalue
\newcommand{\rev}{\mathbf{r}} % spacial eigenvector
\newcommand{\qn}[1]{q_{#1}}
\newcommand{\rn}[1]{r_{#1}}

% tilde variables
\newcommand{\tac}{\tilde{\ac}}
\newcommand{\tbc}{\tilde{\bc}}
\newcommand{\tdc}{\tilde{\dc}}
\newcommand{\tacv}{\tilde{\acv}}

% determinant condition
\newcommand{\dComp}{g}
\newcommand{\dMat}{\mathcal{G}}

% environment for algorithm
\newcommand{\listAlgorithm}[2]{
\noindent \hrulefill \\
\noindent \textit{#1:}
\begin{enumerate}
#2
\end{enumerate}
\noindent \hrulefill
}

% arg min definition
\DeclareMathOperator*{\argmin}{arg\,min}



% ---------------- $

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% defs for discrete variables
\newcommand{\Usv}{\bar{\uv}}
\newcommand{\Vsv}{\bar{\vv}}
\newcommand{\Fsv}{\bar{\Fv}}
\newcommand{\Gsv}{\bar{\gv}}
\newcommand{\Qsv}{\bar{\qv}}
\newcommand{\Hsv}{\bar{\Hv}}
\newcommand{\Sigmasv}{\bar{\sigmav}}
\newcommand{\Tauv}{\tauv}
\newcommand{\Grad}{\grad_h}
\newcommand{\Grads}{\bar{\grad}_h}
\newcommand{\ivs}{{\bar{\iv}}}
\newcommand{\isv}{{\bar{\iv}}}
\newcommand{\Sigmav}{{\sigmav}}

\newcommand{\usv}{\bar{\uv}}
\newcommand{\vsv}{\bar{\vv}}
\newcommand{\wsv}{\bar{\wv}}

\newcommand{\ush}{\hat{\us}}
\newcommand{\usvh}{\hat{\usv}}
\newcommand{\vvh}{\hat{\vv}}
\newcommand{\vh}{\hat{v}}
\newcommand{\ph}{\hat{p}}

\newcommand{\nsv}{\bar{\nv}}
\newcommand{\esv}{\bar{\ev}}
\newcommand{\vvs}{\bar{\vv}}
\newcommand{\uvs}{\bar{\uv}}
\newcommand{\xvs}{\bar{\xv}}
\newcommand{\sigmavs}{\bar{\sigmav}}
\newcommand{\sigmasv}{\bar{\sigmav}}
\newcommand{\fsv}{\bar{\fv}}
\newcommand{\qsv}{\bar{\qv}}

\newcommand{\qsvp}{\qsv^p}
\newcommand{\qsvI}{\qsv^I}
\newcommand{\qvI}{\qv^I}

\newcommand{\vvI}{\vv^I}
\newcommand{\tauvI}{\tauv^I}
\newcommand{\vvIf}{\vv^f}
\newcommand{\tauvIf}{\tauv^f}
% \newcommand{\vvIf}{\vv^{I,f}}
\newcommand{\sigmavI}{\sigmav^I}
\newcommand{\vsvIs}{\vsv^s}
\newcommand{\sigmavIs}{\sigmav^s}

\newcommand{\dvel}{{\delta_v}}
\newcommand{\vDot}{\dot{v}}
\newcommand{\vsDot}{\dot{\vs}}
\newcommand{\vvDot}{\dot{\vv}}
\newcommand{\vsvDot}{\dot{\vsv}}

% \newcommand{\rb}{r_b} % a point on the body surface

% \newcommand{\amp}{{\mathcal{A}}}
\newcommand{\amp}{A}
\newcommand{\ampI}{A} % amplification factor for iterations



% \newcommand{\Energy}{\mathcal{E}}% Energy of the fluid
% \newcommand{\Area}{\mathcal{A}_b}
% \newcommand{\Area}{A_b}
% \newcommand{\width}{\mathcal{W}}
% \newcommand{\width}{w_b}


\newcommand{\charSpeed}{s}% Char. speed
\newcommand{\charVar}{\chi}% Char. variable


\newcommand{\largess}{\sffamily\large}
\newcommand{\Largess}{\sffamily\Large}
\newcommand{\bfss}{\sffamily\bfseries}
\newcommand{\smallss}{\sffamily\small}
\newcommand{\normalss}{\sffamily}
\newcommand{\scriptsizess}{\sffamily\scriptsize}

\newcommand{\hs}{h_s}
% \newcommand{\Hs}{H_s}
\newcommand{\Hs}{\bar{H}}

\newcommand{\kxHat}{\hat{k}_x}
\newcommand{\kyHat}{\hat{k}_y}
\newcommand{\omegaHat}{\hat{\omega}}
\newcommand{\aHat}{\hat{a}}
\newcommand{\bHat}{\hat{b}}

\newcommand{\aTilde}{\tilde{a}}
\newcommand{\bTilde}{\tilde{b}}

\newcommand{\qsHat}{\hat{\qs}}
\newcommand{\phase}{x_0}
\newcommand{\phaset}{t_0}

\newcommand{\as}{\bar{a}}
\newcommand{\bs}{\bar{b}}
\newcommand{\ds}{\bar{d}}
\newcommand{\asHat}{\hat{\as}}
\newcommand{\bsHat}{\hat{\bs}}
\newcommand{\dsHat}{\hat{\ds}}

\newcommand{\dHat}{\hat{d}}
\newcommand{\pHat}{\hat{p}}
\newcommand{\qHat}{\hat{q}}
\newcommand{\vHat}{\hat{v}}
\newcommand{\vvHat}{\hat{\vv}}
\newcommand{\vsHat}{\hat{\vs}}
\newcommand{\sigmaHat}{\hat{\sigma}}
\newcommand{\sigmasHat}{\hat{\sigmas}}

\newcommand{\lambdas}{\bar{\lambda}}% solid Lame' parameter
\newcommand{\mus}{\bar{\mu}}% solid Lame' parameter

\newcommand{\OmegaF}{\Omega^F}% fluid domain
\newcommand{\OmegaS}{\Omega^S}% solid domain

\newcommand{\OmegaFh}{\Omega^F_h}% fluid domain
\newcommand{\OmegaSh}{\Omega^S_h}% solid domain

\newcommand{\GammaI}{\Gamma}% Fluid-Solid Interface
\newcommand{\GammaIs}{\Gamma^S}% Fluid-Solid Interface
\newcommand{\GammaIf}{\Gamma^F}% Fluid-Solid Interface
\newcommand{\GammaIfh}{\Gamma^F_h}% Fluid-Solid Interface
\newcommand{\GammaIsh}{\Gamma^S_h}% Fluid-Solid Interface
\newcommand{\GammaIFh}{\Gamma^F_h}% Fluid-Solid Interface
\newcommand{\GammaISh}{\Gamma^S_h}% Fluid-Solid Interface

\renewcommand{\zp}{\bar{z}_p}
\renewcommand{\zs}{\bar{z}_s}
\newcommand{\zb}{\bar{z}}
\newcommand{\Lt}{\tilde{L}}

\newcommand{\MR}{M_r}% added mass ratio
\newcommand{\Mr}{\mathcal{M}}% another added mass ratio
\newcommand{\Mra}{M}%acoustic mass ratio

\newcommand{\phis}{\phi_s}
\newcommand{\phib}{\phi_b}
% \newcommand{\phit}{\tilde{\phi}}
% \newcommand{\phit}{\phi_<}

\newcommand{\phim}{\phi_-}
\newcommand{\phip}{\phi_+}


\newcommand{\lambday}{\lambda}% 
\newcommand{\lambdax}{\lambda_x}% 

\newcommand{\cb}{\bar{c}}
\newcommand{\kk}{k_x} % wave number of 2d analysis
\newcommand{\kx}{k_x} % wave number of 2d analysis
\newcommand{\ax}{\alpha \amp^{m+1}}
\newcommand{\thetaj}{\theta} % Jeff's theta


% Predicted states:
\newcommand{\vvp}{\vv^p}
\newcommand{\vp}{v^p}
\newcommand{\sigmavp}{\sigmav^p}
\newcommand{\sigmap}{\sigma^p}
\newcommand{\tauvp}{\tauv^p}
\newcommand{\taup}{\tau^p}
\newcommand{\vsvp}{\vsv^p}
\newcommand{\vsp}{\vs^p}
\newcommand{\sigmasvp}{\sigmasv^p}
\newcommand{\sigmasp}{\sigmas^p}


\newcommand{\Achar}{\Ac}% incoming characteristic variable
\newcommand{\Bchar}{\Bc}% characteristic BC operator
\newcommand{\Bcharp}{\Bc_p}% characteristic BC operator

\newcommand{\Af}{A_f}
\newcommand{\Bf}{B_f}
\newcommand{\Df}{\Dc}
\newcommand{\As}{A_s}
\newcommand{\Bs}{B_s}
\newcommand{\Ds}{\bar{\Dc}}


\newcommand{\Ck}{C_k}
\newcommand{\Sk}{S_k}
\newcommand{\Ca}{C_\alpha}
\newcommand{\Sa}{S_\alpha}

\newcommand{\Sas}{S_a}
\newcommand{\Cas}{C_a}
\newcommand{\Sbs}{S_b}
\newcommand{\Cbs}{C_b}

\newcommand{\dsf}{\delta}


\newcommand{\expkw}{e^{i(k x -\omega t)}}
% \newcommand{\ampe}{\Ac_0}% amplitude of exact solution
\newcommand{\ampe}{{\bar u_{{\rm max}}}}


% \newcommand{\nus}{\bar\nu}
% \newcommand{\betas}{\bar\beta}
% \newcommand{\ly}{\ell_y}
% \newcommand{\lx}{\ell_x}
% \newcommand{\ly}{\beta_y}
% \newcommand{\lx}{\beta_x}
% \newcommand{\ly}{\alpha_y}
% \newcommand{\lx}{\alpha_x}
\newcommand{\ly}{\lambda_y}
\newcommand{\lx}{\lambda_x}
% \newcommand{\ly}{\gamma_y}
% \newcommand{\lx}{\gamma_x}

\newcommand{\tanv}{\ev}% tangent 

\newcommand{\strutt}{\rule{0pt}{10pt}}% strutt to make table height bigger


==> texFiles/elasticPiston.tex <==
% \newcommand{\cp}{c_p}
% \newcommand{\xI}{x_I}
\newcommand{\pH}{p_0}
\section{An exact solution for an elastic piston}

We derive an exact solution for a one-dimensional elastic piston by posing a
given motion of the interface $x=\Gb(t)$ and then determining the pressure boundary
condition on the fluid that will result in that motion.

First consider the solution to the one-dimensional IBVP for the wave equation
on strip $x\in[a,b]$,
\begin{align*}
 & \left\{
  \begin{aligned}
   \partial_t \us - \vs &=0 \\
   \rhos\partial_t \vs - \partial_{\xs} \sigmas &=0 \\
  \partial_t \sigmas - \rhos\as^2 \partial_{\xs}\vs  &=0 
 \end{aligned} 
 \right.
, ~~\text{for $\xs\in[a,b]$},  \\
& \us(a,t)=\alpha(t), \quad \us(b,t)=\beta(t), \qquad\text{(boundary conditions)}, \\
& \us(x,t)=\us_0(x), \quad \vs(x,t)=\vs_0(x), \qquad\text{(initial conditions)}.
\end{align*}
\begin{figure}[hbt]
\begin{center}
\begin{tikzpicture}[scale=1]
 \useasboundingbox (-3,-.25) rectangle (3,6);  % set the bounding box (so we have less surrounding white space)
%
  \draw[very thick] (-2,0) -- (-2,5);
  \draw[very thick] (2,0) -- (2,5);
  \draw (-2,0) node[anchor=north] {$a$};
  \draw ( 2,0) node[anchor=north] {$b$};
  \draw (-2,3) node[rotate=90,yshift=+8pt] {$\us=\alpha(t)$};
  \draw ( 2,3) node[rotate=90,yshift=-8pt] {$\us=\beta(t)$};
%
  \draw[->] (-3.5,0)--(2.5,0) node[anchor=north] {$x$};
  \draw[->] (-3.,-.2)--(-3.,6) node[anchor=east] {$t$};
% characteristics
  \draw[blue] (-2,0) -- (2,2) -- (-2,4) -- (2,6);
  \draw[red ] (2,0) -- (-2,2) -- (2,4) -- (-2,6);
%
  \draw (0,.5) node {$A$};
  \draw (-1.25,1.25) node {$B$};
%
%  \draw (-.5,2) node[anchor=south] {$(x,t)$}; 
%  \draw (-.5,2) -- (2,.75) -- (.5,0);
%  \draw (-.5,2) -- (-2,1.25) -- (.5,0);
% grid:
   \draw[step=1cm,gray] (-3,0) grid (3,.);
\end{tikzpicture}
\end{center}
\caption{Wave equation in a strip...}
\label{fig:elasticPistonCartoon}
\end{figure}
%
The solution at a point $P=(x,t)$ can be determined by tracing characteristics.
The characteristic conditions are
\begin{align*}
    w_\pm = \sigmas \mp \zp \vs = \text{const} \quad \text{along $\frac{d x}{d t}=\pm\as$},
\end{align*}
For a point $A$ in region I, the solution is determined from the two conditions
\begin{align*}
  &  w_+(x,t) = w_+(x-\as t,0) = \sigma_0(x-\as t) -\zp \vs_0(x-\as t), \\
  &  w_-(x,t) = w_-(x-\as t,0) = \sigma_0(x+\as t) +\zp \vs_0(x+\as t),
\end{align*}
which gives 
\begin{align*}
    v(x,t) = \half( \vs_0(x-\as t) + \vs_0(x+\as t)) + \frac{1}{2\as}( \sigma_0(x+\as t)-\sigma_0(x-\as t))
\end{align*}
For a point $B$ in region II, the solution is determined from the three equations
\begin{align*}
 &   w_+(x,t) = w_+(x-\as (t-\tau),\tau ) = \sigma+(x-\as (t-\tau),\tau ) -\zp \alpha(\tau), \\
 &   w_-(x,t) = w_-(x-\as t,0) = \sigma_0(x+\as t) +\zp \vs_0(x+\as t), \\
 &   w_-(x-\as (t-\tau),\tau ) = w_-(\xi,0) = \sigma_0(\xi) +\zp \vs_0(\xi)
\end{align*}

Consider a one-dimensional fluid domain $\Omega_F=[\Gb(t),H]$ adjacent to an elastic solid 
on the domain $\Omega_S=[-\Hs,\Gb(t)]$. The governing equations are
\begin{equation}
  \left\{
  \begin{aligned}
   \partial_t \us - \vs &=0 \\
   \rhos\partial_t \vs - \partial_{\xs} \sigmas &=0 \\
  \partial_t \sigmas - \rhos\as^2 \partial_{\xs}\vs  &=0 
 \end{aligned} 
 \right.
, ~~\text{for $\xs\in[-\Hs,0]$}, 
\qquad 
  \left\{
  \begin{aligned}
  \rho (\partial_t v + v \p_x v) + \p_x p &= \mu \p_x^2 v \\
  \p_x v  &=0 \\
 \end{aligned} 
 \right.
, ~~\text{for $x\in[\Gb(t),H]$} , \label{eq:elasticPiston}
\end{equation}




%
% Cartoon showing the grid for the elastic piston
%
\begin{figure}[hbt]
\begin{center}
\begin{tikzpicture}[scale=1]
 \useasboundingbox (-5.,-.5) rectangle (5,1);  % set the bounding box (so we have less surrounding white space)
%
  \filldraw[fill=red!20,line width=2pt] (-5,-.5) -- (0,-.5) -- (0,.5) -- (-5,.5) -- (-5,-.5) ;
  \draw (-2,0) node {solid};
  \filldraw[fill=blue!20,line width=2pt] ( 5,-.5) -- (0,-.5) -- (0,.5) -- (5,.5) -- ( 5,-.5);
  \draw (2,0) node {fluid};
  \draw[color=green,line width=2pt] (0,-.5) -- (0,.5);
%
  \draw (0,-.5) node[anchor=north] {$x=\Gb(t)$};
  \draw (-5,-.5) node[anchor=north] {$x=-\Hs$};
  \draw ( 5,-.5) node[anchor=north] {$x=H$};
% 
  \draw ( 5,0) node[anchor=west] {$p=\pH(t)$};
  \draw (-5,0) node[anchor=east] {$\us=0$};
% grid:
%   \draw[step=1cm,gray] (-5,-1) grid (5,1.);
\end{tikzpicture}
\end{center}
\caption{Elastic piston...}
\label{fig:elasticPistonCartoon}
\end{figure}


The solution for the pressure in the fluid domain subject to a specified pressure boundary condition at $x=H$
and the compatibility condition at $x=\Gb(t)$ together with $[v]=0$, 
\begin{align}
    p(H,t)=\pH(t), \qquad p_x(\Gb(t),t) = -\rho v_t(\Gb(t),t) = -\rho \vs_t(0,t),
\end{align}
is
\begin{align}
    p(x)= \pH(t)  -\rho \vs_t(0,t)\, ( x-H)
\end{align}


The solution to the elasticity equations with
initial conditions $\us(\xs,0)=\us_0(\xs)$ and $\partial_t \us(\xs,0) = \vs_0(\xs)$ and boundary
condition $\us(0,t)=\Gb(t)$ follows from the d'Alembert solution, ({\bf *fix me*} for BC at $\xs=-\Hs$)
\begin{align}
  \us(\xs,t) &= f(\xs-\cp t) + g( \xs+ \cp t ),  \label{eq:dAlembert}  \\
  f(\xi) &= \half\big[ \us_0(\xi)- \cp^{-1}\int_0^\xi \vs_0(s) d s\big]  ~~\text{for $\xi<0$}, \label{eq:f-solution} \\
  g(\xi) &= \begin{cases}
           \half\big[ \us_0(\xi)+ \cp^{-1}\int_0^\xi \vs_0(s) d s\big]  & \text{for $\xi<0$},  \\
           \Gb(\xi/\cp) - f(-\xi)  & \text{for $\xi>0$} .
          \end{cases} \label{eq:g-solution} 
\end{align}
% where $c_p^2 = (\lambda+2\mu)/\rhos$.
The interface traction condition, 
\begin{align*}
  \rhos\cp^2\partial_{\xs}\us(0,t) &= -p(\Gb(t),t) , \\
                                  &= -\pH(t)  + \rho \vs_t(0,t)\, ( \Gb(t) -H)
\end{align*}
determines $\pH$ as a function of the interface position $\Gb$, 
\begin{align}
  \pH(t) =  \rho \vs_t(0,t)\, ( \Gb(t) -H) - \rhos\cp^2\partial_{\xs}\us(0,t) . \label{eq:pH}
\end{align}
Thus, by choosing $\pH$ according to~\eqref{eq:pH} the interface wll undergo the motion $x=\Gb(t)$.


==> texFiles/elasticPistonCompositeGrid-orig.tex <==
\newcommand{\Gcep}{\Gv_{\rm ep}}
\subsection{Composite grid elastic piston}

Here are some initial results for the elastic piston.


It may be easier to work with a solution that ramps up from zero to avoid initialization issues
with the moving grids etc.
Following the discussion in Section~\ref{sec:elasticPistonSolution} we could let the
solution in the solid be of the form
\begin{align}
  &  \us_2(\ys,t) =  F(t + (\ys+\Hs)/\cp ) -  F(t - (\ys+\Hs)/\cp) ,
\end{align}
for any smooth function $F$.
This form for $\us_2$ satisfies the wave equation and boundary condition $\us_2(-\Hs,t)=0$.
To have the solution turn on smoothly from zero we take 
\begin{align}
  & F(\xi) = \alpha \, R(\xi) \,\sin(2\pi k (\xi - \phi_0)),
\end{align}
where $R(\xi)$ is a {\em ramp function} that smoothly transitions from zero to one.
The {\tt rampOrder} defines the number of zero derivatives at the ramp interval ends -- we likely
need at least 2 zero derivatives so the acceleration is continuous.
We need to have the ramp function satisfy
\[
   F(\xi)=0 ~~\text{for}~~ \xi \le (\ys+\Hs)/\cp \le \Hs/\cp. 
\] 
With no ramp function, $R(\xi)=1$, the interface will be at $\ys=0$ at $t=0$ provided
\begin{align}
   \us_2(\ys,t) &=  F(\Hs/\cp ) -  F(-\Hs/\cp) = \alpha \,
              \Big( \sin(2\pi k (\Hs/\cp - \phi_0)) - \sin(2\pi k (-\Hs/\cp - \phi_0))\Big) , \\ 
      &= 2 \alpha \, \sin(2 \pi k \Hs/\cp) \, \cos(2\pi k  \phi_0)
\end{align}
and we can choose $\phi_0=1/(4 k)$. 

Given this solution, the interface quantities are computed **CHECK ME**
\begin{align}
y_I(t) &= \us_2(0,t) =  F(t + \Hs/\cp ) -  F(t - \Hs/\cp),  \\
v_{2,I}(t) &= \partial_t\us_2(0,t) =  F'(t + \Hs/\cp ) -  F'(t - \Hs/\cp), \\
p_I(t) = -\sigmas_{22,I}(t) &= - (\lambdas+2\mus) \partial_y \us_2(0,t)
       = \f{1}{\cp} \, \Big( F'(t + \Hs/\cp ) +  F'(t - \Hs/\cp \Big)
\end{align}
%
Using \eqref{eq:NonlinearInterfaceCondition}, the pressure at $y=H$ is given by
\begin{align}
&  p_0(t) = p_I(t) - \rho H \dot{v}_{2,I}(t) \left(1 - \frac{y_I(t)}{H}\right) ,\\
&   \dot{v}_{2,I}(t) =  F''(t + \Hs/\cp ) -  F''(t - \Hs/\cp),
\end{align}
%
and the exact pressure is given by
\begin{align}
p(y,t) = p_0(t) - \frac{p_0(t) - p_I(t)}{H - y_I(t)} (H - y).
\end{align}
We also have
\begin{align}
&  v_2(y,t) = v_{2,I}(t), \\
  &    \sigmas_{22}(\ys,t) = 
               \f{(\lambdas+2\mus)}{\cp} \, \Big( F'(t + (\ys+\Hs)/\cp ) +  F'(t - (\ys+\Hs)/\cp \Big).
\end{align}
For a second-order accurate solution we may need the ramp to have
at least two, and maybe three?, or four ?, continuous derivatives, $R(0)=R'(0)=R''(0)=R'''(0)=R''''(0)=0$. 


{% ------ GRIDS ------  
%
\newcommand{\figWidth}{6cm}% height 
\newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.225}{.225}{.09}{.09}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (16,6);  % set the bounding box (so we have less surrounding white space)

   \draw( 0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/elasticPistonGrid}{\figWidth}};
% 
   \draw( 5.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p7}{\figWidth}};
   \draw(10.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p8}{\figWidth}};
   % grid:
% \draw[step=1cm,gray] (0,0) grid (16,6);
\end{tikzpicture}
\end{center}
  \caption{Composite grid $\Gcep^{(2)}$ for an elastic piston adjacent to a fluid channel. 
    The green fluid grid adjacent to the piston moves over time. The blue fluid background grid remains fixed.
    The red grid for the solid reference domain also remains fixed over time.
   Middle and right: pressure and $\sigma_{22}$. 
}
  \label{fig:elasticPistonGrid}
\end{figure}
}


==> texFiles/elasticPistonCompositeGrid.tex <==
\newcommand{\Gcep}{\Gv_{\rm ep}}
\subsection{Composite grid elastic piston}

Here are some initial results for the elastic piston.


It may be easier to work with a solution that ramps up from zero to avoid initialization issues
with the moving grids etc.
Following the discussion in Section~\ref{sec:elasticPistonSolution} we could let the
solution in the solid be of the form
\begin{align}
  &  \us_2(\ys,t) =  F(t + (\ys+\Hs)/\cp ) -  F(t - (\ys+\Hs)/\cp) ,
\end{align}
for any smooth function $F$.
This form for $\us_2$ satisfies the wave equation and boundary condition $\us_2(-\Hs,t)=0$.
To have the solution turn on smoothly from zero we take 
\begin{align}
  & F(\xi) = \alpha \, R(\xi) \,\sin(2\pi k (\xi - \phi_0)),
\end{align}
where $R(\xi)$ is a {\em ramp function} that smoothly transitions from zero to one.
The {\tt rampOrder} defines the number of zero derivatives at the ramp interval ends -- we likely
need at least 2 zero derivatives so the acceleration is continuous.
We need to have the ramp function satisfy
\[
   F(\xi)=0 ~~\text{for}~~ \xi \le (\ys+\Hs)/\cp \le \Hs/\cp. 
\] 
With no ramp function, $R(\xi)=1$, the interface will be at $\ys=0$ at $t=0$ provided
\begin{align}
   \us_2(\ys,t) &=  F(\Hs/\cp ) -  F(-\Hs/\cp) = \alpha \,
              \Big( \sin(2\pi k (\Hs/\cp - \phi_0)) - \sin(2\pi k (-\Hs/\cp - \phi_0))\Big) , \\ 
      &= 2 \alpha \, \sin(2 \pi k \Hs/\cp) \, \cos(2\pi k  \phi_0)
\end{align}
and we can choose $\phi_0=1/(4 k)$. 

Given this solution, the interface quantities are computed **CHECK ME**
\begin{align}
y_I(t) &= \us_2(0,t) =  F(t + \Hs/\cp ) -  F(t - \Hs/\cp),  \\
v_{2,I}(t) &= \partial_t\us_2(0,t) =  F'(t + \Hs/\cp ) -  F'(t - \Hs/\cp), \\
p_I(t) = -\sigmas_{22,I}(t) &= - (\lambdas+2\mus) \partial_y \us_2(0,t)
       = \f{1}{\cp} \, \Big( F'(t + \Hs/\cp ) +  F'(t - \Hs/\cp \Big)
\end{align}
%
Using \eqref{eq:NonlinearInterfaceCondition}, the pressure at $y=H$ is given by
\begin{align}
&  p_0(t) = p_I(t) - \rho H \dot{v}_{2,I}(t) \left(1 - \frac{y_I(t)}{H}\right) ,\\
&   \dot{v}_{2,I}(t) =  F''(t + \Hs/\cp ) -  F''(t - \Hs/\cp),
\end{align}
%
and the exact pressure is given by
\begin{align}
p(y,t) = p_0(t) - \frac{p_0(t) - p_I(t)}{H - y_I(t)} (H - y).
\end{align}
We also have
\begin{align}
&  v_2(y,t) = v_{2,I}(t), \\
  &    \sigmas_{22}(\ys,t) = 
               \f{(\lambdas+2\mus)}{\cp} \, \Big( F'(t + (\ys+\Hs)/\cp ) +  F'(t - (\ys+\Hs)/\cp \Big).
\end{align}
For a second-order accurate solution we may need the ramp to have
at least two, and maybe three?, or four ?, continuous derivatives, $R(0)=R'(0)=R''(0)=R'''(0)=R''''(0)=0$. 


{% ------ GRIDS ------  
%
\newcommand{\figWidth}{6cm}% height 
\newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.225}{.225}{.09}{.09}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (16,6);  % set the bounding box (so we have less surrounding white space)

   \draw( 0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/elasticPistonGrid}{\figWidth}};
% 
   \draw( 5.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p7}{\figWidth}};
   \draw(10.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/pistonG4stress0p8}{\figWidth}};
   % grid:
% \draw[step=1cm,gray] (0,0) grid (16,6);
\end{tikzpicture}
\end{center}
  \caption{Composite grid $\Gcep^{(2)}$ for an elastic piston adjacent to a fluid channel. 
    The green fluid grid adjacent to the piston moves over time. The blue fluid background grid remains fixed.
    The red grid for the solid reference domain also remains fixed over time.
   Middle and right: pressure and $\sigma_{22}$. 
}
  \label{fig:elasticPistonGrid}
\end{figure}
}


==> texFiles/elasticPistonMatlab.tex <==
\section{Matlab Results}

The elastic piston solution is given by
\begin{align}
\bar{u}_2(\ys,t) &= \hat{\alpha} \sin( \hat{k} (\ys+\bar{H}) ) 
\cos(\bar{c}_p \hat{k} t + \hat{\phi}_0) \\
&= \hat{\alpha} \sin( \hat{k} (\ys+\bar{H})) \sin(\bar{c}_p \hat{k} t + \pi/2 + \hat{\phi}_0)
\end{align}
%
Here are the parameters used for the runs in the following sections:
\begin{table}[H]
\begin{center}%\footnotesize
\caption{Parameter set (A). }
  \begin{tabular}{|cccccc|}
  \hline
  $\Hs$ & $H$ & $\hat{\alpha}$ & $\hat{k}$  & $\hat{\phi}_0$   & $\rho$ \strutt \\ \hline
  $.5$  & $1$ &   $0.1$  & $\pi$  & $-\pi/2$ & $1$    \\
  \hline
\end{tabular}
\end{center} 
\end{table}
\begin{table}[H]
\begin{center}%\footnotesize
\caption{Parameter set (B). These parameters agree with the overture runs}
  \begin{tabular}{|cccccc|}
  \hline
  $\Hs$ & $H$ & $\hat{\alpha}$ & $\hat{k}$  & $\hat{\phi}_0$   & $\rho$ \strutt \\ \hline
  $.5$  & $1$ &   $0.2$  & $\pi/\sqrt{3}$  & $-\pi/2$ & $1$    \\
  \hline
\end{tabular}
\end{center} 
\end{table}
%
The hat parameters (Matlab) compare with parameters below (Overture) by
\begin{align}
2 \alpha &= \hat{\alpha} \\
\frac{2 \pi k}{\cp} &= \hat{k}
\end{align}
%
given that $\hat{\phi}_0 = -\pi/2.$
Using $\rhos=\delta \rho$, $\lambdas=\delta$, $\mus=\delta$, with $\delta=\text{scf}=\text{solid-scale-factor}$.
This gives $\cp = \sqrt{3}$ and $\cs = 1.$
% {\color{red}{Note: the parameters that agree with the Overture runs are
% \begin{align}
% \hat{k} = \frac{\pi}{\sqrt{3}}, \quad \hat{\alpha} = 0.2. 
% \end{align}
% I will run cases with these parameters in the future.
% }}
%
%
The initial fluid domain is $[0,1]\times[0,H]$ while the solid domain is $[0,1]\times[-\Hs,0]$.

% \subsection{TP, cfl = .25, t = .3, parameter set (A)}

% Found bug, re-ran code for parameter set (B).
% Observation: scf affects magnitude of errors in solid stress. All
% the other errors and ratios are roughly the same.

% \input tables/ep_mat_tp_rs_8000_cfl_25_tf_3
% \input tables/ep_mat_tp_rs_4000_cfl_25_tf_3
% \input tables/ep_mat_tp_rs_1600_cfl_25_tf_3
% \input tables/ep_mat_tp_rs_1000_cfl_25_tf_3
% \input tables/ep_mat_tp_rs_800_cfl_25_tf_3

% \subsection{TP, cfl = .5, t = .7, parameter set (A)}

% Found bug, re-ran code for parameter set (B).
% All variables seem OK. Solid stress is questionable.
% For large scale factors, the ratio recovers on the finest grid. This
% cannot be observed for the smaller scale factors due to the instability.
% \input tables/ep_mat_tp_rs_8000_cfl_5_tf_7
% \input tables/ep_mat_tp_rs_4000_cfl_5_tf_7
% \input tables/ep_mat_tp_rs_1600_cfl_5_tf_7
% \input tables/ep_mat_tp_rs_1000_cfl_5_tf_7
% \input tables/ep_mat_tp_rs_800_cfl_5_tf_7

\subsection{TP, cfl = .5, t = .7, parameter set (B)}


\input tables/ep_mat_tp_b_rs_8000_cfl_5_tf_7
\input tables/ep_mat_tp_b_rs_4000_cfl_5_tf_7
\input tables/ep_mat_tp_b_rs_1600_cfl_5_tf_7
\input tables/ep_mat_tp_b_rs_1000_cfl_5_tf_7
\input tables/ep_mat_tp_b_rs_800_cfl_5_tf_7

\subsection{TP, cfl = .9, t = .7, parameter set (B)}


\input tables/ep_mat_tp_b_rs_8000_cfl_9_tf_7
\input tables/ep_mat_tp_b_rs_4000_cfl_9_tf_7
\input tables/ep_mat_tp_b_rs_1600_cfl_9_tf_7
\input tables/ep_mat_tp_b_rs_1000_cfl_9_tf_7
\input tables/ep_mat_tp_b_rs_800_cfl_9_tf_7

% \subsection{TP, cfl = .9, t = .7, parameter set (A)}

% Found bug, re-ran code for parameter set (B).
% Fluid and displacement are OK. Solid velocity and stress are
% questionable. The finest grid is unstable.
% \input tables/ep_mat_tp_rs_8000_cfl_9_tf_7
% \input tables/ep_mat_tp_rs_4000_cfl_9_tf_7
% \input tables/ep_mat_tp_rs_1600_cfl_9_tf_7
% \input tables/ep_mat_tp_rs_1000_cfl_9_tf_7
% \input tables/ep_mat_tp_rs_800_cfl_9_tf_7



\subsection{AMP, cfl = .5, t = .7, parameter set (B)}

\input tables/ep_mat_amp_b_rs_1000_cfl_5_tf_7
\input tables/ep_mat_amp_b_rs_100_cfl_5_tf_7
\input tables/ep_mat_amp_b_rs_10_cfl_5_tf_7
\input tables/ep_mat_amp_b_rs_1_cfl_5_tf_7
\input tables/ep_mat_amp_b_rs_p1_cfl_5_tf_7
\input tables/ep_mat_amp_b_rs_p01_cfl_5_tf_7
\input tables/ep_mat_amp_b_rs_p001_cfl_5_tf_7

\subsection{AMP, cfl = .9, t = .7, parameter set (B)}
Problems on finest grid

\input tables/ep_mat_amp_b_rs_1_cfl_9_tf_7

\subsection{AMP results, parameter set (A)}

Convergence is lost on finest grid 
\input tables/ep_mat_amp_rs_1000_cfl_9_tf_7

Result is OK
\input tables/ep_mat_amp_rs_1000_cfl_5_tf_7


==> texFiles/elasticPistonMatlab_7-23.tex <==
\begin{table}[H]
\caption{\label{fig:ElasticPistonConvergence}Elastic piston convergence tables for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be 
$\bar{H} = \frac{1}{2},\, H = 1,\, \mus=\lambdas=\rhos,\, \mu =0.01.$
The final time is $t_{\rm final} = 0.3.$
Matlab, \texttt{cdv=0, jv1=1, jv2=1, jvf2=1}.}
\begin{center}
\begin{tabular}{c}
Heavy solid: $\rhos/\rho = 10^3$
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  4.4e-04 &      &  4.6e-05 &      &  3.9e-06 &      &  2.5e-05 &      &  2.0e-02 &     \\
1/ 40 &   105 &  8.8e-05 &  5.0 &  1.3e-05 &  3.4 &  1.1e-06 &  3.4 &  5.0e-06 &  4.9 &  2.8e-03 &  7.1 \\
1/ 80 &   208 &  1.6e-05 &  5.7 &  3.8e-06 &  3.5 &  3.1e-07 &  3.6 &  1.0e-06 &  4.8 &  6.2e-04 &  4.5 \\
1/160 &   416 &  2.3e-06 &  6.9 &  1.1e-06 &  3.6 &  8.0e-08 &  3.9 &  2.3e-07 &  4.5 &  1.8e-04 &  3.4 \\
\hline
\\
\end{tabular}

\begin{tabular}{c}
Medium solid: $\rhos/\rho = 1$
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  6.2e-05 &      &  4.7e-05 &      &  1.8e-05 &      &  1.3e-04 &      &  2.6e-04 &     \\
1/ 40 &   105 &  1.6e-06 & 39.2 &  6.6e-06 &  7.2 &  1.8e-06 &  9.8 &  2.1e-05 &  6.0 &  6.8e-05 &  3.8 \\
1/ 80 &   208 &  2.4e-06 &  0.7 &  3.1e-07 & 21.0 &  3.0e-07 &  6.0 &  1.4e-06 & 14.9 &  9.3e-06 &  7.3 \\
1/160 &   416 &  5.6e-07 &  4.2 &  1.5e-08 & 21.2 &  1.1e-07 &  2.8 &  2.7e-07 &  5.3 &  4.2e-07 & 22.1 \\
\hline
\\
\end{tabular}

% \caption{\label{fig:ElasticPistonConvergence}Convergence for elastic piston.\das{Placeholder for light solid $\rhos/\rho = 10^{-3}.$}}
\begin{tabular}{c}
Light solid: $\rhos/\rho = 10^{-3}$
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  9.2e-06 &      &  4.2e-06 &      &  7.8e-06 &      &  5.1e-06 &      &  4.4e-08 &     \\
1/ 40 &   105 &  2.3e-06 &  3.9 &  1.1e-06 &  3.9 &  1.9e-06 &  4.0 &  1.1e-06 &  4.7 &  9.9e-09 &  4.4 \\
1/ 80 &   208 &  5.9e-07 &  3.9 &  2.8e-07 &  3.9 &  4.8e-07 &  4.0 &  2.8e-07 &  3.8 &  2.2e-09 &  4.5 \\
1/160 &   416 &  1.5e-07 &  4.0 &  6.9e-08 &  4.0 &  1.2e-07 &  4.1 &  7.3e-08 &  3.9 &  5.0e-10 &  4.3 \\
\hline
\end{tabular}
\end{center}
\end{table}


==> texFiles/elasticPistonOverture.tex <==
\clearpage
\das{Old figures are in tables/old/ directory...}
\subsubsection{Block elastic piston: Overture results}

\noindent \textbf{\blue New: use monolithic $z_f$}
\input tables/insElasticPiston.epgp.AmpSCF1e-3NUp05zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.epgp.AmpSCF1e3NUp05zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.epgp.AmpSCF1NUp05zfmImtp6.ConvTable.tex

% \noindent \textbf{\blue New: match fluid and solid at final solid correction: $\zfHat=(\mu\rho)/(\zp\dt)$,  $z_f=1 \mu/h$}
% \input tables/insElasticPiston.epgpN.AmpSCF1e3zf1+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.epgpN.AmpSCF1zf1+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.epgpN.AmpSCF1e-3zf1+0Imtp6.ConvTable.tex

%- \noindent \textbf{Results for $z_f=100 \mu/h$}
%- \input tables/insElasticPiston.epgpN.AmpSCF1e3zf100+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1zf100+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1e-3zf100+0Imtp6.ConvTable.tex
%- 
%- \noindent \textbf{\red Results for zf MONOLITHIC --OK }
%- \input tables/insElasticPiston.epgpN.AmpSCF1e3zfmImtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1zfmImtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1e-3zfmImtp6.ConvTable.tex


%- \noindent \textbf{OLD: Results for $z_f=5 \mu/h$}
%- \input tables/insElasticPiston.epgpN.AmpSCF1e3zf5+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1zf5+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1e-3zf5+0Imtp6.ConvTable.tex

%- \noindent \textbf{Results for $z_f=2 \mu/h$}
%- \input tables/insElasticPiston.epgpN.AmpSCF1e3zf2+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1zf2+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1e-3zf2+0Imtp6.ConvTable.tex
%- 
%- \noindent \textbf{Results for $z_f=1 \mu/h$- check scf=1, coarse grid}
%- \input tables/insElasticPiston.epgpN.AmpSCF1e3zf1+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1zf1+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgpN.AmpSCF1e-3zf1+0Imtp6.ConvTable.tex

% ----------------------------
% \clearpage
\subsubsection{Shear-block elastic piston: Overture results}


\noindent \textbf{\blue New: use monolithic $z_f$}
\input tables/insElasticPiston.epgp.shearAmpSCF1e-3NUp1zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.epgp.shearAmpSCF1e3NUp1zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.epgp.shearAmpSCF1NUp1zfmImtp6.ConvTable.tex

% \noindent \textbf{\blue New: match fluid and solid: $\zfHat=(\mu\rho)/(\zp\dt)$,  $z_f=1 \mu/h$}
% \input tables/insElasticPiston.epgp.shearAmpSCF1e3zf1+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.epgp.shearAmpSCF1e-3zf1+0Imtp6.ConvTable.tex


%- \noindent \textbf{Results for $z_f=100 \mu/h$}
%- \input tables/insElasticPiston.epgp.shearAmpSCF1e3zf100+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgp.shearAmpSCF1e-3zf100+0Imtp6.ConvTable.tex
%- 
%- 
%- \noindent \textbf{\red Results for zf MONOLITHIC -- Trouble with using $z_{fm}$ to replace $\hat{z}_f$ and $z_f$ fine grid heavy, OK only replacing $z_f=\mu/h$ with $z_{fm}$
%- and keeping $\hat{z}_f$}
%- \input tables/insElasticPiston.epgp.shearAmpSCF1e3zfmImtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgp.shearAmpSCF1e-3zfmImtp6.ConvTable.tex
%- 
%- 
%- \noindent \textbf{Results for $z_f=5 \mu/h$}
%- \input tables/insElasticPiston.epgp.shearAmpSCF1e3zf5+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.epgp.shearAmpSCF1e-3zf5+0Imtp6.ConvTable.tex
%- 
% \noindent \textbf{OLD: Results for $z_f=2 \mu/h$}
% \input tables/insElasticPiston.epgp.shearAmpSCF1e3zf2+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.epgp.shearAmpSCF1e-3zf2+0Imtp6.ConvTable.tex



% ----------------------------
\clearpage
\subsubsection{Radial elastic piston: Overture results}

\noindent \textbf{\blue New: use monolithic $z_f$}
\input tables/insElasticPiston.rep.AmpSCF1e-3NUp05zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.rep.AmpSCF1e3NUp05zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.rep.AmpSCF1NUp05zfmImtp6.ConvTable.tex

% \noindent \textbf{\blue New: match fluid and solid: $\zfHat=(\mu\rho)/(\zp\dt)$,  $z_f=1 \mu/h$}
% \input tables/insElasticPiston.rep.AmpSCF1e3zf1+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.rep.AmpSCF1zf1+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.rep.AmpSCF1e-3zf1+0Imtp6.ConvTable.tex

%- \noindent \textbf{\red Results for MONOLITHIC $z_{fm}$ replacing $z_f$ in solid}
%- \input tables/insElasticPiston.rep.AmpSCF1e3zfmImtp6.ConvTable.tex
%- \input tables/insElasticPiston.rep.AmpSCF1zfmImtp6.ConvTable.tex
%- \input tables/insElasticPiston.rep.AmpSCF1e-3zfmImtp6.ConvTable.tex
%- 
%- 
%- \noindent \textbf{Results for $z_f=5 \mu/h$}
%- \input tables/insElasticPiston.rep.AmpSCF1e3zf5+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.rep.AmpSCF1zf5+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.rep.AmpSCF1e-3zf5+0Imtp6.ConvTable.tex

% \noindent \textbf{OLD: Results for $z_f=2 \mu/h$}
% \input tables/insElasticPiston.rep.AmpSCF1e3zf2+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.rep.AmpSCF1zf2+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.rep.AmpSCF1e-3zf2+0Imtp6.ConvTable.tex




% ----------------------------
\clearpage
\subsubsection{Radial SHEAR elastic piston: Overture results}

\noindent \textbf{\blue New: use monolithic $z_f$}
\input tables/insElasticPiston.rep.shearAmpSCF1e-3NUp1zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.rep.shearAmpSCF1e3NUp1zfmImtp6.ConvTable.tex
\input tables/insElasticPiston.rep.shearAmpSCF1NUp1zfmImtp6.ConvTable.tex

% \noindent \textbf{\blue DAS 8/17: new case id's with $\nu=.1$. Note, we use amp$=1$ for these cases.}
% \input tables/insElasticPiston.rep.shearAmpSCF1000pNUp1zf1+0Imt1p.ConvTable.tex
% \input tables/insElasticPiston.rep.shearAmpSCF10pNUp1zf1+0Imt1p.ConvTable.tex
% \input tables/insElasticPiston.rep.shearAmpSCF1pNUp1zf1+0Imt1p.ConvTable.tex
% \input tables/insElasticPiston.rep.shearAmpSCFp1NUp1zf1+0Imt1p.ConvTable.tex
% \input tables/insElasticPiston.rep.shearAmpSCFp001NUp1zf1+0Imt1p.ConvTable.tex

% \noindent \textbf{\blue New: match fluid and solid: $\zfHat=(\mu\rho)/(\zp\dt)$,  $z_f=1 \mu/h$}
% \input tables/insElasticPiston.rep.shearAmpSCF10zf1+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.rep.shearAmpSCF1e3zf1+0Imtp6.ConvTable.tex




%- \noindent \textbf{\red Results for MONOLITHIC $z_{fm}$ replacing $z_f$ in solid}
%- \input tables/insElasticPiston.rep.shearAmpSCF10zfmImtp6.ConvTable.tex
%- \input tables/insElasticPiston.rep.shearAmpSCF1e3zfmImtp6.ConvTable.tex
%- 
%- \noindent \textbf{Results for $z_f=5 \mu/h$}
%- \input tables/insElasticPiston.rep.shearAmpSCF10zf5+0Imtp6.ConvTable.tex
%- \input tables/insElasticPiston.rep.shearAmpSCF1e3zf5+0Imtp6.ConvTable.tex

% \noindent \textbf{*OLD* Results for $z_f=2 \mu/h$}
% \input tables/insElasticPiston.rep.shearAmpSCF10zf2+0Imtp6.ConvTable.tex
% \input tables/insElasticPiston.rep.shearAmpSCF1e3zf2+0Imtp6.ConvTable.tex

% 
% Here is the elastic piston solution (no Ramp function here).
% \begin{align}
%   &  \us_2(\ys,t) =  F(t + (\ys+\Hs)/\cp ) -  F(t - (\ys+\Hs)/\cp) = F(\xi_+)-F(\xi_-) ,\\
%   & F(\xi) = \alpha \,\sin(2\pi k (\xi - \phi_0)),
% \end{align}
% which gives (with $\phi_0=1/(4 k)$) *check me*
% \begin{align}
%   \us_2(\ys,t) &=  \alpha \Big( \sin(2\pi k (\xi_+ - \phi_0)) - \sin(2\pi k (\xi_-  - \phi_0)) \Big) , \\ 
%                &= 2\alpha \, \sin(\pi k (\xi_+ - \xi_-))\, \cos(\pi k (\xi_++\xi-  2\phi_0))  , \\
%                &= 2 \alpha \, \sin(2 \pi k ((\ys+\Hs)/\cp)))\, \cos(2 \pi k (t - \phi_0))  , \\
%                &= 2 \alpha \, \sin(2 \pi k (\ys+\Hs)/\cp) )\, \sin(2 \pi k t )  .
% \end{align}
% 
% Here are the parameters used for the runs in the following sections.
% \begin{center}%\footnotesize
%   \begin{tabular}{|cccccc|}
%   \hline
%   $\Hs$ & $H$ & $\alpha$ & $k$  & $\phi_0$   & $\rho$ \strutt \\ \hline
%   $.5$  & $1$ &   $0.1$  & $.5$  & $1/(4 k)$ & $1$    \\
%   \hline
% \end{tabular}
% \end{center} 
% Using $\rhos=\delta \rho$, $\lambdas=\delta$, $\mus=\delta$, with $\delta=\text{scf}=\text{solid-scale-factor}$
% 
% The initial fluid domain is $[0,1]\times[0,H]$ while the solid domain is $[0,1]\times[-\Hs,0]$.
% The elastic piston grid $\Gc^{(j)}$, $j=1,2,3,\ldots$, has grid spacing $h_j=1/(10 j)$. 
% 
% NOTE: The piston solution in the fluid has a rather simple spatial form (p linear in y, v constant in space)
% and so errors in time should normally dominate.
% 
% 
% % --------------------------------------------------------------------
% \clearpage
% \subsection{*NEW* TP Scheme - INS PC22 explicit PC}
% 
% {\scriptsize\blue
% \begin{verbatim}
% TP: -scf=1000
% conv.p insElasticPiston.conv -tp=.1 -tf=0.1 -cg=epgp -showAllComponents=0 -tsINS=pc -smVariation=g -scf=1000 
% -addedMass=0 -useExactPressureBC=0 -useImplicitAmpBCs=0 -cfl=.9 -diss=0.5 -stressRelaxation=4 -ng=4
% 
% -----------  TP
%  grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%  epg1 &     1 & 5.35e-03 &      & 9.55e-04 &      & 4.26e-05 &      & 7.70e-04 &      & 8.83e-01 &      
%  epg2 &     2 & 1.27e-03 &  4.2 & 1.92e-04 &  5.0 & 1.78e-05 &  2.4 & 2.01e-04 &  3.8 & 1.64e-01 &  5.4 
%  epg4 &     4 & 2.67e-04 &  4.8 & 4.34e-05 &  4.4 & 4.82e-06 &  3.7 & 4.64e-05 &  4.3 & 4.14e-02 &  4.0 
%  epg8 &     8 & 6.42e-05 &  4.2 & 1.03e-05 &  4.2 & 1.20e-06 &  4.0 & 1.10e-05 &  4.2 & 1.03e-02 &  4.0 
% Convergence rates: c0=2.14 c1=2.17 c2=1.73 c3=2.05 c4=2.13 
% \end{verbatim}
% }
% 
% % --------------------------------------------------------------------
% \subsection{*NEW* AMP Scheme - INS PC22 explicit PC}
% 
% Troubles here with wiggles on the interface for medium and light. The AMP velocity BC couples points in the tangential
% direction (from $\nu\Delta \vv$) to the interface but we do not solve the coupled system -- instead we lag some terms.
% This could be the source of the trouble (?)
% 
% {\scriptsize\blue
% \begin{verbatim}
% conv.p insElasticPiston.conv -nu=.01 -tp=.1 -tf=.1 -cg=epgp -showAllComponents=0 -tsINS=pc -smVariation=g -scf=1e3 -addedMass=1 
% -useExactPressureBC=0 -useImplicitAmpBCs=0 -cfl=.9 -diss=0.5 -stressRelaxation=4 -ng=4
% 
% ----HEAVY
% -scf=1e3 -tf=.3
%                 grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.06e-02 &      & 1.11e-03 &      & 3.12e-04 &      & 4.61e-04 &      & 4.30e+00 &      
%                 epg2 &     2 & 2.72e-03 &  3.9 & 2.28e-04 &  4.9 & 8.94e-05 &  3.5 & 1.38e-04 &  3.3 & 9.89e-01 &  4.3 
%                 epg4 &     4 & 7.75e-04 &  3.5 & 4.25e-05 &  5.4 & 2.39e-05 &  3.7 & 3.83e-05 &  3.6 & 2.36e-01 &  4.2 
%                 epg8 &     8 & 2.32e-04 &  3.3 & 9.70e-06 &  4.4 & 6.68e-06 &  3.6 & 9.90e-06 &  3.9 & 6.15e-02 &  3.8 
% Convergence rates: c0=1.84 c1=2.29 c2=1.85 c3=1.85 c4=2.05 
% 
% 
% -----MEDIUM
% -scf=1 -tf=.1
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 6.99e-04 &      & 6.90e-05 &      & 3.12e-05 &      & 5.14e-04 &      & 8.64e-04 &      
%                 epg2 &     2 & 2.55e-04 &  2.7 & 1.48e-05 &  4.7 & 4.93e-06 &  6.3 & 1.34e-04 &  3.8 & 2.41e-04 &  3.6 
%                 epg4 &     4 & 7.33e-05 &  3.5 & 3.43e-06 &  4.3 & 1.17e-06 &  4.2 & 3.41e-05 &  3.9 & 7.10e-05 &  3.4 
%                 epg8 &     8 & 1.85e-05 &  4.0 & 9.00e-07 &  3.8 & 4.80e-07 &  2.4 & 8.72e-06 &  3.9 & 1.83e-05 &  3.9 
% Convergence rates: c0=1.75 c1=2.09 c2=2.01 c3=1.96 c4=1.84 
% 
% -scf=1 -tf=.2  **TROUBLE** MEDIUM HIGH FREQ WIGGLES on the interface
%                 grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 4.98e-04 &      & 1.84e-04 &      & 8.84e-05 &      & 3.55e-04 &      & 2.34e-03 &      
%                 epg2 &     2 & 3.01e-04 &  1.7 & 4.49e-05 &  4.1 & 2.56e-05 &  3.5 & 9.57e-05 &  3.7 & 4.87e-04 &  4.8 
%                 epg4 &     4 & 8.15e-05 &  3.7 & 9.88e-06 &  4.5 & 6.79e-06 &  3.8 & 2.74e-05 &  3.5 & 1.09e-04 &  4.5 
%                 epg8 &     8 & 1.78e-04 &  0.5 & 5.39e-05 &  0.2 & 2.02e-06 &  3.4 & 7.41e-06 &  3.7 & 4.88e-05 &  2.2 
% Convergence rates: c0=0.63 c1=0.75 c2=1.83 c3=1.86 c4=1.89 
% 
% 
% 
% -----LIGHT
% -scf=1e-3 -tf=.1**TROUBLE** MEDIUM HIGH FREQ WIGGLES on the interface
% 
%                 grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.94e-05 &      & 1.18e-05 &      & 3.35e-05 &      & 5.08e-04 &      & 8.62e-07 &      
%                 epg2 &     2 & 3.12e-06 &  6.2 & 2.97e-06 &  4.0 & 5.43e-06 &  6.2 & 1.34e-04 &  3.8 & 2.82e-07 &  3.1 
%                 epg4 &     4 & 7.09e-07 &  4.4 & 7.58e-07 &  3.9 & 1.17e-06 &  4.6 & 3.41e-05 &  3.9 & 7.84e-08 &  3.6 
%                 epg8 &     8 & 2.17e-04 &  0.0 & 8.97e-04 &  0.0 & 8.69e-05 &  0.0 & 1.14e-02 &  0.0 & 3.54e-04 &  0.0 
% Convergence rates: c0=-0.83 c1=-1.68 c2=-0.19 c3=-1.15 c4=-2.42 
% 
% 
% 
% \end{verbatim}
% }
% %-                 
% REFERENCE -- SET ALL INTERFACE VALUES TO EXACT 
% {\scriptsize\orange
% \begin{verbatim}
% AMP -scf=1000
% -tf=.1
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.04e-05 &      & 5.86e-06 &      & 3.71e-05 &      & 5.58e-04 &      & 8.85e-04 &      
%                 epg2 &     2 & 1.28e-06 &  8.1 & 3.74e-07 & 15.7 & 1.42e-05 &  2.6 & 1.42e-04 &  3.9 & 1.70e-04 &  5.2 
%                 epg4 &     4 & 1.59e-07 &  8.1 & 2.42e-08 & 15.5 & 3.87e-06 &  3.7 & 3.61e-05 &  3.9 & 5.56e-05 &  3.1 
%                 epg8 &     8 & 1.88e-08 &  8.5 & 1.43e-09 & 16.9 & 9.85e-07 &  3.9 & 9.11e-06 &  4.0 & 1.61e-05 &  3.5 
% Convergence rates: c0=3.03 c1=4.00 c2=1.76 c3=1.98 c4=1.90 
% 
% -tf=.2
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 3.71e-05 &      & 2.15e-05 &      & 1.65e-04 &      & 5.15e-04 &      & 2.41e-03 &      
%                 epg2 &     2 & 4.61e-06 &  8.0 & 1.42e-06 & 15.1 & 4.93e-05 &  3.3 & 1.12e-04 &  4.6 & 5.79e-04 &  4.2 
%                 epg4 &     4 & 5.78e-07 &  8.0 & 8.93e-08 & 15.9 & 1.23e-05 &  4.0 & 3.07e-05 &  3.6 & 1.47e-04 &  3.9 
%                 epg8 &     8 & 6.61e-08 &  8.7 & 5.05e-09 & 17.7 & 3.04e-06 &  4.0 & 8.04e-06 &  3.8 & 3.67e-05 &  4.0 
% Convergence rates: c0=3.04 c1=4.02 c2=1.93 c3=1.99 c4=2.01 
% \end{verbatim}
% }
% 
% 
% % --------------------------------------------------------------------
% \subsection{*NEW* AMP Scheme - INS IM22 implicit PC}
% 
% {\scriptsize\blue
% \begin{verbatim}
% conv.p insElasticPiston.conv -nu=.1 -tp=.1 -tf=.1 -cg=epgp -showAllComponents=0 -tsINS=im -smVariation=g -scf=1e3 
% -addedMass=1 -useExactPressureBC=0 -useImplicitAmpBCs=1 -cfl=.9 -diss=0.5 -stressRelaxation=4 -ng=4
% 
% -----HEAVY
% -scf=1e3  NU=.1 -tf=.2
%                 grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.05e-03 &      & 1.18e-03 &      & 1.36e-04 &      & 9.22e-04 &      & 2.31e+00 &      
%                 epg2 &     2 & 3.61e-04 &  2.9 & 2.75e-04 &  4.3 & 3.99e-05 &  3.4 & 2.36e-04 &  3.9 & 4.83e-01 &  4.8 
%                 epg4 &     4 & 1.38e-04 &  2.6 & 6.61e-05 &  4.2 & 1.09e-05 &  3.7 & 6.06e-05 &  3.9 & 1.09e-01 &  4.4 
%                 epg8 &     8 & 3.29e-05 &  4.2 & 1.62e-05 &  4.1 & 2.78e-06 &  3.9 & 1.57e-05 &  3.9 & 2.49e-02 &  4.4 
% Convergence rates: c0=1.64 c1=2.06 c2=1.87 c3=1.96 c4=2.18 
% 
% -scf=1e3  NU=.1 -tf=.2
%                 grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.02e-02 &      & 5.86e-04 &      & 3.13e-04 &      & 4.66e-04 &      & 4.31e+00 &      
%                 epg2 &     2 & 2.47e-03 &  4.1 & 1.39e-04 &  4.2 & 8.98e-05 &  3.5 & 1.40e-04 &  3.3 & 9.92e-01 &  4.3 
%                 epg4 &     4 & 6.52e-04 &  3.8 & 3.57e-05 &  3.9 & 2.41e-05 &  3.7 & 3.91e-05 &  3.6 & 2.37e-01 &  4.2 
%                 epg8 &     8 & 1.51e-04 &  4.3 & 8.99e-06 &  4.0 & 6.18e-06 &  3.9 & 1.07e-05 &  3.7 & 5.72e-02 &  4.1 
% Convergence rates: c0=2.02 c1=2.00 c2=1.89 c3=1.82 c4=2.08 
% 
% -scf=1e3  NU=.1 -tf=.6
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.92e-02 &      & 4.50e-03 &      & 3.84e-04 &      & 4.36e-03 &      & 5.06e+00 &      
%                 epg2 &     2 & 5.51e-03 &  3.5 & 1.09e-03 &  4.1 & 1.29e-04 &  3.0 & 1.09e-03 &  4.0 & 1.30e+00 &  3.9 
%                 epg4 &     4 & 1.72e-03 &  3.2 & 2.75e-04 &  4.0 & 3.57e-05 &  3.6 & 2.75e-04 &  4.0 & 3.37e-01 &  3.9 
%                 epg8 &     8 & 5.13e-04 &  3.4 & 6.87e-05 &  4.0 & 9.44e-06 &  3.8 & 6.87e-05 &  4.0 & 8.68e-02 &  3.9 
% Convergence rates: c0=1.74 c1=2.01 c2=1.79 c3=2.00 c4=1.95 
% 
% 
% ---MEDIUM 
% -scf=1 NU=.1 -tf=.1
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 8.08e-04 &      & 5.96e-05 &      & 3.10e-05 &      & 5.14e-04 &      & 8.64e-04 &      
%                 epg2 &     2 & 2.73e-04 &  3.0 & 1.26e-05 &  4.7 & 4.93e-06 &  6.3 & 1.34e-04 &  3.8 & 2.58e-04 &  3.3 
%                 epg4 &     4 & 7.38e-05 &  3.7 & 3.16e-06 &  4.0 & 1.17e-06 &  4.2 & 3.41e-05 &  3.9 & 7.16e-05 &  3.6 
%                 epg8 &     8 & 1.88e-05 &  3.9 & 7.86e-07 &  4.0 & 2.83e-07 &  4.1 & 8.65e-06 &  3.9 & 1.85e-05 &  3.9 
% Convergence rates: c0=1.82 c1=2.07 c2=2.24 c3=1.97 c4=1.85 
% 
% -tf=.2
%                 grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 8.60e-04 &      & 1.45e-04 &      & 8.83e-05 &      & 3.26e-04 &      & 2.34e-03 &      
%                 epg2 &     2 & 3.25e-04 &  2.6 & 3.52e-05 &  4.1 & 2.56e-05 &  3.4 & 9.57e-05 &  3.4 & 4.87e-04 &  4.8 
%                 epg4 &     4 & 8.26e-05 &  3.9 & 8.72e-06 &  4.0 & 6.79e-06 &  3.8 & 2.74e-05 &  3.5 & 1.09e-04 &  4.5 
%                 epg8 &     8 & 2.14e-05 &  3.9 & 2.10e-06 &  4.2 & 1.67e-06 &  4.1 & 7.26e-06 &  3.8 & 2.49e-05 &  4.4 
% Convergence rates: c0=1.80 c1=2.03 c2=1.91 c3=1.83 c4=2.18 
% 
% -tf=.4
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 3.09e-03 &      & 7.50e-05 &      & 3.41e-04 &      & 7.05e-04 &      & 4.12e-03 &      
%                 epg2 &     2 & 5.38e-04 &  5.7 & 1.25e-05 &  6.0 & 9.94e-05 &  3.4 & 1.90e-04 &  3.7 & 8.97e-04 &  4.6 
%                 epg4 &     4 & 1.21e-04 &  4.4 & 2.49e-06 &  5.0 & 2.63e-05 &  3.8 & 4.84e-05 &  3.9 & 2.11e-04 &  4.3 
%                 epg8 &     8 & 2.81e-05 &  4.3 & 6.57e-07 &  3.8 & 6.56e-06 &  4.0 & 1.23e-05 &  3.9 & 5.12e-05 &  4.1 
% Convergence rates: c0=2.25 c1=2.28 c2=1.90 c3=1.95 c4=2.11 
% 
% 
% ---LIGHT
% -scf=1e-3 -tf=.1
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.97e-05 &      & 1.18e-05 &      & 3.35e-05 &      & 5.08e-04 &      & 8.62e-07 &      
%                 epg2 &     2 & 3.22e-06 &  6.1 & 2.93e-06 &  4.0 & 5.43e-06 &  6.2 & 1.34e-04 &  3.8 & 2.82e-07 &  3.1 
%                 epg4 &     4 & 9.11e-07 &  3.5 & 7.20e-07 &  4.1 & 1.17e-06 &  4.6 & 3.41e-05 &  3.9 & 7.83e-08 &  3.6 
%                 epg8 &     8 & 3.69e-07 &  2.5 & 1.86e-07 &  3.9 & 2.83e-07 &  4.1 & 8.65e-06 &  3.9 & 2.02e-08 &  3.9 
% Convergence rates: c0=1.90 c1=2.00 c2=2.29 c3=1.96 c4=1.81 
% 
% -scf=1e-3 -tf=.2
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 4.72e-05 &      & 4.59e-05 &      & 8.54e-05 &      & 2.99e-04 &      & 2.35e-06 &      
%                 epg2 &     2 & 1.26e-05 &  3.7 & 1.14e-05 &  4.0 & 2.52e-05 &  3.4 & 9.28e-05 &  3.2 & 4.87e-07 &  4.8 
%                 epg4 &     4 & 4.27e-06 &  3.0 & 2.77e-06 &  4.1 & 6.67e-06 &  3.8 & 2.72e-05 &  3.4 & 1.09e-07 &  4.5 
%                 epg8 &     8 & 1.55e-06 &  2.8 & 6.96e-07 &  4.0 & 1.65e-06 &  4.0 & 7.25e-06 &  3.8 & 2.69e-08 &  4.1 
% Convergence rates: c0=1.63 c1=2.02 c2=1.90 c3=1.79 c4=2.15 
% 
% -scf=1e-3 -tf=.3
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.54e-04 &      & 1.06e-04 &      & 1.62e-04 &      & 4.13e-04 &      & 3.65e-06 &      
%                 epg2 &     2 & 5.10e-05 &  3.0 & 2.64e-05 &  4.0 & 4.70e-05 &  3.4 & 9.25e-05 &  4.5 & 8.86e-07 &  4.1 
%                 epg4 &     4 & 1.40e-05 &  3.6 & 6.33e-06 &  4.2 & 1.26e-05 &  3.7 & 2.11e-05 &  4.4 & 2.17e-07 &  4.1 
%                 epg8 &     8 & 3.84e-06 &  3.6 & 1.54e-06 &  4.1 & 3.14e-06 &  4.0 & 5.04e-06 &  4.2 & 5.26e-08 &  4.1 
% Convergence rates: c0=1.78 c1=2.04 c2=1.90 c3=2.12 c4=2.04 
% 
% 
% 
% \end{verbatim}
% }
% 
% %-                 
% REFERENCE -- SET ALL INTERFACE VALUES TO EXACT 
% {\scriptsize\orange
% \begin{verbatim}
% AMP -scf=1000
% -tf=.1
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 1.04e-05 &      & 5.86e-06 &      & 3.71e-05 &      & 5.58e-04 &      & 8.85e-04 &      
%                 epg2 &     2 & 1.28e-06 &  8.1 & 3.74e-07 & 15.7 & 1.42e-05 &  2.6 & 1.42e-04 &  3.9 & 1.70e-04 &  5.2 
%                 epg4 &     4 & 1.59e-07 &  8.1 & 2.42e-08 & 15.5 & 3.87e-06 &  3.7 & 3.61e-05 &  3.9 & 5.56e-05 &  3.1 
%                 epg8 &     8 & 1.88e-08 &  8.5 & 1.43e-09 & 16.9 & 9.85e-07 &  3.9 & 9.11e-06 &  4.0 & 1.61e-05 &  3.5 
% Convergence rates: c0=3.03 c1=4.00 c2=1.76 c3=1.98 c4=1.90 
% 
% -tf=.2
%                grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r 
%                 epg1 &     1 & 3.71e-05 &      & 2.15e-05 &      & 1.65e-04 &      & 5.15e-04 &      & 2.41e-03 &      
%                 epg2 &     2 & 4.61e-06 &  8.0 & 1.42e-06 & 15.1 & 4.93e-05 &  3.3 & 1.12e-04 &  4.6 & 5.79e-04 &  4.2 
%                 epg4 &     4 & 5.78e-07 &  8.0 & 8.93e-08 & 15.9 & 1.23e-05 &  4.0 & 3.07e-05 &  3.6 & 1.47e-04 &  3.9 
%                 epg8 &     8 & 6.61e-08 &  8.7 & 5.05e-09 & 17.7 & 3.04e-06 &  4.0 & 8.04e-06 &  3.8 & 3.67e-05 &  4.0 
% Convergence rates: c0=3.04 c1=4.02 c2=1.93 c3=1.99 c4=2.01 
% \end{verbatim}
% }
% 
% 
% 
% 
% 
% % --------------------------------------------------------------------
% \clearpage
% \subsection{*OLD* Traditional Scheme - INS IM22 implicit PC}
% \old{
% Results from the TP scheme using the implicit fluid solver INS-IM22.
% 
% \noindent SCF=8000 -- OK
% \input tables/insElasticPiston.epgp.TPSCF8000Imt0p7.ConvTable.tex
% 
% \noindent SCF=1600 -- OK
% \input tables/insElasticPiston.epgp.TPSCF1600Imt0p7.ConvTable.tex
% }
% % --------------------------------------------------------------------
% \clearpage
% \subsection{*OLD* TP Scheme - INS PC22 explicit PC}
% 
% \old{
% Initial results for the TP scheme using the explicit fluid solver INS-PC22.
% 
% Initial results for the TP scheme (no-sub iterations). 
% 
% 
% Results for Cgsm-Godunov and SCF=1600. CFL=.9 is now OK after some fixes.
% \input tables/insElasticPiston.epgp.TPSc1600t0p7.ConvTable.tex
% 
% % Results for Cgsm-Godunov NOTE CFL=.25 and SCF=1600. Currently some trouble for SCF=800 (on G4) or larger CFL.
% % I wonder if the lower CFL is caused from Cgsm-G requiring the traction-rate as an interface BC : $\partial_t \sigmav_f$. 
% % \input tables/insElasticPiston.epgp.TPscf1600.ConvTable.tex
% 
% Results for Cgsm-SOS-C (conservtive SOS scheme): (SCF=1600. CFL=.9). Also trouble for SCF=800 on G4 I think.
% \input tables/insElasticPiston.epgp.TPscf1600SOSC.ConvTable.tex
% 
% 
% SCF=1000 
% }
% 
% % --------------------------------------------------------------------
% \clearpage
% \subsection{*OLD* AMP Scheme - INS IM22 implicit PC}
% 
% \old{
% Results from the AMP scheme using the implicit fluid solver INS-IM22. 
% 
% SCF=1: 
% \input tables/insElasticPiston.epgp.AmpSCF1Imt0p3.ConvTable.tex
% 
% SCF=1 $t=.7$ -- wiggles form on interface for CFL=.9, but CFL=.25 OK 
% \input tables/insElasticPiston.epgp.AmpSCF1Imt0p7.ConvTable.tex
% 
% SCF=0.1  -- wiggles form on interface for CFL=.9, but CFL=.25 OK 
% \input tables/insElasticPiston.epgp.AmpSCF0p1Imt0p7.ConvTable.tex
% 
% SCF=.01 CFL=.6 OK   (CFL=.75 not ok for G4)
% \input tables/insElasticPiston.epgp.AmpSCF0p01Imt0p7.ConvTable.tex
% }
% 
% % --------------------------------------------------------------------
% \clearpage
% \subsection{*OLD* AMP Scheme - INS PC22 explicit PC}
% 
% \old{
% Initial results for the AMP scheme using the explicit fluid solver INS-PC22.
% 
% SCF=.001, $t=.3$
% \input tables/insElasticPiston.epgp.AmpScf0p001t0p3.ConvTable.tex
% 
% SCF=.001, $t=.7$
% \input tables/insElasticPiston.epgp.AmpScf0p001t0p7.ConvTable.tex
% 
% SCF=0.1
% \input tables/insElasticPiston.epgp.AmpScf0p1t0p3.ConvTable.tex
% 
% Results for SCF=1. 
% \input tables/insElasticPiston.epgp.AmpScf1.ConvTable.tex
% 
% \clearpage
% SCF=10:
% \input tables/insElasticPiston.epgp.AmpScf10t0p3.ConvTable.tex
% 
% 
% SCF=1000: $t=.3$ Fluids rates POOR, may be polluted by solid 
% \input tables/insElasticPiston.epgp.AmpScf1000t0p3.ConvTable.tex
% 
% SCF=1000: $t=.7$ Fluids rates POOR, may be polluted by solid 
% \input tables/insElasticPiston.epgp.AmpScf1000t0p7.ConvTable.tex
% 
% SCF=1000: $t=.8$ 
% \input tables/insElasticPiston.epgp.AmpScf1000t0p8.ConvTable.tex
% }
% 


==> texFiles/elasticShearMatlab_7-23.tex <==
\begin{table}[H]
\caption{\label{fig:ShearSolutionConvergence}Shear solution convergence tables for $\rhos/\rho = 10^3,\, \rhos/\rho=1,$ and $\rhos/\rho=10^{-3}.$
The parameters were chosen to be
$\bar{H} = \frac{1}{2}, H = 1, \rho = 1, \rhos = \mus = \lambdas = \mu$.
The final time is $t_{\rm final} = 0.3.$ 
Matlab, \texttt{cdv=0, jv1=1, jv2=1, jvf2=1}.
}
\begin{center}
\begin{tabular}{c}
Heavy solid: $\rhos/\rho = 10^3$ 
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  1.3e-10 &      &  4.5e-04 &      &  1.9e-04 &      &  5.1e-04 &      &  9.8e-01 &     \\
1/ 40 &   105 &  5.8e-11 &  2.3 &  1.1e-04 &  4.0 &  4.6e-05 &  4.2 &  1.4e-04 &  3.6 &  2.6e-01 &  3.8 \\
1/ 80 &   208 &  2.2e-11 &  2.7 &  2.8e-05 &  4.0 &  1.1e-05 &  4.1 &  3.8e-05 &  3.7 &  6.5e-02 &  3.9 \\
1/160 &   416 &  1.2e-11 &  1.8 &  6.9e-06 &  4.0 &  2.8e-06 &  4.0 &  9.9e-06 &  3.8 &  1.6e-02 &  4.0 \\
\hline
\\
\end{tabular}

\begin{tabular}{c}
Medium solid: $\rhos/\rho = 1$ 
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  5.3e-16 &      &  1.4e-05 &      &  2.9e-06 &      &  1.1e-05 &      &  4.8e-05 &     \\
1/ 40 &   105 &  7.5e-16 &  0.7 &  3.3e-06 &  4.1 &  5.8e-07 &  5.0 &  2.0e-06 &  5.6 &  1.1e-05 &  4.2 \\
1/ 80 &   208 &  1.5e-15 &  0.5 &  8.1e-07 &  4.1 &  1.3e-07 &  4.5 &  4.8e-07 &  4.2 &  2.8e-06 &  4.0 \\
1/160 &   416 &  3.6e-15 &  0.4 &  2.0e-07 &  4.0 &  3.0e-08 &  4.3 &  1.2e-07 &  3.8 &  7.1e-07 &  4.0 \\
\hline
\\
\end{tabular}

\begin{tabular}{c}
Light solid: $\rhos/\rho = 10^{-3}$ 
\end{tabular}
\begin{tabular}{cccccccccccc}
\hline
$h$ & $N_t$ & $E^{(p)}$ & $r$ & $E^{(\vv)}$ & $r$ & $E^{(\usv)}$ & $r$ & $E^{(\vsv)}$ & $r$ & $E^{(\sigmasv)}$ & $r$\\
\hline
1/ 20 &    53 &  7.5e-20 &      &  4.9e-05 &      &  7.5e-06 &      &  4.9e-05 &      &  5.0e-08 &     \\
1/ 40 &   105 &  3.1e-20 &  2.4 &  2.2e-05 &  2.3 &  3.7e-06 &  2.0 &  2.2e-05 &  2.3 &  2.2e-08 &  2.3 \\
1/ 80 &   208 &  6.7e-20 &  0.5 &  6.5e-06 &  3.3 &  1.2e-06 &  2.9 &  6.5e-06 &  3.3 &  6.5e-09 &  3.3 \\
1/160 &   416 &  3.1e-20 &  2.1 &  1.7e-06 &  3.9 &  3.4e-07 &  3.7 &  1.7e-06 &  3.9 &  1.7e-09 &  3.9 \\
\hline
\end{tabular}

\end{center}
\end{table}



==> texFiles/exactSolutions.tex <==
\section{Exact solutions} 

In this section, we discuss various exact solutions to the FSI problem.
These exact solutions are used to test and verify the AMP algorithm in
section \ref{sec:numericalResults}.

\subsection{Rectangular elastic piston} \label{sec:ElasticPiston}

%\input texFiles/rectangularGeometryNumericalResults

The geometry of the rectangular elastic piston is shown in figure
\ref{fig:rectangularModelProblemNumericalResults}.
We consider 1D longitudinal motions in the $y$ dimension. The horizontal fluid velocity, $v_1,$ 
solid displacement, $\us_1,$ and derivatives with respect to $x$ are all zero.
With this simplification, the vertical fluid velocity is equal to the interface velocity everywhere in the domain, $v_2 = v_2(t)$,
and the pressure is a time-dependent linear interpolant between the interface pressure, $p_I(t),$ and the specified boundary pressure at $y=H$, $p_0(t)$. 
The solid boundary at $y=-\Hs$ is held fixed so that $\us_2 = 0.$ The fluid and solid equations simplify to 
\begin{alignat}{2}
\dot{v}_{2}(t) &= - \frac{p_0(t) - p_I(t)}{\rho H} 
\bigg{/}\left(1 - \frac{y_{I}(t)}{H}\right), \quad &&y \in (y_I(t),H)
\label{eq:ElasticPistonMomentum} \\
\bar{u}_{2,tt} &= \bar{c}_p^2 \bar{u}_{2,\bar{y}\bar{y}}, \quad &&\ys \in (-\Hs,0)
\label{eq:LongitudinalWaveEquation}
\end{alignat}
%
where $y_I(t) = u_2(0,t)$ is the solid interface deformation. 
Equation \eqref{eq:ElasticPistonMomentum} implies that the (uniform) fluid velocity is driven by a pressure gradient 
and equation \eqref{eq:LongitudinalWaveEquation} is a longitudinal wave equation for the solid displacement.
The interface conditions are
\begin{align}
v_2(t) &= \dot{y}_I(t) \\
(\lambdas + 2 \mus) \us_{2,\bar{y}}(0,t) &= -p_I(t).
\end{align}
%
The fluid variables can be eliminated from equation \eqref{eq:ElasticPistonMomentum} 
to obtain a boundary condition at the interface for $\us.$
\begin{align}
\us_{tt}(0,t) = - \frac{p_0(t) + (\lambdas+2\mus)\us_\ys(0,t)}{\rho H} \bigg{/}
\left(1 - \frac{\us(0,t)}{H} \right)
\label{eq:NonlinearInterfaceCondition}
\end{align}
%
In general, the nonlinear initial-boundary value problem may not be solvable. When 
$\us(0,t)/H$ is small, an asymptotic solution may be obtained. Instead, we 
manufacture an exact solution by finding $p_0$
for a given solid displacement.
Let the solid displacement be given by
\begin{align}
\bar{u}_2(\ys,t) = F(t + (\ys+\Hs)/\cp ) -  F(t - (\ys+\Hs)/\cp),
\end{align}
% 
for any smooth function $F$.
This satisfies both the wave equation and the displacement boundary 
condition at $\ys=-\Hs$. 
% Given this solution, the interface quantities are computed
% \begin{align}
% y_I(t) &= A \sin(k\bar{H}) \cos(\bar{c}_p k t + \phi_0) \\
% v_{2,I}(t) &= -A \bar{c}_p k \sin(k\bar{H}) \sin(\bar{c}_p k t + \phi_0) \\
% p_I(t) = -\sigma_{22,I}(t) &=  
% - A (\bar{\lambda} + 2 \bar{\mu}) \bar{c}_p k
% \, \wdh{\cos(k\bar{H})} \cos(\bar{c}_p k t + \phi_0).
% \end{align}
% %
% Using \eqref{eq:NonlinearInterfaceCondition}, the pressure at $y=H$ is given by
% \begin{align}
% p_0(t) = p_I(t) - \rho H \dot{v}_{2,I}(t) \left(1 - \frac{y_I(t)}{H}\right)
% \end{align}
% %
% and the exact pressure is given by
% \begin{align}
% p(y,t) = p_0(t) - \frac{p_0(t) - p_I(t)}{H - y_I(t)} (H - y).
% \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ramp function here:
Given this solution, the interface quantities are computed to be
\begin{align}
y_I(t) &= F(t + \Hs/\cp ) -  F(t - \Hs/\cp),  \\
% \dot{y}_{I}(t) &= \us_{2,t}(0,t) =  F'(t + \Hs/\cp ) -  F'(t - \Hs/\cp), \\
% \ddot{y}_{I}(t) &=  F''(t + \Hs/\cp ) -  F''(t - \Hs/\cp),\\
p_I(t) &= 
       -\f{\lambdas+2\mus}{\cp} \, \Big( F'(t + \Hs/\cp ) +  F'(t - \Hs/\cp) \Big).
\end{align}
%
Using \eqref{eq:NonlinearInterfaceCondition}, the $p_0(t)$ is given by
\begin{align}
p_0(t) = p_I(t) - \rho H \ddot{y}_{I}(t) \left(1 - \frac{y_I(t)}{H}\right) ,
\end{align}
%
and the exact pressure is given by
\begin{align}
p(y,t) = p_0(t) - \frac{p_0(t) - p_I(t)}{H - y_I(t)} (H - y).
\end{align}
%
The fluid velocity and solid stress are then given by
\begin{align}
v_2(y,t) &= \dot{y}_{I}(t), \\
    \sigmas_{22}(\ys,t) &= 
               \f{(\lambdas+2\mus)}{\cp} \, \Big( F'(t + (\ys+\Hs)/\cp ) +  F'(t - (\ys+\Hs)/\cp) \Big).
\end{align}
%
This solution is valid for any smooth $F$. We choose
\begin{align}
  & F(\xi) = \alpha \,\sin(2\pi k (\xi - \phi_0)),
\end{align}
%
It can be shown that the interface displacement at $t=0$ is given by
\begin{align}
   y_I(0) %&=  F(\Hs/\cp ) -  F(-\Hs/\cp) = \alpha \,
          %    \Big( \sin(2\pi k (\Hs/\cp - \phi_0)) - \sin(2\pi k (-\Hs/\cp - \phi_0))\Big) , \\ 
      &= 2 \alpha \, \sin(2 \pi k \Hs/\cp) \, \cos(2\pi k  \phi_0).
\end{align}
% 
We choose $\phi_0=1/(4 k)$ so the interface is initially undeformed. 


% \das{here we describe the ramp function, but it seems like we don't use a ramp function in code}
%
% This solution is valid for any smooth $F$. We choose
% \begin{align}
%   & F(\xi) = \alpha \, R(\xi) \,\sin(2\pi k (\xi - \phi_0)),
% \end{align}
% %
% where $R(\xi)$ is a ramp function that smoothly transitions from zero to one.
% A ramp function is used to avoid initialization issues with moving grids. The ramp 
% function is given by
% \begin{align}
% R(t) = 
% \begin{cases}
% 0, & t < 0\\
% (9+(-12+(3+t)t)t)t^3 & 0 \le t \le 1\\
% 1, & t > 1
% \end{cases}.
% \end{align}
% %
% This satisfies $R'(0) = R''(0) = R'(1) = R''(1) = 0,$ so the 
% velocity and acceleration are continuous.

% The {\tt rampOrder} defines the number of zero derivatives at the ramp interval ends. It is
% needed to have at least 2 zero derivatives 
% so the acceleration is continuous.
% We need to have the ramp function satisfy
% \[
%    F(\xi)=0 ~~\text{for}~~ \xi \le (\ys+\Hs)/\cp \le \Hs/\cp. 
% \] 
% With no ramp function, $R(\xi)=1$, the interface will be at $\ys=0$ at $t=0$ provided
% \begin{align}
%    \us_2(\ys,t) &=  F(\Hs/\cp ) -  F(-\Hs/\cp) = \alpha \,
%               \Big( \sin(2\pi k (\Hs/\cp - \phi_0)) - \sin(2\pi k (-\Hs/\cp - \phi_0))\Big) , \\ 
%       &= 2 \alpha \, \sin(2 \pi k \Hs/\cp) \, \cos(2\pi k  \phi_0).
% \end{align}
% % 
% and we can choose $\phi_0=1/(4 k)$. For a second-order accurate solution 
% we may need the ramp to have
% at least two, and maybe three?, or four ?, continuous derivatives, $R(0)=R'(0)=R''(0)=R'''(0)=R''''(0)=0$. 


% $r_a = -10, r_b = -9$

\subsection{Rectangular shear solution} \label{sec:ShearSolution}


The geometry of the rectangular shear solution is identical to that of the 
elastic piston and is shown in figure \ref{fig:rectangularModelProblemNumericalResults}.
We consider pure transverse motions in the fluid and solid.
The vertical fluid velocity, $v_2,$ solid displacement, $\us_2,$
and derivatives with respect to $x$ are all zero. Since there is no 
longitudinal displacement, (ie. $y_I(t) = 0$), the solid reference coordinate $\ys$ is 
equivalent to the physical coordinate $y.$
The equations simplify to
\begin{alignat}{2}
\rho v_{1,t} &= \mu v_{1,yy}, \quad &&y \in (0,H) 
\label{eq:HeatEquationFluid} \\
\us_{1,tt} &= \cs^2 \bar{u}_{1,yy}, \quad &&y \in (-\bar{H},0).
\label{eq:ShearWaveEquation}
\end{alignat}
%
Equation \eqref{eq:HeatEquationFluid} is a heat equation for the horizontal fluid velocity 
and equation \eqref{eq:ShearWaveEquation} is a shear wave equation for the horizontal solid displacement.
These equations can be solved by searching for solutions of the form
\begin{align}
v_1(y,t) = \hat{v}_1(y) e^{i \omega t}, \quad \us_1(y,t) = \hat{\us}_1(y) e^{i \omega t}. 
\end{align}
%
The equations are simplified to second order constant coefficient ODEs in $y$, given by
\begin{align}
\hat{v}_1'' + \lambda^2 \hat{v}_1 &= 0, \\
\hat{\us}_1'' + k_s^2 \hat{\us}_1 &= 0,
\end{align}
%
where
\begin{align}
\lambda^2 = - \frac{i \rho \omega}{\mu}, \quad k_s^2 = \frac{\omega^2}{\cs^2}.
\end{align}
%
The solutions are
\begin{align}
\hat{v}_1(y) &=  a_1 \sin(\lambda (H-y)) + a_2 \cos(\lambda (H-y)), \\
\hat{\us}_1(y) &= b_1 \sin(k_s (y+\Hs)) +b_2 \cos(k_s (y+\Hs)),
\end{align}
%
where $a_1,a_2,b_1,b_2$ are constants to be determined by the boundary conditions.
At the solid boundary, $y = -\Hs,$ the solid is fixed so that $\us_1 = 0$.
A no-slip boundary condition, $v_1 = 0$, is applied at the fluid boundary, $y = H.$
These two conditions imply that $a_2=b_2=0.$
The interface matching conditions are
\begin{alignat}{2}
v_1(0,t) &= \us_{1,t}(0,t),  \\
\mu v_{1,y}(0,t) &= \mus \us_{1,y}(0,t).
\end{alignat}
%
The interface conditions form a homogeneous system of equations for 
$a_1$ and $b_1,$ given by
\begin{align}
\left[\begin{array}{cc}
\sin(\lambda H) & -i \omega \sin(k_s \Hs) \\
-\mu \lambda  \cos(\lambda H) & -\mus k_s \cos(k_s \Hs)
\end{array}\right]
\left[\begin{array}{c}
a_1 \\ b_1
\end{array}\right]
= 0 \label{eq:ShearSolutionSystem}
\end{align}
%
In order for nontrivial solutions for $a_1$ and $b_1$ to exist, the system must be singular.
It can be shown that solutions exist when the following dispersion relation is satisfied.
\begin{align}
\frac{\mus}{\mu \omega} \tan(\lambda H) =-  \frac{i \lambda}{k_s} \tan(k_s \Hs) 
\end{align}
%
This is a condition on $\omega$.
There seems to infinitely many solutions where $\Re(\omega) > 0$
and $\Im(\omega) > 0.$ These solutions correspond to interface oscillations which damp in time. 
Equation \ref{eq:ShearSolutionSystem} can be used to find $a_1$ and $b_1$ up to a scale factor,
namely
\begin{align}
\frac{a_1}{b_1} = i \omega \frac{\sin(k_s \Hs)}{\sin(\lambda H)}.
\end{align}
%
An extra condition is needed to determine the constants uniquely. 
The initial interface displacement is chosen to be $\us_1(0,0) = \us_{\max},$
which gives
\begin{align}
b_1 = \frac{\us_{\max}}{\sin (k_s \Hs)}.
\end{align}


\subsection{Radial elastic piston} \label{sec:RadialElasticPiston}

The radial elastic piston is the analogous solution to the rectangular elastic piston in
polar coordinates. We first define the polar basis vectors to be
\begin{align}
\ev_r = 
\left[\begin{array}{c}
\cos(\theta) \\ \sin(\theta)
\end{array}\right], \quad
\ev_\theta = 
\left[\begin{array}{c}
-\sin(\theta) \\ \cos(\theta)
\end{array}\right].
\end{align}
%
Subscripts $r$ and $\theta$ will be used to denote components of a vector and tensor, (ie.
$\vv = v_r \ev_r + v_\theta \ev_\theta$
and 
$\sigmav = \sigma_{rr} \ev_r \ev_r^T 
+ \sigma_{r\theta} \ev_r \ev_\theta^T
+ \sigma_{\theta r} \ev_\theta \ev_r^T
+ \sigma_{\theta\theta} \ev_\theta \ev_\theta^T$).


\input texFiles/radialElasticPistonGeometry

The geometry of the radial elastic piston solution is shown in figure \ref{fig:radialElasticPistonGeometry}.
Axisymmetric radial motions of the fluid and solid are considered.
The circumferential components of the fluid velocity, $v_\theta,$ and solid displacement, $\us_\theta$, are zero.
Under this assumption, the fluid continuity equation \eqref{eq:fluidContinuity} reduces to 
\begin{align}
\frac{1}{r} \frac{\partial }{\partial r} (r v_r) = 0, \quad r \in (R_I(t),R_f),
\end{align}
%
where $R_I(t)$ is the radial location of the interface.
The solution for the radial component of the fluid velocity is of the form
\begin{align}
v_r(r,t) = \frac{1}{r} f(t)
\end{align}
%
where $f(t)$ is some function of time, determined by a boundary condition.
The radial component of the fluid momentum equation \eqref{eq:fluidMomentum} reduces to
\begin{align}
\frac{\partial p}{ \partial r} = 
\frac{\rho}{r^3} f(t)^2 
- \frac{\rho}{r} f'(t), \quad r \in (R_I(t),R_f).
\end{align}
%
This equation can be integrated to solve for the pressure,
\begin{align}
p(r,t) = g(t) - \frac{\rho}{2r^2} f(t)^2 - \rho f'(t) \log \left( \frac{r}{R_I(I)} \right),
\label{eq:radialPistonPressure}
\end{align}
%
where $g(t)$ is the constant of integration which will be determined by boundary condition on pressure at $r=R_f.$
The solid equations simplify to a wave equation for the radial component of displacement,
\begin{align}
\frac{\partial^2 \us_r}{\partial t^2} = 
\cp^2 \frac{\partial}{\partial \rs} 
\left(  \frac{1}{\rs} \frac{\partial (\rs \us_r)}{\partial \rs}\right), \quad \rs \in (0,R_I(0))
\label{eq:radialWaveEquation}
\end{align}
%
We require the solid displacement remain bounded at $\rs=0.$
Equations \eqref{eq:radialPistonPressure} and \eqref{eq:radialWaveEquation} are 
the counterpart in polar coordinates to equations \eqref{eq:ElasticPistonMomentum} and \eqref{eq:LongitudinalWaveEquation}, respectively.
The interface matching conditions are given by
\begin{align}
v_r(R_I(t),t) &= \vs_r(R,t), \\
 \sigma_{rr}(R_I(t),t) &= \sigmas_{rr}(R,t).
\end{align}
%
Instead of solving the general initial boundary value problem, 
we `choose' a form of solution for the solid and determine $f(t)$ and $g(t)$ so that the equations are satisfied.
We look for solutions where the solid displacement is sinusoidal in time.
\begin{align}
\us_r(\rs,t) = \hat{\us}(\rs) \sin(\cp k t)
\end{align}
%
After substituting into equation \eqref{eq:radialWaveEquation}, 
a Bessel equation for $\hat{\us}(\rs)$ is obtained.
\begin{align}
\rs^2 \hat{\us}'' + \rs \hat{\us}' + (k^2 \rs^2 - 1) \hat{\us} = 0
\end{align}
%
Both $J_1(k\rs)$ and $Y_1(k\rs)$ are solutions to this equation, but only $J_1(k\rs)$ remains bounded at $\rs=0,$
therefore the solution for the solid displacement is 
\begin{align}
\us_r(\rs,t) = \us_0 J_1(k\rs) \sin(\cp k t).
\end{align}
%
The solid velocity and stress are given by
\begin{align}
\vs_r(\rs,t) &= \cp k \us_0 J_1(k \rs) \cos(\cp k t) \\
\sigmas_{rr}(r,t) &= 
 u_0 \sin(\cp k t) \left[ \frac{\lambdas}{r} J_1(k \rs)
+ k (\lambdas+ 2 \mus) J_1'(k \rs)\right].
\end{align}
%
The velocity matching condition is used to obtain $f(t)$, given by
\begin{align}
f(t) =  R_I(t) \; \vs_r(R,t).
\end{align}
%
Using the definition of the fluid stress tensor in equation \eqref{eq:fluidStressTensor},
the fluid stress is given by
\begin{align}
\sigma_{rr}(r,t) = 
-g(t) + \frac{\rho}{2r^2} f(t)^2 + \rho f'(t) \log \left( \frac{r}{R_I(I)} \right)
- \frac{2 \mu}{r^2} f(t).
\end{align}
%
The stress matching condition is then used to obtain $g(t)$.
\begin{align}
g(t) = 
\frac{\rho}{2R_I(t)^2} f(t)^2 - \frac{2 \mu}{R_I(t)^2} f(t)
-\sigmas_{rr}(R,t)
\end{align}

\subsection{Radial shear solution} \label{sec:RadialShearSolution}

The geometry of the radial shear solution is identical to that of the elastic piston 
geometry shown in figure \ref{fig:radialElasticPistonGeometry}, except we consider 
the interface radius to be constant for all time, $R_I(t) = R.$
We consider axisymmetric circumferential motions of the fluid and solid.
The radial component of the fluid velocity, $v_r$, and solid displacement, $\us_r$, is zero.
Under these assumptions, the equations reduce to
\begin{alignat}{2}
\rho \frac{\partial v_\theta}{\partial t} &= 
\mu \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r v_\theta)}{\partial r}\right), \quad &&r \in (R,R_f)
\label{eq:radialHeatEquation} \\
\frac{\partial^2 \us_\theta}{\partial t^2} &= \cs^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_\theta)}{\partial r}\right), \quad &&r \in (0,R)
\label{eq:radialShearWaveEquation}
\end{alignat}
%
Equation \eqref{eq:radialHeatEquation} is a heat equation for the circumferential fluid velocity
and equation \eqref{eq:radialShearWaveEquation} is a wave equation for the circumferential 
solid displacement. These equations are analogous to equations \eqref{eq:HeatEquationFluid}
and \eqref{eq:ShearWaveEquation} obtained for the rectangular shear solution.
We search for solutions of the form
\begin{align}
v_\theta(r,t) = \hat{v}_\theta(r) e^{i \omega t}, \quad
\us_\theta(r,t) = \hat{\us}_\theta(r) e^{i \omega t}
\end{align}
%
The fluid and solid equations simplify to Bessel equations given by
\begin{align}
r^2 \hat{v}_\theta'' + r \hat{v}_\theta' + (\lambda^2 r^2 - 1) \hat{v}_\theta &= 0\\
r^2 \hat{\us}_\theta'' + r \hat{\us}_\theta' + (k_s^2 r^2 - 1) \hat{\us}_\theta &= 0 ,
\end{align}
%
where
\begin{align}
\lambda^2 = - \frac{i \rho \omega}{\mu}, \quad k_s^2 = \frac{\omega^2}{\cs^2}.
\end{align}
%
$\lambda$ and $k_s$ are the same constants that arise in the rectangular shear solution.
Define
% \begin{align}
% \hat{v}_\theta(r,t) &= a_1 (Y_1(\lambda R_f) J_1(\lambda r) - J_1(\lambda R_f) Y_1(\lambda r))
% + a_2 (Y_1(\lambda R_f) J_1(\lambda r) + J_1(\lambda R_f) Y_1(\lambda r)),\\
% \hat{\us}_\theta(r,t) &= b_1 J_1(k_s r) + b_2 Y_1(k_s r),
% \end{align}
\newcommand{\B}{B}
\newcommand{\C}{C}
\begin{align}
\B(\xi) = Y_1(\lambda R_f) J_1(\xi) - J_1(\lambda R_f) Y_1(\xi) \\
\C(\xi) = Y_1(\lambda R_f) J_1(\xi) + J_1(\lambda R_f) Y_1(\xi),
\end{align}
%
then the solutions for the transformed variables are
\begin{align}
\hat{v}_\theta(r,t) &= a_1 \B(\lambda r) + a_2 \C(\lambda r)\\
\hat{\us}_\theta(r,t) &= b_1 J_1(k_s r) + b_2 Y_1(k_s r),
\end{align}
%
where $a_1,a_2,b_1,b_2$ are constants to be determined by the boundary conditions.
At $r=0,$ we enforce that the solid solution is bounded. 
At the fluid boundary, $r=R_f$, a no-slip boundary condition is applied, $\hat{v}_\theta = 0.$
Due to these conditions, we must take $a_2=b_2=0.$

Two interface conditions are required. The interface position in Eulerian coordinates is given by
$\xv_I = R \ev_r + \us_\theta(R,t) \ev_\theta.$ Since $|\xv_I|^2 - R^2 = |\us_\theta(R,t)|^2$,
the radial coordinate of the interface increases when $|\us_\theta|$ is non-zero. 
We ignore this `warping' effect by considering the case when $\frac{|\us_\theta|}{R} \ll 1$.
The interface matching conditions are
\begin{align}
v_\theta(R,t) = \vs_\theta(R,t), \\
\sigma_{r\theta}(R,t) = \sigmas_{r\theta}(R,t) .
\end{align}
%
As in the rectangular shear case, the interface conditions 
form a homogeneous system of equations for $a_1$ and $b_1,$ given by
\begin{align}
\left[\begin{array}{cc}
\B(\lambda R) & - i \omega J_1(k_s R) \\
\mu \left(\lambda \B'(\lambda R) - \frac{\B(\lambda R)}{R} \right) & 
-\mus \left( k_s J_1'(k_s R) - \frac{J_1(k_s R)}{R}\right)
\end{array}\right]
\left[\begin{array}{c}
a_1 \\ b_1
\end{array}\right]
= 0. \label{eq:RadialShearSystem}
\end{align}
%
In order for nontrivial solutions for $a_1$ and $b_1$ to exist, the system must be singular.
It can be shown that solutions exist when the following dispersion relation is satisfied.
\begin{align}
\frac{\mus}{\omega \mu} \left(\frac{J_1'(k_s R)}{J_1(k_s R)} - \frac{1}{R k_s} \right)
= \frac{i \lambda}{k_s} \left(\frac{\B'(\lambda R)}{\B(\lambda R)} - \frac{1}{R \lambda} \right) 
\end{align}
%
This is a condition for $\omega.$
As in the case of the Cartesian shear solution, there are infinitely many solutions
corresponding to interface oscillations which damp in time.
Equation \eqref{eq:RadialShearSystem} can be used to determine the two constants up 
to a scale factor, namely
\begin{align}
\frac{a_1}{b_1} = i \omega \frac{J_1(k_s R)}{B(\lambda R)}.
\end{align}
%
The initial interface displacement, $\us_{\theta}(R,0) = \us_{\max},$ 
is then given as a final condition giving
\begin{align}
b_1 = \frac{\us_{\max}}{J_1(k_s r)}.
\end{align}
%
After obtaining the solution for the fluid velocity, the pressure can be obtained
by solving 
\begin{align}
- \frac{\rho}{r} v_\theta^2 + \frac{\partial p}{\partial r} &= 0 .
\end{align}
%
Since the radial component of momentum is zero, the centripetal force 
in the fluid must be balanced by the pressure gradient.
A final interface condition arises by setting $\sigma_{rr} = \sigmas_{rr}$ at the
interface. Since $\sigmas_{rr}=0$ and the only contribution to $\sigma_{rr}$
is from the fluid pressure, this interface condition becomes
\begin{align}
p(R,t) = 0.
\end{align}
%
The solution for the pressure is thus given by
\begin{align}
p(r,t) = \rho \int_R^r \frac{v_\theta(s,t)^2}{s} \; ds.
\end{align}


\subsection{Radial traveling wave solution} \label{sec:RadialTravelingWave}

\input texFiles/radialTravelingWaveGeometry
The geometry for the radial traveling wave solution is shown in figure \ref{fig:radialTravelingWaveGeometry}.
Consider small disturbance solutions to the fluid equations
\eqref{eq:fluidContinuity}--\eqref{eq:fluidMomentum}
of the form
\begin{align}
\vv(r,\theta,t) = 
\left(\hat{v}_r(r) \ev_r + \hat{v}_\theta(r) \ev_\theta\right)
e^{i (n \theta - \omega t)}, \quad 
p(r,\theta,t) = \hat{p}(r) e^{i (n \theta - \omega t)},
\end{align}
%
where $n\ge1$. We consider $|\hat{v}_r|^2$ and $|\hat{v}_\theta|^2$ to be small, therefore we will ignore 
convection terms.
Under these assumptions, the fluid equations reduce to
\begin{align}
\hat{p}'' 
+ \frac{1}{r} \hat{p}'
- \frac{n^2}{r^2} \hat{p} &= 0 \label{eq:eulerp}\\
r^2 \hat{v}_r'' + 3 r \hat{v}_r' + (\lambda^2 r^2 - n^2+1) \hat{v}_r
&= \frac{r^2}{\mu} \hat{p}' 
\label{eq:besselvr} \\
\hat{v}_\theta &= -\frac{1}{in} \left(\hat{v}_r + r \hat{v}_r' \right),
\label{eq:constraintvt}
\end{align}
%
with $\lambda^2 = - i \rho \omega / \mu$ as defined in the previous solutions.
Equation \eqref{eq:eulerp} 
is an Euler equation for $\hat{p}$ resulting from the pressure Poisson equation.
Equation \eqref{eq:besselvr} can be manipulated into a Bessel equation
for $\hat{v}_r$ with a forcing term.
Equation \eqref{eq:constraintvt} is a constraint on $\hat{v}_\theta$ resulting from the
continuity equation. The solution is
\begin{align}
\hat{p}(r) &= a_1 \left( \frac{r}{R} \right)^n + a_2 \left( \frac{r}{R}\right)^{-n} \\
\hat{v}_r(r) &= 
\frac{a_3}{r} J_n(\lambda r) + \frac{a_4}{r} Y_n(\lambda r) 
+ \frac{a_1}{r} \frac{n}{\mu \lambda^2} \left( \frac{r}{R} \right)^n
- \frac{a_2}{r} \frac{n}{\mu \lambda^2} \left( \frac{r}{R}\right)^{-n},
\end{align}
%
where $a_1,\,a_2,\,a_3,\,a_4,$ are constants determined by the boundary conditions. 
In order for the fluid solution to remain bounded at $r=0$, we must have $a_2=a_4=0.$
$\hat{v}_\theta$ can be obtained using equation \eqref{eq:constraintvt}.

For the solid, we use Helmholtz decomposition to find the solution.
We write the solid displacement as the sum of a divergence-free component and a 
curl-free component,
\begin{align}
\usv = \grad \phi + \grad \curl \Hv.
\end{align}
%
When substituting this into the solid equations 
\eqref{eq:solidDisplacement}--\eqref{eq:solidMomentum},
we find that $\phi$ and $\Hv$ must satisfy wave equations with speeds $\cp$
and $\cs$, respectively.
\begin{align}
\phi_{tt} &= \cp^2 \Delta \phi \label{eq:waveEquationPhi}\\
\Hv_{tt} &= \cs^2 \Delta \Hv. \label{eq:waveEquationH}
\end{align}
%
Since we are only considering 2D displacements, $\Hv = H \ev_3$.
We search for solutions of the form
\begin{align}
\phi(r,\theta,t) = \hat{\phi}(r) e^{i (n \theta - \omega t)}, \quad
H(r,\theta,t) = \hat{H}(r) e^{i (n \theta - \omega t)}
\end{align}
%
Equations \eqref{eq:waveEquationPhi}--\eqref{eq:waveEquationH} reduce to 
the following Bessel equations,
\begin{align}
r^2 \hat{\phi}'' + r \hat{\phi} + \left(\frac{\omega^2}{\cp^2} r^2 - n^2 \right) \hat{\phi}
&= 0 \\
r^2 \hat{H}'' + r \hat{H} + \left(\frac{\omega^2}{\cs^2} r^2 - n^2 \right) \hat{H}
&= 0,
\end{align}
%
of which the solutions are
\begin{align}
\hat{\phi}(r) &= b_1 J_n(k_p r) + b_2 Y_n(k_p r) \\
\hat{H}(r) &= b_3 J_n(k_s r) + b_4 Y_n(k_s r),
\end{align}
%
where
\begin{align}
k_p = \frac{\omega}{\cp}, \quad k_s = \frac{\omega}{\cs}.
\end{align}
%
The displacement can be obtained using
\begin{align}
\hat{\us}_r = \hat{\phi}' + \frac{in}{r} \hat{H}, \quad
\hat{\us}_\theta = \frac{in}{r} \hat{\phi} - \hat{H}'.
\end{align}

Eight boundary conditions in total are needed for this solution.
At the interface, $r=R,$ 
there are two dynamic conditions and two kinetic conditions, given by
\begin{align}
\hat{v}_r(R) = \hat{\vs}_r(R), \quad
\hat{v}_\theta(R) = \hat{\vs}_\theta(R), \quad
\hat{\sigma}_{rr}(R) = \hat{\sigmas}_{rr}(R), \quad
\hat{\sigma}_{r\theta}(R) = \hat{\sigmas}_{r\theta}(R).
\end{align}
%
At $r=R_s,$ we impose a free surface condition for the solid,
\begin{align}
\hat{\sigmas}_{rr}(R_s) = 0, \quad
\hat{\sigmas}_{r\theta}(R_s) = 0.
\end{align}
%
The six non-zero boundary conditions are organized into the following matrix equation
\begin{align}
\Mv(\omega) \av = 0,
\end{align}
%
where $\Mv(\omega) \in \Complex^{6 \times 6}$ and $\av = [a_1,a_3,b_1,b_2,b_3,b_4]^T.$
Non-trivial solutions exist when $\det \Mv(\omega) = 0.$ 
A nonlinear root solver can be used to find solutions for $\omega.$
We require $\Im(\omega) \le 0$ so the solution remains bounded in time. When 
$\omega$ is found, an initial condition is needed to determine
$\av$. For this paper we choose
$\sqrt{|\hat{\us}_r(R)|^2 + |\hat{\us}_\theta(R)|^2} = u_I,$ where $u_I$ is the initial
interface displacement.



==> texFiles/governing-orig.tex <==
\section{Governing equations and interface conditions} \label{sec:governingEquations}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Consider an incompressible fluid coupled with a linear-elastic solid. 
The fluid coordinates are described by an Eulerian domain $\xv \in \OmegaF(t),$ where
$\xv$ is the physical coordinate and $t$ is time. 
The solid coordinates are described by a Lagrangian domain $\xsv \in \OmegaS,$ where
$\xsv$ is the reference coordinate of the undeformed solid. The fluid and solid
are coupled at an interface, represented by regions 
$\GammaIf(t)$ in physical space and $\GammaIs$
in reference space. See figure () for a schematic of the fluid-structure interaction problem.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fluid eq
The fluid is described by the incompressible Navier-Stokes equations
\begin{alignat}{2}
\grad \cdot \vv &= 0, \quad &&\xv \in \OmegaF(t)
\label{eq:fluidContinuity} \\
\rho \vv_t + \rho (\vv \cdot \grad) \vv &=
  \grad \cdot \sigmav, \quad &&\xv \in \OmegaF(t)
\label{eq:fluidMomentum}
\end{alignat}
%
where $\vv = \vv(\xv,t)$ is the fluid velocity and $\rho$ is the fluid density.
The fluid stress tensor, $\sigmav = \sigmav(\xv,t),$ is defined as
\begin{align}
\sigmav &= - p \Iv + \tauv \label{eq:fluidStressTensor} 
\end{align}
%
where $p = p(\xv,t)$ is the fluid pressure and $\Iv$ is the identity matrix.
The viscous stress tensor, $\tauv = \tauv(\xv,t),$ is given by
\begin{align}
\tauv &= \mu \left(\grad \vv + \left(\grad \vv\right)^T \right) \label{eq:fluidViscousStressTensor}
\end{align}
%
where $\mu$ is the dynamic viscosity. Interface matching conditions along with 
initial and boundary conditions are needed to close this problem.
In this paper, components of the vector $\vv$ are denoted by
$v_m$ for $m = 1,\,2,\,3$ and components of the tensor $\sigmav$ are denoted by
$\sigma_{mn}$ for $m,\,n = 1,\,2,\,3.$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pressure formulation for fluid 
The fluid equations are treated in velocity-pressure formulation.
Equation \eqref{eq:fluidContinuity} is replaced by a Poisson equation for 
the pressure obtained by taking the divergence of equation 
\eqref{eq:fluidMomentum}. This formulation requires an extra boundary condition, 
which is naturally chosen to be a zero divergence condition for the velocity.
\begin{alignat}{2}
\rho \grad \vv : \left(\grad \vv\right)^T + \Delta p &= 0, \quad &&\xv \in \OmegaF(t)
\label{eq:pressurePoissonEquation} \\
\grad \cdot \vv &= 0, \quad &&\xv \in \partial\OmegaF(t)
\end{alignat}
%
Here,
\begin{align}
\grad \vv : \left(\grad \vv\right)^T = 
\sum_{i=1}^3 \sum_{j=1}^3 \frac{\partial v_i}{\partial x_j} \frac{\partial v_j}{\partial x_i}.
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% solid eq
The solid is described by the equations of linear elasticity.
The equations describe the evolution of solid displacement $\usv = \usv(\xsv,t)$
and velocity $\vsv = \vsv(\xsv,t)$ and are given by
\begin{alignat}{2}
\usv_t &= \vsv, \quad &&\xvs \in \OmegaS 
\label{eq:solidDisplacement} \\
\rhos \vsv_t &= \grads \cdot \sigmasv + \bsv, \quad &&\xvs \in \OmegaS
\label{eq:solidMomentum}
\end{alignat}
%
where $\rhos$ is the solid density and $\bsv = \bsv(\xsv,t)$ is the body force.
The Cauchy stress tensor $\sigmasv$ is defined as
\begin{align}
\sigmasv &= \lambdas (\grads \cdot \usv) \Iv 
+ \mus \left(\grads \usv + \left(\grads \usv\right)^T\right)
\label{eq:solidStressTensor}
\end{align}
%
where $\lambdas$ and $\mus$ are Lam\'e parameters.
The solid deformation is mapped into physical space coordinates
$\ysv = \ysv(\xsv,t)$ using
\begin{align}
\ysv = \xsv + \usv.
\label{eq:solidPhysicalCoordinates}
\end{align}
%
Since we are only concerned with linear elastic solids, the solid strain will be sufficiently 
small such that a one-to-one mapping from $\xsv$ to $\ysv$ exists. 
% This can be seen by
% examining the deformation gradient, given by
% $\grads \ysv = \Iv + \grads \usv$ where $\grads \usv$ is
% the displacement gradient.
% Since $\| \grads \usv \|_2 \ll 1,$ $\grads \ysv$ is locally invertible.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fos for the solid
The solid equations are treated as a first order system of PDEs. The formulation
is achieved by taking the time derivative of \eqref{eq:solidStressTensor} to obtain 
\begin{align}
\sigmasv_t &= \lambdas (\grads \cdot \vsv) \Iv 
+ \mus \left(\grads \vsv + \left(\grads \vsv \right)^T\right).
\label{eq:solidStressTensor}
\end{align}
%
In this form, upwind solvers can be used to update the solid velocity and stress components.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% interface
The interface between the fluid and solid is defined as the regions
$\GammaIf(t)$ in the physical coordinates and $\GammaIs$ in the solid 
reference coordinates. At this interface, matching conditions for
the position, velocity, and traction are required. These are
\begin{alignat}{2}
\xv &= \ysv, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:geometryMatching} \\
\vv &= \vsv, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs 
\label{eq:velocityMatching} \\
\sigmav \nv &= 
\sigmasv \nsv, \quad &&\xv \in \GammaIf(t), \quad \xsv \in \GammaIs. 
\label{eq:tractionMatching}
\end{alignat}
%
In equation \eqref{eq:tractionMatching}, the solid traction is defined using
the solid reference normal $\nsv$ while the fluid traction is defined using the
physical normal. Under the assumptions of linear elasticity, these choices
are arbitrary. 

%%%%%%%%%%%
Since the solid equations form a hyperbolic system of equations, it 
is informative to consider the propagation of characteristics. The 
longitudinal and shear wave speed are defined as
\begin{align}
\cp = \sqrt{\frac{\lambdas+2 \mus}{\rhos}}, \quad
\cs = \sqrt{\frac{ \mus}{\rhos}},
\label{eq:solidWaveSpeeds}
\end{align}
%
respectively. At the interface, incoming and outgoing characteristics can be 
derived from the normal component of the momentum equations. 
If $\nsv$ is the normal to the reference solid domain and 
$\esv_1$ and $\esv_2$ are mutually orthonormal to $\nsv,$ then
the incoming and outgoing characteristics are given by
\begin{alignat}{2}
\Ac(\sigmasv \nsv, \vsv) &= \nsv^T \sigmasv \nsv - \zp \nsv^T \vsv ,
\quad \phantom{m = 1,2,}
\quad &&\xsv \in \GammaIs,
\quad \text{(outgoing)}
\label{eq:ACharacteristic}
\\
\Ac_m(\sigmasv \nsv, \vsv) &= \esv_m^T \sigmasv \nsv - \zs \esv_m^T \vsv, 
\quad m = 1,2,
\quad &&\xsv \in \GammaIs,
\quad \text{(outgoing)}
\label{eq:AmCharacteristic}
\\
\Bc(\sigmasv \nsv, \vsv) &= \nsv^T \sigmasv \nsv + \zp \nsv^T \vsv ,
\quad \phantom{m = 1,2,}
\quad &&\xsv \in \GammaIs,
\quad \text{(incoming)}
\label{eq:BCharacteristic}
\\
\Bc_m(\sigmasv \nsv, \vsv) &= \esv_m^T \sigmasv \nsv + \zs \esv_m^T \vsv ,
\quad m = 1,2,
\quad &&\xsv \in \GammaIs,
\quad \text{(incoming)}.
\label{eq:BmCharacteristic}
\end{alignat}
%
Here, $\zp = \rhos \cp$ and $\zs = \rhos \cs$ are the solid impedances 
for longitudinal and shear waves, respectively. 
Outgoing denotes information that is propagating out of the solid domain
while incoming denotes the opposite.
The interface matching conditions can be used in equations 
\eqref{eq:ACharacteristic}--\eqref{eq:BmCharacteristic}
to derive equivalent characteristic interface conditions which take into 
account the direction of propagation.
\begin{align}
\Ac(\sigmav \nv, \vv)    &= \Ac_{\;\;\;}((\sigmasv \nsv)^{(p)}, \vsv^{(p)}) 
\label{eq:ACharacteristicBC} \\
\Ac_m(\sigmav \nv, \vv)  &= \Ac_m((\sigmasv \nsv)^{(p)}, \vsv^{(p)}) 
\label{eq:AmCharacteristicBC} \\
\Bc(\sigmasv \nsv, \vsv)    &= \Bc_{\;\;\;}((\sigmav \nv)^{(p)}, \vv^{(p)})
\label{eq:BCharacteristicBC} \\
\Bc_m(\sigmasv \nsv, \vsv) &=  \Bc_m((\sigmav \nv)^{(p)}, \vv^{(p)})
\label{eq:BmCharacteristicBC} 
\end{align}
%
The quantities with superscripts 
($(\sigmasv \nsv)^{(p)}, \vsv^{(p)}, (\sigmav \nv)^{(p)}, \vv^{(p)}$) denote 
predicted values. The quantities without superscripts are being assigned by the 
boundary condition.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% actual implementation
This paper studies partitioned algorithms for solving the above FSI problem.
Partitioned algorithms employ separate PDE solvers for the fluid and solid
which only communicate at the interface.
% traditional scheme
In the traditional scheme used in industry, the fluid velocity 
is determined by the solid and the solid traction is determined by the fluid.
This ordering works well for heavy solids,
but suffers from added mass instabilities when the solid density
is light or the solid grid is very fine.
% anti traditional scheme
In the reverse scheme, referred to as the anti-traditional scheme,
the solid applies a traction to the fluid and the solid velocity 
comes from the fluid. This works well
for light solids, but not for heavy solids.
% amp scheme 
The added-mass-partitioned (AMP) scheme instead applies the characteristic conditions
\eqref{eq:ACharacteristicBC}--\eqref{eq:BmCharacteristicBC} as
boundary conditions. In the limit of heavy solids and light solids, 
the AMP scheme approaches the traditional scheme and anti-traditional scheme, respectively.
In this paper, we will prove and demonstrate that the 
AMP scheme is robust for all solid densities.




==> texFiles/halfDiskInAChannel.tex <==
\clearpage
\subsection{Flow past a half solid annulus in a channel}

Consider the flow of an incompressible fluid past a half solid deformable annular disk.

This may be a cleaner example to show the corner fixup -- although after fixing some things in
the code the non-fixed corner behaves not so bad.


Figure~\ref{fig:halfDiskScf1} shows results for SCF=1. 

{% ------------------------------------------
\newcommand{\figWidth}{5.cm}
\newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.0}{.0}{.25}{.25}}
\newcommand{\figWidtha}{6.5cm}
\newcommand{\trimfiga}[2]{\trimh{#1}{#2}{.0}{.0}{.1}{.0}}
\begin{figure}[H]
\begin{center}
\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0.0,.5) rectangle (16.,6.);  % set the bounding box (so we have less surrounding white space)
%
%  \draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{beamInAChannel/bilcInsSmt5p5Grid}{\figWidtha}};
  \draw(0,1) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/halfDiskG4Scf1vs1ut2p0}{\figWidth}};

%
% grid:
%  \draw[step=1cm,gray] (0,.5) grid (16,6);
\end{tikzpicture}
}% END resize box
\end{center}
\caption{Incompressible flow past an elastic half disk. SCF=1, $t=2$. Note disk is thinner on the front side.
 }
  \label{fig:halfDiskScf1}
\end{figure}
}


==> texFiles/interfaceConditions.tex <==
\section{Notes on simplified interface conditions}
\wdh{

Now that we have a scheme that works, 
I wonder if we can simplify the implementation of the interface
conditions for velocity for the AMP scheme. One goal is to keep the velocity
components from all being coupled on curvilinear grids. Also simpler is generally
better if it works. 

% ---------------------------------------------------------------------
\subsection{Test Case: Decoupling the free surface conditions}

The free-surface boundary conditions for the velocity are 
\begin{align} 
 & \grad\cdot\vv= 0 , \\
 & \tv_m^T \tauv\nv = 0 
\end{align}
On a Cartesian grid with $\vv=(u,v)$ and with boundary $x=0$ these reduce to
\begin{align} 
 &  \pr_x u = - \pr_y v  ,  \label{eq:freeSurfaceDiv} \\
 &  \mu \pr_x v = 0      \label{eq:freeSurfaceTangentialStress}
\end{align}
The boundary conditions couple $v_1$ and $v_2$.

{\red
\noindent Further note:
On a Cartesian grid with boundary $x=0$ we also have $\pr_x(\grad\cdot\vv)=0$, 
\begin{align} 
 &  \partial_x^2 u = - \partial_y\pr_x v = 0  ,  
\end{align}
and thus we have decoupled BCs
\begin{align} 
 &  \pr_x^2 u = 0 ,  \label{eq:freeSurfaceDivX} \\
 &  \mu \pr_x v = 0      \label{eq:freeSurfaceTangentialStressB}
\end{align}
A similiar trick may help on curvilinear grids...
}


\noindent{\bf Question:} For implicit time-stepping can we approximately decouple the equations
in the predictor corrector scheme by
first solving for $v_1^{n+1}$ using a guess for $v_2$ in~\eqref{eq:freeSurfaceDiv}
and then solve for $v_2^{n+1}$  using \eqref{eq:freeSurfaceTangentialStress}. 
(Obviously in this case we could solve for $v_2$ first and then solve for $v_1$ but let's ignore this since
it won't be so simply in general). 
\noindent Stage 1: 
\begin{align} 
 & ( I - \half\nu\dt\Delta) v_1^{n+1} = ... \\ 
  &  \partial_x v_1^{n+1} = - \partial_y v_2^{(p)}    \\
  & v_y^{(p)} = \text{Extrapolated value in time or current best guess} 
\end{align}
\noindent Stage 2: 
\begin{align} 
 & ( I - \half\nu\dt\Delta) v_2^{n+1} = ... \\ 
 &  \mu \partial_x v_2 = 0 
\end{align}

More generally the boundary conditions~\eqref{eq:freeSurfaceDiv}-\eqref{eq:freeSurfaceTangentialStress}
at $r=0$ on a curved grid look something like
\begin{align} 
 &  \av_1^T \partial_r \vv + \av_2^T \partial_s \vv =0 ,  \label{eq:freeSurfaceDivCurved} \\
 &  \bv_1^T\partial_r \vv + \bv_2^T \partial_s \vv  = 0      \label{eq:freeSurfaceTangentialStressCurved}
\end{align}
where after scaling we have $\av_1 \approx \nv$ and $\bv_1\approx \tv_m$. 
To approximately de-couple the Cartesian components of these equations
we could solve~\eqref{eq:freeSurfaceDivCurved}-\eqref{eq:freeSurfaceTangentialStressCurved}
for $\partial_rv_1$ and $\partial_rv_2$:
\begin{align} 
 &  \partial_r v_1 + c_{11} \partial_s v_1 = c_{12} \partial_s v_2, \\
 &  \partial_r v_2 + c_{22} \partial_s v_2 = c_{21} \partial_s v_1, 
\end{align}
Now when we solve for $v_1^{n+1}$  we use a guess for $\partial_s v_2$ and vice versa.
{\bf The question then is whether this is stable and accuarte ?} 

{\bf Can we cook up a 2D matlab code to test this out?}}

\das{
\noindent{\bf Current notes:}
I am algebraically decoupling each condition one at a time to minimize bugs.
First, look at the tangential traction condition:
\begin{align}
\tv^T \tauv \nv = g
\end{align}
%
The Cartesian components of the tangential stress are
\begin{align}
\tau_{11} = 2 \mu \partial_x v_{1}, 
\quad \tau_{12} = \mu (\partial_y v_{1} + \partial_x v_{2}),
\quad \tau_{22} = 2 \mu \partial_y v_{2}.
\end{align}
%
The tangential condition expanded is equivalent to
\begin{align}
\mu \left( t_1 (\tau_{11} n_1 + \tau_{12} n_2) + t_2 (\tau_{12} n_1 + \tau_{22} n_2) \right)&= g  \\
\mu\left( 2 t_1 n_1 \partial_x v_{1}
+ (t_1 n_2 + t_2 n_1) \partial_y v_{1}
+ (t_1 n_2 + t_2 n_1) \partial_x v_{2}
+ 2 t_2 n_2 \partial_y v_2\right) &= g \\
\mu \left((2 t_1 n_1 - 2 t_2 n_2) \partial_x v_{1}
+ (t_1 n_2 + t_2 n_1) \partial_y v_{1}
+ (t_1 n_2 + t_2 n_1) \partial_x v_{2}\right)
 &= g. 
\end{align}
%
Here, we used $\grad \cdot \vv = 0$ to eliminate $\partial_y v_2.$
In code the condition applied is
\begin{align}
\mu \left((2 t_1 n_1 - 2 t_2 n_2) \partial_x v_{1}
+ (t_1 n_2 + t_2 n_1) \partial_y v_{1}
+ (t_1 n_2 + t_2 n_1) \partial_x v_{2}^{(p)}\right)
 &= g.
\end{align}
%
where $v_2^{(p)}$ is extrapolated in time for the predictor stage. For the corrector stage,
the predicted velocity is used. This works so far. TODO: divergence BC

}

\wdh{
% ---------------------------------------------------------------------
\subsection{Decoupling the AMP velocity conditions}


{\bf IGNORE THIS PART FOR NOW}

Refer to velocity boundary conditions
in equations~\eqref{eq:AMPTangentialCharacteristicDiscrete}-\eqref{eq:AMPVfDefinition}

\bigskip
\noindent{\bf Proposed approach: *finish me*}

\medskip
\noindent{\bf Stage 1:} Update solid. 

\noindent{\bf Stage 3} Solve for the predicted velocity
\begin{align}
\frac{\vv_\iv^{(p)} - \vv_\iv^n}{\dt} = \frac{3}{2} \Lv_E^n - \frac{1}{2} \Lv_E^{n-1}
+ \frac{1}{2}  \Lv_I^{(p)} + \frac{1}{2} \Lv_I^{n},
\quad    \iv \in \OmegaFh
\label{eq:VelocityPredictorUpdateA}
\end{align}

\noindent{\bf Stage 3a : for explicit time-stepping} we can advance the solution in the interior and on the boundary.
The boundary conditions are then applied:
(notation needs to be fixed but hopefully idea is clear): 
\bse \label{AMP-BCs}
\begin{align} 
 & \nv^T\vv_\iv^{(p)} = \nv^T(\text{impedance average of current fluid and solid velocities}) , \\
 & \grad\cdot\vv_\iv^{(p)} = 0 , \\
 & \tv_m^T \tauv\nv_\iv^{(p)} - \zs \tv_m^T\vv_{\jv}^{(E)} = \tv_m^T\sigmavs\nv , \\
 & \vv_{\iv-1}^{(E)} = 3 \vv_{\iv}^{(p)} - 3 \vv_{\iv+1}^{(p)} + \vv_{iv_+2}^{(p)} , \qquad \text{Extrapolated value.} 
\end{align}
\ese
Here, instead of using the equation on the boundary it may be simpler to just use an extrapolation
condition which gets turned on as $\zs\rightarrow\infty$. 

\noindent{\bf Stage 3b : for implicit time-stepping} we need boundary conditions to solve~\eqref{eq:VelocityPredictorUpdateA}.
Possible options:
\begin{enumerate}
\item Get a predicted value for the interface velocity $\vv_\iv^{I}$ using an impedance average of the
  current best guesses for fluid and solid velocities,
  \begin{align}
      \vv_\iv^{(p)} = \text{Impedance average of best guesses for $\vv_\iv^{n+1}$, $\vvs_\iv^{n+1}$} , \quad \iv\in\Gamma_h
  \end{align}
  This should be Ok for heavy solids. 
% 
\item 
\end{enumerate}
After advancing the interior points then update the ghost using equations~\eqref{AMP-BCs}. 

% 
% using the current guess for the solid velocity at time $t^{n+1}$, 
% \begin{align}
%      \vv_\iv^{(p)} & = \vvs_\iv^{(p)} = \text{ time extrapolated solid velocity}, \quad \iv\in\Gamma_h. 
% \end{align}
% % 
% Now assign ghost point values using (notation needs to be fixed but hopefully idea is clear): 
% \begin{align}
%  & \grad\cdot\vv_\iv^{(p)} = 0 , \\
%  & \tv_m^T \tauv\nv - \zs \tv_m^T\vv_{\jv}^{(E)} = \tv_m^T\sigmavs\nv , \\
%  & \vv_\jv^{(E)} = 3 \vv_{\iv}^{(p)} - 3 \vv_{\iv+1}^{(p)} + \vv_{iv_2}^{(p)} , \qquad \text{Extrapolated value.} 
% \end{align}
% 
% For a heavy solid, $\zs\rightarrow \infinity$ this reduces to the TP scheme. For a light
% solid, $\zs\rightarrow 0$ this goes to the ATP scheme. (*check me*)


}% end wdh


==> texFiles/intro-orig.tex <==
\section{Introduction} \label{sec:intro}


Fluid-structure interaction (FSI) problems involving incompressible fluids and
elastic bulk solids occur in many areas of engineering and applied
science. 
Examples include modeling flow-induced 
vibrations of structures (i.e.~aircraft wings, undersea cables, wind turbines, and bridges)
and simulating blood flow in arteries and veins.
% wave energy devices, parachutes and airbags, acoustic lenses, thermal expansion in nuclear 
% reactor cores and shock-structure interactions (blast effects), to name just a few.  
These problems are typically modeled using partial differential equations for both the 
fluid and solid in their respective domains combined with coupling conditions
at the fluid-solid interface.
Numerical algorithms used to solve these FSI
problems can be classified as
monolithic, i.e.~schemes that evolve the fluid and solid equations as a
single large system of coupled equations, or partitioned, i.e.~schemes that use separate fluid and solid
solvers together with some approach to couple the solutions at each time step.
Partitioned schemes are often preferred for modularity and computational performance, but
they may suffer from added-mass or other instabilities associated with the method used to couple
the solution at the interface.
Added-mass refers to the surrounding fluid mass that is displaced when a structure deforms.
Added-mass effects are significant when the structure is light compared to surrounding fluid.
In these difficult cases, sub-iterations of a partitioned algorithm
are often performed at each time step to recover stability but at increased cost.

The FSI regime which we consider in this paper concerns the interactions between 
viscous incompressible fluids and bulk elastic solids. 
This is a difficult regime for partitioned schemes since added-mass effects may be 
large even for relatively \textit{heavy} solids, due to the
infinite speed of propagation in the incompressible flow.  
This effect has been studied in previous work~\cite{fib2014} where the 
the traditional partitioned algorithm, 
which uses the solid velocity as a boundary condition for the
fluid and the fluid traction as a boundary condition for the solid, was found to 
be unconditionally unstable if the solid grid is sufficiently fine.

Previous research has shown that the number of necessary sub-iterations can be greatly 
reduced by using Aitken acceleration or quasi-Newton methods, see \cite{Küttler2008,MEHL2016869}.
Sub-iterations can additionally be reduced by using 
Robin-Neumann or Robin-Robin coupling instead of Dirichlet-Neumann coupling 
\cite{Wang2018,BASTING2017312,BadiaNobileVergara2008,MokWallRamm2001,FernandezMullaertVidrascu2014,FernandezMullaertVidrascu2013,FernandezLandajuela2014,Gerardo_GiordaNobileVergara2010,BadiaNobileVergara2009,NobilePozzoliVergara2014}.
% loosely coupled partitioned scheme \cite{BukacCanicMuha2015,doi:10.1002/cnm.2813,LukacovaMedvidovaRusnakovaHundertmarkZauskova2013,GuidoboniGlowinskiCavalliniCanic2009,BukacCanicGlowinskiTambacaQuaini2013}
% combined field with explicit interface \cite{LiuJaimanGurugubelli2014}
%differences of added mass for incompressible and compressible, loosely coupled \cite{vanBrummelen2009}
Added-mass effects can also be treated by adding fictitious mass 
terms in the structure equations~\cite{BaekKarniadakis2012,YuBaekKarniadakis2013} or 
artificial compressibility in the fluid equations~\cite{RabackRuokolainenLyly2001,DegrooteSwillensBruggemanHaeltermanSegersVierendeels2010,Degroote2011}.
For difficult problems with large added-mass effects, monolithic schemes can be used to 
eliminate the need for sub-iterations~\cite{Forti2017,FigueroaVignonClementelJansenHughesTaylor2006}.
The performance of monolithic schemes can be greatly improved through the application of multigrid~\cite{AULISA2018213,Heil2004,GeeKuttlerWall2011,HronTurekMonolithic2006}.
%Immersed boundary type schemes \cite{KIM2018296,TIAN2014451,LEE2015529,LakshminarayanFarhatMain2014,WangGretarssonMainFarhat2012,BorazjaniGeSotiropolous2008}

There has been a significant amount of research into developing stable and 
at least second-order accurate non-iterative partitioned schemes for various other FSI regimes.
% Some works include \cite{fib2014,flunsi2016,beamins2016,lrb2013}.
% The current work builds upon our previous work in other FSI regimes, which we mention here as these
% works provide useful insight into the current algorithm.
In previous work~\cite{fsi2012}, a stable partitioned algorithm for compressible flows and
compressible elastic solids was developed that overcomes the added-mass effect and uses deforming
composite grids to treat large solid motions.  FSI problems involving compressible flows are
somewhat easier to deal with than incompressible flows since the added-mass effects are localized
due to the finite speeds of wave propagation in the fluid~\cite{vanBrummelen2009}.  The scheme
in~\cite{fsi2012}, which is based on the analysis in~\cite{BanksSjogreen2011}, uses a local
characteristic analysis of a fluid-structure Riemann problem to define an impedance weighted
averaging of the fluid and solid interface values (i.e.~a Robin-Robin coupling).  
This algorithm was
extended to the case of rigid bodies in~\cite{lrb2013} where it was shown that the scheme remains
stable even for rigid bodies of zero mass.
Partitioned algorithms were also developed for 
incompressible flows and deforming beams in~\cite{beamins2016}.

To our knowledge the first stable and second-order accurate partitioned scheme
for incompressible fluids and elastic solids
was the added-mass partitioned (AMP) scheme 
described our recent work~\cite{fib2014}, where the algorithm was studied for a 
two-dimensional model problem involving infinitesimal disturbances.
Although seemingly simple, this model problem describes the most
important features of the full problem with respect to added-mass instabilities.
The current article extends this previous AMP algorithm to
practical problems in two dimensions involving finite solid deformations 
(although the solid model is restricted here to linear elasticity). 
Unlike in the previous work~\cite{fib2014}, the new algorithm
uses an implicit-explicit (IMEX) fractional-step scheme based on~\cite{splitStep2003}.
In this scheme, the fluid velocity is first advanced, treating the viscous terms implicitly,
and the pressure is updated by solving a Poisson equation.
This new time-stepping approach has necessitated important modifications 
to the original AMP scheme~\cite{fib2014} which are critical to its success. 
The key new elements involve changes to
the fluid-velocity interface conditions and changes to the updates of the solid interface values.
The interface conditions are written in terms of impedance-weighted average of the interface
velocities or inverse impedance weighted averages of the tractions.  Although the solid impedances
$\zp=\rhos\cp$ and $\zs=\rhos\cs$ are well defined as a product of the solid density $\rhos$ 
with the primary and secondary wave speeds, $\cp$ and $\cs$, the choice of fluid 
impedance $z_f$ is less clear but critical to
the stability of the algorithm. A model problem analysis of the monolithic scheme, 
described in the companion paper~\cite{fibrmp2019}, leads to the appropriate form of $z_f$. 
The expression for $z_f$ only
depends on known material and discretization parameters and is thus well defined for any problem,
with no undetermined parameters.
The stability analysis of the AMP scheme is extended from inviscid fluids in~\cite{fib2014}
to viscous fluids in~\cite{fibrmp2019}. The analysis in the latter is complicated by the
introduction of a viscous CFL number, $\Lambda = \nu \dt / h^2$, as a dimensionless parameter
in addition to the mass ratio of the fluid and solid. 
Despite the added complication, the AMP scheme was shown to be stable for all possible mass ratios
and viscous CFL numbers when applied to a simplified model problem.

Our numerical approach for resolving complex geometries and handling the evolving fluid domain
is based on the use of deforming composite grids (DCG).
The DCG approach was described for the case of inviscid compressible flow coupled with 
linearly elastic solids in \cite{fsi2012} and later for 
compressible flow coupled with nonlinear hyperelastic solids in \cite{flunsi2016}.
Figure \ref{fig:rpiFig} shows a composite grid for the fluid channel domain and 
solid domains (the letters `R', `P', and `I'). The solid undergoes a deformation which causes
the fluid interface-fitted grids to adapt.

\input texFiles/rpiFig

The remainder of the manuscript is organized as follows. 
In Section~\ref{sec:governingEquations} we
define the governing equations and coupling conditions.
In Section~\ref{sec:algorithm}, there is a detailed discussion of the AMP, 
traditional partitioned (TP) and anti-traditional partitioned (ATP) schemes.
In Section~\ref{sec:numericalApproach}, we describe how approximations to spacial derivatives
are handled using deforming composite grids (DCG).
Section~\ref{sec:numericalResults} provides
numerical results confirming the stability and accuracy of the scheme.  
Conclusions are given in Section~\ref{sec:conclusions}.  




%- \bigskip
%- \wdh{From FIB:}
%- 
%- The coupled evolution of fluids and structures is of great interest in a wide range of applications
%- including, for example, structural engineering and biomedicine.  Such fluid-structure interaction
%- (FSI) problems are often modeled mathematically by suitable partial differential equations for the
%- fluids and structures in their respective domains, together with conditions at the boundaries of the
%- domains where the solutions of the equations interact.  Numerical algorithms used to solve these FSI
%- problems can be classified into two main categories.  Algorithms belonging to one category, called
%- monolithic schemes, treat the equations for the domains of the fluids and structures along with
%- interface conditions as a large system of evolution equations, and then advance the solutions
%- together.  The other category of algorithms are partitioned schemes (also known as modular or
%- sequential schemes), and these algorithms employ separate solvers for the fluids and structures
%- which are coupled at the interface.  Partitioned schemes are often preferred for modularity and
%- computaional performance but they may suffer from instabilities due to the choice of interface couplings.
%- In these difficult cases, sub-iterations are often performed at each time step of a
%- partitioned algorithm to recover stability but at increased cost.
%- 
%- Strongly-coupled partitioned schemes perform multiple
%- iterations per time step to solve the coupled equations, while loosely coupled schemes use only one
%- or a few iterations.  Even though many existing partitioned schemes suffer from serious stability
%- issues in certain problem regimes, they are often preferred since they can make use of existing
%- solvers and can be more efficient than monolithic schemes.
%- 
%- 
%- 
%- In this paper we consider an important class of FSI problems where partitioned schemes often have
%- difficulty.  This class involves the coupling of incompressible fluids and relatively {\em light}
%- structures where {\em added-mass} effects are large.  Added-mass effects arise from the fact that
%- the force required to accelerate a solid structure immersed in a fluid must also account for the
%- acceleration of the surrounding fluid.  Partitioned schemes for this class of problem generally
%- suffer from poor convergence, requiring many sub-iterations per time step, or are unstable, when
%- added-mass effects are large.  The instabilities in partitioned schemes can be traced to the
%- application of the interface conditions which must also be partitioned between the fluid and solid
%- solvers.  The traditional partitioned algorithm uses the velocity of the solid as a boundary
%- condition on the fluid and the traction from the fluid as a forcing on the solid.  This is sometimes
%- referred to as Dirichlet-Neumann coupling with the Dirichlet condition being the assignment of the
%- velocity and the Neumann condition the assignment of the traction.  More generally, practitioners
%- have considered Robin-Robin coupling (i.e.~{\em mixed} boundary conditions for the fluid and solid)
%- to impose the interface conditions~\cite{BadiaNobileVergara2008}.
%- 
%- The central aim of the present work is to describe an added-mass partitioned (AMP) algorithm for FSI
%- problems involving an incompressible fluid coupled to an elastic structure.  A key feature of our
%- new AMP algorithm is that it is stable, even when added-mass effects are large, and it retains full
%- accuracy with no sub-iterations.  We discuss the algorithm and analyze its stability for two types
%- of structures.  In Part I of this paper, we describe the algorithm for FSI problems involving
%- compressible bulk solids, while in Part II, we consider problems involving elastic shells.  A common
%- feature of the algorithms for both types of structures is the derivation of an AMP Robin interface
%- condition for the fluid involving the velocity or acceleration of the interface and the stress on
%- it.  The version of the Robin interface condition involving the velocity, which applies for the bulk
%- solid case only, may be used as a boundary condition for the partitioned solver for the fluid in
%- velocity-divergence form.  The version of the interface condition involving the acceleration applies
%- for both cases, and can be used for the fluid solver in velocity-pressure form.  In the latter case,
%- a further manipulation of the Robin condition is carried out so that it provides a suitable boundary
%- condition for the pressure in a fractional-step fluid solver.  The details of the derivation of the
%- AMP Robin condition depends on the type of structure, whether it be an elastic solid or an elastic
%- shell, and this is principally where the discussion of the algorithms in the two parts of the paper,
%- and the corresponding stability analyses and results, differ.  For the case of a compressible bulk
%- solid, the AMP interface condition is obtained based on characteristic equations for the solid
%- applied at the interface, while for the case of the elastic shell, the interface condition is
%- obtained from the evolution equation for the shell itself.  This latter case is described in detail
%- in Part II of the paper~\cite{fis2014}.
%- 
%- 
%- In previous work~\cite{fsi2012}, a stable partitioned algorithm for {\em compressible} flows and
%- compressible elastic solids was developed that overcomes the added-mass effect and uses deforming
%- composite grids to treat large solid motions.  FSI problems involving compressible flows are
%- somewhat easier to deal with than incompressible flows since the added-mass effects are localized
%- due to the finite speeds of wave propagation in the fluid~\cite{vanBrummelen2009}.  The scheme
%- in~\cite{fsi2012}, which is based on the analysis in~\cite{BanksSjogreen2011}, uses a local
%- characteristic analysis of a fluid-structure Riemann problem to define an impedance weighted
%- averaging of the fluid and solid interface values (i.e.~a Robin-Robin coupling).  This algorithm was
%- extended to the case of rigid bodies in~\cite{lrb2013} where it was shown that the scheme remains
%- stable even for rigid bodies of zero mass.
%- 
%- The development and study of numerical algorithms for FSI problems is an active area of research, see for example, the papers~\cite{Farhat2006,SchaferHeckYigit2006,HronTurekMonolithic2006,TezduyarSathe2007,BorazjaniGeSotiropolous2008,DegrooteVierendeels2011,GretarssonKwatraFedkiw2011,HouWangLayton2012} and the references cited therein.
%- %, see for example~\cite{DoneaGiulianiHalleux1982,CebralLohner1997,Lohner99,LeTallecMouro2001,PipernoFarhat2001,SchaferTeschauer2001,GlowinskiPanHelsaJosephPeriaux2001,Guruswamy2002,MillerColella2002,KuhlHulshoffBorst2003,ArientiHungMoranoShepherd2003,Farhat2006,HronTurekMonolithic2006,Tezduyar2006,SchaferHeckYigit2006,AhnKallinderis2006,CirakDeiterdingMauch2007,vanLoon2007,TezduyarSathe2007,BorazjaniGeSotiropolous2008,Wilcox2010,BartonObadiaDrikakis2011,DegrooteVierendeels2011,TezduyarTakizawaBrummerChen2011,CrosettoDeparisFouresteyQuarteroni2011,Degroote2011,GretarssonKwatraFedkiw2011,HouWangLayton2012}.
%- In particular, there has been much work concerning partitioned algorithms and the added-mass effect.  For the case of incompressible fluids coupled to thin structural shells, there has been some success in treating the added-mass instability.  The kinematically-coupled scheme of Guidoboni et~al.~\cite{GuidoboniGlowinskiCavalliniCanic2009}, later extended to the $\beta$-scheme by \v{C}ani\'c, Muha and Buka\v{c}~\cite{CanicMuhaBukac2012}, is a stable partitioned scheme that uses operator splitting.  Nobile and Vergara~\cite{NobileVergara2008}, among others, have developed stable semi-monolithic schemes for the case of thin shells.  Even fully monolithic schemes for thin-shells~\cite{FigueroaVignonClementelJansenHughesTaylor2006} are not overly expensive since the number of degrees of freedom for the structural shell is usually small compared to those in the fluid.  For bulk solids, however, apparently all previous partitioned approaches for coupling incompressible flows and light solids are either unstable or require multiple sub-iterations per time step to converge (tens or hundreds of iterations are typical) with the number of iterations generally increasing as the solid gets lighter.  Indeed, it is common to resort to fully monolithic schemes~\cite{BatheZhang2004,Heil2004,HronTurekMonolithic2006,GeeKuttlerWall2011} or semi-monolithic schemes~\cite{FernandezGerbeauGrandmont2007,AstorinoChoulyFernandez2009,GretarssonKwatraFedkiw2011}.
%- 
%- A number of authors have analyzed the added-mass effect and the stability of FSI
%- algorithms~\cite{Conca1997,LeTallecMani2000,MokWallRamm2001,ForsterWallRamm2007,AstorinoChoulyFernandez2009,vanBrummelen2009,Gerardo_GiordaNobileVergara2010}.
%- Causin, Gerbeau and Nobile~\cite{CausinGerbeauNobile2005}, for example, analyze a model problem of a
%- structural shell coupled to an incompressible fluid and show that the traditional scheme can be
%- unconditionally unstable over a certain range of parameters.  There are numerous approaches that
%- have been developed to reduce the number of iterations required per time step in partitioned
%- schemes~\cite{MokWallRamm2001}.  Robin-Robin interface conditions are used to stabilize partitioned
%- schemes by, for example, Nobile, Vergara and
%- co-workers~\cite{NobileVergara2008,BadiaNobileVergara2008,BadiaNobileVergara2009,Gerardo_GiordaNobileVergara2010,NobileVergara2012}
%- and Astorino, Chouly and Fernandez~\cite{AstorinoChoulyFernandez2009}.  Yu, Baek and
%- Karniadakis~\cite{YuBaekKarniadakis2013} and Baek and Karniadakis~\cite{BaekKarniadakis2012} have
%- developed fictitious-pressure and fictitious-mass algorithms which incorporate additional terms into
%- the governing equations to account for added-mass effects.  The optimal values for parameters are
%- estimated from analysis and computation, and the number of sub-iterations required using Aitken
%- acceleration (tens of iterations) is similar to optimal Robin-Robin approaches.  To stabilize the
%- FSI algorithm and reduce the number of sub-iterations, Riemslagh, Virendeels and
%- Dick~\cite{RiemslaghVierendeelsDick2000}, Degroote
%- et~al.~\cite{DegrooteSwillensBruggemanHaeltermanSegersVierendeels2010}, and Raback, Ruokolainen, and
%- Lyly~\cite{RabackRuokolainenLyly2001} have developed an interface artificial compressibility method
%- that adds a source term to the fluid continuity equation near the interface; the effect of the
%- source term goes away as the sub-iterations converge.  Idelsohn
%- et~al.~\cite{IdelsohnDelPinRossiOnate2012} and Badia, Quaini and
%- Quarteroni~\cite{BadiaQuainiQuarteroni2008} form approximate factorizations of the fully monolithic
%- scheme to construct partitioned schemes but these still may require many iterations to converge.
%- Degroote et~al.~\cite{DegrooteBruggemanHaeltermanVierendeels2008,DegrooteBatheVierendeels2009} use
%- reduced-order models and Aitken acceleration methods to decrease the number of iterations in
%- partitioned schemes.
%- 
%- The remainder of the manuscript is organized as follows. In Section~\ref{sec:governingEquations} we
%- define the governing equations and present the essential form of the AMP interface conditions.  In
%- Section~\ref{sec:partitionedAlgorithms} there is a discussion of partitioned algorithms and how the
%- AMP interface conditions are incorporated into the fluid and solid solution schemes.  Three model
%- problems are defined in Section~\ref{sec:modelProblems} and these are used later for the analysis
%- and numerical results.  In Section~\ref{sec:AMP1D} the form of the AMP algorithm for a
%- one-dimensional model problem is discussed.  A normal mode stability analysis of the AMP scheme as
%- well as the traditional (Dirichlet-Neumann) and anti-traditional (Neumann-Dirichlet) schemes are
%- presented in Section~\ref{sec:analysis}.  The FSI time-stepping algorithm for the AMP scheme is
%- outlined in Section~\ref{sec:timeSteppingAlgorithm}.  Section~\ref{sec:numericalResults} provides
%- numerical results confirming the stability and accuracy of the scheme.  Conclusions are given in
%- Section~\ref{sec:conclusions}.  A summary comparison of the algorithm discussed here for bulk
%-   solids with the one for structural shells is provided at the end of Part II of this
%-   paper~\cite{fis2014}.




==> texFiles/multipleBodies_backup.tex <==
% \subsection{RPI solid} 

% {
% \newcommand{\figWidth}{4cm}% height 
% \newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.1}{.1}{.3}{.3}}
% \begin{figure}[htb]
% \begin{center}
% \begin{tikzpicture}[scale=1]
%   \useasboundingbox (0,.5) rectangle (16,5.25);  % set the bounding box (so we have less surrounding white space)

%    \draw(0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=0pt] {\trimfig{fig/rpiGrid}{\figWidth}};
%    \draw(8.0,0.0) node[anchor=south west,xshift=-15pt,yshift=0pt] {\trimfig{fig/rpiSolution}{\figWidth}};
% % grid:
% % \draw[step=1cm,gray] (0,0) grid (14,5);
% \end{tikzpicture}
% \end{center}
%   \caption{$\delta_R = 1000, \delta_P = 10, \delta_I = 100.$ $tf=40.$}
% \end{figure}
% }

\subsection{Multiple solid domains in a flow} \label{sec:multipleBodies}

To test the robustness of the AMP algorithm we consider a final example
of incompressible fluid flow past four embedded solids with different shapes and densities.
Each solid body has a fixed interior core.
\das{Update this section once we decide on a final configuration.}
The fluid channel occupies the region $[0,10] \times [-2,2].$
There are two rectangular solid beams with length $L_b = 2.5$ and thickness $T_b = .45.$
They are both rotated by an clockwise angle of $\theta_b = 10^{\circ}$ about the center of the 
beam, which is chosen to be 
$(x_{b,u},y_{b,u}) = (2.5,.75)$ for the upper beam and $(x_{b,l},y_{b,l}) = (2.5,-.75)$ for the 
lower beam. For the upper beam, the core center coincides with the center of the beam.
For the lower beam, the core center is located at a length 
of $s_{b,l} = .15 L_b$ away from the leading edge on the beam center-line.
The radius of both the cores are $R_b = .1.$
A solid cross centered at $(x_c,y_c) = (5.5,0)$ has length $L_c = 3$ and thickness $T_c = .45.$
Its core is located at the center with radius $R_c=.1$.
A square centered at $(x_s,y_s) = (8,0)$ has length $L_c = 1.$ 
A core is located at the center with radius $R_c=.2.$
The corners of the rectangular shapes are rounded to ensure the mapping is smooth.

The fluid density is $\rho=1$ and the viscosity is $\mu=0.05.$
For each solid domain, we choose the solid parameters to be 
$\rhos_i=\lambdas_i=\mus_i=\delta_i,$ where $i$ is the domain label.
We choose $\delta_{b,u} = 10^2$ for the upper beam,
$\delta_{b,l} = 10$ for the lower beam,
$\delta_{c} = 10^3$ for the cross,
and $\delta_s = 10$ for the square.
The fluid boundary conditions are the same as in section~\ref{sec:elasticDiskInAChannel}.
At the inlet, the pressure is ramped smoothly from $p=0$ at $t=0$
to $p=p_0$ at $t=1$ using equation \eqref{eq:ramp}. For this computation, we choose $p_0=10$.

\newcommand{\Gmb}{\mathcal{G}_{\rm mb}}
Let $\Gmb^{(j)}$ be the composite grid with target grid spacing $\Delta s = 1 / (10 j).$
The grid is shown in figure~\ref{fig:multipleSolidsGrid}.
The fluid domain is composed of a (blue) background grid and (green) deforming 
interface-fitted grids.
Each solid domain is composed of (red) background grids, (orange) interface-fitted 
grids, and (purple) annular grids around the interior core.

{
\newcommand{\figWidth}{4cm}% height 
\newcommand{\trimfiga}[2]{\trimwb{#1}{#2}{.0}{.0}{.1}{.1}}
\newcommand{\trimfigb}[2]{\trimwb{#1}{#2}{.0}{.0}{.0}{.0}}
\newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.1}{.1}{.3}{.3}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,.5) rectangle (16,11);  % set the bounding box (so we have less surrounding white space)

   \draw(0.0,4.0) node[anchor=south west,xshift=-15pt,yshift=0pt] {\trimfiga{fig/solidObjectsGride4}{8cm}};
   \draw(9.5,4.5) node[anchor=south west,xshift=-15pt,yshift=0pt] {\trimfigb{fig/solidObjectsGride4Zoom}{6cm}};

   \draw(0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=0pt] {\trimfig{fig/fiveBodiesG4StreamLinesAndDisplacement2p0}{\figWidth}};
   \draw(8.0,0.0) node[anchor=south west,xshift=-15pt,yshift=0pt] {\trimfig{fig/fiveBodiesG4StreamLinesAndDisplacement5p0}{\figWidth}};
% grid:
% \draw[step=1cm,gray] (0,0) grid (14,9);
\end{tikzpicture}
\end{center}
  \caption{Possible new configuration...}
\end{figure}
}


\input texFiles/multipleSolidsGrid

A self-convergence study was (\das{will be}) performed to verify that the solution is converging
at second order accuracy. 
The solution is computed on three composite grids of increasing resolution. 
As in the previous section, errors and convergence rates are estimated using a Richardson
extrapolation procedure. Max-norm errors and convergence rates at time $t=1$ are tabulated
in table \ref{tab:multipleSolidsConv}. The solution is converging at close to second order
accuracy.

{
\begin{table}[h]
\centering
\begin{tabular}{c}
placeholder...
\end{tabular}
\caption{placeholder for convergence results.
\label{tab:multipleSolidsConv}}
\end{table}
}

Figure~\ref{fig:multipleSolidsGrid} shows a plot of streamlines in the fluid domain
and shaded contours of the magnitude of displacement in each solid domain.
Figure~\ref{fig:multipleSolidsTime} shows how the shape of the solid interfaces
deform over time. 
Since the lower beam is light ($\delta=10$), it undergoes a noticeable compression due to the
interface pressure. 
Although the upper beam is heavier ($\delta=10^2$) than the lower beam, it experiences larger
displacements.
This is due to the placement of the core. 
The aerodynamic center of the beam is upstream of the core, which causes the beam to increase 
in angle of attack under a lifting force. 
When the angle of attack is increased, the lift force also increases causing a larger deformation.
The opposite (stabilizing) effect occurs in the lower beam.
The solid cross ($\delta=10^3$) undergoes asymmetric vibrations.
The solid square ($\delta=5$) is in the wake of the solid cross and therefore
does not undergo large deformations.



{
\begin{figure}[h]
\centering
\includegraphics[width=.75\textwidth]{fig/fourDisksInterfaceTimePlot}
\caption{
  Position of the interface over time for the four objects in a channel
  computed on grid $\Gmb^{(2)}.$ The displacements for the solid cross 
  ($\delta=10^3$) are magnified by 2 and the displacements for the 
  solid square ($\delta=5$) are magnified by 10.
  \das{When we have convergence results, I may put the table in this figure to save room.}
\label{fig:multipleSolidsTime}}
\end{figure}
}















% {\begin{figure}[h]
% \centering
% \includegraphics[width=.49\textwidth]{fig/fourObjectsNewExampleGrid}
% \includegraphics[width=.49\textwidth]{fig/fourObjectsNewExampleT60}
% \caption{$\delta=100$ for stick on top, $\delta=10$ for stick on bottom.
% $\delta=1000$ for star, $\delta=100$ for square.}
% \end{figure}}

% {\begin{figure}[h]
% \centering
% \includegraphics[width=.49\textwidth]{fig/fiveObjects}
% \includegraphics[width=.49\textwidth]{fig/fiveObjectsContour}
% \caption{$\delta=100$ for sticks on top. $\delta=10$ for sticks on bottom.
% $\delta=1$ for disk. ``What a code!''}
% \end{figure}}

% {\begin{figure}[h]
% \centering
% \includegraphics[width=.49\textwidth]{fig/fiveObjects}
% \includegraphics[width=.49\textwidth]{fig/fiveObjectsT10}
% \caption{$\delta=10$ for all bodies}
% \end{figure}}

% {\begin{figure}[h]
% \centering
% \includegraphics[width=.49\textwidth]{fig/threeSticksGrid}
% \includegraphics[width=.49\textwidth]{fig/threeSticks}
% \caption{$\delta=100$ for all bodies. }
% \end{figure}}


==> texFiles/multipleSolidsGrid.tex <==
{% ----------- ELASTIC ELLIPSE  ------  
% --------- START drawContour -----------
\newcommand{\drawContour}[9]{%
\begin{scope}[#1]
\draw(0.0,-\figHeightA) node[anchor=north west,xshift=-15pt,yshift=-6pt] {\trimfiga{fig/#2}{\figHeightA}};
  \draw(0.025,-9.1) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #4}; % streamlines
  \draw(6,-8.2) node[draw,fill=white,anchor=south west,xshift=2pt,yshift=1pt] {\scriptsize #3}; % ubar
  \draw(11.1,-4.9) node[draw,fill=white,anchor=north east,xshift=3pt,yshift=-1pt] {\scriptsize #5}; % time
\draw(3,-5.5) node[draw,fill=white,xshift=3pt,yshift=-1pt] {\scriptsize $\delta_{b,u}=10^2$};
\draw(3,-7.5) node[draw,fill=white,xshift=3pt,yshift=-1pt] {\scriptsize $\delta_{b,l}=10$};
\draw(6.4,-5.75) node[draw,fill=white,xshift=3pt,yshift=-1pt] {\scriptsize $\delta_c=10^3$};
\draw(9.8,-6) node[draw,fill=white,xshift=3pt,yshift=-1pt] {\scriptsize $\delta_s=5$};
 % colour bar:
\def\xcbShift{-.5}
\def\xcenter{13.5}
\def\xcbg{.5}
\begin{scope}[xshift=-3pt,yshift=-7pt]
  \draw (+\xcb,\ycb) node[anchor=south,xshift=0.25cm,yshift=.5cm,rotate=0] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
\end{scope}
\begin{scope}[xshift=5pt,yshift=-7pt]
  \draw (-.5*\xcbg+\xcbShift+\xcenter,-5) node[anchor=north,xshift=-6pt,yshift=+4pt] {\scriptsize 3.5};
  \draw (-.5*\xcbg+\xcbShift+\xcenter,-7) node[xshift=-6pt,yshift=+4pt,rotate=90] {\scriptsize fluid};
  \draw (-.5*\xcbg+\xcbShift+\xcenter,-9) node[anchor=south,xshift=-6pt,yshift=+4pt] {\scriptsize 0};

    \draw (.5*\xcbg+\xcbShift+\xcenter,-5) node[anchor=north,xshift=+4pt,yshift=+4pt] {\scriptsize .55};
    \draw (.5*\xcbg+\xcbShift+\xcenter,-7) node[xshift=+4pt,yshift=+4pt,rotate=90] {\scriptsize upper beam};
    \draw (.5*\xcbg+\xcbShift+\xcenter,-9) node[anchor=south,xshift=+4pt,yshift=+4pt] {\scriptsize 0};

    \draw (1.5*\xcbg+\xcbShift+\xcenter,-5) node[anchor=north,xshift=+4pt,yshift=+4pt] {\scriptsize .25};
    \draw (1.5*\xcbg+\xcbShift+\xcenter,-7) node[xshift=+4pt,yshift=+4pt,rotate=90] {\scriptsize lower beam};
    \draw (1.5*\xcbg+\xcbShift+\xcenter,-9) node[anchor=south,xshift=+4pt,yshift=+4pt] {\scriptsize 0};

    \draw (2.5*\xcbg+\xcbShift+\xcenter,-5) node[anchor=north,xshift=+4pt,yshift=+4pt] {\scriptsize .15};
    \draw (2.5*\xcbg+\xcbShift+\xcenter,-7) node[xshift=+4pt,yshift=+4pt,rotate=90] {\scriptsize cross};
    \draw (2.5*\xcbg+\xcbShift+\xcenter,-9) node[anchor=south,xshift=+4pt,yshift=+4pt] {\scriptsize 0};

    \draw (3.5*\xcbg+\xcbShift+\xcenter,-5) node[anchor=north,xshift=+4pt,yshift=+4pt] {\scriptsize .03};
    \draw (3.5*\xcbg+\xcbShift+\xcenter,-7) node[xshift=+4pt,yshift=+4pt,rotate=90] {\scriptsize square};
    \draw (3.5*\xcbg+\xcbShift+\xcenter,-9) node[anchor=south,xshift=+4pt,yshift=+4pt] {\scriptsize 0};

\end{scope}
\end{scope}
}
% --------- END drawContour -----------
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{4cm}% colour bar height
\newcommand{\xcb}{13cm}% colour bar lower left corner
\newcommand{\ycb}{-9.5cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*\real{.5}}% colour bar top label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
\newcommand{\figHeightA}{4.5cm}% height
\newcommand{\figHeightB}{4.45cm}% height
\newcommand{\trimfiga}[2]{\trimhb{#1}{#2}{.2}{.2}{.39}{.37}}
\newcommand{\trimfigb}[2]{\trimhb{#1}{#2}{.0}{.0}{.0}{.0}}
\def\gap{.2}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,-.25) rectangle (16,-9);  % set the bounding box (so we have less surrounding white space)

   \draw(0,0.0) node[anchor=north west,xshift=-15pt,yshift=-0pt] {\trimfiga{fig/multiObjectsGrid}{\figHeightA}};

% 
   %\draw(0,-\figHeightA) node[anchor=north west,xshift=-15pt,yshift=-6pt] {\trimfiga{fig/fourObjectsNewExampleT60}{\figHeightA}};
   
   \def\xo{5.4};
   \def\yo{-3.1};
   \draw[line width=1pt] (\xo,\yo) rectangle (\xo+1,\yo+1);
   \draw[line width=1pt,dashed] (\xo,\yo) -- (11.5,-\figHeightA-15*\gap);
   \draw[line width=1pt,dashed] (\xo,\yo+1) -- (11.5,-.75*\gap);
   \draw[line width=1pt,dashed] (\xo+1,\yo) -- (16,-\figHeightA-15*\gap);
   \draw[line width=1pt,dashed] (\xo+1,\yo+1) -- (16,0-.75*\gap);

   \draw(11.5,0.0) node[anchor=north west,xshift=-15pt,yshift=-0pt] {\trimfigb{fig/multiObjectsGridZoom}{\figHeightB}};

   \drawContour{xshift= 0.cm,yshift=0cm}{fourObjectsContour}{$|\usv|$}{streamlines}{$t=30$}{$-.015$}{$.017$}{$-.017$}{$.015$};


   
 % \draw[step=.5cm,gray] (0,0) grid (16,-10);
\end{tikzpicture}
\end{center}
  \caption{
Top left: plot of the composite grid $\Gmb^{(2)}$. The fluid domain is composed of a
blue background Cartesian grid and green deforming interface-fitted grids.
The solid domains are composed of red background Cartesian grids, orange interface-fitted
grids and purple annular core-fitted grids.
Top right: zoomed in view of the composite grid near the fluid-solid interface.
Bottom left: streamlines of the fluid velocity and shaded contours of the 
magnitude of the solid displacement are plotted at $t=30.$
Bottom right: colorbar for the plot. Note that each domain has different limits.
}
  \label{fig:multipleSolidsGrid}
\end{figure}
}


==> texFiles/numericalApproach-7-24-2018.tex <==
\section{Numerical approach using deforming composite grids (DCG)} \label{sec:numericalApproach}

We use deforming composite grids (DCG) to solve the FSI initial value problem.
This FSI-DCG approach was first described
in~\cite{fsi2012} for the case of an inviscid
compressible flow coupled to a linearly elastic solid, and later 
in~\cite{flunsi2014r} for the case of compressible flow coupled to nonlinear
hyperelastic solids.
Here we will extend this approach to incompressible flows and elastic solids.

\subsection{Deforming composite grids} \label{sec:overture}

Define an overlapping grid $\Gc$ with a set of component 
grids $\{G_g\}$ from $g = 1,\, \ldots,\, \Nc$, 
which cover both the fluid and solid domains and
overlap at intersections.
Static Cartesian background grids make up the majority of the domain
while boundary fitted grids are used to resolve complex geometry and moving interfaces.
On each component grid, the computational domain is mapped onto a unit square (or cube).
In the fluid, this mapping may also be time dependent to account for grid motion.
For a fluid grid, this mapping is given by
\begin{align}
\xv = \gv(\rv,t), \quad \rv \in [0,1]^{\nd}, \quad \xv \in \Real^{\nd},
\end{align}
%
where $\nd$ is the number of dimensions.
The equations for the solid are solved in the Lagrangian reference frame, which is independent 
of time. For a solid grid, the mapping is defined as
\begin{align}
\xsv = \bar{\gv}(\rv), \quad \rv \in [0,1]^{\nd}, \quad \xv \in \Real^{\nd}.
\end{align}
%
The solid deformation can be obtained through
\begin{align}
\xv(\xsv,t) = \xsv + \usv(\xsv,t).
\end{align}
%
\das{Show a cartoon.}
%
Fluid component grids next to the solid interface deform over time to match the 
solid deformation. See figure. 
A hyperbolic grid generator ~\cite{HyperbolicGuide} is used to regenerate the grids.
The {\tt Ogen} grid generator~\cite{OGEN} is then called to regenerate the overlapping
grid connectivity between the boundary fitted grids and the background fluid grids.

The incompressible Navier-Stokes equations are solved in velocity-pressure form 
on overlapping grids using a second order fractional-step algorithm
\cite{fis2014,splitStep2003,ICNS} similar to that described in 
section \ref{sec:algorithm}.
The momentum equation is given by
\begin{align}
\rho \frac{\partial v_i}{ \partial t}
+ \rho v_j \frac{\partial v_i}{\partial x_j} =
\frac{\partial \sigma_{ji}}{\partial x_j}, \quad i = 1,\ldots,\nd,
\end{align}
%
using summation convention. Under the coordinate transform
$\xv = \gv(\rv,t),$ the equations become
\begin{align}
\rho \frac{\partial v_i}{ \partial t}
+ \rho (v_j - \dot{x}_j)  \frac{\partial v_i}{\partial r_k} \frac{\partial r_k}{\partial x_j}=
\frac{\partial \sigma_{ji}}{\partial r_k} \frac{\partial r_k}{\partial x_j}, 
\quad i = 1,\ldots,\nd,
\end{align}
%
where the velocity and stress components, $v_i$ and $\sigma_{ji}$, are functions of 
$\rv$ and $t$ and $\dot{x}_j$ is the grid velocity.
The pressure equation in \ref{eq:pressurePoissonEquation} is transformed in a similar way.

For the solid we consider the governing equations written in quasilinear matrix form,
\begin{align}
\frac{\partial \bar{q}_i}{\partial t} +
\frac{\partial }{\partial \xs_k} \left( \bar{A}_{ijk} \bar{q}_{j} \right)
= \bs_i.
\end{align}
%
$\bar{\qv} = [\usv,\vsv,\sigmasv]^T$ is the state variable containing the components of 
displacement, velocity, and stress. $\bar{A}_{ijk}$ is a matrix whose components 
depend on the solid density, $\rhos$, and Lam\'e parameters $\lambdas$ and $\mus.$
Under the coordinate transform
$\xsv = \bar{\gv}(\rv),$ the equations become
\begin{align}
\frac{\partial \bar{q}_i}{\partial t} +
\frac{1}{\bar{J}} \frac{\partial}{\partial r_l} 
\left(\bar{J} \frac{\partial r_l}{\partial \xs_k} \bar{A}_{ijk} \bar{q}_j \right)
 = \bs_i
\end{align}
%
where the components of the state vector, $\bar{q}_i$, are functions of $\rv$ and
$\bar{J} = \det\left(\frac{\partial \xs_i}{\partial r_j} \right)$ 
is the Jacobian of the mapping. 
We use a second-order (Godunov-based) upwind scheme similar to \cite{smog2012,fsi2012}.
\das{Is there anything else done here?}

\subsubsection{Curvilinear interface conditions}

For implementation of the AMP interface conditions for the fluid velocity
in curvilinear coordinates, it is convenient to discretize equivalent vector equations.
We take the scalar conditions and assign a direction 
in the interface coordinate basis ($\nv,\, \tv_1,\, \tv_2$). 
\das{(overall todo, we should change the $\ev_m$'s above to $\tv_m$'s.)}
Noting that $I = \nv \nv^T + \tv_1 \tv_1^T + \tv_2 \tv_2^T$,
the Robin conditions \eqref{eq:AMPVelocityDiscreteCorrect}
and the divergence condition \eqref{eq:DivergenceFreeDiscreteCorrect} are
combined to give
\begin{align}
\nv \nv^T (\Grad \cdot \vv_\iv^{n+1}) 
+ \frac{1}{\mu} \left(I - \nv \nv^T \right)
\left(\tauv_\iv^{n+1} \nv + \zs \vv_\iv^{n+1} \right)
 &= \frac{1}{\mu} \left(I - \nv \nv^T \right)
\left(\sigmasv_\isv^{n+1} \nv + \zs \vvs_\isv^{n+1} \right),
\label{eq:RobinDivergenceVectorEquation}
\end{align}
%
for $\iv \in \GammaIfh$ and $\isv \in \GammaIsh$.
The normal component of the velocity is assigned using the impedance weighted average
\eqref{eq:AMPinterfaceNormalVelocityDiscrete}
and the tangential component of the velocity is assigned using the fluid scheme.
Let $\alpha = \zf / (\zf+\zs)$, then these conditions combine to give
\begin{align}
\vv_\iv^{n+1} &= 
\nv \nv^T \left( \alpha \vv_\iv^{(e)} + (1-\alpha) \vvs_\iv^{n+1} \right)
+ (I- \nv \nv^T) \vv_\iv^{(e)} , \quad \iv \in \GammaIfh, \; \isv \in \GammaIsh.
\label{eq:VelocityUpdateApproach}
\end{align}
%
Let $\mathcal{P} = (1-\alpha) \nv \nv^T$, then \eqref{eq:VelocityUpdateApproach}
can be simplified to 
\begin{align}
\vv^{n+1}_\iv &= \left( I - \mathcal{P} \right) \vv^{(e)}_\iv
+ \mathcal{P} \vvs_\iv^{n+1}, \quad \iv \in \GammaIfh, \; \isv \in \GammaIsh.
\label{eq:VelocityUpdateVectorEquation}
\end{align}
%
$\vv_\iv^{(e)}$ corresponds to the fluid update given by
\begin{align}
\vv_\iv^{(e)} = \vv_\iv^n + \frac{\dt}{2}\left(\Nv(\vv_\iv\sp{(p)},p_\iv\sp{(p)}) + \Nv(\vv_\iv\sp{n},p_\iv\sp{n})\right)
+ \frac{\dt}{2}\left(\Lv(\vv_\iv\sp{n+1}) + \Lv(\vv_\iv\sp n)\right),
\qquad    \iv \in \GammaIfh,
\end{align}
%
where $\Nv$ and $\Lv$ are the same grid operators defined in section
\ref{sec:algorithm}. In practice, equations 
\eqref{eq:RobinDivergenceVectorEquation} and \eqref{eq:VelocityUpdateVectorEquation}
are used in the building of the implicit matrix.

\subsection{Numerical fix-up for corners}


% For the velocity, the amp conditions are applied to obtain the ghost point on the interface line.
% this may not be necessary...
% \begin{align}
% \tv^T_m \tauv_\iv^{n+1} \nv + \zs \tv^T_m \vv_{\tilde{\iv}}^{n+1}
% &=
% \tv^T_m \sigmasv_\iv^{n+1} \nv + \zs \tv^T_m \vsv_{\tilde{\iv}}^{n+1} \\
% \grad_h \cdot \vv_\iv^{n+1} &= 0
% \end{align}
% \begin{align}
% \mu (D_{0,x} (v_2)_{0,0}^{n+1} + D_{0,y} (v_1)_{0,0}^{n+1}) - \zs (v_2)_{-1,0}^{n+1}
% &= \dots \\
% D_{0,x} (v_1)_{0,0} + D_{0,y} (v_2)_{0,0} &= 0
% \end{align}

In the solid, the zero-displacement and interface boundary conditions are incompatible 
if there is a non-zero traction at the corner. 
We can apply a numerical fix-up in two places to avoid wiggles.
The approach is to treat the fluid and solid interfaces as free surfaces near the corners.
The modified pressure condition is
\begin{align}
-p_\iv^{(p)}
-\frac{\zp \dt}{\rho} (\nv\cdot\Grad) p_\iv^{(p)}
&= 
{ \eta_\iv} \nv^T \left(  \Sigmasv_\isv^{(p)} \nv - \tauv_\iv^{(p)} \nv\right)
\nonumber \\
&\qquad + \zp \dt
 \nv^T \left(\nu \Grad \curl \Grad \curl \vv_\iv^{(p)} + (\vsv_t)_\isv^{(p)}\right), \qquad \iv \in \GammaIFh,
\end{align}
%
and the modified solid stress condition is
\begin{align}
\nv^T \sigmasv_\iv \nv = {\eta_\iv} \nv^T (\sigmav_I)_\iv \nv .
\end{align}
%
In the conditions, a ramp function is introduced which goes to zero near the boundaries
and one away from the boundaries.
\begin{align}
\eta_\iv = 1 - \sum \exp(-\gamma \|\xv_\iv - \xv_{\text{corner}}\|^2)
\end{align}
%
Numerical wiggles occur in only a few grid points away from the corners.
Therefore, we choose $\gamma$ to be proportional to $\frac{1}{h^2}.$ 
Due to this choice, $\eta_\iv$ will only affects the same number of grid points near the corner
as the grid is refined. 



\subsection{Decouple velocity components for implicit}

When solving implicitly, the AMP boundary conditions couple all $\nd$ components
of velocity. For computationally efficiency, we solve each component separately.
\das{This is a placeholder in case we decide to do this}.

\subsection{Filtering interface velocity}

The projected interface velocity~\eqref{eq:velocityProjection}
is optionally smoothed using a few iterations of a 
fourth-order filter as described in~\cite{smog2012}.
\das{This is a placeholder in case we decide to do this.}

\subsection{Time step determination}

The PDE solvers for the fluid and solid have different time step restrictions.
A time step restriction which depends on the mesh spacing 
is used to calculate a stable time step on each grid component.
The fluid restriction is 
based on a Von Neumann analysis of the linearized Navier-Stokes system
and the solid time step is chosen from a CFL restriction.
The global time step is then taken to be the minimum stable time step across all
grid components.

% \das{*copied from beamins*}

% Our numerical approach for the solution of the equations governing an
% FSI initial-boundary-value problem is based on the use of deforming
% composite grids (DCG).  This FSI-DCG approach was first described
% in~\cite{fsi2012} for the case of an inviscid
% compressible flow coupled to a linearly elastic solid, and later 
% in~\cite{flunsi2014r} for the case of compressible flow coupled to nonlinear
% hyperelastic solids.  Here, we extend the approach to FSI problems involving an incompressible flow
% coupled to deforming beams. 

% % ----------------------------------------------------------------------------------
% \subsection{Deforming composite grids and the fluid domain solver} \label{sec:dcg}

% Deforming composite grids (DCGs) are used to discretize the evolving fluid domains in physical space.
% An overlapping grid, $\Gs$, consists of a set of structured component grids, $\{G_g\}$,
% $g=1,\ldots,{\mathcal N}$, that cover each fluid domain, $\OmegaF_k(t)$, and overlap where
% the component grids meet. Typically, boundary-fitted curvilinear grids are used near the
% boundaries while one or more
% background Cartesian grids are used to handle the bulk of the fluid domain. 
% Each component grid is a logically rectangular, curvilinear grid in $\nd$~space
% dimensions, and is defined by a smooth
% mapping from parameter space~$\rv$ (the unit square or cube) to physical
% space~$\xv$,
% \[
%   \xv = \gv(\rv,t),\qquad \rv\in[0,1]^\nd,\qquad \xv\in\Real^\nd.
% \]
% Typically, the background grids are static, while the boundary-fitted grids evolve in time to
% match the motion of the boundary.

% {% ------ GRIDS ------
% \newcommand{\figWidth}{7.5cm}
% \newcommand{\trimfig}[2]{\trimFig{#1}{#2}{.1}{.4}{.35}{.375}}
% \begin{figure}[htb]
% \begin{center}
% \begin{tikzpicture}[scale=1]
%   \useasboundingbox (0.0,.75) rectangle (16.,5.5);  % set the bounding box (so we have less surrounding white space)
%   \draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/bic4Gridt0p0}{\figWidth}};
%   \draw(8.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfig{fig/bic4Gridt1p0}{\figWidth}};
% % grid:
% %  \draw[step=1cm,gray] (0,0) grid (16,5);
% \end{tikzpicture}
% \end{center}
%   \caption{Composite grids for a beam in a channel at times  $t=0.0$, and $1.0$. The green fluid grid deforms over
% time to match the evolving beam (shown in white) and overlaps with the background Cartesian fluid grid (shown in blue).  The reference curve
% of the beam is shown in red and the thickness of the beam describes the position of the surface of the beam.}
%   \label{fig:beamGrids}
% \end{figure}
% }

% In the FSI-DCG approach, component grids next to a fluid-structure interface deform over time
% to match the beam motion. This is illustrated in \Fig~\ref{fig:beamGrids} for the case of a beam
% in a fluid channel.
% A green fluid grid is fitted to the boundary of the beam, which is defined in terms of displacement of the reference curve of the beam (shown in red) and the thickness of the beam (c.f.~\eqref{eq:EBsurface}).

% The beam thickness is a function of the position $s\in\OmegaSbar$ along the reference curve, and remains fixed as the beam deforms. $\OmegaSbar$ is defined from a parameterization of the beam reference curve, e.g. $\OmegaSbar=[0,\ls]$
% where $\ls$ is the length of the undeformed beam.
% After each time step, the points on the fluid interface corresponding to the surface of the beam are recomputed according to the current displacement of the beam and the normal to the reference curve using~\eqref{eq:EBsurface},
% and a hyperbolic grid generator~\cite{HyperbolicGuide} is used to regenerate the local interface grids.
% After all deforming component grids have been regenerated, the {\tt Ogen} grid generator~\cite{OGEN}
% is called to regenerate the overlapping grid connectivity (e.g., cut holes, determine interpolation points) between the evolving interface-fitted fluid grids and the fixed background fluid grids, typically Cartesian grids, shown in blue in \Fig~\ref{fig:beamGrids}. 


% The incompressible Navier-Stokes equations are solved in velocity-pressure form 
% on overlapping grids using a 
% second-order accurate fractional-step algorithm~\cite{fis2014,splitStep2003,ICNS} similar to that
% described in Section~\ref{sec:timeStepping}. The treatment of moving overlapping grids, including the 
% assignment of {\em exposed points}, follows the approach
% discussed in~\cite{mog2006} for compressible flow.
% The governing equations for the fluid on a given component grid are solved in a coordinate frame moving with the grid. 
% Consider the momentum equations in~\eqref{eq:fluidMomentum}
% for the fluid in an Eulerian frame,
% \begin{align}
%   & \frac{\partial v_i }{\partial t} + v_j\frac{\partial v_i}{\partial x_j} = 
%       {1\over\rho}\,\frac{\partial \sigma_{ji}}{\partial x_j}, \qquad i=1,\ldots,\nd,  \label{eq:fluidEulerian}
% \end{align}
% with summation convention. Under a general moving coordinate transformation, $\xv=\gv(\rv,t)$, 
% the equations in~\eqref{eq:fluidEulerian} are transformed using the chain rule to become 
% \begin{align}
%   \frac{\partial v_i }{\partial t} 
%      + (v_j-w_j)\frac{\partial r_k}{\partial x_j}\frac{\partial v_i}{\partial r_k} =
%      {1\over\rho}\,\frac{\partial r_k}{\partial x_j}\frac{\partial \sigma_{ji}}{\partial r_k}, \qquad i=1,\ldots,\nd,\label{eq:GMmomentum}
% \end{align}
% where the component of velocity $v_i$ and stress $\sigma_{ji}$ are now considered to be functions of $\rv$ and $t$, and where
% $w_j=\partial g_j/\partial t$ are the components of the {\em grid velocity}, $\wv$.
% The pressure equation in~\eqref{eq:fluidPressure} is transformed to $(\rv,t)$ in a similar way. 


% % ----------------------------------------------------------------------------------
% \subsection{Structural domain solvers and the AMP condition}  \label{sec:beamSolverNumerical}

% Two approaches are implemented to advance the governing equations for the beam.  The first is a second-order accurate predictor-corrector scheme described previously in Section~\ref{sec:timeStepping}, which also uses standard second-order accurate finite differences to approximate the spatial derivatives in~\eqref{eq:BeamModel} assuming an Euler-Bernoulli beam.  The basic AMP condition in~\eqref{eq:AMP_CombinedConditions} for this beam model becomes
% \begin{equation}
%     (\sigmav\nv)_+ + (\sigmav\nv)_- + 
% \frac{\rhos\hs}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  
%          = \Lsv\bigl(\uvs^{(p)},\vsv^{(p)}\bigr) + \rhos\hs \partialt \wsv^{(p)}_\pm(\ss,t) , \qquad \ss\in\OmegaSbar,
%     \label{eq:AMP_CombinedConditionsII}
% \end{equation}
% where the predicted quantities on the right-hand side of~\eqref{eq:AMP_CombinedConditionsII} involving the displacement and velocity of the beam can be computed in terms of the discrete values for $\eta$, $\partial\eta/\partial t$, and $\partial^2\eta/\partial t^2$, and their spatial derivatives, using standard finite differences.  The normal and tangential components of~\eqref{eq:AMP_CombinedConditionsII} then become boundary conditions for the fractional-step fluid solver.


% The second approach implemented to advance the equations in~\eqref{eq:BeamModel} for an Euler-Bernoulli beam uses a standard finite-element approximation in space and the Newmark-beta time-stepping scheme (given below).
% The spatial representation of the beam displacement in the finite-element approximation is taken as 
% \begin{align}
%  \ww_h(s,t) = \sum_{j=1}^{\Nn}\Big\{\, \ww_j(t) \phi_j(s) +\ww_j'(t) \psi_j(s)  \,\Big\}, \label{eq:beamFEM}
% \end{align}
% where the degrees of freedom are the
% nodal displacement $\ww_j(t)$ and slope $\ww\sp\prime_j(t)$, and where $\phi_j(s)$ and $\psi_j(s)$ are 
% cubic Hermite polynomials 
% with support on the interval $[s_{j-1},s_{j+1}]$ and satisfying
% \[
% \begin{array}{ll}
%   \phi_i(s_j)=\delta_{ij}, \quad &\phi_i'(s_j)=0, \medskip\\
%   \psi_i(s_j)=0,                  &\psi_i'(s_j)=\delta_{ij},
% \end{array}
% \]
% where $\delta_{ij}$ is the Kronecker delta.  Following the usual Galerkin approximation in space, the beam equation becomes
% \begin{align}
%    M_h \frac{d^2\wvh}{dt^2}  = - K_h \wvh - B_h \frac{d\wvh}{dt}  + \fvh, \label{eq:discreteBeam}
% \end{align}
% where $M_h$ is a mass matrix, $K_h$ is a stiffness matrix, and $B_h$ is a damping matrix.  The vector $\wvh$ contains the nodal displacements and slopes, $\ww_j(t)$ and $\ww\sp\prime_j(t)$, $j=1,\ldots,\Nn$, and the components of the forcing vector $\fvh$ are given by integrals of $f(\sv,t)$ in~\eqref{eq:BeamModel} with the Hermite basis functions\footnote{Appropriate adjustments are made to the matrices and right-hand-side to account for boundary conditions.}.

% %
% The ODEs in~\eqref{eq:discreteBeam} are advanced in time using a second-order accurate Newmark-beta scheme in predictor-corrector form.
% Let $\wvh^n\approx\wvh(t^n)$, $\vsh^n\approx\frac{d\wvh}{dt}(t^n)$, $\avh^n\approx \frac{d^2\wvh}{dt^2}(t^n)$, and $\Fvh^{n}\approx\Fvh(t^n)$.
% The Newmark-beta scheme is based on a Taylor series in time and is given by
% \begin{align*}
%  &  \wvh^{n+1} = \wvh^n + \dt\,\vsh^n + \frac{\dt^2}{2}\Big[ (1-2\beta) \avh^n + 2\beta \avh^{n+1} \Big],  \\
%  &  \vsh^{n+1} = \vsh^n + \dt\Big[  (1-\gamma) \avh^n + \gamma \avh^{n+1} \Big]    , \\
%  &  M_h \avh^{n+1} = -K_h \wvh^{n+1} -B_h \vsh^{n+1}  + \Fvh^{n+1} .
% \end{align*}
% We take $\beta=1/4$ and $\gamma=1/2$ which defines a second-order accurate approximation.
% During the prediction step, the forcing $\Fvh^{n+1}$ is not yet known in FSI problems and instead 
% a predicted value is used given by extrapolation in time
% \begin{align*}
%  &  \Fvh^{(p)} = 2 \Fvh^{n} - \Fvh^{n-1} .
% \end{align*}


% Given predicted values for $\wvh^{(p)}$ and $d\wvh^{(p)}/dt$ from the first stage of the AMP algorithm, pointwise values
% of the beam operator, $\Lsv\sp{(p)}$, are required to evaluate the right-hand side of the AMP condition
% in~\eqref{eq:AMP_CombinedConditionsII}.  
% This is generally a straightforward computation in the context of finite difference or
% finite volume approximations to the beam operator, whereas the calculation may be more difficult within the finite-element
% approximation.  As an example, consider a beam operator of the form
% \[
%    \Ls = - (\Es\Is\ww_{ss})_{ss},
% \]
% where the subscripts denote partial derivatives with respect to $s$.  It is sufficient to only consider the highest derivative term in~\eqref{eq:BeamModel} for the purposes of the present discussion.
% Let $\Ls$ have the Hermite finite-element representation
% \begin{equation}
%  \Ls_h(s,t) = \sum_{j=1}^{\Nn} \Big\{\, \gamma_j(t) \phi_j(s) + \gamma_j'(t) \psi_j(s) \,\Big\}  ,\label{eq:beamOperatorAMP_APPROX}
% \end{equation}
% where $\gamma_j(t)$ and $\gamma_j'(t)$ are coefficient functions of time, and $\phi_j(s)$ and $\psi_j(s)$ are the cubic polynomial basis functions in~\eqref{eq:beamFEM}.  
% The $2\Nn$ unknowns, $\gamma_j(t)$ and $\gamma_j'(t)$, are determined from 
% the $2\Nn$ Galerkin equations
% \begin{equation}
%     \beamInnerProd{ \chi_j,\Ls_h}  = (\chi_j, 
%         - \beamInnerProd{\Es\Is\ww_{h,ss})_{ss} }, \qquad j=1,2,\ldots,\Nn, \label{eq:galerkin}
% \end{equation}
% where $\chi_j=\phi_j$ or $\psi_j$, and where $\beamInnerProd{f,g}\equiv \int_0^{\ls} f(s) g(s)\, ds$. 
% Integration by parts (twice) gives 
% \begin{equation}
%     \beamInnerProd{\chi_j,\Ls_h} = 
%        - \beamInnerProd{\chi_{j,ss},\Es\Is\ww_{h,ss}} + \left.\Big\{ 
%             - \chi_j (\Es\Is\ww_{h,ss})_{s} + \chi_{j,s} \Es\Is\ww_{h,ss})\Big\}\right\vert_0^{\ls}, \qquad j=1,2,\ldots,\Nn .
% \label{eq:integrationByParts}
% \end{equation}
% The problem now arises in computing second-order accurate approximations to the boundary terms $(\Es\Is\ww_{h,ss})_{s}$ and $\Es\Is\ww_{h,ss}$
% appearing in~\eqref{eq:integrationByParts}. The cubic Hermite representation is not of
% sufficient accuracy for this purpose since, for example, $\ww_{h,sss}$ is constant over an element and at best first-order accurate. 

% There are various possible solutions to the difficulty of evaluating the right-hand side of~\eqref{eq:AMP_CombinedConditionsII}
% in the context of a finite-element approximation, 
% and we have considered and tested two different approaches that require relatively minor changes. 
% The properties of the two approaches are evaluated in Section~\ref{sec:numericalResults} where some
% conclusions are drawn.

% \subsubsection{AMP-PBA : Predict Beam Acceleration} \label{sec:ampadj}

%  In the first approach, which we refer to as AMP-PBA (Predict Beam Acceleration), the vector form of~\eqref{eq:BeamModel} is used in~\eqref{eq:AMP_CombinedConditionsII} to eliminate $\Lsv\sp{(p)}$, which gives an AMP condition of the form,
% \begin{equation}
%     (\sigmav\nv)_+ + (\sigmav\nv)_- + 
% \frac{\rhos\hs}{\rho}\grad\cdot\sigmav(\xsv_\pm(\ss,t),t)  
%          =  \rhos \hs \frac{\partial^2}{\partial t^2}\usv^{(p)} - \fsv\sp{(p)}(s,t) + \rhos\hs \partialt \wsv^{(p)}_\pm(\ss,t) , \qquad \ss\in\OmegaSbar.
%     \label{eq:AMP_CombinedConditionsIIadjusted}
% \end{equation}
% The predicted beam acceleration 
% $\partial\sp2\usv\sp{(p)}/\partial t\sp2$ in~\eqref{eq:AMP_CombinedConditionsIIadjusted} is readily computed from the acceleration term in the weak form~\eqref{eq:discreteBeam}, while the predicted fluid forcing, $\fsv\sp{(p)}(s,t)=-(\sigmav\nv)_+^{(p)}-(\sigmav\nv)_-^{(p)}$, can be obtained from the discrete fluid stress.  This gives the following AMP-PBA algorithm:
% \begin{enumerate}
%    \item Obtain predicted values for $\fsv\sp{(p)}=-(\sigmav\nv)_+^{(p)}-(\sigmav\nv)_-^{(p)}$ 
%          using extrapolation in time during the predictor stage or the current guess during the corrector stage (c.f.~the algorithm in Section~\ref{sec:timeStepping}).
%    \item Solve~\eqref{eq:discreteBeam} for $d^2\wvh^{(p)}/dt^2$ using the predicted force $\fsv\sp{(p)}$, 
%         and evaluate pointwise values for
%         $\rhos \hs (\partial\sp2\usv\sp{(p)}/\partial t\sp2)$
%           from the Hermite representation for this quantity. 
%    \item Evaluate the right-hand side to~\eqref{eq:AMP_CombinedConditionsIIadjusted} and use this when applying the AMP conditions to the fluid.
% \end{enumerate}

% \subsubsection{AMP-PBF : Predict Beam internal Force}


% In the second approach, referred to as AMP-PBF (Predict Beam internal Force), a mixed finite-element/finite-difference approach is used to compute the beam internal force
% $\Lsv\sp{(p)}$ directly from equation~\eqref{eq:integrationByParts} (extended to include all terms in the full EB model). 
% In particular, using the solution nodal values and derivatives on the boundary and two adjacent points, a
% fourth-order accurate approximation to $\Es\Is\ww_{ss}$ and a second-order accurate approximation to $(\Es\Is\ww_{ss})_{s}$ on the boundary can be
% derived. This allows the coefficients $\gamma_j(t)$ and $\gamma_j'(t)$
% to be determined and then pointwise values of $\Lsv\sp{(p)}$ can be computed from~\eqref{eq:beamOperatorAMP_APPROX}.  
% This gives the following AMP-PBF algorithm:
% \begin{enumerate}
%    \item Given predicted values for $\ww_h^{(p)}$, determine second-order accurate approximations to the boundary terms $(\Es\Is\ww_{h,ss})_{s}$ 
%        and $\Es\Is\ww_{h,ss}$ in~\eqref{eq:integrationByParts} using a finite-difference approximation involving the boundary   
%        points and two adjacent points. 
%    \item Compute values for $\Lsv^{(p)}$ by solving the Galerkin equations in~\eqref{eq:integrationByParts} 
%          (extended to include all terms in the full EB model) for
%          $\gamma_j$ and $\gamma_j'$. 
%    \item Evaluate the right-hand side to~\eqref{eq:AMP_CombinedConditionsII} using~\eqref{eq:beamOperatorAMP_APPROX},
%          and use this when applying the AMP conditions to the fluid.
% \end{enumerate}

% %% ====================================================================================
% \subsection{Filtering the projected interface velocity} \label{sec:velocityFilter}

% The projected interface velocity~\eqref{eq:velocityProjection}
% is optionally smoothed using a few iterations of a fourth-order filter as described in~\cite{smog2012}.
% The beam solution can also be smoothed to prevent high-frequency numerical oscillations, 
% for example by choosing the coefficient kxxt in~\eqref{eq:BeamModel} to be proportional to $\Delta\sv^2$. However, for light
% beams the interface velocity is determined primarily from the fluid and thus the 
% filter on the interface velocity is needed for light beams to prevent numerical oscillations on the interface.
% Note that as the beam becomes very light,
% with beam parameters * etc. going to zero, the AMP interface
% condition approaches that of a free surface boundary condition for the fluid.
% Such a free surface condition with no surface tension is susceptible to physical and numerical instabilities, and the fourth-order filter acts to suppress these instabilities and thus serves as a {\em numerical surface tension}. 
% This filter does not affect the overall second-order accuracy of the AMP FSI time-stepping scheme. 


% % ----------------------------------------------------------------------------------
% \subsection{Time step determination} \label{sec:timeStep}

% The global time step, $\dt$, for the AMP FSI time-stepping scheme is chosen to be the 
% minimum of the stable time steps for the fluid domain solver and beam solver. 
% The $\dt$  for the fluid solver is chosen to be a factor
% $\lambda_{{\rm SF}}$ (``SF'' for stability factor)
% times an estimate of the 
% largest stable time step based on a von Neumann analysis of the linearized Navier-Stokes system.
% Typically we choose $\lambda_{{\rm SF}}=0.9$.
% In this work, the FEM beam solver is implicit in time and stable for any time step. However, for 
% accuracy reasons it is convenient to choose $\dt$ based on a condition relating to explicit time-stepping. 
% Thus, the time-step for the beam is chosen as a factor $\bar\lambda_{{\rm SF}}$ 
% times an estimate of the largest time step such that an explicit time-stepping procedure for the beam would 
% satisfy a CFL stability condition.  Here $\bar\lambda_{{\rm SF}}$  is chosen in the range~1 to~10.



==> texFiles/numericalStability.tex <==
% \newcommand{\zfHat}{\hat{z}_f}
% \newcommand{\zfm}{z_{fm}}
% \newcommand{\zfmu}{z_{f\mu}}
% \newcommand{\zfh}{z_{fh}}
% \newcommand{\Cmu}{C_\mu}
% \newcommand{\Cmono}{C_m}
% \newcommand{\alphaV}{\alpha}
% \newcommand{\LambdaSolid}{\bar{\Lambda}}
\section{Numerical stability results}


Here will be tabulated results of what works and what does not work.

Parameters: (what should be our set of non-dimensional parameters?)
\bas
& \zfHat=\f{\mu\rho}{\zp\dt}, \\
& \zfmu = \Cmu \f{\mu}{h}  , \\
& \zfh = \f{\rho h}{\dt}  , \\
& \zfm = \Cmono z_f^v \quad \text{($\Cmono$ times impedance from monolithic scheme, using $k=\f{1}{\Delta n}$} ) , \\
& \Lambda_\nu = \f{\nu\dt}{h^2} = \text{viscous CFL number} ,\\
& \LambdaSolid =  \text{solid CFL number} 
\eas

\noindent Block Elastic Piston: 
\begin{table}[H]
\caption{Block Elastic Piston AMP parameters}
\begin{center}\small
\begin{tabular}{cccccccccccccc}
\hline
$\scf$  & $\mu$  & $h$ & $\f{\nu\dt}{h^2}$ &  $\LambdaSolid$ & $\zp$  & $\zfmu$ & $\zfh$ &  $\zfHat$  & $\zfm$  & $\Cmu$ &  $\Cmono$ & $\alphaV$ & $t_f$  \\
\hline
\multicolumn{13}{c}{OLD WAY: $\zfHat$ and $\zfmu$,  OK} \\
 1e+03 & 0.05 & 0.05 & 0.25 & 0.9 & 1.7e+03 & 1 & 4 & 0.0023 & 7.2 & 1 & 0 & 0.00058 & ? \\ 
 1 & 0.05 & 0.05 & 0.25 & 0.9 & 1.7 & 1 & 4 & 2.3 & 6.9 & 1 & 0 & 0.37  & ?\\ 
 0.001 & 0.05 & 0.05 & 0.25 & 0.9 & 0.0017 & 1 & 4 & 2.3e+03 & 6.8 & 1 & 0 & 1  & ?\\ 
\hline
\multicolumn{13}{c}{Monolithoic: OK} \\
1e+03 & 0.05 & 0.012 & 0.8 & 0.9 & 1.7e+03 & 4 & 5 & 0.012 & 15 & 0 & 1 & 0.0086 & 1.1 \\
1 & 0.05 & 0.012 & 0.8 & 0.9 & 1.7 & 4 & 5 & 12 & 15 & 0 & 1 & 0.89 & 1.1 \\
0.001 & 0.05 & 0.05 & 0.2 & 0.9 & 0.0017 & 1 & 5 & 2.9e+03 & 7.8 & 0 & 1 & 1 & 1.1 \\
0.001 & 0.05 & 0.012 & 0.8 & 0.9 & 0.0017 & 4 & 5 & 1.2e+04 & 15 & 0 & 1 & 1 & 1.1 \\
\hline
\end{tabular}
\end{center}
\label{fig:blockElasticPiston}
\end{table}


\noindent Block Shear elastic piston: (Large $nu$ may impose a CFL restriction from curl-curl)
\begin{table}[H]
\caption{Block SHEAR Elastic Piston AMP parameters}
\begin{center}\small
\begin{tabular}{cccccccccccccc}
\hline
$\scf$  & $\mu$  & $h$ & $\f{\nu\dt}{h^2}$ &  $\LambdaSolid$ & $\zp$  & $\zfmu$ & $\zfh$ &  $\zfHat$  & $\zfm$  & $\Cmu$ &  $\Cmono$ & $\alphaV$ & $t_f$  \\
\hline
\multicolumn{13}{c}{OLD WAY:  $\zfHat$ and $\zfmu$, CFL=.1 looks OK} \\
 1e+03 & 10 & 0.012 & 23 & 0.1 & 1.7e+03 & 8e+02 & 35 & 16 & 1.7e+03 & 5 & 0 & 0.7  & ?\\ 
\hline 
\multicolumn{13}{c}{OLD WAY: Slow growth, wiggles in p, CFL too big?} \\
 1e+03 & 10 & 0.012 & 1.6e+02 & 0.7 & 1.7e+03 & 8e+02 & 5 & 2.3 & 1.6e+03 & 2 & 0 & 0.48  & ?\\ 
 1e+03 & 10 & 0.012 & 1.6e+02 & 0.7 & 1.7e+03 & 8e+02 & 5 & 2.3 & 1.6e+03 & 5 & 0 & 0.7  & ?\\
 \hline
\multicolumn{13}{c}{Monolithic works? CFL=.1, $\Cmono=.1$} \\
 1e+03 & 10 & 0.012 & 23 & 0.1 & 1.7e+03 & 8e+02 & 35 & 16 & 1.7e+03 & 0 & 0.1 & 0.087  & ?\\ 
\hline
\multicolumn{13}{c}{Monolithic FAILED: $\Cmono=1$, CFL=.5} \\
1e+03 & 10 & 0.025 & 80 & 0.9 & 1.7e+03 & 4e+02 & 5 & 1.2 & 8.1e+02 & 0 & 1 & 0.32  & ?\\
1e+03 & 10 & 0.025 & 57 & 0.5 & 1.7e+03 & 4e+02 & 7 & 1.6 & 8.1e+02 & 0 & 1 & 0.32 & ? \\
\hline
\end{tabular}
\end{center}
\label{fig:blockShearElasticPiston}
\end{table}

\noindent Block Shear elastic piston: $\delta=10^3, \nu=.1$
\begin{table}[H]
\caption{Block SHEAR Elastic Piston AMP parameters \das{8/21/18}}
\begin{center}\small
\begin{tabular}{cccccccccccccc}
\hline
$\scf$  & $\mu$  & $h$ & $\f{\nu\dt}{h^2}$ &  $\LambdaSolid$ & $\zp$  & $\zfmu$ & $\zfh$ &  $\zfHat$  & $\zfm$  & $\Cmu$ &  $\Cmono$ & $\alphaV$ & $t_f$  \\
\hline
\multicolumn{13}{c}{Monolithic OK: $\Cmono=1$, CFL=.9} \\
 1e+03 & 0.1 & 0.0031 & 8 & 0.9 & 1.7e+03 & 32 & 4 & 0.074 & 70 & 0 & 1 & 1 & 1 \\ 
 1e+03 & 0.1 & 0.0062 & 4.1 & 0.9 & 1.7e+03 & 16 & 3.9 & 0.036 & 38 & 0 & 1 & 1 & 1 \\ 
 1e+03 & 0.1 & 0.012 & 2.1 & 0.9 & 1.7e+03 & 8 & 3.9 & 0.018 & 22 & 0 & 1 & 0.012 & 1 \\ 
\multicolumn{13}{c}{Monolithic OK after $>3000$ steps: $\Cmono=1$, CFL=.01} \\
 1e+03 & 10 & 0.012 & 2.3 & 0.01 & 1.7e+03 & 8e+02 & 3.5e+02 & 1.6e+02 & 2.1e+03 & 0 & 1 & 1 & 1 \\ 
\multicolumn{13}{c}{Monolithic BAD: $\Cmono=1$, CFL=.9 and CFL=.1, time restriction from curl-curl?} \\
 1e+03 & 10 & 0.012 & 2.1e+02 & 0.9 & 1.7e+03 & 8e+02 & 3.9 & 1.8 & 1.6e+03 & 0 & 1 & 1 & 1 \\ 
 1e+03 & 10 & 0.012 & 23 & 0.1 & 1.7e+03 & 8e+02 & 35 & 16 & 1.7e+03 & 0 & 1 & 1 & 1 \\ 
\multicolumn{13}{c}{OLD WAY BAD: CFL=.9, slow growth (unstable)} \\
1e+03 & 10 & 0.012 & 2.1e+02 & 0.9 & 1.7e+03 & 8e+02 & 3.9 & 1.8 & 1.6e+03 & 1 & 0 & 1 & 1 \\
\multicolumn{13}{c}{OLD WAY BAD: CFL=.1, still slow growth (unstable)} \\
1e+03 & 10 & 0.012 & 23 & 0.1 & 1.7e+03 & 8e+02 & 35 & 16 & 1.7e+03 & 1 & 0 & 1 & 1 \\ 
\hline
\end{tabular}
\end{center}
\label{fig:blockShearElasticPiston}
\end{table}


\noindent RADIAL Elastic Piston: 
\begin{table}[H]
\caption{Radial Elastic Piston AMP parameters}
\begin{center}\small
\begin{tabular}{cccccccccccccc}
\hline
$\scf$  & $\mu$  & $h$ & $\f{\nu\dt}{h^2}$ &  $\LambdaSolid$ & $\zp$  & $\zfmu$ & $\zfh$ &  $\zfHat$  & $\zfm$  & $\Cmu$ &  $\Cmono$ & $\alphaV$ & $t_f$  \\
\hline
\multicolumn{13}{c}{OLD WAY: $\zfHat$ and $\zfmu$,  OK} \\
 1e+03 & 0.05 & 0.021 & 0.52 & 0.9 & 1.7e+03 & 2.3 & 4.5 & 0.0061 & 11 & 2 & 0 & 0.0078 & 1.1 \\
 0.001 & 0.05 & 0.075 & 0.15 & 0.9 & 0.0017 & 0.67 & 4.5 & 1.7e+03 & 6.5 & 2 & 0 & 1 & 1.1 \\ 
 0.001 & 0.05 & 0.037 & 0.32 & 0.9 & 0.0017 & 1.3 & 4.1 & 3.2e+03 & 7.7 & 2 & 0 & 1 & 1.1 \\
 0.001 & 0.05 & 0.011 & 1.1 & 0.9 & 0.0017 & 4.7 & 4.3 & 1.2e+04 & 15 & 2 & 0 & 1 & 1.1 \\ 
\hline
\multicolumn{13}{c}{Monolithoic: OK} \\
1e+03 & 0.05 & 0.011 & 1.1 & 0.9 & 1.7e+03 & 4.7 & 4.3 & 0.012 & 15 & 0 & 1 & 0.0088 & 1.1 \\
1 & 0.05 & 0.011 & 1.1 & 0.9 & 1.7 & 4.7 & 4.3 & 12 & 15 & 0 & 1 & 0.9 & 1.1 \\
1 & 0.05 & 0.021 & 0.52 & 0.9 & 1.7 & 2.3 & 4.5 & 6.1 & 10 & 0 & 1 & 0.86 & 1.1 \\
0.001 & 0.05 & 0.021 & 0.52 & 0.9 & 0.0017 & 2.3 & 4.5 & 6.1e+03 & 10 & 0 & 1 & 1 & 1.1 \\
\hline
\end{tabular}
\end{center}
\label{fig:radialElasticPiston}
\end{table}

\noindent RADIAL SHEAR Elastic Piston: 
\begin{table}[H]
\caption{Radial Shear Elastic Piston AMP parameters}
\begin{center}\small
\begin{tabular}{cccccccccccccc}
\hline
$\scf$  & $\mu$  & $h$ & $\f{\nu\dt}{h^2}$ &  $\LambdaSolid$ & $\zp$  & $\zfmu$ & $\zfh$ &  $\zfHat$  & $\zfm$  & $\Cmu$ &  $\Cmono$ & $\alphaV$ & $t_f$  \\
\hline
\multicolumn{13}{c}{OLD WAY: $\zfHat$ and $\zfmu$, OK} \\
1e+03 & 10 & 0.011 & 2.2e+02 & 0.9 & 1.7e+03 & 9.3e+02 & 4.3 & 2.3 & 1.9e+03 & 5 & 0 & 0.73 & 0.6 \\
1e+03 & 10 & 0.021 & 1e+02 & 0.9 & 1.7e+03 & 4.7e+02 & 4.5 & 1.2 & 9.4e+02 & 5 & 0 & 0.57 & 1.1 \\
\hline
\multicolumn{13}{c}{Monolithoic Better:  CFL=.1 but trouble at t=.2?} \\
 1e+03 & 10 & 0.011 & 24 & 0.1 & 1.7e+03 & 9.3e+02 & 39 & 21 & 1.9e+03 & 0 & 1 & 0.53 & 0.6 \\ 
\multicolumn{13}{c}{Monolithoic: FAILED, CFL=.9} \\
 1e+03 & 10 & 0.011 & 2.2e+02 & 0.9 & 1.7e+03 & 9.3e+02 & 4.3 & 2.3 & 1.9e+03 & 0 & 1 & 0.52 & 0.6 \\ 
 \hline
\end{tabular}
\end{center}
\label{fig:radialShearElasticPiston}
\end{table}



%- \begin{table}[H]
%- \caption{Block Elastic Piston $\zfHat=\f{\mu\rho}{\zp\dt}$, $z_f = \Cmu \f{\mu}{h}$ }
%- \begin{center}
%- \begin{tabular}{cccccccc}
%- \hline
%- $\nu$    & $\scf=10^{-3}$ & $\scf=10^{-2}$ & $\scf=10^{-1}$ & $\scf=1$ &  $\scf=10$  & $\scf=10^2$  & $\scf=10^3$ \\
%- \hline
%- $10^{-2}$  &  $\Cmu=1$  &   ?    &  ?    &  ?     &  ?    &  ?    &  ?   \\
%- $10^{-1}$  &  ?      &   ?    &  ?    &  ?     &  ?    &  ?    &  ?   \\
%- $1$        &  ?      &   ?    &  ?    &  ?     &  ?    &  ?    &  ?     \\
%- $10$       &  ?      &   ?    &  ?    &  ?     &  ?    &  ?    &  ?     \\
%- \hline
%- \end{tabular}
%- \end{center}
%- \label{fig:blockElasticPiston}
%- \end{table}





==> texFiles/oldStuff.tex <==
\clearpage
\section{OLD STUFF}

\input texFiles/elasticPistonOverture.tex

\input texFiles/balloon

\input texFiles/halfDiskInAChannel

\input texFiles/beamInAChannel

\subsection{Radial traveling wave solution}

The radial traveling wave solution is a linearized solution which couples both
radial and circumferential motions together.
See~\ref{sec:RadialTravelingWave} for the derivation.

% \input texFiles/radialTravelingWaveFig

\noindent \textbf{\blue New: use monolithic $z_f$}
\input tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NUp1zfmImtp3.ConvTable.tex
\input tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCFp1NUp1zfmImtp3.ConvTable.tex
\input tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NUp1zfmImtp3.ConvTable.tex

% \input tables/insElasticPiston.rtw.AmpCaseid7SCF200NUp1zf1+0Imtp3.ConvTable.tex
% \input tables/insElasticPiston.rtw.AmpCaseid8SCF200NUp1zf1+0Imtp3.ConvTable.tex


\textbf{Note:} For the traditional scheme, the pressure equation in the interior is singular. The mean value
of $p$ probably wants to be zero so the undeformed state is a steady state. The AMP scheme does have
trouble with the mean of the pressure for large scf.

% \medskip
% \noindent \textbf{\blue New: match fluid and solid: $\zfHat=(\mu\rho)/(\zp\dt)$,  $z_f=1 \mu/h$. Results for caseid=4, scf=10, $\nu=.1$} 
% % \input tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid4SCF10zf1+0Imtp3.ConvTable.tex

% \medskip
% \noindent \textbf{\blue New: match fluid and solid: $\zfHat=(\mu\rho)/(\zp\dt)$,  $z_f=1 \mu/h$. Results for caseid=0, scf=1, $\nu=.1$}
% % \input tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1zf1+0Imtp2.ConvTable.tex

% \noindent \textbf{\blue New: match fluid and solid: $\zfHat=(\mu\rho)/(\zp\dt)$,  $z_f=1 \mu/h$. Results for caseid=2, scf=.001, $\nu=.1$. May need to integrate longer for better solid errors.}
% % \input tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp3.ConvTable.tex
% % \input tables/insElasticPiston.rtw.radialTravelingWaveAmpCaseid2SCF1e-3zf1+0Imtp5.ConvTable.tex



\clearpage
\subsection{Elastic disk in a channel, or rigid disk in an elastic channel, or two disks} 

Here is a potential example. An elastic disk (with an inner hole with displacmenent BCs to fix its position)
lies in a fluid channel. We could add multiple disks and/or elastic channel walls.

For comparison, results are shown for the traditional partitioned (TP) scheme applied to this problem.
Table~\ref{fig:diskInAChannelStability} shows the stability of the computed solution as a function of the
solid scale factor $\scf$ and the grid resolution for the TP scheme. The solution is denoted as \textit{BAD} if it
becomes unstable, while \textit{OK} indicates the scheme remains stable.
Note that the results indicate that a value of $\scf=200$ is already
considered to be a \textit{very light} solid as the TP scheme is unstable for all grids considered.
As expected from the theory, the TP scheme
eventually becomes unstable for any $\scf$ once the grid becomes sufficiently fine.







% \input texFiles/balloonFig.tex

{% ----------- ELASTIC DISK  ------  
%
\newcommand{\figWidtha}{4cm}% width
\newcommand{\trimfiga}[2]{\trimwb{#1}{#2}{.0}{.0}{.0}{.0}}
\newcommand{\figWidth}{6cm}% width
\newcommand{\trimfig}[2]{\trimwb{#1}{#2}{.2}{.2}{.25}{.25}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (15,5);  % set the bounding box (so we have less surrounding white space)

   \draw(-.5,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfiga{fig/diskInAChannelGride2}{\figWidtha}};
% 
   \draw( 3.5,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/diskInChannelScf10G2StreamLinesAndDisplacement}{\figWidth}};
  \draw(9.5,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/diskInChannelScf1G2StreamLinesAndDisplacement}{\figWidth}};
   % grid:
% \draw[step=1cm,gray] (0,0) grid (15,5);
\end{tikzpicture}
\end{center}
  \caption{Left: composite grid $\Gcd^{(2)}$ for the disk in a channel.
    The green fluid grid adjacent to the interface moves over time while the blue fluid background grid remains fixed.
    The red grid for the solid reference domain also remains fixed over time.
    Streamlines and solid displacement norm for $\scf=10$ and $\scf=1$.
%    Middle and right: fluid pressure and $\| \sigmavs\|$ at times $t=2$ and $t=9$, computed
%       on grid $\Gcb^{(8)}$. \wdh{wdh: add colour bars}
}
  \label{fig:elasticDisk}
\end{figure}
}

Figure~\ref{fig:diskInElasticChannel} shows results for a elastic top surface to the channel.
\textbf{NOTE:} For lighter solids (SCF $< 50$) I had to increase to $z_f = 10 \mu/h$ from $z_f = 5 \mu/h$ to avoid
a low mode ``sloshing'' instability.

{% ----------- Rigid Disk in an ELASTIC channel
%
\newcommand{\figWidtha}{5cm}% width
\newcommand{\trimfiga}[2]{\trimwb{#1}{#2}{.0}{.0}{.0}{.0}}
\newcommand{\figWidth}{7cm}% width
\newcommand{\trimfig}[2]{\trimwb{#1}{#2}{.1}{.1}{.25}{.25}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (15,5);  % set the bounding box (so we have less surrounding white space)

   \draw( 0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfiga{fig/diskInADeformingChannelGride2}{\figWidtha}};
% 
   \draw( 7.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/diskInADeformingChannelScf50G2StreamLinesAndDisplacement}{\figWidth}};
%    \draw(10.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/balloonG8t9p0stress}{\figWidth}};
   % grid:
% \draw[step=1cm,gray] (0,0) grid (15,5);
\end{tikzpicture}
\end{center}
  \caption{Left: composite grid $\Gcd^{(2)}$ for the rigid disk in a deforming channel.
    The green fluid grid adjacent to the interface moves over time while the blue fluid background grid remains fixed.
    The red grid for the solid reference domain also remains fixed over time.
    Streamllines and solid displacement norm for SCF=50.
%    Streamllines and solid displacement norm for SCF=10.
%    Middle and right: fluid pressure and $\| \sigmavs\|$ at times $t=2$ and $t=9$, computed
%       on grid $\Gcb^{(8)}$. \wdh{wdh: add colour bars}
}
  \label{fig:diskInElasticChannel}
\end{figure}
}


{% ----------- TWO ELASTIC DISKS  ------  
%
\newcommand{\figWidtha}{4cm}% width
\newcommand{\trimfiga}[2]{\trimwb{#1}{#2}{.0}{.0}{.0}{.0}}
\newcommand{\figWidth}{8cm}% width
\newcommand{\trimfig}[2]{\trimwb{#1}{#2}{.1}{.1}{.25}{.25}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (15,5);  % set the bounding box (so we have less surrounding white space)

%%   \draw(-.5,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfiga{fig/diskInAChannelGride2}{\figWidtha}};
% 
   \draw( 3.5,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/twoDisksG2Scf10StreamLinesAndDisplacement}{\figWidth}};
%%  \draw(9.5,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/diskInChannelScf1G2StreamLinesAndDisplacement}{\figWidth}};
   % grid:
% \draw[step=1cm,gray] (0,0) grid (15,5);
\end{tikzpicture}
\end{center}
  \caption{FINISH ME. Left: composite grid $\Gcd^{(2)}$ for two deforming disks in a channel.
    The green fluid grid adjacent to the interface moves over time while the blue fluid background grid remains fixed.
    The red grid for the solid reference domain also remains fixed over time.
    Streamlines and solid displacement norm for SCF=10. WE COULD USE DIFFERENT SCF's for the two solids.
%    Middle and right: fluid pressure and $\| \sigmavs\|$ at times $t=2$ and $t=9$, computed
%       on grid $\Gcb^{(8)}$. \wdh{wdh: add colour bars}
}
  \label{fig:elasticDisk}
\end{figure}
}


==> texFiles/oscillatingBubble.tex <==
 \subsection{Oscillating Bubble}

On the outer radius, $r=R,$ the boundary condition is
\begin{align}
\sigmav \nv - (\sigmav \nv)_{\text{ref}} = \gamma \kappa \nv.
\end{align}
$\sigmav \nv$ is the fluid traction and $(\sigmav \nv)_{\text{ref}}$ 
is the `equilibrium' traction.
%
$\kappa$ is the curvature at the interface. 
Define the interface curve parametrically as
\begin{align}
x(\theta) &= (R+u_r(\theta)) \cos(\theta) - u_\theta(\theta) \sin(\theta) \\
y(\theta) &= (R+u_r(\theta)) \sin(\theta) + u_\theta(\theta) \cos(\theta)
\end{align}
%
The curvature is 
\begin{align}
\kappa = \frac{x' y'' - y' x''}{(x'^2 + y'^2)^{3/2}}
\end{align}
%
and the normal is
\begin{align}
\nv &= \frac{1}{\sqrt{x'^2 + y'^2}} 
\left[\begin{array}{c}
y' \\ -x'
\end{array}\right] \\
&= \frac{\ev_r (R + u_r + u_\theta') + \ev_\theta (u_\theta - u_r')}
{\sqrt{x'^2 + y'^2}}
\end{align}
%
Since $u/R \ll 1,$ we will neglect order $(u/R)^2$ terms
and find an asymptotic approximation to the traction condition.
\begin{align}
\frac{x' y'' - y' x''}{R^2} &= 1 + 2 \frac{u_r}{R} + 3 \frac{u_\theta'}{R}
- \frac{u_r''}{R} + O\left(\frac{u^2}{R^2} \right) \\
\frac{x'^2 + y'^2}{R^2} &= 1 + 2 \frac{u_r}{R} + 2 \frac{u_\theta'}{R}
+ O\left(\frac{u^2}{R^2} \right) 
\end{align}
%
Asymptotically, the normal is
\begin{align}
\nv &= \frac{\ev_r (R + u_r + u_\theta') + \ev_\theta (u_\theta - u_r')}
{R \left(1 + 2 \frac{u_r}{R} + 2 \frac{u_\theta'}{R}
+ O\left(\frac{u^2}{R^2} \right)\right)^{1/2}}\nonumber \\
&= \left(1 - \frac{u_r}{R} - \frac{u_\theta'}{R} + ...\right)
\left(\ev_r \left(1 + \frac{u_r}{R} + \frac{u_\theta'}{R}\right) 
+ \ev_\theta \left(\frac{u_\theta}{R} - \frac{u_r'}{R} \right) \right)\nonumber \\
&= \ev_r \left(1 + O\left( \left(\frac{u}{R}\right)^2\right) \right)
+ \ev_\theta \left(\frac{u_\theta}{R} - \frac{u_r'}{R} + ...\right)\nonumber \\
&= \ev_r
+ \ev_\theta \left(\frac{u_\theta}{R} - \frac{u_r'}{R} + ...\right) \nonumber
\end{align}
%
Asymptotically, the right hand side ($\kappa \nv$) is
\begin{align}
\kappa\nv &= \frac{1 + 2 \frac{u_r}{R} + 3 \frac{u_\theta'}{R}
- \frac{u_r''}{R} + ...}
{R \left(1 + 2 \frac{u_r}{R} + 2 \frac{u_\theta'}{R} + ... \right)^{2}} 
\left(\ev_r \left(1 + \frac{u_r}{R} + \frac{u_\theta'}{R}\right) 
+ \ev_\theta \left(\frac{u_\theta}{R} - \frac{u_r'}{R} \right) \right) 
\nonumber \\
 &= \frac{1}{R} \left( 1 + 2 \frac{u_r}{R} + 3 \frac{u_\theta'}{R}
- \frac{u_r''}{R} + ...\right)
\left(1 - 4 \frac{u_r}{R} - 4 \frac{u_\theta'}{R} + ... \right) 
\left(\ev_r \left(1 + \frac{u_r}{R} + \frac{u_\theta'}{R}\right) 
+ \ev_\theta \left(\frac{u_\theta}{R} - \frac{u_r'}{R} \right) \right)
\nonumber \\
&= \frac{1}{R} \left(1 + 2 \frac{u_r}{R} + 3 \frac{u_\theta'}{R}
- \frac{u_r''}{R}- 4 \frac{u_r}{R} - 4 \frac{u_\theta'}{R}
+ \frac{u_r}{R} + \frac{u_\theta'}{R} +...\right) \ev_r
+ \frac{1}{R} \left(\frac{u_\theta}{R} - \frac{u_r'}{R}+... \right) \ev_\theta
\nonumber \\
&= \frac{1}{R} \left(1 - \frac{u_r}{R} 
- \frac{u_r''}{R}
+...\right)
 \ev_r
+ \frac{1}{R} \left(\frac{u_\theta}{R} - \frac{u_r'}{R} +...\right) \ev_\theta 
\nonumber \\
&= \frac{1}{R} \ev_r
+\frac{1}{R} \left(- \frac{u_r}{R} 
- \frac{u_r''}{R} 
+...\right)
 \ev_r
+ \frac{1}{R} \left(\frac{u_\theta}{R} - \frac{u_r'}{R} +...\right) \ev_\theta
\nonumber 
\end{align}
%
The normal is equivalent to $\ev_r + \tilde{\nv}$, 
where $\tilde{\nv}$ is a small correction.
Since the traction is also small,
the fluid traction is asymptotically equivalent to
\begin{align}
\sigmav \nv = \sigmav \left(\ev_r +  
\tilde{\nv} \right)
= \left[\begin{array}{c} \sigma_{rr} \\ \sigma_{r\theta} \end{array} \right]
+ O \left( \left(\frac{u}{R} \right)^2 \right)
\end{align}
%
The linearized boundary conditions are 
\begin{align}
-p + 2 \mu \frac{\partial v_r}{\partial r}
&= \frac{\gamma}{R} \left(- \frac{u_r}{R} 
- \frac{u_r''}{R}
\right) \\
\mu \left( \frac{1}{r} \frac{\partial v_r}{\partial \theta}
+\frac{\partial v_\theta}{\partial r}
- \frac{v_\theta}{r} \right)
&= \frac{\gamma}{R} \left(\frac{u_\theta}{R} - \frac{u_r'}{R} \right).
\end{align}
%
In hat variables, this is equivalent to
\begin{align}
-\hat{p} + 2 \mu \hat{v_r}'
&= -\frac{\gamma}{i \omega R^2} \hat{v}_r (n^2 - 1)\\
\mu \left( \frac{i n}{R} \hat{v}_r
+\hat{v}_\theta'
- \frac{\hat{v}_\theta}{R} \right)
&= -\frac{\gamma}{i \omega R^2} 
\left( \hat{v}_\theta - i n \hat{v}_r \right).
\end{align}


==> texFiles/overtureNumericalResults.tex <==
\clearpage
\section{Composite grid numerical results}

\input texFiles/elasticPistonCompositeGrid

\input texFiles/radialPiston


==> texFiles/radialElasticPistonOld.tex <==
\section{Exact solutions in polar coordinates}

An incompressible fluid and elastic solid 
are considered in polar coordinates.
Let $v_r$ and $v_\theta$ be the radial and circumferential components
of the fluid velocity, respectively.
The fluid continuity equation is given by
\begin{align}
\frac{1}{r} \frac{\partial (r v_r)}{\partial r} + 
\frac{1}{r} \frac{\partial v_\theta}{\partial \theta} = 0.
\end{align}
%
The fluid momentum equations are given by
\begin{align}
\rho \frac{\partial v_r}{\partial t}
+ \rho \left(v_r \frac{\partial v_r}{\partial r} 
+ \frac{v_\theta}{r} \frac{\partial v_r}{\partial \theta}
- \frac{1}{r} v_\theta^2 \right)
+ \frac{\partial p}{\partial r} &= 
\mu \left( \frac{1}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_r}{\partial r}\right) 
+ \frac{1}{r^2} \frac{\partial^2 v_r}{\partial \theta^2}
- \frac{v_r}{r^2} 
- \frac{2}{r^2} \frac{\partial v_\theta}{\partial \theta}
\right) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rho \frac{\partial v_\theta}{\partial t}
+ \rho \left(v_r \frac{\partial v_\theta}{\partial r} 
+ \frac{v_\theta}{r} \frac{\partial v_\theta}{\partial \theta}
- \frac{1}{r} v_r v_\theta \right)
+ \frac{1}{r} \frac{\partial p}{\partial \theta} &= 
\mu \left( \frac{1}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_\theta}{\partial r}\right) 
+ \frac{1}{r^2} \frac{\partial^2 v_\theta}{\partial \theta^2}
+ \frac{2}{r^2} \frac{\partial v_r}{\partial \theta}
- \frac{v_\theta}{r^2}
\right).
\end{align}
%
The fluid stress tensor components are
\begin{align}
\sigma_{rr} &= -p + 2 \mu \frac{\partial v_r}{\partial r} \\
\sigma_{r\theta} &= \mu \left(\frac{1}{r} \frac{\partial v_r}{\partial \theta} + 
  \frac{\partial v_\theta}{\partial r}
  - \frac{v_\theta}{r} \right)\\
\sigma_{\theta\theta} &= -p + \frac{2\mu }{r} \left( \frac{\partial v_\theta}{\partial \theta} + v_r \right).
\end{align}
%
Let $\us_r$ and $\us_\theta$ be the radial and circumferential 
components of the solid displacement.
The solid momentum equations are
\begin{align}
\rhos \frac{\partial^2 \us_r}{\partial t^2} &= \frac{\partial \sigmas_{rr}}{\partial r} 
+ \frac{1}{r} \frac{\partial \sigmas_{r\theta}}{\partial \theta} 
+ \frac{1}{r} \left(\sigmas_{rr} - \sigmas_{\theta\theta} \right)
+ \bs_r \\
\rhos \frac{\partial^2 \us_\theta}{\partial t^2} &= \frac{\partial \sigmas_{r\theta}}{\partial r}
+ \frac{1}{r} \frac{\partial \sigmas_{\theta\theta}}{\partial \theta} 
+ \frac{2}{r} \sigmas_{r \theta} 
+ b_\theta.
\end{align}
% 
% The terms of the stress tensor are computed
% \begin{align}
% \grad \cdot \usv &= \frac{1}{r} \frac{\partial (r \us_r)}{ \partial r}
% + \frac{1}{r} \frac{\partial \us_\theta}{\partial \theta}.
% \end{align}
% %
% \begin{align}
% \epsilonsv = 
% \frac{1}{2} \left( \grad \usv + \left(\grad \usv \right)^T\right) &= 
% \left[\begin{array}{cc}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{\partial \us_r}{\partial r} &
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{1}{2} \left( \frac{1}{r} \frac{\partial \us_r}{\partial \theta} 
% + \frac{\partial \us_\theta}{\partial r}
% - \frac{\us_\theta}{r} \right) \\
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{1}{2} \left( \frac{1}{r} \frac{\partial \us_r}{\partial \theta} 
% + \frac{\partial \us_\theta}{\partial r}
% - \frac{\us_\theta}{r} \right) &
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \frac{1}{r} \left(\frac{\partial \us_\theta}{\partial \theta} + \us_r  \right)
% \end{array}\right]
% \end{align}
%
The solid stress components are
\begin{align}
\sigmas_{rr} &= \lambdas \left(\frac{1}{r} \frac{\partial (r \us_r)}{ \partial r}
+ \frac{1}{r} \frac{\partial \us_\theta}{\partial \theta} \right) 
+ 2 \mus \frac{\partial \us_r}{\partial r} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{r\theta} &= \mus \left( \frac{1}{r} \frac{\partial \us_r}{\partial \theta} 
+ \frac{\partial \us_\theta}{\partial r}
- \frac{\us_\theta}{r} \right) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{\theta\theta} &= \lambdas \left(\frac{1}{r} \frac{\partial (r \us_r)}{ \partial r}
+ \frac{1}{r} \frac{\partial \us_\theta}{\partial \theta} \right) 
+ \frac{2 \mus }{r} \left(\frac{\partial \us_\theta}{\partial \theta} + \us_r  \right).
\end{align}



\subsection{Axial symmetry}

We look for solutions in which derivatives with respect to $\theta$
are zero.
The fluid continuity equation simplifies to
\begin{align}
\frac{\partial (r v_r)}{\partial r} &= 0 \nonumber 
\end{align}
%
Using this, an expression for $v_r$ con be obtained in terms of a
single function of time, $f(t)$.
\begin{align}
r v_r &= f(t) \nonumber \\
v_r(r,t) &= \frac{1}{r} f(t).
\end{align}
%
A boundary condition is required to find $f(t).$
The momentum equations simplify to
\begin{align}
\rho \frac{\partial v_r}{\partial t}
+ \rho \left(v_r \frac{\partial v_r}{\partial r} 
- \frac{1}{r} v_\theta^2 \right)
+ \frac{\partial p}{\partial r} &= 
\frac{\mu}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_r}{\partial r}\right) 
- \frac{\mu}{r^2} v_r \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rho \frac{\partial v_\theta}{\partial t}
+ \rho \left(v_r \frac{\partial v_\theta}{\partial r} 
- \frac{1}{r} v_r v_\theta \right)
\phantom{\;\frac{\partial p}{\partial r}}
 &= 
 \frac{\mu}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_\theta}{\partial r}\right) 
- \frac{\mu}{r^2} v_\theta
\end{align}
%
These equations are used to determine $p$ and $v_\theta.$ 
The solid momentum equations simplify to
\begin{align}
\rhos \frac{\partial^2 \us_r}{\partial t^2} &= \frac{\partial \sigmas_{rr}}{\partial r} 
+ \frac{1}{r} \left(\sigmas_{rr} - \sigmas_{\theta\theta} \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\rhos \frac{\partial^2 \us_\theta}{\partial t^2} &= \frac{\partial \sigmas_{r\theta}}{\partial r}
+ \frac{2}{r} \sigmas_{r \theta}.
\end{align}
%
The solid stress tensor simplifies to
\begin{align}
\sigmas_{rr} &=  \frac{\lambdas}{r} \frac{\partial (r \us_r)}{ \partial r}
+ 2 \mus \frac{\partial \us_r}{\partial r} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{r\theta} &= \mus \left( 
\frac{\partial \us_\theta}{\partial r}
- \frac{\us_\theta}{r} \right) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\sigmas_{\theta\theta} &= \frac{\lambdas}{r} \frac{\partial (r \us_r)}{ \partial r}
+ \frac{2 \mus }{r} \us_r  .
\end{align}
%
The solid equations simplify to wave equations.
\begin{align}
 \frac{\partial^2 \us_r}{\partial t^2} &=
\cp^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_r)}{\partial r} \right) \\
\frac{\partial^2 \us_\theta}{\partial t^2} &=
\cs^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_\theta)}{\partial r} \right).
\end{align}

\subsubsection{Radial elastic piston solution}

Consider motions only in the radial direction,
($v_\theta = 0$ and $\us_\theta = 0$).
The fluid momentum equation becomes a quadrature for the pressure.
\begin{align}
\frac{\rho}{r} f'(t)
- \frac{\rho}{r^3} f(t)^2 
+ \frac{\partial p}{\partial r} &= 
0   \nonumber \\
\frac{\partial p}{\partial r} &= 
\frac{\rho}{r^3} f(t)^2 
-\frac{\rho}{r} f'(t).
\end{align}
%
The pressure is obtained by integration
\begin{align}
p(r,t) &= g(t;R)
-\frac{\rho}{2r^2} f(t)^2 
-\rho f'(t) \log\left( \frac{r}{R} \right)  .
\end{align}
%
Another boundary condition for $p$ is needed to determine $g(t;R).$
The arbitrary constant $R$ was introduced to simplify the expression.

In the solid, search for solutions of the form
\begin{align}
\us_r(r,t) = \hat{\us}_r(r) \cos(\cp k t +\phi). \nonumber
\end{align}
%
Plug this in to the equations to obtain
\begin{align}
- k^2 \hat{\us}_r &= \frac{d }{d r} \left( \frac{d \hat{\us}_r}{d r} + \frac{1}{r} \hat{\us}_r \right) \nonumber \\
0 &= \hat{\us}_r'' + \frac{1}{r} \hat{\us}_r'
+ k^2 \hat{\us}_r - \frac{1}{r^2} \hat{\us}_r \nonumber \\
0 &= r^2 \hat{\us}_r'' + r \hat{\us}_r'
+ (k^2 r^2 - 1) \hat{\us}_r.
\end{align}
%
This is the Bessel equation of order 1. The solution is
\begin{align}
\us_r(r,t) = \left(A J_1(kr) + B Y_1(kr)\right) \cos(\cp k t + \phi).
\end{align}

The fluid is in the domain $R+\us_r(R,t) < r < R_0$ and the solid reference 
domain is $0 \le \bar{r} < R.$ The solid displacement must be finite at $r=0,$
therefore the coefficient of $Y_1$ must be 0. The solution in the fluid and solid domains
are given by
\begin{align}
v_r(r,t) &= \frac{1}{r} f(t) \\
p(r,t) &= g(t)
-\frac{\rho}{2r^2} f(t)^2 
-\rho f'(t) \log\left( \frac{r}{R_I(t)} \right)   \\
\us_r(\bar{r},t) &= \us_0 J_1(k\bar{r})  \cos(\cp k t + \phi),
\end{align}
%
where $R_I(t) = R+\us_r(R,t).$
The pressure is supplied to be $p_0(t)$ at $r=R_0.$ 
Instead of solving the general problem, we find $p_0$ for a given
solution to the FSI problem with boundary conditions
\begin{align}
v_r(R+\us_r(R,t),t) &= \partial_t \us_{r}(R,t) \\
\sigma_{rr}(R+\us_r(R,t),t) &= \sigmas_{rr}(R,t) .
\end{align}
%
The stress matching condition is equivalent to
\begin{align}
-p + 2 \mu \frac{\partial v_r}{\partial r} = 
\lambdas \left(\frac{1}{\bar{r}} \frac{\partial (\bar{r} \us_r)}{ \partial \bar{r}}
+ \frac{1}{\bar{r}} \frac{\partial \us_\theta}{\partial \theta} \right) 
+ 2 \mus \frac{\partial \us_r}{\partial \bar{r}},
\quad 
r = R_I(t),\; \bar{r} = R.
\end{align}
%
Solve for $f(t)$ using velocity matching condition.
\begin{align}
v_I &= -\us_0{{ J}_{1}\left(k{R}\right)}\cp k\sin
 \left( \cp kt+\phi \right) 
= \frac{f(t)}{R+\us_0 J_1(k R) \cos(\cp k t + \phi)}. 
\nonumber
\end{align}
%
The solution is
\begin{align}
f(t) &= -\left(R+\us_0 J_1(k R) \cos(\cp k t + \phi) \right) 
\us_0{{ J}_{1}\left(k{R}\right)}\cp k\sin
 \left( \cp kt+\phi \right)  .
\end{align}
%
Solve for $g(t)$ using the traction matching condition
\begin{align}
\sigma_I =\;& \frac{\us_0}{R} \left(k R (\lambdas + 2 \mus) J_0(kR)
 - 2 \mus J_1(kR) \right) \cos(\cp k t + \phi) 
=-g(t) + \frac{1}{2 R_I(t)^2} \left(\rho f(t)^2 - 2 \mu f(t) \right)
\nonumber
\end{align}
%
The solution is
\begin{align}
g(t) = \frac{1}{2 R_I(t)^2} \left(\rho f(t)^2 - 4 \mu f(t) \right)
- \frac{\us_0}{R} \left(k R (\lambdas + 2 \mus) J_0(kR)
 - 2 \mus J_1(kR) \right) \cos(\cp k t + \phi) 
\end{align}
%
See \texttt{/CG/fibr/codes/testSolutions/radialElasticPiston}
for details.

\subsubsection{Pure shear solution}

Consider $v_r = 0$ and $\us_r = 0.$ The equations in the fluid and solid are
\begin{align}
- \frac{\rho}{r} v_\theta^2 + \frac{\partial p}{\partial r} &= 0 \\
\rho \frac{\partial v_\theta}{\partial t}
 &= 
 \frac{\mu}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_\theta}{\partial r}\right) 
- \mu \frac{v_\theta}{r^2} \\
\frac{\partial^2 \us_\theta}{\partial t^2} &=
\cs^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_\theta)}{\partial r} \right).
\end{align}
%
Look for solutions of the form
\begin{align}
v_\theta(r,t) = \hat{v}_\theta(r) e^{i \omega t}, \quad
\us_\theta(r,t) = \hat{\us}_\theta(r) e^{i \omega t}.\nonumber 
\end{align}
%
The fluid and solid equations simplify to
\begin{align}
0 &= r^2 \hat{v}_\theta'' + r \hat{v}_\theta' + (\alpha^2 r^2 - 1) \hat{v}_\theta \\
0 &= r^2 \hat{\us}_\theta'' + r \hat{\us}_\theta' + (\beta^2 r^2 - 1) \hat{\us}_\theta 
\end{align}
%
where
\begin{align}
\alpha^2 = - \frac{i \rho \omega}{\mu}, \quad \beta^2 = \frac{\omega^2}{\cs^2}.
\end{align}
%
The solutions for the transformed variables are
\begin{align}
\hat{v}_\theta(r) &= A J_1(\alpha r) + B Y_1(\alpha r) \\
\hat{\us}_\theta(r) &= C J_1(\beta r) + D Y_1(\beta r).
\end{align}
%
The general solutions are
\begin{align}
{v}_\theta(r,t) &= \left(A J_1(\alpha r) + B Y_1(\alpha r)\right) e^{i\omega t} \\
{\us}_\theta(r,t) &= \left(C J_1(\beta r) + D Y_1(\beta r)\right) e^{i\omega t}.
\end{align}
%
The solid domain is $0 < r < R$ and the fluid domain is 
$R < r < R_0.$ Note that this is an approximation. See the end of this
section.
Since the solid displacement must be finite at $r=0,$ we have $D=0.$
The fluid and solid solutions must obey the matching conditions
\begin{align}
v_\theta(R,t) &= \frac{\partial \us_\theta}{\partial t}(R,t) \\
\sigma_{rr}(R,t) &= \sigmas_{rr}(R,t) \label{eq:srrMatching} \\
\sigma_{r\theta}(R,t) &= \sigmas_{r\theta}(R,t) .
\end{align}
%
A boundary condition is also required at $r=R_0.$ We impose the no-slip condition
\begin{align}
v_\theta(R_0,t) = 0.
\end{align}
%
Since $\sigmas_{rr} = 0$ and the only contribution to $\sigma_{rr}$
is from the fluid pressure,
equation \eqref{eq:srrMatching} simplifies to
\begin{align}
p(R,t) = 0.
\end{align}
%
The solution for the pressure is thus given by
\begin{align}
p(r,t) = \rho \int_R^r \frac{v_\theta(s,t)^2}{s} \; ds.
\end{align}
%
The other three interface/boundary conditions result in an eigenvalue problem for 
$\omega.$ The velocity matching condition is
\begin{align}
A J_1(\alpha R) + B Y_1(\alpha R) = i \omega C J_1 (\beta R) .\nonumber
\end{align}
%
The stress matching condition is
\begin{align}
\frac{\mu}{r} \left(\frac{\partial v_\theta}{\partial r} - \frac{v_\theta}{r} \right)
 &= 
\frac{\mus}{r} \left(\frac{\partial \us_\theta}{\partial r} - \frac{\us_\theta}{r} \right)
\nonumber \\
\frac{\mu}{r} \left(
A \left(J_1'(\alpha R) - \frac{J_1(\alpha R)}{R} \right)
+B \left(Y_1'(\alpha R) - \frac{Y_1(\alpha R)}{R} \right)
 \right)
&= 
\frac{\mu}{r} 
C \left(J_1'(\beta R) - \frac{J_1(\beta R)}{R} \right). \nonumber
\end{align}
%
The no-slip condition is
\begin{align}
A J_1(\alpha R_0) + B J_2(\alpha R_0) = 0 \nonumber
\end{align}
%
These conditions are written as a matrix system
\begin{align}
\Mv(\omega) \av = 0, 
\end{align}
%
where
\begin{align}
\Mv(\omega) =  \left[ \begin {array}{ccc} {{\sl J}_{1}\left(\alpha\,{R}\right)
}&{{\sl Y}_{1}\left(\alpha\,{R}\right)}&-i{{\sl J}_{1}\left(
\beta\,{R}\right)}\omega\\ \noalign{\medskip}{{\sl J}_{1}\left(
\alpha\,{R_0}\right)}&{{\sl Y}_{1}\left(\alpha\,{R_0}\right)}&0
\\ \noalign{\medskip}{\frac {{{\sl J}_{0}\left(\alpha\,{R}
\right)}{R}\,\alpha\,\mu-2\,{{\sl J}_{1}\left(\alpha\,{R}
\right)}\mu}{{{R}}^{2}}}&{\frac {{{\sl Y}_{0}\left(\alpha\,{
R}\right)}{R}\,\alpha\,\mu-2\,{{\sl Y}_{1}\left(\alpha\,{
R}\right)}\mu}{{{R}}^{2}}}&{\frac {-{{\sl J}_{0}\left(\beta\,{
R}\right)}{R}\,\beta\,{\mus}+2\,{{\sl J}_{1}\left(
\beta\,{R}\right)}{\mus}}{{{R}}^{2}}}\end {array}
 \right] \nonumber
\end{align}
%
and $\av = [A,B,C]^T.$ $\omega$ is a solution to $\det(\Mv(\omega))=0.$
For the parameters
\begin{align}
R = 1,\quad R_0 = 2,\quad \rho = 1,\quad \mu = 10,\quad \rhos = 10,\quad \cs = 1,
\end{align}
%
a solution was found to be
\begin{align*}
\omega &= \phantom{-} 1.4841084914290283\text{e}+01 +  
\phantom{-}7.0873356446257796\text{e}-01 i\\
A     &= -1.4894197324861366\text{e}-01 + -2.4826496514057889\text{e}-01 i\\
B     &= -2.7073357963903405\text{e}-01 +  
\phantom{-}1.3818364548148002\text{e}-01 i\\
C     &= \phantom{-} 2.0000000000000000\text{e}-01 +  
\phantom{-}0.0000000000000000\text{e}+00 i
\end{align*}
%
See \texttt{/CG/fibr/codes/testSolutions/radialShear}
for details.

In reality, the deformation of the solid also causes warping.
Consider the solid deformation.
\begin{align*}
\ysv = \usv + \xsv = (\us_r + \rs) \hat{\rv} + \us_\theta \hat{\thetav}.
\end{align*}
%
Since $\us_r = 0,$
\begin{align*}
\ysv &= \rs \hat{\rv} + \us_\theta \hat{\thetav} \\
&= (\rs \cos \theta - \us_\theta \sin \theta) \hat{\xv}_1
+(\rs \sin \theta + \us_\theta \cos \theta) \hat{\xv}_2
\end{align*}
%
Therefore,
\begin{align*}
\|\ysv\|_2^2 = \rs^2 + \us_\theta^2
\end{align*}
%
The relative error of the linearized boundary is
\begin{align*}
\frac{\sqrt{R^2 + \us_\theta^2} - R}{R} \sim
\frac{1}{2} \left(\frac{\us_\theta}{R} \right)^2 + 
O \left( \left(\frac{\us_\theta}{R} \right)^4 \right).
\end{align*}

\section{Vibrational Modes}

\subsection{Fluid}

Consider small disturbance solutions of the form
\begin{align*}
v_r(r,\theta,t) = \hat{v}_r(r) e^{i (n \theta - \omega t)}, \quad
v_\theta(r,\theta,t) = \hat{v}_\theta(r) e^{i (n \theta - \omega t)} , \quad
p(r,\theta,t) = \hat{p}(r) e^{i (n \theta - \omega t)} .\nonumber 
\end{align*}
%
By substitution (neglecting convection terms), the equations become
\begin{align}
\frac{1}{r} (r \hat{v}_r)' + \frac{i n}{r} \hat{v}_\theta &= 0  
\label{eq:smallDistContinuity} \\
-i \omega \rho \hat{v}_r + \hat{p}' &= \mu 
\left(\frac{1}{r} (r \hat{v}_r')' 
- \frac{n^2}{r^2} \hat{v}_r 
- \frac{\hat{v}_r}{r^2} 
- \frac{2 i n}{r^2} \hat{v}_\theta
\right) \label{eq:smallDistRadialMomentum}\\
-i \omega \rho \hat{v}_\theta + \frac{i n}{r} \hat{p}' &= \mu
\left(\frac{1}{r} (r \hat{v}_\theta')'
- \frac{n^2}{r^2} \hat{v}_\theta
+ \frac{2 i n}{r^2} \hat{v}_r
- \frac{\hat{v}_\theta}{r^2} 
\right).\label{eq:smallDistCircumMomentum}
\end{align}
%
Consider equation \eqref{eq:smallDistRadialMomentum}. The equation can 
be manipulated to look like a Bessel equation with a forcing term.
\begin{align}
-\frac{i \omega \rho}{\mu} r^2 \hat{v}_r + \frac{r^2}{\mu} \hat{p}' &= 
r^2 \hat{v}_r'' + r\hat{v}_r'
- n^2 \hat{v}_r 
- \hat{v}_r
-2 i n \hat{v}_\theta \nonumber\\
\frac{r^2 }{\mu} \hat{p}'
+ 2 i n \hat{v}_\theta
&= r^2 \hat{v}_r'' + r \hat{v}_r' + (\lambda^2 r^2 - \alpha^2) \hat{v}_r 
\label{eq:besselVr}
\end{align}
%
where
\begin{align}
\lambda^2 = \frac{i \omega \rho}{\mu}, \quad \alpha^2 = n^2 + 1.\nonumber
\end{align}
%
Similarly for equation \eqref{eq:smallDistCircumMomentum}, the equation becomes
\begin{align}
\frac{i n r }{\mu} \hat{p}
- 2 i n \hat{v}_r
&= r^2 \hat{v}_\theta'' + r \hat{v}_\theta' + (\lambda^2 r^2 - \alpha^2) \hat{v}_\theta .
\label{eq:besselVtheta}
\end{align}
%
The pressure satisfies the Laplace equation, given by
\begin{align}
\frac{\partial^2p}{\partial r^2} 
+ \frac{1}{r} \frac{\partial p}{\partial r}
+ \frac{1}{r^2} \frac{\partial^2 p}{\partial \theta^2}
&= 0 \nonumber\\
\hat{p}'' 
+ \frac{1}{r} \hat{p}'
- \frac{n^2}{r^2} \hat{p} &= 0.
\end{align}
%
We search for solutions with the form
\begin{align}
\hat{p}(r) = p_0 \left(\frac{r}{R} \right)^q.\nonumber
\end{align}
%
The equation reduces to an algebraic condition on $q,$ given by
\begin{align*}
q (q-1) + q - n^2 &= 0 \\
q^2 &= n^2 \\
q &= \pm n.
\end{align*}
%
Therefore,
\begin{align}
\hat{p}(r) = p_0 \left(\frac{r}{R} \right)^n + A \left(\frac{r}{R} \right)^{-n}
\nonumber
\end{align}
% 
Since $p$ is finite at $r=0,$ $A=0.$
\begin{align}
\hat{p}(r) = p_0 \left(\frac{r}{R} \right)^n 
\end{align}
%
Equations \eqref{eq:besselVr} and \eqref{eq:besselVtheta} are 
forced, coupled Bessel equations. The continuity equation \eqref{eq:smallDistContinuity}
is used to eliminate $\hat{v}_\theta$ from \eqref{eq:besselVr}.
\begin{align*}
(r \hat{v}_r)' + i n \hat{v}_\theta &= 0 \\
\hat{v}_r + r \hat{v}_r' + i n \hat{v}_\theta &= 0 \\
\hat{v}_\theta &= -\frac{1}{in} \left(\hat{v}_r + r \hat{v}_r' \right) \\
r^2 \hat{v}_r'' + r \hat{v}_r' + (\lambda^2 r^2 - \alpha^2) \hat{v}_r
&= \frac{r^2}{\mu} \hat{p} '
- 2 i n \left( \frac{1}{in} \left(\hat{v}_r + r \hat{v}_r' \right)\right)\\
r^2 \hat{v}_r'' + r \hat{v}_r' + (\lambda^2 r^2 - \alpha^2) \hat{v}_r
&= \frac{r^2}{\mu} \hat{p} '
- 2 \hat{v}_r - 2 r \hat{v}_r' \\
r^2 \hat{v}_r'' + 3 r \hat{v}_r' + (\lambda^2 r^2 - \alpha^2 + 2) \hat{v}_r
&= \frac{r^2}{\mu} \hat{p}'  \\
r^2 \hat{v}_r'' + 3 r \hat{v}_r' + (\lambda^2 r^2 - \beta^2) \hat{v}_r
&= p_0 \frac{n r^{n+1}}{\mu R^n}
\end{align*}
%
where
\begin{align*}
\beta^2 = \alpha^2 - 2
\end{align*}
%
The solution to a generalized Bessel equation of the form
\begin{align*}
r^2 w'' + (1-2a)r w' + (b^2 c^2 r^{2c} + a^2 - \gamma^2 c^2) w = 0
\end{align*}
%
is 
\begin{align*}
w = c_1 r^a J_\gamma (b r^c) + c_2 r^a Y_\gamma (b r^c).
\end{align*}
%
For our case,
\begin{align}
a = -1, \quad b = \lambda, \quad c = 1, \quad \gamma^2 = \beta^2 + 1 = n^2.
\end{align}
%
Therefore the solution is
\begin{align}
\hat{v}_r(r) = \frac{1}{r} \left( c_1 J_n (\lambda r) + c_2 Y_n (\lambda r) \right)
+ \tilde{v}_r(r).
\end{align}
%
where $\tilde{v}_r$ is the particular solution. Variation of parameters is used
to find $\tilde{v}_r.$ Define 
\begin{align*}
v_1(r) = \frac{1}{r} J_\gamma(\lambda r), \quad 
v_2(r) = \frac{1}{r} Y_\gamma(\lambda r), \quad
W(v_1,v_2) = v_1 v_2' - v_2 v_1', \quad
g(r) = p_0\frac{n r^{n-1}}{\mu R^{n}}.
\end{align*}
%
then
\begin{align}
\tilde{v}_r(r) = - v_1(r) 
\int_0^r \frac{v_2(s) g(s)}{W(v_1(s),v_2(s))} \; d s
+ v_2(r)
\int_0^r \frac{v_1(s) g(s)}{W(v_1(s),v_2(s))} \; d s.
\end{align}
%
The order of the Bessel equation, $\gamma$, simplifies to
\begin{align*}
\gamma^2 = \beta^2 + 1 = \alpha^2 - 2 + 1 = n^2 + 1 - 2 + 1 = n^2.
\end{align*}
%
The Wronskian simplifies to
\begin{align}
W(v_1,v_2) = \frac{\lambda}{r^2} \left(J_{n+1}(\lambda r) Y_n(\lambda r)
- J_{n}(\lambda r) Y_{n+1}(\lambda r) \right). \nonumber
\end{align}
%
Instead Abel's formula can be used,
\begin{align}
W(v_1,v_2) = C e^{-\int \frac{3}{r} \; dr} = C e^{- 3 \log r} = \frac{C}{r^3}.
\end{align}
%
Therefore the particular solution is given by
\begin{align}
\tilde{v}_r(r) = \frac{n p_0}{\lambda \mu R^n r} \bigg{(} \;&
- \int_0^r \frac{Y_{n}(\lambda s) J_{n}(\lambda r) s^n}
{J_{n+1}(\lambda s) Y_n(\lambda s)
- J_{n}(\lambda s) Y_{n+1}(\lambda s)} \; d s \nonumber \\
&+ \int_0^r \frac{J_{n}(\lambda s) Y_{n}(\lambda r) s^n}
{J_{n+1}(\lambda s) Y_n(\lambda s)
- J_{n}(\lambda s) Y_{n+1}(\lambda s)} \; d s \bigg{)}.
\end{align}
%
The solution for $\hat{v}_\theta$ is obtained using the continuity equation.
\begin{align}
\hat{v}_\theta(r) = \frac{i c_1}{ n r} \left( 
   n J_n (\lambda r) - \lambda r J_{n+1}(\lambda r) \right)
 +\frac{i c_2}{ n r}
 \left( n Y_n (\lambda r) - \lambda r Y_{n+1}(\lambda r) \right)
+ \tilde{v}_\theta(r)
\end{align}
%
The particular solution is given by
\begin{align}
\tilde{v}_\theta(r) = 
\frac{i p_0}{\lambda \mu R^n r} \bigg{(} \;&
- \int_0^r \frac{Y_{n}(\lambda s) 
(n J_n(\lambda r) - J_{n+1}(\lambda r) \lambda r) 
s^n}
{J_{n+1}(\lambda s) Y_n(\lambda s)
- J_{n}(\lambda s) Y_{n+1}(\lambda s)} \; d s \nonumber \\
&+ \int_0^r \frac{J_{n}(\lambda s) 
(n Y_{n}(\lambda r) - Y_{n+1}(\lambda r) \lambda r)
s^n}
{J_{n+1}(\lambda s) Y_n(\lambda s)
- J_{n}(\lambda s) Y_{n+1}(\lambda s)} \; d s \bigg{)}.
\end{align}

\subsection{Solid}

Search for solutions of the form
\begin{align}
\us_r(r,\theta,t) = \hat{\us}_r(r) e^{i (n \theta - \omega t)}, \quad
\us_\theta(r,\theta,t) = \hat{\us}_\theta(r) e^{i (n \theta - \omega t)}.
\nonumber 
\end{align}
% 
The solid equations reduce to ODEs for $\hat{\us}_r$ and $\hat{\us}_\theta.$
\begin{align}
r^2 \hat{\us}_r'' + r \hat{\us}_r' +
\left(\frac{\omega^2 \rhos }{\lambdas + 2\mus} r^2
- \frac{\lambdas + 2 \mus + n^2 \mus}{\lambdas + 2 \mus} \right) \hat{u}_r
&=
\frac{in (3 \mus + \lambdas)}{\lambdas + 2 \mus} \hat{\us}_\theta
- \frac{in r (\mus + \lambdas)}{\lambdas + 2 \mus} \hat{\us}_\theta'
\nonumber \\
r^2 \hat{\us}_\theta'' + r \hat{\us}_\theta' +
\left(\frac{\omega^2 \rhos }{\mus} r^2
- \frac{\mus + n^2 (\lambdas + 2\mus)}{\mus} \right) \hat{u}_\theta
&=
- \frac{in (3 \mus + \lambdas)}{\mus} \hat{\us}_r
- \frac{in r (\mus + \lambdas)}{\mus} \hat{\us}_r' \nonumber
\end{align}
%
The longitudinal and shear wave speeds are defined as
\begin{align}
\cp^2 = \frac{\lambdas + 2 \mus}{\rhos}, \quad
\cs^2 = \frac{\mus}{\rhos}.\nonumber 
\end{align}
%
Using this definition,
\begin{align}
r^2 \hat{\us}_r'' + r \hat{\us}_r' +
\left( \frac{\omega^2}{\cp^2} r^2
- \left(1 + \frac{\cs^2}{\cp^2} n^2\right) \right) \hat{u}_r
&=
in \left(1 + \frac{\cs^2}{\cp^2} \right)\hat{\us}_\theta
- in r \left(1 -  \frac{ \cs^2}{\cp^2} \right)\hat{\us}_\theta'
 \\
r^2 \hat{\us}_\theta'' + r \hat{\us}_\theta' +
\left(\frac{\omega^2 }{\cs^2} r^2
- \left(1 + \frac{\cp^2}{\cs^2}n^2\right) \right) \hat{u}_\theta
&=
- in \left(1 + \frac{\cp^2}{\cs^2} \right)\hat{\us}_r
- inr \left(\frac{\cp^2}{\cs^2} - 1\right) \hat{\us}_r' 
\end{align}
%
As a sanity check, this equation agrees with the one obtained in the 
axial-symmetry case when $n=0$ (order 1 Bessel equations).

\section{Balloon Problem}

The fluid domain goes from $R_0 < r < R_I(t).$ At $R_0,$ fluid is being pumped into 
domain at a given mass rate, $\dot{m}(t)$ with units of 
mass per time per unit length. This relates to the velocity through
\begin{align}
\dot{m}(t) = 2 \pi \rho v_0(t) R_0.
\end{align}
%
General solution
\begin{align}
v_r(r,t) &= \frac{f(t)}{r} \\
p(r,t) &= g(t) - \frac{\rho}{2 r^2} f(t)^2 - \rho f'(t) \log \left( \frac{r}{R_I(t)} \right)
\end{align}
%
Use BC to determine $f(t)$
\begin{align}
v_r(R_0,t) &= \frac{f(t)}{R_0} = \frac{\dot{m}(t)}{2 \pi R_0 \rho }
\quad \rightarrow
\quad
f(t) = \frac{\dot{m}(t)}{2 \pi \rho}.
\end{align}
%
Therefore
\begin{align}
v_r(r,t) = \frac{\dot{m}(t)}{2 \pi r \rho}
\end{align}
%
and
\begin{align}
p(r,t) &= g(t) - \frac{\dot{m}(t)^2}{8 \pi^2 r^2 \rho}
- \frac{\ddot{m}(t)}{2 \pi} \log \left(\frac{r}{R_I(t)} \right)
\end{align}
%
The solid reference domain goes from $R < r < R + \Delta r.$
The solid equation is
\begin{align}
% \rhos \frac{\partial^2 \us_r}{\partial t^2} =
% \frac{\partial \sigmas_{rr} }{\partial r} 
% + \frac{1}{r} \left(\sigmas_{rr} - \sigmas_{\theta\theta} \right).
  \frac{\partial^2 \us_r}{\partial t^2} =
\cp^2 \frac{\partial}{\partial r} 
\left(\frac{1}{r} \frac{\partial (r \us_r)}{\partial r} \right)
\end{align}
%
Since $\Delta r / R \ll 1,$ we are more interested in what happens with the solution
in the average sense
\begin{align}
\tilde{u}_r(t) = \frac{1}{\dr} \int_R^{R+\dr} u(r,t) \;  dr
\end{align}
%
By integrating the equations over the solid domain, the equations become
\begin{align}
% \rhos \frac{d^2 \tilde{u}_r}{d t^2}
% &= \frac{\sigmas_{rr}(R+\dr,t) - \sigmas_{rr}(R,t)}{\dr}
% + \frac{1}{\dr} \int_{R}^{R+\dr} \frac{\sigmas_{rr} - \sigmas_{\theta\theta}}{r} \; dr\\
% \rhos \frac{d^2 \tilde{u}_r}{d t^2}
% &= \frac{\sigmas_{rr}(R+\dr,t) - \sigmas_{rr}(R,t)}{\dr}
% + \frac{2\mus}{\dr} 
% \int_{R}^{R+\dr}\left(
%  \frac{1}{r} \frac{\partial \us_r}{\partial r} - \frac{1}{r^2} \us_r 
% \right) \; dr \\
% &= \frac{\sigmas_{rr}(R+\dr,t) - \sigmas_{rr}(R,t)}{\dr}
% + \frac{2\mus}{\dr} 
% \int_{R}^{R+\dr} \frac{\partial }{\partial r} \left(
%  \frac{1}{r} \us_r 
% \right) \; dr \\
% &= \frac{\sigmas_{rr}(R+\dr,t) - \sigmas_{rr}(R,t)}{\dr}
% + \frac{2\mus}{\dr} 
% \left(\frac{\us_r(R+\dr,t)}{R+\dr} - \frac{\us_r(R,t)}{R} \right)\\
\frac{d^2 \tilde{u}_r}{d t^2} &= 
\frac{\cp^2}{\dr} \int_{R}^{R+ \dr} \frac{\partial}{\partial r}
\left(\frac{1}{r} \frac{\partial (r \us_r)}{\partial r} \right) \; dr \\
\frac{d^2 \tilde{u}_r}{d t^2} &=\frac{\cp^2}{\dr} 
\left(\frac{1}{r} \frac{\partial (r \us_r)}{\partial r} \right) \bigg{|}_R^{R+\dr}
\end{align}
%
The solid stress definition is used to simplify the above equation.
\begin{align}
\sigmas_{rr} &= \frac{\lambdas}{r} \frac{\partial (r \us_r)}{\partial r}
 + 2 \mus \frac{\partial \us_r}{\partial r} \\
\frac{1}{r} \frac{\partial(r \us_r)}{\partial r} &= \frac{1}{\lambdas}
\left( \sigmas_{rr} - 2 \mus \frac{\partial \us_r}{\partial r}\right)
\end{align}
%
We make the approximation $\frac{\partial \us_r}{\partial r} \approx 0.$ 
A free surface BC is applied at $r = R+\dr,$ $\sigmas_{rr}(R+\dr,t) = 0,$
and the interface traction is applied at $r = R,$ $\sigmas_{rr}(R,t) = \sigma_I(t).$
The ODE for the interface displacement is
\begin{align}
\frac{d^2 \tilde{u}_r}{d t^2} &= - \frac{\cp^2}{\lambdas \dr} \sigma_I (t).
\end{align}
%
where $\sigma_I$ is the interface traction. We use the matching condition
$v_I(t) = \frac{d \tilde{u}_r}{d t}(R,t)$ to obtain the interface boundary condition
for the fluid.
\begin{align}
\dot{v_I}(t) &= - \frac{\lambdas + 2 \mus}{\rhos \lambdas \dr} \sigma_I(t)
\end{align}
%
The matching condition on velocity is used to obtain the displacement.
\begin{align}
\frac{d}{dt} \tilde{u}_r(t) &= \frac{\dot{m}(t)}{2 \pi (R+\tilde{u}_r) \rho} \\
\frac{1}{R} \int_{0}^{\tilde{u}_r(t)} 
 \left(1 + \frac{u}{R} \right) \; d u
&= \frac{1}{2 \pi R^2 \rho} \int_0^t \dot{m}(\tau) \; d \tau + C \\
\frac{\tilde{u}_r(t)}{R} + \frac{\tilde{u}_r(t)^2}{2R^2}
&= \frac{1}{2 \pi R^2 \rho} \int_0^t \dot{m}(\tau) \; d \tau + C \\
\left(\frac{\tilde{u}_r(t)}{R} + 1 \right)^2
&= \frac{1}{\pi R^2 \rho} \int_0^t \dot{m}(\tau) \; d \tau + \tilde{C} \\
\frac{\tilde{u}_r(t)}{R} 
&= -1 + \sqrt{\frac{1}{\pi R^2 \rho} \int_0^t \dot{m}(\tau) \; d \tau + \tilde{C}} 
\end{align}
%
The positive branch of the square root was chosen since $\tilde{u}_r > 0.$
The initial condition $\tilde{u}_r(0) = \tilde{u}_0$ is enforced to find
$\tilde{C}.$ The solution is given by
\begin{align}
\frac{\tilde{u}_r(t)}{R} 
&= -1 + \sqrt{\frac{1}{\pi R^2 \rho} \int_0^t \dot{m}(\tau) \; d \tau + 
\left(\frac{\tilde{u}_0}{R} + 1 \right)^2} 
\end{align}
%
The location of the interface is given by
\begin{align}
R_I(t) = R + \tilde{u}_r(t) = R \sqrt{\frac{1}{\pi R^2 \rho} \int_0^t \dot{m}(\tau) \; d \tau + 
\left(\frac{\tilde{u}_0}{R} + 1 \right)^2}.
\end{align}
%
The other free constant, $g(t),$ can be found from the traction matching condition.
\begin{align}
\dot{v_I}(t) &= - \frac{\lambdas + 2 \mus}{\rhos \lambdas \dr} \sigma_I(t)\nonumber \\
\frac{\ddot{m}(t)}{2 \pi R_I(t) \rho}
&=
- \frac{\lambdas + 2 \mus}{\rhos \lambdas \dr} 
\left( g(t) - \frac{\dot{m}(t)^2}{8 \pi^2 R_I(t)^2}\right) \nonumber\\
g(t) &= \frac{\dot{m}(t)^2}{8 \pi^2 R_I(t)^2}
- \frac{\rhos \lambdas \ddot{m}(t) \dr}{2 \pi R_I(t) \rho (\lambdas + 2 \mus)}
\end{align}


==> texFiles/radialElasticPistonOverture.tex <==
\newcommand{\urs}{\us_r}
\newcommand{\usr}{\urs}
\newcommand{\vrs}{\vs_r}
\newcommand{\vsr}{\vrs}
% \newcommand{\rs}{\bar{r}}
\newcommand{\Rs}{\bar{R}}
\newcommand{\RI}{R_I}
\newcommand{\rHat}{\hat{\rv}}
\newcommand{\thetaHat}{\hat{\thetav}}
% -----------------------------------------------------------------
\clearpage
\section{Radial elastic piston Overture results}

Here is the radial elastic piston solution
\begin{align}
  &  \urs(\rs,t) =  \alpha \f{J_1(k r)}{J_1(k\Rs)} \sin( \cp k (t-t_0) )
\end{align}
Notes on Dan's elastic piston solution (note factor of 2 difference in one term of g):
\begin{align}
  &  J_n'(z) = \half( J_{n-1}(z) - J_{n+1}(z) ), \\
  & \RI(t) = \Rs + \usr(\Rs,t), \\ 
  & f(t) = \RI(t) \vsr(\Rs,t),  \\
  & g(t) = \f{\rho f^2}{2 \RI^2} - \f{2\mu}{\RI^2} f - (\lambdas+2\mus)\partial_{\rs} \urs(\Rs,t) - \f{\lambdas}{\Rs} \urs(\Rs,t), \\
  & \sigmav^{\xsv} = \sigma_{rr} \rHat\rHat^T + \sigma_{r\theta}\rHat\thetaHat^T
                    + \sigma_{\theta r}\thetaHat\rHat^T  + \sigma_{\theta\theta} \thetaHat\thetaHat^T
\end{align}


Here are the parameters used for the runs in the following sections.
\begin{center}%\footnotesize
  \begin{tabular}{|ccccccc|}
  \hline
  $\Rs$ & $R$ & $\alpha$  & $k$  & $t_0$   & $\rho$ & $\nu$ \strutt \\ \hline
  $.5$  & $1$ &   $0.05$  & $\pi$  & $0$ & $1$ & $0.05$    \\
  \hline
\end{tabular}
\end{center} 
Using $\rhos=\delta \rho$, $\lambdas=\delta$, $\mus=\delta$, with $\delta=\text{scf}=\text{solid-scale-factor}$


% --------------------------------------------------------------------
% \clearpage
\subsection{Radial-Elastic Piston : Traditional Scheme - INS IM22 implicit PC}
Results from the TP scheme using the implicit fluid solver INS-IM22.

\noindent SCF=1600 -- OK although solid a bit slow (similiar rates in solid to using exact interface values)
\input tables/insElasticPiston.rep.TPSCF1600Imtp3.ConvTable.tex

\noindent SCF=8000 -- OK although solid a bit slow 
\input tables/insElasticPiston.rep.TPSCF8000Imtp3.ConvTable.tex

% --------------------------------------------------------------------
\clearpage
\subsection{Radial-Elastic Piston : AMP Scheme - INS IM22 implicit PC}

Results from the AMP scheme using the implicit fluid solver INS-IM22.


\noindent SCF=8000 -- OK? 
\input tables/insElasticPiston.rep.AmpSCF8000Imtp3.ConvTable.tex

\noindent SCF=1 -- Trouble on G8 for $\nu=.05$, Ok for $\nu=.01$.
{\bf Note: I still need to implement proper AMP BC for tangential velocity.}
\input tables/insElasticPiston.rep.AmpSCF1Imtp3.ConvTable.tex


\noindent SCF=0.1 
\input tables/insElasticPiston.rep.AmpSCF0p1Imtp3.ConvTable.tex


==> texFiles/radialElasticPistonSolution.tex <==
\section{Radial elastic piston solution} \label{sec:radialElasticPiston}

Consider motions only in the radial direction,
($v_\theta = 0$ and $\us_\theta = 0$).
The fluid momentum equation becomes a quadrature for the pressure.
\begin{align}
\frac{\rho}{r} f'(t)
- \frac{\rho}{r^3} f(t)^2 
+ \frac{\partial p}{\partial r} &= 
0   \nonumber \\
\frac{\partial p}{\partial r} &= 
\frac{\rho}{r^3} f(t)^2 
-\frac{\rho}{r} f'(t).
\end{align}
%
The pressure is obtained by integration
\begin{align}
p(r,t) &= g(t;R)
-\frac{\rho}{2r^2} f(t)^2 
-\rho f'(t) \log\left( \frac{r}{R} \right)  .
\end{align}
%
Another boundary condition for $p$ is needed to determine $g(t;R).$
The arbitrary constant $R$ was introduced to simplify the expression.

In the solid, search for solutions of the form
\begin{align}
\us_r(r,t) = \hat{\us}_r(r) \cos(\cp k t +\phi). \nonumber
\end{align}
%
Plug this in to the equations to obtain
\begin{align}
- k^2 \hat{\us}_r &= \frac{d }{d r} \left( \frac{d \hat{\us}_r}{d r} + \frac{1}{r} \hat{\us}_r \right) \nonumber \\
0 &= \hat{\us}_r'' + \frac{1}{r} \hat{\us}_r'
+ k^2 \hat{\us}_r - \frac{1}{r^2} \hat{\us}_r \nonumber \\
0 &= r^2 \hat{\us}_r'' + r \hat{\us}_r'
+ (k^2 r^2 - 1) \hat{\us}_r.
\end{align}
%
This is the Bessel equation of order 1. The solution is
\begin{align}
\us_r(r,t) = \left(A J_1(kr) + B Y_1(kr)\right) \cos(\cp k t + \phi).
\end{align}

The fluid is in the domain $R+\us_r(R,t) < r < R_0$ and the solid reference 
domain is $0 \le \bar{r} < R.$ The solid displacement must be finite at $r=0,$
therefore the coefficient of $Y_1$ must be 0. The solution in the fluid and solid domains
are given by
\begin{align}
v_r(r,t) &= \frac{1}{r} f(t) \\
p(r,t) &= g(t)
-\frac{\rho}{2r^2} f(t)^2 
-\rho f'(t) \log\left( \frac{r}{R_I(t)} \right)   \\
\us_r(\bar{r},t) &= \us_0 J_1(k\bar{r})  \cos(\cp k t + \phi),
\end{align}
%
where $R_I(t) = R+\us_r(R,t).$
The pressure is supplied to be $p_0(t)$ at $r=R_0.$ 
Instead of solving the general problem, we find $p_0$ for a given
solution to the FSI problem with boundary conditions
\begin{align}
v_r(R+\us_r(R,t),t) &= \partial_t \us_{r}(R,t) \\
\sigma_{rr}(R+\us_r(R,t),t) &= \sigmas_{rr}(R,t) .
\end{align}
%
The stress matching condition is equivalent to
\begin{align}
-p + 2 \mu \frac{\partial v_r}{\partial r} = 
\lambdas \left(\frac{1}{\bar{r}} \frac{\partial (\bar{r} \us_r)}{ \partial \bar{r}}
+ \frac{1}{\bar{r}} \frac{\partial \us_\theta}{\partial \theta} \right) 
+ 2 \mus \frac{\partial \us_r}{\partial \bar{r}},
\quad 
r = R_I(t),\; \bar{r} = R.
\end{align}
%
Solve for $f(t)$ using velocity matching condition.
\begin{align}
v_I &= -\us_0{{ J}_{1}\left(k{R}\right)}\cp k\sin
 \left( \cp kt+\phi \right) 
= \frac{f(t)}{R+\us_0 J_1(k R) \cos(\cp k t + \phi)}. 
\nonumber
\end{align}
%
The solution is
\begin{align}
f(t) &= -\left(R+\us_0 J_1(k R) \cos(\cp k t + \phi) \right) 
\us_0{{ J}_{1}\left(k{R}\right)}\cp k\sin
 \left( \cp kt+\phi \right)  .
\end{align}
%
Solve for $g(t)$ using the traction matching condition
\begin{align}
\sigma_I =\;& \frac{\us_0}{R} \left(k R (\lambdas + 2 \mus) J_0(kR)
 - 2 \mus J_1(kR) \right) \cos(\cp k t + \phi) 
=-g(t) + \frac{1}{2 R_I(t)^2} \left(\rho f(t)^2 - 2 \mu f(t) \right)
\nonumber
\end{align}
%
The solution is (\das{I fixed the error in the $\mu f(t) / R_I^2$ term})
\begin{align}
g(t) = \frac{1}{2 R_I(t)^2} \left(\rho f(t)^2 - 4 \mu f(t) \right)
- \frac{\us_0}{R} \left(k R (\lambdas + 2 \mus) J_0(kR)
 - 2 \mus J_1(kR) \right) \cos(\cp k t + \phi) .
\end{align}
%
See \texttt{/CG/fibr/codes/testSolutions/radialElasticPiston}
for details.



==> texFiles/radialPiston.tex <==
\newcommand{\Gcrp}{\Gv_{\rm rp}}
\subsection{Radial elastic piston}

Here are some initial results for the radial elastic piston.


{% ------ GRIDS ------  
%
\newcommand{\figWidth}{6cm}% height 
\newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.1}{.1}{.1}{.1}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (16,6);  % set the bounding box (so we have less surrounding white space)

   \draw(0.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/radialElasticPistonGrid}{\figWidth}};
% 
%    \draw(7.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/radialG2SLt0p5}{\figWidth}};
   \draw(7.0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/radialG4SLt0p5}{\figWidth}};
% grid:
 \draw[step=1cm,gray] (0,0) grid (16,6);
\end{tikzpicture}
\end{center}
  \caption{Composite grid $\Gcrp^{(2)}$ for the radial elastic piston problem.
    The green fluid grid adjacent to the interface  moves over time. The blue fluid background grid remains fixed.
    The red and pink grids for the solid reference domain also remain fixed over time.
    Right: speed. 
}
  \label{fig:elasticPistonGrid}
\end{figure}
}


==> texFiles/radialShearSolution.tex <==
\section{Pure shear solution}

Consider $v_r = 0$ and $\us_r = 0.$ The equations in the fluid and solid are
\begin{align}
- \frac{\rho}{r} v_\theta^2 + \frac{\partial p}{\partial r} &= 0 \\
\rho \frac{\partial v_\theta}{\partial t}
 &= 
 \frac{\mu}{r} \frac{\partial}{\partial r} 
\left(r \frac{\partial v_\theta}{\partial r}\right) 
- \mu \frac{v_\theta}{r^2} \\
\frac{\partial^2 \us_\theta}{\partial t^2} &=
\cs^2 \frac{\partial}{\partial r}
\left( \frac{1}{r} \frac{\partial (r \us_\theta)}{\partial r} \right).
\end{align}
%
Look for solutions of the form
\begin{align}
v_\theta(r,t) = \hat{v}_\theta(r) e^{i \omega t}, \quad
\us_\theta(r,t) = \hat{\us}_\theta(r) e^{i \omega t}.\nonumber 
\end{align}
%
The fluid and solid equations simplify to
\begin{align}
0 &= r^2 \hat{v}_\theta'' + r \hat{v}_\theta' + (\alpha^2 r^2 - 1) \hat{v}_\theta \\
0 &= r^2 \hat{\us}_\theta'' + r \hat{\us}_\theta' + (\beta^2 r^2 - 1) \hat{\us}_\theta 
\end{align}
%
where
\begin{align}
\alpha^2 = - \frac{i \rho \omega}{\mu}, \quad \beta^2 = \frac{\omega^2}{\cs^2}.
\end{align}
%
The solutions for the transformed variables are
\begin{align}
\hat{v}_\theta(r) &= A J_1(\alpha r) + B Y_1(\alpha r) \\
\hat{\us}_\theta(r) &= C J_1(\beta r) + D Y_1(\beta r).
\end{align}
%
The general solutions are
\begin{align}
{v}_\theta(r,t) &= \left(A J_1(\alpha r) + B Y_1(\alpha r)\right) e^{i\omega t} \\
{\us}_\theta(r,t) &= \left(C J_1(\beta r) + D Y_1(\beta r)\right) e^{i\omega t}.
\end{align}
%
The solid domain is $0 < r < R$ and the fluid domain is 
$R < r < R_0.$ 
Since the solid displacement must be finite at $r=0,$ we have $D=0.$
The fluid and solid solutions must obey the matching conditions
\begin{align}
v_\theta(R,t) &= \frac{\partial \us_\theta}{\partial t}(R,t) \\
\sigma_{rr}(R,t) &= \sigmas_{rr}(R,t) \label{eq:srrMatching} \\
\sigma_{r\theta}(R,t) &= \sigmas_{r\theta}(R,t) .
\end{align}
%
A boundary condition is also required at $r=R_0.$ We impose the no-slip condition
\begin{align}
v_\theta(R_0,t) = 0.
\end{align}
%
Since $\sigmas_{rr} = 0$ and the only contribution to $\sigma_{rr}$
is from the fluid pressure,
equation \eqref{eq:srrMatching} simplifies to
\begin{align}
p(R,t) = 0.
\end{align}
%
The solution for the pressure is thus given by
\begin{align}
p(r,t) = \rho \int_R^r \frac{v_\theta(s,t)^2}{s} \; ds.
\end{align}
%
The other three interface/boundary conditions result in an eigenvalue problem for 
$\omega.$ The velocity matching condition is
\begin{align}
A J_1(\alpha R) + B Y_1(\alpha R) = i \omega C J_1 (\beta R) .\nonumber
\end{align}
%
The stress matching condition is
\begin{align}
\frac{\mu}{r} \left(\frac{\partial v_\theta}{\partial r} - \frac{v_\theta}{r} \right)
 &= 
\frac{\mus}{r} \left(\frac{\partial \us_\theta}{\partial r} - \frac{\us_\theta}{r} \right)
\nonumber \\
\frac{\mu}{r} \left(
A \left(J_1'(\alpha R) - \frac{J_1(\alpha R)}{R} \right)
+B \left(Y_1'(\alpha R) - \frac{Y_1(\alpha R)}{R} \right)
 \right)
&= 
\frac{\mu}{r} 
C \left(J_1'(\beta R) - \frac{J_1(\beta R)}{R} \right). \nonumber
\end{align}
%
The no-slip condition is
\begin{align}
A J_1(\alpha R_0) + B J_2(\alpha R_0) = 0 \nonumber
\end{align}
%
These conditions are written as a matrix system
\begin{align}
\Mv(\omega) \av = 0, 
\end{align}
%
where
\begin{align}
\Mv(\omega) =  \left[ \begin {array}{ccc} {{\sl J}_{1}\left(\alpha\,{R}\right)
}&{{\sl Y}_{1}\left(\alpha\,{R}\right)}&-i{{\sl J}_{1}\left(
\beta\,{R}\right)}\omega\\ \noalign{\medskip}{{\sl J}_{1}\left(
\alpha\,{R_0}\right)}&{{\sl Y}_{1}\left(\alpha\,{R_0}\right)}&0
\\ \noalign{\medskip}{\frac {{{\sl J}_{0}\left(\alpha\,{R}
\right)}{R}\,\alpha\,\mu-2\,{{\sl J}_{1}\left(\alpha\,{R}
\right)}\mu}{{{R}}^{2}}}&{\frac {{{\sl Y}_{0}\left(\alpha\,{
R}\right)}{R}\,\alpha\,\mu-2\,{{\sl Y}_{1}\left(\alpha\,{
R}\right)}\mu}{{{R}}^{2}}}&{\frac {-{{\sl J}_{0}\left(\beta\,{
R}\right)}{R}\,\beta\,{\mus}+2\,{{\sl J}_{1}\left(
\beta\,{R}\right)}{\mus}}{{{R}}^{2}}}\end {array}
 \right] \nonumber
\end{align}
%
and $\av = [A,B,C]^T.$ $\omega$ is a solution to $\det(\Mv(\omega))=0.$
For the parameters
\begin{align}
R = 1,\quad R_0 = 2,\quad \rho = 1,\quad \mu = 10,\quad \rhos = 10,\quad \cs = 1,
\end{align}
%
a solution was found to be
\begin{align*}
\omega &= \phantom{-} 1.4841084914290283\text{e}+01 +  
\phantom{-}7.0873356446257796\text{e}-01 i\\
A     &= -1.4894197324861366\text{e}-01 + -2.4826496514057889\text{e}-01 i\\
B     &= -2.7073357963903405\text{e}-01 +  
\phantom{-}1.3818364548148002\text{e}-01 i\\
C     &= \phantom{-} 2.0000000000000000\text{e}-01 +  
\phantom{-}0.0000000000000000\text{e}+00 i
\end{align*}
%
See \texttt{/CG/fibr/codes/testSolutions/radialShear}
for details.

In reality, the deformation of the solid also causes warping.
Consider the solid deformation.
\begin{align*}
\ysv = \usv + \xsv = (\us_r + \rs) \hat{\rv} + \us_\theta \hat{\thetav}.
\end{align*}
%
Since $\us_r = 0,$
\begin{align*}
\ysv &= \rs \hat{\rv} + \us_\theta \hat{\thetav} \\
&= (\rs \cos \theta - \us_\theta \sin \theta) \hat{\xv}_1
+(\rs \sin \theta + \us_\theta \cos \theta) \hat{\xv}_2
\end{align*}
%
Therefore, the radius of the deformed solid is actually
\begin{align*}
\|\ysv\|_2^2 = \rs^2 + \us_\theta^2.
\end{align*}
%
The relative error of the linearized boundary is
\begin{align*}
\frac{\sqrt{R^2 + \us_\theta^2} - R}{R} \sim
\frac{1}{2} \left(\frac{\us_\theta}{R} \right)^2 + 
O \left( \left(\frac{\us_\theta}{R} \right)^4 \right).
\end{align*}


==> texFiles/radialTravelingWaveSolution-old.tex <==
\section{Radial traveling wave solution}
\label{sec:radialTravelingWaveSolution}

A Stokes fluid occupies a circular region defined by $0 < r < r_0$ and a linearly elastic 
solid occupies an annular region defined by $r_0 < r < R.$
The solution is linearized about small interface deformations, therefore 
it is assumed that the interface is located at $r=r_0$ for all time. 

In the fluid, solutions are sought of the form
\begin{align*}
v_r(r,\theta,t) = \hat{v}_r(r) e^{i (n \theta - \omega t)}, \quad
v_\theta(r,\theta,t) = \hat{v}_\theta(r) e^{i (n \theta - \omega t)} , \quad
p(r,\theta,t) = \hat{p}(r) e^{i (n \theta - \omega t)} .\nonumber 
\end{align*}
%
After substitution, the equations become
\begin{align}
\frac{1}{r} (r \hat{v}_r)' + \frac{i n}{r} \hat{v}_\theta &= 0  
\label{eq:smallDistContinuity} \\
-i \omega \rho \hat{v}_r + \hat{p}' &= \mu 
\left(\frac{1}{r} (r \hat{v}_r')' 
- \frac{n^2}{r^2} \hat{v}_r 
- \frac{\hat{v}_r}{r^2} 
- \frac{2 i n}{r^2} \hat{v}_\theta
\right) \label{eq:smallDistRadialMomentum}\\
-i \omega \rho \hat{v}_\theta + \frac{i n}{r} \hat{p}' &= \mu
\left(\frac{1}{r} (r \hat{v}_\theta')'
- \frac{n^2}{r^2} \hat{v}_\theta
+ \frac{2 i n}{r^2} \hat{v}_r
- \frac{\hat{v}_\theta}{r^2} 
\right).\label{eq:smallDistCircumMomentum}
\end{align}
%
Equations~\eqref{eq:smallDistContinuity}--\eqref{eq:smallDistCircumMomentum} 
can be manipulated into an Euler equation for $\hat{p},$ given by
\begin{align}
\hat{p}'' 
+ \frac{1}{r} \hat{p}'
- \frac{n^2}{r^2} \hat{p} &= 0. 
\end{align}
%
The solution which remains bounded at $r=0$ is given by
\begin{align}
\hat{p}(r) = p_I \left(\frac{r}{r_0} \right)^n .
\end{align}
%
Equation~\eqref{eq:smallDistContinuity} can be used to eliminate $\hat{v}_\theta$
in equation~\eqref{eq:smallDistRadialMomentum}. The result is a Bessel-like equation for
$\hat{v}_r$ with a right hand side forcing term from the pressure.
\begin{align}
r^2 \hat{v}_r'' + 3 r \hat{v}_r' + (\lambda^2 r^2 - n^2+1) \hat{v}_r
&= p_I \frac{n r^{n+1}}{\mu r_0^n}
\label{eq:besselvr}
\end{align}
%

\begin{align}
\hat{v}_r(r) &= c \frac{J_n(\lambda r)}{r}
+ p_I \frac{n r^{n-1}}{\mu \lambda^2 R^n}.
\end{align}


We can manipulate these equations to obtain an
Euler equation for $\hat{p}$, a Bessel equation for 
$\hat{v}_r$, and a constraint equation for $\hat{v}_\theta.$
The equation for the pressure is


\begin{align}
\end{align}

\begin{align}
\hat{v}_\theta &= -\frac{1}{in} \left(\hat{v}_r + r \hat{v}_r' \right).
\end{align}
%
The solution to equation \eqref{eq:besselvr} is 
\begin{align}
\hat{v}_r(r) = \frac{c}{r} J_n (\lambda r) 
+ \tilde{v}_r(r)
\end{align}
%
where $\tilde{v}_r(r)$ is the particular solution.
Search for a particular solution of the form
\begin{align}
\tilde{v}_r(r) = K r^{n-1}
\end{align}
%
The equation becomes
\begin{align*}
K (n-1) (n-2) (r^2) (r^{n-3})
+ 3 K (n-1) (r) (r^{n-2})
+ (\lambda^2 r^2 - n^2+1) r^{n-1} &= d \frac{n r^{n+1}}{\mu R^n} \\
K r^{n-1} \left[(n-1)(n-2) + 3 (n-1) - n^2 + 1 \right]
+ r^{n+1} \left[K \lambda^2 - d \frac{n}{\mu R^n}\right] &= 0.
\end{align*}
%
Evaluate the coefficient of $r^{n-1}$
\begin{align*}
(n-1)(n-2) + 3 (n-1) - n^2 + 1 = n^2 - 3n + 2 + 3n - 3 - n^2 + 1 = 0.
\end{align*}
%
Therefore
\begin{align}
K = d\frac{n }{\mu R^n \lambda^2}
\end{align}
%
The solution for $\hat{v}_r$ is then
\begin{align}
\hat{v}_r(r) &= c \frac{J_n(\lambda r)}{r}
+ d \frac{n r^{n-1}}{\mu \lambda^2 R^n}.
\end{align}
% 
The solution for $\hat{v}_\theta$ is then obtained:
\begin{align}
\hat{v}_{\theta}(r) &=
i c \left(\frac{J_n(\lambda r)}{r}
- \frac{\lambda}{n} J_{n+1}(\lambda r)
\right)
+ d \frac{i n r^{n-1}}{\mu \lambda^2 R^n}.
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We decompose the solid displacement into the sum of the gradient of 
a potential, $\phi$, and curl of a vector field, $\Hv.$
\begin{align}
\uv = \grad \phi + \grad \curl \Hv
\end{align}
%
In this decomposition, the equations of linear elasticity reduce to
the following wave equations.
\begin{align}
\phi_{tt} &= \cp^2 \Delta \phi \\
\Hv_{tt} &= \cs^2 \Delta \Hv.
\end{align}
%
% \textbf{Proof}: Einstein notation is used for ease of notation.
% $a_i$ represents the i-th component of the vector $\av$ and 
% $b_{,i}$ represents the derivative with respect to the i-th coordinate (ie. $\frac{\partial b}{\partial x_i}$).
% $a_{i}b_i$ represents the sum $a_1 b_1 + a_2 b_2 + a_3 b_3.$
% The equations for linear elasticity are given by
% \begin{align}
% \rho \frac{\partial^2 u_i}{\partial t^2}  = \sigma_{ij,j}.
% \end{align}
% %
% The stress is related to the displacement through
% \begin{align}
% \sigma_{ij} = \lambda u_{k,k} \delta_{ij} + \mu (u_{i,j} + u_{j,i})
% \end{align}
% %
% and the displacement in Einstein notation is
% \begin{align}
% u_i = \phi_{,i} + H_{k,j} \; \epsilon_{jki}.
% \end{align}
% %
% $\delta$ is the Kronecker delta $\epsilon$ is the permutation symbol.
% \begin{align}
% \delta_{ij} = \begin{cases}
% 1, & i=j \\
% 0, & i \ne j
% \end{cases}, \quad\quad
% \epsilon_{ijk} = \begin{cases}
% 1, & \text{even permutations (123, 231, 312)}\\
% 0, & \text{repeated indices}\\
% -1, & \text{odd permutations (321, 213, 132)}.
% \end{cases}\nonumber
% \end{align}
% %
% The divergence of $\uv$ is given by
% \begin{align}
% u_{i,i} &= \phi_{,ii} + H_{k,ji} \epsilon_{jki} \nonumber \\
% u_{i,i} &= \phi_{,ii},
% \end{align}
% %
% since the divergence of the curl of a vector is 0.
% The displacement gradient is given by
% \begin{align}
% u_{i,j} &= \phi_{ij} + H_{k,lj} \epsilon_{lki}.
% \end{align}
% %
% The two previous expressions are substituted into the stress tensor to obtain
% \begin{align}
% \sigma_{ij} &= \lambda \phi_{,kk} \delta_{ij}
% + \mu \left(\phi_{,ij} + \phi_{,ji} \right)
% + \mu \left(H_{k,lj} \epsilon_{lki} + H_{k,li} \epsilon_{lkj} \right)\nonumber\\
% \sigma_{ij} &= \lambda \phi_{,kk} \delta_{ij}
% + 2 \mu \phi_{,ij} 
% + \mu \left(H_{k,lj} \epsilon_{lki} + H_{k,li} \epsilon_{lkj} \right)
% \end{align}
% %
% The divergence of the stress tensor is given by
% \begin{align}
% \sigma_{ij,j} = \lambda \phi_{,kkj} \delta_{ij} 
% + 2 \mu \phi_{,ijj} 
% + \mu \left(H_{k,ljj} \epsilon_{lki} + H_{k,lij} \epsilon_{lkj} \right)
% \end{align}
% %
% Since the labels of the indices are arbitrary, 
% the following simplification occurs
% \begin{align*}
% H_{k,lij} \epsilon_{lkj} = H_{k,jil} \epsilon_{jkl} = -H_{k,jil} \epsilon_{lkj} = 0.
% \end{align*}
% %
% We are left with
% \begin{align}
% \sigma_{ij,j} &= \lambda \phi_{,kki}
% + 2 \mu \phi_{,ijj} 
% + \mu H_{k,ljj} \epsilon_{lki} \\
% \sigma_{ij,j} &= (\lambda+ 2\mu) \phi_{,jji}
% + \mu H_{k,jjl} \epsilon_{lki} .
% \end{align}
% %
% The governing equation is now substituted 
% \begin{align}
% \rho \frac{\partial^2 \phi_{,i}}{\partial t^2} 
% + \rho \frac{\partial^2 H_{k,l}}{\partial t^2} \epsilon_{lki}
%  &= (\lambda+ 2\mu) \phi_{,jji}
% + \mu H_{k,jjl} \epsilon_{lki} .
% \end{align}
% %
% Comparing like terms, we end up with
% \begin{align}
% \left( \rho \frac{\partial^2 \phi_{}}{\partial t^2} - (\lambda + 2 \mu) \phi_{,jj} \right)_{,i}
% + \left( \rho \frac{\partial^2 H_{k}}{\partial t^2} -\mu H_{k,jj}\right)_{,l}  \epsilon_{lki}
%  &= 0.
% \end{align}
% %
% In symbolic notation, this is equivalent to
% \begin{align*}
% \phi_{tt} &= \cp^2 \Delta \phi \\
% \Hv_{tt} &= \cs^2 \Delta \Hv.
% \end{align*}


Consider 2D displacements ($\Hv = H \ev_3$) in the polar basis ($\ev_r$ and $\ev_\theta$).
The equations reduce to
\begin{align}
\phi_{tt} &= \cp^2 \left(\frac{1}{r} \frac{\partial }{\partial r} \left( r \frac{\partial \phi}{\partial r} \right) 
  + \frac{1}{r^2} \frac{\partial^2 \phi }{\partial \theta^2} \right) \\
H_{tt} &= \cs^2 \left(\frac{1}{r} \frac{\partial }{\partial r} \left( r \frac{\partial H}{\partial r} \right) 
  + \frac{1}{r^2} \frac{\partial^2 H }{\partial \theta^2} \right) .
\end{align}
%
To calculate the displacement, the following are needed.
\begin{align}
\grad \phi &= \frac{\partial \phi}{\partial r} \ev_r + \frac{1}{r} \frac{\partial \phi}{\partial \theta} \ev_\theta \\
\grad \curl \Hv &= \frac{1}{r} \frac{\partial H}{\partial \theta} \ev_r - \frac{\partial H}{\partial r} \ev_\theta
\end{align}
%
Therefore,
\begin{align}
u_r &= \frac{\partial \phi}{\partial r} + \frac{1}{r} \frac{\partial H}{\partial \theta} \\
u_\theta &= \frac{1}{r} \frac{\partial \phi}{\partial \theta} - \frac{\partial H}{\partial r}
\end{align}


\subsubsection{Traveling wave ansatz}

Search for solutions of the form
\begin{align}
\phi(r,\theta,t) = \hat{\phi}(r) e^{i (n \theta - \omega t)}, \quad
H(r,\theta,t) = \hat{H}(r) e^{i (n \theta - \omega t)}.
\end{align}
%
The equation for $\hat{\phi}$ is 
\begin{align}
-\frac{\omega^2}{\cp^2} \hat{\phi} &= \frac{1}{r} \left( r \hat{\phi}' \right)' - \frac{n^2}{r^2}\hat{\phi} \\
0&= r^2 \hat{\phi}'' + r \hat{\phi} + \left(\frac{\omega^2}{\cp^2} r^2 - n^2 \right) \hat{\phi}
\end{align}
%
Similarly for $\hat{H}$,
\begin{align}
0&= r^2 \hat{H}'' + r \hat{H} + \left(\frac{\omega^2}{\cs^2} r^2 - n^2 \right) \hat{H}.
\end{align}
%
Solutions are
\begin{align}
\hat{\phi}(r) &= d_1 J_n(k_p r) + d_2 Y_n(k_p r) \\
\hat{H}(r) &= d_3 J_n(k_s r) + d_4 Y_n(k_s r)
\end{align}
%
where
\begin{align}
k_p = \frac{\omega}{\cp}, \quad k_s = \frac{\omega}{\cs}.
\end{align}
%
The displacement is related through
\begin{align}
\hat{u}_r = \hat{\phi}' + \frac{in}{r} \hat{H}, \quad
\hat{u}_\theta = \frac{in}{r} \hat{\phi} - \hat{H}'.
\end{align}
%
The solution is 
\begin{align*}
\hat{u}_r &= \phantom{-}
d_1 \left(\frac{n J_n(k_p r)}{r} - k_p J_{n+1}(k_p r) \right)
+ d_2 \left(\frac{n Y_n(k_p r)}{r} - k_p Y_{n+1}(k_p r) \right)
+ \frac{i n }{r} \left(d_3 J_n (k_s r) + d_4 Y_n(k_s r) \right) \\
\hat{u}_{\theta} &= -d_3 \left(\frac{n J_n(k_s r)}{r} - k_s J_{n+1}(k_s r) \right)
- d_4 \left(\frac{n Y_n(k_s r)}{r} - k_s Y_{n+1}(k_s r) \right)
+ \frac{i n }{r} \left(d_1 J_n (k_p r) + d_2 Y_n(k_p r) \right)
\end{align*}

\subsection{Review of solutions}

% The fluid solution is
% \begin{align}
% \hat{p}(r) &= p_0 \left(\frac{r}{R} \right)^n \\
% \hat{v}_r(r) &= \frac{1}{r} \left( c_1 J_n (\lambda r) + c_2 Y_n (\lambda r) \right)
% + \tilde{v}_r(r)\\
% \hat{v}_\theta(r) &= \frac{i c_1}{ n r} \left( 
%    n J_n (\lambda r) - \lambda r J_{n+1}(\lambda r) \right)
%  +\frac{i c_2}{ n r}
%  \left( n Y_n (\lambda r) - \lambda r Y_{n+1}(\lambda r) \right)
% + \tilde{v}_\theta(r).
% \end{align}
% %
% The particular solution in the fluid is
% \begin{align*}
% \tilde{v}_r(r) &= - \frac{\pi n p_0}{2 \mu R^{n-1} r} \left( \;
% \int_0^r \left( Y_{n}(\lambda s) J_{n}(\lambda r) 
% -  J_{n}(\lambda s) Y_{n}(\lambda r)  \right) s^{n+1} \; ds
% \right)\\
% \tilde{v}_\theta(r) &= 
% -\frac{i \pi p_0}{2 \mu R^{n-1} r} 
% \left( \int_0^r  \left(Y_{n}(\lambda s) 
% (n J_n(\lambda r) - J_{n+1}(\lambda r) \lambda r) 
% -J_{n}(\lambda s) 
% (n Y_{n}(\lambda r) - Y_{n+1}(\lambda r) \lambda r)
%  \right) s^{n+1}
%  \; d s \right).
% \end{align*}
%
% We take $c_2 = 0$ to bound the solution at $r=0$.
\begin{align}
\hat{p}(r) &= d \left(\frac{r}{R} \right)^n \\
\hat{v}_r(r) &= c \frac{J_n(\lambda r)}{r}
+ d \frac{n r^{n-1}}{\mu \lambda^2 R^n} \\
\hat{v}_{\theta}(r) &=
i c \left(\frac{J_n(\lambda r)}{r}
- \frac{\lambda}{n} J_{n+1}(\lambda r)
\right)
+ d \frac{i n r^{n-1}}{\mu \lambda^2 R^n}.
\end{align}

For here on, the solid variables will have an over-bar.
The solution in the solid is
\begin{align*}
\hat{\bar{u}}_r &= \phantom{-}
d_1 \left(\frac{n J_n(k_p r)}{r} - k_p J_{n+1}(k_p r) \right)
+ d_2 \left(\frac{n Y_n(k_p r)}{r} - k_p Y_{n+1}(k_p r) \right)
+ \frac{i n }{r} \left(d_3 J_n (k_s r) + d_4 Y_n(k_s r) \right) \\
\hat{\bar{u}}_{\theta} &= -d_3 \left(\frac{n J_n(k_s r)}{r} - k_s J_{n+1}(k_s r) \right)
- d_4 \left(\frac{n Y_n(k_s r)}{r} - k_s Y_{n+1}(k_s r) \right)
+ \frac{i n }{r} \left(d_1 J_n (k_p r) + d_2 Y_n(k_p r) \right).
\end{align*}

\subsection{Boundary value problem}

\newcommand{\Rf}{1}
\newcommand{\Rs}{2}
\newcommand{\angA}{30}
\newcommand{\angB}{60}
\newcommand{\Hss}{1}
\newcommand{\Lss}{1.5}
\newcommand{\gap}{.3}
\newcommand{\lw}{0.25mm}
\newcommand{\colF}{blue}
\newcommand{\colS}{red}
\newcommand{\colIf}{green}
\newcommand{\colIs}{cyan}

The fluid is in the domain ($0 < r < R_I$) and the solid is in
($R_I < r < R_s$).
\begin{figure}[h]
  \centering
  \begin{tikzpicture}
    \coordinate (A) at (0,0);
    \coordinate (B) at (\Rf*cos{\angA},\Rf*sin{\angA});
    \coordinate (C) at (\Rs*cos{\angB},\Rs*sin{\angB});
    \coordinate (D) at (0,.5*\Rf+.5*\Rs);
    \coordinate (E) at (\Rs,0);
    \coordinate (F) at (1.5*\Rs,.5*\Rf);
    \coordinate (G) at (-\Rf,0);
    \coordinate (H) at (-1.5*\Rs,.5*\Rf);

    % \node [fill=green,circle] at (A) {}; 
    % \node [fill=red,  circle] at (B) {};
    % \node [fill=blue, circle] at (B) {};

    % \draw [\colF] (A) to[out=90,in=-90] (B);
    % \draw [\colF] (B) to[out=0,in=180] (C);
    % \draw [\colF] (C) to[out=-90,in=90] (D);
    % \draw [\colF] (D) to[out=180,in=0] (A);

    % fluid
    \draw [line width=\lw,\colF] (A) circle(\Rf);
    \draw [->,line width=\lw,\colF] (A) to (B);
    \draw (B) node[\colF,right] {$R_I$};
    \draw (A) node[\colF,below] {fluid};

    \draw [line width=\lw] (G) to (H);
    \draw (H) node[anchor=east,align=center] {$\sigmav \cdot \nv = \sigmasv \cdot \nv$ \\ $\vv = \vsv$};

    % \draw (\Lf/2,\Hf/2) node[\colF] {$\Omega(t)$};

    % solid
    \draw [line width=\lw,\colS] (A) circle(\Rs);
    \draw [->,line width=\lw,\colS] (A) to (C);
    \draw (C) node[\colS,right] {$R_s$};    
    \draw (D) node[\colS] {solid};
    % \draw (\Ls/2,-\gap-\Hss/2) node[\colS] {$\bar{\Omega}$};

    \draw [line width=\lw] (E) to (F);
    \draw (F) node[right] {$\sigmasv \cdot \nv = \textbf{0}$};

  \end{tikzpicture}
  \caption{Diagram of fluid and solid domain and boundary conditions.}
\end{figure}

The free surface boundary condition is
\begin{align}
\hat{\sigmas}_{rr}(R_s) &= 0 \\
\hat{\sigmas}_{r\theta}(R_s) &= 0
\end{align}
%
The kinetic conditions between the fluid and solid are
\begin{align}
\hat{\sigma}_{rr}(R_I) &= \hat{\sigmas}_{rr}(R_I) \\
\hat{\sigma}_{r\theta}(R_I) &= \hat{\sigmas}_{r\theta}(R_I).
\end{align}
%
The dynamic conditions between the fluid and solid are
\begin{align}
\hat{v}_r(R_I) &= \hat{\vs}_r(R_I) \\
\hat{v}_\theta(R_I) &= \hat{\vs}_\theta(R_I).
\end{align}
%
The free constants are $d_1,\, d_2,\, d_3,\, d_4,\, c_1,\, p_0.$ 
The maple code\\
\texttt{fibr/codes/testSolutions/radialVibrations/m3\_fsi\_eigenvalue\_problem.mw} \\
generates matlab code for the dispersion matrix.
The matlab code \\
\texttt{fibr/codes/testSolutions/radialVibrations/m3\_fsi\_eigenvalue\_PolarTravelingWaveFSIFibr.m} \\
computes the frequencies, $\omega,$ and plots the solution.

\begin{table}[H]
\centering
\caption{Table of frequencies for $1 \le n \le 4$ with $R_I=1,\, 
R_s=1.2,\, \mu = 0.1,\, \rho = 1,\, \mus=1,\, \lambdas=1,\, \rhos=1.$}
\begin{tabular}{|c|c|}
\hline
$n$ & $\omega$ \\
\hline
1 & -1.1250     $-$ 0.3209i\\
2 & -2.2704     $-$ 0.6868i\\
3 & -3.4912     $-$ 1.1543i\\
4 & -4.7519     $-$ 1.7808i\\
\hline
\end{tabular}
\end{table}


==> texFiles/rpiFig.tex <==
{
\newcommand{\trimfigRPI}[2]{\trimhb{#1}{#2}{.2}{.25}{.375}{.375}}
\newcommand{\trimfigRPIg}[2]{\trimhb{#1}{#2}{.15}{.5}{.35}{.35}}
\newcommand{\trimfigRPIz}[2]{\trimhb{#1}{#2}{.575}{.34}{.49}{.44}}

\begin{figure}[h]
  \centering
  \resizebox{!}{!}{% START resize box
    \begin{tikzpicture}
      \useasboundingbox(0,0) rectangle (16,-3);
      \def\cxl{-.1}
      \def\cxr{11.5}
      \def\cyu{0}
      \def\cyl{-5}
      \def\wx{2.6}

      \draw(\cxl,\cyu) node[anchor=north west,xshift=-.5cm] {
        \trimfigRPI{fig/rpiGridNew0.pdf}{\wx cm}
      };
      \draw(\cxl+6.6,\cyu) node[anchor=north west,xshift=-.5cm] {
        \trimfigRPI{fig/rpiSolution300.pdf}{\wx cm}
      };

      % \draw(\cxr,\cyu) node[anchor=north west,xshift=-.5cm] {
      %   \trimfigRPIz{fig/rpiGrid0.pdf}{\wx cm}
      % };
      \draw(\cxl+6.6+6.6,\cyu) node[anchor=north west,xshift=-.5cm] {
        \trimfigRPIz{fig/rpiGridNew300.pdf}{\wx cm}
      };

      % grid lines
      % \draw[step=1cm,gray] (0,0) grid (16,-10);
    \end{tikzpicture}
  }
  \caption{Left: Initial grid composed of a (blue) background grid and (green)
    deforming interface-fitted grids. The `RPI' shaped solid domain is 
    composed of (red) background grids, (purple) interface-fitted grids,
    and (pink) annular grids around interior cores.
    % Top right: Zoomed-in view of initial grid around upper region of the letter `I'.
    Middle: Solution at $t=15$ depicting 
    streamlines in the fluid domain and shaded contours of the magnitude 
    of the solid displacement. 
    Right: Zoomed-in view of grid after solid deformation.
    \label{fig:rpiFig}}
\end{figure}

}

% {
% \newcommand{\trimfigRPI}[2]{\trimhb{#1}{#2}{.15}{.15}{.35}{.35}}
% \newcommand{\trimfigRPIz}[2]{\trimhb{#1}{#2}{.66}{.24}{.47}{.43}}

% \begin{figure}[h]
%   \centering
%   \resizebox{5in}{!}{% START resize box
%     \begin{tikzpicture}
%       \useasboundingbox(0,0) rectangle (16,-9.75);
%       \def\cxl{0}
%       \def\cxr{11.5}
%       \def\cyu{0}
%       \def\cyl{-5}
%       \def\wx{4.5}
%       \draw(\cxl,\cyu) node[anchor=north west,xshift=-.5cm] {
%         \trimfigRPI{fig/rpiGrid0.pdf}{\wx cm}
%       };
%       \draw(\cxl,\cyl) node[anchor=north west,xshift=-.5cm] {
%         \trimfigRPI{fig/rpiSolution.pdf}{\wx cm}
%       };

%       \draw(\cxr,\cyu) node[anchor=north west,xshift=-.5cm] {
%         \trimfigRPIz{fig/rpiGrid0.pdf}{\wx cm}
%       };
%       \draw(\cxr,\cyl) node[anchor=north west,xshift=-.5cm] {
%         \trimfigRPIz{fig/rpiGrid801.pdf}{\wx cm}
%       };

%       % grid lines
%       \draw[step=1cm,gray] (0,0) grid (16,-10);
%     \end{tikzpicture}
%   }
%   \caption{Top left: Initial grid composed of a (blue) background grid and (green)
%     deforming interface-fitted grids. The `RPI' shaped solid domain is 
%     composed of (red) background grids, (orange) interface-fitted grids,
%     and (purple) annular grids around interior cores.
%     Top right: Zoomed-in view of initial grid around upper region of the letter `I'.
%     Bottom left: Solution at $t=50$ depicting 
%     streamlines in the fluid domain and shaded contours of the magnitude 
%     of the solid displacement. 
%     Bottom right: Zoomed-in view of grid after solid deformation.
%     \label{fig:rpiFig}}
% \end{figure}

% }

==> texFiles/solidEllipseInAChannel.tex <==

\subsection{Elastic ellipse in a channel} \label{sec:elasticEllipseInAChanell}

Here is a potential example. An elliptical solid with a hole is placed in a cross flow.

\newcommand{\Gce}{\Gc_e}
% \input texFiles/balloonFig.tex

{% ----------- ELASTIC ELLIPSE  ------  
%
\newcommand{\figWidtha}{5cm}% width
\newcommand{\trimfiga}[2]{\trimwb{#1}{#2}{.0}{.0}{.0}{.0}}
\newcommand{\figWidth}{5cm}% width
% \newcommand{\trimfig}[2]{\trimwb{#1}{#2}{.2}{.2}{.25}{.25}}
\newcommand{\trimfig}[2]{\trimwb{#1}{#2}{.2}{.2}{.25}{.25}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (15,5);  % set the bounding box (so we have less surrounding white space)

   \draw(-.75,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfiga{fig/rotatedEllipseGride4}{\figWidtha}};
% 
   \draw(4.5,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/ellipseG4Scf5StreamLinesAndDisplacement}{\figWidth}};
   \draw(10,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/ellipseG4Scf2StreamLinesAndDisplacement}{\figWidth}};
   % grid:
 \draw[step=1cm,gray] (0,0) grid (15,5);
\end{tikzpicture}
\end{center}
  \caption{Left: composite grid $\Gcd^{(4)}$ for the solid ellipse in a channel.
    The green fluid grid adjacent to the interface moves over time while the blue fluid background grid remains fixed.
    The red-shaded grids for the solid reference domain also remains fixed over time.
   Streamlines and solid displacement norm for $\scf=5$ and $\scf=2$.
%    Middle and right: fluid pressure and $\| \sigmavs\|$ at times $t=2$ and $t=9$, computed
%       on grid $\Gcb^{(8)}$. \wdh{wdh: add colour bars}
}
  \label{fig:elasticEllipse}
\end{figure}
}


{% ----------- ELASTIC ELLIPSE  ------  
%
\newcommand{\figWidtha}{4.5cm}% width
\newcommand{\trimfiga}[2]{\trimhb{#1}{#2}{.05}{.05}{.3}{.3}}
\newcommand{\figWidth}{6cm}% width
\newcommand{\trimfig}[2]{\trimwb{#1}{#2}{.1}{.1}{.2}{.2}}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}[scale=1]
  \useasboundingbox (0,0.5) rectangle (15,5);  % set the bounding box (so we have less surrounding white space)

   \draw(0,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/ellipseG4LongScf5StreamLinesAndDisplacement}{\figWidth}};
% 
  \draw(6,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfiga{fig/ellipseG4LongerScf10StreamLinesAndDisplacement}{\figWidtha}};
%    \draw(10,0.0) node[anchor=south west,xshift=-15pt,yshift=-8pt] {\trimfig{fig/ellipseG4Scf2StreamLinesAndDisplacement}{\figWidth}};
   % grid:
% \draw[step=1cm,gray] (0,0) grid (15,5);
\end{tikzpicture}
\end{center}
  \caption{
   Streamlines and solid displacement norm for $\scf=5$ at $t=10$ -- this may be too small a value for $\delta$
   Right: $\scf=10$, $t=30$. 
}
  \label{fig:elasticEllipseFlow}
\end{figure}
}



==> texFiles/stabilityAnalysisNotes.tex <==
The system of equations that arise in the FIB analysis are
\begin{align}
\partial_t a + \cp \partial_y a &= i k_x \cp d \\
\partial_t b - \cp \partial_y b &= -i k_x \cp d \\
\partial_t d &= \frac{i k_x \cp}{2} (b-a)
\end{align}
%
Let $\av = [a,b,d]^T.$ Search for spatially independent solutions of the form
$\av = \cv e^{\lambda t}.$
\begin{align}
\lambda \cv &= 
\left[\begin{array}{ccc}
0 & 0 & i k_x \cp \\
0 & 0 & - i k_x \cp \\
\frac{- i k_x \cp}{2} & \frac{i k_x \cp}{2} & 0
\end{array}\right]
\cv 
\end{align}
%
$\lambda$ is an eigenvalue of the RHS matrix.
\begin{align*}
\left|\begin{array}{ccc}
-\lambda & 0 & i k_x \cp \\
0 & -\lambda & - i k_x \cp \\
\frac{- i k_x \cp}{2} & \frac{i k_x \cp}{2} & -\lambda
\end{array}\right| &= 0 \\
(-\lambda)^3 - (-\lambda)(-i k_x \cp)\left(\frac{i k_x \cp}{2}\right)
- (i k_x \cp) (-\lambda) \left(- \frac{i k_x \cp}{2}\right) &= 0 \\
- \lambda^3 
- \frac{\lambda i^2 k_x^2 \cp^2}{2}
- \frac{\lambda i^2 k_x^2 \cp^2}{2} &= 0 \\
- \lambda^3 + \lambda k_x^2 \cp^2 &= 0 \\
\lambda (- \lambda^2 + k_x^2 \cp^2) &= 0 
\end{align*}
% 
Therefore, $\lambda = 0,\, \pm k_x \cp.$

==> texFiles/stabilityNotes.tex <==
\newcommand{\Hbar}{\bar{H}}
\section{A variational analysis of the monolithic scheme}

\wdh{WDH Aug. 5 2018. Here we try to understand how the interface velocity and traction depend
on the various parameters in the scheme so as to expose the form of the fluid impedance $\zf$.}

\bigskip\noindent
Consider the geometry for the block elastic piston.

\input texFiles/rectangularModelProblemCartoon

Discretize the problem in time using an implicit monolithic scheme.
For the incompressible fluid this gives
\bas
& \rho \f{\vv^{n+1} - \vv^n}{\dt} + \grad p^{n+1} = \mu \Delta \vv^{n+1} , \\
&  \Delta p^{n+1} = 0 , \\
& \grad\cdot\vv^{n+1} = 0 
\eas
and for the acoustic solid  (ignore the $\dv$ component for now)
\bas
&  \f{\av^{n+1} - \av^{n}}{\dt} - \cb \partial_y \av^{n+1} = ...,  \\
&  \f{\bv^{n+1} - \bv^{n}}{\dt} + \cb \partial_y \bv^{n+1} = ...
\eas
where $\nv=[0,1]^T$ and
\bas
& \av \eqdef \sigmavs\nv + \zs\vsv , \\
& \bv \eqdef \sigmavs\nv - \zs\vsv . 
\eas
Here $\av$ is downward directed characteristic variable and $\bv$ is the upward.

Take as boundary conditions for the fluid on the top a pressure BC (we could instead take a no-slip wall)
\bas
   p(x,H,t)=p_H(x,y), \qquad u(x,H,t)=u_H(x,t),
\eas
and boundary conditions for the solid at the bottom (this currently plays no role)
\bas
     \vvs(x,\Hbar,t) = \vvs_{\Hbar} .
\eas
The interface conditions are
\bas
  [ \vv ]=0, \qquad [\sigmav\nv ]=0 .
\eas

\bigskip\noindent
The above equations define the solution at the new time in terms of the boundary conditions.
Consider \textbf{perturbing} the boundary conditions by a small amount (e.g. $P_H \rightarrow P_H+\delta P_H$),
resulting in a
pertubation to the solution at the new time, $\vv^{n+1} \rightarrow \vv^{n+1} + \delta\vv^{n+1}$, $p\rightarrow p+\delta p$, etc..
The variational equations for the perturbations are (dropping the $\delta$ and using $\vv$, $p$,
etc. to denote the perturbations),
\bas
& \rho \f{\vv^{n+1}}{\dt} + \grad p^{n+1} = \mu \Delta \vv^{n+1} , \\
&  \Delta p^{n+1} = 0 , \\
& \grad\cdot\vv^{n+1} = 0 , 
\eas
and
\bas
&  \f{\av^{n+1} }{\dt} - \cb \partial_y \av^{n+1} = 0 , \\
&  \f{\bv^{n+1} }{\dt} + \cb \partial_y \bv^{n+1} = 0
\eas
We now solve the perturbation equations.
We now expand the solutions in a Fourier series in $x$,
\bas
  &   \vv(x,y,t) = \hat{\vv}_k(y,t) e^{i k x}, \\
  &   p(x,y,t) = \hat{p}_k(y,t) e^{i k x}, \\
  &   \av(x,y,t) = \hat{\av}_k(y,t) e^{i k x}, \\
  &   \bv(x,y,t) = \hat{\bv}_k(y,t) e^{i k x}.
\eas
After dropping the hats letting $\vv=[u,v]^T$, we get for the
fluid, 
\bas
&  \rho \f{u}{\dt} + i k p = \mu ( -k^2 u + \partial_y^2 u  ) , \\
&  \rho \f{v}{\dt} + \partial_y p = \mu ( -k^2 v + \partial_y^2 v ) , \\
&    -k^2 p + \partial_y^2 p = 0 , \\
&    i k u + \partial_y v = 0
\eas
The solution for $p$ satisfying $p(H,t)=p_H$ and $p(0,t)=P$ is 
\bas
   p = p_H \f{\sinh(ky)}{\sinh(kH)}  - P \, \f{\sinh(k(y-H))}{\sinh(kH)}, 
\eas
where $P$ is a free constant.
The solution for $v$ consists of a solution to the homogeneous equation plus a particular solution, *check me*
\bas
 &    v = A e^{\beta y} + B e^{-\beta y} + v_p ,\\
 &    v_p = -\f{\dt}{\rho}\partial_y p = -\f{k\dt}{\rho} p_H  \f{\cosh(ky)}{\sinh(kH)}  + \f{k\dt}{\rho}   P \f{\cosh(k(y-H))}{\sinh(kH)}  \\
 &  \beta \eqdef \sqrt{ \f{\rho}{\mu\dt} + k^2}
\eas
where $A$ and $B$ are free constants. 
Given $v$, $u$ can be found from the divergence condition, $u =  (i/k) \partial_y v$, 
\bas
& u = \f{i}{k} \beta A e^{\beta y} - \f{i}{k} \beta B e^{-\beta y} + u_p , \\
& u_p = \f{i}{k} \partial_y v_p , 
\eas
Applying the BC $u=u_H$ at $y=H$ implies
\ba
& u_H = \f{i}{k} \beta A e^{\beta H} - \f{i}{k} \beta B e^{-\beta H} + u_p(H) \label{eq:topU}
\ea
which gives one relation between $A$, $B$ and $P$. Note that when $e^{\beta H}$ is large this condition
implies $A\approx 0$.

In the solid we have
\bas
&  \av = \av_0 \, e^{y/(\cb\dt)}, \\
&  \bv = \bv_0 \, e^{-y/(\cb\dt)}. 
\eas
for constants $\av_0$ and $\bv_0$. Let us assume that $\bv_0$ is known from the interior for
the upward directed characteristic.

To apply the interface conditions we first impose 
\ba
   \sigmav\nv - \zb \vv = \bv_0 . \label{eq:interfaceFluid}
\ea
The two conditions in~\eqref{eq:interfaceFluid} plus the condition~\eqref{eq:topU} will determine  $A$, $B$ and $P$ and
thus will determine the solution
in the fluid. Given the fluid solid, the other interface condition
\bas
   \av_0 = \sigmav\nv + \zb \vv, 
\eas
will give $\av_0$ and whence the solid solution will be known.   

With $\nv=[0,1]^T$, interface condition~\eqref{eq:interfaceFluid} is written out as 
\bas
&    -p + 2\mu\, \partial_y v - \zb v = \nv^T\bv_0, \\
&     \mu( \partial_y u + i k v) - \zb u = \tv^T\bv_0. 
\eas
Substituting for $u$, $v$ and $p$ gives *FIX ME -- this is wrong*
\bas
& - p_H e^{kH} + P \, \sinh(kH) +
        2\mu\Big( \beta A - \beta B  - \f{k^2\dt}{\rho} p_H  e^{kH}  - \f{k^2\dt}{\rho} P \cosh(kH) \Big)\\
& \qquad\qquad        -\zb\Big( A+B + \f{k\dt}{\rho} p_H  e^{kH}  - \f{k\dt}{\rho}   P \cosh(kH)\Big) = \nv^T\bv_0, \\
% 
& \mu\Big( \f{i}{k} \beta^2 A  + \f{i}{k} \beta^2 B
        +\f{i k^2\dt}{\rho} p_H  e^{kH}  + \f{i k^2\dt}{\rho} P \sinh(kH)+
        ik\big( A+B + \f{k\dt}{\rho} p_H  e^{kH}  - \f{k\dt}{\rho}   P \cosh(kH)\ \big)  \Big) \\
        & \qquad         -\zb\Big(\f{i}{k} \beta A - \f{i}{k} \beta B
              -\f{i k\dt}{\rho} p_H  e^{kH}  + \f{i k\dt}{\rho}  P \sinh(kH) \Big) = \tv^T\bv_0.
\eas
These equations can be solved for $A$, $B$ and $P$ to give the interface velocity and traction
\bas
& \vv^I \eqdef \vv\vert_{y=0} , \\
& \nv^T\sigmav^I \eqdef (-p\nv + \tauv\nv)\vert_{y=0}
\eas
or
\bas
&   u^I = \\
&   v^I = A + B + \f{k\dt}{\rho}\f{(P-p_H)}{\tanh(kH)} , \\
& p^I = P 
\eas
Note that the values of  $A$, $B$ and $P$ will be complex and the solution in real space will be $\Re(\hat{\vv} e^{i k x})$. 

\medskip
The inteface velocity will be composed of two parts, one proportional to $\bv_0$,
\bas
\vv^I  & = \wv + C \bv_0 = \wv + C (\sigmasv\nv - \zb\vvs) 
% \nv^T\sigmav^I \eqdef (-p\nv + \tauv\nv)\vert_{y=0}
\eas
We wish to write this in the form of an impedance weighted average, \textbf{\red Maybe this is the wrong assumed form?}
\bas
\vv^I  & = \f{z_f}{z_f+\zb} \vv^f + \f{\zb}{z_f+\zb}\vvs + \f{1}{z_f+\zb} [ \sigmav\nv].
\eas
for some appropriate $z_f$ and $\vv^f$. 

See maple code fibr/maple/monolithic.maple for code to solve for $A$, $B$ and $P$. Results are
( nb=$\nv^T\bv_0$, tb=$\tv^T\bv_0$)
{\tiny
\bas
& u^I = {\frac {i \left(  \left(  \left( -i{k}^{2}z{\it tb}+2\,{k}^{3}\mu\,{\it nb} \right) {\it dt}+\rho\, \left( i\beta\,{\it tb}+k{\it nb} \right)  \right) \sinh \left( kH \right) + \left( \beta\, \left( iz{\it tb}-2\,k\mu\,{\it nb} \right) \cosh \left( kH \right) -2\, \left( \beta\,\mu+z/2 \right) {\it pH}\,k \right) k{\it dt} \right) {\it dt}\,{{\rm e}^{2\,\beta\,H}}+ \left( -2\,i \left( i\rho\,{\it uH}-k{\it dt}\,{\it pH} \right)  \left( 2\,{\it dt}\,{k}^{2}\mu+\rho \right) {{\rm e}^{\beta\,H}}-i \left( {k}^{2} \left( iz{\it tb}-2\,k\mu\,{\it nb} \right) {\it dt}+\rho\, \left( i\beta\,{\it tb}-k{\it nb} \right)  \right) {\it dt} \right) \sinh \left( kH \right) -2\,i \left(  \left(  \left( i\rho\,{\it uH}-k{\it dt}\,{\it pH} \right) z{{\rm e}^{\beta\,H}}+1/2\,{\it dt}\,\beta\, \left( iz{\it tb}-2\,k\mu\,{\it nb} \right)  \right) \cosh \left( kH \right) -{\it pH}\, \left( \beta\,\mu-z/2 \right) k{\it dt} \right) k{\it dt}}{ \left(  \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+\rho\, \left( 4\,{k}^{2}\mu+\beta\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) +\cosh \left( kH \right) k \left(  \left( -4\,\beta\,{k}^{2}{\mu}^{2}+\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) {\it dt} \right) {{\rm e}^{2\,\beta\,H}}+ \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}-\rho\, \left( -4\,{k}^{2}\mu+\beta\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) +\cosh \left( kH \right) k{\it dt}\, \left(  \left( 4\,\beta\,{k}^{2}{\mu}^{2}-\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) }} \\
& v^I = -4\,{\frac { \left(  \left(  \left(  \left( i/2{k}^{2}\mu\,{\it tb}-1/4\,kz{\it nb} \right) {\it dt}+i/4\rho\,{\it tb} \right) \sinh \left( kH \right) + \left( -1/2\, \left( ik\mu\,{\it tb}-1/2\,{\it nb}\,z \right) \beta\,{\it dt}+1/4\,\rho\,{\it nb} \right) \cosh \left( kH \right) +1/4\,{\it pH}\, \left(  \left( 2\,{k}^{2}\mu+\beta\,z \right) {\it dt}+\rho \right)  \right) {{\rm e}^{2\,\beta\,H}}+ \left( 1/2\, \left( i\rho\,{\it uH}-k{\it dt}\,{\it pH} \right) z{{\rm e}^{\beta\,H}}+ \left( i/2{k}^{2}\mu\,{\it tb}-1/4\,kz{\it nb} \right) {\it dt}+i/4\rho\,{\it tb} \right) \sinh \left( kH \right) + \left(  \left( i\rho\,{\it uH}-k{\it dt}\,{\it pH} \right) \mu\,k{{\rm e}^{\beta\,H}}+1/2\, \left( ik\mu\,{\it tb}-1/2\,{\it nb}\,z \right) \beta\,{\it dt}+1/4\,\rho\,{\it nb} \right) \cosh \left( kH \right) +1/4\, \left(  \left( 2\,{k}^{2}\mu-\beta\,z \right) {\it dt}+\rho \right) {\it pH} \right) k{\it dt}}{ \left(  \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+\rho\, \left( 4\,{k}^{2}\mu+\beta\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) +\cosh \left( kH \right) k \left(  \left( -4\,\beta\,{k}^{2}{\mu}^{2}+\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) {\it dt} \right) {{\rm e}^{2\,\beta\,H}}+ \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}-\rho\, \left( -4\,{k}^{2}\mu+\beta\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) +\cosh \left( kH \right) k{\it dt}\, \left(  \left( 4\,\beta\,{k}^{2}{\mu}^{2}-\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) }} \\
& p^I = {\frac { \left( 2\,\rho\, \left(  \left( -{k}^{2}\mu\,{\it nb}+i{\it tb}\, \left( \beta\,\mu+z/2 \right) k-1/2\,\beta\,z{\it nb} \right) {\it dt}-1/2\,\rho\,{\it nb} \right) \sinh \left( kH \right) +{\it pH}\,k \left(  \left( -4\,\beta\,{k}^{2}{\mu}^{2}+\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) {\it dt} \right) {{\rm e}^{2\,\beta\,H}}+ \left( -4\, \left( i\rho\,{\it uH}-k{\it dt}\,{\it pH} \right) k \left(  \left( 2\,{\mu}^{2}{k}^{2}-1/2\,{z}^{2} \right) {\it dt}+\mu\,\rho \right) {{\rm e}^{\beta\,H}}-2\,\rho\, \left(  \left( {k}^{2}\mu\,{\it nb}+i{\it tb}\, \left( \beta\,\mu-z/2 \right) k-1/2\,\beta\,z{\it nb} \right) {\it dt}+1/2\,\rho\,{\it nb} \right)  \right) \sinh \left( kH \right) +{\it pH}\,k{\it dt}\, \left(  \left( 4\,\beta\,{k}^{2}{\mu}^{2}-\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) }{ \left(  \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+\rho\, \left( 4\,{k}^{2}\mu+\beta\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) +\cosh \left( kH \right) k \left(  \left( -4\,\beta\,{k}^{2}{\mu}^{2}+\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) {\it dt} \right) {{\rm e}^{2\,\beta\,H}}+ \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}-\rho\, \left( -4\,{k}^{2}\mu+\beta\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) +\cosh \left( kH \right) k{\it dt}\, \left(  \left( 4\,\beta\,{k}^{2}{\mu}^{2}-\beta\,{z}^{2} \right) {\it dt}+\rho\,z \right) }}
\eas
}
Here are the forms for large $e^{k H}$,
\bas
& u^I \sim 2\,{\frac { \left(  \left( i\mu\,{\it nb}\,k+1/2\,z{\it tb} \right)  \left( k-\beta \right) k{\it dt}+1/2\,\rho\, \left( ik{\it nb}-\beta\,{\it tb} \right)  \right) {\it dt}}{ \left( -4\,\beta\,{k}^{3}{\mu}^{2}+4\,{k}^{4}{\mu}^{2}+\beta\,k{z}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+4\,\rho\, \left( {k}^{2}\mu+1/4\,kz+1/4\,\beta\,z \right) {\it dt}+{\rho}^{2}}}\\ 
& v^I \sim -2\,{\frac { \left(  \left( ik\mu\,{\it tb}-1/2\,{\it nb}\,z \right)  \left( k-\beta \right) {\it dt}+1/2\,\rho\, \left( i{\it tb}+{\it nb} \right)  \right) k{\it dt}}{ \left( -4\,\beta\,{k}^{3}{\mu}^{2}+4\,{k}^{4}{\mu}^{2}+\beta\,k{z}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+4\,\rho\, \left( {k}^{2}\mu+1/4\,kz+1/4\,\beta\,z \right) {\it dt}+{\rho}^{2}}}\\ 
& p^I \sim {\frac {\rho\, \left(  \left( -2\,{k}^{2}\mu\,{\it nb}+i{\it tb}\, \left( 2\,\beta\,\mu+z \right) k-\beta\,z{\it nb} \right) {\it dt}-{\it nb}\,\rho \right) }{ \left( -4\,\beta\,{k}^{3}{\mu}^{2}+4\,{k}^{4}{\mu}^{2}+\beta\,k{z}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+4\,\rho\, \left( {k}^{2}\mu+1/4\,kz+1/4\,\beta\,z \right) {\it dt}+{\rho}^{2}}}
\eas


The coefficient in $v^I$ that multiplies
$\nv^T\bv_0=\nv^T\sigmasv\nv - \zb\nv^T\vvs$ is  
{\scriptsize
\bas
& c = \f{n}{d}\\
& n = {\it dt}\,k \left(  \left(  \left( -\beta\,z{\it dt}-\rho \right) \cosh \left( kH \right) +{\it dt}\,kz\sinh \left( kH \right)  \right) {{\rm e}^{2\,\beta\,H}}+ \left( \beta\,z{\it dt}-\rho \right) \cosh \left( kH \right) +{\it dt}\,kz\sinh \left( kH \right)  \right)  \\
& d =  \left(  \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+ \left( 4\,{k}^{2}\mu\,\rho+\beta\,\rho\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) -4\,{\it dt}\,k \left(  \left( {k}^{2}{\mu}^{2}\beta-1/4\,{z}^{2}\beta \right) {\it dt}-1/4\,\rho\,z \right) \cosh \left( kH \right)  \right) {{\rm e}^{2\,\beta\,H}}\\
& + \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+ \left( 4\,{k}^{2}\mu\,\rho-\beta\,\rho\,z \right) {\it dt}+{\rho}^{2} \right) \sinh \left( kH \right) +4\,{\it dt}\,k \left(  \left( {k}^{2}{\mu}^{2}\beta-1/4\,{z}^{2}\beta \right) {\it dt}+1/4\,\rho\,z \right) \cosh \left( kH \right) 
\eas
}
Note that $nb$ and $tb$ are COMPLEX.
For large $e^{\beta H}$ and large $e^{kH}$, only the terms involving $e^{2\beta H}$ remain and we have
\bas
\f{n}{d}= \frac{ {\it dt}\,k  \left(  \left( -\beta\,z{\it dt}-\rho \right) +{\it dt}\,kz \right) }
    { \left(  \left(  \left( 4\,{k}^{4}{\mu}^{2}-{k}^{2}{z}^{2} \right) {{\it dt}}^{2}+ \left( 4\,{k}^{2}\mu\,\rho+\beta\,\rho\,z \right) {\it dt}+{\rho}^{2} \right)  -4\,{\it dt}\,k \left(  \left( {k}^{2}{\mu}^{2}\beta-1/4\,{z}^{2}\beta \right) {\it dt}-1/4\,\rho\,z \right)   \right)  }
\eas
% \bas
% \f{n}{d}= \frac{ k{\it dt}\, \left(  \left(  \left( -{\beta}^{2}\mu+{k}^{2}\mu-\beta\,z \right)  +kz  \right)\right)}
%     { \left(  \left( 2\,{k}^{4}{\it dt}\,{\mu}^{2}+ \left(  \left( 2\,{\beta}^{2}{\mu}^{2}-{z}^{2} \right) {\it dt}+\mu\,\rho \right) {k}^{2}+\rho\,\beta\, \left( \beta\,\mu+z \right)  \right)  -k \left( \mu\, \left( 4\,\beta\,\mu+z \right) {k}^{2}-z\mu\,{\beta}^{2}-{z}^{2}\beta \right)  {\it dt} \right) }
% \eas
The ratio $n/d$ should approach $-1/z$ for $z$ large since $\vv^I$ should approach $\vvs$.
For large $z$ we have
\bas
\f{n}{d}= \frac{ k\dt^2\, (k-\beta)z }
    { z^2( -k^2\dt^2 + k \beta\dt^2) } 
 = - \f{1}{z}
\eas
The ratio $-d/n$ should look like $z_f + \zb$ thus *check me*
\bas
&   z_f^v = -\f{d}{n} - z , \\
% & z_f^v = {\frac {-4\,{k}^{3}{\mu}^{2} \left( k-\beta \right) {{\it dt}}^{2}+ \left( -4\,{k}^{2}\mu\,\rho-\beta\,\rho\,z \right) {\it dt}-{\rho}^{2}}{ \left( z \left( k-\beta \right) {\it dt}-\rho \right) k{\it dt}}} ,\\
%
& z_f^v = {\frac {-4\,{k}^{3}{\mu}^{2} \left( \beta-k \right) {{\it dt}}^{2}+ \left( 4\,{k}^{2}\mu\,\rho +\beta\,\rho\,z \right) {\it dt} +{\rho}^{2}}{ \left( z \left( \beta -k \right) {\it dt} +\rho \right) k{\it dt}}} 
\eas
Here is the impedance coming from the $u^I$ equation (coeff of $\tv^\bv_0$), on term is different ($\rho \beta z \dt \rightarrow \rho k z \dt$)
\bas
z_{f}^u \sim {\frac {-4\,{k}^{3}{\mu}^{2} \left( k-\beta \right) {{\it dt}}^{2}-4\,\rho\, \left( k\mu+z/4 \right) k{\it dt}-{\rho}^{2}}{{\it dt}\, \left( zk \left( k-\beta \right) {\it dt}-\beta\,\rho \right) }}
\eas  

% On the other hand, using the coefficient of $\tv^T\bv_0$ in $v^I$ leads to the impedance 
% \bas
% & z_{f2} = 1/2\,{\frac {2\,i \left( k-\beta \right) k \left( iz\mu\,k-2\,{\mu}^{2}{k}^{2}+1/2\,{z}^{2} \right) {{\it dt}}^{2}+i\rho\, \left( -4\,{k}^{2}\mu- \left( 1-i \right) zk-\beta\,z \right) {\it dt}-i{\rho}^{2}}{{\it dt}\, \left( k\mu\, \left( k-\beta \right) {\it dt}+\rho/2 \right) k}}
% \eas
% which has real and imaginary parts. \wdh{What does $z_{f2}$ mean ? Doesn't look right as $z\rightarrow \infty$.}


If we assume that we take a large viscous CFL number, 
\newcommand{\viscousCFL}{\Lambda_\nu}
\bas
& \viscousCFL \eqdef \f{\mu}{\rho}\dt k^2 = \nu \dt k^2 \gg 1,
\eas
then
\bas
 \beta - k &= \sqrt{ \f{\rho}{\mu\dt} + k^2} -k = k\sqrt{1+\f{1}{\viscousCFL}} -k \approx k + \frac{k}{2\viscousCFL} - k 
           = \frac{k}{2\viscousCFL} = \frac{\rho}{2 \mu \dt k} 
\eas
Substituting this approximation for $\beta$ gives *check me*
\bas
  z_f & \approx {\frac {-4\,{k}^{3}{\mu}^{2} \left( \frac{k}{2\viscousCFL} \right) {{\it dt}}^{2}+ \left( 4\,{k}^{2}\mu\,\rho +\beta\,\rho\,z \right) {\it dt} +{\rho}^{2}}{ \left( z \left( \frac{k}{2\viscousCFL} \right) {\it dt} +\rho \right) k{\it dt}}} \\
%       &= {  \frac {-4\,  \rho^2\viscousCFL^2 \left( \frac{1}{2\viscousCFL} \right) + \left( 4\,{k}^{2}\mu\,\rho +\beta\,\rho\,z \right) {\it dt} +{\rho}^{2}}{ \left( z \left( \frac{k}{2\viscousCFL} \right) {\it dt} +\rho \right) k{\it dt}}} \\
%       &= {  \frac {-2\,  \rho^2\viscousCFL + \left( 4\,{k}^{2}\mu\,\rho +\beta\,\rho\,z \right) {\it dt} +{\rho}^{2}}{ \left( z \left( \frac{k}{2\viscousCFL} \right) {\it dt} +\rho \right) k{\it dt}}} \\
%      &= {  \frac {-2\,  \rho \mu k^2 \dt + \left( 4\,{k}^{2}\mu\,\rho +\beta\,\rho\,z \right) {\it dt} +{\rho}^{2}}{ \left( z \left( \frac{k}{2\viscousCFL} \right) {\it dt} +\rho \right) k{\it dt}}} \\
      &= {  \frac {\left( 2\,{k}^{2}\mu\,\rho +\beta\,\rho\,z \right) {\it dt} +{\rho}^{2}}{ \left( z \left( \frac{k}{2\viscousCFL} \right) {\it dt} +\rho \right) k{\it dt}}} \\
\eas
Whence $z_f$ is approximated as *check me*
\bas
% z_f &\approx \f{ (2 k^2 \mu + \beta z) \rho\dt + \rho^2}{  (\rho + \f{z\dt k}{ {\color{blue}2} \viscousCFL})k\dt }, \\
 z_f &\approx \f{ (2 k^2 \mu + \beta z) \rho\dt + \rho^2}{  (\rho k\dt + \f{\rho\, z\dt}{{\color{blue}2}\mu}) }
\eas
%
This can be simplified to
\bas
z_f &\approx \frac{2 k \mu + \beta \zb / k + \rho / (k \dt)}{1 + \zb / ({\red 2} k \mu)}\\
&=\frac{1}{1 + \zb / z_\mu} \left( z_\mu + \zb \sqrt{\frac{1}{\viscousCFL}+1} + z_\rho \right)\\
&=\frac{z_\mu}{z_\mu+\zb}(z_\mu +z_\rho) + \frac{\zb}{z_\mu +\zb} z_\mu \sqrt{\frac{1}{\Lambda_\nu}+1}
\eas
%
where
\bas
z_\mu = {\color{blue}2}\mu k, \qquad z_\rho = \frac{\rho}{k \dt}
\eas

We are looking for the fluid impedances
\bas
& z_f = \f{\mu}{\dy} \approx \text{ $\mu k$ or $\mu \beta$}, \\
& \hat{z}_f = \f{\mu\rho}{\zb\dt}  = \f{\mu}{\dy}\f{\rho\dy}{\zb\dt} = z_f \, \f{\rho}{\rhos} \, \f{\dy}{\cp\dt}
    = \f{z_f}{\zs} \f{\rho\dy}{\dt}
\eas
% or maybe
% \bas
% & z_f = \f{\mu\rho}{\zb \dt}\f{k}{\beta} = \f{\mu\rho}{\zb \dt}\f{k}{\sqrt{ \f{\rho}{\mu\dt} + k^2}}
% \eas


==> texFiles/stabilityNotesDan.tex <==
\section{Variational analysis}

\newcommand{\zr}{z_\rho}
\newcommand{\zm}{z_\mu}
\das{DAS: I went through the above work with some changes. First, 
  I considered a semi-infinite domain for the fluid (results agreed after taking 
  the limit when $e^{\beta H}$ is large). The second difference is I 
  considered the limits of $\Lambda$ before solving for $v_f$.}
Consider the geometry for the block elastic piston
and the following variational equations for the fluid velocity, $\vv = [u(y),v(y)]^T$, 
and pressure, $p(y)$.
\begin{align}
\rho \frac{u(y)}{\dt} + i k p(y) &= \mu (-k^2 u(y) + u''(y)), \\
\rho \frac{v(y)}{\dt} +  p'(y) &= \mu (-k^2 v(y) + v''(y)),  \\
i k u(y) + v'(y) &= 0.
\end{align}
%
Let $\beta^2 = k^2+\rho/ (\mu \dt).$
The solution which remains bounded as $y\rightarrow \infty$ is given by
\begin{align}
v(y) &= \left(v_f - \frac{k \dt p_f}{\rho} \right) e^{-\beta y} + \frac{k \dt p_f}{\rho} e^{-k y}, \\
p(y) &= p_f e^{-k y}, \\
u(y) &= -\frac{1}{i k} v'(y),
\end{align}
%
where $v_f$ is the vertical component of the velocity at the interface and $p_f$ is the pressure
at the interface. Assume that the incoming characteristics are known in the solid,
then the interface boundary conditions (with $\nv=[0,1]$) are
\begin{align}
-p + 2 \mu v'(0) - \zb v(0) &= \nv^T \bv_I, \\
\mu (u'(0) + i k v(0)) - \zb u(0) &= \tv^T \bv_I.
\end{align}
%
Substituting the fluid solution into the boundary conditions 
reveals a linear system of equations for $v_f$ and $p_f$, given by
\begin{align}
\left[\begin{array}{cc}
-\Gamma\zm - \zb
&
-1 + 2 \Lambda (\Gamma-1)
\\
i\left(\zr+\zm+ \Gamma\zb  \right)
&
-i \left( 1 +  2 \Lambda (\Gamma-1)  \zb/\zm \right)
\end{array}\right]
\left[\begin{array}{c} v_f \\ p_f \end{array}\right]
=
\left[\begin{array}{c} \nv^T \bv_I \\ \tv^T \bv_I \end{array}\right],
\end{align}
%
where
\begin{align}
\zm = 2 \mu k, 
\quad
\zr = \frac{\rho}{\dt k},
\quad
\Lambda = \frac{\mu k^2 \dt}{\rho},
\quad
\Gamma = \sqrt{\frac{1}{\Lambda}+1}.
\end{align}
%
$\zm$ and $\zr$ are fluid impedances and $\Lambda$ is a viscous CFL number.
We are interested in the limits when $\Lambda$ is large and small.
\begin{align}
\Gamma \sim 
\begin{cases}
1 + \frac{1}{2\Lambda}, & \Lambda \gg 1 \\
\frac{1}{\sqrt{\Lambda}}, & \Lambda \ll 1
\end{cases}
\end{align}
%
When we solve for $v_f,$ we expect the solution to be of the form,
\begin{align}
v_f = -\frac{1}{z + z_f} \nv^T \bv_I + C \tv^T \bv_I.
\label{eq:vf}
\end{align}
%
We are interested in $z_f.$

\subsection{Case 1: $\Lambda \gg 1$}

When $\Lambda \gg 1,$ the system becomes
\begin{align}
\left[\begin{array}{cc}
-\zm - \zb
&
0
\\
i\left(\zr+\zm+ \zb  \right)
&
-i \left( 1 + \zb/\zm \right)
\end{array}\right]
\left[\begin{array}{c} v_f \\ p_f \end{array}\right]
+ O\left( \frac{1}{\Lambda} \right)
=
\left[\begin{array}{c} \nv^T \bv_I \\ \tv^T \bv_I \end{array}\right].
\end{align}
%
The solution is
\begin{align}
v_f = - \frac{1}{\zm + \zb} \nv^T \bv_I + O\left( \frac{1}{\Lambda} \right).
\end{align}
%
By equating this to equation \eqref{eq:vf}, we obtain the following expression for
the fluid impedance.
\begin{align}
z_f \sim \zm
\end{align}

\subsection{Case 1: $\Lambda \ll 1$}

When $\Lambda \gg 1,$ the system becomes
\begin{align}
\left[\begin{array}{cc}
-\frac{\zm}{\sqrt{\Lambda}} - \zb
&
-1 
\\
i \frac{\zb}{\sqrt{\Lambda}}
+ i\left(\zr+\zm  \right)
&
-i
\end{array}\right]
\left[\begin{array}{c} v_f \\ p_f \end{array}\right]
+ O\left( \sqrt{\Lambda} \right)
=
\left[\begin{array}{c} \nv^T \bv_I \\ \tv^T \bv_I \end{array}\right].
\end{align}
%
The solution is
\begin{align}
v_f = -\frac{\sqrt{\Lambda}}{\zm+\zb} \left(\nv^T \bv_I + i \tv^T \bv_I \right)
+ O(\Lambda).
\end{align}
%
By equating this to equation \eqref{eq:vf}, we obtain the following expression for
the fluid impedance.
\begin{align}
z_f \sim \frac{\zm + \zb}{\sqrt{\Lambda}} + O(\sqrt{\Lambda})
\end{align}

\subsection{Arbitrary $\Lambda$}

% The following is a potential choice for $\zf$ which shares the same limiting behaviors
% as above.
% \begin{align}
% z_f = \frac{\zm}{1 - e^{-\sqrt{\Lambda}}} + \frac{\zb }{\sqrt{\Lambda}}e^{-\sqrt{\Lambda}}
% \end{align}
We are solving the system,
\begin{align}
\left[\begin{array}{cc}
a_{11} & a_{12} \\ a_{21} & a_{22}
\end{array}\right]
\left[\begin{array}{c}
v_f \\ p_f
\end{array}\right]
= \left[\begin{array}{c}
\nv^T \bv_I \\ \tv^T \bv_I
\end{array}\right].
\end{align}
%
The solutions is
\begin{align}
v_f &= \frac{a_{22}}{a_{11} a_{22} - a_{12} a_{21}} \nv^T \bv_I + ...
\end{align}
%
By matching coefficients we have
\begin{align}
\frac{1}{\zf+\zb} &= -\frac{a_{22}}{a_{11} a_{22} - a_{12} a_{21}} \\
\zf &= - a_{11} + \frac{a_{12} a_{21}}{a_{22}} - \zb \\
&= \Gamma \zm + \frac{(1 - 2 \Lambda (\Gamma-1) ) (\zr + \zm + \Gamma \zb)}
{1 + 2 \Lambda (\Gamma - 1) \zb / \zm} \\
&= \zm \left( \Gamma 
+ \frac{\zr + \zm + \Gamma \zb}{\zm + 2 \Lambda (\Gamma - 1) \zb} 
(1 - 2 \Lambda (\Gamma - 1))\right) \\
&= \zm \left( \Gamma 
+ \frac{\zr/ \zb + \zm / \zb + \Gamma }{\zm / \zb + 2 \Lambda (\Gamma - 1) } 
(1 - 2 \Lambda (\Gamma - 1) )\right)
\end{align}
%
% Side note: $\hat{z}_f$ is hidden in here
% \begin{align}
% \hat{z}_f = \frac{\zm \zr}{\zb} = 
% \frac{\left(2 \mu k \rho\right)  
% \left( \frac{\rho}{k \dt} \right)}{\zb}
% = \frac{2 \mu \rho}{\zb \dt}
% \end{align}
%
Note that $\zr$ can be written in terms of $\zm$ and $\Lambda.$
\begin{align}
\zr = \frac{\rho}{k \dt} = \frac{\rho}{k \rho \Lambda / (\mu k^2)}
= \frac{\mu}{h \Lambda} = \frac{\zm}{2 \Lambda}
\end{align}
%
Therefore we can write
\begin{align}
\zf &= \zm \left( \Gamma 
+ \frac{\zm/ (2 \Lambda \zb) + \zm / \zb + \Gamma }{\zm / \zb + 2 \Lambda (\Gamma - 1) } 
(1 - 2 \Lambda (\Gamma - 1) )\right).
\end{align}
%
Let $Z=\zm / \zb.$ Then the fluid impedance is equal to $\zm$ times a scale factor, 
$\eta(Z,\Lambda).$
\begin{align}
\zf &= \zm \eta(Z, \Lambda)
\end{align}
%
See figure \ref{fig:scaleFactor}.

\begin{figure}[h]
\includegraphics[width=\textwidth]{fig/zfScaleFactor}
\caption{Shaded contours of $\eta(Z,\Lambda)$ 
in the equation $\zf = \zm \eta(Z, \Lambda)$.
\label{fig:scaleFactor}}
\end{figure}



==> texFiles/tablesForZfMono.tex <==
\section{Stability tests will different $\zf_{\rm mono}$}

\begin{align}
\zf = \texttt{zfMono} \left(\frac{\mu}{h} + \frac{\rho h}{\dt}\right)
\end{align}

\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.5}{-3} &      & \num{3.2}{-2} &      & \num{1.8}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  8.8 & \num{4.9}{-4} &  3.7 & \num{3.6}{-4} & 12.4 & \num{7.5}{-3} &  4.3 & \num{1.9}{-5} &  9.8  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.7}{-5} &  4.2 & \num{9.0}{-4} &  8.3 & \num{4.5}{-6} &  4.2  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  4.0 & \num{2.5}{-5} &  4.2 & \num{2.3}{-5} &  3.8 & \num{3.1}{-4} &  2.9 & \num{4.4}{-7} & 10.1  \\ \hline
    rate             &       &  $2.41$       &      &  $2.07$       &      &  $2.49$       &      &  $2.32$       &      &  $2.82$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3NU0p05zfm0p5Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:51:10 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3NU0p05zfm0p5Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.3}{-2} &      & \num{1.3}{-2} &      & \num{4.6}{-4} &      & \num{5.9}{-3} &      & \num{5.4}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.6 & \num{1.3}{-3} &  9.9 & \num{1.1}{-4} &  4.0 & \num{1.4}{-3} &  4.3 & \num{1.5}{0} &  3.5  \\ \hline
                rep4 &     4 & \num{6.4}{-4} &  2.7 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.6}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{1.1}{-5} & 57.1 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.5 & \num{9.7}{-5} &  3.8 & \num{9.9}{-2} &  3.7  \\ \hline
    rate             &       &  $3.21$       &      &  $2.33$       &      &  $1.99$       &      &  $1.97$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3NU0p05zfm0p5Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:54:47 2018}\label{table:insElasticPiston.rep.AmpSCF1e3NU0p05zfm0p5Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.5}{-3} &      & \num{3.2}{-2} &      & \num{1.8}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  8.8 & \num{4.9}{-4} &  3.7 & \num{3.6}{-4} & 12.4 & \num{7.5}{-3} &  4.3 & \num{1.9}{-5} &  9.8  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.7}{-5} &  4.2 & \num{9.0}{-4} &  8.3 & \num{4.5}{-6} &  4.2  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  4.0 & \num{2.5}{-5} &  4.2 & \num{2.3}{-5} &  3.8 & \num{3.1}{-4} &  2.9 & \num{4.4}{-7} & 10.1  \\ \hline
    rate             &       &  $2.41$       &      &  $2.07$       &      &  $2.50$       &      &  $2.32$       &      &  $2.82$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Nov  3 00:02:07 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3NU0p05zfm1Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.3}{-2} &      & \num{1.3}{-2} &      & \num{4.6}{-4} &      & \num{5.9}{-3} &      & \num{5.4}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.6 & \num{1.3}{-3} &  9.9 & \num{1.1}{-4} &  4.0 & \num{1.4}{-3} &  4.3 & \num{1.5}{0} &  3.5  \\ \hline
                rep4 &     4 & \num{6.5}{-4} &  2.7 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.6}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{1.1}{-5} & 56.4 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.5 & \num{9.7}{-5} &  3.8 & \num{9.9}{-2} &  3.7  \\ \hline
    rate             &       &  $3.20$       &      &  $2.33$       &      &  $1.99$       &      &  $1.97$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Nov  3 00:05:52 2018}\label{table:insElasticPiston.rep.AmpSCF1e3NU0p05zfm1Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-3} &      & \num{1.8}{-3} &      & \num{4.5}{-3} &      & \num{3.2}{-2} &      & \num{1.8}{-4} &       \\ \hline
                rep2 &     2 & \num{1.8}{-4} &  8.8 & \num{4.9}{-4} &  3.7 & \num{3.6}{-4} & 12.4 & \num{7.5}{-3} &  4.3 & \num{1.9}{-5} &  9.8  \\ \hline
                rep4 &     4 & \num{4.0}{-5} &  4.5 & \num{1.0}{-4} &  4.7 & \num{8.7}{-5} &  4.2 & \num{9.0}{-4} &  8.3 & \num{4.5}{-6} &  4.2  \\ \hline
                rep8 &     8 & \num{1.0}{-5} &  4.0 & \num{2.5}{-5} &  4.2 & \num{2.3}{-5} &  3.8 & \num{3.1}{-4} &  2.9 & \num{4.4}{-7} & 10.1  \\ \hline
    rate             &       &  $2.41$       &      &  $2.07$       &      &  $2.50$       &      &  $2.32$       &      &  $2.82$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e-3NU0p05zfm2Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:56:39 2018}\label{table:insElasticPiston.rep.AmpSCF1e-3NU0p05zfm2Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.3}{-2} &      & \num{1.3}{-2} &      & \num{4.6}{-4} &      & \num{5.9}{-3} &      & \num{5.4}{0} &       \\ \hline
                rep2 &     2 & \num{1.8}{-3} &  7.6 & \num{1.3}{-3} & 10.0 & \num{1.1}{-4} &  4.0 & \num{1.4}{-3} &  4.3 & \num{1.5}{0} &  3.5  \\ \hline
                rep4 &     4 & \num{6.6}{-4} &  2.7 & \num{3.5}{-4} &  3.7 & \num{2.7}{-5} &  4.3 & \num{3.7}{-4} &  3.7 & \num{3.6}{-1} &  4.2  \\ \hline
                rep8 &     8 & \num{1.2}{-5} & 55.6 & \num{9.3}{-5} &  3.8 & \num{7.5}{-6} &  3.6 & \num{9.7}{-5} &  3.8 & \num{9.9}{-2} &  3.7  \\ \hline
    rate             &       &  $3.19$       &      &  $2.33$       &      &  $1.99$       &      &  $1.97$       &      &  $1.94$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1e3NU0p05zfm2Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Nov  3 00:00:23 2018}\label{table:insElasticPiston.rep.AmpSCF1e3NU0p05zfm2Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{7.0}{-3} &      & \num{1.1}{-2} &      & \num{1.5}{-3} &      & \num{9.4}{-3} &      & \num{1.3}{-2} &       \\ \hline
                rep2 &     2 & \num{8.5}{-4} &  8.3 & \num{1.7}{-3} &  6.6 & \num{7.7}{-5} & 18.9 & \num{1.6}{-3} &  5.8 & \num{1.1}{-3} & 11.8  \\ \hline
                rep4 &     4 & \num{2.5}{-4} &  3.4 & \num{4.0}{-4} &  4.2 & \num{1.8}{-5} &  4.2 & \num{3.9}{-4} &  4.2 & \num{3.3}{-4} &  3.4  \\ \hline
                rep8 &     8 & \num{6.2}{-5} &  4.1 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.8 & \num{9.9}{-5} &  3.9 & \num{8.7}{-5} &  3.9  \\ \hline
    rate             &       &  $2.22$       &      &  $2.23$       &      &  $2.68$       &      &  $2.18$       &      &  $2.36$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1NU0p05zfm0p5Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:53:01 2018}\label{table:insElasticPiston.rep.AmpSCF1NU0p05zfm0p5Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{6.6}{-3} &      & \num{1.1}{-2} &      & \num{1.3}{-3} &      & \num{9.9}{-3} &      & \num{1.1}{-2} &       \\ \hline
                rep2 &     2 & \num{8.6}{-4} &  7.7 & \num{1.7}{-3} &  6.4 & \num{7.1}{-5} & 17.9 & \num{1.6}{-3} &  6.1 & \num{1.1}{-3} &  9.8  \\ \hline
                rep4 &     4 & \num{2.6}{-4} &  3.3 & \num{3.9}{-4} &  4.2 & \num{1.8}{-5} &  4.0 & \num{3.8}{-4} &  4.2 & \num{3.4}{-4} &  3.4  \\ \hline
                rep8 &     8 & \num{6.5}{-5} &  4.0 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.7 & \num{9.9}{-5} &  3.9 & \num{8.9}{-5} &  3.8  \\ \hline
    rate             &       &  $2.17$       &      &  $2.22$       &      &  $2.61$       &      &  $2.20$       &      &  $2.26$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1NU0p05zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Sat Nov  3 00:04:07 2018}\label{table:insElasticPiston.rep.AmpSCF1NU0p05zfm1Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.0}{-2} &      & \num{1.1}{-2} &      & \num{1.2}{-3} &      & \num{1.0}{-2} &      & \num{1.1}{-2} &       \\ \hline
                rep2 &     2 & \num{8.5}{-4} & 12.0 & \num{1.7}{-3} &  6.7 & \num{7.0}{-5} & 17.6 & \num{1.6}{-3} &  6.4 & \num{1.1}{-3} &  9.6  \\ \hline
                rep4 &     4 & \num{2.7}{-4} &  3.2 & \num{3.9}{-4} &  4.2 & \num{1.8}{-5} &  3.9 & \num{3.8}{-4} &  4.2 & \num{3.4}{-4} &  3.3  \\ \hline
                rep8 &     8 & \num{6.7}{-5} &  4.0 & \num{1.0}{-4} &  3.9 & \num{4.9}{-6} &  3.7 & \num{9.9}{-5} &  3.9 & \num{9.1}{-5} &  3.7  \\ \hline
    rate             &       &  $2.35$       &      &  $2.24$       &      &  $2.60$       &      &  $2.22$       &      &  $2.24$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.AmpSCF1NU0p05zfm2Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.05 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=piston startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:58:28 2018}\label{table:insElasticPiston.rep.AmpSCF1NU0p05zfm2Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.5}{-6} &      & \num{1.3}{-5} &      & \num{1.4}{-3} &      & \num{4.3}{-3} &      & \num{1.1}{-5} &       \\ \hline
                rep2 &     2 & \num{1.4}{-7} & 10.6 & \num{2.2}{-6} &  6.0 & \num{4.1}{-4} &  3.3 & \num{1.4}{-3} &  3.2 & \num{3.0}{-6} &  3.7  \\ \hline
                rep4 &     4 & \num{1.5}{-8} &  9.5 & \num{5.4}{-7} &  4.0 & \num{1.0}{-4} &  4.0 & \num{3.2}{-4} &  4.3 & \num{7.0}{-7} &  4.3  \\ \hline
                rep8 &     8 & \num{1.9}{-9} &  7.8 & \num{1.5}{-7} &  3.6 & \num{2.6}{-5} &  3.9 & \num{8.0}{-5} &  4.0 & \num{1.7}{-7} &  4.0  \\ \hline
    rate             &       &  $3.21$       &      &  $2.13$       &      &  $1.91$       &      &  $1.94$       &      &  $2.01$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm0p5Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 22:44:57 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm0p5Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.2}{-6} &      & \num{9.9}{-6} &      & \num{5.3}{-6} &      & \num{6.3}{-6} &      & \num{4.6}{-2} &       \\ \hline
                rep2 &     2 & \num{6.4}{-7} & 12.8 & \num{2.5}{-6} &  3.9 & \num{1.2}{-6} &  4.4 & \num{2.2}{-6} &  2.9 & \num{1.1}{-2} &  4.4  \\ \hline
                rep4 &     4 & \num{3.5}{-7} &  1.8 & \num{5.8}{-7} &  4.3 & \num{2.7}{-7} &  4.4 & \num{6.1}{-7} &  3.6 & \num{2.4}{-3} &  4.5  \\ \hline
                rep8 &     8 & \num{7.9}{-8} &  4.4 & \num{1.4}{-7} &  4.2 & \num{6.4}{-8} &  4.3 & \num{1.7}{-7} &  3.6 & \num{5.5}{-4} &  4.3  \\ \hline
    rate             &       &  $2.10$       &      &  $2.07$       &      &  $2.12$       &      &  $1.75$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm0p5Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 22:56:27 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm0p5Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.5}{-6} &      & \num{1.3}{-5} &      & \num{1.4}{-3} &      & \num{4.3}{-3} &      & \num{1.1}{-5} &       \\ \hline
                rep2 &     2 & \num{1.4}{-7} & 10.6 & \num{2.2}{-6} &  6.0 & \num{4.1}{-4} &  3.3 & \num{1.4}{-3} &  3.2 & \num{3.0}{-6} &  3.7  \\ \hline
                rep4 &     4 & \num{1.5}{-8} &  9.5 & \num{5.4}{-7} &  4.0 & \num{1.0}{-4} &  4.0 & \num{3.2}{-4} &  4.3 & \num{7.0}{-7} &  4.3  \\ \hline
                rep8 &     8 & \num{1.9}{-9} &  7.8 & \num{1.5}{-7} &  3.6 & \num{2.6}{-5} &  3.9 & \num{8.0}{-5} &  4.0 & \num{1.7}{-7} &  4.0  \\ \hline
    rate             &       &  $3.21$       &      &  $2.13$       &      &  $1.91$       &      &  $1.94$       &      &  $2.01$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:22:11 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm1Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.2}{-6} &      & \num{9.9}{-6} &      & \num{5.3}{-6} &      & \num{6.3}{-6} &      & \num{4.6}{-2} &       \\ \hline
                rep2 &     2 & \num{6.4}{-7} & 12.9 & \num{2.5}{-6} &  3.9 & \num{1.2}{-6} &  4.4 & \num{2.2}{-6} &  2.9 & \num{1.1}{-2} &  4.4  \\ \hline
                rep4 &     4 & \num{3.5}{-7} &  1.8 & \num{5.8}{-7} &  4.3 & \num{2.7}{-7} &  4.4 & \num{6.1}{-7} &  3.6 & \num{2.4}{-3} &  4.5  \\ \hline
                rep8 &     8 & \num{7.9}{-8} &  4.4 & \num{1.4}{-7} &  4.2 & \num{6.4}{-8} &  4.3 & \num{1.7}{-7} &  3.6 & \num{5.5}{-4} &  4.3  \\ \hline
    rate             &       &  $2.10$       &      &  $2.07$       &      &  $2.12$       &      &  $1.74$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:36:42 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm1Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.5}{-6} &      & \num{1.3}{-5} &      & \num{1.4}{-3} &      & \num{4.3}{-3} &      & \num{1.1}{-5} &       \\ \hline
                rep2 &     2 & \num{1.4}{-7} & 10.6 & \num{2.2}{-6} &  6.0 & \num{4.1}{-4} &  3.3 & \num{1.4}{-3} &  3.1 & \num{3.0}{-6} &  3.7  \\ \hline
                rep4 &     4 & \num{1.5}{-8} &  9.5 & \num{5.4}{-7} &  4.0 & \num{1.0}{-4} &  4.0 & \num{3.2}{-4} &  4.3 & \num{7.0}{-7} &  4.3  \\ \hline
                rep8 &     8 & \num{1.9}{-9} &  7.8 & \num{1.5}{-7} &  3.6 & \num{2.6}{-5} &  3.9 & \num{8.0}{-5} &  4.0 & \num{1.7}{-7} &  4.0  \\ \hline
    rate             &       &  $3.21$       &      &  $2.13$       &      &  $1.91$       &      &  $1.94$       &      &  $2.01$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm2Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e-3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:02:18 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm2Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{8.2}{-6} &      & \num{9.9}{-6} &      & \num{5.3}{-6} &      & \num{6.3}{-6} &      & \num{4.6}{-2} &       \\ \hline
                rep2 &     2 & \num{6.3}{-7} & 13.0 & \num{2.5}{-6} &  3.9 & \num{1.2}{-6} &  4.4 & \num{2.2}{-6} &  2.9 & \num{1.1}{-2} &  4.4  \\ \hline
                rep4 &     4 & \num{3.5}{-7} &  1.8 & \num{5.8}{-7} &  4.3 & \num{2.7}{-7} &  4.4 & \num{6.1}{-7} &  3.5 & \num{2.4}{-3} &  4.5  \\ \hline
                rep8 &     8 & \num{7.9}{-8} &  4.4 & \num{1.4}{-7} &  4.2 & \num{6.4}{-8} &  4.3 & \num{1.7}{-7} &  3.6 & \num{5.5}{-4} &  4.3  \\ \hline
    rate             &       &  $2.10$       &      &  $2.07$       &      &  $2.12$       &      &  $1.74$       &      &  $2.13$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm2Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1e3, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:14:32 2018}\label{table:insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm2Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.2}{-6} &      & \num{6.1}{-6} &      & \num{1.9}{-6} &      & \num{1.1}{-5} &      & \num{1.5}{-5} &       \\ \hline
                rep2 &     2 & \num{1.6}{-7} &  7.4 & \num{1.7}{-6} &  3.7 & \num{3.8}{-7} &  5.0 & \num{4.4}{-6} &  2.6 & \num{2.3}{-6} &  6.4  \\ \hline
                rep4 &     4 & \num{3.4}{-8} &  4.6 & \num{4.0}{-7} &  4.1 & \num{8.8}{-8} &  4.3 & \num{1.1}{-6} &  4.1 & \num{4.5}{-7} &  5.1  \\ \hline
                rep8 &     8 & \num{4.0}{-9} &  8.3 & \num{9.6}{-8} &  4.2 & \num{2.0}{-8} &  4.3 & \num{2.6}{-7} &  4.2 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $2.67$       &      &  $2.00$       &      &  $2.17$       &      &  $1.85$       &      &  $2.34$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1NU0p1zfm0p5Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 22:50:41 2018}\label{table:insElasticPiston.rep.shearAmpSCF1NU0p1zfm0p5Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.8}{-6} &      & \num{5.7}{-6} &      & \num{1.9}{-6} &      & \num{1.2}{-5} &      & \num{1.4}{-5} &       \\ \hline
                rep2 &     2 & \num{1.8}{-7} & 10.2 & \num{1.7}{-6} &  3.4 & \num{3.8}{-7} &  5.0 & \num{4.4}{-6} &  2.7 & \num{2.2}{-6} &  6.2  \\ \hline
                rep4 &     4 & \num{3.4}{-8} &  5.2 & \num{4.0}{-7} &  4.2 & \num{8.8}{-8} &  4.3 & \num{1.1}{-6} &  4.1 & \num{4.5}{-7} &  5.0  \\ \hline
                rep8 &     8 & \num{4.0}{-9} &  8.4 & \num{9.6}{-8} &  4.2 & \num{2.0}{-8} &  4.3 & \num{2.6}{-7} &  4.2 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $2.88$       &      &  $1.97$       &      &  $2.17$       &      &  $1.86$       &      &  $2.32$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1NU0p1zfm1Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:29:48 2018}\label{table:insElasticPiston.rep.shearAmpSCF1NU0p1zfm1Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rep1 &     1 & \num{1.6}{-5} &      & \num{6.4}{-6} &      & \num{1.9}{-6} &      & \num{1.2}{-5} &      & \num{1.3}{-5} &       \\ \hline
                rep2 &     2 & \num{1.9}{-7} & 85.0 & \num{1.7}{-6} &  3.7 & \num{3.7}{-7} &  5.0 & \num{4.5}{-6} &  2.7 & \num{2.2}{-6} &  5.9  \\ \hline
                rep4 &     4 & \num{3.4}{-8} &  5.7 & \num{4.0}{-7} &  4.2 & \num{8.8}{-8} &  4.2 & \num{1.1}{-6} &  4.1 & \num{4.5}{-7} &  5.0  \\ \hline
                rep8 &     8 & \num{4.0}{-9} &  8.5 & \num{9.6}{-8} &  4.2 & \num{2.0}{-8} &  4.3 & \num{2.6}{-7} &  4.2 & \num{1.1}{-7} &  4.0  \\ \hline
    rate             &       &  $3.85$       &      &  $2.03$       &      &  $2.17$       &      &  $1.87$       &      &  $2.29$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rep.shearAmpSCF1NU0p1zfm2Imt0p6, $t=0.6$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=shear startCurve=spline -caseid=0 -amp=1e-05 Fri Nov  2 23:08:06 2018}\label{table:insElasticPiston.rep.shearAmpSCF1NU0p1zfm2Imt0p6}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.6}{-8} &      & \num{1.7}{-8} &      & \num{6.0}{-9} &      & \num{2.0}{-8} &      & \num{5.7}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.7}{-8} &  2.2 & \num{4.9}{-9} &  3.5 & \num{1.2}{-9} &  4.9 & \num{4.9}{-9} &  4.1 & \num{1.5}{-8} &  3.9  \\ \hline
                rtw8 &     4 & \num{3.4}{-9} &  4.9 & \num{1.1}{-9} &  4.4 & \num{2.7}{-10} &  4.6 & \num{1.1}{-9} &  4.4 & \num{4.5}{-9} &  3.3  \\ \hline
               rtw16 &     8 & \num{8.5}{-10} &  4.0 & \num{2.8}{-10} &  4.0 & \num{6.3}{-11} &  4.3 & \num{2.7}{-10} &  4.1 & \num{1.0}{-9} &  4.5  \\ \hline
    rate             &       &  $1.85$       &      &  $1.99$       &      &  $2.19$       &      &  $2.08$       &      &  $1.93$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm0p5Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-7 Sat Nov  3 01:07:56 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm0p5Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.6}{-8} &      & \num{1.7}{-8} &      & \num{6.0}{-9} &      & \num{2.0}{-8} &      & \num{5.7}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.7}{-8} &  2.2 & \num{4.9}{-9} &  3.5 & \num{1.2}{-9} &  4.9 & \num{4.9}{-9} &  4.1 & \num{1.5}{-8} &  3.9  \\ \hline
                rtw8 &     4 & \num{3.4}{-9} &  4.9 & \num{1.1}{-9} &  4.4 & \num{2.7}{-10} &  4.6 & \num{1.1}{-9} &  4.4 & \num{4.5}{-9} &  3.3  \\ \hline
               rtw16 &     8 & \num{8.5}{-10} &  4.0 & \num{2.8}{-10} &  4.0 & \num{6.3}{-11} &  4.3 & \num{2.7}{-10} &  4.1 & \num{1.0}{-9} &  4.5  \\ \hline
    rate             &       &  $1.85$       &      &  $1.99$       &      &  $2.19$       &      &  $2.08$       &      &  $1.93$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-7 Sat Nov  3 08:23:50 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{3.6}{-8} &      & \num{1.7}{-8} &      & \num{6.0}{-9} &      & \num{2.0}{-8} &      & \num{5.7}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.7}{-8} &  2.2 & \num{4.9}{-9} &  3.5 & \num{1.2}{-9} &  4.9 & \num{4.9}{-9} &  4.1 & \num{1.5}{-8} &  3.9  \\ \hline
                rtw8 &     4 & \num{3.4}{-9} &  4.9 & \num{1.1}{-9} &  4.4 & \num{2.7}{-10} &  4.6 & \num{1.1}{-9} &  4.4 & \num{4.5}{-9} &  3.3  \\ \hline
               rtw16 &     8 & \num{8.5}{-10} &  4.0 & \num{2.8}{-10} &  4.0 & \num{6.3}{-11} &  4.3 & \num{2.7}{-10} &  4.1 & \num{1.0}{-9} &  4.5  \\ \hline
    rate             &       &  $1.85$       &      &  $1.99$       &      &  $2.19$       &      &  $2.08$       &      &  $1.93$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm2Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=0 -amp=1e-7 Sat Nov  3 05:18:38 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm2Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{5.6}{-8} &      & \num{3.1}{-8} &      & \num{4.3}{-8} &      & \num{3.4}{-7} &      & \num{4.6}{-8} &       \\ \hline
                rtw4 &     2 & \num{8.8}{-9} &  6.3 & \num{9.2}{-9} &  3.4 & \num{6.0}{-9} &  7.1 & \num{6.7}{-8} &  5.0 & \num{8.6}{-9} &  5.3  \\ \hline
                rtw8 &     4 & \num{2.0}{-9} &  4.3 & \num{2.4}{-9} &  3.8 & \num{1.3}{-9} &  4.6 & \num{1.6}{-8} &  4.2 & \num{2.3}{-9} &  3.8  \\ \hline
               rtw16 &     8 & \num{5.1}{-10} &  4.0 & \num{6.6}{-10} &  3.6 & \num{3.0}{-10} &  4.3 & \num{3.9}{-9} &  4.1 & \num{5.6}{-10} &  4.1  \\ \hline
    rate             &       &  $2.24$       &      &  $1.86$       &      &  $2.36$       &      &  $2.13$       &      &  $2.10$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm0p5Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=7 -amp=1e-7 Sat Nov  3 00:08:48 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm0p5Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{5.6}{-8} &      & \num{3.1}{-8} &      & \num{4.3}{-8} &      & \num{3.4}{-7} &      & \num{4.6}{-8} &       \\ \hline
                rtw4 &     2 & \num{8.8}{-9} &  6.3 & \num{9.2}{-9} &  3.4 & \num{6.0}{-9} &  7.1 & \num{6.7}{-8} &  5.0 & \num{8.6}{-9} &  5.3  \\ \hline
                rtw8 &     4 & \num{2.0}{-9} &  4.3 & \num{2.4}{-9} &  3.8 & \num{1.3}{-9} &  4.6 & \num{1.6}{-8} &  4.2 & \num{2.3}{-9} &  3.8  \\ \hline
               rtw16 &     8 & \num{5.1}{-10} &  4.0 & \num{6.6}{-10} &  3.6 & \num{3.0}{-10} &  4.3 & \num{3.9}{-9} &  4.1 & \num{5.6}{-10} &  4.1  \\ \hline
    rate             &       &  $2.24$       &      &  $1.86$       &      &  $2.36$       &      &  $2.13$       &      &  $2.10$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=7 -amp=1e-7 Sat Nov  3 07:40:16 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{5.6}{-8} &      & \num{3.1}{-8} &      & \num{4.3}{-8} &      & \num{3.4}{-7} &      & \num{4.6}{-8} &       \\ \hline
                rtw4 &     2 & \num{8.8}{-9} &  6.3 & \num{9.2}{-9} &  3.4 & \num{6.0}{-9} &  7.1 & \num{6.7}{-8} &  5.0 & \num{8.6}{-9} &  5.3  \\ \hline
                rtw8 &     4 & \num{2.0}{-9} &  4.3 & \num{2.4}{-9} &  3.8 & \num{1.3}{-9} &  4.6 & \num{1.6}{-8} &  4.2 & \num{2.3}{-9} &  3.8  \\ \hline
               rtw16 &     8 & \num{5.1}{-10} &  4.0 & \num{6.6}{-10} &  3.6 & \num{3.0}{-10} &  4.3 & \num{3.9}{-9} &  4.1 & \num{5.6}{-10} &  4.1  \\ \hline
    rate             &       &  $2.24$       &      &  $1.86$       &      &  $2.36$       &      &  $2.13$       &      &  $2.10$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm2Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=0.1, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=7 -amp=1e-7 Sat Nov  3 04:00:51 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm2Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{1.9}{-8} &      & \num{1.4}{-8} &      & \num{9.2}{-10} &      & \num{6.3}{-9} &      & \num{8.9}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.4}{-8} &  1.3 & \num{3.7}{-9} &  3.7 & \num{2.5}{-10} &  3.7 & \num{2.0}{-9} &  3.2 & \num{3.2}{-8} &  2.8  \\ \hline
                rtw8 &     4 & \num{3.3}{-9} &  4.4 & \num{8.8}{-10} &  4.2 & \num{5.7}{-11} &  4.4 & \num{5.3}{-10} &  3.8 & \num{1.1}{-8} &  3.0  \\ \hline
               rtw16 &     8 & \num{8.1}{-10} &  4.1 & \num{2.3}{-10} &  3.9 & \num{1.3}{-11} &  4.4 & \num{1.4}{-10} &  3.9 & \num{2.2}{-9} &  4.7  \\ \hline
    rate             &       &  $1.57$       &      &  $1.99$       &      &  $2.06$       &      &  $1.85$       &      &  $1.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm0p5Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=0.5 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=8 -amp=1e-7 Sat Nov  3 02:34:45 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm0p5Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{1.9}{-8} &      & \num{1.4}{-8} &      & \num{9.2}{-10} &      & \num{6.3}{-9} &      & \num{8.9}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.4}{-8} &  1.3 & \num{3.7}{-9} &  3.7 & \num{2.5}{-10} &  3.7 & \num{2.0}{-9} &  3.2 & \num{3.2}{-8} &  2.8  \\ \hline
                rtw8 &     4 & \num{3.3}{-9} &  4.4 & \num{8.8}{-10} &  4.2 & \num{5.7}{-11} &  4.4 & \num{5.3}{-10} &  3.8 & \num{1.1}{-8} &  3.0  \\ \hline
               rtw16 &     8 & \num{8.1}{-10} &  4.1 & \num{2.3}{-10} &  3.9 & \num{1.3}{-11} &  4.4 & \num{1.4}{-10} &  3.9 & \num{2.2}{-9} &  4.7  \\ \hline
    rate             &       &  $1.57$       &      &  $1.99$       &      &  $2.06$       &      &  $1.85$       &      &  $1.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=1 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=8 -amp=1e-7 Sat Nov  3 09:02:05 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm1Imt0p3}
\end{center}
\end{table}
\begin{table}[H]\tableFont % you should set \tableFont to \footnotesize or other size
% \newcommand{\num}[2]{#1e{#2}} % use this command to set the format of numbers in the table.
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|} \hline 
grid  &    N &   $p$   & r &     $\vv$    & r &    $\usv$   & r &     $\vsv$   & r &   $\sigmavs$  & r \\ \hline 
                rtw2 &     1 & \num{1.9}{-8} &      & \num{1.4}{-8} &      & \num{9.2}{-10} &      & \num{6.3}{-9} &      & \num{8.9}{-8} &       \\ \hline
                rtw4 &     2 & \num{1.4}{-8} &  1.3 & \num{3.7}{-9} &  3.7 & \num{2.5}{-10} &  3.7 & \num{2.0}{-9} &  3.2 & \num{3.2}{-8} &  2.8  \\ \hline
                rtw8 &     4 & \num{3.3}{-9} &  4.4 & \num{8.8}{-10} &  4.2 & \num{5.7}{-11} &  4.4 & \num{5.3}{-10} &  3.8 & \num{1.1}{-8} &  3.0  \\ \hline
               rtw16 &     8 & \num{8.1}{-10} &  4.1 & \num{2.3}{-10} &  3.9 & \num{1.3}{-11} &  4.4 & \num{1.4}{-10} &  3.9 & \num{2.2}{-9} &  4.7  \\ \hline
    rate             &       &  $1.57$       &      &  $1.99$       &      &  $2.06$       &      &  $1.85$       &      &  $1.75$       &       \\ \hline
\end{tabular}
\caption{MP, insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm2Imt0p3, $t=0.3$, AM=1, cfl=0.9, nu=0.1 CgSm=SM-Godunov,Cgins=im, tz=none, scf=10, rhoSolid=1 sm-diss=0.5, useImplicitAmpBCs=1 numberOfCorrections=1 useExactPressureBC=0 -stressRelaxation=4 cdv=1 cDt= setGhostByExtrapolation=1 zfOption=m zfMuByH=1 zfRhoHByDt=0 \das{zfMono}=2 dtMax=1e+20 (coarsest grid) known=radialTravelingWave startCurve=spline -caseid=8 -amp=1e-7 Sat Nov  3 06:36:35 2018}\label{table:insElasticPiston.rtw.radialTravelingWaveAmpCaseid8SCF10NU0p1zfm2Imt0p3}
\end{center}
\end{table}


==> texFiles/tablesStressJumpTerms.tex <==
\section{Convergence tests with stress jump terms in fluid}
\input tables/12_03_18/insElasticPiston.epgp.AmpSCF1e-3NU0p05zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.epgp.AmpSCF1e3NU0p05zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.epgp.AmpSCF1NU0p05zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.epgp.shearAmpSCF1e-3NU0p1zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.epgp.shearAmpSCF1e3NU0p1zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.epgp.shearAmpSCF1NU0p1zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.rep.AmpSCF1e-3NU0p05zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.rep.AmpSCF1e3NU0p05zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.rep.AmpSCF1NU0p05zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.rep.shearAmpSCF1e-3NU0p1zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.rep.shearAmpSCF1e3NU0p1zfm1Imt0p6.ConvTable.tex
\input tables/12_03_18/insElasticPiston.rep.shearAmpSCF1NU0p1zfm1Imt0p6.ConvTable.tex
\input tables/12_04_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid0SCF1NU0p1zfm1Imt0p3.ConvTable.tex
\input tables/12_04_18/insElasticPiston.rtw.radialTravelingWaveAmpCaseid7SCF0p1NU0p1zfm1Imt0p3.ConvTable.tex


==> texFiles/thinPlateInAChannel.tex <==
\clearpage
\subsection{Thin plate in a channel} \label{sec:thinPlateInAChannel}

DAS 8/19/18: Interesting example. Vibrations of a thin plate in a channel.
Note, $z_f = \mu/h$ failed here. The viscous CFL number is small due to the tiny grid 
spacing in the solid and small $\nu=.05.$ The monolithic $z_f$ works here. 

{
\begin{figure}[h]
\centering
\includegraphics[width=.4\textwidth]{fig/thinPlate/thinPlateGrid.png}
\end{figure}
}

{
\begin{figure}[h]
\centering
\includegraphics[width=.24\textwidth]{fig/thinPlate/thinPlatet0.png}
\includegraphics[width=.24\textwidth]{fig/thinPlate/thinPlatet10.png}
\includegraphics[width=.24\textwidth]{fig/thinPlate/thinPlatet20.png}
\includegraphics[width=.24\textwidth]{fig/thinPlate/thinPlatet30.png}
\caption{
Solution at $t=0,10,20,$ and $30$.
$\delta=1000, z_f = 30 \mu / h$, $z_f$ factor chosen to agree with monolithic $z_f$.}
\end{figure}
}

% cgmp solidDiskInAChannel -method=ins -smVariation=g  -g=thinRotatedx25PlateGride2.order2  -addedMass=1 -scf=1000. -zfMuByH=30 -zfMono=0. -tp=.01 -tf=31. -tsINS=im -useImplicitAmpBCs=1 -nc=1 -nu=.05 -pOffset=.0  -diss=.5 -debug=1 -rampedInflow=1 -flushFrequency=4 -multiDomainAlgorithm=1 -cfl=.9 -setGhostByExtrapolation=1 -go=halt -p0=10 -tb=.3 -show=./thinPlate_08_19/thinPlateScf1000x25.show
